Stability Based Generalization Bounds for Exponential Family Langevin Dynamics

Recent years have seen advances in generalization bounds for noisy stochastic algorithms, especially stochastic gradient Langevin dynamics (SGLD) based on stability (Mou et al., 2018; Li et al., 2020) and information theoretic approaches (Xu and Raginsky, 2017; Negrea et al., 2019; Steinke and Zakynthinou, 2020). In this paper, we unify and substantially generalize stability based generalization bounds and make three technical contributions. First, we bound the generalization error in terms of expected (not uniform) stability which arguably leads to quantitatively sharper bounds. Second, as our main contribution, we introduce Exponential Family Langevin Dynamics (EFLD), a substantial generalization of SGLD, which includes noisy versions of Sign-SGD and quantized SGD as special cases. We establish data-dependent expected stability based generalization bounds for any EFLD algorithm with a O(1/n) sample dependence and dependence on gradient discrepancy rather than the norm of gradients, yielding significantly sharper bounds. Third, we establish optimization guarantees for special cases of EFLD. Further, empirical results on benchmarks illustrate that our bounds are non-vacuous, quantitatively sharper than existing bounds, and behave correctly under noisy labels.

==> Arxiv(old)/app/exp.tex <==


%\subsection{Preliminary}
We introduce preliminary of exponential family for the analysis. We will use both the natural and expectation parameterization form. Let $\hat{\btheta}_{\sigma} = \btheta/(\alpha)$, and the mean parameter $\hat{\m}_{\sigma} = \nabla_{\hat{\btheta}_{\sigma}} \psi(\hat{\btheta}_{\sigma})$. In our settings, the mean parameter for distribution on batch $B$ is $\m_B = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t})$ so we use $\hat{\m}_{B,\sigma},\hat{\m}'_{B',\sigma}$ to denote $\m_B,\m'_B$ respectively. 
For ease of computation, we denote $\m_{\sigma}$ as the natural gradient: $\m_{\sigma} := \nabla_{\btheta} \psi(\btheta/(\alpha)) = \hat{\m}_{\sigma}/(\alpha)$, and similarly we have $\nabla_{\btheta}^2 \psi(\btheta/(\alpha)) = \nabla_{\btheta/(\alpha)}^2 \psi(\btheta/(\alpha))/(\alpha^2)$. Further, $\btheta/(\alpha) = \nabla \psi^{-1}(\m_{\sigma}) = \nabla \phi_{\sigma}(\m_{\sigma})$. 
% Then, 
% \begin{align*}
% \langle \bxi, \btheta/(\alpha) \rangle - \psi(\btheta/(\alpha)) 
% & = \langle \m_{\sigma}, \btheta/(\alpha) \rangle - \psi(\btheta/(\alpha)) + \langle \bxi - \m_{\sigma}, \btheta/(\alpha) \rangle~\\
% & = \phi(\m_{\sigma}) + \langle \bxi - \m_{\sigma}, \nabla \phi(\m_{\sigma}) \rangle \\
% & = - d_{\phi}(\bxi, \m_{\sigma}) + \phi(\bxi)~.
% \end{align*}
Further, since $\psi$ is strongly convex and smooth, so is $\phi$ by Legendre duality, and there are strongly convex constant $c_1$ and Lipschitz smooth constant $c_2$, where $c_1 \leq c_2$ such that
\begin{equation*}
    c_1 \| \bxi - \m \|_2^2 \leq d_{\phi_\sigma}(\bxi,\m) \leq c_2 \| \bxi - \m \|_2^2~,
\end{equation*}
for any $\bxi,\m$ in the domain $\Theta$, any $\sigma\in \Omega$. From the definition of $d_{\phi_\sigma}$:
\begin{equation}
    d_{\phi_\sigma}(\bxi,\m) = \phi_\sigma(\bxi)-\phi_\sigma(\m)-\langle \bxi - \m, \nabla \phi_\sigma (\m)\rangle,
\end{equation}
the strongly convexity and Lipschitz smoothness on $d_{\phi_\sigma}$ implies $\phi_{\sigma}$ is strongly convex and Lipschitz smooth. By duality, we have $\psi$ is strongly convex and Lipschitz smooth  [see Theorem 6 in \cite{kakade2009duality}]:
\begin{equation}
    \frac{1}{4c_2} \| \bxi - \btheta\|_2^2 \leq d_{\psi}(\bxi,\btheta) \leq \frac{1}{4c_1} \| \bxi - \btheta \|_2^2.
\end{equation}


%We further assume that the base measure $\pi_0(\xi_j) \leq 1, j=1,\ldots,p$, \abcomment{may not be necessary} which is satisfied by many 


Following the earlier analysis, by mean-value theorem, for some $\tilde{\btheta}_B = \alpha_x \btheta_B + (1-\alpha_x) \btheta'_B$, $\alpha_x \in [0,1]$, our goal is to bound:
\begin{align}
I_{A,B} &=  \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \nabla_{\btheta}p_{\tilde{\btheta}_B,\sigma}\rangle ^2}{p_{\btheta_A,\sigma}} d\bxi = \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha)\rangle ^2p_{\tilde{\btheta}_B,\sigma}^2}{\alpha^2 p_{\btheta_A,\sigma}} d\bxi 
% \\
% &\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\tilde{\btheta}_B/\alpha) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi~.
\label{eq:expcore}
\end{align}



% \subsection{Step 1}
% Our goal in this step is to prove the following lemma:
% \begin{lemm}\label{lemm:exp_step1}
% For some $\tilde{\btheta}_B = \alpha_x \btheta_B + (1-\alpha_x) \btheta'_B$, $\alpha_x \in [0,1]$, we have
% \begin{equation}
%     \left\| \nabla \psi(\tilde{\btheta}_B/\alpha) \right\|_2^2\leq \left\| \nabla \psi(\btheta_B/\alpha) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/\alpha) \right\|_2^2.
% \end{equation}
% \end{lemm}

% \proof
% Since $p_{\btheta,\sigma}(\bxi)$ is a product of marginal exponential families, $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$, so that the $j$-th component of the gradient $\nabla \psi(\theta)$ is $\nabla_j \psi(\theta) = \psi'_j(\theta_j)$, where $\psi'_j(\theta_j)$ denotes the derivative of $\psi_j(\theta_j)$. Noting that $\psi'_j$ is a monotonic function since $\psi_j$ is convex, we have
% \begin{align*}
% \left\| \nabla \psi(\tilde{\theta}_B/\alpha) \right\|_2^2 & = \sum_{j=1}^p \left| \psi'_j(\tilde{\theta}_{j,B}/\alpha) \right|^2 \\
% & \stackrel{(a)}{\leq} \sum_{j=1}^p \max\left\{ \left| \psi'_j(\theta_{j,B}/\alpha) \right|^2, \left| \psi'_j(\theta'_{j,B}/\alpha) \right|^2 \right\} \\
% & \leq \sum_{j=1}^p \left\{ \left| \psi'_j(\btheta_{j,B}/\alpha) \right|^2 + \left| \psi'_j(\btheta'_{j,B}/\alpha) \right|^2 \right\} \\
% & = \left\| \nabla \psi(\btheta_B/\alpha) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/\alpha) \right\|_2^2
% \end{align*}
% where (a) follows since $\tilde{\theta}_{j,B} \in ~\text{int}(\theta_{j,B},\theta'_{j,B})$\footnote{We use int$(a,b)$ to denote $[a,b]$ or $[b,a]$, depending on their ordering.} and $\psi'_j$ is monotonic, $\psi'_j(\tilde{\theta}_{j,B}) \in~\text{int}(\psi'_j(\theta_{j,B}),\psi'_j(\theta'_{j,B}))$, which completes the proof. \qed

\subsection{Distributional Dependency on $\tilde{\btheta}_B$}
Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. In this step we focus on bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$. 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/\alpha) \right]}{\exp(\langle \bxi, \btheta_A/\alpha \rangle - \psi(\btheta_A/\alpha))} \pi_0(\bxi) ~.
% \end{align*}



\begin{lemm}\label{lemm:exp_step2}
For some $\alpha_{\bxi} \in [0,1]$, $\tilde{\btheta} = \alpha_{\bxi} \btheta_B + (1-\alpha_{\bxi}) \btheta'_B$, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \alpha \rangle - \psi(\tilde{\btheta}_B/\alpha) \right]}{ \exp\left[\langle \bxi, \btheta_B / \alpha \rangle - \psi(\btheta_B/\alpha) \right] + \exp\left[\langle \bxi, \btheta'_B / \alpha \rangle - \psi(\btheta'_B/\alpha) \right] }
\leq \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right] ~.
\end{align*}
\end{lemm}
\proof Denoting $\alpha_{\bxi}$ as $\alpha$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
\begin{align*}
\langle \bxi, & \tilde{\btheta}_B / \alpha \rangle  - \psi(\tilde{\btheta}_B/\alpha) 
 = \langle \bxi, \alpha \btheta_B/ \alpha + (1-\alpha) \btheta'_B/ 2 \sigma^2 \rangle - \psi\left( \alpha \btheta_B/ 2 \sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \right) \\
& = \alpha \bigg[ \langle \bxi , \btheta_B / 2 \sigma^2 \rangle - \psi(\btheta_B/ 2 \sigma^2) \bigg]  + (1-\alpha) \bigg[ \langle \bxi , \btheta'_B /2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2) \bigg] \\
& ~~~~~~~~~~~~~~~
  + \bigg[ \alpha \psi(\btheta_B/ \alpha ) + (1-\alpha) \psi(\btheta'_B/2 \sigma^2) - \psi( \alpha \btheta_B/\alpha + (1-\alpha) \btheta'_B/\alpha ) \bigg] \\
& \stackrel{(a)}{\leq} \max\bigg[ \langle \bxi , \btheta_B/ \alpha \rangle - \psi(\btheta_B/2 \sigma^2) , \langle \bxi , \btheta'_B / 2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2 )  \bigg] \\
& ~~~~~~~~~~~~~~~ 
  + \bigg[ \alpha d_{\psi}(\btheta_B/\alpha, \tilde{\btheta}_B/\alpha) + (1-\alpha) d_{\psi}(\btheta'_B/\alpha , \tilde{\btheta}_B/\alpha) \bigg]~,
\end{align*}
where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation (See section 3.1.1 in \cite{banerjee2005clustering}).
Now, note that
\begin{align*}
\alpha d_{\psi}(\btheta_B/\alpha, \tilde{\btheta}_B/\alpha)  + (1-\alpha) d_{\psi}(\btheta'_B/\alpha, \tilde{\btheta}_B/\alpha)  
& \leq \alpha d_{\psi}(\btheta_B/\alpha, \btheta'_B/\alpha) + (1-\alpha) d_{\psi}(\btheta'_B/\alpha, \btheta_B/\alpha) \\
& \stackrel{(a)}{=} \alpha d_{\phi}(\m'_{\sigma}, \m_{\sigma}) + (1-\alpha) d_{\phi}(\m_{\sigma},\m'_{\sigma})~\\
& \leq \alpha c_2 \| \m'_{\sigma} - \m_{\sigma} \|_2^2 + (1-\alpha) c_2 \| \m_{\sigma} - \m'_{\sigma} \|_2^2 \\
& \leq \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2~,
\end{align*}
where (a) follows by duality.
As a result,
\begin{align*}
& \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \alpha \rangle - \psi(\tilde{\btheta}_B/\alpha) \right]}{ \exp\left[\langle \bxi, \btheta_B / \alpha \rangle - \psi(\btheta_B/\alpha) \right] + \exp\left[\langle \bxi, \btheta'_B / \alpha \rangle - \psi(\btheta'_B/\alpha) \right] }\\
& ~~~~~ \leq\exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right]
\frac{ \exp \left[ \max\bigg[ \langle \bxi , \btheta_B \rangle - \psi(\btheta_B) , \langle \bxi , \btheta'_B \rangle - \psi(\btheta'_B)  \bigg] \right] }{ \exp\left[\langle \bxi, \btheta_B / \alpha \rangle - \psi(\btheta_B/\alpha) \right] + \exp\left[\langle \bxi, \btheta'_B / \alpha \rangle - \psi(\btheta'_B/\alpha) \right] } \\
& ~~~~~ \leq \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right]~.
\end{align*}
That completes the proof.\qed 

\subsection{Bounding the Density Ratio}
Focusing on density ratio, we have
\begin{lemm}\label{lemm:exp_step3}
For any $\bxi$, we have
\begin{align*}
&\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/\alpha) \right] }{\exp\left[\langle \bxi, \btheta_A / \alpha \rangle - \psi(\btheta_A/\alpha) \right]}\\
&\leq \exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \psi( (2\btheta_B - \btheta_A)/\alpha) \right].
\end{align*}

\end{lemm}

\proof
% \begin{align*}
% & \frac{\left(\exp\left[\langle \bxi, \tilde{\btheta}_B / \alpha \rangle - \psi(\tilde{\btheta}_B/\alpha) \right] \right)^2 }{\exp(\langle \bxi, \btheta_A/\alpha \rangle - \psi(\btheta_A/\alpha))} \pi_0(\bxi)
% = \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/\alpha) \right]}{\exp(\langle \bxi, \btheta_A/\alpha \rangle - \psi(\btheta_A/\alpha))} \pi_0(\bxi) \\
% & ~~~ \leq 2 \exp \left[ \frac{c_2}{2\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B,\sigma} \|_2^2 \right] \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/\alpha) \right] + \exp\left[\langle \bxi, \btheta'_B / \sigma^2 \rangle - 2\psi(\btheta'_B/\alpha) \right]}{\exp(\langle \bxi, \btheta_A/\alpha \rangle - \psi(\btheta_A/\alpha))} \pi_0(\bxi) ~.
% \end{align*}
Note that
\begin{align*}
\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/\alpha) \right] }{\exp\left[\langle \bxi, \btheta_A / \alpha \rangle - \psi(\btheta_A/\alpha) \right]}  
& = \exp\left[ \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \big( 2\psi(\btheta_B/\alpha) - \psi(\btheta_A/\alpha) \big) \right] \\
& = \beta_{B,A,\sigma} \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \psi( (2\btheta_B - \btheta_A)/\alpha) \right]~,
\end{align*}
where
\begin{align*}
\beta_{B,A,\sigma} & = \exp \left[ \psi( (2\btheta_B - \btheta_A)/\alpha) - \big( 2\psi(\btheta_B/\alpha) - \psi(\btheta_A/\alpha) \big) \right] ~.
\end{align*}
Note that
\begin{align*}
\log \beta_{B,A,\sigma} & = \psi( (2\btheta_B - \btheta_A)/\alpha) - \big( 2\psi(\btheta_B/\alpha) - \psi(\btheta_A/\alpha) \big)\\
& = - \bigg( \psi(\btheta_B/\alpha) - \psi( (2\btheta_B - \btheta_A)/\alpha) \bigg) - \bigg( \psi(\btheta_B/\alpha) - \psi(\btheta_A/\alpha) \bigg) \\
& \stackrel{(a)}{\leq} \bigg\langle (\btheta_B - \btheta_A)/\alpha, \nabla \psi( (2\btheta_B - \btheta_A)/\alpha) /\alpha \bigg\rangle + \bigg\langle (\btheta_A - \btheta_B)/\alpha, \nabla \psi( \btheta_A/\alpha) /\alpha \bigg\rangle   \\
& = \bigg\langle (\btheta_B - \btheta_A)/\alpha, \nabla \psi( (2\btheta_B - \btheta_A)/\alpha) - \nabla \psi(\btheta_A/\alpha)  \bigg\rangle /\alpha \\
& \stackrel{(b)}{=} \bigg( d_{\psi}(\btheta_B/\alpha, \btheta_A/\alpha) + d_{\psi}(\btheta_A/\alpha , (2 \btheta_B - \btheta_A)/2\sigma_A^2 ) - d_{\psi}(\btheta_B/\alpha, (2 \btheta_B - \btheta_A)/\alpha \bigg) / 2 \sigma^2 \\
& \leq \big( 1/c_1 \| \btheta_B - \btheta_A \|_2^2 + 1/c_1 \| \btheta_A - (2\btheta_B - \btheta_A) \|_2^2 - 1/c_2 \| \btheta_B - (2\btheta_B - \btheta_A) \|_2^2 \big) / 8 \sigma^6 \\
& = (3/c_1 - 1/c_2) \| \btheta_B/\alpha - \btheta_A/\alpha \|_2^2 / 2 \sigma^2~,
\end{align*}
where (a) follows from the convexity of $\psi$, and (b) follows from the three-point property of Bregman divergences [See Appendix A, property 8 in \cite{banerjee2005clustering}] given by
\begin{equation*}
\langle \x_1 - \x_2, \nabla \psi(\x_3) - \nabla \psi(\x_2) \rangle = d_{\psi}(\x_1,\x_2) + d_{\psi}(\x_2,\x_3) - d_{\psi}(\x_1,\x_3) ~,
\end{equation*}
with $\x_1 = \btheta_B/\alpha, \x_2 = \btheta_A/\alpha, \x_3 = (2\btheta_B - \btheta_A)/\alpha$.
Since $\phi$ is smooth, we also have
\begin{align*}
\| \btheta_B/\alpha - \btheta_A/\alpha \|_2^2 & = \| \nabla \phi( \m_{B,\sigma} ) - \nabla \phi (\m_{A,\sigma}) \|_2^2 \leq  c_2^2 \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 = \frac{c_2^2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 ~,
\end{align*}
we have 
\begin{align*}
&\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/\alpha) \right] }{\exp\left[\langle \bxi, \btheta_A / \alpha \rangle - \psi(\btheta_A/\alpha) \right]}\\
&\leq \exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \psi( (2\btheta_B - \btheta_A)/\alpha) \right]~,
\end{align*}
which completes the proof.\qed

The analysis for the term involving $\btheta'_B$ is similar. 

\subsection{Putting Everything Together}


% Note that we have managed to bound the density ratio term involving $\tilde{\btheta}_B$ and $\btheta_A$ as a sum of two exponential family distributions with parameters $(2\btheta_B - \btheta_A)$ and $(2\btheta'_B - \btheta_A)$. Note that the joint distributions continue to be product of marginal distributions. Thus if the marginals are sub-Gaussian (sub-exponential) distributions, the joint distributions will be sub-Gaussian (sub-Exponential) since they are a product of independent univariate sub-Gaussian (sub-exponential) distributions.

% The only technical part left to show is to bound the expectation of $\langle \u_{B,B'}, \bxi \rangle^2$. If the marginals have a subG distribution with $\psi_2$ norm $\kappa$, we should be able to bound the expectation by $c_3 \kappa^2$. The argument for subE distribution would be similar, the bound may be $\c_4 \kappa^4$.

% \abcomment{Finally, similar to the Gaussian case, choose $\eta_t$ to control the multiplicative terms, and show the stability bound.}\abcomment{which is a sub-Gaussian (sub-exponential) distribution since it is a product of univariate sub-Gaussian (sub-exponential) distributions}
We gather the above steps to bound $I_{A,B}$:
\lemmexpinfo*

\proof 
Starting from \eqref{eq:expcore}, and using Lemma \ref{lemm:exp_step2} and \ref{lemm:exp_step3}, with $c_3 = \frac{(3c_2 - c_1)c_2}{8c_1}$ we have
\begin{align*}
&I_{A,B}\leq \bigintsss_\bxi \frac{ \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi\\
&\leq \frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]
\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta_B-\btheta_A,\sigma} d\bxi \\
& ~~~ + \frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]
\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta_B'-\btheta_A,\sigma} d\bxi~.
% &+ 2\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B-\btheta_A,\sigma}d\bxi\\
%     &\leq\bigintsss_\bxi \frac{1}{\sigma^4} \bigg(  \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{\alpha^2}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{\alpha^2}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg) \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]\\
%   &\left(\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B - \btheta_A,\sigma} +\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B - \btheta_A,\sigma}\right)\pi_0(\bxi) d\bxi.
\end{align*}
Focusing on the integral in the first term (the analysis for the second term is essentially the same), we have
\begin{align*}
& \bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta_B-\btheta_A,\sigma}(\bxi) d\bxi \\
& = \bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \big( \bxi - \E[\bxi] \big) - \left(\nabla \psi(\tilde{\btheta}_B/\alpha) - \E[\bxi] \right) \right\rangle^2 p_{2\btheta_B-\btheta_A,\sigma}(\bxi) d\bxi \\
& \leq 2\underbrace{\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \E[\bxi] \right\rangle^2 p_{2\btheta_B-\btheta_A,\sigma}(\bxi) d\bxi}_{T_1} + 2 \underbrace{\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \nabla \psi(\tilde{\btheta}_B/\alpha) - \E[\bxi] \right\rangle^2 p_{2\btheta_B-\btheta_A,\sigma}(\bxi) d\bxi}_{T_2}~.
\end{align*}
Note that 
\begin{align*}
T_1 & = \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ \left\langle \btheta_B -\btheta'_B, \bxi - \E[\bxi] \right\rangle^2   \right] \\
& = (\btheta_B -\btheta'_B)^T \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ (\bxi - \E[\bxi]) (\bxi - \E[\bxi])^T \right] (\btheta_B -\btheta'_B)~\\
& = (\btheta_B -\btheta'_B)^T \nabla^2 \psi( 2\btheta_B-\btheta_A/\alpha)  (\btheta_B -\btheta'_B) \\
& \leq \frac{1}{4c_1 \sigma^4} \| \btheta_B -\btheta'_B \|_2^2~,
\end{align*}
since the spectral norm of $\nabla^2 \psi$ is bounded by $1/c_1$. 
%\abcomment{check details after earlier notation is clear, we should get the $1/\sigma^2$ scale factor}

To analyze $T_2$, first note that 
\begin{align*}
\E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}[\bxi] = \nabla \psi( (2\btheta_B - \btheta_A)/2 \sigma^2 ) ~.
\end{align*}
Hence, with $\tilde{\btheta}_B = \alpha_{\bxi} \btheta_B + (1-\alpha_{\bxi}) \btheta'_B$, we have
\begin{align*}
T_2 & = \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ \left\langle \btheta_B -\btheta'_B,  \nabla \psi(\tilde{\btheta}_B/\alpha) - \E[\bxi] \right\rangle^2   \right] \\    
& = \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ \left\langle \btheta_B -\btheta'_B,  \nabla \psi(\tilde{\btheta}_B/\alpha) - \nabla \psi( (2\btheta_B - \btheta_A)/2 \sigma^2 ) \right\rangle^2   \right]\\
& \leq  \| \btheta_B -\btheta'_B \|_2^2 \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ \left\|  \nabla \psi(\tilde{\btheta}_B/\alpha) - \nabla \psi( (2\btheta_B - \btheta_A)/2 \sigma^2 \right\|_2^2  \right]\\
& = \frac{\| \btheta_B -\btheta'_B \|_2^2}{c_1} \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ \left\|  \tilde{\btheta}_B/\alpha - ( (2\btheta_B - \btheta_A)/2 \sigma^2 ) \right\|_2^2  \right] \\
& = \frac{\| \btheta_B -\btheta'_B \|_2^2}{4c_1 \sigma^4} \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ \big\| \alpha_{\bxi} \btheta_B + (1-\alpha_{\bxi}) \btheta'_B - \btheta_B - (\btheta_A - \btheta_B) \big\|_2^2 \right] \\
& = \frac{\| \btheta_B -\btheta'_B \|_2^2}{4c_1 \sigma^4} \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ \big\|  (1-\alpha_{\bxi}) (\btheta'_B - \btheta_B) - (\btheta_A - \btheta_B) \big\|_2^2 \right] \\
& \leq \frac{\| \btheta_B -\btheta'_B \|_2^2}{2c_1 \sigma^4} \left( \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ (1-\alpha_{\bxi})^2  \big\|  \btheta'_B - \btheta_B \big\|_2^2 \right]
+ \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ \big\|  \btheta_B - \btheta_A \big\|_2^2 \right]  \right) \\
& = \frac{\| \btheta_B -\btheta'_B \|_2^2}{2c_1 \sigma^4} \left( \|\btheta_B -\btheta'_B\|_2^2  \E_{\bxi \sim p_{2\btheta_B-\btheta_A,\sigma}}\left[ (1-\alpha_{\bxi})^2  \right] 
+ \|  \btheta_B - \btheta_A \|_2^2  \right) \\
& \leq \frac{\| \btheta_B -\btheta'_B \|_2^2}{2c_1 \sigma^4} \left( \| \btheta_B -\btheta'_B\|_2^2  + \| \btheta_B - \btheta_A \|_2^2 \right) ~.
\end{align*}
Putting everything back together
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta_B-\btheta_A,\sigma}(\bxi) d\bxi
& = \frac{1 + 2 \| \btheta_B - \btheta'_B \|_2^2 + 2 \| \btheta_B - \btheta_A \|_2^2}{2c_1 \sigma^4}  \| \btheta_B - \btheta'_B \|_2^2~.
\end{align*}
Similarly
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta'_B-\btheta_A,\sigma}(\bxi) d\bxi 
& = \frac{1 + 2 \| \btheta_B - \btheta'_B \|_2^2 + 2 \| \btheta'_B - \btheta_A \|_2^2}{2c_1 \sigma^4}  \| \btheta_B - \btheta'_B \|_2^2~.
\end{align*}

% \abcomment{please finish the rest, need to check the scaling w.r.t.~$1/\sigma$ once the earlier notation is cleaned up}


Therefore, plugging into bound on $I_{A,B}$, we have
\begin{align*}
&I_{A,B}
\leq \frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]2
\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta_B-\btheta_A,\sigma} d\bxi \\
+ &\frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]2
\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta_B'-\btheta_A,\sigma} d\bxi~.\\
\leq &\frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \frac{1 + 2 \| \btheta_B - \btheta'_B \|_2^2 + 2 \| \btheta_B - \btheta_A \|_2^2}{c_1 \sigma^4}  \| \btheta_B - \btheta'_B \|_2^2\\
+& \frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \frac{1 + 2 \| \btheta_B - \btheta'_B \|_2^2 + 2 \| \btheta'_B - \btheta_A \|_2^2}{c_1 \sigma^4}  \| \btheta_B - \btheta'_B \|_2^2\\
\leq & \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \frac{1 + 2c_2^2 \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 + 2c_2^2 \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2}{c_1 \sigma^8}  \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma}\|_2^2\\
 + & \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \frac{1 + 2c_2^2 \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 + 2c_2^2 \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2}{c_1 \sigma^8}  \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\\
 \stackrel{(a)}{\leq}& 2\cdot 2\cdot \frac{1}{8} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2/\sigma^4 + 2\cdot 2\cdot \frac{1}{8} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2/\sigma^4\\
 = &  \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2/\sigma^4,
\end{align*}
where step (a) is by choosing step size $\eta_t$ data-dependent and adaptively chosen such that $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq \min( \frac{4}{c_2}\ln 2, \frac{\sigma_t^2}{c_3}\ln 2, \frac{1}{4c_2^2}(\frac{c_1}{8}-\frac{1}{\sigma_t^4})) $, we have the result.
\qed

\theoboundexp*
\proof Similar to Theorem \ref{theo:guss_gen}, based on Lemma \ref{lemm:exp_info}, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate,  we have
\begin{align}
\nr K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right) & = \underset{B_{t} \in G_{1},A_{t} \in G_{0}}{\mathbb{E}}\left[\int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}\right]   \leq  \left[ \frac{\eta_{t}^{2}}{\sigma_{t}^{4}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}


Then, based on the chain rule of KL-divergence, we have
\begin{align}
\nr K L\left(P_{0: T} \| P_{0: T}^{\prime}\right) 
& = \sum_{t=1}^{T} \mathbb{E}_{\w_{t-1}} \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{4}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

Following Theorem \ref{theo:stab}, we have
\begin{align*}
\left|\mathbb{E}_{S}\left[L_{D}\left(\mathbf{w}_{T}\right)-L_{S}\left(\mathbf{w}_{T}\right)\right]\right| \leq \frac{b}{n} \mathbb{E}_{\bar{S}} \sqrt{\sum_{t=1}^{T} \underset{\mathbf{w}_{t-1}}{\mathbb{E}}\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{4}}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z_{n}\right)-\ell\left(\mathbf{w}_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]}, 
\end{align*}
 which completes the proof.

==> Arxiv(old)/app/exp_old.tex <==
% \textsc{Proof for Proposition~[]} Since $p_{\btheta,\sigma}(\bxi)$ is a product of marginal exponential families, $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$, so that the $j$-th component of the gradient $\nabla \psi(\theta)$ is $\nabla_j \psi(\theta) = \psi'_j(\theta_j)$, where $\psi'_j(\theta_j)$ denotes the derivative of $\psi_j(\theta_j)$. Noting that $\psi'_j$ is a monotonic function since $\psi_j$ is convex, we have
% \begin{align*}
% \left\| \nabla \psi(\tilde{\theta}_B/2\sigma^2) \right\|_2^2 & = \sum_{j=1}^p \left| \psi'_j(\tilde{\theta}_{j,B}/2\sigma^2) \right|^2 \\
% & \stackrel{(a)}{\leq} \sum_{j=1}^p \max\left\{ \left| \psi'_j(\theta_{j,B}/2\sigma^2) \right|^2, \left| \psi'_j(\theta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
% & \leq \sum_{j=1}^p \left\{ \left| \psi'_j(\btheta_{j,B}/2\sigma^2) \right|^2 + \left| \psi'_j(\btheta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
% & = \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2 \\
% & \stackrel{(b)}{=} \left\| \m_{B,\sigma} \right\|_2^2 + \left\| \m'_{B,\sigma} \right\|_2^2
% \end{align*}
% where (a) follows since $\tilde{\theta}_{j,B} \in ~\text{interval}(\theta_{j,B},\theta'_{j,B})$\footnote{We use interval$(a,b)$ to denote $[a,b]$ or $[b,a]$, depending on their ordering.} and $\psi'_j$ is monotonic, $\psi'_j(\tilde{\theta}_{j,B}) \in~\text{interval}(\psi'_j(\theta_{j,B}),\psi'_j(\theta'_{j,B}))$, and (b) follows since for exponential families, the mean parameter $\m = \nabla \psi(\theta)$ by Legendre duality [][], and $\m_{B,\sigma}, \m_{B',\sigma}$ are respectively the mean parameters for $p_{\btheta_B,\sigma}, p_{\btheta_{B'},\sigma}$. As a result,
% \begin{align*}
% \bigg( \exp & (\langle \bxi, \btheta_B/2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2)) - \exp(\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2)) \bigg)^2 \\
% & \leq \frac{\| \btheta_B - \btheta'_B \|_2^2}{2\sigma^4} \bigg( \big\langle \u_{B,B'}, \bxi \big\rangle^2 + \| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|^2 \bigg) \exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]~.
% \end{align*}
% % \tcedit{Instead, we can do
% % \begin{align*}\leq \frac{\| \theta_A - \theta_B \|_2^2}{2\sigma^4} \bigg(  \langle u_{A,B},x\rangle^2 + \| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|^2 \bigg) \exp\left[\langle x, \tilde{\theta}_B / \sigma^2 \rangle - 2\psi(\tilde{\theta}_B/2\sigma^2)\right]\end{align*}}
% \abcomment{The $\btheta$ difference can be written as $\m$ difference, see Section 6.3}



% \begin{prop}
% For any $\bxi$, we have 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }
% \leq \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right] ~.
% \end{align*}
% \end{prop}
% \proof Given $\bxi$, for some $\alpha_{\bxi} \in [0,1]$, $\tilde{\btheta} = \alpha_{\bxi} \btheta_B + (1-\alpha_{\bxi}) \btheta'_B$. Denoting $\alpha_{\bxi}$ as $\alpha$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
% \begin{align*}
% \langle \bxi, & \tilde{\btheta}_B / 2\sigma^2 \rangle  - \psi(\tilde{\btheta}_B/2\sigma^2) 
%  = \langle \bxi, \alpha \btheta_B/ 2\sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \rangle - \psi\left( \alpha \btheta_B/ 2 \sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \right) \\
% & = \alpha \bigg[ \langle \bxi , \btheta_B / 2 \sigma^2 \rangle - \psi(\btheta_B/ 2 \sigma^2) \bigg]  + (1-\alpha) \bigg[ \langle \bxi , \btheta'_B /2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2) \bigg] \\
% & ~~~~~~~~~~~~~~~
%   + \bigg[ \alpha \psi(\btheta_B/ 2\sigma^2 ) + (1-\alpha) \psi(\btheta'_B/2 \sigma^2) - \psi( \alpha \btheta_B/2\sigma^2 + (1-\alpha) \btheta'_B/2\sigma^2 ) \bigg] \\
% & \stackrel{(a)}{\leq} \max\bigg[ \langle \bxi , \btheta_B/ 2\sigma^2 \rangle - \psi(\btheta_B/2 \sigma^2) , \langle \bxi , \btheta'_B / 2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2 )  \bigg] \\
% & ~~~~~~~~~~~~~~~ 
%   + \bigg[ \alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2 , \tilde{\btheta}_B/2\sigma^2) \bigg]~,
% \end{align*}
% where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation [Section 3.1.1](Banerjee'05).
% Now, note that
% \begin{align*}
% \alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  
% & \leq \alpha d_{\psi}(\btheta_B/2\sigma^2, \btheta'_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \btheta_B/2\sigma^2) \\
% & \stackrel{(a)}{=} \alpha d_{\phi}(\m'_{\sigma}, \m_{\sigma}) + (1-\alpha) d_{\phi}(\m_{\sigma},\m'_{\sigma})~\\
% & \stackrel{(b)}{\leq} \alpha c_2 \| \m'_{\sigma} - \m_{\sigma} \|_2^2 + (1-\alpha) c_2 \| \m_{\sigma} - \m'_{\sigma} \|_2^2 \\
% & \leq \frac{c_2}{4\sigma^2} \| \hat{\m}_{\sigma} - \hat{\m}'_{\sigma} \|_2^2~,
% \end{align*}
% where (a) follows by duality [][], and (b) follows due to smoothness.
% As a result,
% \begin{align*}
% & \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }\\
% & ~~~~~ \leq \exp\left[ \frac{c_2}{4\sigma^2} \| \hat{\m}_{\sigma} - \hat{\m}'_{\sigma} \|_2^2\right]
% \frac{ \exp \left[ \max\bigg[ \langle \bxi , \btheta_B \rangle - \psi(\btheta_B) , \langle \bxi , \btheta'_B \rangle - \psi(\btheta'_B)  \bigg] \right] }{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] } \\
% & ~~~~~ \leq \exp\left[ \frac{c_2}{4\sigma^2} \| \hat{\m}_{\sigma} - \hat{\m}'_{\sigma} \|_2^2\right] ~.
% \end{align*}
% That completes the proof.\qed 



% \textsc{Proof of Proposition }
% \subsection{Step 3}
% Finally, focusing on density ratio, we have
% \begin{align*}
% & \frac{\left(\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right] \right)^2 }{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi)
% = \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) \\
% & ~~~ \leq 2 \exp \left[ \frac{c_2}{2\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B,\sigma} \|_2^2 \right] \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / \sigma^2 \rangle - 2\psi(\btheta'_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% \end{align*}
% Now, note that
% % \begin{align*}
% % \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}  
% % & = \exp\left[ \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] \\
% % & = \beta_{B,A,\sigma} \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
% % \end{align*}
% % where
% % \begin{align*}
% % \beta_{B,A,\sigma} & = \exp \left[ \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] ~.
% % \end{align*}
% % Note that
% % \begin{align*}
% % \log \beta_{B,A,\sigma} & = \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big)\\
% % & = - \bigg( \psi(\btheta_B/2\sigma^2) - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \bigg) - \bigg( \psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \bigg) \\
% % & \stackrel{(a)}{\leq} \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) /2\sigma^2 \bigg\rangle + \bigg\langle (\btheta_A - \btheta_B)/2\sigma^2, \nabla \psi( \btheta_A/2\sigma^2) /2\sigma^2 \bigg\rangle   \\
% % & = \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \nabla \psi(\btheta_A/2\sigma^2)  \bigg\rangle /2\sigma^2 \\
% % & \stackrel{(b)}{=} \bigg( d_{\psi}(\btheta_B/2\sigma^2, \btheta_A/2\sigma^2) + d_{\psi}(\btheta_A/2\sigma^2 , (2 \btheta_B - \btheta_A)/2\sigma_A^2 ) - d_{\psi}(\btheta_B/2\sigma^2, (2 \btheta_B - \btheta_A)/2\sigma^2 \bigg) / 2 \sigma^2 \\
% % & \leq \big( c_2 \| \btheta_B - \btheta_A \|_2^2 + c_2 \| \btheta_A - (2\btheta_B - \btheta_A) \|_2^2 - c_1 \| \btheta_B - (2\btheta_B - \btheta_A) \|_2^2 \big) / 8 \sigma^6 \\
% % & = (5c_2 - c_1) \| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 / 2 \sigma^2~,
% % \end{align*}
% \begin{align*}
%     \log \beta_{B,A,\sigma} & = \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big)\\
%     & \stackrel{(a)}{=}  d_{\psi}((2\btheta_B - \btheta_A)/2\sigma^2, \btheta_B/2\sigma^2) + d_{\psi}(\btheta_A/2\sigma^2, \btheta_B/2\sigma^2)\\
%     &\stackrel{(b)}{=}  d_{\phi}(\m'_{\sigma}, \m_{\sigma}) +  d_{\phi}(\m_{\sigma},\m'_{\sigma})\\
%     &\leq 2c_2\|(\btheta_B - \btheta_A)/2\sigma^2\|_2^2
% \end{align*}
% where (a) follows from the Bregman information of $\psi$, and (b) follows from duality.
% Since $\phi$ is smooth, we also have
% \begin{align*}
% \| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 & = \| \nabla \phi( \m_{B,\sigma} ) - \nabla \phi (\m_{A,\sigma}) \|_2^2 \leq  c_2^2 \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 = \frac{c_2^2}{4\sigma^2} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 ~,
% \end{align*}
% we have 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}
% \leq \exp \left[ \frac{(5c_2 - c_1)c_2^2}{8\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
% \end{align*}
% The analysis for the term involving $\btheta'_B$ is similar. 

% \subsection{Wrap Up}

% \abcomment{These are notes to wrap up the analysis}

% Note that we have managed to bound the density ratio term involving $\tilde{\btheta}_B$ and $\btheta_A$ as a sum of two exponential family distributions with parameters $(2\btheta_B - \btheta_A)$ and $(2\btheta'_B - \btheta_A)$. Note that the joint distributions continue to be product of marginal distributions. Thus if the marginals are sub-Gaussian (sub-exponential) distributions, the joint distributions will be sub-Gaussian (sub-Exponential) since they are a product of independent univariate sub-Gaussian (sub-exponential) distributions.

% The only technical part left to show is to bound the expectation of $\langle \u_{B,B'}, \bxi \rangle^2$. If the marginals have a subG distribution with $\psi_2$ norm $\kappa$, we should be able to bound the expectation by $c_3 \kappa^2$. The argument for subE distribution would be similar, the bound may be $\c_4 \kappa^4$.

% \abcomment{Finally, similar to the Gaussian case, choose $\eta_t$ to control the multiplicative terms, and show the stability bound.}\abcomment{which is a sub-Gaussian (sub-exponential) distribution since it is a product of univariate sub-Gaussian (sub-exponential) distributions}

% \begin{lemm}
% For exponential family, 
% \begin{align*}
%     I_{A,B} &=  \bigintsss_\bxi \frac{(p_{\btheta_B,\sigma} - p_{\btheta'_B,\sigma})^2}{p_{\btheta_A,\sigma}} d\bxi\leq 
% \end{align*}

% \end{lemm}

% \proof
% From equation~\eqref{eq:exp_target}\eqref{eq:exp_step1}\eqref{eq:exp_step2}\eqref{eq:exp_step3}, we have
% \begin{align*}
%     &I_{A,B}\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi\\
%     &\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2 \bigg) \exp\left[ c_2 \| \nabla \psi(\btheta_B/2\sigma^2) - \nabla \psi(\btheta'_B/2\sigma^2) \|_2^2 \right]}{2\sigma^4 } \\
%     &2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B-\btheta_A,\sigma}+ 2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B-\btheta_A,\sigma}d\bxi\\
%     &\leq\bigintsss_\bxi \frac{\| \btheta_B - \btheta'_B \|_2^2}{2\sigma^4} \bigg( \big\langle \u_{B,B'}, \bxi \big\rangle^2 + \| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|_2^2 \bigg) 2\exp\left[ \frac{c_2}{4} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right]\\
%     \qquad &\left(2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B - \btheta_A,\sigma} +2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B - \btheta_A,\sigma}\right)\pi_0(\bxi) d\bxi\\
%     &\stackrel{(a)}{\leq} c_2^2\| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 (\psi_j^{''}(2\btheta_B-\btheta_A)+\psi_j^{''}(2\btheta'_B-\btheta_A)+ \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2+\| \m'_{B,\sigma} - \m_{A,\sigma} \|_2^2+\| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|_2^2)\\
%     &\exp\left[ \frac{c_2}{4} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right]\left(\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8} \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right]  +\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8} \| \m'_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right] \right),
% \end{align*}
% where $(a)$ is from $\|\E[\bxi\bxi^\top]\|_{\operatorname{op}} = \|\E[\bxi]\E[\bxi]^\top +\operatorname{Var}(\bxi)\|_{\operatorname{op}} \leq \|\E[\bxi]\E[\bxi]^\top\|_{\operatorname{op}}+ \|\operatorname{Var}(\bxi)\|_{\operatorname{op}}\leq \|\E[\bxi]\|_2^2 + \max_j \operatorname{Var}(\bxi_j)$, which completes the proof.
% \qed


% \textbf{Examples.}

% \begin{array}{|l||c|c|c|c|}
% \hline \text { Distribution } & \theta & \psi( \theta ) & \psi'(\theta)&\psi''(\theta)\\
% \hline \hline \text {  Gaussian } & \frac{a}{\sigma^{2}} & \frac{\sigma^{2}}{2} \theta^{2} & \sigma^2\theta & \sigma^2 \\
% \hline \text { Poisson } & \log \lambda & \exp (\theta)& \exp (\theta)& \exp (\theta) \\
% \hline \text { Bernoulli } & \log \left(\frac{q}{1-q}\right) & \log (1+\exp (\theta)) & \frac{\exp(\theta)}{1+\exp(\theta)} & \frac{\exp(\theta)}{(1+\exp(\theta))^2}\\
% \hline \text { Binomial } & \log \left(\frac{q}{1-q}\right) & N \log (1+\exp (\theta)) & N\frac{\exp(\theta)}{1+\exp(\theta)} & N\frac{\exp(\theta)}{(1+\exp(\theta))^2}\\
% \hline \text { Exponential } & -\lambda & -\log (-\theta) & -\frac{1}{\theta} & \frac{1}{\theta^2}\\
% % \hline \text { Laplace } & -\frac{1}{b} & \log(-\frac{2}{\theta}) & -\frac{1}{\theta} & \frac{1}{\theta^2}\\
% \hline
% \end{array}


% \begin{array}{|l||c|c|c|c|}
% \hline \text { Distribution } & p( x ; \theta ) & \m & \phi( \m ) & d_{\phi}( x , \m ) \\
% \hline \hline \text { Gaussian } & \frac{1}{\sqrt{\left(2 \pi \sigma^{2}\right)}} \exp \left(-\frac{(x-a)^{2}}{2 \sigma^{2}}\right) & a & \frac{1}{2 \sigma^{2}} \m^{2} & \frac{1}{2 \sigma^{2}}(x-\m)^{2} \\
% \hline \text { Poisson } & \frac{\lambda^{x} \exp (-\lambda)}{x !} & \lambda & \m \log \m-\m & x \log \left(\frac{x}{\m}\right)-(x-\m) \\
% \hline \text { Bernoulli } & q^{x}(1-q)^{1-x} & q & \m \log \m+(1-\m) \log (1-\m) & x \log \left(\frac{x}{\m}\right)+(1-x) \log \left(\frac{1-x}{1-\m}\right) \\
% \hline \text { Binomial } & \frac{N !}{(x) !(N-x) !} q^{x}(1-q)^{N-x} & N q & \m \log \left(\frac{\m}{N}\right)+(N-\m) \log \left(\frac{N-\m}{N}\right) & x \log \left(\frac{x}{\m}\right)+(N-x) \log \left(\frac{N-x}{N-\m}\right) \\
% \hline \text { Exponential } & \lambda \exp (-\lambda x) & 1 / \lambda & -\log \m-1 & \frac{x}{\m}-\log \left(\frac{x}{\m}\right)-1 \\
% % \hline \text { Laplace } & \frac{1}{2 b} \exp \left(-\frac{|x|}{b}\right) & b & -\log \m-1 & \frac{x}{\m}-\log \left(\frac{x}{\m}\right)-1 \\
% \hline
% \end{array}



% \section{Proof for Exponential family}

% We assume that the multi-variate noise is sub-Gaussian and from a suitable exponential family, so that for $\bxi \in W \subseteq \R^p$
% \begin{align*}
% p_{\btheta}(\bxi) = \exp(\langle \bxi, \btheta \rangle - \psi(\btheta)) \pi_0(\bxi)~,
% \end{align*}
% where $\psi(\btheta)$ is the log-partition function and $\pi_0(\w)$ is the base measure. In our context, we will work with a scaled form based on natural parameter $\btheta/2\sigma^2$, so that
% \begin{align*}
% p_{\btheta,\sigma}(\bxi) = \exp(\langle \bxi, \btheta/2\sigma^2 \rangle - \psi(\btheta/2\sigma^2)) \pi_0(\bxi)~.
% \end{align*}
% Note that the base measure $\pi_0(\bxi)$ does not change with such scaling. Recall that by construction, for $\btheta \in \Theta \subseteq \R^p$, $\psi(\theta)$ is smooth and strongly convex [][][]. Our analysis will cover several
% popular exponential families including Gaussians, Poisson, gamma, Laplace, exponential, among others (see Table ?) [][]. Further, we always consider symmetric versions of one sided distributions such as Poisson, gamma, Laplace, and exponential. 

% We consider adding independent exponential family noise to every component of the gradient update, i.e.,
% for a mini-batch $B$, 
% \begin{align*}
% \w_{t+1} = \w_t - \eta_t \nabla F(\w_{t-1},S_B) + \bxi_t~,
% \end{align*}
% where $\bxi_t \sim p_{\theta_t,\sigma_t}$ so that the components $\xi_t^j, j=1,\ldots,p$ are independent. As a result, the joint distribution $p_{\btheta,\sigma}(\bxi)$ can be written as a product over marginal distributions:
% \begin{align*}
% p_{\btheta,\sigma}(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_j/2\sigma^2 - \psi_j(\theta_j)) \pi_0(\xi_j/2\sigma^2)~,
% \end{align*}
% where we have overloaded notation and used $\pi_0$ to also denote the marginal base measure respectively. Note that in our notation, $\pi_0(\bxi) = \prod_{j=1}^p \pi_0(\xi_j)$ and also $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$. 
% \abcomment{The marginal distributions can be assumed to be sub-Gaussian (sub-Exponential), so the high-d distribution will also be sub-G (sub-E) since its a product of marginal sub-G. Need to add text on this, along with examples.}

\subsection{Preliminary}
We introduce preliminary of exponential family for the analysis. We will use both the natural and expectation parameterization form. Let $\hat{\btheta}_{\sigma} = \btheta/(2\sigma^2)$, and the mean parameter $\hat{\m}_{\sigma} = \nabla_{\hat{\btheta}_{\sigma}} \psi(\hat{\btheta}_{\sigma})$. In our settings, the mean parameter for distribution on batch $B$ is $\m_B = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t})$ so we use $\hat{\m}_{B,\sigma},\hat{\m}'_{B',\sigma}$ to denote $\m_B,\m'_B$ respectively. 
For ease of computation, we denote $\m_{\sigma}$ as the natural gradient: $\m_{\sigma} := \nabla_{\btheta} \psi(\btheta/(2\sigma^2)) = \hat{\m}_{\sigma}/(2\sigma^2)$. Further, $\btheta/(2\sigma^2) = \nabla \psi^{-1}(\m_{\sigma}) = \nabla \phi_{\sigma}(\m_{\sigma})$. 
% Then, 
% \begin{align*}
% \langle \bxi, \btheta/(2\sigma^2) \rangle - \psi(\btheta/(2\sigma^2)) 
% & = \langle \m_{\sigma}, \btheta/(2\sigma^2) \rangle - \psi(\btheta/(2\sigma^2)) + \langle \bxi - \m_{\sigma}, \btheta/(2\sigma^2) \rangle~\\
% & = \phi(\m_{\sigma}) + \langle \bxi - \m_{\sigma}, \nabla \phi(\m_{\sigma}) \rangle \\
% & = - d_{\phi}(\bxi, \m_{\sigma}) + \phi(\bxi)~.
% \end{align*}
Further, since $\psi$ is strongly convex and smooth, so is $\phi$ by Legendre duality, and there are strongly convex constant $c_1$ and Lipschitz smooth constant $c_2$, where $c_1 \leq c_2$ such that
\begin{equation*}
    c_1 \| \bxi - \m \|_2^2 \leq d_{\phi_\sigma}(\bxi,\m) \leq c_2 \| \bxi - \m \|_2^2~,
\end{equation*}
for any $\bxi,\m$ in the domain $\Theta$, any $\sigma\in \Omega$. From the definition of $d_{\phi_\sigma}$:
\begin{equation}
    d_{\phi_\sigma}(\bxi,\m) = \phi_\sigma(\bxi)-\phi_\sigma(\m)-\langle \bxi - \m, \nabla \phi_\sigma (\m)\rangle,
\end{equation}
the strongly convexity and Lipschitz smoothness on $d_{\phi_\sigma}$ implies $\phi_{\sigma}$ is strongly convex and Lipschitz smooth. By duality, we have $\psi$ is strongly convex and Lipschitz smooth  [see Theorem 6 in \cite{kakade2009duality}]:
\begin{equation}
    \frac{1}{4c_2} \| \bxi - \btheta \|_2^2 \leq d_{\psi}(\bxi,\btheta) \leq \frac{1}{4c_1} \| \bxi - \btheta \|_2^2.
\end{equation}


%We further assume that the base measure $\pi_0(\xi_j) \leq 1, j=1,\ldots,p$, \abcomment{may not be necessary} which is satisfied by many 


Following the earlier analysis, by mean-value theorem, for some $\tilde{\btheta}_B = \alpha_x \btheta_B + (1-\alpha_x) \btheta'_B$, $\alpha_x \in [0,1]$, our goal is to bound:
\begin{align}
\nonumber I_{A,B} &=  \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \nabla_{\btheta}p_{\tilde{\btheta}_B,\sigma}\rangle ^2}{p_{\btheta_A,\sigma}} d\bxi = \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/2\sigma^2)\rangle ^2p_{\tilde{\btheta}_B,\sigma}^2}{4\sigma^4 p_{\btheta_A,\sigma}} d\bxi \\
&\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi~.
\end{align}



\subsection{Step 1}
Our goal in this step is to prove the following lemma:
\begin{lemm}\label{lemm:exp_step1}
For some $\tilde{\btheta}_B = \alpha_x \btheta_B + (1-\alpha_x) \btheta'_B$, $\alpha_x \in [0,1]$, we have
\begin{equation}
    \left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2\leq \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2.
\end{equation}
\end{lemm}

\proof
Since $p_{\btheta,\sigma}(\bxi)$ is a product of marginal exponential families, $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$, so that the $j$-th component of the gradient $\nabla \psi(\theta)$ is $\nabla_j \psi(\theta) = \psi'_j(\theta_j)$, where $\psi'_j(\theta_j)$ denotes the derivative of $\psi_j(\theta_j)$. Noting that $\psi'_j$ is a monotonic function since $\psi_j$ is convex, we have
\begin{align*}
\left\| \nabla \psi(\tilde{\theta}_B/2\sigma^2) \right\|_2^2 & = \sum_{j=1}^p \left| \psi'_j(\tilde{\theta}_{j,B}/2\sigma^2) \right|^2 \\
& \stackrel{(a)}{\leq} \sum_{j=1}^p \max\left\{ \left| \psi'_j(\theta_{j,B}/2\sigma^2) \right|^2, \left| \psi'_j(\theta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
& \leq \sum_{j=1}^p \left\{ \left| \psi'_j(\btheta_{j,B}/2\sigma^2) \right|^2 + \left| \psi'_j(\btheta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
& = \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2
\end{align*}
where (a) follows since $\tilde{\theta}_{j,B} \in ~\text{int}(\theta_{j,B},\theta'_{j,B})$\footnote{We use int$(a,b)$ to denote $[a,b]$ or $[b,a]$, depending on their ordering.} and $\psi'_j$ is monotonic, $\psi'_j(\tilde{\theta}_{j,B}) \in~\text{int}(\psi'_j(\theta_{j,B}),\psi'_j(\theta'_{j,B}))$, which completes the proof. \qed

\subsection{Step 2}
Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. In this step we focus on bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$. 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% \end{align*}



\begin{lemm}\label{lemm:exp_step2}
For some $\alpha_{\bxi} \in [0,1]$, $\tilde{\btheta} = \alpha_{\bxi} \btheta_B + (1-\alpha_{\bxi}) \btheta'_B$, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }
\leq \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right] ~.
\end{align*}
\end{lemm}
\proof Denoting $\alpha_{\bxi}$ as $\alpha$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
\begin{align*}
\langle \bxi, & \tilde{\btheta}_B / 2\sigma^2 \rangle  - \psi(\tilde{\btheta}_B/2\sigma^2) 
 = \langle \bxi, \alpha \btheta_B/ 2\sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \rangle - \psi\left( \alpha \btheta_B/ 2 \sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \right) \\
& = \alpha \bigg[ \langle \bxi , \btheta_B / 2 \sigma^2 \rangle - \psi(\btheta_B/ 2 \sigma^2) \bigg]  + (1-\alpha) \bigg[ \langle \bxi , \btheta'_B /2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2) \bigg] \\
& ~~~~~~~~~~~~~~~
  + \bigg[ \alpha \psi(\btheta_B/ 2\sigma^2 ) + (1-\alpha) \psi(\btheta'_B/2 \sigma^2) - \psi( \alpha \btheta_B/2\sigma^2 + (1-\alpha) \btheta'_B/2\sigma^2 ) \bigg] \\
& \stackrel{(a)}{\leq} \max\bigg[ \langle \bxi , \btheta_B/ 2\sigma^2 \rangle - \psi(\btheta_B/2 \sigma^2) , \langle \bxi , \btheta'_B / 2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2 )  \bigg] \\
& ~~~~~~~~~~~~~~~ 
  + \bigg[ \alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2 , \tilde{\btheta}_B/2\sigma^2) \bigg]~,
\end{align*}
where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation (See section 3.1.1 in \cite{banerjee2005clustering}).
Now, note that
\begin{align*}
\alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  
& \leq \alpha d_{\psi}(\btheta_B/2\sigma^2, \btheta'_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \btheta_B/2\sigma^2) \\
& \stackrel{(a)}{=} \alpha d_{\phi}(\m'_{\sigma}, \m_{\sigma}) + (1-\alpha) d_{\phi}(\m_{\sigma},\m'_{\sigma})~\\
& \leq \alpha c_2 \| \m'_{\sigma} - \m_{\sigma} \|_2^2 + (1-\alpha) c_2 \| \m_{\sigma} - \m'_{\sigma} \|_2^2 \\
& \leq \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2~,
\end{align*}
where (a) follows by duality.
As a result,
\begin{align*}
& \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }\\
& ~~~~~ \leq\exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right]
\frac{ \exp \left[ \max\bigg[ \langle \bxi , \btheta_B \rangle - \psi(\btheta_B) , \langle \bxi , \btheta'_B \rangle - \psi(\btheta'_B)  \bigg] \right] }{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] } \\
& ~~~~~ \leq \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right]~.
\end{align*}
That completes the proof.\qed 

% \abcomment{Old proof - not complete/correct} Using the expectation parameterization form, we have 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \tilde{\theta}_B / 2\sigma^2 \rangle - \psi(\tilde{\theta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \theta_B / 2\sigma^2 \rangle - \psi(\theta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \theta'_B / 2\sigma^2 \rangle - \psi(\theta'_B/2\sigma^2) \right] } 
% & = \frac{ \exp \left[ -d_{\phi}(\bxi,\tilde{\m}_{\sigma}) \right]}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} 
% \end{align*}
% For $\bxi$ outside interval$[\m_{B,\sigma}, \m'_{B,\sigma})$, the ratio is at most 1 \abcomment{show details, one component of the denominator will dominate, use 1-d argument if it helps}. For $\bxi$ inside interval$[\m_{B,\sigma}, \m'_{B,\sigma}]$, we have
% \begin{align*}
% \frac{ \exp \left[ -d_{\phi}(\bxi,\tilde{\m}_{\sigma}) \right]}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} 
% & \leq \frac{1}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} \\
% &  \leq \frac{1}{ \exp \left[ - c_2 \| \bxi - \m_{B,\sigma} \|_2^2 \right] +  \exp \left[ - c_2 \| \bxi - \m'_{B,\sigma} \|_2^2 \right]} \\
% & \stackrel{(a)}{\leq} \frac{1}{2} \exp \left[ \frac{c_2}{2} \left( \| \bxi - \m_{B,\sigma}\|_2^2 + \| \bxi - \m'_{B,\sigma} \|_2^2 \right) \right] \\
% & \leq \frac{1}{2} \exp \left[ \frac{c_2}{2} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right] \\
% & = \frac{1}{2} \exp \left[ \frac{c_2}{8\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B,\sigma} \|_2^2 \right]~,
% \end{align*}
% where (a) follows from AM-GM inequality. That completes the proof. \qed

\subsection{Step 3}
Finally, focusing on density ratio, we have
\begin{lemm}\label{lemm:exp_step3}
For any $\bxi$, we have
\begin{align*}
&\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}\\
&\leq \exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right].
\end{align*}

\end{lemm}

\proof
% \begin{align*}
% & \frac{\left(\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right] \right)^2 }{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi)
% = \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) \\
% & ~~~ \leq 2 \exp \left[ \frac{c_2}{2\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B,\sigma} \|_2^2 \right] \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / \sigma^2 \rangle - 2\psi(\btheta'_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% \end{align*}
Note that
\begin{align*}
\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}  
& = \exp\left[ \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] \\
& = \beta_{B,A,\sigma} \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
\end{align*}
where
\begin{align*}
\beta_{B,A,\sigma} & = \exp \left[ \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] ~.
\end{align*}
Note that
\begin{align*}
\log \beta_{B,A,\sigma} & = \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big)\\
& = - \bigg( \psi(\btheta_B/2\sigma^2) - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \bigg) - \bigg( \psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \bigg) \\
& \stackrel{(a)}{\leq} \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) /2\sigma^2 \bigg\rangle + \bigg\langle (\btheta_A - \btheta_B)/2\sigma^2, \nabla \psi( \btheta_A/2\sigma^2) /2\sigma^2 \bigg\rangle   \\
& = \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \nabla \psi(\btheta_A/2\sigma^2)  \bigg\rangle /2\sigma^2 \\
& \stackrel{(b)}{=} \bigg( d_{\psi}(\btheta_B/2\sigma^2, \btheta_A/2\sigma^2) + d_{\psi}(\btheta_A/2\sigma^2 , (2 \btheta_B - \btheta_A)/2\sigma_A^2 ) - d_{\psi}(\btheta_B/2\sigma^2, (2 \btheta_B - \btheta_A)/2\sigma^2 \bigg) / 2 \sigma^2 \\
& \leq \big( 1/c_1 \| \btheta_B - \btheta_A \|_2^2 + 1/c_1 \| \btheta_A - (2\btheta_B - \btheta_A) \|_2^2 - 1/c_2 \| \btheta_B - (2\btheta_B - \btheta_A) \|_2^2 \big) / 8 \sigma^6 \\
& = (3/c_1 - 1/c_2) \| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 / 2 \sigma^2~,
\end{align*}
where (a) follows from the convexity of $\psi$, and (b) follows from the three-point property of Bregman divergences [See Appendix A, property 8 in \cite{banerjee2005clustering}] given by
\begin{equation*}
\langle \x_1 - \x_2, \nabla \psi(\x_3) - \nabla \psi(\x_2) \rangle = d_{\psi}(\x_1,\x_2) + d_{\psi}(\x_2,\x_3) - d_{\psi}(\x_1,\x_3) ~,
\end{equation*}
with $\x_1 = \btheta_B/2\sigma^2, \x_2 = \btheta_A/2\sigma^2, \x_3 = (2\btheta_B - \btheta_A)/2\sigma^2$.
Since $\phi$ is smooth, we also have
\begin{align*}
\| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 & = \| \nabla \phi( \m_{B,\sigma} ) - \nabla \phi (\m_{A,\sigma}) \|_2^2 \leq  c_2^2 \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 = \frac{c_2^2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 ~,
\end{align*}
we have 
\begin{align*}
&\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}\\
&\leq \exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
\end{align*}
which completes the proof.\qed

The analysis for the term involving $\btheta'_B$ is similar. 

\subsection{Final step}


% Note that we have managed to bound the density ratio term involving $\tilde{\btheta}_B$ and $\btheta_A$ as a sum of two exponential family distributions with parameters $(2\btheta_B - \btheta_A)$ and $(2\btheta'_B - \btheta_A)$. Note that the joint distributions continue to be product of marginal distributions. Thus if the marginals are sub-Gaussian (sub-exponential) distributions, the joint distributions will be sub-Gaussian (sub-Exponential) since they are a product of independent univariate sub-Gaussian (sub-exponential) distributions.

% The only technical part left to show is to bound the expectation of $\langle \u_{B,B'}, \bxi \rangle^2$. If the marginals have a subG distribution with $\psi_2$ norm $\kappa$, we should be able to bound the expectation by $c_3 \kappa^2$. The argument for subE distribution would be similar, the bound may be $\c_4 \kappa^4$.

% \abcomment{Finally, similar to the Gaussian case, choose $\eta_t$ to control the multiplicative terms, and show the stability bound.}\abcomment{which is a sub-Gaussian (sub-exponential) distribution since it is a product of univariate sub-Gaussian (sub-exponential) distributions}
We gather the above three steps to bound $I_{A,B}$:
\lemmexpinfo*

\proof 
From Lemma~\ref{lemm:exp_step1},\ref{lemm:exp_step2},\ref{lemm:exp_step3}, we have
\begin{align*}
    &I_{A,B}\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi\\
    &\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2 \bigg) \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]}{2\sigma^4 } \\
    &2\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B-\btheta_A,\sigma}+ 2\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B-\btheta_A,\sigma}d\bxi\\
    &\leq\bigintsss_\bxi \frac{1}{\sigma^4} \bigg(  \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg) \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]\\
   &\left(\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B - \btheta_A,\sigma} +\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B - \btheta_A,\sigma}\right)\pi_0(\bxi) d\bxi.
   \end{align*}
   For $p_{2\btheta_B - \btheta_A,\sigma}$, we have
   \begin{align*}
   &\bigintsss_\bxi \frac{1}{\sigma^4} \bigg(  \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg) \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma}\|_2^2\right]\\
   &\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B - \btheta_A,\sigma}\pi_0(\bxi) d\bxi\\
   &=\frac{1}{\sigma^4} \bigg(  \big(\btheta_B -\btheta'_B)^\top \E_{\bxi\sim p_{2\btheta_B-\btheta_A,\sigma}}\bxi\bxi^\top(\btheta_B -\btheta'_B)  + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg)\\
   &\exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]\\
    % &\stackrel{(a)}{\leq} c_2^2\| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 (\psi_j^{''}(2\btheta_B-\btheta_A)+\psi_j^{''}(2\btheta'_B-\btheta_A)+ \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2+\| \m'_{B,\sigma} - \m_{A,\sigma} \|_2^2+\| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|_2^2)\\
    % &\exp\left[ \frac{c_2}{4} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right]\left(\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8} \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right]  +\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8} \| \m'_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right] \right),\\
    &\stackrel{(a)}{\leq}\frac{1}{\sigma^4}  c_2^2 \| \hat{\m}_{B,\sigma} - \hat{\m}_{B',\sigma} \|_2^2 \bigg(\frac{c_2^2}{16c_1^2\sigma^4}\|2\hat{\m}_{B,\sigma}-\hat{\m}_{A,\sigma}\|_2^2 + \frac{1}{8c_1 \sigma^4}  + \frac{1}{4\sigma^4}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{1}{4\sigma^4}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg)\\
    &\exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]
\end{align*}
where $(a)$ is from $\|\E[\bxi\bxi^\top]\|_{\operatorname{op}} = \|\E[\bxi]\E[\bxi]^\top +\operatorname{Var}(\bxi)\|_{\operatorname{op}} \leq \|\E[\bxi]\E[\bxi]^\top\|_{\operatorname{op}}+ \|\operatorname{Var}(\bxi)\|_{\operatorname{op}}\leq \|\E[\bxi]\|_2^2 + \max_j \operatorname{Var}(\bxi_j) =\frac{1}{4\sigma^4} \|\nabla\psi(2\btheta_B-\btheta_A)\|_2^2 +\frac{1}{4\sigma^4} \max_j |\nabla^2_{jj}\psi(2\btheta_B-\btheta_A)|\leq \frac{1}{4c_1^2}\|2\btheta_B-\btheta_A\|_2^2 + \frac{1}{8c_1 \sigma^4}\leq \frac{c_2^2}{16c_1^2\sigma^4}\|2\hat{\m}_{B,\sigma}-\hat{\m}_{A,\sigma}\|_2^2 + \frac{1}{8c_1 \sigma^4}$. Similar analysis holds for $p_{2\btheta'_B - \btheta_A,\sigma}$, with adaptive choice of step size $\eta_t$ completes the proof.
\qed



% \subsection{OLD Text: keeping for ref, remove in the final version}
% \abcomment{Key observation, the ``projection view" (PV), different from previous (Gaussian) analysis } Since $u_{A,B} = \frac{\theta_A - \theta_B}{\|\theta_A - \theta_B \|_2}$ is a unit vector and the distribution is subG, the projection of $\frac{x-\tilde{\m}_B}{2\sigma^2}$ on the unit vector is a 1-d subG random variable. As a result, the second moment will be bounded as long as $p^2_{\tilde{\theta}_B,\sigma}/p_{\theta_A,\sigma}$ is subG. In fact, it suffices to show that the 1-d projection is subG. 

% Key questions: 
% \begin{enumerate}
% \item Should the analysis be done in expectation or natural parameterization?
% \item How should subG exp family be formalized, w.r.t.~the mean or natural parameters?
% \end{enumerate}

% Switching to mean parameterization: We have
% \begin{align*}
% p_{\theta,\sigma}(x) = p_{\m,\sigma}(x) = \exp(-d_{\phi}(x,\m)/2\sigma^2) q_\sigma(x) 
% \end{align*}
% where $q_\sigma(x)$ may have a dependency on $\sigma$.
% So, we have
% \begin{align*}
% I_{A,B} 
% &=  \bigintsss_x \frac{(p_{\theta_B,\sigma} - p_{\theta'_B,\sigma})^2}{p_{\theta_A,\sigma}} dx \\
% & = \bigints_x \frac{ \bigg[ \exp(-d_{\phi}(x,\m_B)/2\sigma^2) - \exp(-d_{\phi}(x,\m'_B)/2\sigma^2) \bigg]^2}{\exp(-d_{\phi}(x,\m_A)/2\sigma^2)} q_\sigma(x) dx     
% \end{align*}
% By mean-value theorem, for some $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B$, $\alpha_x \in [0,1]$, we have
% \begin{align*}
% \exp & (-d_{\phi}(x,\m_B)/2\sigma^2) - \exp(-d_{\phi}(x,\m'_B)/2\sigma^2) \\
% & = \left\langle \m_B - \m'_B, \nabla_{\tilde{\m}_B} \exp(- d_{\phi}(x,\tilde{\m}_B)/2\sigma^2) \right\rangle \\
% & = \| \m_B - \m'_B \|_2 \left\langle \frac{\m_B-\m'_B}{\|\m_B - \m'_B\|_2} , \frac{H_{\phi}(\tilde{\m}_B) (x - \tilde{\m}_B)}{\sigma^2}  \right\rangle \exp\left[ -d_{\phi}(x,\tilde{\m}_B)/\sigma^2 \right] ~,
% \end{align*}
% \abcomment{need to bound probability terms with $\tilde{\theta}$ or $\tilde{\m}$ with corresponding $\theta_B$ or $\m_B$ terms which do not depend on $x$. Fix the analysis for Gaussians first.}
% where $H_{\phi}(\tilde{\m}_B) = \nabla^2 \phi(\tilde{\m}_B)$ is the Hessian. Since $\phi$ is smooth, with $c_{2,\phi} = \| H_{\phi}\|_2$, and with unit vector $u_{B,B'} = \frac{\m_B - \m_B'}{\|\m_B - \m_B' \|_2}$, we have 
% \begin{align*}
% \langle u_{B,B'}^T H_{\phi}(\tilde{\m}_B) (x - \tilde{\m}_B)\rangle ^2 & \leq 2 \langle u_{B,B'}^T H_{\phi}(\tilde{\m}_B) x \rangle^2 + 2 \langle u_{B,B'}^T H_{\phi}(\tilde{\m}_B) \tilde{\m}_B \rangle^2     \\
% & \leq 2 \| H_{\phi}(\tilde{\m}_B) u_{B,B'} \|_2^2 \bigg\{ \big( v_{B.B'}^T x \big)^2 + \big(v_{B,B'}^T \m_B \big)^2 + \big(v_{B,B'}^T \m_B \big)^2 \bigg\}~,
% \end{align*}
% where $v_{B,B'} = \frac{H_{\phi}(\tilde{\m}_B) u_{B,B'}}{ \| H_{\phi}(\tilde{\m}_B) u_{B,B'} \|_2}$ is a unit vector. As a result, $z = v_{B.B'}^T x$ is a univariate subGaussian distribution, and $v_{B,B'}^T \m_B \leq \| \m_B\|_2$ and $v_{B,B'}^T \m'_B \leq \| \m'_B \|_2$. Hence
% \begin{align*}
% \big(u_{B.B'}^T H_{\phi}(\tilde{\m}_B) (x - \tilde{\m}_B)\big)^2 & \leq 2 c_{\phi} \bigg\{ z^2 + \| \m_B\|_2^2 + \| \m'_B \|_2^2 \bigg\}~.
% \end{align*}
% The distribution ratio term is given by
% \begin{align*}
% \frac{\big(\exp\left[ -d_{\phi}(x,\tilde{\m}_B)/2\sigma^2 \right]\big)^2}{\exp\left[ -d_{\phi}(x,\m_A)/2\sigma^2 \right]} q_\sigma(x)
% & = \exp\left[ -\frac{1}{2\sigma^2} \left[ 2 d_{\phi}(x,\tilde{\m}_B) - d_\phi(x,\m_A) \right] \right] \\
% & \leq \exp\left[ \langle x, 2\tilde{\theta}_B - \theta_A \rangle/2\sigma^2 - \left(2\psi(\tilde{\theta}_B/2\sigma^2) - \psi(\theta_A/2\sigma^2\right) \right] \pi_0(x)    \\
% & = \beta_{A,B} \exp \left[ \left \langle x, (2\tilde{\theta}_B - \theta_A)/2\sigma^2 \right\rangle - \psi((2\tilde{\theta}_B - \theta_A)/2\sigma^2) \right] \pi_0(x)~,
% \end{align*}
% where
% \begin{align*}
% \beta_{A,B} & = \exp \left[ \psi((2\tilde{\theta}_B - \theta_A)/2\sigma^2 ) - \left(2 \psi(\tilde{\theta}_B/2\sigma^2) - \psi(\theta_A/2\sigma^2) \right) \right]~.
% \end{align*}



==> Arxiv(old)/app/experiment.tex <==
{\bf Datasets and Network Structure.} The MNIST and Fashion MNIST datasets both consist of 60,000 training examples and 10,000 test examples. To construct the experiments, we randomly sample $10,000$  samples from the original training set of MNIST and Fashion MNIST. 
Details refer to  Table \ref{tab::network_setup_app}. 
For both MNIST and Fashion MNIST, we use a convolutional neural network with architecture  described in Table \ref{tab:network_app}. 
We also consider a MLP network with three hidden layers with 128, 128 and 64 nodes respectively in each layer. 
All experiments have been run on NVIDIA Tesla v100 GPUs.

\begin{table}[h]
\caption{CNN architecture for MNIST and Fashion MNIST.}
\centering
\begin{tabular}{cc} 
Layer & Parameters \\
\hline \hline Convolution & 16 filters of $8 \times 8,$ strides 2 \\
Max-Pooling & $2 \times 2$ \\
Convolution & 32 filters of $4 x 4,$ strides 2 \\
Max-Pooling & $2 \times 2$ \\
Fully connected & 32 units \\
Softmax & 10 units \\
\hline
\end{tabular}
    \label{tab:network_app}
\end{table}



\begin{table}[h]
  \caption{Neural network and datasets setup.}
	\centering
	\footnotesize{
	%\resizebox{\columnwidth}{!}{%
	\begin{tabular}{cccccc}	
	\toprule[1pt]
	Dataset & Model  & features & classes & Training size  & Test size\\ 	
	\toprule[1pt]
		MNIST            & CNN \& MLP & 28$\times$ 28 & 10 &  10,000  & 10,000\\
Fashion MNIST   & CNN \& MLP  &  28$\times$ 28 & 10 &  10,000  & 10,000\\
		\toprule[1pt]
	\end{tabular}}
%	}
	\label{tab::network_setup_app}
\end{table}


\textbf{Training and Hyper-parameters.} 
We use Noisy SGD with Gaussian noise to train the model, i.e., $\mathbf{w}_{t}=\mathbf{w}_{t-1}-\eta_{t} \nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)+\boldsymbol{\xi}_{t}$, where $\boldsymbol{\xi}_{t} \sim$
$\mathcal{N}\left(0, \sigma_{t}^{2} \mathbb{I}_{d}\right)$. In order to balance the optimization error and generalization error and consider improving the predictive performance, we consider learning rate decay and noise variance decay, such that we set $\sigma_t = c\cdot \eta_t$, wich $c \in [0.05, 0.1]$ and we decay $\eta_t$ every 30 epochs by 0.1. We consider  initial step size $\eta_0 \in \{0.01, 0.005 \}$. 
We set batch size $\left|B_{t}\right|=128$ for all datasets, and minimize cross-entropy loss for a fixed number of epochs. We repeat each experiment for 10 runs.

\textbf{Additional Experimental Results.} Figure \ref{fig: mnist_sigma} (a) and (b) compare our bound with the existing bounds for different noise variance, which shows that as the noise variance/step size ratio increase from 0.05 to 0.1, the bound increase as well. Figures \ref{fig: mnist_eta} and \ref{fig: fashion_eta} compare our bound with  the existing bounds for different initial step sizes for CNN, which shows that our bound is sharper than existing bounds under different step size settings. The training and test accuracy are presented in Table \ref{tab:acc}. 

\begin{figure*}
\centering
  \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr05alpha01_mnist_fnn.png}
 } 
  \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr05alpha05_mnist_fnn.png}
 }  
%   \subfigure[CNN, $\sigma_0 = 0.01$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr01alpha05_mnist_cnn.png}
%  }  
%   \subfigure[CNN,  $\sigma_0 = 0.005$ ]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_cnn.png}
%  }
\caption[]{Numerical results for MLP for MNIST with (a) $\sigma_t = 0.1\eta_t$ and (b)  $\sigma_t = 0.05\eta_t$. $\sigma_0 = 0.005$ for both (a) and (b). All x-axes show the number of Epochs of training.  Figure (a-b) compare our bound with the existing bounds for different noise variance, which shows that as the noise variance/step size ratio increase from 0.05 to 0.1, the bound increase as well. 
%But the optimization error is better compared to larger ratio. Figure (c-d) compare our bound with the existing bounds for different initial step sizes for CNN, which shows that as the bounds with $\eta_0 = 0.01$ are slightly smaller compared to $\eta_0 = 0.005$. 
} \label{fig: mnist_sigma}
\end{figure*}

\begin{figure*}
\centering
%   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
%  } 
%   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
%  }  
  \subfigure[CNN, $\sigma_0 = 0.01$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr01alpha05_mnist_cnn.png}
 }  
  \subfigure[CNN,  $\sigma_0 = 0.005$ ]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr05alpha05_mnist_cnn.png}
 }
\caption[]{Numerical results for CNN for MNIST with (a) $\eta_0 = 0.01$  and (b) $\eta_0 = 0.005$. $\sigma_t = 0.05\eta_t$ for both (a) and (b).  Figure (a-b) compare our bound with  the existing bounds for different initial step sizes for CNN, which shows that our bound is sharper than existing bounds under different step size settings.
}\label{fig: mnist_eta}
\end{figure*}

\begin{table}[h]
\caption{Train and test accuracy for different datasets and models.}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &  & CNN, $\eta_0 = 0.01$ & CNN, $\eta_0 = 0.005$ & MLP, $\sigma_t = 0.1\eta_t$  & MLP, $\sigma_t = 0.05\eta_t$ \\ \hline
\multirow{2}{*}{MNIST} & Train accuracy & 98.21 & 96.69 & 90.45 & 90.39 \\ \cline{2-6} 
 & Test accuracy & 97.28 & 96.37 & 89.99 & 89.92 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fashion\\ MNIST\end{tabular}} & Train accuracy & 83.81 & 79.37 & 81.60 & 81.32 \\ \cline{2-6} 
 & Test accuracy & 82.28 & 78.20 & 79.70 & 79.55 \\ \hline
\end{tabular}\label{tab:acc}
\end{table}

\begin{figure*}[h] 
\centering
%   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
%  } 
%   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
%  }  
  \subfigure[CNN, $\sigma_0 = 0.01$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr01alpha01_fashion_fnn.png}
 }  
  \subfigure[CNN,  $\sigma_0 = 0.005$ ]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr05alpha01_fashion_fnn.png}
 }
\caption[]{Numerical results for MLP for Fashion MNIST with (a) $\eta_0 = 0.01$  and (b) $\eta_0 = 0.005$ .  Figure (a-b) compare our bound with  the existing bounds for different initial step sizes for CNN, which shows that our bound is sharper than existing bounds under different step size settings.
}\label{fig: fashion_eta}
\end{figure*}





\clearpage
\textbf{Experiments on Cifar10 dataset.} We run experiments and compare our bound with the bound in \cite{Li2020On} and \cite{negrea2019information} on Cifar10 dataset. We consider vgg 11 network model with 10,000 training samples randomly sampled from Cifar10 dataset. For training we use initial learning rate 0.001, and noise variance decay such that $\sigma_t = 0.3\eta_t$ and $\sigma_t = 0.5\eta_t$, and we decay $\eta_t$ every 10 epochs with decaying rate 0.93. Figure \ref{fig:cifar10} shows our bound is sharper than existing bound under different noise variance settings.
\begin{figure*}[h] 
\centering
%   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
%  } 
%   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
%  }  
  \subfigure[$\sigma_t = 0.3 \eta_t$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_lr0.001_alpha0.3_mo0.0_decay0.93.png}
 }  
  \subfigure[$\sigma_t = 0.5 \eta_t$]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_lr0.001_alpha0.5_mo0.0_decay0.93.png}
 }

\caption[]{Numerical results for cifar10 dataset. Figure (a-b) shows our bound is sharper than existing bound under different settings of noise variance.
}\label{fig:cifar10}
\end{figure*}




\clearpage
% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%  &  & CNN 0.01 & CNN 0.005 & MLP & MLP \\ \hline
% \multirow{2}{*}{MNIST} & Train accuracy & 98.21 & 96.69 & 90.45 & 90.39 \\ \cline{2-6} 
%  & Test accuracy & 97.28 & 96.37 & 89.99 & 89.92 \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fashion\\ MNIST\end{tabular}} & Train accuracy & 83.81 & 79.37 & 81.60 & 81.32 \\ \cline{2-6} 
%  & Test accuracy & 82.28 & 78.20 & 79.70 & 79.55 \\ \hline
% \end{tabular}
% \end{table}

\textbf{Random Label Experiments.} Inspired by \cite{zhang2017understanding}, we run SGLD to fit 10,000 samples from MNIST dataset Figure \ref{fig:random_label_mnist} and fashionMNSIT dataset Figure \ref{fig:random_label_fashion_mnist}, with increasing fractions of randomly labeled data, from fractions $0\%$ (normal data) to $60\%$. We consider a MLP network with two hidden layers with 128,128 nodes respectively in each layer. For different level of randomly labeled data, we use the same training setting with batch size $|B_t|=128$, initial step size $\eta_0 = 0.05$, noise variance $\sigma_t = 0.07 \cdot \eta_t$, and we decay $\eta_t$ every 10 epochs by 0.95. As shown in Figure~\ref{fig:random_label_mnist} (a) and \ref{fig:random_label_fashion_mnist} (a), with a fixed running time, the experiment with higher level of randomly labeled data has lower training accuracy. Figure \ref{fig:random_label_mnist} (b) and \ref{fig:random_label_fashion_mnist} (b) show higher level of randomly labeled data has higher generalization error and our bound also increase with higher level of randomness, which matches the behavior of generalization error.

\begin{figure*}[h] 
\centering
%   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
%  } 
%   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
%  }  
%   \subfigure[Training Error \& Testing Error]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_train_test_error_lr0.05_alpha0.07_mo0.0.png}
%  }  
  \subfigure[Train Error]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_train_lr0.05_alpha0.06_mo0.0.png}
 }  
   \subfigure[Train Error + Our Bound v.s. Test Error]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_train+bound_vs_test_lr0.05_alpha0.06_mo0.0.png}
 }  
  \subfigure[Generalization error v.s. Our bound]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_error_vs_bound_lr0.05_alpha0.06_mo0.0.png}
 }
%  \subfigure[Our bound]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_empirical_bound_lr0.05_alpha0.07_mo0.0.png}
%  }
\caption[]{Numerical results for random label experiment for MNIST dataset. 
}\label{fig:random_label_mnist}
\end{figure*}

\begin{figure*}[h] 
\centering
%   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
%  } 
%   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
%  }  
  \subfigure[Train Error]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/fashion_random_label_train_lr0.05_alpha0.05_mo0.0.png}
 }  
  \subfigure[Train Error + Our Bound v.s. Test Error]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/fashion_random_label_train+bound_vstest_lr0.05_alpha0.05_mo0.0.png}
 }
   \subfigure[Generalization error v.s. Our bound]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_error_vs_bound_lr0.05_alpha0.05_mo0.0.png}
 }
%  \subfigure[Our bound]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_empirical_bound_lr0.05_alpha0.07_mo0.0.png}
%  }
\caption[]{Numerical results for random label experiment for fashionMNIST dataset.
}\label{fig:random_label_fashion_mnist}
\end{figure*}


\begin{figure*}[h] 
\centering
%   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
%  } 
%   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
%  }  
  \subfigure[Train Error\&Test Error]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_random_label_train_test_lr0.001_alpha0.001_mo0.png}
 }  
  \subfigure[Our Bound]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_random_label_bound_lr0.001_alpha0.001_mo0.png}
 }
%   \subfigure[Generalization error v.s. Our bound]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_error_vs_bound_lr0.05_alpha0.05_mo0.0.png}
%  }
%  \subfigure[Our bound]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/random_label_empirical_bound_lr0.05_alpha0.07_mo0.0.png}
%  }
\caption[]{Numerical results for random label experiment for CIFAR10 dataset.
}\label{fig:random_label_fashion_mnist}
\end{figure*}

==> Arxiv(old)/app/gen.tex <==

\prophell*
\proof Let $S=\left(z_{1}, \ldots, z_{n}\right)$ and $\tilde S^{\prime}=\left(z_{1}^{\prime}, \ldots, z_{n}^{\prime}\right)$ two independent random samples and let $S^{(i)}=\left(z_{1}, \ldots, z_{i-1}, z_{i}^{\prime}, z_{i+1}, \ldots, z_{n}\right)$ be the sample that is identical to $S$ except in the $i$-th example where we replace $z_{i}$ with $z_{i}^{\prime}$. 
\begin{align*}
& \E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))] \\
&= \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \mathbb{E}_{A} \left[\frac{1}{n} \sum_{i=1}^{n}\left(\ell(A(S^{(i)}), z_{i}^{\prime})-\ell(A(S), z_{i}^{\prime}) \right)\right] \\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime}  \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_{A} \left(\ell(A(S^{(i)}), z_{i}^{\prime})-\ell(A(S), z_{i}^{\prime}) \right)\\
& \overset{(a)}{=} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \left(\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p^{(i)}(\mathbf{w}) d \mathbf{w}-\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p(\mathbf{w}) d \mathbf{w} \right)\\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) \left( p^{(i)}(\mathbf{w}) d \mathbf{w}- p(\mathbf{w}) \right)d \mathbf{w} \\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime)\left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)  d \mathbf{w} \\
& \overset{(b)}{\leq} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \left\{\left(\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime)^{2}\left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\}
\end{align*}
where (a): $p^{(i)}(\w)$ is the distribution obtained by $A(S^{(i)})$, and (b) 
follows by Cauchy-Schwartz inequality. Focusing on the first integral, we have: 
\begin{align*}
\left(\int_{\mathbb{R}^{d}} \ell(\w ; z_i^\prime)^{2}\left(\sqrt{p^{(i)}(\w)}+\sqrt{p(\w)}\right)^{2} d \w \right)^{1/2} 
& \leq \left(2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}p^{(i)}(\w) d\w +  2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2} p(\w) d \w \right)^{1/2} \\
& \leq \left( c_0^2 + c_0^2 \right)^{1/2} =\sqrt{2} c_0~.
\end{align*}

Hence,
\begin{align*}
\E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))]
& \leq   \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n}c_0 \sqrt{2H^{2}\left(A(S), A(S'_n)\right)}\\
& = c_0 \E_{S \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S), A(S'_{n})\big)}~.
\end{align*}
% (b): need to double check if we can apply the previous argument that ``for any $z$, the loss $\ell(\w;z)$ has bounded expectation and variance'' because there are dependence between $\ell(\w; z_i^\prime)$ and $p^{(i)}(\w)$. The worst case, we bound it by uniform upper bound $C$ on the loss. (c) is true because $z_i^\prime$ for $i =1,...,n$ are i.i.d., so that we can write it as $z^{\prime}$.
% $p^{\prime}(\mathbf{w})$ is the distribution obtained by $A(S^\prime)$, where $S^\prime$ is the dataset differing on only single sample $z^{\prime}$ with $S$.  

% \abcomment{(a) For the analysis, lets use $| \cdots |$ throughout, (b) pls clean up the $\mu^2 + \sigma^2$ analysis, and use a constant. This part needs work}

% \abcomment{For the last part, change to:}
% \begin{align*}
% & \overset{(b)}{\leq} 2c_0  \mathbb{E}_S \mathbb{E}_{S^\prime} \left[ \frac{1}{n} \sum_{i=1}^{n}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)} \right] \\
% & = 2c_0 \mathbb{E}_S \mathbb{E}_{S'} \mathbb{E}_{z_i^\prime \sim S'}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)}\\
% & \overset{(c)}{=} 2c_0 \mathbb{E}_S \mathbb{E}_{z^{\prime}} \sqrt{D_{H}^{2}\left(p^{\prime}(\mathbf{w}), p(\w)\right)}~.
% \end{align*}
That completes the proof. \qed 


\prophellkl*
\proof For the first part, note that:
\begin{align*}
KL(P ,P') & = \int \log \frac{p(\w)}{p'(\w)} p(\w) ~d\w \\
& =  2 \int  \left\{ - \log \sqrt{\frac{p'(\w)}{p(\w)}} \right\} p(\w)~ d\w \\
& \overset{(a)}{\geq} 2 \int \left\{ 1 - \sqrt{\frac{p'(\w)}{p(\w)}} \right\} p(\w)~ d\w \\ 
& = 2 \int \left( p(\w) - \sqrt{p(\w) p'(\w)}) \right) ~d\w \\
& = \int \left(p(\w) + p'(\w) - 2 \sqrt{p(\w)p'(\w)} \right) ~d\w \\
& = \int \left(\sqrt{p(\w)} - \sqrt{p'(\w)}\right)^2~ d\w\\
& = 2 H^2(P,P')~,
\end{align*}
where (a) follows since for $x > 0$, $-\log x = - \log(1- (1-x)) \geq 1-x$.

For the second part, note that:
\begin{align*}
2H^2(P,P') & =  \int_\w ( \sqrt{p(\w)} - \sqrt{p'(\w)} )^2 d\w \\
& =  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| | \sqrt{p(\w)} - \sqrt{p'(\w)}| ~d\w \\
& \leq  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| | \sqrt{p(\w)} + \sqrt{p'(\w)}|~ d\w \\
& =  \int_\w | p(\w) - p'(\w)|~ d\w \\
& =  TV(P,P')~,
\end{align*}
where $TV(P,P')$ denotes the total variation distance \cite{pollard2002user}. Further, from Pinsker's inequality \cite{tsybakov2008introduction}, we have
\begin{align*}
TV(P,P') \leq \sqrt{\frac{1}{2} KL(P,P')}~.
\end{align*}
Combining the two results completes the proof. \qed 


\subsection{Proofs for Section 2.2}

\mixmodel*
\proof The proof follows the argument in the proof of Lemma 21 in \cite{Li2020On}.\qed

\subsection{Proofs for Section 2.3}

Similar results have appeared in \citep{Li2020On, bun2018composable}, we give a simple proof.
\begin{lemm}\label{lemm:mix_bound}
Let $Q,Q',R$ be any three distributions such that $Q,Q'$ are both absolutely continuous w.r.t.~$R$. Then, for $s \in (0,1)$
\begin{equation}
KL\left(sQ+(1-s)R ~\big\| ~sQ' + (1-s)R \right) \leq 
\frac{s^2}{1-s}~\int_{\w} \frac{(Q(\w) - Q'(\w))^2}{R(\w)} d\w~ .
%\frac{s^2}{1-s} \lsd( Q - Q', R)~.
\end{equation}
\end{lemm}

\proof Let $U=sQ' + (1-s)R$. Then, with $F(x) = Q(x)-Q'(x)$, we have
\begin{align*}
     KL(sQ+(1-s)R \| sQ' + (1-s)R) & =  KL(U + s(Q - Q')  \| U ) \\
     & = \int (U(x) + sF(x)) \log \left( \frac{U(x) + s F(x)}{U(x)} \right) dx \\
     & = \int (U(x) + sF(x)) \log \left( 1 + \frac{s F(x)}{U(x)} \right) dx \\
     & = \int sF(x) + \frac{s^2 F^2(x)}{2U(x)} -  \frac{s^3 F^3(x)}{6U^2(x)} + \frac{s^4 F^4(x)}{12U^3(x)}  -\cdots dx \\
     & = s^2 \int \frac{F^2(x)}{U(x)}\left(  \frac{1}{2} -  \frac{s F(x)}{6U(x)} + \frac{s^2 F^2(x)}{12U^2(x)} - \cdots \right) dx~,
%     & = \int U(x) \left( \left(1+ \frac{sF(x)}{U(x)} \right) \log \left(1 + \frac{sF(x)}{U(x)} \right) - \frac{sF(x)}{U(x)} \right) dx
\end{align*}
where the first term vanishes since $\int F(x) dx = \int (Q(x) - Q'(x)) dx = 0$. This is the reason the dependency is on $s^2$, not $s$. With $W(x) = s F(x)/U(x)$, noting that $W(x) > -1$, and 
\begin{equation}
    \left( \frac{1}{2} - \frac{W(x)}{6} + \frac{W^2(x)}{12} - \cdots \right) = \frac{(1+W(x))\log(1+W(x)) - W(x)}{W^2(x)} \leq 1~,
\end{equation}
we have
\begin{align*}
   KL(sP+(1-s)R \| sQ + (1-s)R) 
     & = s^2 \int \frac{F^2(x)}{U(x)} \left( \frac{ (1+W(x)) \log (1+W(x)) - W(x)}{W^2(x)} \right) dx \\
     & \leq s^2 \int \frac{F^2(x)}{U(x)} dx~ \\
     & \leq \frac{s^2}{(1-s)} \int \frac{(Q(x) - Q'(x))^2}{R(x)} dx~.
\end{align*}
That completes the proof. \qed


\begin{lemm}
Consider a general NSI algorithm with updates of the form~\eqref{eq:nmia} with mini-batch size $B_t = b$. Then, for any trajectory $\w_{0:t-1}$, we have
\begin{align}
KL\left(P_{t|} \| P_{t|} \right) \leq  \frac{b^2}{n^2} \frac{n}{n-b} \E_{B_t \in G_1} \E_{A_t \in G_0} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t}(\bxi_t)} d\bxi_t \right]~.
\end{align}
\label{lemm:lsd}
\vspace*{-6mm}
\end{lemm}

\proof By definition,
\begin{align*}
KL\left(P_{t|} \| P'_{t|}\right) & \stackrel{(a)}{\leq} \left(\frac{b}{n} \right)^2 \left(\frac{n}{n-b}\right) \int_{\w} \frac{(Q - Q')^2}{R} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \bigintsss_{\w} \frac{ \left(  \frac{1}{|G_1|} \left[ \sum_{B \in G_1} P_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right] \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} P_{A,\bxi}(\w)} d\w \\
 & \stackrel{(b)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}\sum_{B \in G_1}  \frac{ \left(  P_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} P_{A,\bxi}(\w)} d\w \\
 & \stackrel{(c)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}  \sum_{B \in G_1} \left\{ \left(  P_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right)^2  \frac{1}{|G_0|}\sum_{A \in G_0} \frac{ 1 }{ P_{A,\bxi}(\w)} \right\} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \frac{1}{|G_1| |G_0|}  \sum_{B \in G_1} \sum_{A \in G_0}  \bigintsss_{\w} \frac{ \left( P_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right)^2 }{ P_{A,\bxi}(\w)} d\w ~,
\end{align*}
where (a) is from Lemma \ref{lemm:mix_bound}, (b)(c) is from Jensen's inequality since function $f(x) = x^2$ is convex and $f(x)=\frac{1}{x}$ is convex on $(0,\infty)$. That completes the proof. \qed



\theostab*

\subsection{Proofs for Section 2.4}

If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered very stable; if $\kappa_A=O(\sqrt[4]{n})$, then $A$ can be considered somewhat stable; and if $\kappa^2_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as the generalization error $\frac{1}{n}Y(S)$ itself. 

\theohighp*

%
%
\proof Let $S=(Z_1,\ldots,Z_n)$ and let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% % Let
% % \begin{align}
% % Y & = f(Z_1,\ldots,Z_n) \\
% % Y'_i & = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)~,~i=1,2,\ldots,n~.
% % \end{align}
With $(x)_+ = max(x,0)$, let
\begin{align}
    V^+ = V^+(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_+^2 ]~,
\end{align}
% % Let
% With $(x)_- = min(x,0)$, let
% \begin{align}
%     V^- = V^-(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~,
% \end{align}

Our proof uses the following exponential version of the Efron-Stein inequality [Theorem 6.16 in \cite{boucheron2013concentration}], whose proof is based on a combination of the symmetric modified log-Sobolev inequality [Theorem 6.15 in \cite{boucheron2013concentration}] with the change of measure:
\begin{theo}\label{theo:exp_efst}
Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
\begin{equation}
\log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
\end{equation}
\end{theo}

% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$ such that $(Y-Y'_i)$ is bounded and $\| Y-Y'_i\|_{\psi_2} = \kappa_A$. Then, with $(x)_+ = \max(0,x)$,
% \begin{equation}
% V^+_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
% \end{equation}
% is sub-Gaussian and $\| V_i^+ \|_{\psi_2} \leq 4\kappa_A^2$. \abcomment{should follow by definition, by bounding $L_p$ norms, since $Y-Y'_i$ is bounded.}
% \end{lemm}


For the proof of Theorem~\ref{theo:hp}, note that $V^+$ is sub-Gaussian with $\| V^+ \|_{\psi_2} \leq n \kappa_A^2$.
Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_2}$. Then from Theorem \ref{theo:exp_efst}, we have
\begin{align*}
\psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right].
\end{align*}
Then, by Markov's inequality we have
\begin{align*}
\log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
 & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
\end{align*}
Choosing $\theta = 1/(2\lambda)$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) 
& \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
\end{align*}
Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
\Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
\end{align*}
With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa_A^2$, with $c_1 = c_0 \sqrt{2}$, we have
\begin{align*}
\P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right) ~.
\end{align*}
Now, we choose $\delta$ such that
\begin{align*}
 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right)   
 \leq 8 \exp \left( - n \epsilon \right)  + 8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta~.
\end{align*}
It suffices to choose $\epsilon$ such that
\begin{align*}
8 \exp \left( - n \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{1}{n} \log \left( \frac{16}{\delta} \right) \\
8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{c_1 \kappa_A}{\sqrt{n}} \log \left( \frac{16}{\delta} \right)~.
\end{align*}
As a result,
\begin{align*}
\P\left( \frac{1}{n}(Y - \E Y) >  \max \left( \frac{1}{n}, \frac{c_1 \kappa_A}{\sqrt{n}} \right) \log \left( \frac{16}{\delta} \right) \right) & \leq \delta~.
\end{align*}
That completes the proof. \qed







% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of random variables. Let $Y= f(Z_1,\ldots,Z_n)$ be sub-Gaussian. Then $\E_{Z_i}[Y]$ is sub-Gaussian. 
% \end{lemm}

% \tcedit{Proof. By Jensen's inequality, we have for any convex function $f$,
% \begin{align*}
%     \E_{Z_2,\cdots, Z_n} f(\E_{Z_1}[Y])\leq \E_{Z_2,\cdots, Z_n} \E_{Z_1}f(Y) = \E f(Y),
% \end{align*}
% by taking $f(x) = |x|^p$, we have $\E_{Z_i}[Y]$ is sub-Gaussian with $\psi_2$ norm bounded by the $\psi_2$ norm of $Y$.}

% \tccomment{Checked.}

% \begin{corr}
% In the setting of Lemma ?, let $Z'_i$ be an independent copy of $Z_i$, and $Y'_i = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, $\E_{Z'_i}[Y'_i]$ is sub-Gaussian.
% \end{corr}

% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, with $(x)_+ = \max(0,x)$,
% \begin{equation}
% V_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
% \end{equation}
% is sub-Exponential. 
% \end{lemm}

% \begin{lemm}
% Let $V_1,\ldots,V_n$ be a set of (identically distributed) sub-Exponential random variables as in Lemma 2 such that $\| V_i \|_{\psi_1} \leq \kappa$ for $i=1,\ldots,n$. Then, 
% \begin{align}
%   \| V^+ \|_{\psi_1} = \left\| \sum_{i=1}^n V_i \right\|_{\psi_1} \leq n \kappa~. 
% \end{align}
% \end{lemm}
% \tcedit{Proof. By triangle inequality:
% \begin{align*}
%     \| V^+ \|_{\psi_1} = \left\| \sum_{i=1}^n V_i^+ \right\|_{\psi_1}\leq \sum_{i=1}^n \left\| V_i^+ \right\|_{\psi_1} \leq n \kappa.
% \end{align*}}\tccomment{checked}



% \subsubsection{Upper Tail Bound}

% The following result is a consequence of combining the Symmetric Modified Logarithmic Sobolev Inequalities (SM-LSI) and the change of measure inequality, which also forms the basis of PAC-Bayes bounds:
% \begin{theo}
% Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
% \begin{equation}
% \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
% \end{equation}
% \end{theo}
% Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_1}$. Then, we have
% \begin{align*}
% \psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right] 
% \end{align*}
% Then, by Markov's inequality we have
% \begin{align*}
% \log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
%  & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
% \end{align*}
% Choosing $\theta = 1/(2\lambda)$, we have 
% \begin{align*}
% \log \P( Y - \E Y > t ) 
% & \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
% \end{align*}
% Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
% \begin{align*}
% \log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
% \Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
% \end{align*}
% With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa$ for a constant $\kappa$, with $c_1 = c_0 \sqrt{2\kappa}$, we have
% \begin{align*}
% \P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \sqrt{n}/c_1 \right\} \epsilon \right) ~.
% \end{align*}
% \abcomment{Instead of $\epsilon$, write the bound in terms of $\log(1/\delta)$}

% \subsubsection{Lower Tail Bound}
% For the lower tail bound, we will use the following result which comes from combining LSI with Chebyshev's association inequality.
% \begin{theo}
% Assume that for some non-decreasing function $g : \R \mapsto \R$, 
% \begin{align*}
%     V^{-} \leq g(Y)~.
% \end{align*}
% Then for all $t > 0$,
% \begin{align*}
%     \P [ Y < \E Y -t ] \leq e^{-t^2/(4 \E [g(Y)])}~.
% \end{align*}
% \end{theo}

% We have
% \begin{align*}
%      V^- & = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~ \\
%      & \leq \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)^2 ] \\
%      & \leq 2 \sum_{i=1}^n \E_{S'} \left[ Y^2 + (Y'_i)^2 \right] \\
%      & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{S'}[ (Y'_i)^2] \\
%      & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{Z'_i}[ (Y'_i)^2] \\
%      & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{Z_i}[ Y^2] \\
%      & \triangleq g(Y)~.
% \end{align*}
% Further, note that
% \begin{align*}
%     \E[g(Y)] = |\E[g(Y)]| \leq \E|g(Y)| \leq \| g(Y) \|_{\psi_1} \leq c n \kappa~.
% \end{align*}
% As a result,
% \begin{align*}
%     \P [ Y < \E Y -t ] \leq e^{-t^2/(4c n \kappa)}~.
% \end{align*}
% With $t = n \epsilon$, we have
% \begin{align*}
%     \P [ Y < \E Y - n \epsilon ] \leq e^{-n\epsilon^2/(4 c \kappa)}~.
% \end{align*}


==> Arxiv(old)/app/guss.tex <==
\lemmaiabguss*


\proof Recall that we want to bound

\begin{align}
 \nr I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t},~~\text{where} ~~ \bxi_t \sim \cN(0, \sigma_t^2\mathbb{I}_d) ~. 
\end{align}

For Noisy SGD with Gaussian noise, we have $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ to be two Gaussian distributions with variance $\sigma_t^2\mathbb{I}_d$, and with mean $\m_{B_t}$ and $\m^\prime_{B_t}$ respectively to be
\begin{align*}
    \m_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t}) \\
    \m'_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_{B_t}) ~.
\end{align*}

Similarly, $P_{A_t,\bxi_t}$ is also a Gaussian noise with mean 
$\m_{A_t}  = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{A_t})$. 
Thus, for any $B_t$ and $A_t$, since $P_{B_{t}, \boldsymbol{\xi}_{t}}$, $P^\prime_{B_{t}, \boldsymbol{\xi}_{t}}$ and $P_{A_{t}, \boldsymbol{\xi}_{t}}$ are Gaussian distributions, $d P_{B_{t}, \boldsymbol{\xi}_{t}}$, $d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}$ and $d P_{A_{t},\boldsymbol{\xi}_{t}}$ are distribution density functions of Gaussian distribution. Then, it is straightforward to have 
\begin{align}
\nr I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{d}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w-\m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
\end{align}
Note that the above calculation considers integral over $d$-dimensional space which introduced an undesired dimension dependence. However, isotropic Gaussian noise is spherical symmetric, we can translate and rotate the coordinate system so that 
$\m_{A_t}=0$  and $ \m_{B_t}, \m_{B_t}^{\prime}$ are mapped to a 2-dimensional space and the Euclidean distances $\|\w-\m_{B_t} + \m_{A_t}\|$, $\|\w-\m_{B_t}^\prime + \m_{A_t}\|$ do not change.  Now, we omit the subscript $t$ in $A_t$, $B_t$, $\bxi_t$ and $\sigma_t$, since the analysis below holds at any $t$-th iteration. We first translate them by $\m_A$ and write $\Delta \m = \m_B - \m_A$, $\Delta \m' = \m'_B - \m_A$. 
% \begin{align*}
%      p_{\m_B,\sigma} \rightarrow x - \m_B + \m_A = x - \Delta \m 
% \end{align*}
% \begin{align*}
%      p_{\m'_B,\sigma} \rightarrow x - \m'_B + \m_A = x - \Delta \m'
% \end{align*}
% \begin{align*}
%      p_{\m_A,\sigma} \rightarrow x - \m_A + \m_A = x~.
% \end{align*}

Let $\w$ be a $d$-dimensional Gaussian distribution with zero mean. Fix a basis $\mathbf{b}_1,...,\mathbf{b}_p$ and draw $\w$ by first drawing signed lengths $\lambda_{i} \sim \mathcal{N}\left(0, \sigma^{2}\right), \text { for } i \in[d]$, then $\w = \sum_{i=1}^d \lambda_i \mathbf{b}_i$. We can choose the basis such that $\Delta \m$ and $\Delta \m'$ are parallel to $\mathbf{b}_1$ and $\mathbf{b}_2$ such that $\Delta \m = a_1 \mathbf{b}_1 + a_2 \mathbf{b}_2$ and $\Delta \m' = a'_1 \mathbf{b}_1 + a'_2 \mathbf{b}_2$. Note that $a_1^2 + a_1^2 = \|\Delta \m\|_2^2 = \|\m_B - \m_A\|_2^2$ and $a'_1^2 + a'_1^2 = \|\Delta \m'\|_2^2 = \|\m'_B - \m'_A\|_2^2$
\begin{align*}
I_{A,B}  & = \bigintsss_\w \frac{ \left(  d P_{\m_B,\bxi} -    d P_{\m'_B,\bxi} \right)^2 }{  d P_{\m_A,\bxi}} d \w   \\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| \w -  \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| \w -  \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \w -  \m_A\|_2^2/2\sigma^2)} d \w  ~\\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| \w -  \Delta\m \|_2^2 / 2\sigma^2 ) - \exp(- \| \w -  \Delta \m'\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x\|_2^2/2\sigma^2)} d \w ~ \\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\sum_{i=1}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~ \\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(-  (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2+ \sum_{i=3}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~\\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\mathbb{R}^2} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2)} d_{\lambda_1, \lambda_2}~\\
 & \qquad \cdot \bigints_{\mathbb{R}^{d-2}}\frac{1}{(\sqrt{2 \pi} \sigma)^{d-2}} \exp(- \sum_{i=3}^d \lambda_i^2/2\sigma^2) ~ d_{\lambda_3,...,\lambda_d} \\
 & =  \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\x \in \mathbb{R}^2} \frac{ \bigg( \exp(- \|\x -  \Delta \m \|_2^2 / 2\sigma^2 ) - \exp(- \|\x -  \Delta \m'\|_2^2 / 2\sigma^2 )\bigg)^2 }{\exp( - \|\x\|_2^2 / 2\sigma^2)} d_{\x}
\end{align*}
We abuse the notation and write $ \m_B - \m_A = \Delta \m$ and $ \m'_B - \m_A = \Delta \m'$ as a two dimensional vector with the norm preserved. Then 
\begin{align*}
I_{A,B} 
 = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\x \in \mathbb{R}^p} \frac{ \bigg( \exp(- \| \x -  \m_B + \m_A \|_2^2 / 2\sigma^2 ) - \exp(- \| \x -  \m'_B + \m_A\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \x \|_2^2/2\sigma^2)} d \x ~.
\end{align*}



Then
we have $I_{A_t, B_t}$ as 
\begin{align}
I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{2}} \int_{\x} \frac{\left(\exp \left(-\left\|\x-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\x-\m_{B}^{\prime} + \m_{A_t} \right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \x~.
\end{align}
Then we treat $\exp \left(-\left\|\x-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ and $\exp \left(-\left\|\x-\m_{B_t}^\prime + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ as two functions of $\x$ where we can 
use Taylor expansion and apply mean-field theorem. Thus, 
%to bound $I_{A_t, B_t}$ as
for each $\x$, we have:
\begin{align*}
 \exp(- \| \x - \m_B +  {\m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| \x - \m'_B +  {\m_A}\|_2^2 / 2\sigma^2 ) 
 & = \bigg\langle \m_B - \m'_B , \nabla \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
\end{align*}
where $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B  {- \m_A}$, where $\alpha_x \in [0,1]$ depends on $\x$. 
Let $\| \tilde{\m}_B\|_2 \leq \max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2) \triangleq \bar{\m}_B$. 

We have
\begin{align*}
  \nabla \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2) & = -\frac{\x -\tilde{\m}_B}{\sigma^2} \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2)~, 
\end{align*}
so that
\begin{align*}
& \frac{ \bigg( \exp(- \| \x - \m_B  { + \m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| \x - \m'_B  { + \m_A} \|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
= \frac{\bigg\langle \m_B - \m'_B , -\frac{\x -\tilde{\m}_B}{\sigma^2} \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{\| \m_B - \m'_B \|_2^2 \| \frac{\x -\tilde{\m}_B}{\sigma^2} \|_2^2 \exp(- \| \x - \tilde{\m}_B\|_2^2 / \sigma^2) }{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|\x\|^2 + \| \tilde {\m}_B \|_2^2 \bigg)  \exp\left(-\frac{\| \x-\tilde{\m}_B\|_2^2}{\sigma^2} + \frac{\|\x\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
= \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|\x\|^2 + \|  \tilde{\m}_B \|_2^2 \bigg)  \exp\left( \frac{ {3}\|\tilde{\m}_B\|_2^2}{ {2}\sigma^2}\right)  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
\leq \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{ {3}\|\bar{\m}_B\|_2^2}{ {2}\sigma^2}\right) \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) ~.
\end{align*}

Since $\tilde{\m}_B$ interpolate between $\m_B  { - \m_A}$ and $\m'_B  { - \m_A} $ and $\exp$ is positive, based on Proposition \ref{prop:mid_step}, with $\m = 2(\m_B  { - \m_A})$, $\m' = 2(\m'_B  { - \m_A})$ and $\tilde \m = 2 \tilde \m_B$,
we have 
% \abcomment{This step is not correct, should be fixable with a scale factor}
% \begin{align*}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left(-\frac{\|x-2(\m_B   { - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2(\m'_B   { - \m_A})\|_2^2}{2\sigma^2}~, \right) 
% \end{align*}

\begin{align*}
\exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) 
\max\left(\exp\left(-\frac{\|\x -2\m_B + 2\m_A\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|\x -2\m_B' + 2\m_A\|_2^2}{\sigma^2}\right) \right)\\
& \leq \exp \left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \left(\exp\left(-\frac{\|\x -2\m_B + 2\m_A\|_2^2}{\sigma^2}\right) + \exp\left(-\frac{\|\x -2\m_B' + 2\m_A\|_2^2}{\sigma^2}\right) \right)
\end{align*}

% \begin{align*}
% \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) \leq \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right).
% \end{align*}



Continuing
\begin{align*}
& \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) d\x \\
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)  \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|\x-2(\m_B { - \m_A})\|_2^2}{2\sigma^2} \right) d\x \\ 
& \phantom{\leq ......} + \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|\x-2(\m'_B  { - \m_A})\|_2^2}{2\sigma^2} \right) d\x \\
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \bigg( 2\sigma^2 + 4\|\m_B  { - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 + 2\sigma^2 + 4\|\m'_B  { - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) \\
& \leq 4 \big(\sigma^2 + \|\m_B  { - \m_A}\|_2^2 + \|\m'_B   { - \m_A} \|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)
\end{align*}


Putting everything back together, we have 
%\yzcomment{Now it just depends on the gradient difference.}
\begin{align*}
I_{A,B} & \leq \frac{1}{2\pi \sigma^2} \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{ {3}\|\bar{\m}_B\|_2^2}{ {2}\sigma^2}\right) 4 \big(\sigma^2 + \|\m_B  { - \m_A}\|_2^2 + \|\m'_B  { - \m_A}\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)\\
& \leq \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{ \|\bar{\m}_B\|_2^2}{2\sigma^2} \bigg) \exp\left( \frac{3\|\bar{\m}_B\|_2^2}{2\sigma^2}\right)~\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \|\m_B-\m_B'\|_2^2 \\
& = \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2)^2}{2\sigma^2} \bigg) \\
& \qquad \exp\left( \frac{\max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2)\|_2^2}{\sigma^2}\right)~\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)\|\m_B-\m_B'\|_2^2
\end{align*}

Now we are interested in $\|\m_B -\m_A\|_2$,  $\|\m'_B -\m_A\|_2$ and $\|\m_B -\m_B'\|_2$. Recall that we have $B \in G_1$ which contains the $z_n'$ and $A \in G_0$: 
\begin{align*}
    \m_B & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_B) \\
    \m'_B & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_B) ~.
\end{align*}
\begin{align*}
    \m_A & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_A) ~.
\end{align*}

So that 

\begin{align*}
\m_B - \m_A & = \eta_t \nabla \ell(\w_{t-1},S_B)  - \eta_t \nabla \ell(\w_{t-1},S_A) \\
& = \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell(\w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(\w_{t-1},\tilde{z}) \right]~,
\end{align*}
and
\begin{align*}
\m'_B - \m_A & = \eta_t \nabla \ell(\w_{t-1},S'_B)  - \eta_t \nabla \ell(\w_{t-1},S_A) \\
& = \frac{\eta_t}{m} \left[ \sum_{z \in S'_B} \nabla \ell(\w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(\w_{t-1},\tilde{z}) \right]~.
\end{align*}
Also, 
\begin{align*}
\m'_B - \m_B = \frac{\eta_t}{m} \left( \nabla \ell (\w_{t-1}, z_n) - \nabla \ell (\w_{t-1}, z'_n) \right) ~.  
\end{align*}

Let $\Delta_t(\bar{S}) \triangleq \max_{z,\tilde{z} \in \bar{S}} \| \nabla \ell(w_{t-1},z) - \nabla \ell( \w_{t-1},\tilde{z}) \|_2$, where $\bar{S} \sim D^{n+1}$ as before. Now, note that 
%\abcomment{note that the pairing $(z_i,\tilde{z}_i)$ below is arbitrary, the analysis does not depend on the pairing}
\begin{align*}
\| \m_B - \m_A \|_2^2 & = \left\| \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell( \w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell( \w_{t-1},\tilde{z} \right] \right\|_2^2 \\
& \leq \eta_t^2 \left\| \frac{1}{m} \sum_{i=1}^m \big( \nabla \ell( \w_{t-1},z_i) - \nabla \ell( \w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
& \leq \eta_t^2 \frac{1}{m} \sum_{i=1}^m  \left\|  \big( \nabla \ell( \w_{t-1},z_i) - \nabla \ell( \w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
& \leq \eta_t^2 \Delta^2_t(\bar{S})~.
\end{align*}

Also, $\| \m_B' - \m_A \|_2^2 \leq \eta_t^2 \Delta^2_t(\bar{S})$ and  $\| \m_B' - \m_B \|_2^2 \leq \eta_t^2 \Delta^2_t(\bar{S})$. With the setting that $ \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \leq \ln 3/2$, we have

\begin{align}
I_{A_t, B_t} \leq  \frac{\|\m_{B_t} - \m_{B_t}^\prime \|_2^2}{\sigma_t^2}=  18(1+ \frac{5}{2}\ln\frac{3}{2})\ln \frac{3}{2} \frac{\eta_t^2\left\|\nabla \ell\left( \w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}}{\sigma_t^2}~, \label{eq:guss_with_c}
\end{align}
That completes the proof. \qed


\genboundguss*

\proof Based on Lemma \ref{lemm:iab_guss}, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate,  we have
\begin{align}
\nr K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right) & = \underset{B_{t} \in G_{1},A_{t} \in G_{0}}{\mathbb{E}}\left[\int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}\right]   \leq  \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c = 41 \ln \frac{3}{2}$ based on \eqref{eq:guss_with_c}.

Then, based on the chain rule of KL-divergence, we have
\begin{align}
\nr K L\left(P_{0: T} \| P_{0: T}^{\prime}\right) 
& = \sum_{t=1}^{T} \mathbb{E}_{\w_{t-1}} \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

Following Theorem \ref{theo:stab}, we have
\begin{align*}
\left|\mathbb{E}_{S}\left[L_{D}\left(\mathbf{w}_{T}\right)-L_{S}\left(\mathbf{w}_{T}\right)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar{S}} \sqrt{\sum_{t=1}^{T} \underset{\mathbf{w}_{t-1}}{\mathbb{E}}\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z_{n}\right)-\ell\left(\mathbf{w}_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]},  
\end{align*}
where $c = 41 \ln \frac{3}{2}$. 


\begin{prop}
Assume $\m,\m'$ fixed and $\tilde{\m}$ on the line segment of $\m$ and $\m'$, we have
    \begin{align*}
    \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) \leq \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right).
\end{align*} \label{prop:mid_step}
\end{prop}

\proof  From the law of cosine, we have 
\begin{align*}
    \|x -\m\|_2^2 = \|x-\tilde{\m}\|_2^2 + \|\m-\tilde{\m}\|_2^2 -2 \|x-\tilde{\m}\|_2  \|\m-\tilde{\m}\|_2 \cos \angle x\tilde{\m} \m,
\end{align*}
and
\begin{align*}
    \|x -\m'\|_2^2 = \|x-\tilde{\m}\|_2^2 + \|\m'-\tilde{\m}\|_2^2 -2 \|x-\tilde{\m}\|_2  \|\m'-\tilde{\m}\|_2 \cos \angle x\tilde{\m} \m',
\end{align*}
where $\angle x\tilde{\m} \m + \angle x\tilde{\m} \m' = \frac{\pi}{2}$ so we have $\cos\angle x\tilde{\m} \m + \cos\angle x\tilde{\m} \m' = 0$. By canceling out $\cos$ via weighted sum of the above two equations, we have
\begin{align*}
    &\|x -\m\|_2^2 \|\m'-\tilde{\m}\|_2 + \|x -\m'\|_2^2 \|\m-\tilde{\m}\|_2\\
    =& \|x-\tilde{\m}\|_2^2\|\m'-\tilde{\m}\|_2 + \|\m-\tilde{\m}\|_2^2\|\m'-\tilde{\m}\|_2 + \|x-\tilde{\m}\|_2^2\|\m-\tilde{\m}\|_2 + \|\m'-\tilde{\m}\|_2^2\|\m-\tilde{\m}\|_2.
\end{align*}
Equivalently we have 
\begin{align*}
    \|x-\tilde{\m}\|_2^2 = \frac{\|\m-\tilde{\m}\|_2}{\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2} \|x -\m'\|_2^2 + \frac{\|\m'-\tilde{\m}\|_2}{\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2} \|x -\m\|_2^2 - \|\m-\tilde{\m}\|_2\|\m'-\tilde{\m}\|_2.
\end{align*}
Since $\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2 = \|\m-\m'\|_2$, from AM-GM inequality we have
\begin{align*}
    \|x-\tilde{\m}\|_2^2\geq \min \left(\|x -\m\|_2^2,\|x -\m'\|_2^2\right) - \frac{1}{4} \|\m-\m'\|_2^2,
\end{align*}
therefore we have
\begin{align*}
    \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) &\leq \exp\left(-\min \left(\frac{\|x -\m\|_2^2}{\sigma^2},\frac{\|x -\m'\|_2^2}{\sigma^2}\right) + \frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\\
    &= \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right),
\end{align*}
which completes the proof.
\qed





% Consider two collection of points $\{\m_B : B \in G \}$ and $\{\m_B : B \in G\}$. In our context, at any stage $t$, conditioned on $w_{t-1}$, for mini-batch $B$, we have
% \begin{align*}
%     \m_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S_B) \\
%     \m'_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S'_B) ~.
% \end{align*}
% Let $p_{\m,\sigma}$ denote the Gaussian distribution $\cN(\m, \sigma^2 \I)$.


% If the noise added is Gaussian, without loss of generality, we can translate and rotate the coordinate system so that $\m_A=0$, and $\m_B,\m'_B$ have the last $(d-2)$ coordinates as 0. With abuse of notation, we denote the first two coordinates of $\m_A,\m_B,\m'_B$ as $\m_{A},\m_B,\m'_B$, noting that the remaining $(d-2)$ coordinates are 0.  Note that the translation and rotation does not change the Euclidean distances $\|\m_B - \m'_B\|_2$, $\|\m_B - \m_A\|_2 = \| \m_B \|_2$, and $\|\m'_B - \m_A\|_2 = \| \m'_B \|_2$. Then, since the integral over the last $(d-2)$ simply cancel out the partition function $1/(\sqrt{2\pi \sigma^2}^{d-2}$, we have
% \yzcomment{I think it should be  $\exp(- \| x - \m_B + \m_A\|_2^2/2\sigma^2  )$ and  $\exp(- \| x - \m'_B + \m_A\|_2^2/2\sigma^2  )$}
% \begin{align*}
% I_{A,B}  & = \bigintsss_x \frac{ \left(  p_{\m_B,\sigma} -   p_{\m'_B,\sigma} \right)^2 }{ p_{\m_A,\sigma}} d \w  \\

%  = \frac{1}{2\pi \sigma^2} \bigints_\w \frac{ \bigg( \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} d \w ~,
% \end{align*}
% where the latter is a 2-d integral. For each $\w$, we can apply mean-field theorem [][] to get:
% \begin{align*}
%  \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) 
%  & = \bigg\langle \m_B - \m'_B , \nabla \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
% \end{align*}
% where $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B$, where $\alpha_x \in [0,1]$ depends on $\w$. Note that $\| \tilde{\m}_B\|_2 \leq \max(\|\m_B\|_2,\|\m'_B\|_2) \triangleq \bar{\m}_B$. We have
% \begin{align*}
%   \nabla \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2) & = -\frac{x -\tilde{\m}_B}{\sigma^2} \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2)~, 
% \end{align*}
% so that
% \begin{align*}
% & \frac{ \bigg( \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% = \frac{\bigg\langle \m_B - \m'_B , -\frac{x -\tilde{\m}_B}{\sigma^2} \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% \leq \frac{\| \m_B - \m'_B \|_2^2 \| \frac{x -\tilde{\m}_B}{\sigma^2} \|_2^2 \exp(- \| x - \tilde{\m}_B\|_2^2 / \sigma^2) }{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% \leq \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \exp\left(-\frac{\|x-\tilde{\m}_B\|_2^2}{\sigma^2} + \frac{\|x\|_2^2}{2\sigma^2} \right) \\
% & \phantom{......................} 
% = \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \exp\left( \frac{\|\tilde{\m}_B\|_2^2}{\sigma^2}\right)  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) \\
% & \phantom{......................} 
% \leq \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{\|\bar{\m}_B\|_2^2}{\sigma^2}\right) \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) ~.
% \end{align*}
% % Now, consider the random variable $\tilde{X} \sim \cN(\tilde{\m}_B, \sigma^2 )$. 
% % Note that $\tilde{X}$ is sub-Gaussian with $\| \tilde{X} \|_{\psi_2} \leq c_0 (\sigma^2 + \| \tilde{\m}_B\|_2^2) \leq c_0 (\sigma^2 + \|\bar{\m}_B\|_2^2)$, where $c_0$ is an absolute constant. Then \abcomment{this needs to be shown, some variant of this should be true}, for an absolute constant $c_1$ \abcomment{apply Jensen's?}
% Since $\tilde{\m}_B$ interpolate between $\m_B$ and $\m'_B$ and $\exp$ is positive, we have
% \begin{align*}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left(-\frac{\|x-2\m_B\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2\m'_B\|_2^2}{2\sigma^2}~, \right) 
% \end{align*}
% so that
% \begin{align*}
% \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) & \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) d \w  \\
% & \leq \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|x-2\m_B\|_2^2}{2\sigma^2} \right) d \w  \\ 
% & \phantom{\leq ......} + \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|x-2\m'_B\|_2^2}{2\sigma^2} \right) d \w  \\
% & \leq \bigg( 2\sigma^2 + 4\|\m_B\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) + \bigg( 2\sigma^2 + 4\|\m'_B\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) \\
% & \leq 4 \big(\sigma^2 + \|\m_B\|_2^2 + \|\m'_B\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)
% \end{align*}

% \yzcomment{It is better to work with gradient difference, instead of $\m_B$ and $\bar \m_B$ which contains $w$.}

% Putting everything back together, we have 
% \begin{align*}
% I_{A,B} & \leq \frac{1}{2\pi \sigma^2} \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{\|\bar{\m}_B\|_2^2}{\sigma^2}\right) 4 \big(\sigma^2 + \|\m_B\|_2^2 + \|\m'_B\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\\
% & \leq \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B\|_2^2}{\sigma^2} + \frac{\|\m'_B\|_2^2}{\sigma^2} + \frac{ \|\bar{\m}_B\|_2^2}{2\sigma^2} \bigg) \exp\left( \frac{\|\bar{\m}_B\|_2^2}{\sigma^2}\right)~~\| \m_B - \m'_B \|_2^2
% \end{align*}


% \yzcomment{ --------- updated analysis below --------}

% Details on the rotation and translation:\\
% We are interested in three $d$-dimensional Gaussian distributions:
% \begin{align*}
%  p_{\m_B,\sigma} =   \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 )~,
% \end{align*}
% \begin{align*}
%  p_{\m'_B,\sigma} =   \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 )~,
% \end{align*}
% \begin{align*}
%  p_{\m_A,\sigma} =   \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \exp(- \| x - \m_A\|_2^2 / 2\sigma^2 )~.
% \end{align*}
% By definition, we want to calculate:
% \begin{align*}
% I_{A,B}  = \bigintsss_x \frac{ \left(  p_{\m_B,\sigma} -   p_{\m'_B,\sigma} \right)^2 }{ p_{\m_A,\sigma}} d \w  
%  = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x - \m_A\|_2^2/2\sigma^2)} d \w ~.
% \end{align*}
% Since Gaussian is a spherically symmetric normal which
% is independent of the orthogonal basis from which its constituent
% normals are drawn. We first translate three of them by $\m_A$ and write $\Delta \m = \m_B - \m_A$, $\Delta \m' = \m'_B - \m_A$:
% \begin{align*}
%      p_{\m_B,\sigma} \rightarrow x - \m_B + \m_A = x - \Delta \m 
% \end{align*}
% \begin{align*}
%      p_{\m'_B,\sigma} \rightarrow x - \m'_B + \m_A = x - \Delta \m'
% \end{align*}
% \begin{align*}
%      p_{\m_A,\sigma} \rightarrow x - \m_A + \m_A = x~.
% \end{align*}
% Note that $\w$ is a $d$-dimensional Gaussian distribution with zero mean. $\w$ is a  spherically symmetric distribution. Fix a basis $\mathbf{b}_1,...,\mathbf{b}_p$ and draw $\w$ by first drawing signed lengths $\lambda_{i} \sim \mathcal{N}\left(0, \sigma^{2}\right), \text { for } i \in[d]$, then $x = \sum_{i=1}^d \lambda_i \mathbf{b}_i$. We can choose the basis such that $\Delta \m$ and $\Delta \m'$ are parallel to $\mathbf{b}_1$ and $\mathbf{b}_2$ such that $\Delta \m = a_1 \mathbf{b}_1 + a_2 \mathbf{b}_2$ and $\Delta \m' = a'_1 \mathbf{b}_1 + a'_2 \mathbf{b}_2$. Note that $a_1^2 + a_1^2 = \|\Delta \m\|_2^2 = \|\m_B - \m_A\|_2^2$ and $a'_1^2 + a'_1^2 = \|\Delta \m'\|_2^2 = \|\m'_B - \m'_A\|_2^2$
% \begin{align*}
% I_{A,B}  & = \bigintsss_x \frac{ \left(  p_{\m_B,\sigma} -   p_{\m'_B,\sigma} \right)^2 }{ p_{\m_A,\sigma}} dx 
%  = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x - \m_A\|_2^2/2\sigma^2)} dx ~\\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| x - \Delta\m \|_2^2 / 2\sigma^2 ) - \exp(- \| x - \Delta \m'\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x\|_2^2/2\sigma^2)} dx~ \\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_{\mathbb{R}^d} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\sum_{i=1}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~ \\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_{\mathbb{R}^d} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(-  (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2+ \sum_{i=3}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~\\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\mathbb{R}^2} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2)} d_{\lambda_1, \lambda_2}~\\
%  & \qquad \cdot \bigints_{\mathbb{R}^{d-2}}\frac{1}{(\sqrt{2 \pi} \sigma)^{d-2}} \exp(- \sum_{i=3}^d \lambda_i^2/2\sigma^2) ~ d_{\lambda_3,...,\lambda_d} \\
%  & =  \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{x \in \mathbb{R}^2} \frac{ \bigg( \exp(- \|x - \Delta \m \|_2^2 / 2\sigma^2 ) - \exp(- \|x - \Delta \m'\|_2^2 / 2\sigma^2 )\bigg)^2 }{\exp( - \|x\|_2^2 / 2\sigma^2)} d_{x}
% \end{align*}
% We abuse the notation and write $ \m_B - \m_A = \Delta \m$ and $ \m'_B - \m_A = \Delta \m'$ as a two dimensional vector with the norm preserved. Then 
% \begin{align*}
% I_{A,B}  = \bigintsss_x \frac{ \left(  p_{\m_B,\sigma} -   p_{\m'_B,\sigma} \right)^2 }{ p_{\m_A,\sigma}} dx 
%  = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{x \in \mathbb{R}^p} \frac{ \bigg( \exp(- \| x - \m_B + \m_A \|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B + \m_A\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} dx~.
% \end{align*}


% \yzcomment{----------- below mainly follows Prof. Banerjee's analysis ------}

% For each $\w$, we can apply mean-field theorem [][] to get:
% \begin{align*}
%  \exp(- \| x - \m_B + \yzedit{\m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B + \yzedit{\m_A}\|_2^2 / 2\sigma^2 ) 
%  & = \bigg\langle \m_B - \m'_B , \nabla \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
% \end{align*}
% where $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B \yzedit{- \m_A}$, where $\alpha_x \in [0,1]$ depends on $\w$. Note that $\| \tilde{\m}_B\|_2 \leq \max(\|\m_B \yzedit{-\m_A}\|_2,\|\m'_B \yzedit{-\m_A} \|_2) \triangleq \bar{\m}_B$. We have
% \begin{align*}
%   \nabla \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2) & = -\frac{x -\tilde{\m}_B}{\sigma^2} \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2)~, 
% \end{align*}
% so that
% \begin{align*}
% & \frac{ \bigg( \exp(- \| x - \m_B \yzedit{ + \m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B \yzedit{ + \m_A} \|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% = \frac{\bigg\langle \m_B - \m'_B , -\frac{x -\tilde{\m}_B}{\sigma^2} \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% \leq \frac{\| \m_B - \m'_B \|_2^2 \| \frac{x -\tilde{\m}_B}{\sigma^2} \|_2^2 \exp(- \| x - \tilde{\m}_B\|_2^2 / \sigma^2) }{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% \leq \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|x\|^2 + \| \tilde {\m}_B \|_2^2 \bigg)  \exp\left(-\frac{\|x-\tilde{\m}_B\|_2^2}{\sigma^2} + \frac{\|x\|_2^2}{2\sigma^2} \right) \\
% & \phantom{......................} 
% = \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|x\|^2 + \|  \tilde{\m}_B \|_2^2 \bigg)  \exp\left( \frac{\yzedit{3}\|\tilde{\m}_B\|_2^2}{\yzedit{2}\sigma^2}\right)  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) \\
% & \phantom{......................} 
% \leq \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{\yzedit{3}\|\bar{\m}_B\|_2^2}{\yzedit{2}\sigma^2}\right) \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) ~.
% \end{align*}
% % Now, consider the random variable $\tilde{X} \sim \cN(\tilde{\m}_B, \sigma^2 )$. 
% % Note that $\tilde{X}$ is sub-Gaussian with $\| \tilde{X} \|_{\psi_2} \leq c_0 (\sigma^2 + \| \tilde{\m}_B\|_2^2) \leq c_0 (\sigma^2 + \|\bar{\m}_B\|_2^2)$, where $c_0$ is an absolute constant. Then \abcomment{this needs to be shown, some variant of this should be true}, for an absolute constant $c_1$ \abcomment{apply Jensen's?}
% Since $\tilde{\m}_B$ interpolate between $\m_B \yzedit{ - \m_A}$ and $\m'_B \yzedit{ - \m_A} $ and $\exp$ is positive, we have \abcomment{This step is not correct, should be fixable with a scale factor}
% \begin{align*}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left(-\frac{\|x-2(\m_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2(\m'_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2}~, \right) 
% \end{align*}
% \begin{prop}
% We have 
% \begin{align}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left( \frac{\| \m_B - \m'_B \|_2^2}{2\sigma^2} \right) \exp\left(-\frac{\|x-2(\m_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2(\m'_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2}~ \right)~.     
% \end{align}
% \end{prop}
% \abcomment{needs a proof}
% \proof (outline, need to check) Consider the ratio and note that we can set $x=\tilde{\m}_B$. Then, the problem reduces to lower bounding
% \begin{align*}
% \exp\left(-\frac{\|\tilde{\m}_B-2(\m_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|\tilde{\m}_B -2(\m'_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2}~ \right)~,
% \end{align*}
% which gives the desired bound. \qed





% \abcomment{We should use the fact that integral (expectation) is really 1-d}

% Continuing
% \begin{align*}
% \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) & \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) dx \\
% & \leq \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|x-2(\m_B \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) dx \\ 
% & \phantom{\leq ......} + \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|x-2(\m'_B \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) dx \\
% & \leq \bigg( 2\sigma^2 + 4\|\m_B \yzedit{ - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) + \bigg( 2\sigma^2 + 4\|\m'_B \yzedit{ - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) \\
% & \leq 4 \big(\sigma^2 + \|\m_B \yzedit{ - \m_A}\|_2^2 + \|\m'_B  \yzedit{ - \m_A} \|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)
% \end{align*}


% Putting everything back together, we have \yzcomment{Now it just depends on the gradient difference.}
% \begin{align*}
% I_{A,B} & \leq \frac{1}{2\pi \sigma^2} \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{\yzedit{3}\|\tilde{\m}_B\|_2^2}{\yzedit{2}\sigma^2}\right) 4 \big(\sigma^2 + \|\m_B \yzedit{ - \m_A}\|_2^2 + \|\m'_B \yzedit{ - \m_A}\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\\
% & \leq \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B \yzedit{ - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B \yzedit{ - \m_A}\|_2^2}{\sigma^2} + \frac{ \|\bar{\m}_B\|_2^2}{2\sigma^2} \bigg) \exp\left( \frac{\|\bar{\m}_B\|_2^2}{\sigma^2}\right)~~\| \m_B - \m'_B \|_2^2 \\
% & = \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B \yzedit{ - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B \yzedit{ - \m_A}\|_2^2}{\sigma^2} + \frac{\max(\|\m_B \yzedit{-\m_A}\|_2,\|\m'_B \yzedit{-\m_A} \|_2)^2}{2\sigma^2} \bigg) \\
% & \qquad \exp\left( \frac{\max(\|\m_B \yzedit{-\m_A}\|_2,\|\m'_B \yzedit{-\m_A} \|_2)\|_2^2}{\sigma^2}\right)~~\| \m_B - \m'_B \|_2^2
% \end{align*}

% \abcomment{I think the first part $(1+x^2+y^2+z^2)$ term can be avoided. See how it is being done for the subG case, based on the ``projection view" (PV), i.e., the analysis is essentially 1-dimensional. I will help transfer that argument to Gaussian. The main term $\exp(\Delta \m^2/\sigma^2)$ will stay, but we expect that.}

% \yzcomment{-------- Calculate KL-divergence ----------}

% Note that we are interested in $\|\m_B -\m_A\|_2$ and  $\|\m'_B -\m_A\|_2$. Recall that $B \in G_1$ which contains the $z_n'$ and $A \in G_0$ which contains the same mini-batch for $w$ and $w'$: 
% \begin{align*}
%     \m_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S_B) \\
%     \m'_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S'_B) ~.
% \end{align*}
% \begin{align*}
%     \m_A & = w_{t-1} - \eta_t \nabla F(w_{t-1},S_A) ~.
% \end{align*}

% So that \abcomment{minor typo: second line is based on gradient, not loss. Assume gradient is subG, for a fixed $w_{t-1}$, then we can get a $1/\sqrt{b}$ concentration. Also, the analysis may improve based on the "projection view".}
% \begin{align*}
% \m_B - \m_A & = \eta_t \nabla F(w_{t-1},S_B)  - \eta_t \nabla F(w_{t-1},S_A) \\
% %& = \eta _t \frac{1}{b} \left(\sum_{z \in \{S_B/z_{n}\} } \nabla \ell (w_{t-1}, z) + \ell (w_{t-1}, z_n) - \sum_{z \in \{S_A\} } \nabla \ell (w_{t-1}, z) \right)  \\
% & = \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell(w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(w_{t-1},\tilde{z}) \right]~,
% \end{align*}
% and
% \begin{align*}
% \m'_B - \m_A & = \eta_t \nabla F(w_{t-1},S'_B)  - \eta_t \nabla F(w_{t-1},S_A) \\
% %& = \eta _t \frac{1}{b} \left(\sum_{z \in \{S_B/z_{n}\} } \ell (w_{t-1}, z) + \ell (w_{t-1}, z'_n) - \sum_{z \in \{S_A\} } \ell (w_{t-1}, z) \right)  \\
% %& \triangleq \eta_t \Delta_t({S'_B,S_A})~
% & = \frac{\eta_t}{m} \left[ \sum_{z \in S'_B} \nabla \ell(w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(w_{t-1},\tilde{z}) \right]~.
% \end{align*}
% Also, 
% \begin{align*}
% \m'_B - \m_B = \frac{\eta_t}{m} \left( \nabla \ell (w_{t-1}, z_n) - \nabla \ell (w_{t-1}, z'_n) \right) ~.  
% \end{align*}

% Let $A_*$ and $B_*$ be the set that maximize $\|\m_B - \m_A\|^2$  and $\|\m'_B - \m_A\|^2$.  \abcomment{Lets see if we can avoid bounding things by $I_{A*,B*}$. We can assume that the stochastic gradients are sub-Gaussian, so an average over $b$ samples will have concentration with rate $1/\sqrt{b}$. Alternative is to assume expected gradient discrepancy is bounded. The goal is to avoid taking sup over samples/mini-batches. We already have the result as an expectation over mini-batches, lets keep that if possible.}
% Now we put $I_{A,B}$ back to the KL-divergence and set $b \leq \frac{n}{2}$: 
% \begin{align*}
%  & KL(w_t | w_{t-1} \| w_t' | w_{t-1})  \\
%  & \leq \frac{b^{2}}{n^{2}}\left(1+\frac{b}{n-b}\right) \frac{1}{\left|G_{0}\right|\left|G_{1}\right|} \sum_{A \in G_{0}} \sum_{B \in G_{1}} \int_{x} \frac{\left(p_{\m_{B}, \sigma}-p_{\m_{B}^{\prime}, \sigma}\right)^{2}}{p_{\m_{A}, \sigma}} d x = \frac{b^{2}}{n^{2}}\left(1+\frac{b}{n-b}\right) \frac{1}{\left|G_{0}\right|\left|G_{1}\right|} \sum_{A \in G_{0}} \sum_{B \in G_{1}} I_{A,B} \\
%  & \leq \frac{b^{2}}{n^{2}}\left(1+\frac{b}{n-b}\right) \frac{1}{\left|G_{0}\right|\left|G_{1}\right|} \sum_{A \in G_{0}} \sum_{B \in G_{1}}  I_{A_*,B_*} \\
%  & \leq \frac{b^{2}}{n^{2}}\left(1+\frac{b}{n-b}\right)   I_{A_*,B_*} \\
%  & \leq \frac{b^{2}}{n^{2}}  \frac{3}{2} I_{A_*,B_*} \\
%  & \leq \frac{b^{2}}{n^{2}}  \frac{12}{\sigma^2}  \bigg(1 + \frac{\|\m_{B_*} - \m_{A_*}\|_2^2}{\sigma^2} + \frac{\|\m'_{B_*} - \m_{A_*}\|_2^2}{\sigma^2} + \frac{\max(\|\m_{B_*} {-\m_{A_*}}\|_2,\|\m'_{B_*} {-\m_{A_*}} \|_2)^2}{2\sigma^2} \bigg) \\
% & \qquad \exp\left( \frac{\max(\|\m_{B_*} {-\m_{A_*}}\|_2,\|\m'_{B_*} {-\m_{A_*}} \|_2)\|_2^2}{\sigma^2}\right)~~\| \m_{B_*} - \m'_{B_*} \|_2^2\\
% & \leq \frac{b^{2}}{n^{2}}  \frac{12}{\sigma^2}  \bigg(1 + \frac{5}{2} \frac{\max(\|\m_{B_*} {-\m_{A_*}}\|_2^2,\|\m'_{B_*} {-\m_{A_*}} \|_2^2)}{2\sigma^2} \bigg)  \exp\left( \frac{\max(\|\m_{B_*} {-\m_{A_*}}\|_2^2,\|\m'_{B_*} {-\m_{A_*}} \|_2^2)}{\sigma^2}\right)\| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2\\
% & = \frac{b^{2}}{n^{2}}  \frac{12}{\sigma^2}  \bigg(1 + \frac{5 }{2} \frac{ \eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{2\sigma^2} \bigg)  \\
% & \qquad
% \exp\left( \frac{\eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{\sigma^2}\right)~\| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2
% \end{align*}


% \textbf{Condition: } Let $\exp\left( \frac{\eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{\sigma_t^2}\right) \leq c $ for all $t \in [T]$, which means
% \begin{align*}
% \frac{\eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{\sigma_t^2} \leq \ln c~.
% \end{align*}
% Then we have
% \begin{align*}
%  KL(w_t | w_{t-1} \| w_t' | w_{t-1}) \leq \frac{b^{2}}{n^{2}}  \frac{12 c }{\sigma^2} (1 + \frac{5\ln c}{2})  \| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2~.
% \end{align*}

% Note that for $b=1$, the \textbf{condition} translates to, for all $t \in [T]$
% \begin{align*}
% \frac{\eta_t^2\max_{z \in S_0, z_n, z'_n}(\|\nabla \ell (w_{t-1},z_n) - \nabla \ell (w_{t-1},z) \|_2^2,\|\nabla \ell (w_{t-1},z'_n) - \nabla \ell (w_{t-1},z) \|_2^2)}{\sigma_t^2} \leq \ln c~,  
% \end{align*}

% \tccomment{The quantity of interest:
% $\E_S\E_{w_{t-1}}\E_{z_n} \exp \frac{\eta_t^2\max(\|\nabla \ell (w_{t-1},z_n) - \nabla \ell (w_{t-1},z) \|_2^2,\|\nabla \ell (w_{t-1},z'_n) - \nabla \ell (w_{t-1},z) \|_2^2)}{\sigma_t^2}$, if we fix $S$ and $w_{t-1}$ then randomness come from minibatch, then $\max(\|\nabla \ell (w_{t-1},z_n) - \nabla \ell (w_{t-1},z) \|_2^2,\|\nabla \ell (w_{t-1},z'_n) - \nabla \ell (w_{t-1},z) \|_2^2)$ is a random pick from constant and its $\psi_2$ norm has dependence on $A*,B*$; if we fix $S$, randomness comes from $w_{t-1}$ and mini-batch, then $\nabla \ell (w_{t-1},z_n)$ has dependent coordinates on $w_{t-1}$ where norm cannot be easily controlled.}



% \begin{theo}
% With $T$ iterations, for a given training set $\bar S$, and for $\{\eta_t, \sigma_t\}_{t=1}^T$ satisfying 
% \begin{align*}
% \frac{\eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{\sigma_t^2} \leq \ln c~,
% \end{align*}
% we have
% \begin{align*}
%  KL(w_1,..., w_T \| w'_1,..., w'_T) \leq  \frac{b^{2}}{n^{2}}  \frac{12 c }{\sigma^2} (1 + \frac{5\ln c}{2})  \sum_{t=1}^T \| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2~.
% \end{align*}
% \end{theo}

% The generalization bound follows by taking the expectation of the  KL divergence over the random draw of $\bar S$. If one uses uniform stability, then the generalization bound follows by taking the supreme of the  KL divergence over $\bar S$. 

% \subsection*{Bounding the exp term} 
% Let $\Delta_t(\bar{S}) \triangleq \max_{z,\tilde{z} \in \bar{S}} \| \nabla \ell(w_{t-1},z) - \nabla \ell(w_{t-1},\tilde{z}) \|_2$, where $\bar{S} \sim D^{n+1}$ as before. Now, note that \abcomment{note that the pairing $(z_i,\tilde{z}_i)$ below is arbitrary, the analysis does not depend on the pairing}
% \begin{align*}
% \| \m_B - \m_A \|_2^2 & = \left\| \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell(w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(w_{t-1},\tilde{z} \right] \right\|_2^2 \\
% & \leq \eta_t^2 \left\| \frac{1}{m} \sum_{i=1}^m \big( \nabla \ell(w_{t-1},z_i) - \nabla \ell(w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
% & \leq \eta_t^2 \frac{1}{m} \sum_{i=1}^m  \left\|  \big( \nabla \ell(w_{t-1},z_i) - \nabla \ell(w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
% & \leq \eta_t^2 \Delta^2_t(\bar{S})~.
% \end{align*}
% Note that $\eta_t = \eta_t(\bar{S})$ and $\sigma_t = \sigma_t(\bar{S})$, i.e., they would be data dependent.
% Then, the overall bound is \abcomment{need to add the $\sum_t$, this is just one term}
% \begin{align*}
% KL & \leq \frac{m^2}{n^2} \frac{12}{\sigma_t^2} \exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \E_{B,B'}\left[ \| \m_B - \m'_B\|_2^2 \right] ~\\
% & = \frac{m^2}{n^2} \frac{\eta_t^2}{m^2} \frac{12}{\sigma_t^2} \exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \E_{z_n,z'_n}\left[\| \nabla \ell(w_{t-1},z_n) - \ell(w_{t-1},z'_n) \|_2^2 \right] \\
% & = \frac{12}{m n^2} \frac{\eta_t^2}{\sigma_t^2} \exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \E_{z_n,z'_n}\left[\| \nabla \ell(w_{t-1},z_n) - \ell(w_{t-1},z'_n) \|_2^2 \right]~.
% \end{align*}
% For any $\sigma_t$, it suffices to choose $\eta_t$ such that $\eta_t \leq \sigma_t/(2\Delta_t(\bar{S}))$, so that $\exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \leq 3/2$. 

% Or,  for any $\eta_t$, it suffices to choose $\sigma_t$ such that $\sigma_t \geq \eta_t \Delta_t(\bar{S})/2$, so that $\exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \leq 3/2$.

% {\bf Adpative choice of $\eta_t,\sigma_t$.} Check if $\eta_t$ can deterministically depend on the history. Check if $\sigma_t$ can depend on history and depend on $\eta_t$ to satisfy the scaling condition.




% \abcomment{we can discuss the fresh sample case, and why the condition depending on $\Delta_t$ is unnecessary as long as gradients are subG. I wll add a proof.}



==> Arxiv(old)/app/high-prob.tex <==

% \subsection{Bounded Deviation}
% If the loss function $\ell(w,z)$ is bounded, then we can get a high probability bound by the bounded difference inequality. 

\subsection{Sub-Gaussian Deviation}

Let $S=(Z_1,\ldots,Z_n)$ and let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. Let
\begin{align}
Y & = f(Z_1,\ldots,Z_n) \\
Y'_i & = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)~,~i=1,2,\ldots,n~.
\end{align}
Let
\begin{align}
    V^+ = V^+(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_+^2 ]~,
\end{align}
and let
\begin{align}
    V^- = V^-(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~,
\end{align}

\begin{lemm}
Let $Z_1,\ldots,Z_n$ be a set of random variables. Let $Y= f(Z_1,\ldots,Z_n)$ be sub-Gaussian. Then $\E_{Z_i}[Y]$ is sub-Gaussian. 
\end{lemm}

\tcedit{Proof. By Jensen's inequality, we have for any convex function $f$,
\begin{align*}
    \E_{Z_2,\cdots, Z_n} f(\E_{Z_1}[Y])\leq \E_{Z_2,\cdots, Z_n} \E_{Z_1}f(Y) = \E f(Y),
\end{align*}
by taking $f(x) = |x|^p$, we have $\E_{Z_i}[Y]$ is sub-Gaussian with $\psi_2$ norm bounded by the $\psi_2$ norm of $Y$.}

\tccomment{Checked.}

\begin{corr}
In the setting of Lemma ?, let $Z'_i$ be an independent copy of $Z_i$, and $Y'_i = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, $\E_{Z'_i}[Y'_i]$ is sub-Gaussian.
\end{corr}

\begin{lemm}
Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, with $(x)_+ = \max(0,x)$,
\begin{equation}
V_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
\end{equation}
is sub-Exponential. 
\end{lemm}

\begin{lemm}
Let $V_1,\ldots,V_n$ be a set of (identically distributed) sub-Exponential random variables as in Lemma 2 such that $\| V_i \|_{\psi_1} \leq \kappa$ for $i=1,\ldots,n$. Then, 
\begin{align}
   \| V^+ \|_{\psi_1} = \left\| \sum_{i=1}^n V_i \right\|_{\psi_1} \leq n \kappa~. 
\end{align}
\end{lemm}
\tcedit{Proof. By triangle inequality:
\begin{align*}
    \| V^+ \|_{\psi_1} = \left\| \sum_{i=1}^n V_i^+ \right\|_{\psi_1}\leq \sum_{i=1}^n \left\| V_i^+ \right\|_{\psi_1} \leq n \kappa.
\end{align*}}\tccomment{checked}
\subsubsection{Upper Tail Bound}

The following result is a consequence of combining the Symmetric Modified Logarithmic Sobolev Inequalities (SM-LSI) and the change of measure inequality, which also forms the basis of PAC-Bayes bounds:
\begin{theo}
Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
\begin{equation}
\log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
\end{equation}
\end{theo}
Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_1}$. Then, we have
\begin{align*}
\psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right] 
\end{align*}
Then, by Markov's inequality we have
\begin{align*}
\log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
 & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
\end{align*}
Choosing $\theta = 1/(2\lambda)$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) 
& \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
\end{align*}
Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
\Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
\end{align*}
With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa$ for a constant $\kappa$, with $c_1 = c_0 \sqrt{2\kappa}$, we have
\begin{align*}
\P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \sqrt{n}/c_1 \right\} \epsilon \right) ~.
\end{align*}
\abcomment{Instead of $\epsilon$, write the bound in terms of $\log(1/\delta)$}

\subsubsection{Lower Tail Bound}
For the lower tail bound, we will use the following result which comes from combining LSI with Chebyshev's association inequality.
\begin{theo}
Assume that for some non-decreasing function $g : \R \mapsto \R$, 
\begin{align*}
    V^{-} \leq g(Y)~.
\end{align*}
Then for all $t > 0$,
\begin{align*}
    \P [ Y < \E Y -t ] \leq e^{-t^2/(4 \E [g(Y)])}~.
\end{align*}
\end{theo}

We have
\begin{align*}
     V^- & = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~ \\
     & \leq \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)^2 ] \\
     & \leq 2 \sum_{i=1}^n \E_{S'} \left[ Y^2 + (Y'_i)^2 \right] \\
     & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{S'}[ (Y'_i)^2] \\
     & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{Z'_i}[ (Y'_i)^2] \\
     & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{Z_i}[ Y^2] \\
     & \triangleq g(Y)~.
\end{align*}
Further, note that
\begin{align*}
    \E[g(Y)] = |\E[g(Y)]| \leq \E|g(Y)| \leq \| g(Y) \|_{\psi_1} \leq c n \kappa~.
\end{align*}
As a result,
\begin{align*}
    \P [ Y < \E Y -t ] \leq e^{-t^2/(4c n \kappa)}~.
\end{align*}
With $t = n \epsilon$, we have
\begin{align*}
    \P [ Y < \E Y - n \epsilon ] \leq e^{-n\epsilon^2/(4 c \kappa)}~.
\end{align*}

==> Arxiv(old)/app/notes.tex <==

\abcomment{This is a place-holder section -- some/most of this will get dropped. Please do not add important proofs to this section. We should have a separate appendix section corresponding to each main section.}

\subsection{Bounding Uniform Stability.} %Bound uniform stability with Hellinger divergence, generalize to losses with first 2 moments bounded.
%
%
Take $p(\w)$ and $p^\prime(\w)$ as the probability density functions over $\w$ from running $\cA$ with $S$ and $S^\prime$. Thus, we have
\begin{align*}
\epsilon_{n} &=\sup _{x, S, S^{\prime}}\left|\int_{\mathbb{R}^{d}} \ell(\w ; z) p(\w) d \w-\int_{\mathbb{R}^{d}} \ell(\w ; z) p^\prime(\w) d \w\right| \\
&=\sup _{x, S, S^{\prime}}\left|\int_{\mathbb{R}^{d}} \ell(\w ; z)\left(\sqrt{p(\w)}+\sqrt{p(\w)^{\prime}}\right)\left(\sqrt{p(\w)}-\sqrt{p(\w)^{\prime}}\right) d \w\right| \\
& \leq \sup \left\{\left(\int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}\left(\sqrt{p(\w)}+\sqrt{p(\w)^{\prime}}\right)^{2} d \w\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p(\w)}-\sqrt{p(\w)^{\prime}}\right)^{2} d \w\right)^{\frac{1}{2}}\right\} ~.
%&<2 C \sqrt{D_{H}\left(p(\w) \| p(\w)^{\prime}\right)}~,
\end{align*}
where the inequality follows by Cauchy-Schwarz. Focusing on the first integral, we have:
\begin{align*}
 I & = \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}\left(\sqrt{p(\w)}+\sqrt{p(\w)^{\prime}}\right)^{2} d \w \\
 & \leq 2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}p(\w) d\w + 
 2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2} p^{\prime}(\w) d \w~.
\end{align*}
We assume that for any $z$, the loss $\ell(\w;z)$ has bounded expectation and variance, i.e., for $\w \sim p$ or $\w \sim p'$
\begin{align*}
    \E_{\w}[\ell(\w;z)] & \leq \mu \\
    \E_{\w}\left[\left(\ell(\w,z) - \E_{w}[\ell(\w;z)]  \right)^2 \right] & \leq \sigma^2~.
\end{align*}
Ideally, we want the analysis to be either over $\E_z$ or have the bounds hold with high probability over the distribution of $z$; otherwise, the assumption is uniform over $z$.

When the loss $\ell(w;z) = - \log p(z|\w)$, i.e., log-likelihood of $z$ on a model with parameter $\w$, the moment assumptions may be translated to assumptions on the tails of $p(z|\w)$, e.g., sub-Gaussian.

Based on the assumption, we have:
\begin{align*}
    I & \leq 2 \E_{\w \sim p} [ \ell^2(\w;z)] + 2 \E_{\w \sim p} [ \ell^2(\w;z)] \leq 4 (\mu^2 + \sigma^2)~.
\end{align*}
As a result,
\begin{align*}
\epsilon_{n} & \leq 2 \sqrt{\mu^2 + \sigma^2} \sqrt{D_H^2(P,P')}~,
\end{align*}
where $D_H^2$ denotes the squared Hellinger divergence. Now, recall that $D_H^2 \leq KL(P, P')$, the KL-divergence. As a result, we have
As a result,
\begin{align*}
\epsilon_{n} & \leq 2 \sqrt{\mu^2 + \sigma^2} \sqrt{KL(P,P')}
\end{align*}
Note that we can bound uniform stability with the square root of the KL-divergence, which gives a few advantages over the current literature:
\begin{itemize}
\item Avoids the "Bayes Stability" business of Li et al., which does not have a high-probability version and does not quite align with other results in stability.
\item Avoids the information theoretic approach of Pensia et al., etc., which also does not (yet) have a high probability bound.
\item Simplifies the approach of Mou et al., by working KL rather than Hellinger so more tools, such as chain rule become available. Note that the Hellinger bound is sharper, but the approach to bound the Hellinger in Mou et al., did not yield a data dependent bound (although this may be possible).
\end{itemize}

%\subsubsection{Expected Stability}


\subsection{Overall Argument [Old, Placeholder]}
\noindent {\bf Bounding squared Hellinger with TV and KL.} We have
\begin{equation}
H^2(P,P') \leq  TV(P.P') \leq \sqrt{KL(P,P')}~.
\end{equation}

\noindent {\bf Bounding KL with gradients.} For a noisy iterative algorithm, 
\begin{equation}
    w_{t+1} = w_t - \eta_t \nabla F(w_t,z_i) + \sigma_t \cN0(0,1)~,
\end{equation}
we have
\begin{equation}
    KL(P, P') \leq \frac{1}{n^2}  \E_{S \sim D^n} \left[ \sum_{t=1}^T \frac{\gamma_t^2}{\sigma_t^2} \E_{w \sim W_{t-1}}\left[ \frac{1}{n} \sum_{i=1}^n \| \nabla F(w,z)i) \|_2^2 \right] \right] ~.
\end{equation}
For basic SGD or Adam, the bound should be based on PAC-Bayes.

\noindent {\bf In expectation to High Probability.} Using the Feldman-Vondrak result.



\subsection{Bounding the KL divergence with $\chi^2$-divergence}

Recall that $f$-divergence is defined as: for any convex function $f : (0,\infty) \rightarrow \R$ and $P \ll Q$, the $f$ divergence from $P$ to $Q$ is defined by:
\[
D_f(P \| Q) = \int f\left( \frac{dP}{dQ} \right) dQ~. 
\]
For the special case of $f(t) = (t-1)^2$ or $f(t) = t^2 -1$, we get the $\chi^2$ divergence:
\begin{equation}
    \chi^2(P \| Q)  = \int \left( \frac{dP}{dQ} - 1\right)^2 dQ = \int \left( \frac{dP}{dQ} \right)^2 dQ - 1~. 
\end{equation}

Let $P,Q,R$ be any three distributions. Then, for $s \in (0,1)$
\begin{equation}
    KL\left(sP+(1-s)R ~\big\| ~sQ + (1-s)R \right) \leq s^2~\int \frac{(P(x) - Q(x))^2}{U(x)} dx~ = s^2 \E\left[ \frac{(P(x)-Q(x))^2}{U^2(x)}\right] ~.
\end{equation}
Using
\begin{equation}
    (P-Q)^2 = 2(P^2 + Q^2) - 4 \left( \frac{P}{2} + \frac{Q}{2} \right)^2~,
\end{equation}
we have
\begin{align*}
\frac{1}{s^2} KL\left(sP+(1-s)R ~\big\| ~sQ + (1-s)R \right) & \leq 2 \E_U \left[ \frac{P^2}{U^2} \right] 
+ 2 \E_U \left[ \frac{Q^2}{U^2} \right] - 4  \E_U \left[ \frac{(P/2+Q/2)^2}{U^2} \right] \\
& \leq 2 \E_U \left[ \frac{P^2}{U^2} \right] 
+ 2 \E_U \left[ \frac{Q^2}{U^2} \right] -   \E_U \left[ \frac{P^2+Q^2}{U^2} \right] \\
& = \E_U \left[ \frac{P^2}{U^2} \right] 
+ \E_U \left[ \frac{Q^2}{U^2} \right] \\
& =  \E_U \left[ \frac{P^2}{(sQ + (1-s)R)^2} \right] 
+ \E_U \left[ \frac{Q^2}{(sQ + (1-s)R)^2} \right] 
\end{align*}
We focus on each term.


\begin{comment}

We show that Assumption~\ref{asmp:subg} is related to the assumption of extended uniform stability:
\begin{asmp}
A randomized algorithm $A$ is $\gamma$-extended uniformly stable if
\begin{enumerate}[(a)]
\item $A$ is $\gamma$-uniformly stable, i.e., 
\begin{equation}
    \sup_{\substack{S,S' \in \cZ^n\\S \setminus S'=1}} \sup_{z \in \cZ} \E_A \big[ \ell(A(S),z) - \ell(A(S'),z) \big] \leq \gamma~.
    \label{eq:us}
\end{equation}
\item $A$ is $\gamma$-training set stable, i.e.,
\begin{equation}
    \sup_{S,S'_i \in \cZ^n} \E_A \big[ \ell(A(S),z_i) - \ell(A(S'_i),z'_i) \big] \leq \gamma~.
    \label{eq:tss}
\end{equation}
\end{enumerate}
\label{asmp:us}
\end{asmp}
Note that \eqref{eq:us} is standard uniform stability (US). We call \eqref{eq:tss} training set stability (TSS), as it measures the change in training set loss on $z_i$ when it is swapped with an independent copy $z'_i$ before training. TSS is arguably a more benign assumption as it involves only the training set. For example, recent work on over-parameterized models show that they interpolate the training set, which would imply TSS. For squared loss, interpolation achieves zero training set loss on each $z_i$; for logistic loss, interpolation can achieve desired low loss (say, $\gamma$) if one continues training [][][].  

\begin{lemm}
Under Assumption~\ref{asmp:us}, $\| Y - Y'_i \|_{\psi_2} \leq c \gamma \sqrt{n} $, for some absolute constant $c > 0$.
\end{lemm}
\proof \abcomment{Do not read} Note that
\begin{align*}
Y - Y'_i & = \sum_{i=1}^n \E_A \big[  \ell(A(S),z_i) - \E_z [\ell(A(S),z) ]\big] - \left( \sum_{i=1, i\neq i'}^n \E_A \big[  \ell(A(S'_i),z_i)] + \ell(A(S'_i),z'_i) - \E_z [\ell(A(S'_i),z) ]\big] \right) \\
& = \sum_{j=1,j\neq i}^n  \E_A \bigg[ \big(\ell(A(S),z_j) - \ell(A(S'_i),z_j)\big) \bigg] + \big( \ell(A(S),z_i) - \ell(A(S'_i),z'_i) \big) -  n (\E_z [\ell(A(S),z) - \ell(A(S'_i),z)]  \\
& = \sum_{i=1}^n U_i(S,S'_i)~,
\end{align*}
where 
\begin{align*}
U_i(S,S'_i) & = \E_A \bigg[ \big(\ell(A(S),z_i) - \ell(A(S'_i),z'_i)\big)  -  \E_z [\ell(A(S),z) - \ell(A(S'_i),z) ] \bigg] ~.
\end{align*}

\abcomment{Check this argument, need not be correct} Note that $U_i(S,S')$ is a symmetric random variable since (i) $\ell(A(S),z_i)$ and $\ell(A(S'_i,z'_i)$ are identically distributed, and (ii) $\E_z [\ell(A(S),z)]$ and $\E_z [\ell(A(S'_i),z)]$ are also identically distributed. So, $U_i(S,S'_i)$ is identically distributed as $U_i(S'_i,S)$. Further, for an independent Rademacher random variable $\varepsilon_i$, $U_i(S,S'_i)$ is identically distributed as $\varepsilon_i U_i(S,S'_i)$. Finally, note that swapping $Z_i$ and $Z'_i$ does not change the distribution of $U_{j}(S,S'_j)$ for $j \neq i$, and the distribution of $\sum_{j\neq i} U_{j}(S,S'_j)$. As a result, $(Y-Y'_i)$ is identically distributed as $\sum_{i=1}^n \varepsilon_i U_i(S,S'_i)$, i.e.,
\begin{align*}
  \sum_{i=1}^n U_i(S,S'_i) \sim  \sum_{i=1}^n \varepsilon_i U_i(S,S'_i)~.
\end{align*}


\abcomment{if the above is correct, we know how to do the rest [not written out fully]}
Let $\varepsilon = (\varepsilon_1,\ldots,\varepsilon_n)$ where $\varepsilon_i, i=1,\ldots,n$ are independent Rademacher random variables. Then, for any $p \geq 1$,
\begin{align*}
\| Y - Y'_i \|_p^p & =  \E_{S,S'}|Y - Y'_i|^p  
  =  \E_{S,S'}\left|\sum_{i=1}^nU(S,S'_i)\right|^p  \\
& =  \E_{S,S',\varepsilon}\left|\sum_{i=1}^n \varepsilon_i U(S,S'_i)\right|^p 
  =  \E_{S,S'}  \E_{\varepsilon} \left[\left|\sum_{i=1}^n \varepsilon_i U(S,S'_i)\right|^p \bigg| S,S' \right]  
\end{align*}
Focusing on the conditional expectation, for any fixed realization of $S,S'$, by Khintchine's inequality we have
\begin{align*}
\E_{\varepsilon} \left|\sum_{i=1}^n \varepsilon_i U(S,S'_i)\right|^p \leq c_0^p p^{p/2} \left[ \sum_{i=1}^n |U(S,S'_i)|^2 \right]^{p/2}~,
\end{align*}
where $c_0$ is an absolute constant.

\abcomment{ongoing ...} \qed 

The desired operating regime for the uniform stability assumption (Assumption~\ref{asmp:us}) is $\gamma \lesssim \frac{1}{\sqrt{n}}$ [][][], and in this operating regime, the uniorm stability assumption (Assumption~\ref{asmp:us}) implies the sub-Gaussian assumption (Assumption~\ref{asmp:subg}).


\begin{corr}
If a randomized algorithm $A$ is $\gamma$-uniformly stable with $\gamma \lesssim \frac{1}{\sqrt{n}}$, then $\| Y - Y'_i \|_{\psi_2} \leq \kappa$ for some absolute constant $\kappa > 0$.
\end{corr}
\end{comment}

==> Arxiv(old)/sec/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  %For example:
% % \begin{itemize}
% %   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
% %   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% %   \item Did you include the license to the code and datasets? \answerNA{}
% % \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerTODO{}
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerTODO{}
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    % \answerTODO{}
    \answerYes{}
    %See %Appendix~\ref{sec:app_tsgd},~\ref{sec:app_opt}, and \ref{sec:app_gen}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See our supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes
    %{See Section~\ref{sec:experiments} and Appendix~\ref{sec:app_exp}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> Arxiv(old)/sec/conc.tex <==

Inspired by recent advances in stability based and information theoretic approaches to generalization bounds [Mou et al][Pensea et al.][Negrea et al][Li et al][Hegifam et al], we have presented a framework for developing such bounds based on expected stability for noisy stochastic iterative (NSI) learning algorithms. Further, we have simplified the task to one of bounding expected for the NSI algorithm. We have developed a specific bound for SGD with Gaussian noise which inherits strengths of a variety of existing results and quantitatively outperforms them based on preliminary experiments. We have also developed similar bounds for SGD with exponential family noise, which seem to be the first result of this type. Our work also highlights few key directions for future work, including sharper notions of gradient discrepancy/incoherence and better understanding of the trade-offs between stability and optimization for NSI algorithms.

==> Arxiv(old)/sec/exp.tex <==
\begin{figure*}[t] 
\centering
  \subfigure[CNN, $\sigma_t = 10^{-3}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/grad_mnist_cnn_lr2.png}
 } 
  \subfigure[CNN, $\sigma_t = 10^{-3}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha3mo0_mnist_cnn.png}
 }  
  \subfigure[CNN, $\sigma_t = 10^{-4}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_mnist_cnn.png}
 }  
  \subfigure[MLP, $\sigma_t = 10^{-4}$ ]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_mnist_fnn.png}
 }
  \subfigure[CNN, $\sigma_t = 10^{-3}$]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/grad_fashion_cnn_lr2.png}
 }
  \subfigure[CNN, $\sigma_t = 10^{-3}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha3mo0_fashion_cnn.png}
 }  
   \subfigure[CNN, $\sigma_t = 10^{-4}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_fashion_cnn.png}
 }  
  \subfigure[MLP, $\sigma_t = 10^{-4}$]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_fashion_fnn.png}
 }
\caption[]{Numerical results for MNIST (a-d) and Fashion MNIST (e-h) with CNN and MLP. All x-axes show the number of Epochs of training. Figure (a) (MNIST)  and (e) (Fashion MNIST) show the key factors in the bounds, i.e., gradient norms in \cite{Li2020On}, gradient incoherence in \cite{negrea2019information}, gradient discrepancy in our bound. Figure (b-d) and (f-h) compare our bound with the existing bounds for small noise variance, i.e., $\sigma_t^2 = 10^{-4}$ and large  variance i.e., $\sigma_t^2 = 10^{-3}$ for CNN, and MLP, demonstrating that our bounds are numerically sharper than the existing bounds. Figure (b-c) and (f-g) suggest that increasing noise variance leading to smaller generalization bounds which is consistent with the theoretical analysis.
}
\label{fig:mnist}
\end{figure*}





In this section, we conduct a series of experiments to evaluate the generalization error bounds. We aim to compare the proposed  bound in Theorem \ref{theo:guss_gen} with the existing bounds in \cite{Li2020On} and  \cite{negrea2019information} for various datasets, model structures and noise scales. Note that we do not consider the bound in \cite{haghifam2020sharpened} as a baseline because the bound in \cite{haghifam2020sharpened} only applies to full-batch setting, but we focus on noisy mini-batch gradient descent.
%however the bound in \cite{haghifam2020sharpened} only applies to full-batch setting which is not in the scope of our empirical evaluation. 

\textbf{Experimental setup.} We consider MNIST \cite{mnist} and Fashion-MNIST \cite{fashion-mnist} with a 2- layer convolutional neural networks (CNN) and 3-layer multilayer perceptron (MLP). We use Noisy SGD with Gaussian noise to train the model, i.e., $\mathbf{w}_{t}=\mathbf{w}_{t-1}-\eta_{t} \nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)+\boldsymbol{\xi}_{t}, \text { where } \boldsymbol{\xi}_{t} \sim \mathcal{N}\left(0, \sigma_{t}^{2} \mathbb{I}_{d}\right)$.
We use constant learning rate $\eta_t = 0.001$ and batch size $|B_t| = 128$ for all datasets, and minimize cross-entropy loss for a fixed number of epochs. We consider small and large noise variance for $\sigma_t$, i.e., $\sigma_t \in \{10^{-4},, 10^{-3}\}$. We repeat each experiment for 20 runs. 

\textbf{Experimental results.} We derive theoretical generalization error bounds that depend on the data-dependent quantity \emph{gradient discrepancy}, i.e., $\|\ell(\w,z) - \ell(\w,z^\prime)\|$. We acknowledge that existing bounds in \cite{Li2020On} and \cite{negrea2019information} also
have improved the Lipschitz constants in \cite{mou2018generalization} to a data-dependent quantity. Since the first key difference between our bound and others is that we replace the \emph{gradient norms}, i.e., $\frac{1}{n}\sum_{z \in S}\|\ell(\w,z)\|$ in \cite{Li2020On} and \emph{gradient incoherence} in  \cite{negrea2019information} with
gradient discrepancy. We report those data-dependent quantities in Figure \ref{fig:mnist} (a) and 
(b) for MNIST and Fashion MNIST respectively. The results suggest that the gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors, and the gradient incoherence in \cite{negrea2019information} is much smaller than the gradient discrepancy in our bound as well. 
However, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$ which has a worse sample dependence compared to our bound. The results in (b-d) for MNIST and (f-h) for Fashion MNIST show that our bounds are much sharper than those of \cite{negrea2019information} due to improving the dependence on $n$ from a order of $\frac{1}{\sqrt{n}}$ to $\frac{1}{n}$. Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to those for CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases, leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence. We 
note that  \cite{haghifam2020sharpened} show that Negrea et al. bound is smaller than Li et al. in their empirical evaluation, which is opposite to what we observed in Figure \ref{fig:mnist}.
We think this is because \cite{haghifam2020sharpened} consider the full-batch setting which has a different form of gradient incoherence compared to the mini-batch setting in our paper. \yzcomment{added the discussion about the inconsistent of our result and \cite{haghifam2020sharpened}}


% The second key difference is the order of dependence on the sample size $n$, i.e., both of our bound and $\cite{Li2020On}$ has a bound of order $\frac{1}{n}$, however, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$. 
%Figure \ref{fig:mnist} (a) and 
% (b) suggests that the gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors, and the gradient incoherence in \cite{negrea2019information} is much smaller than the gradient discrepancy in our bound as well.
% However, the results in (b-d) for MNIST and (f-h) for Fashion MNIST show that our bounds are much sharper than those of \cite{negrea2019information} due to improving the dependence on $n$ from a order of $\frac{1}{\sqrt{n}}$ to $\frac{1}{n}$. Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence.


More details of our model architectures and addtional experimental results can be found in Appendix. 
We acknowledge that we did not aim to achieve the state-of-the art predictive performance. With further tuning, the prediction results could be improved.

% \begin{figure*}[t] 
% \centering
%  \subfigure[CNN for F-MNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/grad_fashion_cnn_lr2.png}
%  }
%   \subfigure[CNN for F-MNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha3mo0_fashion_cnn.png}
%  }  
%   \subfigure[CNN for F-MNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_fashion_cnn.png}
%  }  
%   \subfigure[MLP for F-MNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_fashion_fnn.png}
%  }
% \caption[]{$\eta = 0.001$, $\sigma = 0.001$, repeat = 20
% }
% \label{fig:fashion}
% \end{figure*}


% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN for MNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/lr3alpha3mo0_mnist_cnn.png}
%  }  \vspace{-2mm}
%   \subfigure[MLP for MNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/lr3alpha3mo0_mnist_fnn.png}
%  }\vspace{-2mm}
% \caption[]{$\eta = 0.001$, $\sigma = 0.001$, repeat = 20
% }\vspace*{-2mm}
% \label{fig:mnist_large_sigma}
% \end{figure*}



% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN for FashionMNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/lr3alpha4mo0_fashion_cnn.png}
%  }  \vspace{-2mm}
%   \subfigure[MLP for FashionMNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/lr3alpha4mo0_fashion_fnn.png}
%  }\vspace{-2mm}
% \caption[]{$\eta = 0.001$, $\sigma = 0.0001$, repeat = 20
% }\vspace*{-2mm}
% \label{fig:mnist_small_sigma}
% \end{figure*}



% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN for MNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/grad_mnist_cnn_lr2.png}
%  }  \vspace{-2mm}
%   \subfigure[CNN for FashionMNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/grad_fashion_cnn_lr2.png}
%  }\vspace{-2mm}
% \caption[]{$\eta = 0.001$, $\sigma = 0.001$, repeat = 20
% }\vspace*{-2mm}
% \label{fig:mnist_large_sigma}
% \end{figure*}



==> Arxiv(old)/sec/gen_stability.tex <==

In the setting of statistical learning, there is an instance space $\cZ$, a hypothesis space $\cW$, and a loss function $\ell : \cW \times \cZ \mapsto \R_+$. Let $D$ be an unknown distribution of $\cZ$ and let $S \sim D^n$ be $n$ i.i.d.~draws from $D$. For any specific hypothesis $\w \in \cW$, the population and empirical loss are respectively given by
\vspace*{-3mm}
\begin{equation}
L_D(\w) \triangleq \E_{z \sim D}[\ell(\w,z)]~, \qquad \text{and} \qquad  L_S(\w) \triangleq \frac{1}{n} \sum_{i=1}^n \ell(\w,z_i)~.   
\vspace*{-3mm}
\end{equation}
\\For any distribution $P$ over the hypothesis space, we respectively denote the expected population and empirical loss as
\vspace*{-3mm}
\begin{equation}
L_D(P) \triangleq \E_{z \sim D}\E_{\w \sim P}[\ell(\w,z)]~, \qquad \text{and} \qquad  L_S(P) \triangleq \frac{1}{n} \sum_{i=1}^n \E_{\w \sim P}\ell(\w,z_i)~.
\vspace*{-3mm}
\end{equation}
\\Consider a randomized algorithm $A$ which works with $S =\{z_1,\ldots,z_n\} \sim D^n$ and creates a distribution over the hypothesis space $\cW$. For convenience, we will denote the distribution as $A(S)$. The focus of the analysis is to bound the generalization error of $A$ defined as:
\begin{align}
\gen(A(S)) \triangleq L_D(A(S)) - L_S(A(S))~.    
\end{align} 
We will assume $A$ is permutation invariant, i.e., the ordering of samples in $S$ do not modify $A(S)$, an assumption satisfied by most learning algorithms. We will primarily focus on developing bounds for the expectation $\E_S[L_D(A(S)) - L_S(A(S))]$, and subsequently discuss high-probability bounds.
%\abcomment{mention that $A$ is assumed to be permutation invariant}




\subsection{Bounds based on Expected Stability}
% For our analysis, we assume that the $L_2$ norm of the loss is bounded:
% \begin{asmp}
% Let $c_{\ell_2}(z) = \E_{w \sim  p_{A(S)}}[\ell^2(w,z)]$. Two options:
% \begin{enumerate}
% \item Uniform bound: $\forall z$, $c_{\ell_2}(z) \leq c_0$.
% \item Expectation bound: $\E_{z \sim D}[c_{\ell_2}(z)] \leq c_0$ \abedit{and $\E_{z \sim S}[c_{\ell_2}(z)] \leq c_0$}.
% \end{enumerate}
% The analysis would look different depending on which one we choose. \abcomment{Discuss}
% \end{asmp}
% \abcomment{need a discussion on assumptions for info-theoretic analysis}

We start our analysis by noting that the expected generalization error can be upper bounded by stability based on the Hellinger divergence~\cite{save16,Li2020On}: $H^2(P\| P') = \frac{1}{2}\int_{\w} (\sqrt{p(\w)} - \sqrt{p'(\w)})^2 d\w$.
\begin{restatable}{prop}{prophell}
Let $S \sim D^n$ and let $S'_{n}$ be a dataset obtained by replacing $z_n \in S$ with $z'_n \sim D$. Let $A(S),A(S'_{n})$ respectively denote the distributions over the hypothesis space $\cW$ obtained by running randomized algorithm $A$ on $S,S'_{n}$.
Assume that for any $S \sim D^n, z \in \cZ$, $\E_{\w \sim  A(S)}[\ell^2(\w,z)] \leq c_0/2, c_0>0$. Then, with $H(\cdot,\cdot)$ denoting the Hellinger divergence, we have
\begin{equation}
| \E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))] | \leq c_0 \E_{S \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S), A(S'_{n})\big)}~. 
\end{equation}
\vspace*{-6mm}
\label{prop:hell}
\end{restatable}
Note that the result does not need the loss function to be bounded, but just the second moment of $\ell(\w,z), \w \sim A(S)$ to be bounded for any $z \in \cZ$. The assumption is satisfied by bounded losses. It is also instructive to compare the assumption to that in recent information theoretic bounds~\cite{haghifam2020sharpened,xu2017information}, where one assumes $\ell(\w,z), z \sim D$ to be sub-Gaussian for any $\w \in \cW$.

Next, we note that the Hellinger divergence can be bounded by the KL-divergence, so we focus on bounding the KL divergence in the sequel. 
\begin{restatable}{prop}{prophellkl}
For any two distributions $P$ and $P'$, we have
\begin{equation}
    2 H^2(P,P') \leq \min \bigg\{ KL(P,P'),\sqrt{\frac{1}{2}KL(P,P')} \bigg\}~.
\end{equation}
\vspace*{-6mm}
\label{prop:hellkl}
\end{restatable}





\subsection{Noisy Stochastic Iterative Algorithms: The Mixture Model Perspective}

We consider a general family of noisy stochastic iterative (NSI) algorithms. Given $S \sim D^n$, such iterative algorithms have two additional sources of randomness in each iteration $t$: (a) a stochastic mini-batch of samples $S_{B_t}$, with $|S_{B_t}| = b$, drawn uniformly at random with replacement from $S$; and (b) noise $\bxi_t$ suitably included in the iterative update. Given a trajectory of past iterates $\w_{0:(t-1)}$, the new iterate $\w_t$ is drawn from a distribution $P_{B_t,\bxi_t,\w_{0:(t-1)}}$ over $\cW$:
\begin{align}
\w_{t} \sim P_{B_t,\bxi_t|\w_{0:(t-1)}} = f_t(B_t,\bxi_t,\w_{0:(t-1)})~,
\label{eq:nmia}
\end{align}
for some suitable function $f_t$. We will often drop the conditioning $\w_{0:(t-1)}$ to avoid clutter and represent the distribution as $P_{B_t,\bxi_t}$ in the sequel.
Since our analysis is based on KL-divergence, we assume that the distributions $P_{B_t,\bxi_t}$ are absolutely continuous with respect to each other. \abcomment{need to be more precise}

From Propositions~\ref{prop:hell} and \ref{prop:hellkl}, to get a bound on the expected generalization of such NSI algorithms, it suffices to focus on the KL-divergence between $A(S)$ and $A(S'_{n})$. Let $P_T, P'_T$ denote the distributions over hypotheses $\w \in \cW$ after $T$ steps of the algorithm based on $S,S'_{n}$ respectively. 
% \abdelete{i.e., $P_T = A(S)$ and $P'_T = A(S'_{(n)})$.} 
Further, let $P_{0:(t-1)}$ denote the joint distribution over $\w_{0:(t-1)} = (\w_0,\ldots,\w_{t-1})$, and let $P_{t|} \equiv P_{B_t,\bxi_t}$ denote the conditional distribution conditioned as $\w_{0:t-1}$. We will use the following chain rule for KL-divergence which has been effectively used in recent advances in information theoretic bounds for generalization~\cite{negrea2019information,haghifam2020sharpened,pensia2018generalization}:
\vspace*{-2mm}
\begin{equation}
KL(P_T \| P'_T) \leq KL(P_{0:T} \| P'_{0:T} ) = \sum_{t=1}^T P_{0:(t-1)}\left[ KL(P_{t|} \| P'_{t|}) \right]~.
\label{eq:klchain}
\end{equation}
Note that the analysis which follows also apply to such information theoretic bounds~\citep{negrea2019information,haghifam2020sharpened,pensia2018generalization}.

We present a mixture model perspective for $P_{t|},P'_{t|}$ following [Li et al.]. Consider sampling $\bar{S} \sim D^{n+1}$. Let $S,S'_{n}$ be size $n$ subsets of $\bar{S}$ such that $S=\{Z_1,\ldots,Z_{n-1},Z_n\}$ and $S'_{n} = \{Z_1,\ldots,Z_{n-1},Z'_n\}$, where $Z'_n = Z_{n+1}$. Let $S_0 = \{Z_1,\ldots,Z_{n-1}\}$. The algorithms we consider use a mini-batch of size $b$ in each iteration. Let the set of all mini-batches be denoted by $G$. Let the set of all mini-batches drawn from $S_0$ be denoted by $G_0$. Note that $|G_0| = \binom{n-1}{b}$. Let the set of all mini-batches which includes the last sample, viz.~$z_n$ for $S$ and $z'_n$ for $S'_n$, be denoted by $G_1$. Note that $|G_1| = \binom{n-1}{b-1}$. Also note that 
%\begin{align*}
$|G_0| + |G_1| = \binom{n-1}{b} + \binom{n-1}{b-1} = \binom{n}{b} = |G|$.
%\end{align*}
%the total number of $b$-sized mini-batch samples from a dataset of size $n$. \abcomment{The subsets of $S$ and $S'_{(n)}$ corresponding to mini-batch $B$ will be denoted as $S_B$ and $S'_B$.}

We focus on bounding $KL(P_{t|} \| P'_{t|})$. 
For for a given $\w_{0:(t-1)}$ and a fixed mini-batch $B_t$, following \eqref{eq:nmia}, let $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively be distributions over $\cW$ corresponding to $S, S'_{n}$. Then, $P_{t|}$ and $P'_{t|}$ can be viewed as mixture models with shared components~\citep{Li2020On}:
%due to the randomness in $\bxi_t$. 
\begin{restatable}{prop}{mixmodel}
Consider the mixture models 
%\begin{align*}
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  
%\end{align*}
Then, with 
%\begin{equation*}
$s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}$,
%\end{equation*}
we have 
\begin{align*}
    P_{t|} = s Q_{t|} + (1-s) R_{t|}~, \qquad \text{and} \qquad P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~.
\end{align*}
\label{prop:mixmodel}
\vspace*{-6mm}
\end{restatable}
%Thus, $P_{t|}$ and $P'_{t|}$ are each mixture models with (a set of) shared components $R_{t|}$

% Consider two collection of points $\{\mu_B : B \in G \}$ and $\{\mu_B : B \in G\}$. In our context, at any stage $t$, for mini-batch $B$ and step specific randomness $\bxi_t$, \yzcomment{$S_B$ is random due to the random draw of mini-batch. What is randomness $\bxi_t$? example of $\bxi_t$? } we have 
% \begin{align*}
%     \w_t \sim P_{\mu_B,t} where \qquad  \mu_B = \E[f_t(w_{1:t-1},S_B, \bxi_t)]
% \end{align*}
% \abcomment{highlight the fact that $f_t$ can be general, may depend on the entire trajectory, etc.} \abcomment{DISCUSS -- examples}
% Let $p_{\mu,\sigma}$ denote the Gaussian distribution $\cN(\mu, \sigma^2 \I)$. Let $P = \frac{1}{|G|} \sum_{B \in G} p_{\mu_B,\sigma}$ and  $P' = \frac{1}{|G|} \sum_{B \in G} p_{\mu'_B,\sigma}$. Our goal is to bound $KL(P \| P')$ {\em without making any additional assumptions}. Note that $\eta_t,\sigma_t$ can depend on $w_{1:t-1}$, but since the analysis is conditioned on $w_{1:t-1}$, these are effectively constants for the current analysis. 

% \abcomment{This analysis immediately shows why KL-divergence cannot be used for the non-noisy case -- these will be Dirac measures, and KL-div will be $\infty$. A bound based on TV or Hellinger would still be valid.}

% Let 
% \begin{align*}
% Q_1 = \frac{1}{|G_1|} \sum_{B \in G_1} p_{\mu_B,\sigma} \qquad Q_2 = \frac{1}{|G_1|} \sum_{B \in G_1} p_{\mu'_B,\sigma} \qquad R = \frac{1}{|G_0|} \sum_{B \in G_0} p_{\mu_B,\sigma}~.  
% \end{align*}
% Then, with 
% \begin{equation*}
% s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}~,
% \end{equation*}
% we have 
% \begin{align*}
%     P = s Q_1 + (1-s) R \qquad P' = s Q_2 + (1-s) R~.
% \end{align*}


\subsection{Bounds with Le Cam Style Divergence (LSD)}
The mixture model structure in $P_{t|}, P'_{t|}$ can be utilized to bound their KL-divergence in terms of Le Cam Style Divegence (LSD). While the classical Le Cam divergence~\cite{save16} is $LCD(P\|P') = \frac{1}{2} \int \frac{(dP - dP')^2}{dP + dP'}$ (where $dP$ denotes the density), given the mixture model structure in $P_{t|}, P'_{t|}$ in Proposition~\ref{prop:mixmodel}, we get our bounds in terms of  $\int \frac{(dP_{B,\bxi} - dP'_{B,\bxi})^2}{dP_{A}(\bxi)}, B \in G_1, A \in G_0$, %\yzcomment{$P_B(\bxi)$ should be  $dP_{B_t,\bxi_t}$? }\abcomment{fixed}
which we call LSD. 
[Li et al.] pursued a similar route for SGLD, but our proofs are significantly more simple and illustrates applicability of LSD to general NSI algorithms, not just SGLD. 
Putting Propositions~\ref{prop:hell} and \ref{prop:hellkl}, and \eqref{eq:klchain} together, with some additional analysis we have the following LSD based generalization bound: 
\begin{restatable}{theo}{theostab}
Consider a noisy stochastic iterative algorithms of the form~\eqref{eq:nmia} with mini-batch size $b \leq n/2$. Then, with $c = \sqrt{2} c_0$, we have
\vspace*{-2mm}
\begin{equation}
\hspace*{-5mm}
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq c\frac{b}{n} \E_{S} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \E_{\w_{0:(t-1)}}\E_{B_t \in G_1} \E_{A_t \in G_0} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t}(\bxi_t)} d\bxi_t \right] }~.
\end{equation}
\label{theo:stab}
\vspace*{-6mm}
\end{restatable}
%A few properties of the bound can be immediately notes: 
Note that the bound holds for any NSI algorithm of the form~\eqref{eq:nmia}, does not assume the loss to be bounded, depends on expectations over samples, trajectories, and mini-batches, and does not depend on any uniform assumptions. Further, as an expected stability based bound to generalization error, the bound depends on the distribution discrepancy as captured by the expected LSD. 

%Qualitatively, even if we assume that each term in $\sum_t$ is bounded by a constant

%In Sections~\ref{sec:stab_gauss}

%\abcomment{We are still missing an overall bound by combining (4)-(7)}

%The analysis upto this point does not need the distributions to be Gaussian.




\subsection{High Probability Bounds}
\label{sec:highp}
\input{sec/high_prob}

==> Arxiv(old)/sec/high_prob.tex <==

Let $S \sim D^n$ with $S=(Z_1\ldots,Z_n)$ corresponding to the training data. Consider the random variable $Y(S)$, the Scaled (by $n$) Generalization Error (SGE), defined as
\begin{align}
Y(S) \triangleq \sum_{i=1}^n \E_A \big[  \E_{Z \sim D} [\ell(A(S),Z) ] - \ell(A(S),Z_i) \big] = n\big(L_D(A(S)) - L_S(A(S))\big) ~.
\end{align}
%where $A(S)$ is the distribution over $\cW$ due to randomized algorithm $A$ run on $S$.
Theorem~\ref{theo:stab} establishes a bound on $|\frac{1}{n}\E_S[Y(S)]|$. We now focus on establishing a high probability bound on $\frac{1}{n}(Y(S)-\E_S[Y(S)])$. Let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. Further, let $S'_i = (Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, the change in SGE
\begin{equation}
Y(S) - Y(S'_i) = n \big[ \big( L_D(A(S)) - L_D(A(S'_i)) \big) - \big( L_S(A(S)) - L_{S'_i}(A(S'_i) \big) \big]    
\end{equation}
is a symmetric random variable, and is identically distributed for $i=1,\ldots,n$.
% \begin{align}
% Y(S) - Y(S'_i) = \sum_{j=1}^n \E_A \big[ \ell(A(S'_i),Z_j) - \ell(A(S),Z_j) \big] = n \big(L_{S'_i}(A(S'_i) - L_S(A(S)) \big)
% \end{align}
%Note that $(Y-Y'_i)$ \abedit{is symmetric} and are identically distributed for any $i$. 
Our analysis is based on the following assumption: %\abcomment{cite for $\psi_2$ norm} 
\begin{asmp}
The random variable $(Y(S)-Y(S'_i))^2$ is sub-Gaussian with $\psi_2$-norm $\kappa_A^2$, i.e., $\| (Y-Y'_i)^2 \|_{\psi_2} = \sup_{q \geq 1} (\E_{S.S'}|Y(S)-Y(S'_i)|^{2q})^{1/q}/\sqrt{q} = \kappa_A^2$. 
%has bounded second moment, i.e., $\E_{S,Z'_i}[(Y(S)-Y(S'_i))^2] \leq \nu_A$, for some constant $\nu_A$.\abcomment{should this be a definition? i.e., just call the second moment $\nu_A$?}
\label{asmp:2moment}
\end{asmp}
Assumption~\ref{asmp:2moment} implies that $\|Y-Y'_i\|_{\psi_2} \leq \kappa_A$.
Note that since $Y(S) - Y(S'_i)$ is identically distributed for all $i$, $\kappa_A$ is the same for all $i$. Further, $\kappa_A$ is a property of the algorithm $A$, and can be viewed as a measure of stability.
If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered stable; on the other hand, if $\kappa_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as typical generalization error $\frac{1}{n}Y(S)$ itself. The sharpness of the high-probability bound we present meaningfully depends on $\kappa_A$, with smaller values implying sharper bounds.



\begin{restatable}{theo}{theohighp}
Under Assumption~\ref{asmp:2moment}, with probability at least $(1-\delta)$ over the draw $S \sim D^n$, we have
\begin{equation}
L_D(A(S)) \leq L_S(A(S)) + \E_S\bigg[L_D(A(S) - L_S(A(S))\bigg] + \max\left( \frac{1}{n}, \frac{ c_1 \kappa_A}{\sqrt{n}} \right) \log \left(\frac{16}{\delta} \right)~.      
\end{equation}
\label{theo:hp}
\vspace*{-5mm}
\end{restatable}


==> Arxiv(old)/sec/intro.tex <==


Recent years have seen renewed interest and advances in characterizing generalization performance of learning algorithms in terms of stability, which considers change in performance of a learning algorithm based on change of a single training point \citep{hardt2016train,bousquet2002stability,Li2020On,mou2018generalization}. For stochastic gradient descent (SGD), \cite{hardt2016train} established generalization bounds based on uniform stability \citep{hardt2016train,bousquet2002stability}, although the analysis needed rather small step sizes $\eta_t = 1/t$ which is not useful in practice. While improving the analysis for SGD has remained a challenge, advances have been made on noisy SGD algorithms such as stochastic gradient Langevin dynamics (SGLD) \citep{mou2018generalization,Li2020On}. In parallel, there has been key developments on related information-theoretic generalization bounds applicable to SGLD type algorithms \citep{negrea2019information,haghifam2020sharpened,xu2017information,russo2016controlling, pensia2018generalization}.

While these developments have led to major advances in analyzing generalization of noisy SGD algorithms, they each have certain limitations which leave room for further improvements. Using uniform stability, \cite{mou2018generalization} established a bound for SGLD of the form $\frac{L}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ which depends on $L$, the Lipschitz constant for the gradient, and the step size $\eta_t \leq \frac{\sigma_t \ln 2}{L}$. The bound has a desirable dependency of $O(\frac{1}{n})$ on the samples, but has an undesirable dependence on $L$, and the step sizes, bounded by $\frac{\sigma_t}{L}$, are too small. \cite{mou2018generalization} also presented another bound which addresses some of these issues, but gets an undesirable $O(\frac{1}{\sqrt{n}})$ sample dependence. \cite{Li2020On} made advances on such results based on Bayes-stability, and got a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \g_e(t)/\sigma_t^2}$, where $\g_e(t)$ is the expected gradient norm square at step $t$. While the bound avoids dependency on $L$ with expected gradient norm, as shown in the information theoretic bounds of \cite{negrea2019information,haghifam2020sharpened}, the dependency can be potentially be improved to some measure of gradient incoherence. Further, the analysis of \cite{Li2020On} still needs small step sizes, bounded by $\frac{\sigma_t}{L}$. By building on the developments of \cite{russo2016controlling,xu2017information,pensia2018generalization}, \cite{negrea2019information} made advances from the information theoretic perspective and established bounds for SGLD which have the desirable dependence on gradient discrepancy, but has an undesirable $O(\frac{1}{\sqrt{n}})$ sample dependence. \cite{haghifam2020sharpened} also approached the problem from an information theoretic perspective and obtained bounds based on gradient incoherence with $O(\frac{1}{n})$ sample dependence, but their analysis holds for full batch Langevin dynamics, not mini-batch SGLD.

In this paper, we build on the strengths of these stability based and information theoretic approaches to develop a general framework (Section~\ref{sec:gen}) for analyzing stability of noisy stochastic iterative (NSI) algorithms, which include SGLD as an important special case. Our framework considers generalization based on the concept of {\em expected stability}, rather than uniform stability \citep{mou2018generalization,hardt2016train,bousquet2002stability, bousquet2020sharper}, and arguably puts less demands on the assumptions needed to analyze NSI algorithms. We show that expected stability can be bounded by KL-divergence between posterior distribution over hypothesis from training sets differing in one point, connecting our analysis to the information theoretic approach initiated by \cite{pensia2018generalization} and followed by \cite{negrea2019information,haghifam2020sharpened}. Building on the developments of \cite{Li2020On}, we show that posterior distribution for general NSI algorithms can be viewed as mixture models, and the KL divergence over posteriors can be bounded by the expectation of Le Cam Style Diveregnces (LSD). For any specific NSI algorithm, the task then reduces to suitable bounding the expected LSD. While our analysis mainly focuses on expected generalization \cite{Li2020On,mou2018generalization,negrea2019information,haghifam2020sharpened}, we show that one get high probability generalization bounds under suitable assumptions. 

In Section~\ref{sec:stab_gauss}, we apply the expected stability approach to SGLD by suitably bounding the expected LSD  for Gaussian noise. The resulting bound inherits the strengths of the existing bounds with dependence on norms of gradient discrepancy, no dependence on $L$, flexible data dependent choices for $\eta_t,\sigma_t$, and a $O(\frac{1}{n})$ sample dependence. The concept of gradient incoherence in \cite{negrea2019information,haghifam2020sharpened} and our gradient discrepancy are mildly different, but they all qualitatively capture a much more desirable and quantitatively smaller quantity compared to the gradient norm in \cite{Li2020On}. Conceptually, gradient discrepancy norm captures the notion of stability, which the gradient norm does not. The crux of the technical argument in our analysis relies on an approach to bounding the LSD based on an application of mean-value theorem and a careful approach to handle density ratios. We briefly discuss the relationship of our bound for mini-batch SGLD with \cite{mou2018generalization,Li2020On,negrea2019information}, and demonstrate how our bound picks up most of the strengths of each while avoiding the weakness. 
%Further, we show that the gradient incoherence of \cite{negrea2019information} are quantitatively smaller than our gradient discrepancy, but our bounds are tighter because of the $O(\frac{1}{n})$ sample dependence compared to the $O(\frac{1}{\sqrt{n}})$ sample dependence of \cite{negrea2019information}. 

In Section~\ref{sec:stab_exp_family}, we establish expected stability based generalization bounds for mini-batch stochastic gradient descent with exponential family noise. The result is an important technical extension to existing work on SGLD and, to the best of our knowledge, the first result of its type. The extension also illustrates the power of our framework as we only needed to bound the expected LSD for exponential family noise. The technical argument for bounding the expected LSD for general exponential families are a bit more involved compared to the Gaussian case. As in the case of SGLD with Gaussian noise, the bounds with exponential family noise also depends on the gradient discrepancy, have data dependent flexibly on the choices  of $\eta_t,\sigma_t$, and a $O(\frac{1}{n})$ sample dependence.  

In Section~\ref{sec:experiment}, we empirically verify the sharpness of our bounds for SGLD in comparison to \cite{Li2020On,negrea2019information} on standard benchmarks (MNIST, Fashion-MNIST) using both multi-layer perceptrons (MLPs) and convolution neural networks (CNNs). For both datasets, both models, and for the entire range of training epochs in each setting, our bounds are shown to be substantially smaller than that of \cite{Li2020On}\cite{negrea2019information}. Interestingly, gradient incoherence of \cite{negrea2019information} is quantitatively smaller than our gradient discrepancy, but our bounds are tighter because of the $O(\frac{1}{n})$ sample dependence compared to $O(\frac{1}{\sqrt{n}})$ of \cite{negrea2019information}. We present additional empirical results and all technical proofs in the Appendix.



% {\bf Post on April 9 [slack]:} A tentative task assignment for the near term — lets see if we can meet next Fri:
% \begin{itemize}
% \item  Related work on uniform stability of noisy iterative algorithms: @Yingxue
% \item Related work on information theoretic bounds for noisy iterative algorithms: @Tiancong
% \item Related work on generalization bounds for normalizing flows: @robert
% \item Detailed analysis of SGD with Gaussian noise (Section 4): @Yingxue and @Tiancong (pls work out the details based on the sketch)
% \item Validity of assumptions for NF analysis + alternatives (Section 3.3): @Yingxue and @robert
% \item Related work on noisy SGD with Levy processes, stable distributions: @Tiancong
% \item Prelim analysis of noisy SGD with Levy processes: @arindam
% \item Experiments with deep networks, include image-net variants: @Tiancong
% \item Experiments with NFs: @robert
% \end{itemize}

% For the related work, we want
% to have a fine grained exposition, using our notation + language
% differences in (a) assumptions and (b) results w.r.t. our new material



==> Arxiv(old)/sec/noisy_iterative.tex <==









==> Arxiv(old)/sec/notes.tex <==
\subsection{Gaussian Noise: Without Projection}
\abcomment{this is just for reference, will be removed}

If the noise added is Gaussian, then we have
\begin{align*}
I_{A,B}  = \bigintsss_x \frac{ \left(  p_{\mu_B,\sigma} -   p_{\mu'_B,\sigma} \right)^2 }{ p_{\mu_A,\sigma}} dx 
 = \frac{1}{(\sqrt{2\pi} \sigma)^d} \bigints_x \frac{ \bigg( \exp(- \| x - \mu_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \mu'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} dx~,
\end{align*}
where the latter is a full $p$-dimensional integral. For each $x$, we can apply mean-field theorem [][] to get:
\begin{align*}
 \exp(- \| x - \mu_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \mu'_B\|_2^2 / 2\sigma^2 ) 
 & = \bigg\langle \mu_B - \mu'_B , \nabla \exp(- \| x - \tilde{\mu}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
\end{align*}
where $\tilde{\mu}_B = \alpha_x \mu_B + (1-\alpha_x) \mu'_B$, where $\alpha_x \in [0,1]$ depends on $x$. Note that $\| \tilde{\mu}_B\|_2 \leq \max(\|\mu_B\|_2,\|\mu'_B\|_2) \triangleq \bar{\mu}_B$. We have
\begin{align*}
  \nabla \exp(- \| x - \tilde{\mu}_B\|_2^2 / 2\sigma^2) & = \frac{x -\tilde{\mu}_B}{\sigma^2} \exp(- \| x - \tilde{\mu}_B\|_2^2 / 2\sigma^2)~, 
\end{align*}
so that
\begin{align*}
& \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{ \bigg( \exp(- \| x - \mu_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \mu'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
= \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{\bigg\langle \mu_B - \mu'_B , \frac{x -\tilde{\mu}_B}{\sigma^2} \exp(- \| x - \tilde{\mu}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{\| \mu_B - \mu'_B \|_2^2 \| \frac{x -\tilde{\mu}_B}{\sigma^2} \|_2^2 \exp(- \| x - \tilde{\mu}_B\|_2^2 / \sigma^2) }{\exp(-\| x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{2}{\sigma^4} \| \mu_B - \mu'_B \|_2^2 \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg)  \exp\left(-\frac{\|x-\tilde{\mu}\|_2^2}{\sigma^2} + \frac{\|x\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
= \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{2}{\sigma^4} \| \mu_B - \mu'_B \|_2^2 \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg)  \exp\left( \frac{\|\tilde{\mu}_B\|_2^2}{\sigma^2}\right)  \exp\left(-\frac{\|x-2\tilde{\mu}_B\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
\leq \frac{2}{\sigma^4} \| \mu_B - \mu'_B \|_2^2 \exp\left( \frac{\|\bar{\mu}_B\|_2^2}{\sigma^2}\right) \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg)  \frac{1}{(\sqrt{2\pi} \sigma)^d} \exp\left(-\frac{\|x-2\tilde{\mu}_B\|_2^2}{2\sigma^2} \right) ~.
\end{align*}
% Now, consider the random variable $\tilde{X} \sim \cN(\tilde{\mu}_B, \sigma^2 )$. 
% Note that $\tilde{X}$ is sub-Gaussian with $\| \tilde{X} \|_{\psi_2} \leq c_0 (\sigma^2 + \| \tilde{\mu}_B\|_2^2) \leq c_0 (\sigma^2 + \|\bar{\mu}_B\|_2^2)$, where $c_0$ is an absolute constant. Then \abcomment{this needs to be shown, some variant of this should be true}, for an absolute constant $c_1$ \abcomment{apply Jensen's?}
We have
\begin{align*}
\exp\left(-\frac{\|x-2\tilde{\mu}_B\|_2^2}{2\sigma^2} \right) 
\leq \exp\left(-\frac{\|x-2\mu_B\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2\mu'_B\|_2^2}{2\sigma^2}~, \right) 
\end{align*}
so that
\begin{align*}
\bigintss_x \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg) & \frac{1}{(\sqrt{2\pi} \sigma)^d} \exp\left(-\frac{\|x-2\tilde{\mu}_B\|_2^2}{2\sigma^2} \right) dx \\
& \leq \bigintss_x \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg) \frac{1}{(\sqrt{2\pi} \sigma)^d} \exp\left(-\frac{\|x-2\mu_B\|_2^2}{2\sigma^2} \right) dx \\ 
& \phantom{\leq ......} + \bigintss_x \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg) \frac{1}{(\sqrt{2\pi} \sigma)^d} \exp\left(-\frac{\|x-2\mu'_B\|_2^2}{2\sigma^2} \right) dx \\
& \leq \bigg( d\sigma^2 + 2d\|\mu_B\|_2^2 + \| \bar{\mu}_B\|_2^2 \bigg) + \bigg( d\sigma^2 + 2d\|\mu'_B\|_2^2 + \| \bar{\mu}_B\|_2^2 \bigg) \\
& \leq 2d \big(\sigma^2 + 2\|\mu_B\|_2^2 + 2\|\mu'_B\|_2^2 + \frac{1}{d} \|\bar{\mu}_B\|_2^2 \big)
\end{align*}
Putting everything back together, we have
\begin{align*}
I_{A,B} & \leq \frac{2}{\sigma^4} \| \mu_B - \mu'_B \|_2^2 \exp\left( \frac{\|\bar{\mu}_B\|_2^2}{\sigma^2}\right) 2 \big(d\sigma^2 + 2d\|\mu_B\|_2^2 + 2d\|\mu'_B\|_2^2 + \frac{1}{2} \|\bar{\mu}_B\|_2^2 \big)\\
& \leq 2  \bigg( \frac{d}{\sigma^2} + \frac{d\|\mu_B\|_2^2}{\sigma^4} + \frac{d\|\mu'_B\|_2^4}{\sigma^4} + \frac{ \|\bar{\mu}_B\|_2^2}{2\sigma^4} \bigg) \exp\left( \frac{\|\bar{\mu}_B\|_2^2}{\sigma^2}\right)~~\| \mu_B - \mu'_B \|_2^2~.
\end{align*}
The current analysis without projection ends up getting a dependence on $d$, so that we need $d \leq c_0 \sigma^2$.

==> Arxiv(old)/sec/related.tex <==


\textbf{Uniform stability.} Uniform stability has been a classical approach for bounding generalization error \citep{bousquet2002stability,bousquet2020sharper,feldman2018generalization,feldman2019high}, pioneered by \cite{rogers1978finite,devroye1979distribution}. 
Recently, uniform stability has been shown powerful in analyzing the  stability of SGLD \citep{WellingT11}. \cite{mou2018generalization} prove the uniform stability of SGLD
by showing that the uniform stability can be bounded by the squared Hellinger distance, and further they establish discretized Fokker-Planck equations for analyzing the squared Hellinger distance. Then they provide the uniform stability bound of SGLD as $\frac{L}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ which depends on $L$, the Lipschitz constant for the gradient, and the step size $\eta_t \leq \frac{\sigma_t \ln 2}{L}$ \citep{mou2018generalization,Li2020On}. 
Recently, \cite{Li2020On} follow up on \cite{mou2018generalization} and derive a data-dependent bound using based on Bayes-stability, and got a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \g_e(t)/\sigma_t^2}$, where $\g_e(t)$ is the expected gradient norm square at step $t$. Their bound improves the Lipschitz constant to the expected gradient norm square.  As a special case, SGLD can be viewed as a differentially private SGD algorithm (DP-SGD) with constant noise variance. 
Uniform stability has also been popular in the differential privacy literature for analyzing the generalization error bound of DP-SGD algorithms. 
Recently, \cite{bassily2019private} analyze the uniform stability of DP-SGD for convex optimization by showing the gradient update is a non-expansive operation, which is the key fact in proving the stability of SGD \citep{hardt2016train}. 
The approach in \cite{hardt2016train} can extend to non-convex setting as well, however it requires fast decaying in step size as $\eta_t = O(1/t)$.  \cite{bassily2020stability} provide stability analysis of SGD for convex and non-smooth functions. 

\textbf{Information-theoretic bound.} Besides the works mentioned above, other theories of deriving generalization bounds for noisy iterative algorithms have been proposed via information-theoretic approaches \citep{russo2016controlling, xu2017information}. Such results show that the generalization error of any learning algorithm can be bounded as $O(\sqrt{I(S; \w)/n})$, where $I(S; \w)$ is the mutual information
between the algorithm input $S$ and the algorithm output $\w$. Thus, recent works following this approach focus on bounding the mutual information for a broad class of iterative algorithms, including SGLD  which obtains a $O(\sqrt{\log T/n})$ generalization bound by choosing $\eta_t = O(1/t)$, where $T$ is the total number of iterations~\cite{pensia2018generalization,bu2019tightening}. Subsequent improvements to this technique were made by 
\cite{negrea2019information, haghifam2020sharpened} 
to prove data-dependent generalization bounds that do not depend
on the Lipschitz constant of the loss function and obtain $\sqrt{\sum_t \eta_{t}/n} $ bounds. 
Especially, \cite{haghifam2020sharpened} introduce generalization bounds based on conditional mutual information inspired by \cite{steinke2020reasoning}, leading to tighter bounds than those based on mutual information. Recently, \cite{neu2021informationtheoretic} extend this information-theoretic to derive generalization bound for vanilla SGD.

==> Arxiv(old)/sec/stab_exp_familly.tex <==

\abcomment{The notation needs work} 


In this section, we consider Noisy SGD with Exponential family noise \citep{barndorff2014information,brown1986fundamentals,wainwright2008graphical}. Exponential families are typically represented in terms of natural parameters $\btheta$, and we consider componentwise independent distributions with scaled natural parameter $\btheta_{\alpha} = \btheta/\alpha$ with scaling $\alpha > 0$, i.e., 
\begin{align*}
\vspace{-3mm}
p_{\btheta_{\alpha}}(\bxi) = \exp(\langle \bxi, \btheta/\alpha \rangle - \psi(\btheta/\alpha)) \ppi_0(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_j/\alpha - \psi_j(\theta_j/\alpha)) \pi_0(\xi_j)~,
\end{align*}
where $\bxi$ is the sufficient statistic and the log-partition function $\psi(\btheta/\alpha)= \sum_{j=1}^p \psi_j(\theta_j/\alpha)$ is smooth and strongly convex \citep{barndorff2014information,banerjee2005clustering}, and $\ppi_0(\xi) = \prod_{j=1}^p \pi_0(\xi_j)$ is the base measure. Note that $\alpha=1$ gives the canonical form of the exponential family distributions. For general scaling $\alpha > 0$, for some cases the base measure $\pi_0$  may depend on the scaling, i.e., $\pi_{0,\alpha}$. A scaling $\alpha >0$ is valid as long as $\exp(\langle \bxi,\btheta/\alpha \rangle$ is integrable, i.e., $\int_{\bxi} \exp(\langle \bxi,\btheta/\alpha \rangle \pi_0(\bxi) d\bxi < \infty$ [][][].  

\abbcomment{we may be able to completely drop any mention of $\phi$ and expectation parameterization in the analysis}

By Lengendre duality, exponential families can also be written in terms of Bregman divergences as $\exp(-d_{\phi}(\bxi,\bmu))q_0(\bxi)$ \citep{barndorff2014information,banerjee2005clustering,frigyik2008functional,forster2002relative}, where $\phi$ is the dual convex function, i.e., $\phi(\bmu) = \sup_{\btheta'} ( \langle \bmu, \btheta' \rangle - \psi(\btheta') )$, $\bmu$ is the expectation parameter, and $q_0$ is a modified base measure\abcomment{say what it is exactly in terms of $\pi_0$}. For the natural parameter $\btheta$ and expectation parameter $\bmu$, Legendre duality implies the following relationship between $\psi(\btheta)$ and $\phi(\bmu)$:
\begin{equation}
    \nabla_{\btheta} \psi(\btheta) = \bmu~, \qquad \text{and} \qquad \nabla_{\bmu} \phi(\bmu) = \btheta~.
\end{equation}
Before proceeding further, we take a moment to understand how the representations and relationships change with scaling. Let $\btheta_{\alpha} \triangleq \btheta/\alpha$ and $\bmu_{\alpha} \triangleq \nabla \psi(\btheta_\alpha)$. Then, $\btheta_\alpha = \nabla \phi(\bmu_{\alpha})$. Further,\abcomment{show details as a proposition -- following Section 4.3 of Banerjee et al., 2005}
\begin{equation}
p_{\bmu_{\alpha}}(\bxi) = \exp(-d_{\phi}(\bxi,\bmu_{\alpha}) \q_0(\bxi) = \prod_{j=1}^p \exp(-d_{\phi}(\xi_j,\mu_{j,\alpha}) q_0(\xi_j)~.
\end{equation}
Note that $\psi$ is a smooth and strongly convex function [WaJo'08, Banerjee et al.,'05].In particular, there exists constants $c_1, c_2, c_2 \geq c_1 > 0$ such that
\begin{equation*}
    c_1 \I \leq \nabla^2 \psi(\btheta) \leq c_2 \I~,
\end{equation*}
for any $\btheta \in \dom(\psi)$. By duality~[][]\cite{kakade2009duality}, $\phi$ is also a strongly convex and smooth function with $\frac{c_2} \I \leq \nabla^2 \phi(\m) \leq \frac{1}{c_2} \I$ for any $\m \in \dom(\phi)$. 

\begin{exam}[Gaussian]
For univariate Gaussians with fixed variance $\sigma^2$, the scaling $\alpha = \sigma$, the sufficient statistic $\xi = x/\sigma$, the log-partition function  $\psi(\theta) = \theta^2/2$, and the base measure $\pi_0(\xi) = \frac{1}{\sqrt{2\pi}} \exp(-\xi^2/2)$ or equivalently $\pi_0(x) = \frac{1}{\sqrt{2\pi}\sigma} \exp(-x^2/2\sigma^2)$ using $\xi = x/\sigma$ and $d\xi = dx/\sigma$. The scaled parameter $\theta_{\alpha} = \theta_{\sigma} = \theta/\sigma$. Then, the distribution from the natural parameter form is:
\begin{equation}
    p_{\theta/\sigma}(x) = \exp( x \theta / \sigma^2 - \theta^2/(2\sigma^2) ) \times \frac{1}{\sqrt{2\pi}\sigma} \exp(-x^2/2\sigma^2)
    = \frac{1}{\sqrt{2\pi}\sigma} \exp(-(x-\mu)^2/2\sigma^2)~.
\end{equation}
The expectation parameter $\mu = \nabla \psi(\theta) = \theta$. The scaled expectation parameter $\mu_{\alpha} = \nabla \psi(\theta_\alpha) = \theta_\alpha = \theta/\sigma = \mu/\sigma$. Since $\xi = x/\sigma$ and the Bregman divergence $d_{\phi}(\xi,\mu) = \frac{1}{2}(\xi-\mu)^2$, the expectation parameter form
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(-(x/\sigma - \mu/\sigma )^2/2) \frac{1}{\sqrt{2\pi} \sigma} = \frac{1}{\sqrt{2\pi}\sigma} \exp(-(x-\mu)^2/2\sigma^2)~.
\end{equation}
\abcomment{some text} \qed
\end{exam}

\begin{exam}[Bernoulli]
For Bernoulli, the sufficient statistic $\xi = x \in \{0,1\}$, base measure is 1 on $\{0,1\}$, and the log-partition function $\psi(\theta) = \log(1+\exp(\theta))$ for natural parameter $\theta \in \R$. The expectation parameter $\mu = \nabla \psi(\theta) = \frac{exp(\theta)}{1+\exp(\theta)} = \frac{1}{1+\exp(-\theta)}$, the sigmoid function of $\theta$. The Bregman divergence is the Bernoulli KL-divergence given by: $d_{\phi}(\xi,\mu) = x \log \frac{x}{\mu} + (1-x) \log \frac{1-x}{1-\mu}$. For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{1}{1+\exp(-\theta_{\alpha})}$. 
The distribution is given by
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha}) = \mu_{\alpha}^{\xi} (1-\mu_{\alpha})^{1-\xi}~.
\end{equation}
\abcomment{some text} \qed
\end{exam}

\begin{exam}[Categorical]
The sufficient statistic $\xi = x = \{-1,0,1\}$, base measure is 1 on $\{-1,0,1\}$, natural parameters $\btheta = [\theta_1~~~\theta_2]^T \in \R^2$, and the log-partition function $\psi(\btheta) = \log(1+\exp(\theta_1) + \exp(-\theta_2))$. \abcomment{complete the example} \qed
\end{exam}





\subsection{Exponential Family Langevin Dynamics}

For convenience, we will denote
\begin{equation}
\btheta_B \triangleq \nabla \ell(\w_{t-1}, S_{B})~, \qquad \m_B = \nabla_{\btheta} \psi(\btheta_B)~.
\end{equation}


{\bf Option A:} The ``density'' for a mini-batch $B$ at scale $\alpha$ is:
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\alpha}) = \exp(\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha} \triangleq \frac{\btheta_B}{\alpha} = \frac{\nabla \ell(\w_{t-1}, S_{B})}{\alpha}~.
\end{equation}
Note that the corresponding expectation parameter
\begin{equation}
\m_{B,\alpha} = \nabla_{\btheta_{B,\alpha}} \psi( \theta_{B,\alpha} )~.
\end{equation}
For mini-batch $B_t$ and scaling $\alpha_t$, exponential family Langevin dynamics (EFLD) updates the parameters as
\begin{equation}
    \w_t = \w_{t-1} - \eta_t \bxi_t~, \qquad \bxi_t \sim p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})~.
\end{equation}
%\noindent\rule{\textwidth}{1pt}

{\bf Option B:} The ``density'' for a mini-batch $B$ at scale $\alpha$ and step-size $\eta$ is:
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\eta/\alpha}) = \exp(\langle \bxi, \btheta_{B,\eta/\alpha} \rangle - \psi(\btheta_{B,\eta/\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\eta/\alpha} \triangleq \frac{\eta \btheta_B}{\alpha} = \frac{\eta \nabla \ell(\w_{t-1}, S_{B})}{\alpha}~.
\end{equation}
Note that the corresponding expectation parameter
\begin{equation}
\m_{B,\eta/\alpha} = \nabla_{\btheta_{B,\eta/\alpha}} \psi( \theta_{B,\eta/\alpha} )~.
\end{equation}
For mini-batch $B_t$ and scaling $\alpha_t$, exponential family Langevin dynamics (EFLD) updates the parameters as
\begin{equation}
    \w_t = \w_{t-1} -  \bxi_t~, \qquad \bxi_t \sim p_{\psi}(\bxi; \btheta_{B_t,\eta_t/\alpha_t})~.
\end{equation}


{\bf Option C:} The parameter is
\begin{equation}
    \btheta_{B,\alpha,\eta} = h(\w_{t-1}) - \eta \nabla \ell(\w_{t-1},S_B)/\alpha~,
\end{equation}
for some function $h(\cdot)$.

The ``density'' for a mini-batch $B$ at scale $\alpha$ and step-size $\eta$ is:
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\eta_t,\alpha_t}) = \exp(\langle \bxi,\btheta_{B,\alpha_t,\eta_t} \rangle - \psi(\btheta_{B,\alpha_t,\eta_t})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha_t,\eta_t} \triangleq h(\w_{t-1}) - \eta \nabla \ell(\w_{t-1},S_B)/\alpha~.
\end{equation}
% Note that the corresponding expectation parameter
% \begin{equation}
% \m_{B,\eta/\alpha} = \nabla_{\btheta_{B,\eta/\alpha}} \psi( \theta_{B,\eta/\alpha} )~.
% \end{equation}
For mini-batch $B_t$ and scaling $\alpha_t$, exponential family Langevin dynamics (EFLD) updates the parameters as
\begin{equation}
    \w_t = \w_{t-1} -  \rho~, \qquad \bxi_t \sim p_{\psi}(\bxi; \btheta_{B_t,\eta_t/\alpha_t})~.
\end{equation}


\abbcomment{the analysis for the three cases give the same stability bound}

\abcomment{work out examples for the above three cases -- they should turn out to be sgld, noisy sign-SGD, and noisy truncated sign-SGD}



\subsection{Stability of EFLD}


By mean-value theorem, for each $\bxi$, we have a $\gamma_{\bxi} \in [0,1]$ such that $\tilde{\btheta}_B = \gamma_{\bxi} \btheta_B + (1-\gamma_{\bxi}) \btheta'_B$. Our goal is to bound:
\begin{align}
I_{A,B} &=  \bigintsss_\bxi \frac{\big( p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) \big)^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \\
&= \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \\
& = \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla_{\tilde{\btheta}_{B,\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2p_{\psi}^2(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi 
\label{eq:expcore}
\end{align}

\abcomment{ONGOING -- DO NOT READ}


\subsubsection{Handling Distributional Dependency of $\tilde{\btheta}_B$}
Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. In this step we focus on bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$. 


\begin{lemm}\label{lemm:exp_step2}
For some $\gamma_{\bxi} \in [0,1]$, $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alppha}$, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, \tilde{\btheta}_{B, \alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha}) \right]}{ \max\left( \exp\big[\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha}) \big] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right]\right) }
\leq \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right] ~.
\end{align*}
\end{lemm}
\proof Denoting $\gamma_{\bxi}$ as $\gamma$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
\begin{align*}
\langle \bxi, & \tilde{\btheta}_{B,  \alpha} \rangle  - \psi(\tilde{\btheta}_{B,\alpha}) 
 = \langle \bxi, \gamma \btheta_{B, \alpha} + (1-\gamma) \btheta'_{B,\alpha} \rangle - \psi\left( \gamma \btheta_{B, \alpha} + (1-\gamma) \btheta'_{B, \alpha} \right) \\
& = \gamma \bigg[ \langle \bxi , \btheta_{B,\alpha} \rangle - \psi(\btheta_{B, \alpha}) \bigg]  + (1-\gamma) \bigg[ \langle \bxi , \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \bigg] \\
& ~~~~~~~~~~~~~~~
  + \bigg[ \gamma \psi(\btheta_{B, \alpha} ) + (1-\gamma) \psi(\btheta'_{B,\alpha}) - \psi( \gamma \btheta_{B,\alpha} + (1-\gamma) \btheta'_{B,\alpha} ) \bigg] \\
& \stackrel{(a)}{\leq} \max\bigg( \langle \bxi , \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) , \langle \bxi , \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha} )  \bigg) \\
& ~~~~~~~~~~~~~~~ 
  + \bigg[ \gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha} , \tilde{\btheta}_{B,\alpha}) \bigg]~,
\end{align*}
where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation (See section 3.1.1 in \cite{banerjee2005clustering}):
\begin{align*}
  \gamma \psi(\btheta_{B, \alpha} ) + (1-\gamma) \psi(\btheta'_{B,\alpha}) - \psi( \gamma \btheta_{B,\alpha} + (1-\gamma) \btheta'_{B,\alpha} )  =  \gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha} , \tilde{\btheta}_{B,\alpha})~.
\end{align*}
Now, note that
\begin{align*}
\gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha})  + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha}, \tilde{\btheta}_{B,\alpha})  
& \leq \gamma d_{\psi}(\btheta_{B,\alpha}, \btheta'_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha}, \btheta_{B,\alpha}) \\
%& \stackrel{(a)}{=} \gamma d_{\phi}(\m'_{B,\alpha}, \m_{B,\alpha}) + (1-\gamma) d_{\phi}(\m_{B,\alpha},\m'_{B,\alpha})~\\
& \leq \gamma c_2 \| \btheta'_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 + (1-\gamma) c_2 \| \btheta_{B,\alpha} - \btheta'_{B,\alpha} \|_2^2 \\
& \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2~.
\end{align*}
As a result,
\begin{align*}
& \frac{\exp\left[\langle \bxi, \tilde{\btheta}_{B, \alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha}) \right]}{\max\left( \exp\left[\langle \bxi, \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) \right] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right] \right) }\\
& ~~~~~ \leq\exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right]
\frac{ \exp \left[ \max\bigg( \langle \bxi , \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) , \langle \bxi , \btheta'_{B,\alpha} \rangle - \psi(\btheta'_{B,\alpha})  \bigg) \right] }{ \max\left( \exp\left[\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha}) \right] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right] \right) } \\
& ~~~~~ = \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right]~.
\end{align*}
That completes the proof.\qed 







\subsubsection{Bounding the Density Ratio}

\abcomment{add text and basic -- helping the reader understand why we are looking at this}

Focusing on density ratio, we have
\begin{lemm}\label{lemm:exp_step3}
For any $\bxi$, we have
\begin{align*}
&\frac{\exp\left[\langle \bxi, 2\btheta_{B, \alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A,\alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}\\
&\leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \psi( (2\btheta_B - \btheta_A)/\alpha) \right].
\end{align*}

\end{lemm}

\proof  Note that
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B,\alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A , \alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}  
& = \exp\left[ \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \rangle - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big) \right] \\
& = \beta_{B,A,\alpha} \exp \left[  \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha} \rangle - \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \right]~,
\end{align*}
where
\begin{align*}
\beta_{B,A,\alpha} & = \exp \left[ \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big) \right] ~.
\end{align*}
Note that
\begin{align*}
\log \beta_{B,A,\alpha} & = \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big)\\
& = - \bigg( \psi(\btheta_{B,\alpha}) - \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \bigg) - \bigg( \psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \bigg) \\
& \stackrel{(a)}{\leq} \bigg\langle \btheta_{B,\alpha} - \btheta_{A,\alpha}, \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \bigg\rangle + \bigg\langle \btheta_{A,\alpha} - \btheta_{B,\alpha}, \nabla \psi( \btheta_{A,\alpha} \bigg\rangle   \\
& = \bigg\langle \btheta_{B,\alpha} - \btheta_{A,\alpha}, \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\btheta_{A,\alpha})  \bigg\rangle  \\
& \stackrel{(b)}{\leq} \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2 \| \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\btheta_{A,\alpha}) \|_2  \\
& \stackrel{(c)}{\leq} c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2 \| (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \btheta_{A,\alpha} \|_2 \\
& = 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2~,
\end{align*}
where (a) follows from the convexity of $\psi$, (b) follows from Cauchy-Schwartz, and (c) follows by smoothness of $\psi$.


As a result, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B,\alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A, \alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}
&\leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \psi( (2\btheta_B - \btheta_A)/\alpha) \right]~.
\end{align*}
That completes the proof.\qed

The analysis for the term involving $\btheta'_B$ is exactly the same. 

\abcomment{state a Lemma by combining Lemma 2 and Lemma 3?}

\abbcomment{A Lemma will also help the reader understand that the base measure scales correctly, and essentially stays unchanged}

\subsubsection{Putting Everything Together}



\abcomment{add text}

\begin{restatable}{lemm}{lemmexpinfo}
\label{lemm:exp_info}
Consider Noisy SGD with exponetial family noise such that the log-partition function is  $c_1$-strongly convex and $c_2$-smooth, for a given sample set $\bar S$ and parameters $\w_{t-1}$, let $\Delta_{t}(\bar{S}) \triangleq \max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ be data-dependent and adaptively chosen such that $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq \abedit{c(c_1,c_2)}$, then for any $B_t \in G_1$ and  $A_t \in G_0$,  we have \abcomment{notation and constants need work, result needs to be updated}
\begin{align}
I_{A_t, B_t} \leq c_0 c_2^2\frac{\eta_{t}^{2}}{\alpha_t^2} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c(c_1,c_2) = \frac{c_1^2}{(3c_2-c_1)c_2(1+c_1)}$.
\end{restatable} 

\proof 
\abedit{From Lemma ?? and ??}, \abcomment{update} we have
\begin{align*}
&I_{A,B}\leq \bigintsss_\bxi \frac{ \left\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi( \tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{ p_{\psi}(\bxi;\btheta_{A,\alpha})} d\bxi\\
&\leq  \exp\left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2\right] \\
& ~~~~~~~~~~~~~~~~~~~~\times \max\left(  \exp \left[ 4c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \right. ~, \\
& ~~~~~~~~~~~~~~~~~~~~~~~~~~~
\left.   \exp \left[ 4c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B',\alpha}-\btheta_{A,\alpha}) d\bxi \right)~.
\end{align*}
Focusing on the integral in the first term (the analysis for the second term is essentially the same), we have
\begin{align*}
& \bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi; 2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = \bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \big( \bxi - \E[\bxi] \big) - \left(\nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& \leq 2\underbrace{\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \E[\bxi] \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi}_{T_1} + 2 \underbrace{\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi}_{T_2}~.
\end{align*}
For $T_1$, note that 
\begin{align*}
T_1 & = \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \E[\bxi] \right\rangle^2   \right] \\
& = (\btheta_{B,\alpha} -\btheta_{B',\alpha})^T \E_{\bxi \sim p_{\psi}(2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (\bxi - \E[\bxi]) (\bxi - \E[\bxi])^T \right] (\btheta_{B,\alpha} -\btheta_{B',\alpha})~\\
& = (\btheta_{B,\alpha} -\btheta_{B,\alpha})^T \nabla^2 \psi( 2\btheta_{B,\alpha}-\btheta_{A,\alpha})  (\btheta_{B,\alpha} -\btheta_{B',\alpha}) \\
& \leq c_2 \| \btheta_{B,\alpha} -\btheta_{B,\alpha} \|_2^2~,
\end{align*}
since the spectral norm of $\nabla^2 \psi$ is bounded by $c_2$. 

For $T_2$, first note that 
\begin{align*}
\E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}[\bxi] = \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) ) ~.
\end{align*}
Hence, with $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta_{B',\alpha}$, we have
\begin{align*}
T_2 & = \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha},  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right\rangle^2   \right] \\    
& = \E_{\bxi \sim p_{\psi}(\bxi; 2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha},  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha})  \right\rangle^2   \right]\\
& \leq  \| \btheta_{B,\alpha} -\btheta_{B,\alpha} \|_2^2 ~~~\E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\|  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \right\|_2^2  \right]\\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\|  \tilde{\btheta}_{B,\alpha} - (2\btheta_{B,\alpha} - \btheta_{A,\alpha} ) \right\|_2^2  \right] \\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})} \left[ \big\| \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta_{B',\alpha} - \btheta_{B,\alpha} - (\btheta_{B,\alpha} - \btheta_{A,\alpha}) \big\|_2^2 \right] \\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}
\left[ \big\|  (1-\gamma_{\bxi}) (\btheta_{B',\alpha} - \btheta_{B,\alpha}) - (\btheta_{B,\alpha} - \btheta_{A,\alpha}) \big\|_2^2 \right] \\
& \leq  2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ 
\left( \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (1-\gamma_{\bxi})^2  \big\|  \btheta_{B',\alpha} - \btheta_{B,\alpha} \big\|_2^2 \right]
+  \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})} \left[ \big\|  \btheta_{B,\alpha} - \btheta_{A,\alpha} \big\|_2^2 \right]  \right) \\
& = 2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ 
\left( \big\|  \btheta_{B',\alpha} - \btheta_{B,\alpha} \big\|_2^2 \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (1-\gamma_{\bxi})^2   \right]
+   \big\|  \btheta_{B,\alpha} - \btheta_{A,\alpha} \big\|_2^2  \right) \\
& \leq  2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~  \left( \| \btheta_{B,\alpha} -\btheta_{B',\alpha}\|_2^2  + \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right) ~.
\end{align*}
Putting everything back together
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 & p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 ~~\left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
Similarly
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 & p_{\psi}(\bxi;2\btheta_{B',\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 ~~\left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
Since the bound is the same for both the terms, the $\max$ can be bounded by the right-hand-side.
% \abcomment{please finish the rest, need to check the scaling w.r.t.~$1/\sigma$ once the earlier notation is cleaned up}


Then, plugging into bound on $I_{A,B}$, we have
\begin{align*}
I_{A,B} &
\leq  \exp\bigg[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 4c_2 \max\left(  \| \btheta_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 , \| \btheta_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 \right)  \bigg] \\
& ~~~~~~~~~~ \times c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)\\
% &\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta_B-\btheta_A,\sigma} d\bxi \\
% + &\frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]2
% \bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha) \right\rangle^2 p_{2\btheta_B'-\btheta_A,\sigma} d\bxi~.\\
% \leq &\frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \frac{1 + 2 \| \btheta_B - \btheta'_B \|_2^2 + 2 \| \btheta_B - \btheta_A \|_2^2}{c_1 \sigma^4}  \| \btheta_B - \btheta'_B \|_2^2\\
% +& \frac{1}{\sigma^4} \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \frac{1 + 2 \| \btheta_B - \btheta'_B \|_2^2 + 2 \| \btheta'_B - \btheta_A \|_2^2}{c_1 \sigma^4}  \| \btheta_B - \btheta'_B \|_2^2\\
% \leq & \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \frac{1 + 2c_2^2 \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 + 2c_2^2 \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2}{c_1 \sigma^8}  \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma}\|_2^2\\
%  + & \exp\left[ \frac{c_2}{\alpha^2} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right] \exp \left[ \frac{c_3}{\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \frac{1 + 2c_2^2 \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 + 2c_2^2 \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2}{c_1 \sigma^8}  \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\\
%  \stackrel{(a)}{\leq}& 2\cdot 2\cdot \frac{1}{8} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2/\sigma^4 + 2\cdot 2\cdot \frac{1}{8} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2/\sigma^4\\
%  = &  \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2/\sigma^4,
\end{align*}
where step (a) is by choosing step size $\eta_t$ data-dependent and adaptively chosen such that $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq \min( \frac{4}{c_2}\ln 2, \frac{\sigma_t^2}{c_3}\ln 2, \frac{1}{4c_2^2}(\frac{c_1}{8}-\frac{1}{\sigma_t^4})) $, we have the result.
\qed


\abcomment{{\bf main result}, needs work}
\begin{theo}
Consider the noisy SGD with Exponential family noise of the update rule \eqref{eq:exp_update},  with mini-batch size $b \leq n/2$, for any given sample $\bar S$, let step size $\eta_t$ and noise $\sigma_t$ be adaptively chosen as in Lemma \ref{lemm:exp_info},
%such that, for any observed $\w_{t-1}$,  $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq c(c_1,c_2)$, where $\Delta_{t}(\bar{S})=\max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z\right)-\nabla \ell\left(\mathbf{w}_{t-1}, \tilde{z}\right)\right\|_{2}$ 
%Then 
we have 
\begin{align}
\left|\mathbb{E}_{S}\left[L_{D}(\w_T)-L_{S}(\w_T)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar S} \sqrt{\sum_{t=1}^{T} \underset{\w_{t-1}}{\mathbb{E} }\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~}~.
\end{align}
where $c$ is a constant with detailed value presented in Appendix.
\label{theo:exp_bound}
\end{theo}

\proof Similar to Theorem \ref{theo:guss_gen}, based on Lemma \ref{lemm:exp_info}, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate,  we have
\begin{align}
\nr K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right) & = \underset{B_{t} \in G_{1},A_{t} \in G_{0}}{\mathbb{E}}\left[\int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}\right]   \leq  \left[ \frac{\eta_{t}^{2}}{\sigma_{t}^{4}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}


Then, based on the chain rule of KL-divergence, we have
\begin{align}
\nr K L\left(P_{0: T} \| P_{0: T}^{\prime}\right) 
& = \sum_{t=1}^{T} \mathbb{E}_{\w_{t-1}} \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{4}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

Following Theorem \ref{theo:stab}, we have
\begin{align*}
\left|\mathbb{E}_{S}\left[L_{D}\left(\mathbf{w}_{T}\right)-L_{S}\left(\mathbf{w}_{T}\right)\right]\right| \leq \frac{b}{n} \mathbb{E}_{\bar{S}} \sqrt{\sum_{t=1}^{T} \underset{\mathbf{w}_{t-1}}{\mathbb{E}}\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{4}}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z_{n}\right)-\ell\left(\mathbf{w}_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]}, 
\end{align*}
 which completes the proof.






\newpage
.
\newpage

\subsubsection*{(OLD WRITEUP -- To be dropped)} 
Noisy SGD with exponential families at step $t$ have mean parameter $\m_{B_t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t})$ so that the next iterate 
\begin{align}
\label{eq:exp_update}
  \w_{t} \sim P_{B_t,\bxi_t,\alpha_t|\w_{0:t-1}} & = \exp(-d_{\phi_{\alpha_t}}(\bxi,\m_{B_t})) q_{\alpha_t}(\bxi) \\
  &= \exp(-d_{\phi_{\alpha_t}}(\bxi, \w_{t-1} - \eta_t \nabla \ell (\w_{t-1},S_{B_t})) q_{\alpha_t}(\bxi)~.\nonumber
\end{align}

By duality~\cite{kakade2009duality}, $\phi_{\alpha_t}:\R^d\rightarrow \R$ is a strongly convex and smooth function parameterized by $\alpha$.
Since $\phi_{\alpha_t}$ is strongly convex and smooth, there exists constants 
\begin{equation*}
    c_1 \| \bxi - \m \|_2^2 \leq d_{\phi_{\alpha_t}}(\bxi,\m) \leq c_2 \| \bxi - \m \|_2^2~,
    % \quad\text{and}~ c_1 \| \bxi - \btheta \|_2^2 \leq d_{\psi}(\bxi,\btheta) \leq c_2 \| \bxi - \btheta \|_2^2
\end{equation*}
for any $\bxi,\m$ in the domain $\Theta$ and any $\alpha\in \Omega$.  


Recall that running SGD with Exponential family noise with $S$ and $S_n^\prime$, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate, for a fixed mini-batch $B_t$, following \eqref{eq:nmia}, we have $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively to denote distributions over $\cW$ corresponding to $S, S'_{n}$, where $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively have mean parameters:
\begin{align*}
    \m_{B_t}  = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t}) \qquad \text{and} \qquad
    \m'_{B_t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_{B_t}) ~.
\end{align*}
Based on Proposition \ref{prop:mixmodel}, the conditional distributions $P_{t \mid} $ and $ P_{t}^{\prime}$  over $\cW$ respectively corresponding to $S, S'_{n}$ are mixture of Exponential family, i.e., $ P_{t|} = s Q_{t|} + (1-s) R_{t|}~$ and$ P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~$, where 
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  In order to bound
the KL divergence $K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right)$
based on Theorem \ref{theo:stab}, 
the goal is to bound 
$$I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}$$
for  $B_t \in G_1$ and  $A_t \in G_0$. 




%\subsection{Preliminary}
We introduce preliminary of exponential family for the analysis. We will use both the natural and expectation parameterization form. Let $\hat{\btheta}_{\alpha} = \btheta/(\alpha)$, and the mean parameter $\hat{\m}_{\alpha} = \nabla_{\hat{\btheta}_{\alpha}} \psi(\hat{\btheta}_{\alpha})$. In our settings, the mean parameter for distribution on batch $B$ is $\m_B = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t})$ so we use $\hat{\m}_{B,\alpha},\hat{\m}'_{B',\alpha}$ to denote $\m_B,\m'_B$ respectively. 
For ease of computation, we denote $\m_{\alpha}$ as the natural gradient: $\m_{\alpha} := \nabla_{\btheta} \psi(\btheta/(\alpha)) = \hat{\m}_{\alpha}/(\alpha)$, and similarly we have $\nabla_{\btheta}^2 \psi(\btheta/(\alpha)) = \nabla_{\btheta/(\alpha)}^2 \psi(\btheta/(\alpha))/(\alpha^2)$. Further, $\btheta/(\alpha) = \nabla \psi^{-1}(\m_{\alpha}) = \nabla \phi_{\alpha}(\m_{\alpha})$. 
% Then, 
% \begin{align*}
% \langle \bxi, \btheta/(\alpha) \rangle - \psi(\btheta/(\alpha)) 
% & = \langle \m_{\alpha}, \btheta/(\alpha) \rangle - \psi(\btheta/(\alpha)) + \langle \bxi - \m_{\alpha}, \btheta/(\alpha) \rangle~\\
% & = \phi(\m_{\alpha}) + \langle \bxi - \m_{\alpha}, \nabla \phi(\m_{\alpha}) \rangle \\
% & = - d_{\phi}(\bxi, \m_{\alpha}) + \phi(\bxi)~.
% \end{align*}
Further, since $\psi$ is strongly convex and smooth, so is $\phi$ by Legendre duality, and there are strongly convex constant $c_1$ and Lipschitz smooth constant $c_2$, where $c_1 \leq c_2$ such that
\begin{equation*}
    c_1 \| \bxi - \m \|_2^2 \leq d_{\phi_\alpha}(\bxi,\m) \leq c_2 \| \bxi - \m \|_2^2~,
\end{equation*}
for any $\bxi,\m$ in the domain $\Theta$, any $\alpha\in \Omega$. From the definition of $d_{\phi_\alpha}$:
\begin{equation}
    d_{\phi_\alpha}(\bxi,\m) = \phi_\alpha(\bxi)-\phi_\alpha(\m)-\langle \bxi - \m, \nabla \phi_\alpha (\m)\rangle,
\end{equation}
the strongly convexity and Lipschitz smoothness on $d_{\phi_\alpha}$ implies $\phi_{\alpha}$ is strongly convex and Lipschitz smooth. By duality, we have $\psi$ is strongly convex and Lipschitz smooth  [see Theorem 6 in \cite{kakade2009duality}]:
\begin{equation}
    \frac{1}{4c_2} \| \bxi - \btheta\|_2^2 \leq d_{\psi}(\bxi,\btheta) \leq \frac{1}{4c_1} \| \bxi - \btheta \|_2^2.
\end{equation}


%We further assume that the base measure $\pi_0(\xi_j) \leq 1, j=1,\ldots,p$, \abcomment{may not be necessary} which is satisfied by many 


Following the earlier analysis, by mean-value theorem, for some $\tilde{\btheta}_B = \alpha_x \btheta_B + (1-\alpha_x) \btheta'_B$, $\alpha_x \in [0,1]$, our goal is to bound:
\begin{align}
I_{A,B} &=  \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \nabla_{\btheta}p_{\tilde{\btheta}_B,\alpha}\rangle ^2}{p_{\btheta_A,\alpha}} d\bxi = \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/\alpha)\rangle ^2p_{\tilde{\btheta}_B,\alpha}^2}{\alpha^2 p_{\btheta_A,\alpha}} d\bxi 
% \\
% &\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\tilde{\btheta}_B/\alpha) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\alpha}^2}{2\alpha^4 p_{\btheta_A,\alpha}} d\bxi~.
\label{eq:expcore}
\end{align}



\subsection{Main Result (old Main Paper)}

Similar as the analysis for Gaussian noise, we have the following result for Exponential family noise:
\begin{restatable}{lemm}{lemmexpinfo}\label{lemm:exp_info}
Consider Noisy SGD with exponential family noise  such that $d_{\phi}$ in \eqref{eq:exp_update} is  $c_1$-strongly convex and $c_2$-smooth for a given set $\bar S$ and $\w_{t-1}$, and  $\alpha_t > (8/c_1)^{1/4}$. Let $\Delta_{t}(\bar{S}) = \max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ be data-dependent and adaptively chosen such that $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\alpha_t^4 \leq c(c_1,c_2)$, then for any $B_t \in G_1$ and  $A_t \in G_0$,  we have
\begin{align}
I_{A_t, B_t} \leq \frac{\eta_{t}^{2}}{\alpha_t^4} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c(c_1,c_2) = \min( \frac{4}{c_2}\ln 2, \frac{8c_1\alpha_t^2}{(3c_2-c_1)c_2}\ln 2, \frac{1}{4c_2^2}(\frac{c_1}{8}-\frac{1}{\alpha_t^4}))$.
\end{restatable} 



Here we outline the main ideas of the proof. The details can be found in the Appendix~\ref{app:exp}. Compared to Gaussian case, exponential family does not maintain invariant under rotation, here we apply mean-value theorem to the natural parameter form
\begin{align}
\label{eq:exp_target}
\nonumber I_{A,B} &=  \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \nabla_{\btheta}p_{\tilde{\btheta}_B,\alpha_t}\rangle ^2}{p_{\btheta_A,\alpha_t}} d\bxi = \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/2\alpha_t^2)\rangle ^2p_{\tilde{\btheta}_B,\alpha_t}^2}{\alpha_t^2 p_{\btheta_A,\alpha_t}} d\bxi \\
\nonumber &= \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \big( \bxi - \E[\bxi] \big) - \left(\nabla \psi(\tilde{\btheta}_B/2\alpha_t^2) - \E[\bxi] \right)\rangle^2 p_{\tilde{\btheta}_B,\alpha_t}^2 }{\alpha_t^2 p_{\btheta_A,\alpha_t}} d\bxi~\\
&\leq \underbrace{\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \bxi - \E[\bxi] \right\rangle^2 \frac{p_{\tilde{\btheta}_B,\alpha_t}^2 }{2\alpha_t^4 p_{\btheta_A,\alpha_t}} d\bxi}_{T_1} + \underbrace{\bigintsss_\bxi  \left\langle \btheta_B -\btheta'_B, \nabla \psi(\tilde{\btheta}_B/2\alpha_t^2) - \E[\bxi] \right\rangle^2 \frac{p_{\tilde{\btheta}_B,\alpha_t}^2 }{2\alpha_t^4 p_{\btheta_A,\alpha_t}} d\bxi}_{T_2}.
\end{align}
So far we have rewritten $I_{A,B}$ as a sum of a second moment of $\bxi$: $T_1$ and a seemingly constant based on $\tilde{\btheta}_B$: $T_2$ evaluated on a seemingly scaled probabilistic function $\frac{p_{\tilde{\btheta}_B,\alpha_t}^2}{p_{\btheta_A,\alpha_t}}$.
However, since $\tilde{\btheta}_B$ depends on $\bxi$ by $\beta_\xi$ which has an intractable dependence on $\bxi$, we derive technical arguments: 
    1) We bound $p_{\tilde{\btheta}_B,\alpha_t}$ by a combination of $p_{\btheta_B,\alpha_t}$ and $p_{\btheta'_B,\alpha_t}$: $
p_{\tilde{\btheta}_B,\alpha_t}
\leq \exp\left[ c_2 \| \m_B-\m'_B \|_2^2 \right] (p_{\btheta_B,\alpha_t}+p_{\btheta'_B,\alpha_t})
$; 2) We show the combination of $p_{\btheta_B,\alpha_t}$ and $p_{\btheta'_B,\alpha_t}$ derived by step 1 divided by $p_{\btheta_A,\alpha_t}$ can be bounded by a proper probabilistic function: $\frac{p_{\btheta_B,\alpha_t}^2}{p_{\btheta_A,\alpha_t}}
    \leq \exp \left[ \frac{(3c_2-c_1)c_2}{8c_1\alpha_t^4} \| \m_{B} - \m_{A} \|_2^2 \right] p_{2\btheta_B-\btheta_A,\alpha_t}$;
    3) Finally, we show $T_1$ and $T_2$ can be bounded under the proper probability distribution generated by step 2.


The final step is to gather Equation~\eqref{eq:exp_target},  three steps above, and a proper choice of step size stated in Lemma~\ref{lemm:exp_info}, to complete the proof. 
%The details can be found in Appendix~\ref{app:exp}.
Combining Lemma~\ref{lemm:exp_info} with Theorem~\ref{theo:stab}, we have the following generalization bound for update based on Exponential family:
\begin{restatable}{theo}{theoboundexp}
Consider the noisy SGD with Exponential family noise of the update rule \eqref{eq:exp_update},  with mini-batch size $b \leq n/2$, for any given sample $\bar S$, let step size $\eta_t$ and noise $\alpha_t$ be adaptively chosen as in Lemma \ref{lemm:exp_info},
we have 
\begin{align}
\left|\mathbb{E}_{S}\left[L_{D}(\w_T)-L_{S}(\w_T)\right]\right| \leq  \frac{b}{n} \mathbb{E}_{\bar S} \sqrt{\sum_{t=1}^{T} \underset{\w_{t-1}}{\mathbb{E} }\left[\frac{\eta_{t}^{2}}{\alpha_{t}^{4}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~}~.
\end{align}
\label{theo:exp_bound}
\end{restatable}



Theorem~\ref{theo:exp_bound} extends the result on the expected generalization error of Gaussian noise in Theorem~\ref{theo:guss_gen} to general Exponential family distribution and shows the bound scales as $O(\sqrt{\sum_t^T \frac{\eta_t^2}{\alpha_t^4}}/n)$.



==> Arxiv(old)/sec/stab_gauss.tex <==
% \abcomment{The initial part, before the analysis specific to Gaussian noise, should be moved to Section 3}

% Consider sampling $\bar{S} \sim D^{n+1}$. Let $S,S'$ be size $n$ subsets of $\bar{S}$ which differ by one point. Without loss of generality, we let $S=\{z_1,\ldots,z_{n-1},z_n\}$ and $S' = \{z_1,\ldots,z_{n-1},z'_n\}$, where $z'_n = z_{n+1}$. let $S_0 = \{z_1,\ldots,z_{n-1}\}$. The algorithm uses a mini-batch $B$ of size $b$ in each step. Let the set of all mini-batches be denoted by $G$. Let the set of all mini-batches drawn from $S_0$ be denoted by $G_0$. Note that $|G_0| = \binom{n-1}{b}$. Let the set of all mini-batches which includes the last sample, viz., $z_n$ for $S$ and $z'_n$ for $S'$, be denoted by $G_1$. Note that $|G_1| = \binom{n-1}{b-1}$. Also note that 
% \begin{align*}
%     |G_0| + |G_1| = \binom{n-1}{b} + \binom{n-1}{b-1} = \binom{n}{b} = |G|~,
% \end{align*}
% the total number of $b$-sized mini-batch samples from a dataset of size $n$. The subset of $S$ and $S'$ corresponding to mini-batch $B$ will be denoted as $S_B$ and $S'_B$.

% Consider two collection of points $\{\mu_B : B \in G \}$ and $\{\mu_B : B \in G\}$. In our context, at any stage $t$, conditioned on $w_{t-1}$, for mini-batch $B$, we have
% \begin{align*}
%     \mu_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S_B) \\
%     \mu'_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S'_B) ~.
% \end{align*}
% Let $p_{\mu,\sigma}$ denote the Gaussian distribution $\cN(\mu, \sigma^2 \I)$. Let $P = \frac{1}{|G|} \sum_{B \in G} p_{\mu_B,\sigma}$ and  $P' = \frac{1}{|G|} \sum_{B \in G} p_{\mu'_B,\sigma}$. Our goal is to bound $KL(P \| P')$ {\em without making any additional assumptions}. Note that $\eta_t,\sigma_t$ can depend on $w_{1:t-1}$, but since the analysis is conditioned on $w_{1:t-1}$, these are effectively constants for the current analysis. 

% Remark: This analysis immediately shows why KL-divergence cannot be used for the non-noisy case -- these will be Dirac measures, and KL-div will be $\infty$. A bound based on TV or Hellinger would still be valid.

% Let 
% \begin{align*}
% Q_1 = \frac{1}{|G_1|} \sum_{B \in G_1} p_{\mu_B,\sigma} \qquad Q_2 = \frac{1}{|G_1|} \sum_{B \in G_1} p_{\mu'_B,\sigma} \qquad R = \frac{1}{|G_0|} \sum_{B \in G_0} p_{\mu_B,\sigma}~.  
% \end{align*}
% Then, with 
% \begin{equation*}
% s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}~,
% \end{equation*}
% we have 
% \begin{align*}
%     P = s Q_1 + (1-s) R \qquad P' = s Q_2 + (1-s) R~.
% \end{align*}
% Then,
% \begin{align*}
% KL(P \| P') & \stackrel{(a)}{\leq} \left(\frac{b}{n} \right)^2 \left(\frac{n}{n-b}\right) \int_x \frac{(Q_1 - Q_2)^2}{R} dx \\
%  & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \bigintsss_x \frac{ \left(  \frac{1}{|G_1|} \left[ \sum_{B \in G_1} p_{\mu_B,\sigma} -  \sum_{B \in G_1} p_{\mu'_B,\sigma} \right] \right)^2 }{\frac{1}{|G_0|} \sum_{B \in G_0} p_{\mu_B,\sigma}} dx \\
%  & \stackrel{(b)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_x \frac{1}{|G_1|}\sum_{B \in G_1}  \frac{ \left(  p_{\mu_B,\sigma} -   p_{\mu'_B,\sigma} \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} p_{\mu_A,\sigma}} dx \\
%  & \stackrel{(c)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_x \frac{1}{|G_1|}  \sum_{B \in G_1} \left(  p_{\mu_B,\sigma} -   p_{\mu'_B,\sigma} \right)^2  \frac{1}{|G_0|}\sum_{A \in G_0} \frac{ 1 }{ p_{\mu_A,\sigma}} dx \\
%  & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \frac{1}{|G_0| |G_1|}  \sum_{A \in G_0} \sum_{B \in G_1} \bigintsss_x \frac{ \left(  p_{\mu_B,\sigma} -   p_{\mu'_B,\sigma} \right)^2 }{ p_{\mu_A,\sigma}} dx ~,
% \end{align*}
% where (a) is from Lemma [], (b)(c) is from Jensen's inequality since function $f(x) = x^2$ is convex and $f(x)=\frac{1}{x}$ is convex on $(0,\infty)$. 
% The analysis upto this point does not need the distributions to be Gaussian.

% \abcomment{Lets move the above part to Section 3. The following can become Section 4 -- the analysis specific to Gaussians, the above is general}

%\subsection{Gaussian Noise: With Projection}

% \abcomment{start by stating the noisy gradient descent algorithm. The earlier sections will be written for general iterative algorithms (not necessarily gradient descnet) with additive noise}

\begin{algorithm}[t] 
\caption{Noisy SGD with Gaussian Noise}
	\begin{algorithmic}[1] \label{algo:nsgd_gauss}
		\STATE \textbf{Input}: Dataset $\bar S = S \cup \{z_{n+1}\}$, certain loss $\ell(\cdot)$, initial point $\w_0$
		\STATE \textbf{Set}:  Iteration time $T$, noise parameter $\{\sigma_t\}_{t\leq T}$,   learning rate $\{\eta_t\}_{t\leq T}$.  \yzcomment{do we want to write the step size condition $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$ here?}
		\FOR{$t = 0,...,T$}
		\STATE $\nabla\ell(\w_t, S_{B_t}) = \frac{1}{|S_{B_t}|}\sum_{z_i \in B_t}\nabla \ell(\w_t,z_i)$, with $S_{B_t}$ uniformly sampled from $S$ with replacement.
		\STATE $\w_{t} =  \w_{t-1} - \eta_t \nabla \ell (\w_{t-1},S_{B_t}) + \bxi_t, ~~\text{where}~~
  \bxi_t \sim  \cN(0, \sigma_t^2\mathbb{I}_d)~$.
		\ENDFOR 
	\end{algorithmic}
\end{algorithm}





In this section, we consider Noisy SGD with Gaussian noise. Specifically, we consider the following update
\begin{align}
  \w_{t} =  \w_{t-1} - \eta_t \nabla \ell (\w_{t-1},S_{B_t}) + \bxi_t, ~~\text{where}~~
  \bxi_t \sim  \cN(0, \sigma_t^2\mathbb{I}_d)~, \label{eq: sgd_guss_update}
\end{align}

where $S_{B_t}$ is a mini-batch drawn randomly from training set $S$ and 
$\nabla \ell (\w_{t-1},S_{B_t})$ is the stochastic gradient evaluated on $S_{B_t}$, i.e., $\nabla \ell (\w_{t-1},S_{B_t}) = \frac{1}{|S_{B_t}|} \sum_{z \in {S_{B_t}}}\nabla \ell(\w_{t-1},z)$. $\bxi \sim \cN(0, \sigma_t^2\mathbb{I}_d)$ is a d-dimensional isotropic Gaussian noise with variance $\sigma_t^2\mathbb{I}_d$. The pseudo code of Noisy SGD with Gaussian noise is given in Algorithm \ref{algo:nsgd_gauss}.
Note that the update in \eqref{eq: sgd_guss_update} with the
special case of $\sigma_t = \sqrt{{2\eta_t}/{\beta}}$ for $\beta >0$  captures the SGLD algorithm. 

Consider running Noisy SGD with Gaussian noise on two datasets $S$ and $S_n^\prime$, 
% we get two joint distributions $P_{0: T}$ and $P_{0: T}^\prime$ over $\w_{0:T}$. Based on the chain rule of KL-divergence in \eqref{eq:klchain}, in order to bound $K L\left(P_{0: T} \| P_{0: T}^{\prime}\right)$, we are interested in analyzing the KL-divergence $K L(P_{t \mid} \| P_{t \mid}^{\prime})$ conditioned on past iterates $\w_{0:(t-1)}$. 
conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate, for a fixed mini-batch $B_t$, following \eqref{eq:nmia}, we have $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively to denote distributions over $\cW$ corresponding to $S, S'_{n}$. Note that, since $\bxi_t$ is Gaussian noise, 
$P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ are two Gaussian distributions with the same variance $\sigma_t^2\mathbb{I}_d$, and with mean $\m_{B_t}$ and $\m^\prime_{B_t}$ respectively  to be
\begin{align*}
    \m_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t}) \\
    \m'_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_{B_t}) ~.
\end{align*}

Based on Proposition \ref{prop:mixmodel}, the conditional distributions $P_{t \mid} $ and $ P_{t}^{\prime}$  over $\cW$ respectively corresponding to $S, S'_{n}$ are mixture of Gassuains, i.e., $ P_{t|} = s Q_{t|} + (1-s) R_{t|}~$ and$ P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~$, where 
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  In order to bound
the KL divergence $K L(P_{t \mid} \| P_{t \mid}^{\prime})$
based on Theorem \ref{theo:stab}, for  $B_t \in G_1$ and  $A_t \in G_0$，we need to bound
\begin{align}
 I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t},~~\text{where} ~~ \bxi_t \sim \cN(0, \sigma_t^2\mathbb{I}_d) ~. 
\end{align}

% $$I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}$$
% with $\bxi_t \sim \cN(0, \sigma_t^2\mathbb{I}_d)$ 

In the following lemma, we show that we can bound $I_{A_t, B_t}$ by the gradient discrepancy between $S$ and $S_n^\prime$, i.e., $\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|$, if we slightly control the step size $\eta_t$, noise variance $\sigma_t^2$ based on a data-dependent quantity that can be evaluated given $S$ and $S_n^\prime$.

\begin{restatable}{lemm}{lemmaiabguss}
For a given set $\bar S$ and $\w_{t-1}$ observed at ${t-1}$ iteration, let $\Delta_{t}(\bar{S}) = \max _{z, \bar{z} \in \bar S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ and $\sigma_t$ to be data-dependent and adaptively chosen such that $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$, for any $B_t \in G_1$ and  $A_t \in G_0$,  we have
\begin{align}
I_{A_t, B_t} \leq c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c= 41 \ln \frac{3}{2}$.\label{lemm:iab_guss}
\end{restatable}


% \begin{lemm}
% For a given set $\bar S$ and $\w_{t-1}$ observed at ${t-1}$ iteration, let $\Delta_{t}(\bar{S}) = \max _{z, \bar{z} \in \bar S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ and $\sigma_t$ to be data-dependent and adaptively chosen such that $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$, for any $B_t \in G_1$ and  $A_t \in G_0$,  we have
% \begin{align}
% I_{A_t, B_t} \leq c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
% \end{align}
% where $c$ is a constant~\footnote{ Detail value of $c$ can be found in Appendix.}.
% \label{lemm:iab_guss}
% \end{lemm}

% To analyze $I_{A_t, B_t}$, we note that $d P_{B_{t}, \boldsymbol{\xi}_{t}}$, $d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}$ and $d P_{A_{t},\boldsymbol{\xi}_{t}}$ are distribution functions of Gaussian distribution with different mean, i.e., $\m_{B_t}$, $\m_{B_t}^\prime$ and $\m_{A_t}^\prime$. Thus it is straightforward to write 
% \begin{align}
% I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{d}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w-\m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
% \end{align}


We highlight the essentials of the proofs here. For any $B_t$ and $A_t$, since $P_{B_{t}, \boldsymbol{\xi}_{t}}$, $P^\prime_{B_{t}, \boldsymbol{\xi}_{t}}$ and $P_{A_{t}, \boldsymbol{\xi}_{t}}$ are Gaussian distributions. Thus, $d P_{B_{t}, \boldsymbol{\xi}_{t}}$, $d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}$ and $d P_{A_{t},\boldsymbol{\xi}_{t}}$ are distribution density functions of Gaussian distribution. Then, it is straightforward to have 
\begin{align}
I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{d}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w-\m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
\end{align}
Note that the above calculation considers integral over $d$-dimensional space which introduced an undesired dimension dependence. However, we note that
isotropic Gaussian noise is spherical symmetric,  we can translate and rotate the coordinate system so that 
$\m_{A_t}=0$  and $ \m_{B_t}, \m_{B_t}^{\prime}$ are mapped to a 2-dimensional space and the Euclidean distances $\|\w-\m_{B_t} + \m_{A_t}\|$, $\|\w-\m_{B_t}^\prime + \m_{A_t}\|$ do not change (Details  can be found in  Appendix \ref{app:guss}). Then
we have $I_{A_t, B_t}$ as 
\begin{align}
I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{2}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime} + \m_{A_t} \right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
\end{align}
Then we treat $\exp \left(-\left\|\w-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ and $\exp \left(-\left\|\w-\m_{B_t}^\prime + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ as two functions of $\w$ where we can 
use Taylor expansion and apply mean-field theorem to bound $I_{A_t, B_t}$ as
\begin{align*}
I_{A_t, B_t} \leq c \frac{\|\m_{B_t} - \m_{B_t}^\prime \|_2^2}{\sigma_t^2}=  c \frac{\eta_t^2\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}}{\sigma_t^2}~,
\end{align*}
where $c$ is a constant with detailed value in  Appendix. Thus, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate,  we have
\begin{align}
\nr K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right) & = \underset{B_{t} \in G_{1},A_{t} \in G_{0}}{\mathbb{E}}\left[\int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}\right]   \leq  \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

Then, based on the chain rule of KL-divergence, we have
\begin{align}
\nr K L\left(P_{0: T} \| P_{0: T}^{\prime}\right) 
& = \sum_{t=1}^{T} \mathbb{E}_{\w_{t-1}} \left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

\begin{restatable}{theo}{genboundguss}
Consider Noisy SGD of update rule \eqref{eq: sgd_guss_update},  with mini-batch size $b \leq n/2$, for any given sample $\bar S$, at every $t$-th iteration, let step size $\eta_t$ and noise $\sigma_t$ be adaptively chosen as in Lemma \ref{lemm:iab_guss}, 
% such that, for any observed $\w_{t-1}$,  $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$, where $\Delta_{t}(\bar{S})=\max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z\right)-\nabla \ell\left(\mathbf{w}_{t-1}, \tilde{z}\right)\right\|_{2}$ 
%Then, with $c = \sqrt{2} c_0$, 
we have 
\begin{align}
\left|\mathbb{E}_{S}\left[L_{D}(\w_T)-L_{S}(\w_T)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar S} \sqrt{\sum_{t=1}^{T} \underset{\w_{t-1}}{\mathbb{E} }\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~},
\end{align}
where $c = 41 \ln \frac{3}{2}$.
\label{theo:guss_gen}
\end{restatable}

% \begin{theo}
% Consider Noisy SGD of update rule \eqref{eq: sgd_guss_update},  with mini-batch size $b \leq n/2$, for any given sample $\bar S$, at every $t$-th iteration, let step size $\eta_t$ and noise $\sigma_t$ be adaptively chosen as in Lemma \ref{lemm:iab_guss}, 
% % such that, for any observed $\w_{t-1}$,  $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$, where $\Delta_{t}(\bar{S})=\max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z\right)-\nabla \ell\left(\mathbf{w}_{t-1}, \tilde{z}\right)\right\|_{2}$ 
% %Then, with $c = \sqrt{2} c_0$, 
% we have 
% \begin{align}
% \left|\mathbb{E}_{S}\left[L_{D}(\w_T)-L_{S}(\w_T)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar S} \sqrt{\sum_{t=1}^{T} \underset{\w_{t-1}}{\mathbb{E} }\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~},
% \end{align}
% where $c$ is a constant with detailed value presented in Appendix.
% \label{theo:guss_gen}
% \end{theo}

Theorem \ref{theo:guss_gen} shows that 
the expected generalization error of Noisy SGD with Gaussian noise scales as $O(\sqrt{\sum_t^T \frac{\eta_t^2}{\sigma_t^2}}/n)$, capturing the same dependence on $n$, $T$, step size $\eta_t$ as the bound in \cite{Li2020On}. However there are two key differences making our bound sharper than existing bounds in \cite{Li2020On} and \cite{negrea2019information}. The first key difference between our result and \cite{Li2020On} is that we replace the \emph{gradient norms}, i.e., $\frac{1}{n}\sum_{z \in S}\|\ell(\w_t,z)\|$ in \cite{Li2020On} and with gradient discrepancy $\|\nabla \ell(\w_t,z) - \nabla \ell(\w_t, z^\prime) \|$, which is quantitatively smaller than gradient norms as we show in the experiment section. 
The second key difference is the sample dependence compared to  \cite{negrea2019information}.
Although, \cite{negrea2019information} also derived a generalization error bound depending a factor that is similar to gradient discrepancy, named  \emph{gradient incoherence} in their paper.  
The difference between gradient discrepancy and gradient incoherence is that, gradient discrepancy is evaluated on $z$ from training set and $z^\prime$ from a validation set. The gradient incoherence is the difference between gradients on subset of training samples. Although gradient incoherence is empirically smaller as observed in the experiment section, their bound depends on $\frac{1}{\sqrt{n}}$, which is worse than the $\frac{1}{n}$ dependence in our bound. 
Thus, our bound in Theorem \ref{theo:guss_gen} inherits the strengths of the existing bounds with dependence on norms of gradient discrepancy, and an $O(1/n)$ sample dependence

% The key difference is the order of dependence on the sample size $n$, i.e., both of our bound and $\cite{Li2020On}$ has a bound of order $\frac{1}{n}$, however, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$.




%Based on the chain rule of  KL-divergence, we have
% \begin{align*}
%  KL(w_1,..., w_T \| w'_1,..., w'_T) \leq  \frac{b^{2}}{n^{2}}  \frac{12 c }{\sigma^2} (1 + \frac{5\ln c}{2})  \sum_{t=1}^T \| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2~.
% \end{align*}




%\newpage

==> Arxiv(old)/sec/stab_heavy_tailed.tex <==

Results for noise with $\exp(-t)$ tail

\subsection{Laplace Noise}


\subsection{Sub-Exponential Noise}


\subsection{Heavy Tails: Infinitely Divisible, Stable Noise}


\section{Experiment}

Model: MLP,~ CNN.

Datasets: MNIST, Fashion MNIST, CIFAR10.

Noise: Gaussian, discrete noise

Plot: Bounds, gradient norm, gradient difference norm. 


==> ICLR2022/app/app_exp.tex <==
{\bf Datasets.} We use MNIST \cite{mnist}, Fashion-MNIST \cite{fashion-mnist}, CIFAR-10 \cite{cifar10} and CIFAR-100 \cite{cifar10} in our experiments.


%The MNIST and Fashion MNIST datasets both consist of 60,000 training examples and 10,000 test examples. %To construct the experiments, we randomly sample $10,000$  samples from the original training set of MNIST and Fashion MNIST. 
%Details refer to  Table \ref{tab::network_setup_app}. 

\noindent {\bf MNIST dataset:} 60,000 black and white training images, including handwritten digits 0 to 9. We use a subset of MNIST with $n = 10,000$ data points where 1,000 samples from each class are randomly selected. Each image of size $28 \times 28$ is first re-scaled into [0,1] by dividing each pixel value by 255, then z-scored by subtracting the mean and dividing the standard deviation of the training set.


\noindent {\bf Fashion-MNIST dataset:} 60,000 gray-scale training images and 10,000 test images, including 10 clothing categories such as shirts, dresses, sandals, etc. Each image of size $28 \times 28$ is first re-scaled into [0,1] by dividing each pixel value by 255, then z-scored by subtracting the mean and dividing the standard deviation of the training set. 


\noindent {\bf CIFAR-10/-100 dataset:} 60,000 color images consisting of 10/100 categories, e.g., airplane, cat, dog etc. The training set includes 50,000 images while the test set contains the rest 10,000 images. Each image of size $32 \times 32$ has 3 color channels. We first re-scale each image into [0, 1] by dividing each pixel value by 255, then each image is normalized by subtracting the mean and dividing the standard deviation of the training set for each color channel. We also use \textit{RandomCrop} and \textit{RandomHorizontalFlip} for data augmentation.




{\bf Network Architectures.} For experiments on both MNIST and Fashion-MNIST, we use a convolutional neural network with two convolutional layers followed by two fully connected layers with ReLU activations. For experiments use the CIFAR-10 dataset, we consider CNN architecture with two convolutional layers
and three fully connected layers. The detail of each CNN architecture can be found in Table \ref{tab:cnn1} and Table~\ref{tab:cnn2}.

\begin{table}[h]
\caption{CNN architecture for MNIST and Fashion MNIST.}
\centering
\begin{tabular}{cc} 
Layer & Parameters \\
\hline \hline Convolution & 32 filters of $5 \times 5$ \\
Max-Pooling & $2 \times 2$ \\
Convolution & 64 filters of $5 \times 5$\\
Max-Pooling & $2 \times 2$ \\
Fully connected & 1024 units \\
Softmax & 10 units \\
\hline
\end{tabular}
    \label{tab:cnn1}
\end{table}


\begin{table}[h]
\caption{CNN architecture for CIFAR-10.}
\centering
\begin{tabular}{cc} 
Layer & Parameters \\
\hline \hline Convolution & 64 filters of $5 \times 5$ \\
Max-Pooling & $2 \times 2$ \\
Convolution & 192 filters of $5 \times 5$\\
Max-Pooling & $2 \times 2$ \\
Fully connected & 384 units \\
Fully connected & 192 units \\
Softmax & 10 units \\
\hline
\end{tabular}
    \label{tab:cnn2}
\end{table}



% \begin{table}[h]
%   \caption{Neural network and datasets setup.}
% 	\centering
% 	\footnotesize{
% 	%\resizebox{\columnwidth}{!}{%
% 	\begin{tabular}{cccccc}	
% 	\toprule[1pt]
% 	Dataset & Model  & features & classes & Training size  & Test size\\ 	
% 	\toprule[1pt]
% 		MNIST            & CNN \& MLP & 28$\times$ 28 & 10 &  10,000  & 10,000\\
% Fashion MNIST   & CNN \& MLP  &  28$\times$ 28 & 10 &  10,000  & 10,000\\
% 		\toprule[1pt]
% 	\end{tabular}}
% %	}
% 	\label{tab::network_setup_app}
% \end{table}


\textbf{Experimental setup.}  We are interested in stochastic gradient Langevin dynamics,
whose iterative updates are given by $\mathbf{w}_{t}=\mathbf{w}_{t-1}-\eta_{t} \boldsymbol{\xi}_{t}, ~\text{where}~ \boldsymbol{\xi}_{t} \sim \mathcal{N}\left(\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right), \sigma_{t}^{2}/\eta_t^2 \mathbb{I}_{d}\right)$. In particular, we consider $\sigma_t=\sqrt{2\eta_t/\beta_t}$, where $\beta_t$ is the the inverse temperature at time t. For MNIST and Fashion-MNIST, the initial learning rate is $\eta_0=0.004$ and it decays by 0.96 after every 5 epochs. For CIFAR-10,the initial learning rate is $\eta_0=0.005$ and it decays by 0.995 after every 5 epochs. We use batch size $|B_t| = 100$ for MNIST and Fashion-MNIST, and $|B_t| = 200$ for CIFAR-10. %We also consider SGLD with $\sigma_t=\alpha_t\cdot\eta_t$ can be found in Figure~\ref{fig:mnist_noisysgd} in Appendix \ref{app:exp}. 


Motivated by \cite{zhang2017understanding}, we train CNN with SGLD on a smaller subset of MNIST dataset ($n=10000$) with randomly corrupted labels. The corruption fraction varies from $0\%$ (without label corruption) to $60\%$. For different level of randomness, we use the same training setting with batch size $|B_t|=100$, initial step size $\eta_0 = 0.005$, noise variance $\sigma_t = 0.2 \cdot \eta_t$, and we decay $\eta_t$ by 0.995 for every 30 epochs. 



We are also interested in Noisy Sign-SGD whose iterative updates are given by %$\mathbf{w}_{t}=\mathbf{w}_{t-1}-\eta_{t}\boldsymbol{\xi}_{t}$, where $\boldsymbol{\xi}_{t} \sim \text{Bernoulli} \left(\frac{1}{1+\exp{\left(-\frac{\nabla \ell(w_{t-1},S_{B_{t}})}{\alpha_t}\right)}}\right)$
$\w_{t+1} = \w_{t} - \eta_t \bxi_t$, where $\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(\xi_j)=\frac{\exp(\xi_j \btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})}$. The initial learning rate is $\eta_0=10^{-4}$ and it decays by 0.1 after every 30 epochs. We use batch size $|B_t| = 100$ for all benchmarks.




%where $~ \bxi_{t,i} \sim p_{\alpha_t}(\xi) = \frac{1}{\exp((1-\xi)\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)/\alpha_t)+\exp((-1-\xi)\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)/\alpha_t)}~, ~ \xi\in\{-1,+1\}$. 




All experiments minimize cross-entropy loss for a fixed number of epochs and have been run on NVIDIA Tesla K40m GPUs. For CNN, we repeat each experiment 30 times, and for ResNet-18, we repeat 5 times.


\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:sgld_bound} and \ref{fig:sgld_mnist} for MNIST and Fashion-MNIST with CNN}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & MNIST/ Fashion-MNIST \\\hline
Architecture & CNN with 2 conv. layers and 2 linear layers \\\hline
Batch Size & $100$\\\hline
Learning Rate & $\eta_0=4\times10^{-3}$, decay epochs=5, decay rate=0.96 \\\hline
Inverse Temperature& $\beta \in [5000, 55000]$ \\\hline
Number of Epochs & 50\\\hline
No. of training examples & 55000 \\\hline
Number of Repeated Runs & 30 \\
\hline
\end{tabular}
\label{tab:mnist}
\end{table}


\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:sgld_bound} and \ref{fig:sgld_cifar10} for CIFAR-10 with CNN}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & CIFAR-10\\\hline
Architecture & CNN with 2 conv. layers and 3 linear layers \\\hline
Batch Size & $200$\\\hline
Learning Rate & $\eta_0=5\times10^{-3}$, decay epochs=5, decay rate=0.995 \\\hline
Inverse Temperature& $\beta \in [5000, 55000]$ \\\hline
Number of Epochs & 1000\\\hline
No. of training examples & 55000 \\\hline
Number of Repeated Runs & 20 \\
\hline
\end{tabular}
\label{tab:cifar10}
\end{table}



\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:bound_random} for MNIST with CNN ($\sigma_t = 0.2 \cdot \eta_t$)}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & MNIST\\\hline
Architecture & CNN with 2 conv. layers and 2 linear layers \\\hline
Batch Size & $100$\\\hline
Learning Rate & $\eta_0=5\times10^{-3}$, decay epochs=30, decay rate=0.995 \\\hline
Number of Epochs & 1000\\\hline
No. of training examples & 10000 \\\hline
Number of Repeated Runs & 30 \\
\hline
\end{tabular}
\label{tab:random}
\end{table}





\begin{figure*}[t] 
\centering
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-c.png}
 }
  \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-c.png}
 }
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
\includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-b.png}
 }
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
\includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-b.png}
 }   
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-a.png}
 }
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a.png}
 } 
\caption[]{Numerical results for CNN trained on MNIST using SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$). $\beta=55000$ which is equivalent a small noise variance $\sigma_t\approx 10^{-4}$.
}
\label{fig:sgld_mnist}
\end{figure*}




\begin{figure*}[t] 
\centering
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-c.png}
 }
\subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-c.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-b.png}
 } 
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-b.png}
 }
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-a.png}
 }
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a.png}
 } 

%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-5000.0-b.png}
%  } 
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-55000.0-b.png}
%  }
%   \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a.png}
%  } 
%   \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-a.png}
%  }
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-5000.0-a.png}
%  } 
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-55000.0-a.png}
%  }  
\caption[]{Numerical results for training CNN using SGLD with $\sigma_t = \sqrt{2\eta_t/\beta_t}$ on CIFAR-10. 
}
\label{fig:sgld_cifar10}
\end{figure*}






% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN, MNIST]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/cnn1-mnist-n0-bs100-sign-sgd-train-dynamics.png}
%  } 
%   \subfigure[CNN, Fashion]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/cnn1-fashion-n0-bs100-sign-sgd-train-dynamics.png}
%  }
%  \subfigure[ResNet-18, CIFAR10]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/resnet18-cifar10-n0-bs100-sign-sgd-train-dynamics.png}
%  }
%  \subfigure[ResNet-18, CIFAR100]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/resnet18-cifar100-n0-bs100-sign-sgd-train-dynamics.png}
%  }
% \caption[]{Training dynamics of Noisy sign-SGD with different scaling $\alpha_t$. Legends indicate the choice of  $\alpha_t$ and the numbers in brackets are the test accuracy at convergence. As $\alpha_t\to 0$, Nosiy sign-SGD matches both the optimization trajectory as well as the final test accuracy of original sign-SGD \citep{bernstein2018signsgd}.
% }
% \label{fig:train_noisy_signsgd_full}
% \end{figure*}






% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN, MNIST, Noisy sign-SGD, $\alpha_t = 0.1$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-bernoulli-beta-0.1.png}
%  } 
%  \subfigure[CNN, Fashion, Noisy sign-SGD, $\alpha_t = 0.1$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-bernoulli-beta-0.1.png}
%  }
%  \subfigure[ResNet-18, CIFAR-10, Noisy sign-SGD, $\alpha_t = 0.1$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/resnet18-cifar10-bounds-bernoulli-beta-0.1.png}
%  }
%  \subfigure[ResNet-18, CIFAR-100, Noisy sign-SGD, $\alpha_t = 0.1$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/resnet18-cifar100-bounds-bernoulli-beta-0.1.png}
%  } 
 
% \caption[]{Numerical results for training CNN on MNIST and Fashion-MNIST, and ResNet-18 on Cifar-10 and Cifar-100 using Noisy Sign-SGD.
% }
% \label{fig:bound_noisy_signsgd_full}
% \end{figure*}









\begin{figure*}[th] 
\centering
  \subfigure[CNN, MNIST, Noisy-SGD, $\alpha_t = 0.2$, $\sigma_t\approx 10^{-4}$]{
 \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-beta-0.2.png}
 } 
  \subfigure[CNN, MNIST, Noisy-SGD, $\alpha_t = 0.002$, $\sigma_t\approx 10^{-6}$]{
 \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-beta-0.002.png}
 }
\caption[]{Numerical results for CNN trained on MNIST using Noisy SGD, where $\sigma_t=\alpha_t\eta_t$. We follow the setting described in \cite{Li2020On}. The initial $\eta_t$ is $4\times 10^{-3}$, and decays by 0.95 ($\alpha_t=0.2$) or 0.995 ($\alpha_t=0.002$) for every 5 epochs. 
}
\label{fig:mnist_noisysgd}
\end{figure*}




\begin{figure*}[t] 
\centering
 \subfigure[MNIST, $\alpha_t = 1.0$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
 }
 \subfigure[MNIST, $\alpha_t = 0.1$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-d.png}
 }
 \subfigure[MNIST, $\alpha_t = 0.01$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-e.png}
 }
  \subfigure[MNIST, Our Bound]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-b.png}
 }  
 \subfigure[MNIST, Gradient Discrepancy]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-a.png}
 }
 
 \subfigure[Fashion, $\alpha_t = 1.0$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
 }
 \subfigure[Fashion, $\alpha_t = 0.1$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-d.png}
 }
 \subfigure[Fashion, $\alpha_t = 0.01$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-e.png}
 }
  \subfigure[Fashion, Our Bound]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-b.png}
 }  
 \subfigure[Fashion, Gradient Discrepancy]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-a.png}
 }  
 
\caption[]{Numerical results for training CNN on MNIST and Fashion-MNIST using Noisy Sign-SGD. Increasing $\alpha_t$ leads to a tighter generalization bound even though it leads to a slightly larger gradient discrepancy. 
}
\label{fig:bound_noisy_signsgd}
\end{figure*}





% \clearpage
% \textbf{Experiments on Cifar10 dataset.} We run experiments and compare our bound with the bound in \cite{Li2020On} and \cite{negrea2019information} on Cifar10 dataset. We consider vgg 11 network model with 10,000 training samples randomly sampled from Cifar10 dataset. For training we use initial learning rate 0.001, and noise variance decay such that $\sigma_t = 0.3\eta_t$ and $\sigma_t = 0.5\eta_t$, and we decay $\eta_t$ every 10 epochs with decaying rate 0.93. Figure \ref{fig:cifar10} shows our bound is sharper than existing bound under different noise variance settings.
% \begin{figure*}[h] 
% \centering
% %   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
% %  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
% %  } 
% %   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
% %  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
% %  }  
%   \subfigure[$\sigma_t = 0.3 \eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_lr0.001_alpha0.3_mo0.0_decay0.93.png}
%  }  
%   \subfigure[$\sigma_t = 0.5 \eta_t$]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_lr0.001_alpha0.5_mo0.0_decay0.93.png}
%  }

% \caption[]{Numerical results for cifar10 dataset. Figure (a-b) shows our bound is sharper than existing bound under different settings of noise variance.
% }\label{fig:cifar10}
% \end{figure*}






% \textbf{Random Label Experiments.} Inspired by \cite{zhang2017understanding}, we run SGLD to fit 10,000 samples from MNIST dataset Figure \ref{fig:random_label_mnist} and fashionMNSIT dataset Figure \ref{fig:random_label_fashion_mnist}, with increasing fractions of randomly labeled data, from fractions $0\%$ (normal data) to $60\%$. We consider a MLP network with two hidden layers with 128,128 nodes respectively in each layer. For different level of randomly labeled data, we use the same training setting with batch size $|B_t|=128$, initial step size $\eta_0 = 0.05$, noise variance $\sigma_t = 0.07 \cdot \eta_t$, and we decay $\eta_t$ every 10 epochs by 0.95. As shown in Figure~\ref{fig:random_label_mnist} (a) and \ref{fig:random_label_fashion_mnist} (a), with a fixed running time, the experiment with higher level of randomly labeled data has lower training accuracy. Figure \ref{fig:random_label_mnist} (b) and \ref{fig:random_label_fashion_mnist} (b) show higher level of randomly labeled data has higher generalization error and our bound also increase with higher level of randomness, which matches the behavior of generalization error.



==> ICLR2022/app/efld.tex <==

%\abcomment{some text}

In this section, we provide the proofs for Section \ref{sec:efld}. We first review and show details of a few examples of exponential family.



\subsection{Examples of Exponential Family}\label{app:example}
\begin{exam}[Gaussian]
For univariate Gaussians with fixed variance $\sigma^2$, the scaling $\alpha = \sigma$, the sufficient statistic $\xi = x/\sigma$, the log-partition function  $\psi(\theta) = \theta^2/2$, and the base measure $\pi_0(\xi) = \frac{1}{\sqrt{2\pi}} \exp(-\xi^2/2)$ or equivalently $\pi_0(x) = \frac{1}{\sqrt{2\pi}\sigma} \exp(-x^2/2\sigma^2)$ using $\xi = x/\sigma$ and $d\xi = dx/\sigma$. The scaled parameter $\theta_{\alpha} = \theta_{\sigma} = \theta/\sigma$. Then, the distribution from the natural parameter form is:
\begin{equation}
    p_{\theta/\sigma}(x) = \exp( x \theta / \sigma^2 - \theta^2/(2\sigma^2) ) \times \frac{1}{\sqrt{2\pi}\sigma} \exp(-x^2/2\sigma^2)
    = \frac{1}{\sqrt{2\pi}\sigma} \exp(-(x-\mu)^2/2\sigma^2)~.
\end{equation}
The expectation parameter $\mu = \nabla \psi(\theta) = \theta$. The scaled expectation parameter $\mu_{\alpha} = \nabla \psi(\theta_\alpha) = \theta_\alpha = \theta/\sigma = \mu/\sigma$. Since $\xi = x/\sigma$ and the Bregman divergence $d_{\phi}(\xi,\mu) = \frac{1}{2}(\xi-\mu)^2$, the expectation parameter form
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(-(x/\sigma - \mu/\sigma )^2/2) \frac{1}{\sqrt{2\pi} \sigma} = \frac{1}{\sqrt{2\pi}\sigma} \exp(-(x-\mu)^2/2\sigma^2)~.\qed
\end{equation}
\end{exam}

\begin{exam}[Bernoulli over $\{0,1\}$]
For Bernoulli over $\{0,1\}$, the sufficient statistic $\xi = x \in \{0,1\}$, base measure is 1 on $\{0,1\}$, and the log-partition function $\psi(\theta) = \log(1+\exp(\theta))$ for natural parameter $\theta \in \R$. The expectation parameter $\mu = \nabla \psi(\theta) = \frac{exp(\theta)}{1+\exp(\theta)} = \frac{1}{1+\exp(-\theta)}$, the sigmoid function of $\theta$. The Bregman divergence is the Bernoulli KL-divergence given by: $d_{\phi}(\xi,\mu) = x \log \frac{x}{\mu} + (1-x) \log \frac{1-x}{1-\mu}$. For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{1}{1+\exp(-\theta_{\alpha})}$. 
The mean parameter form distribution is given by
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha}) = \mu_{\alpha}^{\xi} (1-\mu_{\alpha})^{1-\xi}~.
\end{equation}
\qed
\end{exam}

\begin{exam}[Bernoulli over $\{-1,1\}$]
For Bernoulli over $\{-1,1\}$, the sufficient statistic $\xi = x \in \{-1,1\}$, base measure is 1 on $\{-1,1\}$, and the log-partition function $\psi(\theta) = \log(\exp(-\theta)+\exp(\theta))$ for natural parameter $\theta \in \R$. The expectation parameter $\mu = \nabla \psi(\theta) = \frac{\exp(\theta)- \exp(-\theta)}{\exp(-\theta)+\exp(\theta)} = \frac{\exp(2\theta)-1}{\exp(2\theta)+1}$, then its inverse function $\theta = \nabla \phi(\mu) = \frac{1}{2}\log \left(\frac{1+\mu}{1-\mu}\right)$, by integration we have $\phi(\mu) = \frac{1+\mu}{2}\log\frac{1+\mu}{2}+ \frac{1-\mu}{2}\log\frac{1-\mu}{2}$. The Bregman divergence is given by: $d_{\phi}(\xi,\mu) = \frac{1+\xi}{2} \log \frac{1+\xi}{1+\mu} + \frac{1-\xi}{2} \log \frac{1-\xi}{1-\mu}$. For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{\exp(2\theta_\alpha)-1}{\exp(2\theta_\alpha)+1}$. Noting that $\frac{1+\xi}{2} \log \frac{1+\xi}{2} = \frac{1-\xi}{2} \log \frac{1-\xi}{2} = 0$ for the base measure, the distribution is given by
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha})) = \left(\frac{1+\mu_\alpha}{2}\right)^{\frac{1+\xi}{2}} \left(\frac{1-\mu_\alpha}{2}\right)^{\frac{1-\xi}{2}},
\end{equation}
which is $\xi = 1$ with probability $\frac{1+\mu_\alpha}{2}$ and $\xi = -1$ with probability $\frac{1-\mu_\alpha}{2}$.\qed
% Therefore, the EFLD update reduces to a noisy version of sign-SGD: \begin{equation}\label{eq:signSGD_mini_batch_1}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, ~\bxi_{t,i} \sim p_{\btheta_{B_t,\alpha_t,i}}(\xi) =  \frac{1}{\exp((1-\xi)\btheta_{B_t,\alpha_t,i})+\exp((-1-\xi)\btheta_{B_t,\alpha_t,i})}~, ~ \xi\in\{-1,+1\}
% \end{equation}
% for any $i\in [d]$, where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
\end{exam}

% \begin{exam}[Categorical]
% \abcomment{do we have the details for this? otherwise deop}
% The sufficient statistic $\xi = x = \{-1,0,1\}$, base measure is 1 on $\{-1,0,1\}$, natural parameters $\btheta = [\theta_1~~~\theta_2]^T \in \R^2$, and the log-partition function $\psi(\btheta) = \log(1+\exp(\theta_1) + \exp(-\theta_2))$. The expectation parameter $\mu  = \nabla \psi(\btheta) = [\frac{\exp(\theta_1)}{1+\exp(\theta_1) + \exp(-\theta_2)}, \frac{\exp(-\theta_2)}{1+\exp(\theta_1) + \exp(-\theta_2)}]$ \qed
% \end{exam}











\subsection{Proof of Theorem~\ref{theo:efld}}

\theoefld*

To avoid clutter, we drop the subscript $t$ for the analysis and note that the analysis holds for any step $t$.  When the density $dP_{B,\bxi} = \p_{\psi}(\bxi;\btheta_{B,\alpha})$, by mean-value theorem, for each $\bxi$, we have 
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) 
= \langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ~,
\end{equation}
for some $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$ where $\gamma_{\bxi} \in [0,1]$. Then,
\begin{align}
I_{A,B} &=  \bigintsss_\bxi \frac{\big( p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) \big)^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber 
= \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber \\
& = \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla_{\tilde{\btheta}_{B',\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2p_{\psi}^2(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi ~,
\label{eq:expcore}
\end{align}
since $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) = \exp(\langle \bxi, \tilde{\btheta}_{B,\alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha})) \pi_0(\bxi)$. 


\subsubsection{Handling Distributional Dependency of $\tilde{\btheta}_B$}
Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. In this step we focus on bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$. 


\exptilde*

\proof Denoting $\gamma_{\bxi}$ as $\gamma$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
\begin{align*}
\langle \bxi, & \tilde{\btheta}_{B,  \alpha} \rangle  - \psi(\tilde{\btheta}_{B,\alpha}) 
 = \langle \bxi, \gamma \btheta_{B, \alpha} + (1-\gamma) \btheta'_{B,\alpha} \rangle - \psi\left( \gamma \btheta_{B, \alpha} + (1-\gamma) \btheta'_{B, \alpha} \right) \\
& = \gamma \bigg[ \langle \bxi , \btheta_{B,\alpha} \rangle - \psi(\btheta_{B, \alpha}) \bigg]  + (1-\gamma) \bigg[ \langle \bxi , \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \bigg] \\
& ~~~~~~~~~~~~~~~
  + \bigg[ \gamma \psi(\btheta_{B, \alpha} ) + (1-\gamma) \psi(\btheta'_{B,\alpha}) - \psi( \gamma \btheta_{B,\alpha} + (1-\gamma) \btheta'_{B,\alpha} ) \bigg] \\
& \stackrel{(a)}{\leq} \max\bigg( \langle \bxi , \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) , \langle \bxi , \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha} )  \bigg) \\
& ~~~~~~~~~~~~~~~ 
  + \bigg[ \gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha} , \tilde{\btheta}_{B,\alpha}) \bigg]~,
\end{align*}
where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation (See section 3.1.1 in \cite{banerjee2005clustering}):
\begin{align*}
  \gamma \psi(\btheta_{B, \alpha} ) + (1-\gamma) \psi(\btheta'_{B,\alpha}) - \psi( \gamma \btheta_{B,\alpha} + (1-\gamma) \btheta'_{B,\alpha} )  =  \gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha} , \tilde{\btheta}_{B,\alpha})~.
\end{align*}
Now, note that
\begin{align*}
\gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha})  + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha}, \tilde{\btheta}_{B,\alpha})  
& \leq \gamma d_{\psi}(\btheta_{B,\alpha}, \btheta'_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha}, \btheta_{B,\alpha}) \\
%& \stackrel{(a)}{=} \gamma d_{\phi}(\m'_{B,\alpha}, \m_{B,\alpha}) + (1-\gamma) d_{\phi}(\m_{B,\alpha},\m'_{B,\alpha})~\\
& \leq \gamma c_2 \| \btheta'_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 + (1-\gamma) c_2 \| \btheta_{B,\alpha} - \btheta'_{B,\alpha} \|_2^2 \\
& \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2~.
\end{align*}
As a result,
\begin{align*}
& \frac{\exp\left[\langle \bxi, \tilde{\btheta}_{B, \alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha}) \right]}{\max\left( \exp\left[\langle \bxi, \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) \right] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right] \right) }\\
& ~~~~~ \leq\exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right]
\frac{ \exp \left[ \max\bigg( \langle \bxi , \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) , \langle \bxi , \btheta'_{B,\alpha} \rangle - \psi(\btheta'_{B,\alpha})  \bigg) \right] }{ \max\left( \exp\left[\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha}) \right] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right] \right) } \\
& ~~~~~ = \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right]~.
\end{align*}
That completes the proof.\qed 







\subsubsection{Bounding the Density Ratio}



Focusing on density ratio, we have

\expdr*

\proof  Note that
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B,\alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A , \alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}  
& = \exp\left[ \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \rangle - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big) \right] \\
& = \beta_{B,A,\alpha} \exp \left[  \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha} \rangle - \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \right]~,
\end{align*}
where
\begin{align*}
\beta_{B,A,\alpha} & = \exp \left[ \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big) \right] ~.
\end{align*}
Note that
\begin{align*}
\log \beta_{B,A,\alpha} & = \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big)\\
& = - \bigg( \psi(\btheta_{B,\alpha}) - \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \bigg) - \bigg( \psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \bigg) \\
& \stackrel{(a)}{\leq} \bigg\langle \btheta_{B,\alpha} - \btheta_{A,\alpha}, \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \bigg\rangle + \bigg\langle \btheta_{A,\alpha} - \btheta_{B,\alpha}, \nabla \psi( \btheta_{A,\alpha} \bigg\rangle   \\
& = \bigg\langle \btheta_{B,\alpha} - \btheta_{A,\alpha}, \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\btheta_{A,\alpha})  \bigg\rangle  \\
& \stackrel{(b)}{\leq} \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2 \| \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\btheta_{A,\alpha}) \|_2  \\
& \stackrel{(c)}{\leq} c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2 \| (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \btheta_{A,\alpha} \|_2 \\
& = 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2~,
\end{align*}
where (a) follows from the convexity of $\psi$, (b) follows from Cauchy-Schwartz, and (c) follows by smoothness of $\psi$.


As a result, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B,\alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A, \alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}
&\leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \psi( (2\btheta_B - \btheta_A)/\alpha) \right]~.
\end{align*}
That completes the proof.\qed

The analysis for the term involving $\btheta'_B$ is exactly the same. 

% \abcomment{state a Lemma by combining Lemma 2 and Lemma 3?}

% \abbcomment{Lemma will help the reader understand that the base measure scales correctly, and essentially stays unchanged}

Combining Lemma~\ref{lemm:exp_step2} and \ref{lemm:exp_step3}, we have the following result:
\begin{restatable}{lemm}{expcompile}
We have
\begin{equation}
\begin{split}
\frac{p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi;\btheta_{A,\alpha})} 
 & \leq \exp\left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right] \\
 & \phantom{...........} 
\times \max\big( \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B,\alpha} - \btheta_{A,\alpha})~,  \big. \\
& \phantom{........................} \left. 
\exp \left[2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B',\alpha} - \btheta_{A,\alpha}) \right)~.
\end{split}
\end{equation}
\label{corr:expcompile}
\end{restatable}
\proof 


From Lemma \ref{lemm:exp_step2}, we have
\begin{align*}
p_{\psi}^2(\boldsymbol{\xi} ; \tilde{\boldsymbol{\theta}}_{B, \alpha}) & = \exp \left[2\left\langle\boldsymbol{\xi}, \tilde{\boldsymbol{\theta}}_{B, \alpha}\right\rangle-2\psi\left(\tilde{\boldsymbol{\theta}}_{B, \alpha}\right)\right] \\
& \leq \exp \left[c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{B^{\prime}, \alpha}\right\|_{2}^{2}\right] \cdot \max \left(\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right], \exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B^{\prime}, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{B^{\prime}, \alpha}\right)\right]\right)
\end{align*}

Thus,

\begin{align*}
\frac{p_{\psi}^{2}\left(\boldsymbol{\xi} ; \tilde{\boldsymbol{\theta}}_{B, \alpha}\right)}{p_{\psi}\left(\boldsymbol{\xi} ; \boldsymbol{\theta}_{A, \alpha}\right)} \leq \exp \left[2 c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{B^{\prime}, \alpha}\right\|_{2}^{2}\right] \cdot  \frac{\max \left(\exp \left[2\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B, \alpha}\right\rangle-2\psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right], \exp \left[2\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B^{\prime}, \alpha}\right\rangle-2\psi\left(\boldsymbol{\theta}_{B^{\prime}, \alpha}\right)\right]\right)}{\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{A, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{A, \alpha}\right)\right]}
\end{align*}

Based on Lemma \ref{lemm:exp_step3}, we have
\begin{align*}
\frac{\exp \left[\left\langle\boldsymbol{\xi}, 2 \boldsymbol{\theta}_{B, \alpha}\right\rangle-2 \psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right]}{\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{A, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{A, \alpha}\right)\right]} \leq \exp \left[2 c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{A, \alpha}\right\|_{2}^{2}\right] \exp \left[\left\langle\boldsymbol{\xi},\left(2 \boldsymbol{\theta}_{B}-\boldsymbol{\theta}_{A}\right) / \alpha\right\rangle-\psi\left(\left(2 \boldsymbol{\theta}_{B}-\boldsymbol{\theta}_{A}\right) / \alpha\right)\right]
\end{align*}

Combining above inequalities we have
\begin{equation}
\begin{split}
\frac{p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi;\btheta_{A,\alpha})} 
 & \leq \exp\left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right] \\
 & \phantom{...........} 
\times \max\big( \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B,\alpha} - \btheta_{A,\alpha})~,  \big. \\
& \phantom{........................} \left. 
\exp \left[2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B',\alpha} - \btheta_{A,\alpha}) \right)~.
\end{split}
\end{equation}

That completes the proof. \qed


\subsubsection{Bounding the Integral}

Ignoring multiplicative terms which do not depend on $\bxi$ for the moment, the analysis needs to bound an integral term of the form
\begin{equation}
    \bigintsss_\bxi \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2 ~p_{\psi}(\bxi;2 \btheta_{B,\alpha} - \btheta_{A,\alpha}) d\bxi~,
\end{equation}
and a similar term with $p_{\psi}^2(\bxi;2 \btheta_{B',\alpha} - \btheta_{A,\alpha})$. The proof of Theorem~\ref{theo:efld} can be done by suitably bounding the integral.
% \begin{restatable}{lemm}{lemmexpinfo}
% \label{lemm:exp_info}
% Consider Noisy SGD with exponetial family noise such that the log-partition function is  $c_1$-strongly convex and $c_2$-smooth, for a given sample set $\bar S$ and parameters $\w_{t-1}$, let $\Delta_{t}(\bar{S}) \triangleq \max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ be data-dependent and adaptively chosen such that $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq \abedit{c(c_1,c_2)}$, then for any $B_t \in G_1$ and  $A_t \in G_0$,  we have \abcomment{notation and constants need work, result needs to be updated}
% \begin{align}
% I_{A_t, B_t} \leq c_0 c_2^2\frac{\eta_{t}^{2}}{\alpha_t^2} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
% \end{align}
% where $c(c_1,c_2) = \frac{c_1^2}{(3c_2-c_1)c_2(1+c_1)}$.
% \end{restatable} 

{\em Proof of Theorem~\ref{theo:efld}.} From Lemma~\ref{corr:expcompile}, we have
\begin{align*}
&I_{A,B}\leq \bigintsss_\bxi \frac{ \left\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi( \tilde{\btheta}_{B,\alpha}) \right\rangle^2 p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{ p_{\psi}(\bxi;\btheta_{A,\alpha})} d\bxi\\
&\leq  \exp\left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2\right] \\
& ~~~~~~~~~~~~~~~~~~~~\times \max\left(  \exp \left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \right. ~, \\
& ~~~~~~~~~~~~~~~~~~~~~~~~~~~
\left.   \exp \left[ 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B',\alpha}-\btheta_{A,\alpha}) d\bxi \right)~.
\end{align*}
Focusing on the integral in the first term (the analysis for the second term is essentially the same), we have
\begin{align*}
& \bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi; 2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = \bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \big( \bxi - \E[\bxi] \big) - \left(\nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& \leq 2\underbrace{\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \E[\bxi] \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi}_{T_1} \\
& \phantom{\leq} + 2 \underbrace{\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi}_{T_2}~.
\end{align*}
For $T_1$, note that 
\begin{align*}
T_1 & = \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \E[\bxi] \right\rangle^2   \right] \\
& = (\btheta_{B,\alpha} -\btheta_{B',\alpha})^T \E_{\bxi \sim p_{\psi}(2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (\bxi - \E[\bxi]) (\bxi - \E[\bxi])^T \right] (\btheta_{B,\alpha} -\btheta_{B',\alpha})~\\
& = (\btheta_{B,\alpha} -\btheta_{B,\alpha})^T \nabla^2 \psi( 2\btheta_{B,\alpha}-\btheta_{A,\alpha})  (\btheta_{B,\alpha} -\btheta_{B',\alpha}) \\
& \leq c_2 \| \btheta_{B,\alpha} -\btheta_{B,\alpha} \|_2^2~,
\end{align*}
since, by smoothness, the spectral norm of $\nabla^2 \psi$ is bounded by $c_2$. 

For $T_2$, first note that 
\begin{align*}
\E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}[\bxi] = \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) ) ~.
\end{align*}
Hence, with $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta_{B',\alpha}$ for some $\gamma_{\bxi} \in [0,1]$, we have
\begin{align*}
T_2 & = \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha},  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right\rangle^2   \right] \\    
& = \E_{\bxi \sim p_{\psi}(\bxi; 2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha},  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha})  \right\rangle^2   \right]\\
& \leq  \| \btheta_{B,\alpha} -\btheta_{B,\alpha} \|_2^2 ~~~\E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\|  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \right\|_2^2  \right]\\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\|  \tilde{\btheta}_{B,\alpha} - (2\btheta_{B,\alpha} - \btheta_{A,\alpha} ) \right\|_2^2  \right] \\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})} \left[ \big\| \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta_{B',\alpha} - \btheta_{B,\alpha} - (\btheta_{B,\alpha} - \btheta_{A,\alpha}) \big\|_2^2 \right] \\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}
\left[ \big\|  (1-\gamma_{\bxi}) (\btheta_{B',\alpha} - \btheta_{B,\alpha}) - (\btheta_{B,\alpha} - \btheta_{A,\alpha}) \big\|_2^2 \right] \\
& \leq  2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ 
\left( \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (1-\gamma_{\bxi})^2  \big\|  \btheta_{B',\alpha} - \btheta_{B,\alpha} \big\|_2^2 \right]
+  \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})} \left[ \big\|  \btheta_{B,\alpha} - \btheta_{A,\alpha} \big\|_2^2 \right]  \right) \\
& = 2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ 
\left( \big\|  \btheta_{B',\alpha} - \btheta_{B,\alpha} \big\|_2^2 \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (1-\gamma_{\bxi})^2   \right]
+   \big\|  \btheta_{B,\alpha} - \btheta_{A,\alpha} \big\|_2^2  \right) \\
& \leq  2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~  \left( \| \btheta_{B,\alpha} -\btheta_{B',\alpha}\|_2^2  + \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right) ~.
\end{align*}
Putting everything back together
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 & p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 ~~\left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
Similarly
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 & p_{\psi}(\bxi;2\btheta_{B',\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 ~~\left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
%Since the bound is the same for both the terms, the $\max$ can be bounded by the right-hand-side.
% \abcomment{please finish the rest, need to check the scaling w.r.t.~$1/\sigma$ once the earlier notation is cleaned up}


Then, plugging into bound on $I_{A,B}$, we have
\begin{align*}
I_{A,B} & \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times 
\exp\left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2\right] \\
& ~~~~~ \times \max\big(  \exp \left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right) \big. ~,\\
& ~~~~~~~~~~~~  \exp \left[ 2 c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \right) \big)~.
%\exp\bigg[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \max\left(  \| \btheta_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 , \| \btheta_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 \right)  \bigg] \\
%& ~~~~~~~~~~ \times c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
Since $\alpha^2 \geq 8 c_2 \Delta^2(S_{n+1})$ where $\Delta(S_{n+1}) = \max_{z,z' \in S_{n+1}} \| \nabla \ell (\w,z) - \nabla \ell (\w,z') \|_2$, recalling that $\btheta_{B,\alpha} = \nabla \ell(\w,B)/\alpha$, we have 
\begin{align*}
2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 & \leq \frac{1}{4}~, ~~~
2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \leq \frac{1}{4} ~, ~~~
2 c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \leq \frac{1}{4} ~.
\end{align*}
As a result, we have 
\begin{align*}
I_{A,B} & \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times \exp\left( \frac{1}{4}\right) \times \exp\left(\frac{1}{4}\right) \times \left( 1 +\frac{1}{4} + \frac{1}{4} \right) \\
& \leq \frac{5c_2}{2 \alpha^2} \| \nabla \ell(\w,S_B) - \nabla \ell(\w,S'_B) \|_2^2~.
\end{align*}
That completes the proof. \qed


\subsection{Expected Stability of EFLD}

\theoefldstab*

\proof 
% \abcomment{add a proof -- just use Theorem~\ref{theo:efld} in Lemma~\ref{theo:stab}} 
% \yzcomment{added a proof here}

Based on Lemma \ref{theo:stab}, we have
\begin{equation}
\hspace*{-5mm}
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq c_1 \frac{b}{n} \E_{S} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \underset{B_t \in G_1}{\E} \underset{A_t \in G_0}{\E} \left[ I_{A_t, B_t} \right] }~.
\end{equation}
with $I_{A_t, B_t} = \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t$. 

From Theorem \ref{theo:efld}, we have 
\begin{align*}
I_{A_{t}, B_{t}} & \leq \frac{5 c_{2}}{2 \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\|\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)-\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}^{\prime}\right)\right\|_{2}^{2}\right] \\
& =\frac{5 c_{2}}{2  \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\| \frac{1}{b}  \sum_{z\in S'_{B_t}}\nabla \ell\left(\mathbf{w}_{t-1}, z \right)- \frac{1}{b}  \sum_{z\in S_{B_t}} \nabla \ell\left(\mathbf{w}_{t-1}, z \right)\right\|_{2}^{2}\right]  \\
& =\frac{5 c_{2}}{2 b \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\| \nabla \ell\left(\mathbf{w}_{t-1}, z_n \right)-\nabla \ell\left(\mathbf{w}_{t-1}, z_n^\prime \right)\right\|_{2}^{2}\right]~,
\end{align*}
where the last equation holds because $S_{B_t}$ and $S'_{B_t}$ only differ at $z_n$ and $z_n^\prime$. 

Combining the above two inequalities, we have
\begin{align*}
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq c_1 \frac{b}{n} \E_{S} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \left[\left\| \nabla \ell\left(\mathbf{w}_{t-1}, z_n \right)-\nabla \ell\left(\mathbf{w}_{t-1}, z_n^\prime \right)\right\|_{2}^{2}\right] }~.
\end{align*}
That completes the proof. 
\qed


==> ICLR2022/app/exp_stability.tex <==
\prophell*
\proof Let $S=\left(z_{1}, \ldots, z_{n}\right)$ and $\tilde S^{\prime}=\left(z_{1}^{\prime}, \ldots, z_{n}^{\prime}\right)$ two independent random samples and let $S^{(i)}=\left(z_{1}, \ldots, z_{i-1}, z_{i}^{\prime}, z_{i+1}, \ldots, z_{n}\right)$ be the sample that is identical to $S$ except in the $i$-th example where we replace $z_{i}$ with $z_{i}^{\prime}$. 
\begin{align*}
& \E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))] \\
&= \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \mathbb{E}_{A} \left[\frac{1}{n} \sum_{i=1}^{n}\left(\ell(A(S^{(i)}), z_{i}^{\prime})-\ell(A(S), z_{i}^{\prime}) \right)\right] \\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime}  \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_{A} \left(\ell(A(S^{(i)}), z_{i}^{\prime})-\ell(A(S), z_{i}^{\prime}) \right)\\
& \overset{(a)}{=} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \left(\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p^{(i)}(\mathbf{w}) d \mathbf{w}-\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p(\mathbf{w}) d \mathbf{w} \right)\\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) \left( p^{(i)}(\mathbf{w}) d \mathbf{w}- p(\mathbf{w}) \right)d \mathbf{w} \\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime)\left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)  d \mathbf{w} \\
& \overset{(b)}{\leq} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \left\{\left(\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime)^{2}\left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\}
\end{align*}
where (a): $p^{(i)}(\w)$ is the distribution obtained by $A(S^{(i)})$, and (b) 
follows by Cauchy-Schwartz inequality. Focusing on the first integral, we have: 
\begin{align*}
\left(\int_{\mathbb{R}^{d}} \ell(\w ; z_i^\prime)^{2}\left(\sqrt{p^{(i)}(\w)}+\sqrt{p(\w)}\right)^{2} d \w \right)^{1/2} 
& \leq \left(2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}p^{(i)}(\w) d\w +  2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2} p(\w) d \w \right)^{1/2} \\
& \leq \left( c_0^2 + c_0^2 \right)^{1/2} =\sqrt{2} c_0~.
\end{align*}

Hence,
\begin{align*}
\E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))]
& \leq   \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n}c_0 \sqrt{2H^{2}\left(A(S), A(S'_n)\right)}\\
& = c_0 \E_{S \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S), A(S'_{n})\big)}~.
\end{align*}
% (b): need to double check if we can apply the previous argument that ``for any $z$, the loss $\ell(\w;z)$ has bounded expectation and variance'' because there are dependence between $\ell(\w; z_i^\prime)$ and $p^{(i)}(\w)$. The worst case, we bound it by uniform upper bound $C$ on the loss. (c) is true because $z_i^\prime$ for $i =1,...,n$ are i.i.d., so that we can write it as $z^{\prime}$.
% $p^{\prime}(\mathbf{w})$ is the distribution obtained by $A(S^\prime)$, where $S^\prime$ is the dataset differing on only single sample $z^{\prime}$ with $S$.  

% \abcomment{(a) For the analysis, lets use $| \cdots |$ throughout, (b) pls clean up the $\mu^2 + \sigma^2$ analysis, and use a constant. This part needs work}

% \abcomment{For the last part, change to:}
% \begin{align*}
% & \overset{(b)}{\leq} 2c_0  \mathbb{E}_S \mathbb{E}_{S^\prime} \left[ \frac{1}{n} \sum_{i=1}^{n}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)} \right] \\
% & = 2c_0 \mathbb{E}_S \mathbb{E}_{S'} \mathbb{E}_{z_i^\prime \sim S'}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)}\\
% & \overset{(c)}{=} 2c_0 \mathbb{E}_S \mathbb{E}_{z^{\prime}} \sqrt{D_{H}^{2}\left(p^{\prime}(\mathbf{w}), p(\w)\right)}~.
% \end{align*}
That completes the proof. \qed 


\prophellkl*
\proof For the first part, note that:
\begin{align*}
KL(P ,P') & = \int \log \frac{p(\w)}{p'(\w)} p(\w) ~d\w \\
& =  2 \int  \left\{ - \log \sqrt{\frac{p'(\w)}{p(\w)}} \right\} p(\w)~ d\w \\
& \overset{(a)}{\geq} 2 \int \left\{ 1 - \sqrt{\frac{p'(\w)}{p(\w)}} \right\} p(\w)~ d\w \\ 
& = 2 \int \left( p(\w) - \sqrt{p(\w) p'(\w)}) \right) ~d\w \\
& = \int \left(p(\w) + p'(\w) - 2 \sqrt{p(\w)p'(\w)} \right) ~d\w \\
& = \int \left(\sqrt{p(\w)} - \sqrt{p'(\w)}\right)^2~ d\w\\
& = 2 H^2(P,P')~,
\end{align*}
where (a) follows since for $x > 0$, $-\log x = - \log(1- (1-x)) \geq 1-x$.

For the second part, note that:
\begin{align*}
2H^2(P,P') & =  \int_\w ( \sqrt{p(\w)} - \sqrt{p'(\w)} )^2 d\w \\
& =  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| | \sqrt{p(\w)} - \sqrt{p'(\w)}| ~d\w \\
& \leq  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| | \sqrt{p(\w)} + \sqrt{p'(\w)}|~ d\w \\
& =  \int_\w | p(\w) - p'(\w)|~ d\w \\
& =  TV(P,P')~,
\end{align*}
where $TV(P,P')$ denotes the total variation distance \cite{pollard2002user}. Further, from Pinsker's inequality \cite{tsybakov2008introduction}, we have
\begin{align*}
TV(P,P') \leq \sqrt{\frac{1}{2} KL(P,P')}~.
\end{align*}
Combining the two results completes the proof. \qed 


% \subsection{Proofs for Section 2.2}

% \mixmodel*
% \proof The proof follows the argument in the proof of Lemma 21 in \cite{Li2020On}.\qed

\subsection{Proofs for Section \ref{sec: exp_stab_nsi}}

Similar results have appeared in \citep{Li2020On, bun2018composable}, we give a simple proof.
\begin{lemm}\label{lemm:mix_bound}
Let $Q,Q',R$ be any three distributions such that $Q,Q'$ are both absolutely continuous w.r.t.~$R$. Then, for $s \in (0,1)$
\begin{equation}
KL\left(sQ+(1-s)R ~\big\| ~sQ' + (1-s)R \right) \leq 
\frac{s^2}{1-s}~\int_{\w} \frac{(Q(\w) - Q'(\w))^2}{R(\w)} d\w~ .
%\frac{s^2}{1-s} \lsd( Q - Q', R)~.
\end{equation}
\end{lemm}

\proof Let $U=sQ' + (1-s)R$. Then, with $F(x) = Q(x)-Q'(x)$, we have
\begin{align*}
     KL(sQ+(1-s)R \| sQ' + (1-s)R) & =  KL(U + s(Q - Q')  \| U ) \\
     & = \int (U(x) + sF(x)) \log \left( \frac{U(x) + s F(x)}{U(x)} \right) dx \\
     & = \int (U(x) + sF(x)) \log \left( 1 + \frac{s F(x)}{U(x)} \right) dx \\
     & = \int sF(x) + \frac{s^2 F^2(x)}{2U(x)} -  \frac{s^3 F^3(x)}{6U^2(x)} + \frac{s^4 F^4(x)}{12U^3(x)}  -\cdots dx \\
     & = s^2 \int \frac{F^2(x)}{U(x)}\left(  \frac{1}{2} -  \frac{s F(x)}{6U(x)} + \frac{s^2 F^2(x)}{12U^2(x)} - \cdots \right) dx~,
%     & = \int U(x) \left( \left(1+ \frac{sF(x)}{U(x)} \right) \log \left(1 + \frac{sF(x)}{U(x)} \right) - \frac{sF(x)}{U(x)} \right) dx
\end{align*}
where the first term vanishes since $\int F(x) dx = \int (Q(x) - Q'(x)) dx = 0$. This is the reason the dependency is on $s^2$, not $s$. With $W(x) = s F(x)/U(x)$, noting that $W(x) > -1$, and 
\begin{equation}
    \left( \frac{1}{2} - \frac{W(x)}{6} + \frac{W^2(x)}{12} - \cdots \right) = \frac{(1+W(x))\log(1+W(x)) - W(x)}{W^2(x)} \leq 1~,
\end{equation}
we have
\begin{align*}
   KL(sP+(1-s)R \| sQ + (1-s)R) 
     & = s^2 \int \frac{F^2(x)}{U(x)} \left( \frac{ (1+W(x)) \log (1+W(x)) - W(x)}{W^2(x)} \right) dx \\
     & \leq s^2 \int \frac{F^2(x)}{U(x)} dx~ \\
     & \leq \frac{s^2}{(1-s)} \int \frac{(Q(x) - Q'(x))^2}{R(x)} dx~.
\end{align*}
That completes the proof. \qed


\begin{restatable}{prop}{mixmodel}
Consider the mixture models 
%\begin{align*}
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  
%\end{align*}
Then, with 
%\begin{equation*}
$s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}$,
%\end{equation*}
we have 
\begin{align*}
    P_{t|} = s Q_{t|} + (1-s) R_{t|}~, \qquad \text{and} \qquad P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~.
\end{align*}
\label{prop:mixmodel}
\vspace*{-6mm}
\end{restatable}
\proof The proof follows the argument in the proof of Lemma 21 in \cite{Li2020On}.\qed



\begin{lemm}
Consider a general NSI algorithm with updates of the form~\eqref{eq:nmia} with mini-batch size $B_t = b$. Then, for any trajectory $\w_{0:t-1}$, we have
\begin{align}
KL\left(P_{t|} \| P_{t|} \right) \leq  \frac{b^2}{n^2} \frac{n}{n-b} \E_{B_t \in G_1} \E_{A_t \in G_0} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t \right]~.
\end{align}
\label{lemm:lsd}
\vspace*{-6mm}
\end{lemm}

\proof By definition and Proposition \ref{prop:mixmodel},
\begin{align*}
KL\left(dP_{t|} \| P'_{t|}\right) & \stackrel{(a)}{\leq} \left(\frac{b}{n} \right)^2 \left(\frac{n}{n-b}\right) \int_{\w} \frac{(Q - Q')^2}{R} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \bigintsss_{\w} \frac{ \left(  \frac{1}{|G_1|} \left[ \sum_{B \in G_1} dP_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right] \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} dP_{A,\bxi}(\w)} d\w \\
 & \stackrel{(b)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}\sum_{B \in G_1}  \frac{ \left(  dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} dP_{A,\bxi}(\w)} d\w \\
 & \stackrel{(c)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}  \sum_{B \in G_1} \left\{ \left(  dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2  \frac{1}{|G_0|}\sum_{A \in G_0} \frac{ 1 }{ dP_{A,\bxi}(\w)} \right\} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \frac{1}{|G_1| |G_0|}  \sum_{B \in G_1} \sum_{A \in G_0}  \bigintsss_{\w} \frac{ \left( dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2 }{ dP_{A,\bxi}(\w)} d\w ~,
\end{align*}
% \yzcomment{In order to make sure (b) holdes, we do need $B = B^\prime$, which should be  defined as mini-batches of indexes. }
where (a) is from Lemma \ref{lemm:mix_bound}, (b)(c) is from Jensen's inequality since function $f(x) = x^2$ is convex and $f(x)=\frac{1}{x}$ is convex on $(0,\infty)$. That completes the proof. \qed



\theostab*

\proof 

Based on Proposition \ref{prop:hell} and \ref{prop:hellkl}, we have

\begin{align*}
\E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))]
& \leq  \sqrt{2 K L\left(P_{T} \| P_{T}^{\prime}\right)} \\
& \leq \sqrt{ 2 \sum_{t=1}^{T} P_{0:(t-1)}\left[K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right)\right]} 
\end{align*}
Bringing the result of Lemma \ref{lemm:lsd} into the above inequality completes the proof. \qed


\subsection{High Probability Generalization Bounds}


%\subsection{High Probability Bounds}

%\yzcomment{strongly suggest moving this section to the appendix}

%\abbcomment{This subsection can be moved to the appendix}

Let $S \sim D^n$ with $S=(Z_1\ldots,Z_n)$ corresponding to the training data. Consider the random variable $Y(S)$, the Scaled (by $n$) Generalization Error (SGE), defined as
\begin{align}
Y(S) \triangleq \sum_{i=1}^n \E_A \big[  \E_{Z \sim D} [\ell(A(S),Z) ] - \ell(A(S),Z_i) \big] = n\big(L_D(A(S)) - L_S(A(S))\big) ~.
\end{align}
%where $A(S)$ is the distribution over $\cW$ due to randomized algorithm $A$ run on $S$.
Theorem~\ref{theo:stab} establishes a bound on $|\frac{1}{n}\E_S[Y(S)]|$. We now focus on establishing a high probability bound on $\frac{1}{n}(Y(S)-\E_S[Y(S)])$. Let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. Further, let $S'_i = (Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, the change in SGE
\begin{equation}
Y(S) - Y(S'_i) = n \big[ \big( L_D(A(S)) - L_D(A(S'_i)) \big) - \big( L_S(A(S)) - L_{S'_i}(A(S'_i) \big) \big]    
\end{equation}
is a symmetric random variable, and is identically distributed for $i=1,\ldots,n$.
% \begin{align}
% Y(S) - Y(S'_i) = \sum_{j=1}^n \E_A \big[ \ell(A(S'_i),Z_j) - \ell(A(S),Z_j) \big] = n \big(L_{S'_i}(A(S'_i) - L_S(A(S)) \big)
% \end{align}
%Note that $(Y-Y'_i)$ \abedit{is symmetric} and are identically distributed for any $i$. 
Our analysis is based on the following assumption: %\abcomment{cite for $\psi_2$ norm} 
\begin{asmp}
The random variable $(Y(S)-Y(S'_i))^2$ is sub-Gaussian with $\psi_2$-norm $\kappa_A^2$, i.e., $\| (Y-Y'_i)^2 \|_{\psi_2} = \sup_{q \geq 1} (\E_{S.S'}|Y(S)-Y(S'_i)|^{2q})^{1/q}/\sqrt{q} = \kappa_A^2$. 
%has bounded second moment, i.e., $\E_{S,Z'_i}[(Y(S)-Y(S'_i))^2] \leq \nu_A$, for some constant $\nu_A$.\abcomment{should this be a definition? i.e., just call the second moment $\nu_A$?}
\label{asmp:2moment}
\end{asmp}
Assumption~\ref{asmp:2moment} implies that $\|Y-Y'_i\|_{\psi_2} \leq \kappa_A$.
Note that since $Y(S) - Y(S'_i)$ is identically distributed for all $i$, $\kappa_A$ is the same for all $i$. Further, $\kappa_A$ is a property of the algorithm $A$, and can be viewed as a measure of stability.
If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered stable; on the other hand, if $\kappa_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as typical generalization error $\frac{1}{n}Y(S)$ itself. The sharpness of the high-probability bound we present meaningfully depends on $\kappa_A$, with smaller values implying sharper bounds.



\begin{restatable}{theo}{theohighp}
Under Assumption~\ref{asmp:2moment}, with probability at least $(1-\delta)$ over the draw $S \sim D^n$, we have
\begin{equation}
L_D(A(S)) \leq L_S(A(S)) + \E_S\bigg[L_D(A(S) - L_S(A(S))\bigg] + \max\left( \frac{1}{n}, \frac{ c_1 \kappa_A}{\sqrt{n}} \right) \log \left(\frac{16}{\delta} \right)~.      
\end{equation}
\label{theo:hp}
\vspace*{-5mm}
\end{restatable}







If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered very stable; if $\kappa_A=O(\sqrt[4]{n})$, then $A$ can be considered somewhat stable; and if $\kappa^2_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as the generalization error $\frac{1}{n}Y(S)$ itself. 

%\theohighp*

%
%
\proof Let $S=(Z_1,\ldots,Z_n)$ and let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% % Let
% % \begin{align}
% % Y & = f(Z_1,\ldots,Z_n) \\
% % Y'_i & = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)~,~i=1,2,\ldots,n~.
% % \end{align}
With $(x)_+ = max(x,0)$, let
\begin{align}
    V^+ = V^+(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_+^2 ]~,
\end{align}
% % Let
% With $(x)_- = min(x,0)$, let
% \begin{align}
%     V^- = V^-(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~,
% \end{align}

Our proof uses the following exponential version of the Efron-Stein inequality [Theorem 6.16 in \cite{boucheron2013concentration}], whose proof is based on a combination of the symmetric modified log-Sobolev inequality [Theorem 6.15 in \cite{boucheron2013concentration}] with the change of measure:
\begin{theo}\label{theo:exp_efst}
Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
\begin{equation}
\log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
\end{equation}
\end{theo}

% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$ such that $(Y-Y'_i)$ is bounded and $\| Y-Y'_i\|_{\psi_2} = \kappa_A$. Then, with $(x)_+ = \max(0,x)$,
% \begin{equation}
% V^+_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
% \end{equation}
% is sub-Gaussian and $\| V_i^+ \|_{\psi_2} \leq 4\kappa_A^2$. \abcomment{should follow by definition, by bounding $L_p$ norms, since $Y-Y'_i$ is bounded.}
% \end{lemm}


For the proof of Theorem~\ref{theo:hp}, note that $V^+$ is sub-Gaussian with $\| V^+ \|_{\psi_2} \leq n \kappa_A^2$.
Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_2}$. Then from Theorem \ref{theo:exp_efst}, we have
\begin{align*}
\psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right].
\end{align*}
Then, by Markov's inequality we have
\begin{align*}
\log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
 & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
\end{align*}
Choosing $\theta = 1/(2\lambda)$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) 
& \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
\end{align*}
Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
\Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
\end{align*}
With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa_A^2$, with $c_1 = c_0 \sqrt{2}$, we have
\begin{align*}
\P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right) ~.
\end{align*}
Now, we choose $\delta$ such that
\begin{align*}
 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right)   
 \leq 8 \exp \left( - n \epsilon \right)  + 8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta~.
\end{align*}
It suffices to choose $\epsilon$ such that
\begin{align*}
8 \exp \left( - n \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{1}{n} \log \left( \frac{16}{\delta} \right) \\
8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{c_1 \kappa_A}{\sqrt{n}} \log \left( \frac{16}{\delta} \right)~.
\end{align*}
As a result,
\begin{align*}
\P\left( \frac{1}{n}(Y - \E Y) >  \max \left( \frac{1}{n}, \frac{c_1 \kappa_A}{\sqrt{n}} \right) \log \left( \frac{16}{\delta} \right) \right) & \leq \delta~.
\end{align*}
That completes the proof. \qed





==> ICLR2022/app/guss.tex <==
\lemmaiabguss*


\proof Recall that we want to bound

\begin{align}
 \nr I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t},~~\text{where} ~~ \bxi_t \sim \cN(0, \sigma_t^2\mathbb{I}_d) ~. 
\end{align}

For Noisy SGD with Gaussian noise, we have $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ to be two Gaussian distributions with variance $\sigma_t^2\mathbb{I}_d$, and with mean $\m_{B_t}$ and $\m^\prime_{B_t}$ respectively to be
\begin{align*}
    \m_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t}) \\
    \m'_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_{B_t}) ~.
\end{align*}

Similarly, $P_{A_t,\bxi_t}$ is also a Gaussian noise with mean 
$\m_{A_t}  = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{A_t})$. 
Thus, for any $B_t$ and $A_t$, since $P_{B_{t}, \boldsymbol{\xi}_{t}}$, $P^\prime_{B_{t}, \boldsymbol{\xi}_{t}}$ and $P_{A_{t}, \boldsymbol{\xi}_{t}}$ are Gaussian distributions, $d P_{B_{t}, \boldsymbol{\xi}_{t}}$, $d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}$ and $d P_{A_{t},\boldsymbol{\xi}_{t}}$ are distribution density functions of Gaussian distribution. Then, it is straightforward to have 
\begin{align}
\nr I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{d}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w-\m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
\end{align}
Note that the above calculation considers integral over $d$-dimensional space which introduced an undesired dimension dependence. However, isotropic Gaussian noise is spherical symmetric, we can translate and rotate the coordinate system so that 
$\m_{A_t}=0$  and $ \m_{B_t}, \m_{B_t}^{\prime}$ are mapped to a 2-dimensional space and the Euclidean distances $\|\w-\m_{B_t} + \m_{A_t}\|$, $\|\w-\m_{B_t}^\prime + \m_{A_t}\|$ do not change.  Now, we omit the subscript $t$ in $A_t$, $B_t$, $\bxi_t$ and $\sigma_t$, since the analysis below holds at any $t$-th iteration. We first translate them by $\m_A$ and write $\Delta \m = \m_B - \m_A$, $\Delta \m' = \m'_B - \m_A$. 
% \begin{align*}
%      p_{\m_B,\sigma} \rightarrow x - \m_B + \m_A = x - \Delta \m 
% \end{align*}
% \begin{align*}
%      p_{\m'_B,\sigma} \rightarrow x - \m'_B + \m_A = x - \Delta \m'
% \end{align*}
% \begin{align*}
%      p_{\m_A,\sigma} \rightarrow x - \m_A + \m_A = x~.
% \end{align*}

Let $\w$ be a $d$-dimensional Gaussian distribution with zero mean. Fix a basis $\mathbf{b}_1,...,\mathbf{b}_p$ and draw $\w$ by first drawing signed lengths $\lambda_{i} \sim \mathcal{N}\left(0, \sigma^{2}\right), \text { for } i \in[d]$, then $\w = \sum_{i=1}^d \lambda_i \mathbf{b}_i$. We can choose the basis such that $\Delta \m$ and $\Delta \m'$ are parallel to $\mathbf{b}_1$ and $\mathbf{b}_2$ such that $\Delta \m = a_1 \mathbf{b}_1 + a_2 \mathbf{b}_2$ and $\Delta \m' = a'_1 \mathbf{b}_1 + a'_2 \mathbf{b}_2$. Note that $a_1^2 + a_1^2 = \|\Delta \m\|_2^2 = \|\m_B - \m_A\|_2^2$ and $a'_1^2 + a'_1^2 = \|\Delta \m'\|_2^2 = \|\m'_B - \m'_A\|_2^2$
\begin{align*}
I_{A,B}  & = \bigintsss_\w \frac{ \left(  d P_{\m_B,\bxi} -    d P_{\m'_B,\bxi} \right)^2 }{  d P_{\m_A,\bxi}} d \w   \\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| \w -  \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| \w -  \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \w -  \m_A\|_2^2/2\sigma^2)} d \w  ~\\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| \w -  \Delta\m \|_2^2 / 2\sigma^2 ) - \exp(- \| \w -  \Delta \m'\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x\|_2^2/2\sigma^2)} d \w ~ \\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\sum_{i=1}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~ \\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(-  (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2+ \sum_{i=3}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~\\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\mathbb{R}^2} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2)} d_{\lambda_1, \lambda_2}~\\
 & \qquad \cdot \bigints_{\mathbb{R}^{d-2}}\frac{1}{(\sqrt{2 \pi} \sigma)^{d-2}} \exp(- \sum_{i=3}^d \lambda_i^2/2\sigma^2) ~ d_{\lambda_3,...,\lambda_d} \\
 & =  \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\x \in \mathbb{R}^2} \frac{ \bigg( \exp(- \|\x -  \Delta \m \|_2^2 / 2\sigma^2 ) - \exp(- \|\x -  \Delta \m'\|_2^2 / 2\sigma^2 )\bigg)^2 }{\exp( - \|\x\|_2^2 / 2\sigma^2)} d_{\x}
\end{align*}
We abuse the notation and write $ \m_B - \m_A = \Delta \m$ and $ \m'_B - \m_A = \Delta \m'$ as a two dimensional vector with the norm preserved. Then 
\begin{align*}
I_{A,B} 
 = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\x \in \mathbb{R}^p} \frac{ \bigg( \exp(- \| \x -  \m_B + \m_A \|_2^2 / 2\sigma^2 ) - \exp(- \| \x -  \m'_B + \m_A\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \x \|_2^2/2\sigma^2)} d \x ~.
\end{align*}



Then
we have $I_{A_t, B_t}$ as 
\begin{align}
I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{2}} \int_{\x} \frac{\left(\exp \left(-\left\|\x-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\x-\m_{B}^{\prime} + \m_{A_t} \right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \x~.
\end{align}
Then we treat $\exp \left(-\left\|\x-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ and $\exp \left(-\left\|\x-\m_{B_t}^\prime + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ as two functions of $\x$ where we can 
use Taylor expansion and apply mean-field theorem. Thus, 
%to bound $I_{A_t, B_t}$ as
for each $\x$, we have:
\begin{align*}
 \exp(- \| \x - \m_B +  {\m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| \x - \m'_B +  {\m_A}\|_2^2 / 2\sigma^2 ) 
 & = \bigg\langle \m_B - \m'_B , \nabla \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
\end{align*}
where $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B  {- \m_A}$, where $\alpha_x \in [0,1]$ depends on $\x$. 
Let $\| \tilde{\m}_B\|_2 \leq \max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2) \triangleq \bar{\m}_B$. 

We have
\begin{align*}
  \nabla \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2) & = -\frac{\x -\tilde{\m}_B}{\sigma^2} \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2)~, 
\end{align*}
so that
\begin{align*}
& \frac{ \bigg( \exp(- \| \x - \m_B  { + \m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| \x - \m'_B  { + \m_A} \|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
= \frac{\bigg\langle \m_B - \m'_B , -\frac{\x -\tilde{\m}_B}{\sigma^2} \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{\| \m_B - \m'_B \|_2^2 \| \frac{\x -\tilde{\m}_B}{\sigma^2} \|_2^2 \exp(- \| \x - \tilde{\m}_B\|_2^2 / \sigma^2) }{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|\x\|^2 + \| \tilde {\m}_B \|_2^2 \bigg)  \exp\left(-\frac{\| \x-\tilde{\m}_B\|_2^2}{\sigma^2} + \frac{\|\x\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
= \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|\x\|^2 + \|  \tilde{\m}_B \|_2^2 \bigg)  \exp\left( \frac{ {3}\|\tilde{\m}_B\|_2^2}{ {2}\sigma^2}\right)  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
\leq \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{ {3}\|\bar{\m}_B\|_2^2}{ {2}\sigma^2}\right) \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) ~.
\end{align*}

Since $\tilde{\m}_B$ interpolate between $\m_B  { - \m_A}$ and $\m'_B  { - \m_A} $ and $\exp$ is positive, based on Proposition \ref{prop:mid_step}, with $\m = 2(\m_B  { - \m_A})$, $\m' = 2(\m'_B  { - \m_A})$ and $\tilde \m = 2 \tilde \m_B$,
we have 
% \abcomment{This step is not correct, should be fixable with a scale factor}
% \begin{align*}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left(-\frac{\|x-2(\m_B   { - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2(\m'_B   { - \m_A})\|_2^2}{2\sigma^2}~, \right) 
% \end{align*}

\begin{align*}
\exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) 
\max\left(\exp\left(-\frac{\|\x -2\m_B + 2\m_A\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|\x -2\m_B' + 2\m_A\|_2^2}{\sigma^2}\right) \right)\\
& \leq \exp \left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \left(\exp\left(-\frac{\|\x -2\m_B + 2\m_A\|_2^2}{\sigma^2}\right) + \exp\left(-\frac{\|\x -2\m_B' + 2\m_A\|_2^2}{\sigma^2}\right) \right)
\end{align*}

% \begin{align*}
% \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) \leq \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right).
% \end{align*}



Continuing
\begin{align*}
& \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) d\x \\
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)  \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|\x-2(\m_B { - \m_A})\|_2^2}{2\sigma^2} \right) d\x \\ 
& \phantom{\leq ......} + \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|\x-2(\m'_B  { - \m_A})\|_2^2}{2\sigma^2} \right) d\x \\
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \bigg( 2\sigma^2 + 4\|\m_B  { - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 + 2\sigma^2 + 4\|\m'_B  { - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) \\
& \leq 4 \big(\sigma^2 + \|\m_B  { - \m_A}\|_2^2 + \|\m'_B   { - \m_A} \|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)
\end{align*}


Putting everything back together, we have 
%\yzcomment{Now it just depends on the gradient difference.}
\begin{align*}
I_{A,B} & \leq \frac{1}{2\pi \sigma^2} \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{ {3}\|\bar{\m}_B\|_2^2}{ {2}\sigma^2}\right) 4 \big(\sigma^2 + \|\m_B  { - \m_A}\|_2^2 + \|\m'_B  { - \m_A}\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)\\
& \leq \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{ \|\bar{\m}_B\|_2^2}{2\sigma^2} \bigg) \exp\left( \frac{3\|\bar{\m}_B\|_2^2}{2\sigma^2}\right)~\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \|\m_B-\m_B'\|_2^2 \\
& = \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2)^2}{2\sigma^2} \bigg) \\
& \qquad \exp\left( \frac{\max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2)\|_2^2}{\sigma^2}\right)~\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)\|\m_B-\m_B'\|_2^2
\end{align*}

Now we are interested in $\|\m_B -\m_A\|_2$,  $\|\m'_B -\m_A\|_2$ and $\|\m_B -\m_B'\|_2$. Recall that we have $B \in G_1$ which contains the $z_n'$ and $A \in G_0$: 
\begin{align*}
    \m_B & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_B) \\
    \m'_B & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_B) ~.
\end{align*}
\begin{align*}
    \m_A & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_A) ~.
\end{align*}

So that 

\begin{align*}
\m_B - \m_A & = \eta_t \nabla \ell(\w_{t-1},S_B)  - \eta_t \nabla \ell(\w_{t-1},S_A) \\
& = \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell(\w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(\w_{t-1},\tilde{z}) \right]~,
\end{align*}
and
\begin{align*}
\m'_B - \m_A & = \eta_t \nabla \ell(\w_{t-1},S'_B)  - \eta_t \nabla \ell(\w_{t-1},S_A) \\
& = \frac{\eta_t}{m} \left[ \sum_{z \in S'_B} \nabla \ell(\w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(\w_{t-1},\tilde{z}) \right]~.
\end{align*}
Also, 
\begin{align*}
\m'_B - \m_B = \frac{\eta_t}{m} \left( \nabla \ell (\w_{t-1}, z_n) - \nabla \ell (\w_{t-1}, z'_n) \right) ~.  
\end{align*}

Let $\Delta_t(\bar{S}) \triangleq \max_{z,\tilde{z} \in \bar{S}} \| \nabla \ell(w_{t-1},z) - \nabla \ell( \w_{t-1},\tilde{z}) \|_2$, where $\bar{S} \sim D^{n+1}$ as before. Now, note that 
%\abcomment{note that the pairing $(z_i,\tilde{z}_i)$ below is arbitrary, the analysis does not depend on the pairing}
\begin{align*}
\| \m_B - \m_A \|_2^2 & = \left\| \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell( \w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell( \w_{t-1},\tilde{z} \right] \right\|_2^2 \\
& \leq \eta_t^2 \left\| \frac{1}{m} \sum_{i=1}^m \big( \nabla \ell( \w_{t-1},z_i) - \nabla \ell( \w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
& \leq \eta_t^2 \frac{1}{m} \sum_{i=1}^m  \left\|  \big( \nabla \ell( \w_{t-1},z_i) - \nabla \ell( \w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
& \leq \eta_t^2 \Delta^2_t(\bar{S})~.
\end{align*}

Also, $\| \m_B' - \m_A \|_2^2 \leq \eta_t^2 \Delta^2_t(\bar{S})$ and  $\| \m_B' - \m_B \|_2^2 \leq \eta_t^2 \Delta^2_t(\bar{S})$. With the setting that $ \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \leq \ln 3/2$, we have

\begin{align}
I_{A_t, B_t} \leq  \frac{\|\m_{B_t} - \m_{B_t}^\prime \|_2^2}{\sigma_t^2}=  18(1+ \frac{5}{2}\ln\frac{3}{2})\ln \frac{3}{2} \frac{\eta_t^2\left\|\nabla \ell\left( \w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}}{\sigma_t^2}~, \label{eq:guss_with_c}
\end{align}
That completes the proof. \qed


\genboundguss*

\proof Based on Lemma \ref{lemm:iab_guss}, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate,  we have
\begin{align}
\nr K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right) & = \underset{B_{t} \in G_{1},A_{t} \in G_{0}}{\mathbb{E}}\left[\int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}\right]   \leq  \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c = 41 \ln \frac{3}{2}$ based on \eqref{eq:guss_with_c}.

Then, based on the chain rule of KL-divergence, we have
\begin{align}
\nr K L\left(P_{0: T} \| P_{0: T}^{\prime}\right) 
& = \sum_{t=1}^{T} \mathbb{E}_{\w_{t-1}} \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

Following Theorem \ref{theo:stab}, we have
\begin{align*}
\left|\mathbb{E}_{S}\left[L_{D}\left(\mathbf{w}_{T}\right)-L_{S}\left(\mathbf{w}_{T}\right)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar{S}} \sqrt{\sum_{t=1}^{T} \underset{\mathbf{w}_{t-1}}{\mathbb{E}}\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z_{n}\right)-\ell\left(\mathbf{w}_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]},  
\end{align*}
where $c = 41 \ln \frac{3}{2}$. 


\begin{prop}
Assume $\m,\m'$ fixed and $\tilde{\m}$ on the line segment of $\m$ and $\m'$, we have
    \begin{align*}
    \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) \leq \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right).
\end{align*} \label{prop:mid_step}
\end{prop}

\proof  From the law of cosine, we have 
\begin{align*}
    \|x -\m\|_2^2 = \|x-\tilde{\m}\|_2^2 + \|\m-\tilde{\m}\|_2^2 -2 \|x-\tilde{\m}\|_2  \|\m-\tilde{\m}\|_2 \cos \angle x\tilde{\m} \m,
\end{align*}
and
\begin{align*}
    \|x -\m'\|_2^2 = \|x-\tilde{\m}\|_2^2 + \|\m'-\tilde{\m}\|_2^2 -2 \|x-\tilde{\m}\|_2  \|\m'-\tilde{\m}\|_2 \cos \angle x\tilde{\m} \m',
\end{align*}
where $\angle x\tilde{\m} \m + \angle x\tilde{\m} \m' = \frac{\pi}{2}$ so we have $\cos\angle x\tilde{\m} \m + \cos\angle x\tilde{\m} \m' = 0$. By canceling out $\cos$ via weighted sum of the above two equations, we have
\begin{align*}
    &\|x -\m\|_2^2 \|\m'-\tilde{\m}\|_2 + \|x -\m'\|_2^2 \|\m-\tilde{\m}\|_2\\
    =& \|x-\tilde{\m}\|_2^2\|\m'-\tilde{\m}\|_2 + \|\m-\tilde{\m}\|_2^2\|\m'-\tilde{\m}\|_2 + \|x-\tilde{\m}\|_2^2\|\m-\tilde{\m}\|_2 + \|\m'-\tilde{\m}\|_2^2\|\m-\tilde{\m}\|_2.
\end{align*}
Equivalently we have 
\begin{align*}
    \|x-\tilde{\m}\|_2^2 = \frac{\|\m-\tilde{\m}\|_2}{\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2} \|x -\m'\|_2^2 + \frac{\|\m'-\tilde{\m}\|_2}{\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2} \|x -\m\|_2^2 - \|\m-\tilde{\m}\|_2\|\m'-\tilde{\m}\|_2.
\end{align*}
Since $\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2 = \|\m-\m'\|_2$, from AM-GM inequality we have
\begin{align*}
    \|x-\tilde{\m}\|_2^2\geq \min \left(\|x -\m\|_2^2,\|x -\m'\|_2^2\right) - \frac{1}{4} \|\m-\m'\|_2^2,
\end{align*}
therefore we have
\begin{align*}
    \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) &\leq \exp\left(-\min \left(\frac{\|x -\m\|_2^2}{\sigma^2},\frac{\|x -\m'\|_2^2}{\sigma^2}\right) + \frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\\
    &= \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right),
\end{align*}
which completes the proof.
\qed



==> ICLR2022/app/signSGD_opt.tex <==
% The ``density'' for a mini-batch $B$ at scale $\alpha$ is:
% \begin{equation}
% p_{\psi}(\bxi; \btheta_{B,\alpha}) = \exp(\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha} \triangleq \frac{\btheta_B}{\alpha} = \frac{\nabla \ell(\w_{t-1}, S_{B})}{\alpha}~.
% \end{equation}
% Note that the corresponding expectation parameter
% \begin{equation}
% \m_{B,\alpha} = \nabla_{\btheta_{B,\alpha}} \psi( \theta_{B,\alpha} )~.
% \end{equation}

% For mini-batch $B_t$ and scaling $\alpha_t$, Noisy Sign-SGD updates the parameters as
% \begin{equation}
%     \w_t = \w_{t-1} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim B\left(\frac{1}{1+\exp \left(-\boldsymbol{\theta}_{B_{t}, \alpha_{t}}\right)}\right)~, ~ \forall i\in [d]~.
% \end{equation}
% % Here we consider the special case of Bernoulli distribution. Thus
% % $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$

% \begin{asmp}\label{asmp: smooth}
% [Smoothness] For all $\w$ and $\w^\prime$, for some non-negative constant $\vec{L}:=\left[L_{1}, \ldots, L_{d}\right]$, we have
% \begin{align}
% \cL_S(\w) \leq \cL_S(\w^\prime) + \nabla \cL_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} L_i (\w_i - \w^\prime_i)^2
% \end{align}
% \end{asmp}

% Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have
% \begin{align*}
%     \cL_S(\w_{t+1}) -\cL_S(\w_{t}) & \leq \nabla \cL_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d L_i (\w_{t,i} - \w^\prime_{t,i})^2\\
%     & = - \eta_t  \nabla \cL_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{L_i}{2}\\
%     & = - \eta_t  \|\nabla \cL_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{L}\|_1 + 2 \eta_t \sum_{i=1}^d |\nabla_i \cL_S(\w_t)| \mathbb{I}\{\bxi_{t, i} \neq \sign(\nabla_i \cL_S(\w_t))\}
% \end{align*}

% Take the conditional expectation, we have
% \begin{align*}
% \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq   - \eta_t  \|\nabla \cL_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{L}\|_1 + 2 \eta_t \sum_{i=1}^d |\nabla_i \cL_S(\w_t)| \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i \cL_S(\w_t))\} 
% \end{align*}

% For now, we have the following approaches:
% \begin{itemize}
%     \item Option I: Show $ \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i \cL_S(\w_t))\} \leq 1/2$ for all $i \in [d]$, then we will have $-\eta_t \cdot c \|\nabla \cL_S(\w_t)\|_1$ for $0<c < 1/2$ on the right hand side. The rest will be standard optimization analysis. 
%     \item Option II: 
%     \begin{align*}
%         \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i \cL_S(\w_t))\} & \leq \mathbb{P}\{ |\bxi_{t, i} - \nabla_i \cL_S(\w_t)| > |\nabla_i \cL_S(\w_t)|\}\\
%         & \leq \frac{\mathbb{E}[|\bxi_{t, i} - \nabla_i \cL_S(\w_t)| ]}{ |\nabla_i \cL_S(\w_t)|}
%     \end{align*}
% \end{itemize}


% \tccomment{
% Case 1: $\nabla_i \cL_S(\w_t)) > 0$, we have
% \begin{align*}
%     \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i \cL_S(\w_t))\} = \mathbb{P}\{\bxi_{t, i} = -1\} = 1-\frac{1}{1+\exp \left(-\nabla_i \cL_S(\w_t)\right)} < 1-\frac{1}{1+\exp \left(0\right)} = \frac{1}{2}.
% \end{align*}
% Case 2: $\nabla_i \cL_S(\w_t)) < 0$, we have
% \begin{align*}
%     \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i \cL_S(\w_t))\} = \mathbb{P}\{\bxi_{t, i} = 1\} = \frac{1}{1+\exp \left(-\nabla_i \cL_S(\w_t)\right)} < \frac{1}{1+\exp \left(0\right)} = \frac{1}{2}.
% \end{align*}
% Therefore, we conclude that $ \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i \cL_S(\w_t))\} < 1/2$ holds. $c$ approaches zero when $\nabla_i \cL_S(\w_t)$ approaches zero.
% \yzcomment{To be more rigours, it should be 
% \begin{align*}
% \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i \cL_S(\w_t))\} \leq  \mathbb{P}\{\bxi_{t, i} = -1|\nabla_i \cL_S(\w_t)) > 0\} +    \mathbb{P}\{\bxi_{t, i} = 1|\nabla_i \cL_S(\w_t)) < 0\} 
% \end{align*}
% I am not sure whether there is dependence between $\bxi_t$ and $ \nabla \cL_S(\w_t))$, i.e.,
% $\mathbb{P}\{\bxi_{t, i} = -1|\nabla_i \cL_S(\w_t)) > 0\} = \mathbb{P}\{\bxi_{t, i} = -1\}$ ?
% }
% \subsection{Choice 2:} 
% Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have
% \begin{align*}
%     \cL_S(\w_{t+1}) -\cL_S(\w_{t}) & \leq \nabla \cL_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d L_i (\w_{t,i} - \w^\prime_{t,i})^2\\
%     & = - \eta_t  \nabla \cL_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{L_i}{2}
% \end{align*}
% Define a function $f:\R^p \rightarrow \R$, where $p$ is the dimension of model parameters: 
% \begin{align*}
%     f(\theta) = \sum_i \theta_i \frac{\exp \theta_i -1}{\exp \theta_i +1} = \sum_i \theta_i \tanh \frac{\theta_i}{2},
% \end{align*}
% we have $f(\theta) \geq 0$, and equality holds if and only if $\theta_i = 0$. Then taking conditional expectation on both side we have 
% \begin{align*}
% \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla \cL_S(\w_t)^T \E\bxi_t  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
% &= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \left(\frac{2}{1+\exp \left(-\nabla \cL_S(\w_t)_i\right)}-1\right)  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
% &= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \left(\frac{\exp \left(-\nabla \cL_S(\w_t)_i\right) -1 }{\exp \left(-\nabla \cL_S(\w_t)_i\right)+1}\right)  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
% &= - \eta_t  f(\nabla \cL_S(\w_t))  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
% \end{align*}
% Taking $\eta_t = \frac{1}{\sqrt{T}}$, by telescope sum we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T f(\nabla \cL_S(\w_t))\right] \leq \frac{1}{\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% \yzcomment{The distribution of $\bxi_t$ depends on $\nabla \ell(\w_t, S_B)$ instead of full batch gradient $\nabla \cL_S(\w_t)$, i.e., $\mathbb{P}\{\bxi_{t, i} = -1\} = 1-\frac{1}{1+\exp \left(-\nabla_i \ell(\w_t, S_B)/\alpha\right)}$, where $\mathbb{E}[\nabla \ell(\w_t, S_B)] = \nabla \cL_S(\w_t)$ . Can we use Jensen's inequality here?}
% Mini-batch settings: 
% \begin{align*}
% \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla \cL_S(\w_t)^T \E\bxi_t  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
% &= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \E\left[\frac{2}{1+\exp \left(-\nabla_i \ell(\w_{t-1}, S_{B}/\alpha)\right)}-1\right]  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
% &= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \E\left[\frac{\exp \left(\nabla_i \ell(\w_{t-1}, S_{B})/\alpha\right) -1 }{\exp \left(\nabla_i \ell(\w_{t-1}, S_{B})/\alpha\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
% & = - \eta_t  \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{L}\|_1.
% \end{align*}
% The first quantity can be decomposed as
% \begin{align*}
% & = - \eta_t  \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] - \eta_t\left( \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right)
% \end{align*}
% The first part is $- \eta_t \alpha  f(\nabla \cL_S(\w_t)/\alpha)$, the second part can be upper bounded by
% \begin{align*}
%   & - \eta_t\left( \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right) \\
%     & \leq  \eta_t\sum_i |\E\theta_{B,i}|\left|\E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right|\\
%     & \leq \eta_t/\alpha \sum_i |\E\theta_{B,i}|\left|\E|\theta_{B,i} -\E[\theta_{B,i}]|\right|\\
%     & = \eta_t/\alpha \sum_i |\E\theta_{B,i}| \|\theta_{B,i} -\E[\theta_{B,i}]\|_{L^1}\\
%     & \leq \frac{\sigma_t\eta_t}{\alpha} \|\E\theta_{B}\|_1\\
%     & \leq \frac{\sigma\eta_t}{\alpha\sqrt{|B_t|}} \|\E\theta_{B}\|_1
% \end{align*}
% where $\tanh$ is 1-Lipschitz function, and we assume first order moment of stochastic gradient is upper bounded by $\sigma_t$ and we can naturally define $\sigma_t\leq \sigma/\sqrt{|B_t|}$. \yzcomment{We can also assume bounded variance/second moment which is common.}
% Gathering everything we have
% \begin{align*}
%   \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}]\leq - \eta_t \alpha  f(\nabla \cL_S(\w_t)/\alpha) + \frac{\sigma\eta_t}{\alpha\sqrt{|B_t|}} \|\nabla \cL_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{L}\|_1.
% \end{align*}
% Bt taking $\eta_t = \frac{1}{\sqrt{T}}$, $|B_t| = T$ \yzcomment{This requires $n > = T$, usually we use $|B_t| = \sqrt{T}$ } by telescope sum we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \left(\alpha f(\nabla \cL_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla \cL_S(\w_t)\|_1\right) \right] \leq \frac{1}{\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% % Note that $T\rightarrow \infty $, equation implies $$\frac{1}{T}\sum_{t=1}^T \left(\alpha f(\nabla \cL_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla \cL_S(\w_t)\|_1\right)  \rightarrow 0,$$ implies $$\alpha f(\nabla \cL_S(\w_T)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla \cL_S(\w_T)\|_1\rightarrow 0, $$ implies $$\alpha f(\nabla \cL_S(\w_T)/\alpha ) \rightarrow 0, $$ implies $$\nabla\cL_S(\w_T) \rightarrow 0.$$
% Since we have
% \begin{equation}
%     x\tanh x/2 > x^2 \frac{1}{2(1+2\log(\frac{\sinh x}{x})},
% \end{equation}
% and
% \begin{equation}
%     \sinh x 
% \end{equation}
% \begin{align*}
%     \alpha f(\nabla \cL_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla \cL_S(\w_t)\|_1 \geq 
% \end{align*}}
% \section{Noisy-SignSGD Optimization analysis}
The ``density'' for a mini-batch $B$ at scale $\alpha$ is:
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\alpha}) = \exp(\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha} \triangleq \frac{\btheta_B}{\alpha} = \frac{\nabla \ell(\w_{t}, S_{B})}{\alpha}~.
\end{equation}
Note that the corresponding expectation parameter
\begin{equation}
\m_{B,\alpha} = \nabla_{\btheta_{B,\alpha}} \psi( \theta_{B,\alpha} )~.
\end{equation}
The full-batch Noisy Sign-SGD update the parameters as
\begin{equation}\label{eq:app_signSGD_full_batch}
    \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim B\left(\frac{1}{1+\exp \left(-2\nabla \cL_S(\w_t)/\alpha_{t}\right)}\right)~, ~ \forall i\in [d]~,
\end{equation}
where $B(x)$ is a pdf with density $x$ at $1$ and density $1-x$ at $-1$.
For mini-batch $B_t$ and scaling $\alpha_t$, mini-batch Noisy Sign-SGD updates the parameters as
\begin{equation}\label{eq:app_signSGD_mini_batch}
    \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim B\left(\frac{1}{1+\exp \left(-2\boldsymbol{\theta}_{B_{t}, \alpha_{t}}\right)}\right)~, ~ \forall i\in [d]~.
\end{equation}
% Here we consider the special case of Bernoulli distribution. Thus
% $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$
We make the following smoothness assumptions of the empirical loss function $\cL_S(\w)$:
\asmpsmooth*
% \begin{asmp}\label{asmp: smooth}
% The loss function $\cL_S$ satisfies: for all $\w$ and $\w^\prime$, for some non-negative constant $\vec{L}:=\left[L_{1}, \ldots, L_{d}\right]$, we have
% \begin{align}
% \cL_S(\w) \leq \cL_S(\w^\prime) + \nabla \cL_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} L_i (\w_i - \w^\prime_i)^2
% \end{align}
% \end{asmp}
The assumption on on the empirical loss $\cL_S(\w)$ is common in optimization analysis, besides that, we also assume some natural statistical properties of the batch gradient of the loss $\nabla \ell(\w_{t}, S_{B_t})$, where the randomness comes from batches conditioned on $\w_t$, satisfies the following assumptions:
\asmpbatch*
% \begin{asmp}\label{asmp:batch}
% [Batch Gradient] Given $\w_t$, the batched gradient $\nabla \ell(\w_t, S_{B_t})$ satisfies the following property:
% \begin{itemize}
%     \item (Unbiased) The batched gradient $\nabla \ell(\w_{t}, S_{{B_t}})$ is an unbiased estimator of true gradient $\cL_S(\w_{t})$: $$\E_{B_t|\w_t}\nabla \ell(\w_{t}, S_{B_t}) = \nabla \cL_S(\w_{t}).$$
%     \item (Symmetricity) The pdf $p_{BG}(x)$ of batched gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is symmetric around its expectation $\cL_S(\w_{t})$:$$p_{BG}(x) = p_{BG}(2\nabla\cL_S(\w_{t})-x).$$
%     \item (Sub-Gaussian) The batched gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is Sub-Gaussian with $\psi_2$ norm $\kappa_t$, where $\kappa_t \leq \kappa_t/\sqrt{|B_t|}$: for any $\lambda >0$, $v\in S^{d-1}$, we have $$\E_{B_t|\w_t}\exp \lambda\langle v,\nabla \ell(\w_{t}, S_{B_{t}})-\nabla \cL_S(\w_{t})\rangle \leq \exp(\lambda^2\kappa_t^2/2)\leq \exp\left(\frac{\lambda^2\kappa_t^2}{2|B_t|}\right).$$
% \end{itemize}
% \end{asmp}
With Assumption \ref{asmp: smooth} and Assumption \ref{asmp:batch}, we have the following guarantee for convergence of noisy signSGD under full batch and mini batch settings. The following is a restate theorem from the main paper for the mini-batch noisy sign-SGD
\theosignSGDconv*
% \begin{theo}\label{theo:signSGD_conv}
% Assume Assumption~\ref{asmp: smooth} holds for loss function $\cL_S$. For Full-batch Noisy Sign-SGD algorithm equation~\eqref{eq:signSGD_full_batch} with stepsize $\eta_t = 1/\sqrt{T}$ and choose $\alpha_t$ satisfies $c\geq \alpha_t \geq \|\nabla \cL_S(\w_t)\|_{\infty}/2$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \cL_S(\w_t)\|_2^2\right] \leq \frac{10c}{3\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right),
% \end{equation}
% Further assume Assumption~\ref{asmp:batch} holds for batch gradient $\nabla\ell(\w_t,S_{B_t})$, for mini-batch noisy Sign-SGD algorithm equation~\eqref{eq:signSGD_mini_batch} with stepsize $\eta_t = 1/\sqrt{T}$, $|B_t|=T$, and 
% % $\alpha_t = 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \cL_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa_t^2}{8T G^2}))}{\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% % \end{equation}
% % or choose $c\geq\alpha_t\geq 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \cL_S(\w_t)\|_2^2  \right] \leq  \frac{2c (1+\exp(\frac{\kappa_t^2}{8T G^2}))}{\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% % \end{equation}
% % or without assuming $G$, 
% choose $\alpha_t$ by $c \geq \alpha_t \geq \max[\frac{\kappa_t}{\sqrt{2T}}, 2\|\nabla \cL_S(\w_t)\|_{\infty}]$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \cL_S(\w_t)\|_2^2  \right] \leq  \frac{8c}{\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% \end{theo}
Here we state and prove the result for both full-batch and mini-batch settings:
\begin{theo}\label{theo:signSGD}
If the loss satisfies Assumption~\ref{asmp: smooth}, for full-batch noisy Sign-SGD with step size $\rho_t = 1/\sqrt{T}$ and $\alpha_t$ satisfying $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}$, we have
\begin{equation}\label{eq:sign_SGD_full_batch_convergence_1}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{5c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
\end{equation}
Further, if Assumption~\ref{asmp:batch} holds, for mini-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$, and 
% $\alpha_t = 2G$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% or choose $c\geq\alpha_t\geq 2G$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{2c (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% or without assuming $G$, 
$\alpha_t$ satisfying $c \geq \alpha_t \geq \max[\sqrt{2}\kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, we have
\begin{equation}\label{eq:sign_SGD_mini_batch_convergence_1}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
\end{equation}
where equation \eqref{eq:sign_SGD_full_batch_convergence_1}\eqref{eq:sign_SGD_mini_batch_convergence_1} holds for any $S$, any initialization $\w_0$, and the expectation is taken over the randomness of  algorithm.
\end{theo}










\textit{Proof for full-batch:} 
Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have
\begin{align*}
    \cL_S(\w_{t+1}) -\cL_S(\w_{t}) & \leq \nabla \cL_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d L_i (\w_{t+1,i} - \w_{t,i})^2\\
    & = - \eta_t  \nabla \cL_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{L_i}{2}
\end{align*}
% Define a function $f:\R^d \rightarrow \R$, where $d$ is the dimension of model parameters: 
% \begin{align*}
%     f(\theta) = \sum_i \theta_i \frac{\exp \theta_i -1}{\exp \theta_i +1} = \sum_i \theta_i \tanh \frac{\theta_i}{2},
% \end{align*}
% we have $f(\theta) \geq 0$, and equality holds if and only if $\theta_i = 0$. 
Then taking conditional expectation on both side we have 
\begin{align*}
\mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla \cL_S(\w_t)^T \E_{\bxi_t|\w_t}\bxi_t  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
&= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \left(\frac{2}{1+\exp \left(-2\nabla \cL_S(\w_t)_i/\alpha_t\right)}-1\right)  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
&= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \left(\frac{\exp \left(2\nabla \cL_S(\w_t)_i/\alpha_t\right) -1 }{\exp \left(2\nabla \cL_S(\w_t)_i/\alpha_t\right)+1}\right)  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
&= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \tanh (\nabla \cL_S(\w_t)_i/\alpha_t)  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
&= - \eta_t  \sum_i |\nabla \cL_S(\w_t)_i| |\tanh (\nabla \cL_S(\w_t)_i/\alpha_t)|  + \frac{\eta_t^2}{2} \|\vec{L}\|_1
\end{align*}
By taking $c\geq \alpha_t \geq \|\nabla \cL_S(\w_t)\|_{\infty}$, and $\eta_t=1/\sqrt{T}$, we have $\nabla \cL_S(\w_t)_i/\alpha_t\leq 1$ so we can apply Lemma \ref{lemm:tanh_bound} to have
\begin{align*}
\mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] &\leq  - \frac{e^2-1}{(e^2+1)\alpha_t\sqrt{T}}  \|\nabla \cL_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{L}\|_1\\
&\leq - \frac{3}{5c\sqrt{T}}  \|\nabla \cL_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{L}\|_1
\end{align*}



by telescope sum we have
\begin{equation}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \cL_S(\w_t)\|_2^2\right] \leq \frac{5c}{3\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right),
\end{equation}
which completes the proof of full-batch updates.

\begin{lemm}\label{lemm:tanh_bound}
For any $-1\leq x\leq 1$, the following holds:
\begin{equation}
    |\tanh x|\geq \frac{e^2-1}{e^2+1}|x|
\end{equation}
\end{lemm}
\proof Without loss of generality, we focus on $0<x\leq 1$. we prove $\tanh x/ x$ is decreasing function on $\R^+$, which is equivalent to
\begin{align*}
    (\frac{\tanh x}{x})' =  \frac{x(1-\tanh^2 x) - \tanh x }{x^2}\leq 0,
\end{align*}
and is equivalent to 
\begin{align*}
    x\leq \frac{\tanh x}{1 -\tanh^2 x},
\end{align*}
where the right hand side is $\sinh x$ and use the fact that $x\leq \sinh x$ for $x > 0$ implies $\tanh x/x$ is decreasing function, so 
\begin{align*}
    \tanh x/x\geq \tanh 1 = \frac{e^2-1}{e^2 +1},
\end{align*} which completes the proof. \qed








\textit{Proof for mini-batch:}
From smoothness condition Assumption \ref{asmp: smooth}, we have
\begin{align*}
\mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] &\leq \E_{\w_{t+1}|\w_t}\nabla \cL_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \E_{\w_{t+1}|\w_t} \sum_{i=1}^d L_i (\w_{t+1,i} - \w_{t,i})^2\\
&= \E_{\bxi_t|\w_t} \nabla \cL_S(\w_t)^T(-\eta_t \bxi_t) + \frac{1}{2} \E_{\bxi_t|\w_t} \sum_{i=1}^d L_i (-\eta_t \bxi_t)^2\\
    &=- \eta_t  \nabla \cL_S(\w_t)^T \E_{\bxi_t|\w_t}\bxi_t  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
&= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \E_{B_t|\w_t}\left[\frac{2}{1+\exp \left(-2\nabla_i \ell(\w_t, S_{B_{t}}/\alpha_t)\right)}-1\right]  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
&= - \eta_t  \sum_i \nabla \cL_S(\w_t)_i \E_{B_t|\w_t}\left[\frac{\exp \left(2\nabla_i \ell(\w_t, S_{B_{t}})/\alpha_t\right) -1 }{\exp \left(2\nabla_i \ell(\w_t, S_{B_{t}})/\alpha_t\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{L}\|_1\\
& = - \eta_t  \sum_i \E_{B_t|\w_t} \theta_{B_{t},i} \E\left[\frac{\exp \left(2\theta_{B_{t},i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_{t},i}/\alpha_t\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{L}\|_1.
\end{align*}

Focus on each individual term in the sum, we have
\begin{align*}
    &\E_{B_t|\w_t}\theta_{B,i} \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_t,i}/\alpha_t\right)+1}\right]\\ =& \E_{B_t|\w_t}\theta_{B_t,i} \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t - 2\E_{B_t|\w_t}\theta_{B_t,i}/\alpha_t\right) -\exp - 2\E_{B_t|\w_t}\theta_{B_t,i}/\alpha_t }{\exp \left(2\theta_{B_t,i}/\alpha_t - 2\E_{B_t|\w_t}\theta_{B_t,i}/\alpha_t\right)+\exp - 2\E_{B_t|\w_t}\theta_{B_t,i}/\alpha_t}\right]
\end{align*}


For ease of notation, denote $2\theta_{B,i}/\alpha_t - 2\E_{B_t|\w_t}\theta_{B,i}/\alpha_t = \theta,~\E_{B_t|\w_t}2\theta_{B,i}/\alpha_t =\mu$, and the pdf of $\theta$ is $p_{\theta}$ for the moment, then from Assumption \ref{asmp:batch}, we have $\theta$ is mean zero, symmetric around zero, and subgaussian with $\psi_2$ norm $2\kappa_t/\alpha_t$ by taking $\lambda=1,~v = \1_i$ in Sub-Gaussian assumption: $\E_\theta\exp\theta \leq \exp(2\kappa_t^2/\alpha_t^2)$.

Therefore, by changing notation we have 
\begin{align*}
     \E_{B_t|\w_t}\theta_{B,i} \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_t,i}/\alpha_t\right)+1}\right] = \frac{\alpha_t \mu}{2} \E_\theta\left[\frac{\exp \theta -\exp(-\mu) }{\exp \theta +\exp(-\mu)}\right].
\end{align*}
By symmetricity of $\theta$, we have
\begin{align*}
    \frac{\alpha_t \mu}{2} \mu\E&_\theta\left[\frac{\exp \theta -\exp(-\mu) }{\exp \theta +\exp(-\mu)}\right]\\
    &= \frac{\alpha_t \mu}{2}\int_{-\infty}^{\infty}p_\theta(x)\left[\frac{\exp x-\exp(-\mu) }{\exp x +\exp(-\mu)}\right]dx\\
    &=\frac{\alpha_t \mu}{2}\int_{0}^{\infty}p_\theta(x)\left[\frac{\exp x -\exp(-\mu) }{\exp x +\exp(-\mu)}+\frac{\exp (-x) -\exp(-\mu) }{\exp (-x) +\exp(-\mu)}\right]dx\\
    &=\frac{\alpha_t \mu}{2}\int_{0}^{\infty}p_\theta(x)\frac{(\exp x -\exp(-\mu))(\exp (-x) +\exp(-\mu)) + (\exp (-x) -\exp(-\mu))(\exp x +\exp(-\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\alpha_t/2 \int_{0}^{\infty}p_\theta(x)\frac{2\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx
\end{align*}
By symmetricity, we have $p_\theta(x) = p_\theta(-x)$, and therefore
\begin{align*}
    &\alpha_t/2\int_{0}^{\infty}p_\theta(x)\frac{2\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\alpha_t/2\int_{-\infty}^{\infty}p_\theta(x)\frac{\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \E_\theta\frac{1}{(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}
\end{align*}
Since $\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu)))\geq 0$, and $\frac{1}{x}$ is convex on $\R^+$, we have
\begin{align*}
   & \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \E_\theta\frac{1}{(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}\\ \geq &\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{\E_\theta(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}.
\end{align*}
% Since $\exp \theta +\exp(-\mu)$ and $\exp (-\theta) +\exp(-\mu)$ are inversely monotone function, by chebyshev sum's inequality, we have
% \begin{align*}
%     \E(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))\leq \E(\exp \theta +\exp(-\mu)) 
% \end{align*}
Using Sub-Gaussian property of $\theta$: $\E_\theta\exp\theta \leq \exp(2\kappa_t^2/\alpha_t^2)$, and symmetricity so $\E_\theta\exp -\theta \leq \exp(2\kappa_t^2/\alpha_t^2)$, we have
\begin{align*}
    &\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{\E_\theta(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}\\
    &= \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+\exp(-\mu)(\E\exp \theta +\E\exp (-\theta))}\\
    &\geq  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+2\exp(-\mu)\exp(2\kappa_t^2/\alpha_t^2)}\\
    &\geq  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}.
\end{align*}
Switching back to our previous notation:
\begin{align*}
    \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}
  & = \E_{B_t|\w_t} \theta_{B,i} (1-\exp(-4\E_{B_t|\w_t}\theta_{B,i}/\alpha_t)) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}\\
  & = \nabla \cL_S(\w_t)_i (1-\exp(-4\nabla \cL_S(\w_t)_i/\alpha_t)) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)},
\end{align*}

% By telescope sum, we have
% \begin{equation}
%     \nabla \cL_S(\w_t)_i (1-\exp(-2\nabla \cL_S(\w_t)_i/\alpha_t))
% \end{equation}

which implies we have
\begin{align*}
    \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{2+2\exp(2\kappa_t^2/\alpha_t^2)}  \sum_i \nabla \cL_S(\w_t)_i (1-\exp(-4\nabla \cL_S(\w_t)_i/\alpha_t))  + \frac{\eta_t^2}{2} \|\vec{L}\|_1.
\end{align*}
Using Lemma \ref{lemm:mix_norm}, we have
\begin{equation}
    \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{2(1+\exp(2\kappa_t^2/\alpha_t^2))}  \sum_i |\nabla \cL_S(\w_t)_i| \min \bigg[ |2\nabla \cL_S(\w_t)_i/\alpha_t| ,0.5\bigg]  + \frac{\eta_t^2}{2} \|\vec{L}\|_1.
 \end{equation}
% We assume $\kappa_t = \frac{\kappa_t}{\sqrt{|B_t|}}$, and we take batch size $|B_t|$.
 

 
%  We choose $2\min_i |\nabla \cL_S(\w_t)_i|\geq \alpha_t\geq \frac{\kappa_t^2}{2\log c} = \frac{\kappa_t^2}{2|B_t|\log c}$, $\eta_t =\frac{2(1+c)}{\sqrt{T}}$ then we have 
%  \begin{equation}
%     \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq - \frac{1}{2\sqrt{T}}  \|\nabla \cL_S(\w_t)\|_1  + \frac{2(1+c)^2}{T} \|\vec{L}\|_1.
%  \end{equation}
 
 
% By telescope sum, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \cL_S(\w_t)\|_1  \right] \leq  \frac{1}{2\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + 2(1+c)^2\|\vec{L}\|_1\right).
% \end{equation}
% which completes the proof.


We choose $\alpha_t$ such that $\alpha_t \geq 4\|\nabla \cL_S(\w_t)\|_{\infty}$, then we have
\begin{equation}
\mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{\alpha_t (1+\exp(2\kappa_t^2/\alpha_t^2))}  \|\nabla \cL_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{L}\|_1.
\end{equation}
% Since $\exp(x) \leq  1 + x + x^2$ for $x < 1.79$, if we choose $\kappa_t,\alpha_t$ s.t. $\kappa_t/\alpha_t< \sqrt{3.58}$, we have
% \begin{equation}
%     \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{2\alpha_t (2+\kappa_t^2/2\alpha_t^2+ \kappa_t^4/4\alpha_t^4)}  \|\nabla \cL_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{L}\|_1.
% \end{equation}
We choose $\alpha_t$ such that $\alpha_t \geq \max[\sqrt{2} \kappa_t, 4\|\nabla \cL_S(\w_t)\|_{\infty}]$, then we have
\begin{equation}
    \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{c (1+e)}  \|\nabla \cL_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{L}\|_1.
\end{equation}
Therefore, if we choose $\eta_t = 1/\sqrt{T}$, we have
\begin{equation}
    \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq - \frac{1}{c (1+e)\sqrt{T}}  \|\nabla \cL_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{L}\|_1.
\end{equation}
By telescope sum, we have
\begin{equation}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \cL_S(\w_t)\|_2^2  \right] \leq  \frac{(1+e)c}{\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
\end{equation}
and note that $1+e<4 $ which completes the proof.


% Choice 2: We choose $\alpha_t = 2G$, $\eta_t = 1/\sqrt{T}$, $|B_t|=\sqrt{T}$, then we have
% \begin{equation}
%     \mathbb{E}[ \cL_S(\w_{t+1}) -\cL_S(\w_{t})|\w_{t}] \leq - \frac{1}{4G (1+\exp(\frac{\kappa_t^2}{8T G^2}))\sqrt{T}}  \|\nabla \cL_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{L}\|_1.
% \end{equation}
% By telescope sum, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \cL_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa_t^2}{8T G^2}))}{\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% which completes the proof.

\qed

% Using Lemma \ref{lemm:mix_norm}, we have
% \begin{align*}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \sum_i^d \min (\nabla_i \cL_S(\w_t)^2/\alpha_t^2,|\nabla_i \cL_S(\w_t)|/2\alpha_t  )  \right] \leq \frac{2+2\exp(\kappa_t^2/2\alpha_t^2)}{\alpha_t} \frac{1}{\sqrt{T}}\left(\cL_S(\w_{0}) - \cL_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right)
% \end{align*}
% Since $\exp(\theta) \geq 1+ \theta + \frac{1}{2} \theta^2$ for $\theta \geq 0$ and reverse for $\theta <0$, so $\theta\exp(\theta) \geq \theta+ \theta^2 + \frac{1}{2} \theta^3$ then
% \begin{align*}
%     \theta_i(1-\exp(-2\theta_i)) \geq \theta_i - \theta_i -2 \theta_i^2 - 2\theta_i^3
% \end{align*}



\begin{lemm}\label{lemm:mix_norm} For any $x$,
$$|1-\exp(-2x))|\geq \min (|x|,\frac{1}{2}).$$
\end{lemm}
\proof 
Since $\exp(-x)\geq 1-x$, so we have for $x<0$:
$$1-\exp (-2x)\leq 2x\leq x.$$

For $x>0$, since $\exp x \geq 1+x$, we have $\exp -x\leq \frac{1}{1+x}$, so
$$1-\exp (-2x)\geq \frac{2x}{1+2x}.$$
Then when $\frac{1}{2}>x>0$, $$\frac{2x}{1+2x} > x,$$
and when $x\geq \frac{1}{2}$, $$\frac{2x}{1+2x} \geq \frac{1}{2},$$
which completes the proof.\qed


\theoSGLDopt*

\proof Recall the update of SGLD:
\begin{equation}
\mathbf{w}_{t+1}=\mathbf{w}_{t}-\eta_{t} \nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)+\frac{\sigma_{t}}{\sqrt{2}} \mathcal{N}\left(0, \mathbb{I}_{d}\right)~.
\end{equation}
\begin{align*}
\mathbb{E} [\cL_S(\w_{t+1})] &\leq \cL_S(\w_t) + \mathbb{E} [\left\langle \nabla \cL_S(\w_t), \w_{t+1} - \w_t \right\rangle ]  + \frac{L}{2} \mathbb{E} [ \|  \w_{t+1} - \w_t\|^2] \\
& =  \cL_S(\w_t) -\eta_t \|\nabla \cL_S(\w_t)\|^2 + \frac{L \eta_t^2}{2}\left(\kappa^2 + p\sigma_t^2/\eta_t^2\right)~,
\end{align*}
where $\kappa^2$ is the upper bound of the variance of $\nabla \ell(\w_{t}, S_{B_t})$.

Rearrange the above inequality, with $\alpha_t = \sqrt{\sigma_t/\eta_t}$ we have
\begin{align} \label{eq:one_step_descend}
    \eta_t\mathbb{E}\| \nabla \cL_S(\w_t)\|^2 \leq  \cL_S(\w_t) - \mathbb{E} [\cL_S(\w_{t+1})]  + \frac{L \eta_k^2}{2}\left(\kappa^2 + p\alpha_t^4\right)~.
\end{align}

Sum over $t =1$ to $t =T$ and apply expectation to each step, we have
\begin{align*}
\sum_{t =1}^T \eta_t\mathbb{E}\| \nabla \cL_S(\w_t)\|^2 
\leq \cL_S(\w_t) - \cL_S(\w_n^\star) +  \sum_{t=1}^T \frac{L \eta_k^2}{2} (p \alpha_t^4 + \kappa^2)~.
%+\frac{(p \sigma^2 + G^2) \sum_{k=1}^T \eta_k^2}{\sum_{k=1}^T \eta_k}.  
\end{align*}

Take $\eta_t= \frac{1}{\sqrt{T}}$ for all $k \in [T]$, we have

\begin{align*}
\frac{1}{T} \sum_{t =1}^T \mathbb{E} \| \nabla \cL_S(\w_t)\|^2 
%\min_{k\in [T]} \mathbb{E} \| \nabla \cL_S(\w_t)\|^2
\leq O\left(\frac{1}{\sqrt{T}}\right) +O\left(L \frac{  p \sum_{t=1}^T\alpha_t^4 +  \kappa^2 \log T }{\sqrt{T}}\right).  
\end{align*}



\qed 

==> ICLR2022/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR2022/sec/conc.tex <==
\vspace*{-2mm}
Inspired by recent advances in stability based and information theoretic approaches to generalization bounds \citep{mou2018generalization,pensia2018generalization,negrea2019information,Li2020On,haghifam2020sharpened}, we have presented a framework for developing such bounds based on expected stability for noisy stochastic iterative (NSI) learning algorithms. We have also introduced Exponential Family Langevin Dynamics (EFLD), a family of noisy gradient descent algorithms based on exponential family noise, including SGLD and Noisy Sign-SGD as two special cases.  We have developed an expected stability based generalization bound applicable to any EFLD algorithm with a $O({1}/{n})$ sample dependence and a dependence on gradient incoherence, rather than gradient norms. Further, we have provided optimization guarantees for EFLD and establish such results for Noisy Sign-SGD and SGLD. Our experiments on various benchmarks illustrate that our bounds are non-vacuous and quantitatively much sharper than existing bounds~\citep{Li2020On,negrea2019information}. 


%Further, we have simplified the task to one of bounding expected for the NSI algorithm. We have developed a specific bound for SGD with Gaussian noise which inherits strengths of a variety of existing results and quantitatively outperforms them based on preliminary experiments. We have also developed similar bounds for SGD with exponential family noise, which seem to be the first result of this type. Our work also highlights few key directions for future work, including sharper notions of gradient discrepancy/incoherence and better understanding of the trade-offs between stability and optimization for NSI algorithms.

==> ICLR2022/sec/efld.tex <==
\vspace*{-2mm} 

In recent years, considerable advances have been made in establishing generalization bounds for stochastic gradient Langevin dynamics (SGLD) \citep{Li2020On, pensia2018generalization, negrea2019information, haghifam2020sharpened}. As an example of NSI algorithms of the form~\eqref{eq:nmia}, SGLD adds an isotropic Gaussian noise at every step of SGD:
%\begin{align}\label{eq:sgld}
 $\w_{t+1} = \w_{t} - \eta_t \nabla \ell(\w_t, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right)$,
%\end{align}
where $ \nabla \ell(\w_t, S_{B_t})$ is the stochastic gradient on mini-batch $B_t$, $\eta_t$ is the step size, and $\sigma_t^2$ is noise vairance. 


In this paper, we introduce a substantial generalization of SGLD called Exponential Family Langevin Dynamics (EFLD) which uses general exponential family noise in noisy iterative updates of the form~\eqref{eq:nmia}. 
In addition to being a mathematical generalization of the popular SGLD, the proposed EFLD provides flexibility to use noise gradient algorithms with different representation of the gradient, e.g., Bernoulli noise for Sign-SGD, discrete distribution for quantized or finite precision SGD, etc. \citep{canonne2020discrete, quantized-sgd, jiang2018, yang2019swalp}.
%\abbcomment{pls add more cites}\yzcomment{done}\abcomment{great, pls drop one to prevent spill over to new line}.
\vspace*{-2mm} 
\subsection{Exponential Family Langevin Dynamics (EFLD)}
\vspace*{-2mm} 
Exponential families \citep{barndorff2014information,brown1986fundamentals,wainwright2008graphical} constitute a large family of parametric distributions which include Gaussian, Bernoulli, gamma, Poisson, Dirichlet, etc., as special cases. Exponential families are typically represented in terms of natural parameters $\btheta$, and we consider component-wise independent distributions with scaled natural parameter $\btheta_{\alpha} = \btheta/\alpha$ with scaling $\alpha > 0$, i.e., $p_{\psi}(\bxi, \btheta_{\alpha}) = \exp(\langle \bxi, \btheta_{\alpha} \rangle - \psi(\btheta_{\alpha})) \ppi_0(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_{j\alpha} - \psi_j(\theta_{j\alpha})) \pi_0(\xi_j)~$,
% \vspace{-2mm}
% \begin{align*}
% \vspace{-3mm}
% p_{\psi}(\bxi, \btheta_{\alpha}) = \exp(\langle \bxi, \btheta_{\alpha} \rangle - \psi(\btheta_{\alpha})) \ppi_0(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_{j\alpha} - \psi_j(\theta_{j\alpha})) \pi_0(\xi_j)~,
% \vspace*{-2mm}
% \end{align*}
where $\bxi$ is the sufficient statistic, $\psi(\btheta_{\alpha})= \sum_{j=1}^p \psi_j(\theta_{j\alpha})$ is the log-partition function, and $\ppi_0(\xi) = \prod_{j=1}^p \pi_0(\xi_j)$ is the base measure. Note that $\alpha=1$ gives the canonical form of the exponential family distributions. For general scaling $\alpha > 0$, for some cases the base measure $\pi_0$  may depend on the scaling, i.e., $\pi_{0,\alpha}$. A scaling $\alpha >0$ is valid as long as $\exp(\langle \bxi,\btheta_{\alpha} \rangle$ is integrable, i.e., $\int_{\bxi} \exp(\langle \bxi,\btheta_{\alpha} \rangle \pi_0(\bxi) d\bxi < \infty$. Further, $\psi$ is a smooth function by construction \citep{barndorff2014information,banerjee2005clustering,wainwright2008graphical} and the smoothness of $\psi$ implies $\nabla^2 \psi(\btheta_{\alpha}) \leq c_2 \I$. %\abcomment{briefly explain why $\psi$ is smooth, in the appendix} 


Exponential family Langevin dynamics (EFLD) uses noisy stochastic gradient updates similar to SGLD, but using exponential family noise rather than Gaussian noise as in SGLD. In particular, for mini-batch $S_{B_t}$, EFLD updates are as follows: with step size $\rho_t > 0$
\begin{equation}
    \w_t = \w_{t-1} - \rho_t \bxi_t~, \qquad \bxi_t \sim p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})~,
\vspace{-2mm}    
\label{eq:efld1}
\end{equation}
where 
\vspace*{-2mm}
\begin{equation}
p_{\psi}(\bxi; \btheta_{B_t,\alpha_t}) = \exp(\langle \bxi, \btheta_{B_t,\alpha_t} \rangle - \psi(\btheta_{B_t,\alpha_t})) \ppi_0(\bxi)   ~, \qquad \btheta_{B_t,\alpha_t} \triangleq \frac{\btheta_{B_t}}{\alpha_t} = \frac{\nabla \ell(\w_{t-1}, S_{B_t})}{\alpha_t}~.
\label{eq:efld2}
\vspace*{-1mm}
\end{equation}
For EFLD, the natural parameter $\btheta_{B_t,\alpha_t}$ at step $t$ is simply a scaled version of the mini-batch gradient $\nabla \ell(\w_{t-1}, S_{B_t})$. We first show that EFLD becomes SGLD when the exponential family is Gaussian, and becomes a noisy version of sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise} when the exponential family is Bernoulli over $\{-1,+1\}$. More details and examples are in Appendix \ref{app:example}.
% \abdelete{\yzedit{Similarly, for EFLD with neighboring dataset $S'_n$, we write  $\btheta_{B'_t,\alpha_t} \triangleq \frac{\btheta_{B_t}}{\alpha_t} = \frac{\nabla \ell(\w_{t-1}, S'_{B_t})}{\alpha_t}$ as the natural parameter for distribution $p_{\psi}(\bxi; \btheta_{B'_t,\alpha_t})$, where $S'_{B_t}$ is the mini-batch sampled from $S'_n$. }
% As examples we first show that EFLD becomes SGLD when the exponential family is Gaussian, and then show that we get a noisy version of sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise} when the exponential family is Bernoulli over $\{-1,+1\}$. For the details of properties of examples, we refer to Appendix \ref{app:example}.}
\begin{exam}[SGLD] 
% \abbcomment{Example is incorrect -- in terms of choice of $\rho_t, \alpha_t$}
% \abcomment{just keep the part showing this is a special case of EFLD}\tccomment{Updated.}\abcomment{updated}
% For multi-variate Gaussians with fixed covariance $\sigma^2\I$, the scaling $\alpha = \sigma$, the sufficient statistic $\bxi = \x/\sigma$, the log-partition function  $\psi(\btheta) = \|\btheta\|_2^2/2$, and the base measure $\pi_0(\bxi) = \frac{1}{(\sqrt{2\pi)^d}} \exp(-\|\bxi\|_2 ^2/2)$ or equivalently $\pi_0(\x) = \frac{1}{\sqrt{(2\pi)^d}\sigma^d} \exp(-\|\x\|_2^2/2\sigma^2)$ using $\bxi = \x/\sigma$ and $d\bxi = d\x/\sigma$. The scaled parameter $\btheta_{\alpha} = \btheta_{\sigma} = \btheta/\sigma$. Then, the distribution from the natural parameter form is:
% \begin{equation}
%     p_{\btheta/\sigma}(\x) = \exp( \langle \x, \btheta\rangle / \sigma^2 - \|\btheta\|_2^2/(2\sigma^2) ) \times \frac{1}{\sqrt{(2\pi)^d}\sigma^d} \exp(-\|\x\|_2^2/2\sigma^2)
%     = \frac{1}{\sqrt{(2\pi)^d}\sigma^d} \exp(-\|\x-\btheta\|_2^2/2\sigma^2).
% \end{equation}
SGLD uses scaled Gaussian noise with $\psi(\btheta)= \|\btheta\|_2^2/2, \alpha_t = \sqrt{\sigma_t/\eta_t}$, so that $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t}) = \mathcal{N}(\btheta_{B_t}, \alpha_t^2 \I_d)$. By taking $\rho_t = \sqrt{\eta_t\sigma_t}$, the update \eqref{eq:efld1} based on $\rho_t \bxi_t$ is distributed as $\mathcal{N}(\rho_t\btheta_{B_t}, \rho_t^2\alpha_t^2 \I_d) = \mathcal{N}(\eta_t\nabla \ell(\w_{t-1}, S_{B_t}), \sigma_t^2 \I_d)$. Thus the EFLD update reduces to the SGLD update: $\w_{t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1}, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right).$
\qed
% By taking $\rho_t = \sqrt{\eta_t\sigma_t},~\alpha_t = \sqrt{\sigma_t/\eta_t},~ \psi(\btheta)= \|\btheta\|_2^2/2,~ \bxi = \x/\alpha_t,~\pi_0(\bxi) = \frac{1}{\sqrt{(2\pi)^d}} \exp(-\|\bxi\|_2 ^2/2)$ in exponential family update equation \eqref{eq:efld1}, the exponential family distribution $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ becomes
% \begin{align*}
%     p_{\btheta_{B_t,\alpha_t}}(\x) = \exp( \langle \x, \btheta_{B_t}\rangle / \alpha_t ^2 - \|\btheta_{B_t}\|_2^2/(2\alpha_t^2) )  \frac{1}{\sqrt{(2\pi)^d}\alpha_t^d} \exp(-\|\x\|_2^2/2\alpha_t^2)
%     = \frac{1}{\sqrt{(2\pi)^d}\alpha_t^d} \exp(-\|\x-\btheta_{B_t}\|_2^2/2\alpha_t^2),
% \end{align*}
% which is a normal distribution $\mathcal{N}(\btheta_{B_t}, \alpha_t^2 \I_d)$, by scaling $\rho_t$ it becomes $\mathcal{N}(\rho_t\btheta_{B_t}, \rho_t^2\alpha_t^2 \I_d)$ which is $\mathcal{N}(\eta_t\nabla \ell(\w_{t-1}, S_{B_t}), \sigma_t^2 \I_d)$. Thus the EFLD update reduces to the SGLD update:
% $\w_{t+1} = \w_{t} - \eta_t \nabla \ell(\w_t, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right).$
% \qed
\end{exam}

\begin{exam}[Noisy Sign-SGD]
\label{exam:noisy_signsgd}
%\abcomment{just keep the part showing this is a special case of EFLD}\tccomment{Updated.}
By taking $\rho_t = \eta_t$ and component-wise $\xi_j \in\{-1,1\},~\pi_0(\xi_j)=1,~\psi(\theta) = \log(\exp(-\theta)+\exp(\theta))$ in exponential family update equation \eqref{eq:efld1}, the $j$-th component of exponential family distribution $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ becomes
$p_{\btheta_{B_t,\alpha_t,j}}(\xi_j)  = \frac{\exp(\xi_j \btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})}$.
%\begin{align*}
    % p_{\btheta_{B_t,\alpha_t,j}}(\xi) = \exp(x\btheta_{B_t,\alpha_t,j} - \log(\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j}))) = \frac{\exp(x\btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})}.
%\end{align*}
Thus, the EFLD update reduces to a noisy version of Sign-SGD: 
$\w_{t} = \w_{t-1} - \eta_t \bxi_t$, $\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(\xi_j)$, 
% \begin{equation}\label{eq:signSGD_mini_batch_1}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, ~\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(x) =  \frac{\exp(x \btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})},~ x\in\{-1,+1\}
% \end{equation}
$j\in [d]$, where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
% for mini-batch $B_t$ and scaling $\alpha_t$, mini-batch noisy sign-SGD updates the parameters as
% \begin{equation}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim p_{\alpha_t}(\xi) =  \left(\frac{1}{0.5+\exp(-\theta_{B_t,\alpha_t})}\right)^{\frac{1+\xi}{2}} \left(\frac{1-\mu_\alpha}{2}\right)^{\frac{1-\xi}{2}}   ~, ~ \forall i\in [d],
% \end{equation}
\qed
\end{exam}



\vspace*{-2mm} 
\subsection{Expected Stability of Exponential Family Langevin Dynamics}
\input{ICLR2022/sec/stability}


\vspace*{-2mm} 
\subsection{Optimization Guarantees for EFLD}
\vspace*{-2mm} 
% \abcomment{need a general story for the opt guarantees}

% \abcomment{fall back -- show specific cases for SGLD and noisy sign-SGD}

% The ``density'' for a mini-batch $B$ at scale $\alpha$ is:
% \begin{equation}
% p_{\psi}(\bxi; \btheta_{B,\alpha}) = \exp(\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha} \triangleq \frac{\btheta_B}{\alpha} = \frac{\nabla \ell(\w_{t}, S_{B})}{\alpha}~.
% \end{equation}
% Note that the corresponding expectation parameter
% \begin{equation}
% \m_{B,\alpha} = \nabla_{\btheta_{B,\alpha}} \psi( \theta_{B,\alpha} )~.
% \end{equation}


We now establish optimization guarantees for two examples of EFLD, i.e., Noisy Sign-SGD with Bernoulli noise over $\{-1,+1\}$ and SGLD with Gaussian noise.  

{\bf Noisy Sign-SGD.}
% We first provide a optimization guarantees for Noisy sign-SGD under both full-batch and mini-batch settings. Focusing on the natural parameter form, the full-batch Noisy Sign-SGD update the parameters as
% \begin{equation}\label{eq:signSGD_full_batch}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, ~ \bxi_{t,i} \sim p_{\alpha_t}(\xi) =  \frac{1}{\exp((1-\xi)\nabla L_S(\w_t)/\alpha_t)+\exp((-1-\xi)\nabla L_S(\w_t)/\alpha_t)}~, ~ \xi\in\{-1,+1\}
% \end{equation}
% for any $i\in [d]$.
For mini-batch $B_t$ and scaling $\alpha_t$, mini-batch Noisy Sign-SGD updates the parameters as $\w_{t} = \w_{t-1} - \eta_t \bxi_t$, where each component $j\in [d]$ 
\begin{equation}\label{eq:signSGD_mini_batch}
    \bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(x) =  \frac{\exp(x \btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})},~ x\in\{-1,+1\}
\end{equation}
where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
The full-batch version uses parameters $\E_{B_t}[\btheta_{B_t,\alpha_t}] = \nabla L_S(\w_{t-1})$
% Here we consider the special case of Bernoulli distribution. Thus
% $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$
For the optimization analysis, we assume that the loss is smooth and mini-batch gradients are unbiased, symmetric, and sub-Gaussian.
%of the empirical loss function $L_S(\w)$:
\begin{restatable}{asmp}{asmpsmooth}\label{asmp: smooth}
The loss function $L_S$ satisfies: for all $\w$ and $\w^\prime$, for some non-negative constant $\vec{K}:=\left[K_{1}, \ldots, K_{d}\right]$, we have
%\begin{align}
$L_S(\w) \leq L_S(\w^\prime) + \nabla L_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} K_i (\w_i - \w^\prime_i)^2$.
%\end{align}
\vspace*{-1mm}
\end{restatable}
% The assumption on the empirical loss $L_S(\w)$ is common in optimization analysis [Bernstein's][][], besides that, we also assume some natural statistical properties of the batch gradient of the loss $\nabla \ell(\w_{t}, S_{B_t})$, where the randomness comes from batches conditioned on $\w_t$, satisfies the following assumptions:
\begin{restatable}{asmp}{asmpbatch}\label{asmp:batch}
Given $\w_{t-1}$, the mini-batch gradient $\nabla \ell(\w_{t-1}, S_{B_t})$ is
(a) unbiased,  i.e., $\E_{B_t|\w_{t-1}}\nabla \ell(\w_{t-1}, S_{B_t}) = \nabla L_S(\w_{t-1})$;
%\abbcomment{notation not consistent}\tccomment{Switch $\cL$ to $L$, use $K$ for Lipschitz constants}; 
(b) symmetric, i.e., the density $p(x)$ of $x \equiv \nabla \ell(\w_{t-1}, S_{B_{t}})$ is symmetric around its expectation $L_S(\w_{t-1})$: $p(x) = p(2\nabla L_S(\w_{t-1})-x)$ %\abbcomment{notation not consistent};
and 
(c) sub-Gaussian, i.e., for any $\lambda >0$, {any $\v$ s.t. $\|\v\|_2 =1$}, $\E_{B_t|\w_{t-1}}\exp \lambda\langle \v,\nabla \ell(\w_{t-1}, S_{B_{t}})-\nabla  L_S(\w_{t-1})\rangle \leq \exp(\lambda^2\kappa_t^2/2)$ for some constant $\kappa_t > 0$.
%\end{itemize}
%[Batch Gradient] 
% Given $\w_{t-1}$, the mini-batch gradient $\nabla \ell(\w_t, S_{B_t})$ is
% \begin{itemize}
% \item (Unbiased)  The mini-batch gradient $\nabla \ell(\w_{t}, S_{{B_t}})$ is an unbiased estimator of true gradient $L_S(\w_{t})$: $\E_{B_t|\w_t}\nabla \ell(\w_{t}, S_{B_t}) = \nabla L_S(\w_{t}).$
%     \item (Symmetricity) The pdf $p_{BG}(x)$ of mini-batch gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is symmetric around its expectation $L_S(\w_{t})$: $p_{BG}(x) = p_{BG}(2\nabla L_S(\w_{t})-x).$
%     \item (Sub-Gaussian) The mini-batch gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is Sub-Gaussian with $\psi_2$ norm $\kappa$: for any $\lambda >0$, $v\in S^{d-1}$, we have $\E_{B_t|\w_t}\exp \lambda\langle v,\nabla \ell(\w_{t}, S_{B_{t}})-\nabla L_S(\w_{t})\rangle \leq \exp(\lambda^2\kappa^2/2).$
% \end{itemize}
\vspace{-2mm}
\end{restatable}
%With Assumption \ref{asmp: smooth} and Assumption \ref{asmp:batch}, we have the following guarantee for convergence of noisy signSGD under full batch and mini batch settings:
Based on the assumptions, we have the following optimization guarantee for mini-batch noisy Sign-SGD. We defer the optimization guarantee for full-batch noisy Sign-SGD to Appendix \ref{app:opt}. %\tccomment{Full-batch drops to appendix}



\begin{restatable}{theo}{theosignSGDconv}\label{theo:signSGD_conv}
Under Assumption~\ref{asmp: smooth} and \ref{asmp:batch}, for mini-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$, 
% $\alpha_t = 2G$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% or choose $c\geq\alpha_t\geq 2G$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{2c (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% or without assuming $G$, 
$\alpha_t$ satisfying $c \geq \alpha_t \geq \max[\sqrt{2}\kappa_t, 4\|\nabla L_S(\w_{t-1})\|_{\infty}]$, we have for any $S$ and any initialization $\w_0$
\vspace{-2mm}
\begin{equation}\label{eq:sign_SGD_mini_batch_convergence}
\vspace{-1mm}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
\end{equation}
where the expectation is taken over the randomness of  algorithm.
\vspace{-2mm}
\end{restatable}



% \abcomment{add as remark or drop (space limit)} Theorem \ref{theo:signSGD_conv} shows the convergence rate for noisy-signSGD update is $O\left(\frac{1}{\sqrt{T}}\right)$ which matches the same rate as the noiseless signSGD in \cite{bernstein2018signsgd}.


% \begin{asmp} \label{asmp: sample_lip}
% The loss function $\ell(\w,z)$ is:\vspace*{-2mm}
% \begin{enumerate}
%     \item Bounded, i.e., $\forall \w, z, \ell(\w,z) \leq c_0$; and
%     \item Sample-Lipschitz, i.e., 
%     \begin{equation}
%       \forall z, z', \w  \quad \| \nabla f(\w,z) - \nabla f(\w,z') \| \leq L~.
%       \vspace*{-2mm}
%     \end{equation}
% \end{enumerate}
% \end{asmp}
% Note the Sample-Lipschitz property follows if the gradients $\nabla \ell(\w,z)$ are bounded, i.e., $\ell$ is Lipshitz. Further, the norm $\| \cdot \|$ can be viewed as the $L_2$ norm for now.

{\bf SGLD.} We acknowledge that the following optimization result of SGLD exists in various forms, as noisy gradient descent algorithms have been studied in literature such as differential privacy, where SGLD can be viewed as DP-SGD  \citep{bassily2014private, wang2019differentially} and the proof technique boils down to bounding the stochastic variance of the noisy gradient \citep{shamir2013stochastic}.
%\abcomment{ack that this result exists in various forms, is not new}
\begin{restatable}{theo}{theoSGLDopt}
Under Assumption \ref{asmp: smooth} and \ref{asmp:batch}, with $K_i = K, \forall i \in [d]$, for any $S$, SGLD (EFLD with step size $\rho_t = \sqrt{\eta_t\sigma_t}$, $\alpha_t = \sqrt{\sigma_t/\eta_t} $), $|B_t| = b$, and $\eta_t = \frac{1}{\sqrt{T}}$, can achieve
\begin{align}
\vspace{-3mm}
\frac{1}{T} \sum_{t =1}^T \mathbb{E} \| \nabla L_S(\w_t)\|^2 
%\min_{k\in [T]} \mathbb{E} \| \nabla L_S(\w_t)\|^2
\leq O\left(\frac{1}{\sqrt{T}}\right) +O\left(K \frac{  p \sum_{t=1}^T\alpha_t^4 +  \log T }{\sqrt{T}}\right)~,
\end{align}
where the expectation is over the randomness of the algorithm.
\vspace*{-2mm}
\end{restatable}
%\yzcomment{will add a comment here} \yzcomment{done}
%SGLD also converges with the rate of $O(1/\sqrt{T})$ which is the same as SGD for non-convex and smooth problems. 
The error rate of SGLD depends on the noise variance $\alpha_t$.  One can choose a decaying noise variance such as  $\alpha_t = 1/\sqrt[4]{t}$ to guarantee the convergence. Then the rate will become $O(\log T/\sqrt{T})$. We note that similar to the optimization guarantees of DP-SGD, the convergence rate depends on the dimension of the gradient $p$ due to the isotropic Gaussian noise. Special noise structures such as anisotropic noise that aligned with the gradient structure can reduce the dependence on dimension \citep{kairouz2020dimension,zhang2021wide,asi2021private, zhou2020bypassing}.  









==> ICLR2022/sec/exp.tex <==
\vspace*{-2mm}
\begin{figure*}[t] 
\centering
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-c-new.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-c-new.png}
 }
\subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-c-new.png}
 } 
 \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-c-new.png}
 } \vspace*{-3mm}
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-b-new.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-b-new.png}
 }
\subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-b-new.png}
 } 
 \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-b-new.png}
 }\vspace*{-1mm}
  \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a-new.png}
 } 
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a-new.png}
 }
  \subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-a-new.png}
 } 
  \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-a-new.png}
 }
\vspace*{-4mm}
\caption[]{Numerical results for training CNN using SGLD ($\sigma_t = \sqrt{2\eta_t/\beta_t}$) on MNIST, Fashion-MNIST and CIFAR-10. X-axis shows the number of training epochs. (a)-(d) shows our bound is non-vacuous and can be used to bound the empirical test error. (e)-(h) compare our bound with the existing bounds and show the effect on $\alpha_t^2$. (i)-(l) show the key factors in each bound, i.e., the squared gradient norm in \cite{Li2020On}, the gradient incoherence in \cite{negrea2019information}, the two-sample incoherence in \cite{rodriguez2021random}, and the gradient discrepancy in our bound.  Our bounds are numerically sharper than existing bounds, and larger $\alpha_t^2$ leads to tighter generalization bounds which is consistent with the theoretical analysis.
}
\vspace*{-6mm}
\label{fig:sgld_bound}
\end{figure*}






In this section, we conduct a series of experiments to evaluate our generalization error bounds. For SGLD, we aim to compare the proposed  bound in Theorem \ref{theo:efldstab} with existing bounds in \cite{Li2020On}, \cite{negrea2019information}, and \cite{rodriguez2021random} for various datasets. Note that the bound presented in \cite{rodriguez2021random} is an extension of that in \cite{haghifam2020sharpened} from full-batch setting to mini-batch setting . %We note that the squared norm of ``two-sample incoherence'' appeared in \cite{haghifam2020sharpened} (Theorem 4.2) roughly has the same order of magnitude as the gradient incoherence appeared in \cite{negrea2019information}. 
We also evaluate the optimization performance of proposed Noisy Sign-SGD by comparing it with the original sign-SGD \citep{bernstein2018signsgd} and present the corresponding generalization bound in Theorem \ref{theo:efldstab}. 

The details of our model architectures, learning rate scheduling, hyper-parameter selections and additional experimental results can be found in Appendix \ref{app:exp}. We acknowledge that we did not achieve the state-of-the art predictive performance, mainly due to the simplicity of our model architectures. With more complex model and further tuning, the prediction results could be improved.

\vspace*{-2mm}
\subsection{Stochastic Gradient Langevin Dynamics}
\vspace*{-2mm}
\textbf{Comparison with existing work.} We have derived theoretical generalization error bounds that depend on the data-dependent quantity \emph{gradient discrepancy}, i.e., $\left\|\nabla \ell\left(\w_{t}, z_n \right)  -  \nabla \ell\left(\w_{t}, z'_n\right)\right\|_{2}^{2}$. Existing bounds in \cite{Li2020On} and \cite{negrea2019information} have also improved the Lipschitz constant in \cite{mou2018generalization} to a data-dependent quantity. As shown in Figure~\ref{fig:sgld_bound} (a)-(d), by combining with the empirical training error, all four generalization error bounds can be used to bound the empirical test error, but our bound is able to generate a much tighter upper bound. Such difference is mainly due to the fact that we replace the squared \emph{gradient norm} in \cite{Li2020On}, the squared norm of \emph{gradient incoherence}
in  \cite{negrea2019information}, and that of \emph{two-sample incoherence} in \cite{rodriguez2021random} with the gradient discrepancy. Results in Figure~\ref{fig:sgld_bound} (e)-(h) show that our bounds are much sharper than those of \cite{Li2020On} because our gradient discrepancy (Figure~\ref{fig:sgld_bound} (i)-(l)) is usually 2-4 order of magnitude smaller than the squared gradient norms appeared in \cite{Li2020On}. Our bounds are also sharper than those of \cite{negrea2019information} and \cite{rodriguez2021random} due to an improved dependence on $n$ from an order of $1/\sqrt{n}$ to ${1}/{n}$. Note that, even though the gradient incoherence in \cite{negrea2019information} is about 1 to 2 order of magnitude smaller than the gradient discrepancy for simple problems such as MNIST and Fashion-MNIST, the difference between the gradient incoherence and our gradient discrepancy reduces as the problem becomes harder (see results for CIFAR-10 in Figure~\ref{fig:sgld_bound}(j)).


%We report those data-dependent quantities in Figure \ref{fig:sgld_bound} for MNIST (i), Cifar-10 (j), and Fashion-MNIST (k)-(l),respectively. The results suggest that the squared gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors. The gradient incoherence in \cite{negrea2019information} is about 1 to 2 order of magnitude smaller than the gradient discrepancy for simple problems such as MNIST and Fashion-MNIST. %However, as problem becomes more difficult, i.e., CIFAR-10, the difference between the gradient incoherence and our gradient discrepancy reduces. Moreover, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$ which has a worse sample dependence compared to our bound. 







\begin{figure*}[t] 
\centering
%\subfigure[CNN, MNIST, SGLD, $\alpha_t=0.2$, $\sigma_t=\alpha_t\eta_t \approx 10^{-4}$]{\includegraphics[width=0.95\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2.png}}
\subfigure[Bounded Test Error]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-d.png}
 }  
\subfigure[Our Bound]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-b.png}
 }  
\subfigure[Gradient Discrepancy]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-a.png}
 } 
\subfigure[Training Error]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-c.png}
 }
\vspace*{-3mm}
\caption[]{Numerical results for training CNN using SGLD ($\sigma_t = 0.2\eta_t$) on a subset of MNIST ($n=10000$) with different randomness on labels. (a) demonstrates that, as the randomness increases, the empirical test error (dashed lines) increases but still can be bounded by our generalization bound by combining the empirical training error (solid lines). (b) presents our bound in Theorem \ref{theo:efldstab}. (c) shows the gradient discrepancy $\left\|\nabla \ell\left(\w_t, z_n \right)  -  \nabla \ell\left(\w_t, z'_n\right)\right\|_{2}^{2}$. (d) plots the training error. The gradient discrepancy increases as randomness increases, so does our generalization bound.
}
\vspace*{-4mm}
\label{fig:bound_random}
\end{figure*}




\begin{figure*}[t] 
\centering
  \subfigure[CNN, MNIST]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/cnn1-mnist-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 } 
  \subfigure[CNN, Fashion]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/cnn1-fashion-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
 \subfigure[ResNet-18, CIFAR10]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/resnet18-cifar10-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
 \subfigure[ResNet-18, CIFAR100]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/resnet18-cifar100-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }\vspace*{-2mm}
\subfigure[MNIST, $\alpha_t=1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
 } 
  \subfigure[MNIST, $\alpha_t=0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-e.png}
 }
  \subfigure[Fashion, $\alpha_t=1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
 } 
  \subfigure[Fashion, $\alpha_t=0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-e.png}
 }
\vspace*{-4mm}
\caption[]{(a)-(d) show the training dynamics of CNN on MNIST and Fashion-MNIST, and ResNet-18 on CIFAR-10 and CIFAR-100 using noisy sign-SGD with different scaling $\alpha_t$. Legends indicate the choice of $\alpha_t$ and the numbers in brackets are test errors at convergence. As $\alpha_t\to 0$, Nosiy sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original sign-SGD \citep{bernstein2018signsgd}. (e)-(f) show that empirical test error can be bounded by our bound and the corresponding training error. The larger $\alpha_t$ is the sharper our bound is.}
\vspace*{-5mm}
\label{fig:noisy_signsgd}
\end{figure*}



\textbf{Effect of Randomness.} Motivated by \cite{zhang2017understanding}, we train CNN with SGLD on a smaller subset of MNIST dataset ($n=10000$) with randomly corrupted labels. The corruption fraction varies from $0\%$ (without label corruption) to $60\%$. As shown in Figure~\ref{fig:bound_random} (d), for long enough training time, all experiments with different level of label randomness can achieve almost zero training error. However, the one with higher level of randomness has higher generalization/test error (Figure \ref{fig:bound_random} (a) dashed lines). Our generalization bound also becomes larger as the randomness increases since the corresponding gradient discrepancy increases.



\vspace*{-2mm}
\subsection{Noisy Sign-SGD}
\vspace*{-2mm}
%In this section, we present numerical results for Noisy Sign-SGD presented in Example \ref{exam:noisy_signsgd}.  Since none of the existing bounds is derived to handle Bernoulli noisy, we only present our bound here.

\textbf{Optimization.} Figure~\ref{fig:noisy_signsgd} (a)-(d) show the training dynamics of Noisy Sign-SGD under various selections of $\alpha_t$. As $\alpha_t\to 0$, Noisy Sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original Sign-SGD \citep{bernstein2018signsgd}. However, as $\alpha_t$ increases, the probability of getting 1 approaches 0.5, and $\xi_t$ approximates a uniform distribution. As a result, the corresponding Noisy Sign-SGD still converges, but the generalization performance is much worse.

\textbf{Generalization Bound.} Figure \ref{fig:noisy_signsgd}(e)-(f) show that our bound successfully bounds the empirical test error.
%and the corresponding training error. 
The larger $\alpha_t$ is the sharper the upper bound is. However, larger $\alpha_t$ would slow down and adversely affect the optimization, e.g., Figure~\ref{fig:noisy_signsgd} (a)-(d) blue and orange lines. In practice, one needs to balance the optimization error and generalization by choosing a suitable scaling $\alpha_t$.
















% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN, MNIST, SGLD, $\beta_t = 55000$, $\sigma_t\approx 4\times 10^{-4}$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-pretrain.png}
%  } 
% \caption[]{Numerical results for CNN trained on MNIST with pre-training on a prertained dataset $\mathbf{J}_0$ where $|\mathbf{J}_0|=m$. As we increase the pretrain dataset size m, the gradient discrepancy decreases so does our bound.
% }
% \label{fig:mnist_sgld_pretrain}
% \end{figure*}




















%Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to those for CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases, leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence. 

%We note that  \cite{haghifam2020sharpened} show that Negrea et al. bound is smaller than Li et al. in their empirical evaluation, which is opposite to what we observed in Figure \ref{fig:mnist}.We think this is because \cite{haghifam2020sharpened} consider the full-batch setting which has a different form of gradient incoherence compared to the mini-batch setting in our paper. \yzcomment{added the discussion about the inconsistent of our result and \cite{haghifam2020sharpened}}


% The second key difference is the order of dependence on the sample size $n$, i.e., both of our bound and $\cite{Li2020On}$ has a bound of order $\frac{1}{n}$, however, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$. 
%Figure \ref{fig:mnist} (a) and 
% (b) suggests that the gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors, and the gradient incoherence in \cite{negrea2019information} is much smaller than the gradient discrepancy in our bound as well.
% However, the results in (b-d) for MNIST and (f-h) for Fashion MNIST show that our bounds are much sharper than those of \cite{negrea2019information} due to improving the dependence on $n$ from a order of $\frac{1}{\sqrt{n}}$ to $\frac{1}{n}$. Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence.


%More details of our model architectures and addtional experimental results can be found in Appendix. We acknowledge that we did not aim to achieve the state-of-the art predictive performance. With further tuning, the prediction results could be improved








% \begin{figure*}[t] 
% \centering
% \includegraphics[ width=0.5\textwidth]{ICLR2022/images/vgg5-mnist-n1000-bs100-BernoulliSGD-train-dynamics.png}
% \caption[]{Training dynamics of Noisy SignSGD with Bernoulli noise with various selection of $\alpha$ for VGG5 trained on MNIST.When $\alpha \to 0$, Bernoulli SignSGD reduces to SignSGD. As a results, Bernoulli SignSGD with small enough $\alpha$ matches the training trajectory of SignSGD.
% } 
% \label{fig:mnist}
% \end{figure*}

% \textbf{To Do List}

% The following experiments follow the setting described in  \cite{negrea2019information}. \textbf{[By the end of this week (September 19)]}
% \begin{enumerate}
%     \item CNN (two convolutional layers + two fully connected layers) on MNIST and Fashion MNIST
%     \item CNN (two convolutional layers + three fully connected layers) on CIFAR-10
% \end{enumerate}

% The following experiments follow the standard setting most DL papers likely to perform. \textbf{[Before next Wednesday (September 22)]}
% \begin{enumerate}
%     \item VGG5 on MNIST and Fashion MNIST
%     \item ResNet-18 on CIFAR-10 and CIFAR-100
% \end{enumerate}



% \textbf{To Plot}
% \begin{enumerate}
%     \item Gradient norms \citep{Li2020On}
%     \item Gradient incoherence \citep{negrea2019information}
%     \item Gradient discrepancy $\| \mathbf{\theta}_{B,\alpha} - \mathbf{\theta}_{B',\alpha} \|_2^2$ (our bound)
%     \item Our bound, Negrea's bound, and Li et al., bound.
% \end{enumerate}

% \newpage

% \begin{table}
%   \caption{Summary of Experiments for SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $\beta_t$ & Our bound & Li bound & Negrea Bound \\
%     \midrule
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.96 & 55000 & $\checkmark$ & $\checkmark$ & $\checkmark$   \\
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.96 & 5000 & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
%     CNN-1 & Fashion  & $4\times 10^{-3}$ & 0.93 & 55000 & $\checkmark$ & $\checkmark$ & $\checkmark$  \\
%     CNN-1 & Fashion & $4\times 10^{-3}$ & 0.93 & 5000 & $\checkmark$ & $\checkmark$ &$\checkmark$  \\
%     \midrule
%     CNN-2 & CIFAR-10  & $5\times 10^{-3}$ & 0.95 & 55000 &  &  &   \\
%     CNN-2 & CIFAR-10  & $5\times 10^{-3}$ & 0.95 & 5000 &  &  &  \\
%   \midrule
%   ResNet-18/50 & Mini ImageNet & ? & ?&? & & &\\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for Noisy SGD with Gaussian Noise ($\sigma_t=c\eta_t$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $c$ & Our bound & Li bound & Negrea Bound \\
%     \midrule
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.995 & 0.002 &$\checkmark$  & $\checkmark$ &   \\
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.95 & 0.2 &$\checkmark$  &$\checkmark$  &  \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$) with pretrain ($|J_0|=m$)}
%   \label{tab:sgld_pretrain}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & m &$\eta_0$& decay & $\beta_t$ & Our bound\\
%     \midrule
%     CNN-1 & MNIST  & 100 & $4\times 10^{-3}$ & 0.96 & 55000 &   \\
%     CNN-1 & MNIST  & 1000 & $4\times 10^{-3}$ & 0.96 & 55000 &   \\
%     CNN-1 & MNIST  & 10000 & $4\times 10^{-3}$ & 0.96 & 55000 &    \\
%     CNN-1 & MNIST  & 50000 & $4\times 10^{-3}$ & 0.96 & 55000 &    \\
%     \midrule
%     CNN-1 & Fashion & 100 & $4\times 10^{-3}$ & 0.93 & 55000 &   \\
%     CNN-1 & Fashion & 1000 & $4\times 10^{-3}$ & 0.93 & 55000 &    \\
%     CNN-1 & Fashion & 10000 & $4\times 10^{-3}$ & 0.93 & 55000 &    \\
%     CNN-1 & Fashion & 50000 & $4\times 10^{-3}$ & 0.93 & 55000 &   \\
%     \bottomrule
%   \end{tabular}
% \end{table}



% \begin{table}
%   \caption{Summary of Experiments for Random Labels with SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & Randomness & $\eta_0$& decay & $\beta_t$ & Our bound  \\
%     \midrule
%     CNN-1 & MNIST  &0 &$4\times 10^{-3}$ & 0.96 & 55000 & $\checkmark$  \\
%     CNN-1 & MNIST  &10\% &? & ? & ? & \\
%     CNN-1 & MNIST & 20\% &? & ? & ? & \\
%     CNN-1 & MNIST & 50\% &? & ? & ? & \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for Noisy SGD with Bernoulli Noise ($\mu_{\alpha} = \frac{1}{1+\exp(-\theta/\alpha})$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $\alpha_t$ & Our bound \\
%     \midrule
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-6}$ &   \\
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-2}$ &  \\
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-1}$ &  \\
%     CNN-1 & Fashion  & $10^{-4}$ & 0.1 & $10^{-6}$ &     \\
%     CNN-1 & Fashion & $10^{-4}$ & 0.1 & $10^{-2}$&   \\
%     CNN-1 & Fashion & $10^{-4}$ & 0.1 & $10^{-1}$&   \\
%     \midrule
%     CNN-2 & CIFAR-10  & $10^{-3}$ &0.1  & $10^{-6}$ &   \\
%     CNN-2 & CIFAR-10  & $10^{-3}$ & 0.1 & $10^{-2}$ &  \\
%     CNN-1 & CIFAR-10  & $10^{-3}$ &0.1  & $10^{-1}$ &  \\
%   \midrule
%   ResNet-18/50 & Mini ImageNet & ? & ?&? & \\
%     \bottomrule
%   \end{tabular}
% \end{table}



==> ICLR2022/sec/exp_old.tex <==
\vspace*{-2mm}
\begin{figure*}[t] 
\centering
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-c.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-c.png}
 }
\subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-c.png}
 } 
 \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-c.png}
 } \vspace*{-3mm}
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-b.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-b.png}
 }
\subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-b.png}
 } 
 \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-b.png}
 }\vspace*{-1mm}
  \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a.png}
 } 
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a.png}
 }
  \subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-a.png}
 } 
  \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-a.png}
 }
\vspace*{-4mm}
\caption[]{Numerical results for training CNN using SGLD ($\sigma_t = \sqrt{2\eta_t/\beta_t}$) on MNIST, Fashion-MNIST and CIFAR-10. X-axis shows the number of training epochs. (a)-(d) shows our bound is non-vacuous and can be used to bound the empirical test error. (e)-(h) compare our bound with the existing bounds and show the effect on $\alpha_t^2$. (i)-(l) show the key factors in each bound, i.e., the squared gradient norm in \cite{Li2020On}, the gradient incoherence in \cite{negrea2019information}, and the gradient discrepancy in our bound.  Our bounds are numerically sharper than existing bounds, and larger $\alpha_t^2$ leads to tighter generalization bounds which is consistent with the theoretical analysis.
}
\vspace*{-3mm}
\label{fig:sgld_bound}
\end{figure*}






In this section, we conduct a series of experiments to evaluate our generalization error bounds. For SGLD, we aim to compare the proposed  bound in Theorem \ref{theo:efldstab} with existing bounds in \cite{Li2020On} and  \cite{negrea2019information} for various datasets.
Note that we do not consider the bound in \cite{haghifam2020sharpened} as a baseline because the bound in \cite{haghifam2020sharpened} only applies to full-batch setting, but we focus on noisy mini-batch gradient descent. We note that the squared norm of ``two-sample incoherence'' appeared in \cite{haghifam2020sharpened} (Theorem 4.2) roughly has the same order of magnitude as the gradient incoherence appeared in \cite{negrea2019information}. We also evaluate the optimization performance of proposed Noisy Sign-SGD by comparing it with the original sign-SGD \citep{bernstein2018signsgd} and present the corresponding generalization bound in Theorem \ref{theo:efldstab}. 

The details of our model architectures, learning rate scheduling, hyper-parameter selections and additional experimental results can be found in Appendix \ref{app:exp}. We acknowledge that we did not achieve the state-of-the art predictive performance, mainly due to the simplicity of our model architectures. With more complex model and further tuning, the prediction results could be improved.

\vspace*{-2mm}
\subsection{Stochastic Gradient Langevin Dynamics}
\vspace*{-2mm}
\textbf{Comparison with existing work.} We have derived theoretical generalization error bounds that depend on the data-dependent quantity \emph{gradient discrepancy}, i.e., $\left\|\nabla \ell\left(\w_{t}, z_n \right)  -  \nabla \ell\left(\w_{t}, z'_n\right)\right\|_{2}^{2}$. Existing bounds in \cite{Li2020On} and \cite{negrea2019information} have also improved the Lipschitz constant in \cite{mou2018generalization} to a data-dependent quantity. As shown in Figure~\ref{fig:sgld_bound} (a)-(d), by combining with the empirical training error, all three generalization error bounds can be used to bound the empirical test error, but our bound is able to generate a much tighter upper bound. Such difference is mainly due to the fact that we replace the squared \emph{gradient norm} in \cite{Li2020On} and the squared norm of \emph{gradient incoherence}
%i.e., $\frac{1}{n}\sum_{z \in S}\|\nabla \ell(\w_t,z)\|$ in \cite{Li2020On} and the squared norm of \emph{gradient incoherence}, i.e., $\|\zeta_t\|=\left\|\nabla \ell\left(\w_{t-1}, z_J \right)  -  \nabla \ell\left(\w_{t-1}, z_{i\in[n],i\neq J}\right)\right\|$
in  \cite{negrea2019information} with the gradient discrepancy. Results in Figure~\ref{fig:sgld_bound} (e)-(h) show that our bounds are much sharper than those of \cite{Li2020On} because our gradient discrepancy (Figure~\ref{fig:sgld_bound} (i)-(l)) is usually 2-4 order of magnitude smaller than the squared gradient norms appeared in \cite{Li2020On}. Our bounds are also sharper than those of \cite{negrea2019information} due to an improved dependence on $n$ from an order of $1/\sqrt{n}$ to ${1}/{n}$. Note that, even though the gradient incoherence in \cite{negrea2019information} is about 1 to 2 order of magnitude smaller than the gradient discrepancy for simple problems such as MNIST and Fashion-MNIST, the difference between the gradient incoherence and our gradient discrepancy reduces as the problem becomes harder (see results for CIFAR-10 in Figure~\ref{fig:sgld_bound}(j)).


%We report those data-dependent quantities in Figure \ref{fig:sgld_bound} for MNIST (i), Cifar-10 (j), and Fashion-MNIST (k)-(l),respectively. The results suggest that the squared gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors. The gradient incoherence in \cite{negrea2019information} is about 1 to 2 order of magnitude smaller than the gradient discrepancy for simple problems such as MNIST and Fashion-MNIST. %However, as problem becomes more difficult, i.e., CIFAR-10, the difference between the gradient incoherence and our gradient discrepancy reduces. Moreover, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$ which has a worse sample dependence compared to our bound. 







\begin{figure*}[t] 
\centering
%\subfigure[CNN, MNIST, SGLD, $\alpha_t=0.2$, $\sigma_t=\alpha_t\eta_t \approx 10^{-4}$]{\includegraphics[width=0.95\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2.png}}
\subfigure[Bounded Test Error]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-d.png}
 }  
\subfigure[Our Bound]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-b.png}
 }  
\subfigure[Gradient Discrepancy]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-a.png}
 } 
\subfigure[Training Error]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-c.png}
 }
\vspace*{-3mm}
\caption[]{Numerical results for training CNN using SGLD ($\sigma_t = 0.2\eta_t$) on a subset of MNIST ($n=10000$) with different randomness on labels. (a) demonstrates that, as the randomness increases, the empirical test error (dashed lines) increases but still can be bounded by our generalization bound by combining the empirical training error (solid lines). (b) presents our bound in Theorem \ref{theo:efldstab}. (c) shows the gradient discrepancy $\left\|\nabla \ell\left(\w_t, z_n \right)  -  \nabla \ell\left(\w_t, z'_n\right)\right\|_{2}^{2}$. (d) plots the training error. The gradient discrepancy increases as randomness increases, so does our generalization bound.
}
\vspace*{-4mm}
\label{fig:bound_random}
\end{figure*}




\begin{figure*}[t] 
\centering
  \subfigure[CNN, MNIST]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/cnn1-mnist-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 } 
  \subfigure[CNN, Fashion]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/cnn1-fashion-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
 \subfigure[ResNet-18, CIFAR10]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/resnet18-cifar10-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
 \subfigure[ResNet-18, CIFAR100]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/resnet18-cifar100-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }\vspace*{-2mm}
\subfigure[MNIST, $\alpha_t=1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
 } 
  \subfigure[MNIST, $\alpha_t=0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-e.png}
 }
  \subfigure[Fashion, $\alpha_t=1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
 } 
  \subfigure[Fashion, $\alpha_t=0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-e.png}
 }
\vspace*{-4mm}
\caption[]{(a)-(d) show the training dynamics of CNN on MNIST and Fashion-MNIST, and ResNet-18 on CIFAR-10 and CIFAR-100 using noisy sign-SGD with different scaling $\alpha_t$. Legends indicate the choice of $\alpha_t$ and the numbers in brackets are test errors at convergence. As $\alpha_t\to 0$, Nosiy sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original sign-SGD \citep{bernstein2018signsgd}. (e)-(f) show that empirical test error can be bounded by our bound and the corresponding training error. The larger $\alpha_t$ is the sharper our bound is.}
\vspace*{-5mm}
\label{fig:noisy_signsgd}
\end{figure*}



\textbf{Effect of Randomness.} Motivated by \cite{zhang2017understanding}, we train CNN with SGLD on a smaller subset of MNIST dataset ($n=10000$) with randomly corrupted labels. The corruption fraction varies from $0\%$ (without label corruption) to $60\%$. As shown in Figure~\ref{fig:bound_random} (d), for long enough training time, all experiments with different level of label randomness can achieve almost zero training error. However, the one with higher level of randomness has higher generalization/test error (Figure \ref{fig:bound_random} (a) dashed lines). Our generalization bound also becomes larger as the randomness increases since the corresponding gradient discrepancy increases.



\vspace*{-2mm}
\subsection{Noisy Sign-SGD}
\vspace*{-2mm}
%In this section, we present numerical results for Noisy Sign-SGD presented in Example \ref{exam:noisy_signsgd}.  Since none of the existing bounds is derived to handle Bernoulli noisy, we only present our bound here.

\textbf{Optimization.} Figure~\ref{fig:noisy_signsgd} (a)-(d) show the training dynamics of Noisy Sign-SGD under various selections of $\alpha_t$. As $\alpha_t\to 0$, Noisy Sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original Sign-SGD \citep{bernstein2018signsgd}. However, as $\alpha_t$ increases, the probability of getting 1 approaches 0.5, and $\xi_t$ approximates a uniform distribution. As a result, the corresponding Noisy Sign-SGD still converges, but the generalization performance is much worse.

\textbf{Generalization Bound.} Figure \ref{fig:noisy_signsgd}(e)-(f) show that our bound successfully bounds the empirical test error.
%and the corresponding training error. 
The larger $\alpha_t$ is the sharper the upper bound is. However, larger $\alpha_t$ would slow down and adversely affect the optimization, e.g., Figure~\ref{fig:noisy_signsgd} (a)-(d) blue and orange lines. In practice, one needs to balance the optimization error and generalization by choosing a suitable scaling $\alpha_t$.
















% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN, MNIST, SGLD, $\beta_t = 55000$, $\sigma_t\approx 4\times 10^{-4}$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-pretrain.png}
%  } 
% \caption[]{Numerical results for CNN trained on MNIST with pre-training on a prertained dataset $\mathbf{J}_0$ where $|\mathbf{J}_0|=m$. As we increase the pretrain dataset size m, the gradient discrepancy decreases so does our bound.
% }
% \label{fig:mnist_sgld_pretrain}
% \end{figure*}




















%Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to those for CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases, leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence. 

%We note that  \cite{haghifam2020sharpened} show that Negrea et al. bound is smaller than Li et al. in their empirical evaluation, which is opposite to what we observed in Figure \ref{fig:mnist}.We think this is because \cite{haghifam2020sharpened} consider the full-batch setting which has a different form of gradient incoherence compared to the mini-batch setting in our paper. \yzcomment{added the discussion about the inconsistent of our result and \cite{haghifam2020sharpened}}


% The second key difference is the order of dependence on the sample size $n$, i.e., both of our bound and $\cite{Li2020On}$ has a bound of order $\frac{1}{n}$, however, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$. 
%Figure \ref{fig:mnist} (a) and 
% (b) suggests that the gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors, and the gradient incoherence in \cite{negrea2019information} is much smaller than the gradient discrepancy in our bound as well.
% However, the results in (b-d) for MNIST and (f-h) for Fashion MNIST show that our bounds are much sharper than those of \cite{negrea2019information} due to improving the dependence on $n$ from a order of $\frac{1}{\sqrt{n}}$ to $\frac{1}{n}$. Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence.


%More details of our model architectures and addtional experimental results can be found in Appendix. We acknowledge that we did not aim to achieve the state-of-the art predictive performance. With further tuning, the prediction results could be improved








% \begin{figure*}[t] 
% \centering
% \includegraphics[ width=0.5\textwidth]{ICLR2022/images/vgg5-mnist-n1000-bs100-BernoulliSGD-train-dynamics.png}
% \caption[]{Training dynamics of Noisy SignSGD with Bernoulli noise with various selection of $\alpha$ for VGG5 trained on MNIST.When $\alpha \to 0$, Bernoulli SignSGD reduces to SignSGD. As a results, Bernoulli SignSGD with small enough $\alpha$ matches the training trajectory of SignSGD.
% } 
% \label{fig:mnist}
% \end{figure*}

% \textbf{To Do List}

% The following experiments follow the setting described in  \cite{negrea2019information}. \textbf{[By the end of this week (September 19)]}
% \begin{enumerate}
%     \item CNN (two convolutional layers + two fully connected layers) on MNIST and Fashion MNIST
%     \item CNN (two convolutional layers + three fully connected layers) on CIFAR-10
% \end{enumerate}

% The following experiments follow the standard setting most DL papers likely to perform. \textbf{[Before next Wednesday (September 22)]}
% \begin{enumerate}
%     \item VGG5 on MNIST and Fashion MNIST
%     \item ResNet-18 on CIFAR-10 and CIFAR-100
% \end{enumerate}



% \textbf{To Plot}
% \begin{enumerate}
%     \item Gradient norms \citep{Li2020On}
%     \item Gradient incoherence \citep{negrea2019information}
%     \item Gradient discrepancy $\| \mathbf{\theta}_{B,\alpha} - \mathbf{\theta}_{B',\alpha} \|_2^2$ (our bound)
%     \item Our bound, Negrea's bound, and Li et al., bound.
% \end{enumerate}

% \newpage

% \begin{table}
%   \caption{Summary of Experiments for SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $\beta_t$ & Our bound & Li bound & Negrea Bound \\
%     \midrule
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.96 & 55000 & $\checkmark$ & $\checkmark$ & $\checkmark$   \\
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.96 & 5000 & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
%     CNN-1 & Fashion  & $4\times 10^{-3}$ & 0.93 & 55000 & $\checkmark$ & $\checkmark$ & $\checkmark$  \\
%     CNN-1 & Fashion & $4\times 10^{-3}$ & 0.93 & 5000 & $\checkmark$ & $\checkmark$ &$\checkmark$  \\
%     \midrule
%     CNN-2 & CIFAR-10  & $5\times 10^{-3}$ & 0.95 & 55000 &  &  &   \\
%     CNN-2 & CIFAR-10  & $5\times 10^{-3}$ & 0.95 & 5000 &  &  &  \\
%   \midrule
%   ResNet-18/50 & Mini ImageNet & ? & ?&? & & &\\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for Noisy SGD with Gaussian Noise ($\sigma_t=c\eta_t$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $c$ & Our bound & Li bound & Negrea Bound \\
%     \midrule
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.995 & 0.002 &$\checkmark$  & $\checkmark$ &   \\
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.95 & 0.2 &$\checkmark$  &$\checkmark$  &  \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$) with pretrain ($|J_0|=m$)}
%   \label{tab:sgld_pretrain}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & m &$\eta_0$& decay & $\beta_t$ & Our bound\\
%     \midrule
%     CNN-1 & MNIST  & 100 & $4\times 10^{-3}$ & 0.96 & 55000 &   \\
%     CNN-1 & MNIST  & 1000 & $4\times 10^{-3}$ & 0.96 & 55000 &   \\
%     CNN-1 & MNIST  & 10000 & $4\times 10^{-3}$ & 0.96 & 55000 &    \\
%     CNN-1 & MNIST  & 50000 & $4\times 10^{-3}$ & 0.96 & 55000 &    \\
%     \midrule
%     CNN-1 & Fashion & 100 & $4\times 10^{-3}$ & 0.93 & 55000 &   \\
%     CNN-1 & Fashion & 1000 & $4\times 10^{-3}$ & 0.93 & 55000 &    \\
%     CNN-1 & Fashion & 10000 & $4\times 10^{-3}$ & 0.93 & 55000 &    \\
%     CNN-1 & Fashion & 50000 & $4\times 10^{-3}$ & 0.93 & 55000 &   \\
%     \bottomrule
%   \end{tabular}
% \end{table}



% \begin{table}
%   \caption{Summary of Experiments for Random Labels with SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & Randomness & $\eta_0$& decay & $\beta_t$ & Our bound  \\
%     \midrule
%     CNN-1 & MNIST  &0 &$4\times 10^{-3}$ & 0.96 & 55000 & $\checkmark$  \\
%     CNN-1 & MNIST  &10\% &? & ? & ? & \\
%     CNN-1 & MNIST & 20\% &? & ? & ? & \\
%     CNN-1 & MNIST & 50\% &? & ? & ? & \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for Noisy SGD with Bernoulli Noise ($\mu_{\alpha} = \frac{1}{1+\exp(-\theta/\alpha})$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $\alpha_t$ & Our bound \\
%     \midrule
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-6}$ &   \\
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-2}$ &  \\
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-1}$ &  \\
%     CNN-1 & Fashion  & $10^{-4}$ & 0.1 & $10^{-6}$ &     \\
%     CNN-1 & Fashion & $10^{-4}$ & 0.1 & $10^{-2}$&   \\
%     CNN-1 & Fashion & $10^{-4}$ & 0.1 & $10^{-1}$&   \\
%     \midrule
%     CNN-2 & CIFAR-10  & $10^{-3}$ &0.1  & $10^{-6}$ &   \\
%     CNN-2 & CIFAR-10  & $10^{-3}$ & 0.1 & $10^{-2}$ &  \\
%     CNN-1 & CIFAR-10  & $10^{-3}$ &0.1  & $10^{-1}$ &  \\
%   \midrule
%   ResNet-18/50 & Mini ImageNet & ? & ?&? & \\
%     \bottomrule
%   \end{tabular}
% \end{table}



==> ICLR2022/sec/exp_stability.tex <==

In the setting of statistical learning, there is an instance space $\cZ$, a hypothesis space $\cW$, and a loss function $\ell : \cW \times \cZ \mapsto \R_+$. Let $D$ be an unknown distribution of $\cZ$ and let $S \sim D^n$ be $n$ i.i.d.~draws from $D$. For any specific hypothesis $\w \in \cW$, the population and empirical loss are respectively given by
%\vspace*{-3mm}
%\begin{equation}
$L_D(\w) \triangleq \E_{z \sim D}[\ell(\w,z)]$, and $L_S(\w) \triangleq \frac{1}{n} \sum_{i=1}^n \ell(\w,z_i)$.  
%\vspace*{-3mm}
%\end{equation}
For any distribution $P$ over the hypothesis space, we respectively denote the expected population and empirical loss as
\vspace*{-3mm}
\begin{equation}
L_D(P) \triangleq \E_{z \sim D}\E_{\w \sim P}[\ell(\w,z)]~, \qquad \text{and} \qquad  L_S(P) \triangleq \frac{1}{n} \sum_{i=1}^n \E_{\w \sim P}[\ell(\w,z_i)]~.
\vspace*{-3mm}
\end{equation}
\\Consider a randomized algorithm $A$ which works with $S =\{z_1,\ldots,z_n\} \sim D^n$ and creates a distribution over the hypothesis space $\cW$. For convenience, we will denote the distribution as $A(S)$. The focus of the analysis is to bound the generalization error of $A$ defined as: $\gen(A(S)) \triangleq L_D(A(S)) - L_S(A(S))~.  $
% \begin{align}
% \gen(A(S)) \triangleq L_D(A(S)) - L_S(A(S))~.    
% \end{align} 
We will assume $A$ is permutation invariant, i.e., the ordering of samples in $S$ do not modify $A(S)$, an assumption satisfied by most learning algorithms. We will focus on developing bounds for the expectation $\E_S[L_D(A(S)) - L_S(A(S))]$, and discuss high-probability bounds in the Appendix~\ref{sec:app_exp_stability}.
%\abcomment{mention that $A$ is assumed to be permutation invariant}




\subsection{Bounds based on Expected Stability}
% For our analysis, we assume that the $L_2$ norm of the loss is bounded:
% \begin{asmp}
% Let $c_{\ell_2}(z) = \E_{w \sim  p_{A(S)}}[\ell^2(w,z)]$. Two options:
% \begin{enumerate}
% \item Uniform bound: $\forall z$, $c_{\ell_2}(z) \leq c_0$.
% \item Expectation bound: $\E_{z \sim D}[c_{\ell_2}(z)] \leq c_0$ \abedit{and $\E_{z \sim S}[c_{\ell_2}(z)] \leq c_0$}.
% \end{enumerate}
% The analysis would look different depending on which one we choose. \abcomment{Discuss}
% \end{asmp}
% \abcomment{need a discussion on assumptions for info-theoretic analysis}

We start our analysis by noting that the expected generalization error can be upper bounded by {\em expected stability} based on the Hellinger divergence~\citep{save16,Li2020On}: $H^2(P\| P') = \frac{1}{2}\int_{\w} (\sqrt{p(\w)} - \sqrt{p'(\w)})^2 d\w$.
\begin{restatable}{prop}{prophell}
Let $S_n \sim D^n$ and let $S'_{n}$ be a dataset obtained by replacing $z_n \in S_n$ with $z'_n \sim D$. Let $A(S_n),A(S'_{n})$ respectively denote the distributions over the hypothesis space $\cW$ obtained by running randomized algorithm $A$ on $S_n,S'_{n}$.
Assume that for $S_n \sim D^n, \forall z \in \cZ$, $\E_{W \sim  A(S_n)}[\ell^2(W,z)] \leq c_0/2, c_0>0$. %Then, 
With $H(\cdot,\cdot)$ denoting the Hellinger divergence, we have
\begin{equation}
| \E_{S_n \sim D^n}[L_D(A(S_n)) - L_S(A(S_n))] | \leq c_0 \E_{S_n \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S_n), A(S'_{n})\big)}~. 
\end{equation}
\vspace*{-3mm}
\label{prop:hell}
\end{restatable}
\begin{remark}
Proposition~\ref{prop:hell} does not need bounded losses. Just the {\em second moment} of $\ell(W,z), W \sim A(S_n), S_n \sim D^n, \forall z\in \cZ$ need to be bounded. The assumption is satisfied by bounded losses. It is instructive to compare the assumption to that in recent information theoretic bounds~\citep{haghifam2020sharpened,xu2017information}, where one assumes $\ell(\w,Z), Z \sim D, \forall \w \in \cW$ to be {\em sub-Gaussian}. 
\end{remark}
\begin{remark}
The bound in Proposition~\ref{prop:hell} is in terms of {\em expected stability} where we consider $\E_{S \sim D^n} \E_{z'_n \sim D}[\cdots]$, an important departure from bounds based on {\em uniform stability} \citep{elisseeff2005stability, bousquet2002stability, mou2018generalization,bousquet2020sharper, feldman2018generalization,feldman2019high} where one considers $\sup_{S,S' \in \cZ^n, |S \setminus S'| = 1}[\cdots]$. Replacing $\sup$ by $\E$ makes the bounds distribution dependent, and arguably leads to quantitatively tighter bounds. 
\end{remark}
Note that the Hellinger divergence can be bounded by the KL divergence. %so we focus on bounding the KL divergence in the sequel. 
\begin{restatable}{prop}{prophellkl}
For any distributions $P$ and $P'$,
% \vspace*{-2mm}
% \begin{equation}
$2 H^2(P,P') \leq \min \big\{ KL(P,P'),\sqrt{\frac{1}{2}KL(P,P')} \big\}$.
% \end{equation}
\vspace*{-6mm}
\label{prop:hellkl}
\end{restatable}





\subsection{Expected Stability of Noisy Stochastic Iterative Algorithms}
\label{sec: exp_stab_nsi}

We consider a general family of noisy stochastic iterative (NSI) algorithms. Given $S \sim D^n$, such iterative algorithms have two additional sources of randomness in each iteration $t$: (a) a stochastic mini-batch of samples $S_{B_t}$, with $|S_{B_t}| = b$, drawn uniformly at random with replacement from $S$; and (b) noise $\bxi_t$ suitably included in the iterative update. Given a trajectory of past iterates $W_{0:(t-1)} = \w_{0:(t-1)}$, the new iterate $W_t$ is drawn from a distribution $P_{B_t,\bxi_t|\w_{0:(t-1)}}$ over $\cW$:
\begin{align}
W_{t} \sim P_{B_t,\bxi_t|\w_{0:(t-1)}}(W) ~.
%= f_t(B_t,\bxi_t,\w_{0:(t-1)})~,
\label{eq:nmia}
\end{align}
%for some suitable function $f_t$. 
We will drop the conditioning $\w_{0:(t-1)}$ to avoid clutter in the sequel.
%and represent the distribution as $P_{B_t}(\bxi_t)$ in the sequel.
% \abdelete{Since our analysis is based on KL-divergence, we assume that the distributions $P_{B_t,\bxi_t}$ are absolutely continuous with respect to each other. \abcomment{need to be more precise}}
%
% \abdelete{From Propositions~\ref{prop:hell} and \ref{prop:hellkl}, to get a bound on the expected generalization of such NSI algorithms, it suffices to focus on the KL-divergence between $A(S)$ and $A(S'_{n})$. }
Let $P_T, P'_T$ denote the marginal distributions over hypotheses $\w \in \cW$ after $T$ steps of the algorithm based on $S_n,S'_{n}$ respectively. 
% \abdelete{i.e., $P_T = A(S)$ and $P'_T = A(S'_{(n)})$.} 
Further, let $P_{0:(t-1)}$ denote the joint distribution over $W_{0:(t-1)} = (W_0,\ldots,W_{t-1})$, and 
let $P_{t|} \equiv P_{B_t,\bxi_t|\w_{0:(t-1)}}$ compactly denote the conditional distribution on $W_t$ conditioned on the trajectory $W_{0:(t-1)} = \w_{0:t-1}$. Following \citep{negrea2019information,haghifam2020sharpened,pensia2018generalization}, we use the following chain rule for KL-divergence:
%which has been effectively used in recent advances in information theoretic bounds for generalization~:
% \vspace*{-4mm}
% \begin{equation}
$KL(P_T \| P'_T) \leq KL(P_{0:T} \| P'_{0:T} ) = \sum_{t=1}^T \E_{P_{0:(t-1)}}[ KL(P_{t|} \| P'_{t|}) ]$.
% \label{eq:klchain}
% \vspace*{-2mm}
% \end{equation}
Let $\bar{S} \sim D^{n+1}$, and let $S_n,S'_{n}$ be size $n$ subsets of $\bar{S}$ such that $S_n=\{Z_1,\ldots,Z_{n-1},Z_n\}$ and $S'_{n} = \{Z_1,\ldots,Z_{n-1},Z'_n\}$, where $Z'_n = Z_{n+1}$. Let $S_0 = \{Z_1,\ldots,Z_{n-1}\}$. The algorithms we consider use a mini-batch of size $b$ in each iteration uniformly sampled from $n$ samples. Let the set of all mini-batch index sets be denoted by $G$. Let the set of all mini-batch index sets $A$ drawn from $S_0$ be denoted by $G_0$. Note that $|G_0| = \binom{n-1}{b}$. Let $G_1$ denote the set of all mini-batch index sets $B$ which includes the last sample, viz.~$z_n$ for $S$ with mini-batches and $z'_n$ for $S'_n$. 
Note that $|G_1| = \binom{n-1}{b-1}$. Also note that 
$|G_0| + |G_1| = \binom{n-1}{b} + \binom{n-1}{b-1} = \binom{n}{b} = |G|$.
%the total number of $b$-sized mini-batch samples from a dataset of size $n$. \abcomment{The subsets of $S$ and $S'_{(n)}$ corresponding to mini-batch $B$ will be denoted as $S_B$ and $S'_B$.}
% \abdelete{We focus on bounding $KL(P_{t|} \| P'_{t|})$. 
% For for a given $\w_{0:(t-1)}$ and a fixed mini-batch $B_t$, following \eqref{eq:nmia}, let $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively be distributions over $\cW$ corresponding to $S, S'_{n}$. }
% \abbdelete{Then, $P_{t|}$ and $P'_{t|}$ can be viewed as mixture models with shared components~\citep{Li2020On}:
% %due to the randomness in $\bxi_t$. 
% \begin{restatable}{prop}{mixmodel}[\cite{Li2020On}]
% Consider the mixture models 
% %\begin{align*}
% $Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  
% %\end{align*}
% Then, with 
% %\begin{equation*}
% $s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}$,
% %\end{equation*}
% we have 
% \begin{align*}
%     P_{t|} = s Q_{t|} + (1-s) R_{t|}~, \qquad \text{and} \qquad P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~.
% \end{align*}
% \label{prop:mixmodel}
% \vspace*{-6mm}
% \end{restatable}}

% \yzcomment{
% If we are considering $B$ and $B'$ as different mini-batch of \textbf{samples}, and $G_1$ as the set of mini-batches,
% then we should be introduce $G_1^\prime$ for $S_n^\prime$. Because $G_1$ includes sample $z_n$ and $G_1^\prime$ includes$z_n^\prime$.  $G_1$ and $G_1^\prime$ are different sets of different mini-batches. Thus, we cannot use $G_1$ for both $S_n$ and $S_n^\prime$. But I \textbf{don’t} recommend doing this.}

% \yzcomment{Instead, we can consider $G_1$ and $G_0$ as sets of sample indexes, which is the setting  in DP and Li et al paper. In this case, $B$ and $B^\prime$ are the same indexes, but $S_B$ and $S_{B^\prime}$ are different mini-batches only differing in $z_n$ and $z_n^\prime$. }


%\subsection{Bounds with Le Cam Style Divergence (LSD)}
%The mixture model structure in $P_{t|}, P'_{t|}$ can be utilized to 


Following \cite{Li2020On}, we can bound their conditional KL-divergences $KL(P_{t|} \| P'_{t|})$ 
%in the right-hand-side of \eqref{eq:klchain} 
in terms of a Le Cam Style Divergence (LSD). While the classical Le Cam divergence~\citep{save16} is $LCD(P\|P') \triangleq \frac{1}{2} \int \frac{(dP - dP')^2}{dP + dP'}$ (where $dP$ denotes the density), our bounds in terms of  $LSD(P_{t|}| \| P'_{t|}) \triangleq \int \frac{(dP_{B_t,\bxi_t} - dP'_{B_t,\bxi_t})^2}{dP_{A_t,\bxi_t}}, B_t \in G_1, A_t \in G_0$. Note that $P_{B_t,\bxi_t}$ and $P'_{B_t,\bxi_t}$ represent the distribution of $W_t$ for $S_n$ and $S_n^\prime$ respectively since the mini-batch $S_{B_t}$ of $S_n$ and $S_n^\prime$ differs in the $n$-th sample. 
%Putting Propositions~\ref{prop:hell} and \ref{prop:hellkl}, and \eqref{eq:klchain} together, with some additional analysis 
Putting everything together, we have the following LSD based bound.
\begin{restatable}{lemm}{theostab}
Consider a noisy stochastic iterative algorithms of the form~\eqref{eq:nmia} with mini-batch size $b \leq n/2$. Then, with $c_1 = \sqrt{2} c_0$ (with $c_0$ as in Proposition~\ref{prop:hell}), we have
%\vspace*{-1mm}
\begin{equation}
\hspace*{-5mm}
| \E_{S_n}[L_D(A(S_n)) - L_{S_n}(A(S_n))] | \leq c_1 \frac{b}{n} \E_{S_n} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \underset{B_t \in G_1}{\E} \underset{A_t \in G_0}{\E} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t \right] }~.
\end{equation}
\label{theo:stab}
\vspace*{-6mm}
\end{restatable}
\begin{remark}
\cite{Li2020On} essentially has this result for SGLD and inspired our work. Our proofs are significantly simpler and, more importantly, illustrates applicability to general noisy iterative algorithms of the form~\eqref{eq:nmia}, not just SGLD with Gaussian noise as in \cite{Li2020On}. 
\end{remark}
\begin{remark}
Note that the bound does not assume the loss to be bounded, depends on expectations over samples $S_n,z'_n$, trajectories $\w_{0:(t-1)}$, and mini-batches $B_t,A_t$.
%and does not depend on any uniform assumptions. 
Further, 
%as an expected stability based bound to generalization error, 
the bound depends on the distribution discrepancy as captured by the expected LSD. 
\end{remark}
\begin{remark}
The bound seems to worsen with $b$, the size of the mini-batch. As we shown in Section~\ref{sec:efld}, the expected LSD term has a $\frac{1}{b^2}$ dependence for the Exponential Family Langevin dynamics (EFLD) models  we introduce, so the leading $b$ is neutralized.
\end{remark}

%Qualitatively, even if we assume that each term in $\sum_t$ is bounded by a constant

%In Sections~\ref{sec:stab_gauss}

%\abcomment{We are still missing an overall bound by combining (4)-(7)}

%The analysis upto this point does not need the distributions to be Gaussian.



==> ICLR2022/sec/intro.tex <==


Recent years have seen renewed interest and advances in characterizing generalization performance of learning algorithms in terms of stability, which considers change in performance of a learning algorithm based on change of a single training point \citep{hardt2016train,bousquet2002stability,Li2020On,mou2018generalization}. For stochastic gradient descent (SGD), \cite{hardt2016train} established generalization bounds based on uniform stability \citep{hardt2016train,bousquet2002stability}, although the analysis needed rather small step sizes $\eta_t = 1/t$ which is not useful in practice. While improving the analysis for SGD has remained a challenge, advances have been made on noisy SGD algorithms, especially stochastic gradient Langevin dynamics (SGLD) \citep{WellingT11, mou2018generalization,Li2020On}, which adds Gaussian noise to the stochastic gradients of marginal variance $\sigma_t^2$. In parallel, there has been key developments on related information-theoretic generalization bounds applicable to SGLD type algorithms \citep{negrea2019information,haghifam2020sharpened,xu2017information,russo2016controlling, pensia2018generalization}.

While these developments have led to major advances in analyzing generalization of noisy SGD algorithms, they each have certain limitations which leave room for further improvements. Using uniform stability, \cite{mou2018generalization} established a bound for SGLD of the form $\frac{K}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ which depends on $K$, the global Lipschitz constant for the loss, and with step size $\eta_t \leq {\sigma_t \ln 2}/{K}$. The bound has a desirable dependency of $O({1}/{n})$ on the samples, but has an undesirable dependence on $K$, and the step sizes, bounded by ${\sigma_t}/{K}$, are too small. \cite{mou2018generalization} also presented another bound which addresses some of these issues, but gets an undesirable $O({1}/{\sqrt{n}})$ sample dependence.  By building on the developments of \cite{russo2016controlling,xu2017information,pensia2018generalization}, \cite{negrea2019information} made advances from the information theoretic perspective and established bounds for SGLD which have the desirable dependence on the norm of gradient incoherence, i.e., difference in gradients over different mini-batches, avoids dependence on Lipschitz constant $K$, and is applicable to unbounded sub-Gaussian losses, but have an undesirable $O({1}/{\sqrt{n}})$ sample dependence. \cite{haghifam2020sharpened} made further advances on the problem from an information theoretic perspective based on the conditional mutual information framework of~\cite{steinke2020reasoning} and obtained generalization bounds based on gradient incoherence with $O({1}/{n})$ sample dependence, but their analysis holds for full batch Langevin dynamics, not mini-batch SGLD. \cite{Li2020On} made advances on such bounds based on the notion of Bayes-stability, by combining ideas from PAC-Bayes bounds into stability, and established a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \mathbf{g}_e(t)/\sigma_t^2}$ for bounded losses, where $\mathbf{g}_e(t)$ is the expected gradient norm square at step $t$. While the bound avoids dependency on the Lipschitz constant $K$, the dependence on the gradient norm makes such bounds much weaker than the information theoretic bounds of \cite{negrea2019information,haghifam2020sharpened} which depend on the norm of gradient incoherence, which are typically orders of magnitude smaller. Further, the analysis of \cite{Li2020On} still needs small step sizes, bounded by ${\sigma_t}/{K}$. 


In this paper, we build on the core strengths of such existing approaches, most notably the $O({1}/{n})$ sample dependence of stability based bounds~\citep{mou2018generalization,Li2020On} and the dependence on gradient incoherence for information theoretic bounds~\citep{negrea2019information,haghifam2020sharpened}, 
and develop a framework (Section~\ref{sec:exp_stability}) for developing generalization bounds for noisy stochastic iterative (NSI) algorithms. 
Our framework considers generalization based on the concept of {\em expected stability}, rather than uniform stability \citep{hardt2016train,bousquet2002stability, bousquet2020sharper,mou2018generalization}, which yields distribution dependent generalization bounds and avoids the worst-case setting of uniform stability. Building on \cite{Li2020On}, we show that expected stability of general NSI algorithms can be bounded by the expected Le Cam Style Divergence with dependence on parameter distributions from mini-batches differing by one sample. In Section~\ref{sec:efld}, we introduce Exponential Family Langevin Dynamics (EFLD), a family of noisy gradient descent algorithms based on exponential family noise. Special cases of EFLD include SGLD and noisy versions of Sign-SGD or quantized SGD algorithms widely used in practice \citep{bernstein2018signsgd, bernstein2018signsgdnoise, jin2020stochastic, quantized-sgd}% chen2019distributed},. 
Our main result provides an expected stability based generalization bound applicable to any EFLD algorithm with a $O({1}/{n})$ sample dependence and a dependence on gradient incoherence, rather than gradient norms. Existing generalization bounds for SGLD~\citep{Li2020On,negrea2019information} usually use properties of the Gaussian distribution, and our analysis on EFLD illustrates that this was unnecessary. We also consider optimization guarantees for EFLD and establish such results for noisy Sign-SGD and SGLD. Through experiments on benchmark datasets (Section~\ref{sec:exp}), we illustrate that our bounds are non-vacuous and quantitatively much sharper than existing bounds~\citep{Li2020On,negrea2019information}.

{\bf Related work.} Uniform stability has been a classical approach for bounding generalization error \citep{bousquet2002stability,bousquet2020sharper,feldman2018generalization,feldman2019high}, pioneered by \cite{rogers1978finite,devroye1979distribution}. Beyond the aforementioned work, there has been recent work on differential privacy that analyzes the uniform stability of differentially private SGD (DP-SGD)
\citep{hardt2016train, bassily2020stability}. Beyond uniform stability, information-theoretic approaches \citep{russo2016controlling, xu2017information}  that bounds the generalization error by the mutual information between the algorithm input $S$ and the algorithm output $\w$, have been used for deriving generalization bounds for noisy iterative algorithms \citep{pensia2018generalization,bu2019tightening}. Along this line of literature, \cite{negrea2019information, haghifam2020sharpened, rodriguez2021random} 
prove  data-dependent generalization bounds dropping dependence on 
the Lipschitz constant. Further, tighter bounds \citep{haghifam2020sharpened, zhou2021individually, rodriguez2021random, neu2021informationtheoretic, hellstrom2021fast}  are proposed based on conditional mutual information \citep{steinke2020reasoning, grunwald2021pac, hellstrom2020generalization}. Due to space limitations, an extended discussion of the related work is deferred to Appendix~\ref{sec:related_work}. 

% where the generalization error of any learning algorithm can be bounded as $O(\sqrt{I(S; \w)/n})$, where $I(S; \w)$ is the mutual information between the algorithm input $S$ and the algorithm output $\w$. Following this approach,  \cite{pensia2018generalization,bu2019tightening} bound the mutual information for a broad class of iterative algorithms, including SGLD  which obtains a $O(\sqrt{\log T/n})$ generalization bound by choosing $\eta_t = O(1/t)$, where $T$ is the total number of iterations. Subsequent improvements to this technique were made by 
% \cite{negrea2019information, haghifam2020sharpened, rodriguez2021random} 
% to prove data-dependent generalization bounds that do not depend
% on the Lipschitz constant of the loss function and obtain $\sqrt{\sum_t \eta_{t}/n} $ bounds. 
% Especially, \cite{haghifam2020sharpened, zhou2021individually} introduce generalization bounds based on conditional mutual information inspired by \cite{steinke2020reasoning}, leading to tighter bounds than those based on mutual information. Recently, \cite{rodriguez2021random} extend the result of \cite{haghifam2020sharpened} from full-batch gradient to stochastic setting. 
% \cite{neu2021informationtheoretic} extend this information-theoretic approach to derive generalization bound for vanilla SGD. \cite{hellstrom2021fast} provide a fast-rate bound for bounded loss functions based via Conditional Information Measures \citep{grunwald2021pac, hellstrom2020generalization}. 


%\textbf{PAC-Bayesian bound.} 

% \textbf{Noisy iterative algorithms.} Introducing additional noise in the stochastic gradient has been popular in training deep nets. Noisy iterative methods have proven to be useful for machine learning applications, especially for deep neural networks in terms of escaping from saddle points \citep{jin2017escape,jin2019nonconvex}, preserving privacy  \citep{bassily2020stability,wang2019differentially}, boosting generalization and stability \citep{mou2018generalization,Li2020On}. SGLD \citep{WellingT11} has been one of the most popular noisy iterative algorithms for non-convex learning problems, where an isotropic Gaussian noise is added to the stochastic gradient.  As a special case, SGLD can be viewed as a differentially private SGD  algorithm (DP-SGD) \citep{bassily2020stability,wang2019differentially} with constant noise variance. 
% Uniform stability has also been popular in the differential privacy literature for analyzing the generalization error bound of DP-SGD algorithms. Recently, noise has been proven to be useful in Sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise, chen2019distributed} which is proposed to reduce communication cost in distributed learning.  Algorithm such as noisy sign-SGD will first add symmetric
% noises to the stochastic gradient, then take the sign of the noisy stochastic gradient to update the parameters \citep{chen2019distributed, jin2020stochastic}. \cite{bernstein2018signsgdnoise, chen2019distributed, jin2020stochastic} have shown that
% when noise is unimodal and symmetric, sign-SGD can guarantee convergence to stationary point.



% KL-divergence between posterior distribution over hypothesis from training sets differing in one point, relating our analysis to existing information theoretic approaches~\citep{pensia2018generalization,negrea2019information,haghifam2020sharpened}. 

% Building on the developments of \cite{Li2020On}, we show that posterior distribution for general NSI algorithms can be viewed as mixture models, and the KL divergence over posteriors can be bounded by the expectation of Le Cam Style Diveregnces (LSD). For any specific NSI algorithm, the task then reduces to suitable bounding the expected LSD. While our analysis mainly focuses on expected generalization \cite{Li2020On,mou2018generalization,negrea2019information,haghifam2020sharpened}, we show that one get high probability generalization bounds under suitable assumptions. 

% In Section~\ref{sec:stab_gauss}, we apply the expected stability approach to SGLD by suitably bounding the expected LSD  for Gaussian noise. The resulting bound inherits the strengths of the existing bounds with dependence on norms of gradient discrepancy, no dependence on $L$, flexible data dependent choices for $\eta_t,\sigma_t$, and a $O(\frac{1}{n})$ sample dependence. The concept of gradient incoherence in \cite{negrea2019information,haghifam2020sharpened} and our gradient discrepancy are mildly different, but they all qualitatively capture a much more desirable and quantitatively smaller quantity compared to the gradient norm in \cite{Li2020On}. Conceptually, gradient discrepancy norm captures the notion of stability, which the gradient norm does not. The crux of the technical argument in our analysis relies on an approach to bounding the LSD based on an application of mean-value theorem and a careful approach to handle density ratios. We briefly discuss the relationship of our bound for mini-batch SGLD with \cite{mou2018generalization,Li2020On,negrea2019information}, and demonstrate how our bound picks up most of the strengths of each while avoiding the weakness. 

% In Section~\ref{sec:stab_exp_family}, we establish expected stability based generalization bounds for mini-batch stochastic gradient descent with exponential family noise. The result is an important technical extension to existing work on SGLD and, to the best of our knowledge, the first result of its type. The extension also illustrates the power of our framework as we only needed to bound the expected LSD for exponential family noise. The technical argument for bounding the expected LSD for general exponential families are a bit more involved compared to the Gaussian case. As in the case of SGLD with Gaussian noise, the bounds with exponential family noise also depends on the gradient discrepancy, have data dependent flexibly on the choices  of $\eta_t,\sigma_t$, and a $O(\frac{1}{n})$ sample dependence.  

% In Section~\ref{sec:experiment}, we empirically verify the sharpness of our bounds for SGLD in comparison to \cite{Li2020On,negrea2019information} on standard benchmarks (MNIST, Fashion-MNIST) using both multi-layer perceptrons (MLPs) and convolution neural networks (CNNs). For both datasets, both models, and for the entire range of training epochs in each setting, our bounds are shown to be substantially smaller than that of \cite{Li2020On}\cite{negrea2019information}. Interestingly, gradient incoherence of \cite{negrea2019information} is quantitatively smaller than our gradient discrepancy, but our bounds are tighter because of the $O(\frac{1}{n})$ sample dependence compared to $O(\frac{1}{\sqrt{n}})$ of \cite{negrea2019information}. We present additional empirical results and all technical proofs in the Appendix.






==> ICLR2022/sec/related.tex <==

% \begin{itemize}
%     \item Generalization approaches (stability, information-theory bound, PAC Bayesian, Uniform Bound)
%     \item Noisy iterative algorithm (Sign SGD, SGLD, DP SGD etc)
%     \item More?
% \end{itemize}

% \textbf{(Old Materials)}]



\textbf{Uniform stability.} Uniform stability has been a classical approach for bounding generalization error \citep{bousquet2002stability,bousquet2020sharper,feldman2018generalization,feldman2019high}, pioneered by \cite{rogers1978finite,devroye1979distribution}. 
Recently, uniform stability has been shown powerful in analyzing the  stability of SGLD \citep{WellingT11}. \cite{mou2018generalization} prove the uniform stability of SGLD
by showing that the uniform stability can be bounded by the squared Hellinger distance, and further they establish discretized Fokker-Planck equations for analyzing the squared Hellinger distance. Then they provide the uniform stability bound of SGLD as $\frac{L}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ which depends on $L$, the Lipschitz constant for the gradient, and the step size $\eta_t \leq \frac{\sigma_t \ln 2}{L}$ \citep{mou2018generalization,Li2020On}. 
Recently, \cite{Li2020On} follow up on \cite{mou2018generalization} and derive a data-dependent bound using based on Bayes-stability, and got a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \g_e(t)/\sigma_t^2}$, where $\g_e(t)$ is the expected gradient norm square at step $t$. Their bound improves the Lipschitz constant to the expected gradient norm square.  
Recently, \cite{bassily2019private} analyze the uniform stability of  differentially private SGD (DP-SGD) for convex optimization by showing the gradient update is a non-expansive operation, which is the key fact in proving the stability of SGD \citep{hardt2016train}. 
The approach in \cite{hardt2016train} can extend to non-convex setting as well, however it requires fast decaying in step size as $\eta_t = O(1/t)$.  \cite{bassily2020stability} provide stability analysis of SGD for convex and non-smooth functions. 

\textbf{Information-theoretic bound.} Besides the works mentioned above, other theories of deriving generalization bounds for noisy iterative algorithms have been proposed via information-theoretic approaches \citep{russo2016controlling, xu2017information}. Such results show that the generalization error of any learning algorithm can be bounded as $O(\sqrt{I(S; \w)/n})$, where $I(S; \w)$ is the mutual information
between the algorithm input $S$ and the algorithm output $\w$. Thus, recent works following this approach focus on bounding the mutual information for a broad class of iterative algorithms, including SGLD  which obtains a $O(\sqrt{\log T/n})$ generalization bound by choosing $\eta_t = O(1/t)$, where $T$ is the total number of iterations~\citep{pensia2018generalization,bu2019tightening}. Subsequent improvements to this technique were made by 
\cite{negrea2019information, haghifam2020sharpened, rodriguez2021random} 
to prove data-dependent generalization bounds that do not depend
on the Lipschitz constant of the loss function and obtain $\sqrt{\sum_t \eta_{t}/n} $ bounds. 
Especially, \cite{haghifam2020sharpened, zhou2021individually} introduce generalization bounds based on conditional mutual information inspired by \cite{steinke2020reasoning}, leading to tighter bounds than those based on mutual information. Recently, \cite{rodriguez2021random} extend the result of \cite{haghifam2020sharpened} from full-batch gradient to stochastic setting. 
\cite{neu2021informationtheoretic} extend this information-theoretic approach to derive generalization bound for vanilla SGD. \cite{hellstrom2021fast} provide a fast-rate bound for bounded loss functions based via Conditional Information Measures \citep{grunwald2021pac, hellstrom2020generalization}. 


%\textbf{PAC-Bayesian bound.} 

\textbf{Noisy iterative algorithms.} Introducing additional noise in the stochastic gradient has been popular in training deep nets. Noisy iterative methods have proven to be useful for machine learning applications, especially for deep neural networks in terms of escaping from saddle points \citep{jin2017escape,jin2019nonconvex}, preserving privacy  \citep{bassily2020stability,wang2019differentially}, boosting generalization and stability \citep{mou2018generalization,Li2020On}. SGLD \citep{WellingT11} has been one of the most popular noisy iterative algorithms for non-convex learning problems, where an isotropic Gaussian noise is added to the stochastic gradient.  As a special case, SGLD can be viewed as a differentially private SGD  algorithm (DP-SGD) \citep{bassily2020stability,wang2019differentially} with constant noise variance. 
Uniform stability has also been popular in the differential privacy literature for analyzing the generalization error bound of DP-SGD algorithms. Recently, noise has been proven to be useful in Sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise, chen2019distributed} which is proposed to reduce communication cost in distributed learning.  Algorithm such as noisy sign-SGD will first add symmetric
noises to the stochastic gradient, then take the sign of the noisy stochastic gradient to update the parameters \citep{chen2019distributed, jin2020stochastic}. \cite{bernstein2018signsgdnoise, chen2019distributed, jin2020stochastic} have shown that
when noise is unimodal and symmetric, sign-SGD can guarantee convergence to stationary point.







==> ICLR2022/sec/stability.tex <==
From Lemma~\ref{theo:stab}, conditioned on a trajectory $\w_{0:(t-1)}$, mini-batches $S_{B_t}, S_{A_t}$, %\yzcomment{sometimes, we use $S_{B_t}$ as mini-batch, sometimes we use $B_t$ as mini-batch. To be consistent, let’s use $S_{B_t}$ for mini-batch, and ${B_t}$ for indexes} 
we can get generalization bound by suitably bounding the Le Cam Style Divergence (LSD) given by:
$I_{A_t,B_t} = \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t$.
For EFLD, the density functions $dP_{B_t,\bxi_t}$ are exponential family densities $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ as in \eqref{eq:efld1}-\eqref{eq:efld2}, and we have the following bound on the per step LSD:
\begin{restatable}{theo}{theoefld}
For a given set $\bar{S} \sim D^{n+1}$ and $\w_{t-1}$ at iteration $(t-1)$, let $\Delta_{t|\w_{t-1}}(\bar{S}) = \max _{z, z' \in  \bar{S}}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, z'\right)\right\|_{2}~$. Further, for a $c_2$-smooth log-partition function $\psi$, let the scaling $\alpha_{t|\w_{t-1}}$ be data-dependent such that $\alpha_{t|\w_{t-1}}^2 \geq  8 c_2 \Delta_{t|\w_{t-1}}^{2}(S_{n+1})$. Then, we have
%\vspace*{-2mm} 
\begin{align}
I_{A_t, B_t} \leq 5 c_2 \| \btheta_{B_t,\alpha_t} - \btheta_{B'_t,\alpha_t} \|_2^2 = \frac{5c_2}{2\alpha_{t|\w_{t-1}}^2} \left[\left\|\nabla \ell\left(\w_{t-1}, {S_{B_t}}\right)  -  \nabla \ell\left(\w_{t-1}, S'_{B_t}\right)\right\|_{2}^{2}\right]~,
\end{align}
\label{theo:efld}
\vspace*{-5mm}
\end{restatable}
Note that $S_{B_t}$ and  $S'_{B_t}$ only differ at samples $z_n$ and $z'_n$. The above bound can now be directly applied to Lemma~\ref{theo:stab} to get expected stability based generalization bounds for any EFLD algorithm.
\begin{restatable}{theo}{theoefldstab}
Consider an exponential family Langevin dynamics (EFLD) algorithm of the form~\eqref{eq:efld1}-\eqref{eq:efld2} with a $c_2$-smooth log-partition function $\psi$.  Then, for mini-batch size $b \leq n/2$, with $c = c_0 \sqrt{5 c_2}$ (with $c_0$ as in Lemma~\ref{theo:stab}) and $\alpha_{t|}^2 \geq 8 c_2 \Delta_{t|}^2(S_{n+1})$ (as in Theorem~\ref{theo:efld}, with the conditioning on $\w_{t-1}$ hidden to avoid clutter), we have
\vspace*{-2mm}
\begin{equation}
\hspace*{-5mm}
% | \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq  c \frac{b}{n} ~\underset{S_{n+1}}{\E} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \frac{1}{\alpha_{t|}^2} \underset{S_{B_t}, S'_{B_t} \in G_1}{\E} \left[\left\|\nabla \ell\left(\w_{t-1}, B_t\right)  -  \nabla \ell\left(\w_{t-1}, B'_t\right)\right\|_{2}^{2}\right] }~.
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq  c \frac{1}{n} ~\underset{S_{n+1}}{\E} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \frac{1}{\alpha_{t|}^2}  \left[\left\|\nabla \ell\left(\w_{t-1}, {z_n} \right)  -  \nabla \ell\left(\w_{t-1}, {z'_n}\right)\right\|_{2}^{2}\right] }~.
\end{equation}
\label{theo:efldstab}
\vspace*{-5mm}
\end{restatable}
%\yzcomment{Deleted $\underset{{B_t} \in G_1}{\E}$ in the bound.  We don’t need this.}
\begin{remark}
%\yzcomment{needs to be updated, will do} \yzcomment{done}.
Theorem \ref{theo:efldstab} captures the generalization error of SGLD, which is a special case of EFLD.
% Theorem \ref{theo:efldstab} shows that 
% the expected generalization error of EFLD  scales as $O(\sqrt{\sum_{t=1}^T \frac{1}{\alpha_t^2}}/n)$. With the special case $\alpha_t = \sigma_t/\eta_t$, EFLD reduces to SGLD and  Theorem \ref{theo:efldstab} captures the generalization error of SGLD, i.e., $O(\sqrt{\sum_{t=1}^T \frac{\eta_t^2}{\sigma_t^2}}/n)$ 
Our bound has the same dependence on $n$, $T$, step size $\eta_t$ as the bound in \cite{Li2020On}. 
However, our bound is numerically sharper because we replace the \emph{gradient norms}, i.e., $\frac{1}{n}\sum_{z \in S}\|\ell(\w_t,z)\|$ in \cite{Li2020On} and with gradient discrepancy $\|\nabla \ell(\w_t,z) - \nabla \ell(\w_t, z^\prime) \|$, which is quantitatively smaller than gradient norms as we show in the experiment section. The bound in \cite{negrea2019information} depends on \emph{gradient incoherence} which is empirically smaller than gradient discrepancy as observed in the experiment section, their bound depends on ${1}/{\sqrt{n}}$, which is worse than the ${1}/{n}$ dependence in our bound. 
%Thus, our bound in Theorem \ref{theo:efldstab} inherits the strengths of the existing bounds with dependence on norms of gradient discrepancy, and an $O(1/n)$ sample dependence.


% there are two key differences making our bound sharper than existing bounds in \cite{Li2020On} and \cite{negrea2019information}. The first key difference between our result and \cite{Li2020On} is that we replace the \emph{gradient norms}, i.e., $\frac{1}{n}\sum_{z \in S}\|\ell(\w_t,z)\|$ in \cite{Li2020On} and with gradient discrepancy $\|\nabla \ell(\w_t,z) - \nabla \ell(\w_t, z^\prime) \|$, which is quantitatively smaller than gradient norms as we show in the experiment section. 
% The second key difference is the sample dependence compared to  \cite{negrea2019information}.
% Although, \cite{negrea2019information} also derived a generalization error bound depending a factor that is similar to gradient discrepancy, named  \emph{gradient incoherence} in their paper.  
% The difference between gradient discrepancy and gradient incoherence is that, gradient discrepancy is evaluated on $z_n$ from training set and $z_n^\prime$ from a validation set. The gradient incoherence is the difference between gradients on subset of training samples. Although gradient incoherence is empirically smaller as observed in the experiment section, their bound depends on $\frac{1}{\sqrt{n}}$, which is worse than the $\frac{1}{n}$ dependence in our bound. 
% Thus, our bound in Theorem \ref{theo:efldstab} inherits the strengths of the existing bounds with dependence on norms of gradient discrepancy, and an $O(1/n)$ sample dependence.

%  Note that $B_t$ and $B'_t$ have $(b-1)$ samples $B_{t,0}$ and $B'_{t,0}$ respectively from $G_0$ and and the one sample $z_n$ and $z'_n$ respectively which is unique. Since $B_{t,0}$ and $B'_{t,0}$ are both part of the `training set' for the two algorithms working with $S_n$ and $S'_n$, the gradient discrepancy $\nabla \ell(\w_{t-1},B_{t,0}) - \nabla \ell(\w_{t-1},B'_{t,0})$ will be quite small, say $\eepsilon_t \approx \mathbf{0}$. Thus, the overall gradient discrepancy 
% $\nabla \ell\left(\w_{t-1}, B_t\right)  -  \nabla \ell\left(\w_{t-1}, B'_t\right) 
% \approx \frac{1}{b} \left[ \eepsilon_t + \left( \nabla \ell(\w_{t-1},z_n) - \nabla \ell(\w_{t-1},z'_n) \right) \right]$. The $1/b$ factor here will effectively neutralize the $b$ in the $b/n$ leading term, so larger mini-batches do not have an adverse effect on the bound  (see Section~\ref{sec:exp}) and we get a $O(1/n)$ rate. 
\end{remark}

\begin{remark}
EFLD can be extended to work with anisotropic noise by using $\btheta_{B_t,\aalpha_t} = \nabla \ell(\w_{t-1},S_{B_t}) \oslash \aalpha_t$ in \eqref{eq:efld2} where $\aalpha_t \in \R^p$ determines different scaling for each dimension and $\oslash$ denotes Hadamard division. Theorems~\ref{theo:efld} and \ref{theo:efldstab} can be extended to such anisotropic noise by using $\aalpha$-scaled norms for the gradient discrepancy, i.e., $\| \g - \g'\|_{2,\aalpha}^2 = \sum_j (g_j - g'_j)^2/\alpha_j^2$. \qed 
\end{remark}

\begin{remark}
The condition on $\alpha_t$ is a data-dependent quantity, which can be computed along the training process. It gives much more benign condition of the step size compared to those in the related work (Mou et al., 2018; Li et al., 2020, Hardt et al. 2016), which require step size being bounded by ${\sigma_{t}}/{L}$. However, the step sizes in Theorem \ref{theo:efldstab} need to be bounded by ${\sigma_{t}}/{\Delta_{t}(\bar{S})}$, which is considerably more relaxed since $\Delta_{t}(\bar{S})$ is much smaller than Lipschitz constant $L$, which is a uniform bound over the whole parameter space. 
%Also Hardt et al. (2016) requires $1/t$ step sizes.
Also, usually one would expect $\Delta_{t}(\bar{S})$ to decrease as training proceeds since the gradients shrink as the loss function being minimized. Thus, the constraint on step size does not require the step sizes to be as small as $\sigma_t/L$.
% \\
% - We have mentioned that $\alpha_t$ is a data-dependent quantity that can be computed in the experiments.  We  numerically verified that the learning rates used in our experiments satisfy the conditions in the theory. 
\end{remark}

\subsection{Proof Sketches of Main Results: Theorems~\ref{theo:efld} and \ref{theo:efldstab}}
%\vspace*{-2mm} 
We focus on Theorem~\ref{theo:efld}. To avoid clutter, we drop the subscript $t$ for the analysis and note that the analysis holds for any step $t$.  When the density $dP_{B,\bxi} = p_{\psi}(\bxi;\btheta_{B,\alpha})$, by mean-value theorem, for each $\bxi$, we have 
%\begin{equation}
$p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) 
= \langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle$,
%\end{equation}
for some $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$ where $\gamma_{\bxi} \in [0,1]$. Then,
{\small
\begin{align*}
I_{A,B} &=  \bigintsss_\bxi \frac{\big( p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) \big)^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber 
%= \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber \\
= \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla_{\tilde{\btheta}_{B,\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2~p_{\psi}^2(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi ~,
\label{eq:expcore}
\end{align*}}
since $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) = \exp(\langle \bxi, \tilde{\btheta}_{B,\alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha})) \pi_0(\bxi)$. 


{\bf Handling Distributional Dependence of $\tilde{\btheta}_B$.}
Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_{B,\alpha}$ since $\tilde{\btheta}_{B,\alpha}$ depends on $\bxi$. So, we first bound the density term depending on $\tilde{\btheta}_{B,\alpha}$ in terms of exponential family densities with parameters $\btheta_{B,\alpha}$ and $\btheta_{B,\alpha}$ using $c_2$-smoothness of $\psi$.
\begin{restatable}{lemm}{exptilde}
For some $\gamma_{\bxi} \in [0,1]$, $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, \tilde{\btheta}_{B, \alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha}) \right]}{ \max\left( \exp\big[\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha}) \big] , \exp\left[\langle \bxi, \btheta_{B', \alpha} \rangle - \psi(\btheta_{B',\alpha}) \right]\right) }
\leq \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right] ~.
\end{align*}
%\vspace*{-3mm}
\label{lemm:exp_step2}
\end{restatable}


{\bf Bounding the Density Ratio.} Next we focus on the density ratio $p^2_{\psi}(\bxi,\tilde{\btheta}_{B,\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$. By Lemma~\ref{lemm:exp_step2}, it suffices to focus on $p^2_{\psi}(\bxi,\btheta_{B,\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$ or the equivalent term for $\btheta_{B',\alpha}$. We show that the density ratio can be bounded by another exponential family with parameters $(2\btheta_{B,\alpha} - \btheta_{A,\alpha})$.
\begin{restatable}{lemm}{expdr}
\vspace*{-3mm}
For any $\bxi$, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B, \alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A,\alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}
\leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha} \rangle - \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha} )\right].
\end{align*}
\label{lemm:exp_step3}
\vspace*{-4mm}
\end{restatable}
The analysis for the term $p^2_{\psi}(\bxi,\btheta_{B',\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$ is exactly the same. 

{\bf Bounding the Integral.} Ignoring multiplicative terms which do not depend on $\bxi$ for the moment, the analysis needs to bound an integral term of the form
%\begin{equation}
$\bigintsss_\bxi \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2 ~p_{\psi}(\bxi;2 \btheta_{B,\alpha} - \btheta_{A,\alpha}) d\bxi$,
%\end{equation}
and a similar term with $p_{\psi}^2(\bxi;2 \btheta_{B',\alpha} - \btheta_{A,\alpha})$. First, note that  $\nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) = \tilde{\m}_{B,\alpha}$, the expectation parameter for $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})$~\cite{wainwright2008graphical,banerjee2005clustering}. The integral, however, is with respect to $p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})$. We handle this discrepancy by using $\bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) = (\bxi - \E[\bxi]) + (\E[\bxi] - \nabla \psi (\bxi; \tilde{\btheta}_{B,\alpha}))$, and decomposing as sum-of-squares. Quadratic form for the first term yields the covariance $\E[(\bxi- \E[\bxi])(\bxi - \E[\bxi])^T] = \nabla^2 \psi(\btheta_{2\btheta_{B,\alpha} - \btheta_{A,\alpha}}) \leq c_2 \I$, by smoothness. The second term depends on the difference of gradients $\nabla \psi ( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\tilde{\btheta}_{B,\alpha})$ which, using smoothness and additional analysis, can be bounded by the norm of $(\btheta_{B,\alpha} - \btheta_{A,\alpha})$. All the pieces can be put together to get the bound in Theorem~\ref{theo:efld}, which when used in Lemma~\ref{theo:stab}
yields Theorem~\ref{theo:efldstab}.








==> ICML2022/app/app_exp.tex <==
\subsection{Datasets} 
We use MNIST \cite{mnist}, Fashion-MNIST \cite{fashion-mnist}, CIFAR-10 \cite{cifar10} and CIFAR-100 \cite{cifar10} in our experiments.


%The MNIST and Fashion MNIST datasets both consist of 60,000 training examples and 10,000 test examples. %To construct the experiments, we randomly sample $10,000$  samples from the original training set of MNIST and Fashion MNIST. 
%Details refer to  Table \ref{tab::network_setup_app}. 

\noindent {\bf MNIST dataset:} 60,000 black and white training images, including handwritten digits 0 to 9. We use a subset of MNIST with $n = 10,000$ data points where 1,000 samples from each class are randomly selected. Each image of size $28 \times 28$ is first re-scaled into [0,1] by dividing each pixel value by 255, then z-scored by subtracting the mean and dividing the standard deviation of the training set.


\noindent {\bf Fashion-MNIST dataset:} 60,000 gray-scale training images and 10,000 test images, including 10 clothing categories such as shirts, dresses, sandals, etc. Each image of size $28 \times 28$ is first re-scaled into [0,1] by dividing each pixel value by 255, then z-scored by subtracting the mean and dividing the standard deviation of the training set. 


\noindent {\bf CIFAR-10/-100 dataset:} 60,000 color images consisting of 10/100 categories, e.g., airplane, cat, dog etc. The training set includes 50,000 images while the test set contains the rest 10,000 images. Each image of size $32 \times 32$ has 3 color channels. We first re-scale each image into [0, 1] by dividing each pixel value by 255, then each image is normalized by subtracting the mean and dividing the standard deviation of the training set for each color channel. We also use \textit{RandomCrop} and \textit{RandomHorizontalFlip} for data augmentation.




\subsection{Network Architectures} 
For experiments on both MNIST and Fashion-MNIST, we use a convolutional neural network with two convolutional layers followed by two fully connected layers with ReLU activations. For experiments use the CIFAR-10 dataset, we consider CNN architecture with two convolutional layers
and three fully connected layers. The detail of each CNN architecture can be found in Table \ref{tab:cnn1} and Table~\ref{tab:cnn2}.

\begin{table}[h]
\caption{CNN architecture for MNIST and Fashion MNIST.}
\centering
\begin{tabular}{cc} 
Layer & Parameters \\
\hline \hline Convolution & 32 filters of $5 \times 5$ \\
Max-Pooling & $2 \times 2$ \\
Convolution & 64 filters of $5 \times 5$\\
Max-Pooling & $2 \times 2$ \\
Fully connected & 1024 units \\
Softmax & 10 units \\
\hline
\end{tabular}
    \label{tab:cnn1}
\end{table}


\begin{table}[h]
\caption{CNN architecture for CIFAR-10.}
\centering
\begin{tabular}{cc} 
Layer & Parameters \\
\hline \hline Convolution & 64 filters of $5 \times 5$ \\
Max-Pooling & $2 \times 2$ \\
Convolution & 192 filters of $5 \times 5$\\
Max-Pooling & $2 \times 2$ \\
Fully connected & 384 units \\
Fully connected & 192 units \\
Softmax & 10 units \\
\hline
\end{tabular}
    \label{tab:cnn2}
\end{table}



% \begin{table}[h]
%   \caption{Neural network and datasets setup.}
% 	\centering
% 	\footnotesize{
% 	%\resizebox{\columnwidth}{!}{%
% 	\begin{tabular}{cccccc}	
% 	\toprule[1pt]
% 	Dataset & Model  & features & classes & Training size  & Test size\\ 	
% 	\toprule[1pt]
% 		MNIST            & CNN \& MLP & 28$\times$ 28 & 10 &  10,000  & 10,000\\
% Fashion MNIST   & CNN \& MLP  &  28$\times$ 28 & 10 &  10,000  & 10,000\\
% 		\toprule[1pt]
% 	\end{tabular}}
% %	}
% 	\label{tab::network_setup_app}
% \end{table}


\subsection{Experimental Setup}  
We are interested in stochastic gradient Langevin dynamics,
whose iterative updates are given by $\w_{t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1}, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right).$ %$\w_{t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1}, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right)$. 
We also denote $\beta_t =2\eta_t/\sigma_t^2$ as the inverse temperature at time t. 
For MNIST and Fashion-MNIST, the initial learning rate is $\eta_0=0.004$ and it decays by 0.96 after every 5 epochs. For CIFAR-10,the initial learning rate is $\eta_0=0.005$ and it decays by 0.995 after every 5 epochs. We use batch size $|B_t| = 100$ for MNIST and Fashion-MNIST, and $|B_t| = 200$ for CIFAR-10. %We also consider SGLD with $\sigma_t=\alpha_t\cdot\eta_t$ can be found in Figure~\ref{fig:mnist_noisysgd} in Appendix \ref{app:exp}. 


Motivated by \cite{zhang2017understanding}, we train CNN with SGLD on a smaller subset of MNIST dataset ($n=10000$) with randomly corrupted labels. The corruption fraction varies from $0\%$ (without label corruption) to $60\%$. For different level of randomness, we use the same training setting with batch size $|B_t|=100$, initial step size $\eta_0 = 0.005$, noise variance $\sigma_t = 0.2 \cdot \eta_t$, and we decay $\eta_t$ by 0.995 for every 30 epochs. 



We are also interested in Noisy Sign-SGD whose iterative updates are given by %$\mathbf{w}_{t}=\mathbf{w}_{t-1}-\eta_{t}\boldsymbol{\xi}_{t}$, where $\boldsymbol{\xi}_{t} \sim \text{Bernoulli} \left(\frac{1}{1+\exp{\left(-\frac{\nabla \ell(w_{t-1},S_{B_{t}})}{\alpha_t}\right)}}\right)$
$\w_{t+1} = \w_{t} - \eta_t \bxi_t$, where $\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(\xi_j)=\frac{\exp(\xi_j \btheta_{B_t,\alpha_t})}{\exp(-\btheta_{B_t,\alpha_t})+\exp(\btheta_{B_t,\alpha_t})}$. The initial learning rate is $\eta_0=10^{-4}$ and it decays by 0.1 after every 30 epochs. We use batch size $|B_t| = 100$ for all benchmarks.




%where $~ \bxi_{t,i} \sim p_{\alpha_t}(\xi) = \frac{1}{\exp((1-\xi)\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)/\alpha_t)+\exp((-1-\xi)\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)/\alpha_t)}~, ~ \xi\in\{-1,+1\}$. 




All experiments minimize cross-entropy loss for a fixed number of epochs and have been run on NVIDIA Tesla K40m GPUs. For CNN, we repeat each experiment 30 times, and for ResNet-18, we repeat 5 times.

\subsection{Evaluation of the bound in Theorem~\ref{theo:efldstab}} 

{\bf Estimation of $c_0$ in Proposition 1.} Something similar to $c_0$ exists in all prior bounds, e.g., see Lemma 1 of \citet{xu2017information}, Theorem 9 in \citet{Li2020On}, etc. If the loss is bounded, then one can get $c_0$, but in general, it is difficult. Empirically, we chose $c_0$ based on maximum observed training loss for our bound as well as baseline approaches. 
%\abcomment{we must have assumed a constant for the other bounds as well -- what was it?}
%\xlcomment{In our experiments, $c_0$ can be estimated based on the network architecture and the dataset. For example, for smallCNN trained on MNIST, we empirically observe that the training losses never exceed 1. As a result, we can assume $c_0=2$ in our bound,  $a_1 =0, a_2=1$ when use Eq. (6) for Negrea's bound, $C=1$ for Li et al.' bound, and $a=0, b=1$ for Rodriguez-Galves' bound.}
% {\bf 2.~How are the constants optimized in the bounds?} We have not tried to optimize the constants in the bounds. As noted in Remark 3.3, the only exponential family specific constant in the bounds is $c_2$, the smoothness constant for the log-partition function. {\bf 3.~How to interpret $\alpha_t$?} $\alpha_t$ measures how noisy the updates are. Large $\alpha_t$ implies more noisy updates which helps the stability but hurt the optimization, i.e., training set error will be large, but training set error will accurately reflect test set error. 

{\bf Computation of $\Delta_t^2( \bar{S}_{n+1} )$ and the expectation over $S_{n+1}$ in Theorem~\ref{theo:efldstab}.}
We start with the uniform analysis. Let $L$ be the Lipschitz constant so $\| \nabla \ell(w,z)\|_2 \leq L$. Then $\Delta_{t|}(\bar{S}_{n+1}) \leq 2L$. So, suffices to have $\alpha_t = 4\sqrt{2} c_2 L$.  This will always work if $L$ is known or ensured using gradient clipping. 
%and such a large value of $\alpha_t$ in fact improves the bound in Theorem 2, since $\alpha_{t|}$ is in the denominator. Please also see the uniform bound in \eqref{eq:fixedbnd} and note that our data dependent bounds are much sharper. 
%

More generally, for any given $\bar{S}_{n+1}$, $\Delta_{t|}(\bar{S}_{n+1})$ can be computed by definition
from Theorem~\ref{theo:efld} by taking the maximum discrepancy over  all $\binom{n+1}{2}$ pairs of points in $\bar{S}_{n+1}$. The argmax for the discrepancy will arguably have $z \in S_n$ and $z'=z_{n+1}$, which simplifies the argmax to just consider $n$ pairs rather than $\binom{n+1}{2}$. We verified and used this simpler calculation for the experiments.  


The expectation over $\bar{S}_{n+1}$ is hard to compute but (re)sampling based estimates can be used. The term entails sampling $\bar{S}_{n+1}$, running the training with $n$ samples $S_n$, using $z_{n+1}$ to compute the discrepancy. 
To get Monte Carlo estimates, the analysis has to be repeated for different $z_{n+1}$ (done in the main paper) or by resampling $(S_n,z_{n+1})$, and computing the average which we show in Figure \ref{fig:batch_size} (a). The estimates are shown to have rather low variance.  
%
\begin{figure}[t]
    \centering
      \subfigure[Estimates of $\Delta_t^2( \bar{S}_{n+1} )$]{\includegraphics[width=0.49\textwidth]{ICML2022/images/smallcnn-mnist-bounds-b-100-beta-5000.0-a-rebuttal.png}}  
      \subfigure[Effect of batch size]{\includegraphics[width=0.49\textwidth]{ICML2022/images/smallcnn-mnist-bounds-beta-5000.0-a-rebuttal-batch-size.png}}
    \vspace{-3mm}
    \caption[]{Results for training CNN using SGLD on MNIST. (a) Estimation of $\Delta_t^2( \bar{S}_{n+1} )$ using re-sampled $(S_n,z_{n+1})$. %by replacing  $z_i$ in the training set with $z_i'$ in the holdout set. 
    The variance of such estimation is small. (b) The gradient discrepancy for different batch sizes. Overall, the differences are not significant. }
    \label{fig:batch_size}
    \vspace{-4mm}
\end{figure}

{\bf Dependence of the bound on batchsize $b$.} Our bound in Theorem~\ref{theo:efldstab} does not have a dependence on $b$, because of what Remark 3.2 shows, i.e., the $1/b$ scale factor neutralizes the leading b term in Lemma 1. The gradient discrepancy term itself may have a mild dependence on $b$, with smaller batch sizes having mildly smaller empirical gradient discrepancy as shown in Figure~\ref{fig:batch_size} (b).

\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:sgld_bound} and \ref{fig:sgld_mnist} for MNIST and Fashion-MNIST with CNN}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & MNIST/ Fashion-MNIST \\\hline
Architecture & CNN with 2 conv. layers and 2 linear layers \\\hline
Batch Size & $100$\\\hline
Learning Rate & $\eta_0=4\times10^{-3}$, decay epochs=5, decay rate=0.96 \\\hline
Inverse Temperature& $\beta \in [5000, 55000]$ \\\hline
Number of Epochs & 50\\\hline
No. of training examples & 55000 \\\hline
Number of Repeated Runs & 30 \\
\hline
\end{tabular}
\label{tab:mnist}
\end{table}


\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:sgld_bound} and \ref{fig:sgld_cifar10} for CIFAR-10 with CNN}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & CIFAR-10\\\hline
Architecture & CNN with 2 conv. layers and 3 linear layers \\\hline
Batch Size & $200$\\\hline
Learning Rate & $\eta_0=5\times10^{-3}$, decay epochs=5, decay rate=0.995 \\\hline
Inverse Temperature& $\beta \in [5000, 55000]$ \\\hline
Number of Epochs & 1000\\\hline
No. of training examples & 55000 \\\hline
Number of Repeated Runs & 20 \\
\hline
\end{tabular}
\label{tab:cifar10}
\end{table}



\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:bound_random} for MNIST with CNN ($\sigma_t = 0.2 \cdot \eta_t$)}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & MNIST\\\hline
Architecture & CNN with 2 conv. layers and 2 linear layers \\\hline
Batch Size & $100$\\\hline
Learning Rate & $\eta_0=5\times10^{-3}$, decay epochs=30, decay rate=0.995 \\\hline
Number of Epochs & 1000\\\hline
No. of training examples & 10000 \\\hline
Number of Repeated Runs & 30 \\
\hline
\end{tabular}
\label{tab:random}
\end{table}





\begin{figure*}[t] 
\centering
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-c.png}
 }
  \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-c.png}
 }
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
\includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-b.png}
 }
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
\includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-b.png}
 }   
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-a.png}
 }
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a.png}
 } 
\caption[]{Numerical results for CNN trained on MNIST using SGLD %($\sigma_t=\sqrt{2\eta_t/\beta_t}$). $\beta=55000$ which is equivalent 
with a small noise variance $\sigma_t\approx 10^{-4}$.
}
\label{fig:sgld_mnist}
\end{figure*}




\begin{figure*}[t] 
\centering
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-c.png}
 }
\subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-c.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-b.png}
 } 
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-b.png}
 }
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-a.png}
 }
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a.png}
 } 

%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-5000.0-b.png}
%  } 
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-55000.0-b.png}
%  }
%   \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a.png}
%  } 
%   \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-a.png}
%  }
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-5000.0-a.png}
%  } 
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-55000.0-a.png}
%  }  
\caption[]{Numerical results for training CNN using SGLD %with $\sigma_t = \sqrt{2\eta_t/\beta_t}$ 
on CIFAR-10. 
}
\label{fig:sgld_cifar10}
\end{figure*}






\begin{figure*}[th] 
\centering
  \subfigure[CNN, MNIST, Noisy-SGD, $\alpha_t = 0.2$, $\sigma_t\approx 10^{-4}$]{
 \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-beta-0.2.png}
 } 
  \subfigure[CNN, MNIST, Noisy-SGD, $\alpha_t = 0.002$, $\sigma_t\approx 10^{-6}$]{
 \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-beta-0.002.png}
 }
\caption[]{Numerical results for CNN trained on MNIST using Noisy SGD. %where $\sigma_t=\alpha_t\eta_t$. 
We follow the setting described in \cite{Li2020On}. The initial $\eta_t$ is $4\times 10^{-3}$, and decays by 0.95 ($\alpha_t=0.2$) or 0.995 ($\alpha_t=0.002$) for every 5 epochs. 
}
\label{fig:mnist_noisysgd}
\end{figure*}




\begin{figure*}[th!] 
\centering
  \subfigure[CNN, MNIST]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/cnn1-mnist-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 } 
  \subfigure[CNN, Fashion]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/cnn1-fashion-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
 \subfigure[ResNet-18, CIFAR10]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/resnet18-cifar10-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
 \subfigure[ResNet-18, CIFAR100]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/resnet18-cifar100-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
\caption[]{Training dynamics of CNN on MNIST and Fashion-MNIST, and ResNet-18 on CIFAR-10 and CIFAR-100 using noisy sign-SGD with different scaling $\alpha_t$. Legends indicate the choice of $\alpha_t$ and the numbers in brackets are test errors at convergence. As $\alpha_t\to 0$, Nosiy sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original sign-SGD \citep{bernstein2018signsgd}.} %(e)-(f) show that empirical test error can be bounded based on our generalization bound and the corresponding training error. The larger $\alpha_t$ (noise) is the sharper our bound is.}
%\vspace*{-3mm}
\label{fig:noisy_signsgd_train}
\end{figure*}



\begin{figure*}[t] 
\centering
 \subfigure[MNIST, $\alpha_t = 1.0$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
 }
 \subfigure[MNIST, $\alpha_t = 0.1$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-d.png}
 }
 \subfigure[MNIST, $\alpha_t = 0.01$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-e.png}
 }
  \subfigure[MNIST, Our Bound]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-b.png}
 }  
 \subfigure[MNIST, Gradient Discrepancy]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-a.png}
 }
 
 \subfigure[Fashion, $\alpha_t = 1.0$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
 }
 \subfigure[Fashion, $\alpha_t = 0.1$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-d.png}
 }
 \subfigure[Fashion, $\alpha_t = 0.01$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-e.png}
 }
  \subfigure[Fashion, Our Bound]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-b.png}
 }  
 \subfigure[Fashion, Gradient Discrepancy]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-a.png}
 }  
 
\caption[]{Numerical results for training CNN on MNIST and Fashion-MNIST using Noisy Sign-SGD. Increasing $\alpha_t$ leads to a tighter generalization bound even though it leads to a slightly larger gradient discrepancy. 
}
\label{fig:bound_noisy_signsgd}
\end{figure*}



% \end{figure*}

% \begin{figure*}[th!] 
% \centering
% \subfigure[MNIST, $\alpha_t=1$]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
%  } 
%   \subfigure[MNIST, $\alpha_t=0.01$]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-e.png}
%  }
%   \subfigure[Fashion, $\alpha_t=1$]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
%  } 
%   \subfigure[Fashion, $\alpha_t=0.01$]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-e.png}
%  }
%\vspace*{-4mm}




% \clearpage
% \textbf{Experiments on Cifar10 dataset.} We run experiments and compare our bound with the bound in \cite{Li2020On} and \cite{negrea2019information} on Cifar10 dataset. We consider vgg 11 network model with 10,000 training samples randomly sampled from Cifar10 dataset. For training we use initial learning rate 0.001, and noise variance decay such that $\sigma_t = 0.3\eta_t$ and $\sigma_t = 0.5\eta_t$, and we decay $\eta_t$ every 10 epochs with decaying rate 0.93. Figure \ref{fig:cifar10} shows our bound is sharper than existing bound under different noise variance settings.
% \begin{figure*}[h] 
% \centering
% %   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
% %  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
% %  } 
% %   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
% %  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
% %  }  
%   \subfigure[$\sigma_t = 0.3 \eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_lr0.001_alpha0.3_mo0.0_decay0.93.png}
%  }  
%   \subfigure[$\sigma_t = 0.5 \eta_t$]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_lr0.001_alpha0.5_mo0.0_decay0.93.png}
%  }

% \caption[]{Numerical results for cifar10 dataset. Figure (a-b) shows our bound is sharper than existing bound under different settings of noise variance.
% }\label{fig:cifar10}
% \end{figure*}






% \textbf{Random Label Experiments.} Inspired by \cite{zhang2017understanding}, we run SGLD to fit 10,000 samples from MNIST dataset Figure \ref{fig:random_label_mnist} and fashionMNSIT dataset Figure \ref{fig:random_label_fashion_mnist}, with increasing fractions of randomly labeled data, from fractions $0\%$ (normal data) to $60\%$. We consider a MLP network with two hidden layers with 128,128 nodes respectively in each layer. For different level of randomly labeled data, we use the same training setting with batch size $|B_t|=128$, initial step size $\eta_0 = 0.05$, noise variance $\sigma_t = 0.07 \cdot \eta_t$, and we decay $\eta_t$ every 10 epochs by 0.95. As shown in Figure~\ref{fig:random_label_mnist} (a) and \ref{fig:random_label_fashion_mnist} (a), with a fixed running time, the experiment with higher level of randomly labeled data has lower training accuracy. Figure \ref{fig:random_label_mnist} (b) and \ref{fig:random_label_fashion_mnist} (b) show higher level of randomly labeled data has higher generalization error and our bound also increase with higher level of randomness, which matches the behavior of generalization error.



==> ICML2022/app/efld.tex <==

%\abcomment{some text}

In this section, we provide the proofs for Section \ref{sec:efld}. We first review and show details of a few examples of exponential family.



\subsection{Examples of Exponential Family}
\label{app:example}

We show that EFLD becomes SGLD when the exponential family is Gaussian, and becomes a noisy version of sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise} when the exponential family is skewed  over $\{-1,+1\}$. 
%
\begin{exam}[Gaussian] 
SGLD uses scaled Gaussian noise with $\psi(\btheta)= \|\btheta\|_2^2/2, \alpha_t = \sigma_t/\eta_t$, %\tcedit{$\bxi = \x/\alpha_t,~\pi_0(\bxi) = \frac{1}{\sqrt{(2\pi)^d}} 
$\ppi_{0,\alpha_t}(\bxi) = \frac{1}{\sqrt{(2\pi)^p \alpha_t^p}} \exp(-\|\bxi\|_2^2/2\alpha_t^2)$ so that $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t}) = \mathcal{N}(\btheta_{B_t}, \alpha_t^2 \I_d)$. 
Then, the distribution from the natural parameter form is:
\begin{equation}
    p_{\btheta/\sigma}(\xi) = \exp( \langle\xi, \btheta\rangle / \sigma^2 - \|\theta\|_2^2/(2\sigma^2) ) \times \frac{1}{\sqrt{2\pi}\sigma} \exp(-\|\xi\|_2^2/2\sigma^2)
    = \frac{1}{\sqrt{2\pi}\sigma} \exp(-\|\bxi-\bmu\|_2^2/2\sigma^2)~.
\end{equation}
The expectation parameter $\bmu = \nabla \psi(\btheta) = \btheta$. The scaled expectation parameter $\bmu_{\alpha} = \nabla \psi(\btheta_\alpha) = \btheta_\alpha = \btheta/\sigma = \bmu/\sigma$. Since $\xi = x/\sigma$ and the Bregman divergence $d_{\phi}(\bxi,\bmu) = \frac{1}{2}\|\bxi-\bmu\|_2^2$, the expectation parameter form
\begin{equation}
p_{\bmu_{\alpha}}(\bxi) = \exp(-\|\bxi/\sigma - \bmu/\sigma\|_2^2/2) \frac{1}{\sqrt{2\pi} \sigma} = \frac{1}{\sqrt{2\pi}\sigma} \exp(-\|\bxi-\bmu\|_2^2/2\sigma^2)~.
\end{equation}
By taking $\rho_t = \eta_t$, the update \eqref{eq:efld1} based on $\rho_t \bxi_t$ is distributed as $\mathcal{N}(\eta_t \btheta_{B_t}, \eta_t^2 \alpha_t^2 \I_d) = \mathcal{N}(\eta_t\nabla \ell(\w_{t-1}, S_{B_t}), \sigma_t^2 \I_d)$. Thus the EFLD update reduces to the SGLD update: $\w_{t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1}, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right).$
\label{exam:sgld}
\qed 
\end{exam}
%
\begin{exam}[Skewed Rademacher]
\label{exam:noisy_signsgd}
%\abcomment{just keep the part showing this is a special case of EFLD}\tccomment{Updated.}
%\begin{align*}
    % p_{\btheta_{B_t,\alpha_t,j}}(\xi) = \exp(x\btheta_{B_t,\alpha_t,j} - \log(\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j}))) = \frac{\exp(x\btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})}.
%\end{align*}
For skewed Rademacher over $\{-1,1\}$, the sufficient statistic $\xi = x \in \{-1,1\}$, base measure is 1 on $\{-1,1\}$, and the log-partition function $\psi(\theta) = \log(\exp(-\theta)+\exp(\theta))$ for natural parameter $\theta \in \R$. The expectation parameter $\mu = \nabla \psi(\theta) = \frac{\exp(\theta)- \exp(-\theta)}{\exp(-\theta)+\exp(\theta)} = \frac{\exp(2\theta)-1}{\exp(2\theta)+1}$, then its inverse function $\theta = \nabla \phi(\mu) = \frac{1}{2}\log \left(\frac{1+\mu}{1-\mu}\right)$, by integration we have $\phi(\mu) = \frac{1+\mu}{2}\log\frac{1+\mu}{2}+ \frac{1-\mu}{2}\log\frac{1-\mu}{2}$. The expectation parameter $\mu = \nabla \psi(\theta) = \frac{\exp(\theta)}{1+\exp(\theta)} = \frac{1}{1+\exp(-\theta)}$, the sigmoid function of $\theta$. The Bregman divergence is the Bernoulli KL-divergence given by: $d_{\phi}(\xi,\mu) = \xi \log \frac{\xi}{\mu} + (1-\xi) \log \frac{1-\xi}{1-\mu}$. 
For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{1}{1+\exp(-\theta_{\alpha})}$. 
The mean parameter form distribution is given by
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha})) = \mu_{\alpha}^{\xi} (1-\mu_{\alpha})^{1-\xi}~.
\end{equation}
Noisy Sign-SGD takes $\rho_t = \eta_t$ and componentwise $\xi_j \in\{-1,1\},~\pi_{0,\alpha_t}(\xi_j)=1,~\psi(\theta) = \log(\exp(-\theta)+\exp(\theta))$ in exponential family update equation \eqref{eq:efld1}, the $j$-th component of exponential family distribution $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ becomes
$p_{\psi}(\xi_j; \btheta_{B_t,\alpha_t,j})  = \frac{\exp(\xi_j \btheta_{B_t,\alpha_t,j})}{\exp(-\theta_{B_t,\alpha_t,j})+\exp(\theta_{B_t,\alpha_t,j})}$.
Thus, the EFLD update reduces to a noisy version of Sign-SGD: 
$\w_{t} = \w_{t-1} - \eta_t \bxi_t$, $\xi_{t,j} \sim p_{\psi}(\xi_j,\theta_{B_t,\alpha_t,j})$, 
% \begin{equation}\label{eq:signSGD_mini_batch_1}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, ~\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(x) =  \frac{\exp(x \btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})},~ x\in\{-1,+1\}
% \end{equation}
$j\in [p]$, where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
% for mini-batch $B_t$ and scaling $\alpha_t$, mini-batch noisy sign-SGD updates the parameters as
% \begin{equation}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim p_{\alpha_t}(\xi) =  \left(\frac{1}{0.5+\exp(-\theta_{B_t,\alpha_t})}\right)^{\frac{1+\xi}{2}} \left(\frac{1-\mu_\alpha}{2}\right)^{\frac{1-\xi}{2}}   ~, ~ \forall i\in [d],
% \end{equation}
\qed
\end{exam}

\begin{exam}[Bernoulli over $\{0,1\}$]
For Bernoulli over $\{0,1\}$, the sufficient statistic $\xi = x \in \{0,1\}$, base measure is 1 on $\{0,1\}$, and the log-partition function $\psi(\theta) = \log(1+\exp(\theta))$ for natural parameter $\theta \in \R$. 
The expectation parameter $\mu = \nabla \psi(\theta) = \frac{exp(\theta)}{1+\exp(\theta)} = \frac{1}{1+\exp(-\theta)}$, the sigmoid function of $\theta$. The Bregman divergence is the Bernoulli KL-divergence given by: $d_{\phi}(\xi,\mu) = x \log \frac{x}{\mu} + (1-x) \log \frac{1-x}{1-\mu}$. For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{1}{1+\exp(-\theta_{\alpha})}$. 
The mean parameter form distribution is given by
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha})) = \mu_{\alpha}^{\xi} (1-\mu_{\alpha})^{1-\xi}~.
\end{equation}
By taking the $j$-th component of exponential family distribution $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ becomes
$p_{\psi}(\xi_j; \theta_{B_t,\alpha_t,j})  = \frac{\exp(\xi_j \theta_{B_t,\alpha_t,j})}{1+\exp(\theta_{B_t,\alpha_t,j})}$.
Thus, the EFLD update reduces to : 
$\w_{t} = \w_{t-1} - \eta_t \bxi_t$, $\xi_{t,j} \sim p_{\psi}(\xi_j,\btheta_{B_t,\alpha_t,j})$, $j\in [p]$, where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
\qed
\end{exam}

% \begin{exam}[Gaussian]
% For univariate Gaussians with fixed variance $\sigma^2$, the scaling $\alpha = \sigma$, the sufficient statistic $\xi = x/\sigma$, the log-partition function  $\psi(\theta) = \theta^2/2$, and the base measure $\pi_0(\xi) = \frac{1}{\sqrt{2\pi}} \exp(-\xi^2/2)$ or equivalently $\pi_0(x) = \frac{1}{\sqrt{2\pi}\sigma} \exp(-x^2/2\sigma^2)$ using $\xi = x/\sigma$ and $d\xi = dx/\sigma$. The scaled parameter $\theta_{\alpha} = \theta_{\sigma} = \theta/\sigma$. 
% Then, the distribution from the natural parameter form is:
% \begin{equation}
%     p_{\theta/\sigma}(x) = \exp( x \theta / \sigma^2 - \theta^2/(2\sigma^2) ) \times \frac{1}{\sqrt{2\pi}\sigma} \exp(-x^2/2\sigma^2)
%     = \frac{1}{\sqrt{2\pi}\sigma} \exp(-(x-\mu)^2/2\sigma^2)~.
% \end{equation}
% The expectation parameter $\mu = \nabla \psi(\theta) = \theta$. The scaled expectation parameter $\mu_{\alpha} = \nabla \psi(\theta_\alpha) = \theta_\alpha = \theta/\sigma = \mu/\sigma$. Since $\xi = x/\sigma$ and the Bregman divergence $d_{\phi}(\xi,\mu) = \frac{1}{2}(\xi-\mu)^2$, the expectation parameter form
% \begin{equation}
% p_{\mu_{\alpha}}(\xi) = \exp(-(x/\sigma - \mu/\sigma )^2/2) \frac{1}{\sqrt{2\pi} \sigma} = \frac{1}{\sqrt{2\pi}\sigma} \exp(-(x-\mu)^2/2\sigma^2)~.\qed
% \end{equation}
% \end{exam}

% \begin{exam}[Bernoulli over $\{0,1\}$]
% For Bernoulli over $\{0,1\}$, the sufficient statistic $\xi = x \in \{0,1\}$, base measure is 1 on $\{0,1\}$, and the log-partition function $\psi(\theta) = \log(1+\exp(\theta))$ for natural parameter $\theta \in \R$. 
% The expectation parameter $\mu = \nabla \psi(\theta) = \frac{exp(\theta)}{1+\exp(\theta)} = \frac{1}{1+\exp(-\theta)}$, the sigmoid function of $\theta$. The Bregman divergence is the Bernoulli KL-divergence given by: $d_{\phi}(\xi,\mu) = x \log \frac{x}{\mu} + (1-x) \log \frac{1-x}{1-\mu}$. For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{1}{1+\exp(-\theta_{\alpha})}$. 
% The mean parameter form distribution is given by
% \begin{equation}
% p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha})) = \mu_{\alpha}^{\xi} (1-\mu_{\alpha})^{1-\xi}~.
% \end{equation}
% \qed
% \end{exam}

% \begin{exam}[Skewed Rademacher over $\{-1,1\}$]
% For skewed Rademacher over $\{-1,1\}$, the sufficient statistic $\xi = x \in \{-1,1\}$, base measure is 1 on $\{-1,1\}$, and the log-partition function $\psi(\theta) = \log(\exp(-\theta)+\exp(\theta))$ for natural parameter $\theta \in \R$. The expectation parameter $\mu = \nabla \psi(\theta) = \frac{\exp(\theta)- \exp(-\theta)}{\exp(-\theta)+\exp(\theta)} = \frac{\exp(2\theta)-1}{\exp(2\theta)+1}$, then its inverse function $\theta = \nabla \phi(\mu) = \frac{1}{2}\log \left(\frac{1+\mu}{1-\mu}\right)$, by integration we have $\phi(\mu) = \frac{1+\mu}{2}\log\frac{1+\mu}{2}+ \frac{1-\mu}{2}\log\frac{1-\mu}{2}$. The Bregman divergence is given by: $d_{\phi}(\xi,\mu) = \frac{1+\xi}{2} \log \frac{1+\xi}{1+\mu} + \frac{1-\xi}{2} \log \frac{1-\xi}{1-\mu}$. For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{\exp(2\theta_\alpha)-1}{\exp(2\theta_\alpha)+1}$. Noting that $\frac{1+\xi}{2} \log \frac{1+\xi}{2} = \frac{1-\xi}{2} \log \frac{1-\xi}{2} = 0$ for the base measure, the distribution is given by
% \begin{equation}
% p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha})) = \left(\frac{1+\mu_\alpha}{2}\right)^{\frac{1+\xi}{2}} \left(\frac{1-\mu_\alpha}{2}\right)^{\frac{1-\xi}{2}},
% \end{equation}
% which is $\xi = 1$ with probability $\frac{1+\mu_\alpha}{2}$ and $\xi = -1$ with probability $\frac{1-\mu_\alpha}{2}$.\qed
% % Therefore, the EFLD update reduces to a noisy version of sign-SGD: \begin{equation}\label{eq:signSGD_mini_batch_1}
% %     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, ~\bxi_{t,i} \sim p_{\btheta_{B_t,\alpha_t,i}}(\xi) =  \frac{1}{\exp((1-\xi)\btheta_{B_t,\alpha_t,i})+\exp((-1-\xi)\btheta_{B_t,\alpha_t,i})}~, ~ \xi\in\{-1,+1\}
% % \end{equation}
% % for any $i\in [d]$, where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
% \end{exam}

% \begin{exam}[Categorical]
% \abcomment{do we have the details for this? otherwise deop}
% The sufficient statistic $\xi = x = \{-1,0,1\}$, base measure is 1 on $\{-1,0,1\}$, natural parameters $\btheta = [\theta_1~~~\theta_2]^T \in \R^2$, and the log-partition function $\psi(\btheta) = \log(1+\exp(\theta_1) + \exp(-\theta_2))$. The expectation parameter $\mu  = \nabla \psi(\btheta) = [\frac{\exp(\theta_1)}{1+\exp(\theta_1) + \exp(-\theta_2)}, \frac{\exp(-\theta_2)}{1+\exp(\theta_1) + \exp(-\theta_2)}]$ \qed
% \end{exam}











\subsection{Proof of Theorem~\ref{theo:efld}}

\theoefld*

To avoid clutter, we drop the subscript $t$ for the analysis and note that the analysis holds for any step $t$.  When the density $dP_{B,\bxi} = \p_{\psi}(\bxi;\btheta_{B,\alpha})$, by mean-value theorem, for each $\bxi$, we have 
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) 
= \langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ~,
\end{equation}
for some $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$ where $\gamma_{\bxi} \in [0,1]$. Then,
\begin{align}
I_{A,B} &=  \bigintsss_\bxi \frac{\big( p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) \big)^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber 
= \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber \\
& = \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla_{\tilde{\btheta}_{B',\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2p_{\psi}^2(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi ~,
\label{eq:expcore}
\end{align}
since $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) = \exp(\langle \bxi, \tilde{\btheta}_{B,\alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha})) \pi_0(\bxi)$. 


\subsubsection{Handling Distributional Dependency of $\tilde{\btheta}_B$}
Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. In this step we focus on bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$. 


\exptilde*

\proof Denoting $\gamma_{\bxi}$ as $\gamma$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
\begin{align*}
\langle \bxi, & \tilde{\btheta}_{B,  \alpha} \rangle  - \psi(\tilde{\btheta}_{B,\alpha}) 
 = \langle \bxi, \gamma \btheta_{B, \alpha} + (1-\gamma) \btheta'_{B,\alpha} \rangle - \psi\left( \gamma \btheta_{B, \alpha} + (1-\gamma) \btheta'_{B, \alpha} \right) \\
& = \gamma \bigg[ \langle \bxi , \btheta_{B,\alpha} \rangle - \psi(\btheta_{B, \alpha}) \bigg]  + (1-\gamma) \bigg[ \langle \bxi , \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \bigg] \\
& ~~~~~~~~~~~~~~~
  + \bigg[ \gamma \psi(\btheta_{B, \alpha} ) + (1-\gamma) \psi(\btheta'_{B,\alpha}) - \psi( \gamma \btheta_{B,\alpha} + (1-\gamma) \btheta'_{B,\alpha} ) \bigg] \\
& \stackrel{(a)}{\leq} \max\bigg( \langle \bxi , \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) , \langle \bxi , \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha} )  \bigg) \\
& ~~~~~~~~~~~~~~~ 
  + \bigg[ \gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha} , \tilde{\btheta}_{B,\alpha}) \bigg]~,
\end{align*}
where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation (See section 3.1.1 in \cite{banerjee2005clustering}):
\begin{align*}
  \gamma \psi(\btheta_{B, \alpha} ) + (1-\gamma) \psi(\btheta'_{B,\alpha}) - \psi( \gamma \btheta_{B,\alpha} + (1-\gamma) \btheta'_{B,\alpha} )  =  \gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha} , \tilde{\btheta}_{B,\alpha})~.
\end{align*}
Now, note that
\begin{align*}
\gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha})  + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha}, \tilde{\btheta}_{B,\alpha})  
& \leq \gamma d_{\psi}(\btheta_{B,\alpha}, \btheta'_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha}, \btheta_{B,\alpha}) \\
%& \stackrel{(a)}{=} \gamma d_{\phi}(\m'_{B,\alpha}, \m_{B,\alpha}) + (1-\gamma) d_{\phi}(\m_{B,\alpha},\m'_{B,\alpha})~\\
& \leq \gamma c_2 \| \btheta'_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 + (1-\gamma) c_2 \| \btheta_{B,\alpha} - \btheta'_{B,\alpha} \|_2^2 \\
& \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2~.
\end{align*}
As a result,
\begin{align*}
& \frac{\exp\left[\langle \bxi, \tilde{\btheta}_{B, \alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha}) \right]}{\max\left( \exp\left[\langle \bxi, \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) \right] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right] \right) }\\
& ~~~~~ \leq\exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right]
\frac{ \exp \left[ \max\bigg( \langle \bxi , \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) , \langle \bxi , \btheta'_{B,\alpha} \rangle - \psi(\btheta'_{B,\alpha})  \bigg) \right] }{ \max\left( \exp\left[\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha}) \right] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right] \right) } \\
& ~~~~~ = \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right]~.
\end{align*}
That completes the proof.\qed 







\subsubsection{Bounding the Density Ratio}



Focusing on density ratio, we have

\expdr*

\proof  Note that
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B,\alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A , \alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}  
& = \exp\left[ \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \rangle - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big) \right] \\
& = \beta_{B,A,\alpha} \exp \left[  \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha} \rangle - \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \right]~,
\end{align*}
where
\begin{align*}
\beta_{B,A,\alpha} & = \exp \left[ \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big) \right] ~.
\end{align*}
Note that
\begin{align*}
\log \beta_{B,A,\alpha} & = \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big)\\
& = - \bigg( \psi(\btheta_{B,\alpha}) - \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \bigg) - \bigg( \psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \bigg) \\
& \stackrel{(a)}{\leq} \bigg\langle \btheta_{B,\alpha} - \btheta_{A,\alpha}, \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \bigg\rangle + \bigg\langle \btheta_{A,\alpha} - \btheta_{B,\alpha}, \nabla \psi( \btheta_{A,\alpha} \bigg\rangle   \\
& = \bigg\langle \btheta_{B,\alpha} - \btheta_{A,\alpha}, \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\btheta_{A,\alpha})  \bigg\rangle  \\
& \stackrel{(b)}{\leq} \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2 \| \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\btheta_{A,\alpha}) \|_2  \\
& \stackrel{(c)}{\leq} c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2 \| (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \btheta_{A,\alpha} \|_2 \\
& = 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2~,
\end{align*}
where (a) follows from the convexity of $\psi$, (b) follows from Cauchy-Schwartz, and (c) follows by smoothness of $\psi$.


As a result, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B,\alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A, \alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}
&\leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \psi( (2\btheta_B - \btheta_A)/\alpha) \right]~.
\end{align*}
That completes the proof.\qed

The analysis for the term involving $\btheta'_B$ is exactly the same. 

% \abcomment{state a Lemma by combining Lemma 2 and Lemma 3?}

% \abbcomment{Lemma will help the reader understand that the base measure scales correctly, and essentially stays unchanged}

Combining Lemma~\ref{lemm:exp_step2} and \ref{lemm:exp_step3}, we have the following result:
\begin{restatable}{lemm}{expcompile}
We have
\begin{equation}
\begin{split}
\frac{p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi;\btheta_{A,\alpha})} 
 & \leq \exp\left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right] \\
 & \phantom{...........} 
\times \max\big( \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B,\alpha} - \btheta_{A,\alpha})~,  \big. \\
& \phantom{........................} \left. 
\exp \left[2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B',\alpha} - \btheta_{A,\alpha}) \right)~.
\end{split}
\end{equation}
\label{corr:expcompile}
\end{restatable}
\proof 


From Lemma \ref{lemm:exp_step2}, we have
\begin{align*}
p_{\psi}^2(\boldsymbol{\xi} ; \tilde{\boldsymbol{\theta}}_{B, \alpha}) & = \exp \left[2\left\langle\boldsymbol{\xi}, \tilde{\boldsymbol{\theta}}_{B, \alpha}\right\rangle-2\psi\left(\tilde{\boldsymbol{\theta}}_{B, \alpha}\right)\right] \\
& \leq \exp \left[c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{B^{\prime}, \alpha}\right\|_{2}^{2}\right] \cdot \max \left(\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right], \exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B^{\prime}, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{B^{\prime}, \alpha}\right)\right]\right)
\end{align*}

Thus,

\begin{align*}
\frac{p_{\psi}^{2}\left(\boldsymbol{\xi} ; \tilde{\boldsymbol{\theta}}_{B, \alpha}\right)}{p_{\psi}\left(\boldsymbol{\xi} ; \boldsymbol{\theta}_{A, \alpha}\right)} \leq \exp \left[2 c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{B^{\prime}, \alpha}\right\|_{2}^{2}\right] \cdot  \frac{\max \left(\exp \left[2\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B, \alpha}\right\rangle-2\psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right], \exp \left[2\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B^{\prime}, \alpha}\right\rangle-2\psi\left(\boldsymbol{\theta}_{B^{\prime}, \alpha}\right)\right]\right)}{\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{A, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{A, \alpha}\right)\right]}
\end{align*}

Based on Lemma \ref{lemm:exp_step3}, we have
\begin{align*}
\frac{\exp \left[\left\langle\boldsymbol{\xi}, 2 \boldsymbol{\theta}_{B, \alpha}\right\rangle-2 \psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right]}{\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{A, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{A, \alpha}\right)\right]} \leq \exp \left[2 c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{A, \alpha}\right\|_{2}^{2}\right] \exp \left[\left\langle\boldsymbol{\xi},\left(2 \boldsymbol{\theta}_{B}-\boldsymbol{\theta}_{A}\right) / \alpha\right\rangle-\psi\left(\left(2 \boldsymbol{\theta}_{B}-\boldsymbol{\theta}_{A}\right) / \alpha\right)\right]
\end{align*}

Combining above inequalities we have
\begin{equation}
\begin{split}
\frac{p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi;\btheta_{A,\alpha})} 
 & \leq \exp\left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right] \\
 & \phantom{...........} 
\times \max\big( \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B,\alpha} - \btheta_{A,\alpha})~,  \big. \\
& \phantom{........................} \left. 
\exp \left[2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B',\alpha} - \btheta_{A,\alpha}) \right)~.
\end{split}
\end{equation}

That completes the proof. \qed


\subsubsection{Bounding the Integral}

Ignoring multiplicative terms which do not depend on $\bxi$ for the moment, the analysis needs to bound an integral term of the form
\begin{equation}
    \bigintsss_\bxi \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2 ~p_{\psi}(\bxi;2 \btheta_{B,\alpha} - \btheta_{A,\alpha}) d\bxi~,
\end{equation}
and a similar term with $p_{\psi}^2(\bxi;2 \btheta_{B',\alpha} - \btheta_{A,\alpha})$. The proof of Theorem~\ref{theo:efld} can be done by suitably bounding the integral.
% \begin{restatable}{lemm}{lemmexpinfo}
% \label{lemm:exp_info}
% Consider Noisy SGD with exponetial family noise such that the log-partition function is  $c_1$-strongly convex and $c_2$-smooth, for a given sample set $\bar S$ and parameters $\w_{t-1}$, let $\Delta_{t}(\bar{S}) \triangleq \max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ be data-dependent and adaptively chosen such that $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq \abedit{c(c_1,c_2)}$, then for any $B_t \in G_1$ and  $A_t \in G_0$,  we have \abcomment{notation and constants need work, result needs to be updated}
% \begin{align}
% I_{A_t, B_t} \leq c_0 c_2^2\frac{\eta_{t}^{2}}{\alpha_t^2} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
% \end{align}
% where $c(c_1,c_2) = \frac{c_1^2}{(3c_2-c_1)c_2(1+c_1)}$.
% \end{restatable} 

{\em Proof of Theorem~\ref{theo:efld}.} From Lemma~\ref{corr:expcompile}, we have
\begin{align*}
&I_{A,B}\leq \bigintsss_\bxi \frac{ \left\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi( \tilde{\btheta}_{B,\alpha}) \right\rangle^2 p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{ p_{\psi}(\bxi;\btheta_{A,\alpha})} d\bxi\\
&\leq  \exp\left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2\right] \\
& ~~~~~~~~~~~~~~~~~~~~\times \max\left(  \exp \left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \right. ~, \\
& ~~~~~~~~~~~~~~~~~~~~~~~~~~~
\left.   \exp \left[ 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B',\alpha}-\btheta_{A,\alpha}) d\bxi \right)~.
\end{align*}
Focusing on the integral in the first term (the analysis for the second term is essentially the same), we have
\begin{align*}
& \bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi; 2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = \bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \big( \bxi - \E[\bxi] \big) - \left(\nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& \leq 2\underbrace{\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \E[\bxi] \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi}_{T_1} \\
& \phantom{\leq} + 2 \underbrace{\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi}_{T_2}~.
\end{align*}
For $T_1$, note that 
\begin{align*}
T_1 & = \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \E[\bxi] \right\rangle^2   \right] \\
& = (\btheta_{B,\alpha} -\btheta_{B',\alpha})^T \E_{\bxi \sim p_{\psi}(2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (\bxi - \E[\bxi]) (\bxi - \E[\bxi])^T \right] (\btheta_{B,\alpha} -\btheta_{B',\alpha})~\\
& = (\btheta_{B,\alpha} -\btheta_{B,\alpha})^T \nabla^2 \psi( 2\btheta_{B,\alpha}-\btheta_{A,\alpha})  (\btheta_{B,\alpha} -\btheta_{B',\alpha}) \\
& \leq c_2 \| \btheta_{B,\alpha} -\btheta_{B,\alpha} \|_2^2~,
\end{align*}
since, by smoothness, the spectral norm of $\nabla^2 \psi$ is bounded by $c_2$. 

For $T_2$, first note that 
\begin{align*}
\E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}[\bxi] = \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) ) ~.
\end{align*}
Hence, with $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta_{B',\alpha}$ for some $\gamma_{\bxi} \in [0,1]$, we have
\begin{align*}
T_2 & = \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha},  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right\rangle^2   \right] \\    
& = \E_{\bxi \sim p_{\psi}(\bxi; 2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha},  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha})  \right\rangle^2   \right]\\
& \leq  \| \btheta_{B,\alpha} -\btheta_{B,\alpha} \|_2^2 ~~~\E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\|  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \right\|_2^2  \right]\\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\|  \tilde{\btheta}_{B,\alpha} - (2\btheta_{B,\alpha} - \btheta_{A,\alpha} ) \right\|_2^2  \right] \\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})} \left[ \big\| \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta_{B',\alpha} - \btheta_{B,\alpha} - (\btheta_{B,\alpha} - \btheta_{A,\alpha}) \big\|_2^2 \right] \\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}
\left[ \big\|  (1-\gamma_{\bxi}) (\btheta_{B',\alpha} - \btheta_{B,\alpha}) - (\btheta_{B,\alpha} - \btheta_{A,\alpha}) \big\|_2^2 \right] \\
& \leq  2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ 
\bigg( \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (1-\gamma_{\bxi})^2  \big\|  \btheta_{B',\alpha} - \btheta_{B,\alpha} \big\|_2^2 \right]\\
&\qquad+  \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})} \left[ \big\|  \btheta_{B,\alpha} - \btheta_{A,\alpha} \big\|_2^2 \right]  \bigg) \\
& = 2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ 
\left( \big\|  \btheta_{B',\alpha} - \btheta_{B,\alpha} \big\|_2^2 \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (1-\gamma_{\bxi})^2   \right]
+   \big\|  \btheta_{B,\alpha} - \btheta_{A,\alpha} \big\|_2^2  \right) \\
& \leq  2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~  \left( \| \btheta_{B,\alpha} -\btheta_{B',\alpha}\|_2^2  + \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right) ~.
\end{align*}
Putting everything back together
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 & p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 ~~\left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
Similarly
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 & p_{\psi}(\bxi;2\btheta_{B',\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 ~~\left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
%Since the bound is the same for both the terms, the $\max$ can be bounded by the right-hand-side.
% \abcomment{please finish the rest, need to check the scaling w.r.t.~$1/\sigma$ once the earlier notation is cleaned up}


Then, plugging into bound on $I_{A,B}$, we have
\begin{align*}
I_{A,B} & \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times 
\exp\left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2\right] \\
& ~~~~~ \times \max\big(  \exp \left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right) \big. ~,\\
& ~~~~~~~~~~~~  \exp \left[ 2 c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \right) \big)~.
%\exp\bigg[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \max\left(  \| \btheta_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 , \| \btheta_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 \right)  \bigg] \\
%& ~~~~~~~~~~ \times c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
Since $\alpha^2 \geq 8 c_2 \Delta^2(S_{n+1})$ where $\Delta(S_{n+1}) = \max_{z,z' \in S_{n+1}} \| \nabla \ell (\w,z) - \nabla \ell (\w,z') \|_2$, recalling that $\btheta_{B,\alpha} = \nabla \ell(\w,B)/\alpha$, we have 
\begin{align*}
2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 & \leq \frac{1}{4}~, ~~~
2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \leq \frac{1}{4} ~, ~~~
2 c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \leq \frac{1}{4} ~.
\end{align*}
As a result, we have 
\begin{align*}
I_{A,B} & \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times \exp\left( \frac{1}{4}\right) \times \exp\left(\frac{1}{4}\right) \times \left( 1 +\frac{1}{4} + \frac{1}{4} \right) \\
& \leq \frac{5c_2}{2 \alpha^2} \| \nabla \ell(\w,S_B) - \nabla \ell(\w,S'_B) \|_2^2~.
\end{align*}
That completes the proof. \qed

% \subsection{Coordinate-wise Scaling $\aalpha$}
% We use bold letter $\aalpha$ to denote the vector $[\alpha_1,\cdots,\alpha_p]^T$ representing different scaling for different coordinates.
% \begin{theo}
%     xxx
% \end{theo}




\subsection{Expected Stability of EFLD}

\theoefldstab*

\proof 
% \abcomment{add a proof -- just use Theorem~\ref{theo:efld} in Lemma~\ref{theo:stab}} 
% \yzcomment{added a proof here}

Based on Lemma \ref{theo:stab}, we have
\begin{equation}
\hspace*{-5mm}
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq c_1 \frac{b}{n} \E_{S} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \underset{B_t \in G_1}{\E} \underset{A_t \in G_0}{\E} \left[ I_{A_t, B_t} \right] }~.
\end{equation}
with $I_{A_t, B_t} = \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t$. 

From Theorem \ref{theo:efld}, we have 
\begin{align*}
I_{A_{t}, B_{t}} & \leq \frac{5 c_{2}}{2 \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\|\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)-\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}^{\prime}\right)\right\|_{2}^{2}\right] \\
& =\frac{5 c_{2}}{2  \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\| \frac{1}{b}  \sum_{z\in S'_{B_t}}\nabla \ell\left(\mathbf{w}_{t-1}, z \right)- \frac{1}{b}  \sum_{z\in S_{B_t}} \nabla \ell\left(\mathbf{w}_{t-1}, z \right)\right\|_{2}^{2}\right]  \\
& =\frac{5 c_{2}}{2 b \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\| \nabla \ell\left(\mathbf{w}_{t-1}, z_n \right)-\nabla \ell\left(\mathbf{w}_{t-1}, z_n^\prime \right)\right\|_{2}^{2}\right]~,
\end{align*}
where the last equation holds because $S_{B_t}$ and $S'_{B_t}$ only differ at $z_n$ and $z_n^\prime$. 

Combining the above two inequalities, we have
\begin{align*}
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq c_1 \frac{b}{n} \E_{S} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \left[\left\| \nabla \ell\left(\mathbf{w}_{t-1}, z_n \right)-\nabla \ell\left(\mathbf{w}_{t-1}, z_n^\prime \right)\right\|_{2}^{2}\right] }~.
\end{align*}
That completes the proof. 
\qed


==> ICML2022/app/exp_stability.tex <==
\prophell*
\proof Let $S_n=\left(z_{1}, \ldots, z_{n}\right)$ and $\tilde S^{\prime}_n=\left(z_{1}^{\prime}, \ldots, z_{n}^{\prime}\right)$ two independent random samples and let $S^{(i)}_n=\left(z_{1}, \ldots, z_{i-1}, z_{i}^{\prime}, z_{i+1}, \ldots, z_{n}\right)$ be the sample that is identical to $S$ except in the $i$-th example where we replace $z_{i}$ with $z_{i}^{\prime}$. Note that $S^{(n)}=S'_n$ where $S'_n$ is the dataset obtained by replacing $z_n \in S_n$ with $z'_n$ as in the Proposition statement. Now, by definition we have
\begin{align*}
& \left| \E_{S_n \sim D^n}[L_D(A(S_n)) - L_S(A(S_n))]\right| \\
& = \left| \E_{S_n \sim D^n}[L_S(A(S_n)) - L_D(A(S_n))]\right| \\
&= \left|\mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \mathbb{E}_{A} \left[\frac{1}{n} \sum_{i=1}^{n}\left(\ell(A(S_n^{(i)}), z_{i}^{\prime})-\ell(A(S_n), z_{i}^{\prime}) \right)\right] \right| \\
& = \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime}  \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_{A} \left[ \ell(A(S_n^{(i)}), z_{i}^{\prime})-\ell(A(S_n), z_{i}^{\prime}) \right]\right|\\
& \overset{(a)}{=} \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n} \left(\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p^{(i)}(\mathbf{w}) d \mathbf{w}-\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p(\mathbf{w}) d \mathbf{w} \right) \right|\\
& = \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) \left( p^{(i)}(\mathbf{w}) - p(\mathbf{w}) \right)d \mathbf{w} \right| \\
& = \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime)\left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)  d \mathbf{w} \right| \\
& \overset{(b)}{\leq} \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n} \left\{\left(\int_{\mathbb{R}^{d}} \ell^2(\mathbf{w} ; z_i^\prime) \left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\} \right|
\end{align*}
where in (a) $p^{(i)}(\w), p(\w)$ are respectively the distributions obtained by $A(S_n^{(i)}),A(S_n)$, and (b) 
follows by Cauchy-Schwartz inequality. Focusing on the first integral, we have: 


% %\yzcomment{We do need $\mathbb{E}_{W \sim A\left(S_{n}\right)}\left[\ell^{2}(W, z)\right] \leq c_{0} / 2$, \textbf{for all} $\forall S_{n} \sim D^{n}, \forall z \in \mathcal{Z} $, it is hard to relax the condition to  $\mathbb{E}_{S_n}\mathbb{E}_{W \sim A\left(S_{n}\right)}\left[\ell^{2}(W, z)\right] \leq c_{0} / 2$. Because:
% \begin{align*}
%     & \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \left\{\left(\int_{\mathbb{R}^{d}} \ell^2(\mathbf{w} ; z_i^\prime) \left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\}
%     \\
% & = \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \left\{\left(\int_{\mathbb{R}^{d}} \ell^2(\mathbf{w} ; z_i^\prime) \left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\} \\
% & = \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} [ U_{+}(S, \tilde S^\prime)^{\frac{1}{2}} ~ U_{-}(S, \tilde S^\prime)^{\frac{1}{2}} ]~,
% \end{align*} 
% where 
% \begin{align*}
%     U_{+}(S, \tilde S^\prime) = \left(\int_{\mathbb{R}^{d}} \ell^2(\mathbf{w} ; z_i^\prime) \left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)
% \end{align*}
% and
% \begin{align*}
%      U_{-}(S, \tilde S^\prime) = \left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)~.
% \end{align*}
% We need the expectation $\mathbb{E}_S \mathbb{E}_{\tilde S^\prime}$ to go with $ U_{-}(S, \tilde S^\prime)^{\frac{1}{2}}$ so that we have the expected Hellinger  divergence:  $\mathbb{E}_S \mathbb{E}_{\tilde S^\prime} U_{-}(S, \tilde S^\prime)^{\frac{1}{2}} = \E_{S \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S), A(S'_{n})\big)}$. Thus, we need to uniformly bound $U_{+}(S, \tilde S^\prime)^{\frac{1}{2}}$.
% }






\begin{align*}
\left(\int_{\mathbb{R}^{d}} \ell^2(\w ; z_i^\prime) \left(\sqrt{p^{(i)}(\w)}+\sqrt{p(\w)}\right)^{2} d \w \right)^{1/2} 
& \leq \left(2 \int_{\mathbb{R}^{d}} \ell^2(\w ; z_i^\prime) p^{(i)}(\w) d\w +  2 \int_{\mathbb{R}^{d}} \ell^2(\w ; z_i^\prime) p(\w) d \w \right)^{1/2} \\
& \leq \left( c_0^2/2 + c_0^2/2 \right)^{1/2} =c_0 ~.
\end{align*}

Hence, by definition of the Hellinger divergence, we have 
\begin{align*}
\E_{S_n \sim D^n}[L_D(A(S_n)) - L_S(A(S_n))]
& \leq   \mathbb{E}_{S_n} \mathbb{E}_{\tilde {S_n}^\prime} \frac{1}{n} \sum_{i=1}^{n}c_0 \sqrt{2H^{2}\left(A(S_n), A(S_n^{(i)})\right)}\\
& \overset{(a)}{=}   \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n}c_0 \sqrt{2H^{2}\left(A(S_n), A(S'_n)\right)}\\
& = c_0 \E_{S_n \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S_n), A(S'_{n})\big)}~,
\end{align*}
where (a) follows since the samples are drawn i.i.d.~and the randomized algorithm $A(\cdot)$ is permutation invariant. That completes the proof. \qed 

% (b): need to double check if we can apply the previous argument that ``for any $z$, the loss $\ell(\w;z)$ has bounded expectation and variance'' because there are dependence between $\ell(\w; z_i^\prime)$ and $p^{(i)}(\w)$. The worst case, we bound it by uniform upper bound $C$ on the loss. (c) is true because $z_i^\prime$ for $i =1,...,n$ are i.i.d., so that we can write it as $z^{\prime}$.
% $p^{\prime}(\mathbf{w})$ is the distribution obtained by $A(S^\prime)$, where $S^\prime$ is the dataset differing on only single sample $z^{\prime}$ with $S$.  

% \abcomment{(a) For the analysis, lets use $| \cdots |$ throughout, (b) pls clean up the $\mu^2 + \sigma^2$ analysis, and use a constant. This part needs work}

% \abcomment{For the last part, change to:}
% \begin{align*}
% & \overset{(b)}{\leq} 2c_0  \mathbb{E}_S \mathbb{E}_{S^\prime} \left[ \frac{1}{n} \sum_{i=1}^{n}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)} \right] \\
% & = 2c_0 \mathbb{E}_S \mathbb{E}_{S'} \mathbb{E}_{z_i^\prime \sim S'}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)}\\
% & \overset{(c)}{=} 2c_0 \mathbb{E}_S \mathbb{E}_{z^{\prime}} \sqrt{D_{H}^{2}\left(p^{\prime}(\mathbf{w}), p(\w)\right)}~.
% \end{align*}

\begin{prop}
%{prop}{prophellkl}
For any distributions $P$ and $P'$,
% \vspace*{-2mm}
% \begin{equation}
$2 H^2(P,P') \leq \min \big\{ KL(P,P'),\sqrt{\frac{1}{2}KL(P,P')} \big\}$. 
% \end{equation}
%\vspace*{-5mm}
\label{prop:hellkl}
\end{prop}
%\prophellkl*
\proof For the first part, note that:
\begin{align*}
KL(P ,P') & = \int \left(\log \frac{p(\w)}{p'(\w)} \right) p(\w) ~d\w \\
& =  2 \int  \left( - \log \sqrt{\frac{p'(\w)}{p(\w)}} \right) p(\w)~ d\w \\
& \overset{(a)}{\geq} 2 \int \left( 1 - \sqrt{\frac{p'(\w)}{p(\w)}} \right) p(\w)~ d\w \\ 
& = 2 \int \left( p(\w) - \sqrt{p(\w) p'(\w)}) \right) ~d\w \\
& = \int \left(p(\w) + p'(\w) - 2 \sqrt{p(\w)p'(\w)} \right) ~d\w \\
& = \int \left(\sqrt{p(\w)} - \sqrt{p'(\w)}\right)^2~ d\w\\
& = 2 H^2(P,P')~,
\end{align*}
where (a) follows since for $z > -1$, $\log (1+z) \leq z$, using $x = 1+z$ and changing signs gives $-\log x \geq 1-x$.

For the second part, note that:
\begin{align*}
2H^2(P,P') & =  \int_\w ( \sqrt{p(\w)} - \sqrt{p'(\w)} )^2 d\w \\
& =  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| \times | \sqrt{p(\w)} - \sqrt{p'(\w)}| ~d\w \\
& \leq  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| \times | \sqrt{p(\w)} + \sqrt{p'(\w)}|~ d\w \\
& =  \int_\w | p(\w) - p'(\w)|~ d\w \\
& =  TV(P,P')~,
\end{align*}
where $TV(P,P')$ denotes the total variation distance \citep{pollard2002user}. Further, from Pinsker's inequality \citep{tsybakov2008introduction}, we have
\begin{align*}
TV(P,P') \leq \sqrt{\frac{1}{2} KL(P,P')}~.
\end{align*}
Combining the two results completes the proof. \qed 


% \subsection{Proofs for Section 2.2}

% \mixmodel*
% \proof The proof follows the argument in the proof of Lemma 21 in \cite{Li2020On}.\qed

\subsection{Proofs for Section \ref{sec: exp_stab_nsi}}

Our first result establishes a bound on the KL-divergence between two component mixture models in terms of the mixing weight of the unique components. Similar results have appeared in \citep{Li2020On, bun2018composable} in related contexts. Our proof is different, simple, and self-contained.
\begin{lemm}\label{lemm:mix_bound}
Let $Q,Q',R$ be any three distributions such that $Q,Q'$ are both absolutely continuous w.r.t.~$R$. Then, for any $s \in (0,1)$
\begin{equation}
KL\left(sQ+(1-s)R ~\big\| ~sQ' + (1-s)R \right) \leq 
\frac{s^2}{1-s}~\int_{\w} \frac{(Q(\w) - Q'(\w))^2}{R(\w)} d\w~ .
%\frac{s^2}{1-s} \lsd( Q - Q', R)~.
\end{equation}
\end{lemm}

\proof Let $U=sQ' + (1-s)R$. Then, with $F(x) = Q(x)-Q'(x)$, we have
\begin{align*}
     KL(sQ+(1-s)R \| sQ' + (1-s)R) & =  KL(U + s(Q - Q')  \| U ) \\
     & = \int (U(x) + sF(x)) \log \left( \frac{U(x) + s F(x)}{U(x)} \right) dx \\
     & = \int (U(x) + sF(x)) \log \left( 1 + \frac{s F(x)}{U(x)} \right) dx \\
     & = \int sF(x) + \frac{s^2 F^2(x)}{2U(x)} -  \frac{s^3 F^3(x)}{6U^2(x)} + \frac{s^4 F^4(x)}{12U^3(x)}  -\cdots dx \\
     & = s^2 \int \frac{F^2(x)}{U(x)}\left(  \frac{1}{2} -  \frac{s F(x)}{6U(x)} + \frac{s^2 F^2(x)}{12U^2(x)} - \cdots \right) dx~,
%     & = \int U(x) \left( \left(1+ \frac{sF(x)}{U(x)} \right) \log \left(1 + \frac{sF(x)}{U(x)} \right) - \frac{sF(x)}{U(x)} \right) dx
\end{align*}
where the first term vanishes since $\int F(x) dx = \int (Q(x) - Q'(x)) dx = 0$. This is the reason the dependency is on $s^2$, not $s$. With $W(x) = s F(x)/U(x)$, noting that $W(x) > -1$, and 
\begin{equation}
    \left( \frac{1}{2} - \frac{W(x)}{6} + \frac{W^2(x)}{12} - \cdots \right) = \frac{(1+W(x))\log(1+W(x)) - W(x)}{W^2(x)} \leq 1~,
\end{equation}
we have
\begin{align*}
   KL(sP+(1-s)R \| sQ + (1-s)R) 
     & = s^2 \int \frac{F^2(x)}{U(x)} \left( \frac{ (1+W(x)) \log (1+W(x)) - W(x)}{W^2(x)} \right) dx \\
     & \leq s^2 \int \frac{F^2(x)}{U(x)} dx~ \\
     & \leq \frac{s^2}{(1-s)} \int \frac{(Q(x) - Q'(x))^2}{R(x)} dx~.
\end{align*}
That completes the proof. \qed


\begin{restatable}{prop}{mixmodel}
Consider the mixture models 
%\begin{align*}
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  
%\end{align*}
Then, with 
%\begin{equation*}
$s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}$,
%\end{equation*}
we have 
\begin{align*}
    P_{t|} = s Q_{t|} + (1-s) R_{t|}~, \qquad \text{and} \qquad P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~.
\end{align*}
\label{prop:mixmodel}
\vspace*{-6mm}
\end{restatable}
\proof The proof follows the argument in the proof of Lemma 21 in \cite{Li2020On}.\qed



\begin{lemm}
Consider a general noisy stochastic iterative algorithm with updates of the form~\eqref{eq:nmia} with mini-batch size $B_t = b$. Then, conditioned on any trajectory $\w_{0:t-1}$, we have
\begin{align}
KL\left(P_{t|} \| P_{t|} \right) \leq  \frac{b^2}{n^2} \frac{n}{n-b} \E_{B_t \in G_1} \E_{A_t \in G_0} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t \right]~.
\end{align}
\label{lemm:lsd}
\vspace*{-6mm}
\end{lemm}

\proof By definition, Proposition \ref{prop:mixmodel}, and Lemma~\ref{lemm:mix_bound} with $s=b/n$, we have 
\begin{align*}
KL\left(P_{t|} \| P'_{t|}\right) & \stackrel{(a)}{\leq} \left(\frac{b}{n} \right)^2 \left(\frac{n}{n-b}\right) \int_{\w} \frac{(Q - Q')^2}{R} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \bigintsss_{\w} \frac{ \left(  \frac{1}{|G_1|} \left[ \sum_{B \in G_1} dP_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right] \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} dP_{A,\bxi}(\w)} d\w \\
 & \stackrel{(b)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}\sum_{B \in G_1}  \frac{ \left(  dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} dP_{A,\bxi}(\w)} d\w \\
 & \stackrel{(c)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}  \sum_{B \in G_1} \left\{ \left(  dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2  \frac{1}{|G_0|}\sum_{A \in G_0} \frac{ 1 }{ dP_{A,\bxi}(\w)} \right\} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \frac{1}{|G_1| |G_0|}  \sum_{B \in G_1} \sum_{A \in G_0}  \bigintsss_{\w} \frac{ \left( dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2 }{ dP_{A,\bxi}(\w)} d\w ~,
\end{align*}
% \yzcomment{In order to make sure (b) holdes, we do need $B = B^\prime$, which should be  defined as mini-batches of indexes. }
where (a) is from Lemma \ref{lemm:mix_bound}, (b)(c) is from Jensen's inequality since function $f(x) = x^2$ is convex and $f(x)=\frac{1}{x}$ is convex on $(0,\infty)$. That completes the proof. \qed

Now we have all the pieces to prove the following result:

\theostab*

\proof  Based on Propositions \ref{prop:hell} and \ref{prop:hellkl}, %and \eqref{eq:klchain}, 
we have
\begin{align*}
\E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))]
& \leq  \sqrt{K L\left(P_{T} \| P_{T}^{\prime}\right)} \leq \sqrt{ \sum_{t=1}^{T} \E_{P_{0:(t-1)}}\left[KL\left(P_{t \mid} \| P_{t \mid}^{\prime}\right)\right]} 
\end{align*}
Applying Lemma \ref{lemm:lsd} to bound $KL\left(P_{t \mid} \| P_{t \mid}^{\prime}\right)$ and noting that $b/(n-b) \leq 1$ for $b \leq n/2$ completes the proof. \qed


\subsection{High Probability Generalization Bounds}
\label{ssec:highp}

%\subsection{High Probability Bounds}

%\yzcomment{strongly suggest moving this section to the appendix}

%\abbcomment{This subsection can be moved to the appendix}

Let $S \sim D^n$ with $S=(Z_1\ldots,Z_n)$ corresponding to the training data. Consider the random variable $Y(S)$, the Scaled (by $n$) Generalization Error (SGE), defined as
\begin{align}
Y(S) \triangleq \sum_{i=1}^n \E_A \big[  \E_{Z \sim D} [\ell(A(S),Z) ] - \ell(A(S),Z_i) \big] = n\big(L_D(A(S)) - L_S(A(S))\big) ~.
\end{align}
%where $A(S)$ is the distribution over $\cW$ due to randomized algorithm $A$ run on $S$.
Theorem~\ref{theo:stab} establishes a bound on $|\frac{1}{n}\E_S[Y(S)]|$. We now focus on establishing a high probability bound on $\frac{1}{n}(Y(S)-\E_S[Y(S)])$. Let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. Further, let $S'_i = (Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, the change in SGE
\begin{equation}
Y(S) - Y(S'_i) = n \big[ \big( L_D(A(S)) - L_D(A(S'_i)) \big) - \big( L_S(A(S)) - L_{S'_i}(A(S'_i) \big) \big]    
\end{equation}
is a symmetric random variable, and is identically distributed for $i=1,\ldots,n$.
% \begin{align}
% Y(S) - Y(S'_i) = \sum_{j=1}^n \E_A \big[ \ell(A(S'_i),Z_j) - \ell(A(S),Z_j) \big] = n \big(L_{S'_i}(A(S'_i) - L_S(A(S)) \big)
% \end{align}
%Note that $(Y-Y'_i)$ \abedit{is symmetric} and are identically distributed for any $i$. 
Our analysis is based on the following assumption: %\abcomment{cite for $\psi_2$ norm} 
\begin{asmp}
The random variable $(Y(S)-Y(S'_i))^2$ is sub-Gaussian with $\psi_2$-norm $\kappa_A^2$, i.e., $\| (Y-Y'_i)^2 \|_{\psi_2} = \sup_{q \geq 1} (\E_{S.S'}|Y(S)-Y(S'_i)|^{2q})^{1/q}/\sqrt{q} = \kappa_A^2$. 
%has bounded second moment, i.e., $\E_{S,Z'_i}[(Y(S)-Y(S'_i))^2] \leq \nu_A$, for some constant $\nu_A$.\abcomment{should this be a definition? i.e., just call the second moment $\nu_A$?}
\label{asmp:2moment}
\end{asmp}
Assumption~\ref{asmp:2moment} implies that $\|Y-Y'_i\|_{\psi_2} \leq \kappa_A$.
Note that since $Y(S) - Y(S'_i)$ is identically distributed for all $i$, $\kappa_A$ is the same for all $i$. Further, $\kappa_A$ is a property of the algorithm $A$, and can be viewed as a measure of stability.
If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered stable; on the other hand, if $\kappa_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as typical generalization error $\frac{1}{n}Y(S)$ itself. The sharpness of the high-probability bound we present meaningfully depends on $\kappa_A$, with smaller values implying sharper bounds.



\begin{restatable}{theo}{theohighp}
Under Assumption~\ref{asmp:2moment}, with probability at least $(1-\delta)$ over the draw $S \sim D^n$, we have
\begin{equation}
L_D(A(S)) \leq L_S(A(S)) + \E_S\bigg[L_D(A(S) - L_S(A(S))\bigg] + \max\left( \frac{1}{n}, \frac{ c_1 \kappa_A}{\sqrt{n}} \right) \log \left(\frac{16}{\delta} \right)~.      
\end{equation}
\label{theo:hp}
\vspace*{-5mm}
\end{restatable}







If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered very stable; if $\kappa_A=O(\sqrt[4]{n})$, then $A$ can be considered somewhat stable; and if $\kappa^2_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as the generalization error $\frac{1}{n}Y(S)$ itself. 

%\theohighp*

%
%
\proof Let $S=(Z_1,\ldots,Z_n)$ and let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% % Let
% % \begin{align}
% % Y & = f(Z_1,\ldots,Z_n) \\
% % Y'_i & = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)~,~i=1,2,\ldots,n~.
% % \end{align}
With $(x)_+ = max(x,0)$, let
\begin{align}
    V^+ = V^+(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_+^2 ]~,
\end{align}
% % Let
% With $(x)_- = min(x,0)$, let
% \begin{align}
%     V^- = V^-(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~,
% \end{align}

Our proof uses the following exponential version of the Efron-Stein inequality [Theorem 6.16 in \cite{boucheron2013concentration}], whose proof is based on a combination of the symmetric modified log-Sobolev inequality [Theorem 6.15 in \cite{boucheron2013concentration}] with the change of measure:
\begin{theo}\label{theo:exp_efst}
Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
\begin{equation}
\log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
\end{equation}
\end{theo}

% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$ such that $(Y-Y'_i)$ is bounded and $\| Y-Y'_i\|_{\psi_2} = \kappa_A$. Then, with $(x)_+ = \max(0,x)$,
% \begin{equation}
% V^+_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
% \end{equation}
% is sub-Gaussian and $\| V_i^+ \|_{\psi_2} \leq 4\kappa_A^2$. \abcomment{should follow by definition, by bounding $L_p$ norms, since $Y-Y'_i$ is bounded.}
% \end{lemm}


For the proof of Theorem~\ref{theo:hp}, note that $V^+$ is sub-Gaussian with $\| V^+ \|_{\psi_2} \leq n \kappa_A^2$.
Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_2}$. Then from Theorem \ref{theo:exp_efst}, we have
\begin{align*}
\psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right].
\end{align*}
Then, by Markov's inequality we have
\begin{align*}
\log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
 & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
\end{align*}
Choosing $\theta = 1/(2\lambda)$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) 
& \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
\end{align*}
Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
\Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
\end{align*}
With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa_A^2$, with $c_1 = c_0 \sqrt{2}$, we have
\begin{align*}
\P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right) ~.
\end{align*}
Now, we choose $\delta$ such that
\begin{align*}
 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right)   
 \leq 8 \exp \left( - n \epsilon \right)  + 8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta~.
\end{align*}
It suffices to choose $\epsilon$ such that
\begin{align*}
8 \exp \left( - n \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{1}{n} \log \left( \frac{16}{\delta} \right) \\
8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{c_1 \kappa_A}{\sqrt{n}} \log \left( \frac{16}{\delta} \right)~.
\end{align*}
As a result,
\begin{align*}
\P\left( \frac{1}{n}(Y - \E Y) >  \max \left( \frac{1}{n}, \frac{c_1 \kappa_A}{\sqrt{n}} \right) \log \left( \frac{16}{\delta} \right) \right) & \leq \delta~.
\end{align*}
That completes the proof. \qed





==> ICML2022/app/signSGD_opt.tex <==
% The ``density'' for a mini-batch $B$ at scale $\alpha$ is:
% \begin{equation}
% p_{\psi}(\bxi; \btheta_{B,\alpha}) = \exp(\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha} \triangleq \frac{\btheta_B}{\alpha} = \frac{\nabla \ell(\w_{t-1}, S_{B})}{\alpha}~.
% \end{equation}
% Note that the corresponding expectation parameter
% \begin{equation}
% \m_{B,\alpha} = \nabla_{\btheta_{B,\alpha}} \psi( \theta_{B,\alpha} )~.
% \end{equation}

% For mini-batch $B_t$ and scaling $\alpha_t$, Noisy Sign-SGD updates the parameters as
% \begin{equation}
%     \w_t = \w_{t-1} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim B\left(\frac{1}{1+\exp \left(-\boldsymbol{\theta}_{B_{t}, \alpha_{t}}\right)}\right)~, ~ \forall i\in [d]~.
% \end{equation}
% % Here we consider the special case of Bernoulli distribution. Thus
% % $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$

% \begin{asmp}\label{asmp: smooth}
% [Smoothness] For all $\w$ and $\w^\prime$, for some non-negative constant $\vec{K}:=\left[L_{1}, \ldots, L_{d}\right]$, we have
% \begin{align}
% L_S(\w) \leq L_S(\w^\prime) + \nabla L_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} L_i (\w_i - \w^\prime_i)^2
% \end{align}
% \end{asmp}

% Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have
% \begin{align*}
%     L_S(\w_{t+1}) -L_S(\w_{t}) & \leq \nabla L_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d L_i (\w_{t,i} - \w^\prime_{t,i})^2\\
%     & = - \eta_t  \nabla L_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{L_i}{2}\\
%     & = - \eta_t  \|\nabla L_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{K}\|_1 + 2 \eta_t \sum_{i=1}^d |\nabla_i L_S(\w_t)| \mathbb{I}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\}
% \end{align*}

% Take the conditional expectation, we have
% \begin{align*}
% \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq   - \eta_t  \|\nabla L_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{K}\|_1 + 2 \eta_t \sum_{i=1}^d |\nabla_i L_S(\w_t)| \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} 
% \end{align*}

% For now, we have the following approaches:
% \begin{itemize}
%     \item Option I: Show $ \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} \leq 1/2$ for all $i \in [d]$, then we will have $-\eta_t \cdot c \|\nabla L_S(\w_t)\|_1$ for $0<c < 1/2$ on the right hand side. The rest will be standard optimization analysis. 
%     \item Option II: 
%     \begin{align*}
%         \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} & \leq \mathbb{P}\{ |\bxi_{t, i} - \nabla_i L_S(\w_t)| > |\nabla_i L_S(\w_t)|\}\\
%         & \leq \frac{\mathbb{E}[|\bxi_{t, i} - \nabla_i L_S(\w_t)| ]}{ |\nabla_i L_S(\w_t)|}
%     \end{align*}
% \end{itemize}


% \tccomment{
% Case 1: $\nabla_i L_S(\w_t)) > 0$, we have
% \begin{align*}
%     \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} = \mathbb{P}\{\bxi_{t, i} = -1\} = 1-\frac{1}{1+\exp \left(-\nabla_i L_S(\w_t)\right)} < 1-\frac{1}{1+\exp \left(0\right)} = \frac{1}{2}.
% \end{align*}
% Case 2: $\nabla_i L_S(\w_t)) < 0$, we have
% \begin{align*}
%     \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} = \mathbb{P}\{\bxi_{t, i} = 1\} = \frac{1}{1+\exp \left(-\nabla_i L_S(\w_t)\right)} < \frac{1}{1+\exp \left(0\right)} = \frac{1}{2}.
% \end{align*}
% Therefore, we conclude that $ \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} < 1/2$ holds. $c$ approaches zero when $\nabla_i L_S(\w_t)$ approaches zero.
% \yzcomment{To be more rigours, it should be 
% \begin{align*}
% \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} \leq  \mathbb{P}\{\bxi_{t, i} = -1|\nabla_i L_S(\w_t)) > 0\} +    \mathbb{P}\{\bxi_{t, i} = 1|\nabla_i L_S(\w_t)) < 0\} 
% \end{align*}
% I am not sure whether there is dependence between $\bxi_t$ and $ \nabla L_S(\w_t))$, i.e.,
% $\mathbb{P}\{\bxi_{t, i} = -1|\nabla_i L_S(\w_t)) > 0\} = \mathbb{P}\{\bxi_{t, i} = -1\}$ ?
% }
% \subsection{Choice 2:} 
% Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have
% \begin{align*}
%     L_S(\w_{t+1}) -L_S(\w_{t}) & \leq \nabla L_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d L_i (\w_{t,i} - \w^\prime_{t,i})^2\\
%     & = - \eta_t  \nabla L_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{L_i}{2}
% \end{align*}
% Define a function $f:\R^p \rightarrow \R$, where $p$ is the dimension of model parameters: 
% \begin{align*}
%     f(\theta) = \sum_i \theta_i \frac{\exp \theta_i -1}{\exp \theta_i +1} = \sum_i \theta_i \tanh \frac{\theta_i}{2},
% \end{align*}
% we have $f(\theta) \geq 0$, and equality holds if and only if $\theta_i = 0$. Then taking conditional expectation on both side we have 
% \begin{align*}
% \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla L_S(\w_t)^T \E\bxi_t  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  \sum_i \nabla L_S(\w_t)_i \left(\frac{2}{1+\exp \left(-\nabla L_S(\w_t)_i\right)}-1\right)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  \sum_i \nabla L_S(\w_t)_i \left(\frac{\exp \left(-\nabla L_S(\w_t)_i\right) -1 }{\exp \left(-\nabla L_S(\w_t)_i\right)+1}\right)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  f(\nabla L_S(\w_t))  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% \end{align*}
% Taking $\eta_t = \frac{1}{\sqrt{T}}$, by telescope sum we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T f(\nabla L_S(\w_t))\right] \leq \frac{1}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% \end{equation}
% \yzcomment{The distribution of $\bxi_t$ depends on $\nabla \ell(\w_t, S_B)$ instead of full batch gradient $\nabla L_S(\w_t)$, i.e., $\mathbb{P}\{\bxi_{t, i} = -1\} = 1-\frac{1}{1+\exp \left(-\nabla_i \ell(\w_t, S_B)/\alpha\right)}$, where $\mathbb{E}[\nabla \ell(\w_t, S_B)] = \nabla L_S(\w_t)$ . Can we use Jensen's inequality here?}
% Mini-batch settings: 
% \begin{align*}
% \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla L_S(\w_t)^T \E\bxi_t  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  \sum_i \nabla L_S(\w_t)_i \E\left[\frac{2}{1+\exp \left(-\nabla_i \ell(\w_{t-1}, S_{B}/\alpha)\right)}-1\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  \sum_i \nabla L_S(\w_t)_i \E\left[\frac{\exp \left(\nabla_i \ell(\w_{t-1}, S_{B})/\alpha\right) -1 }{\exp \left(\nabla_i \ell(\w_{t-1}, S_{B})/\alpha\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% & = - \eta_t  \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% \end{align*}
% The first quantity can be decomposed as
% \begin{align*}
% & = - \eta_t  \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] - \eta_t\left( \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right)
% \end{align*}
% The first part is $- \eta_t \alpha  f(\nabla L_S(\w_t)/\alpha)$, the second part can be upper bounded by
% \begin{align*}
%   & - \eta_t\left( \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right) \\
%     & \leq  \eta_t\sum_i |\E\theta_{B,i}|\left|\E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right|\\
%     & \leq \eta_t/\alpha \sum_i |\E\theta_{B,i}|\left|\E|\theta_{B,i} -\E[\theta_{B,i}]|\right|\\
%     & = \eta_t/\alpha \sum_i |\E\theta_{B,i}| \|\theta_{B,i} -\E[\theta_{B,i}]\|_{L^1}\\
%     & \leq \frac{\sigma_t\eta_t}{\alpha} \|\E\theta_{B}\|_1\\
%     & \leq \frac{\sigma\eta_t}{\alpha\sqrt{|B_t|}} \|\E\theta_{B}\|_1
% \end{align*}
% where $\tanh$ is 1-Lipschitz function, and we assume first order moment of stochastic gradient is upper bounded by $\sigma_t$ and we can naturally define $\sigma_t\leq \sigma/\sqrt{|B_t|}$. \yzcomment{We can also assume bounded variance/second moment which is common.}
% Gathering everything we have
% \begin{align*}
%   \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}]\leq - \eta_t \alpha  f(\nabla L_S(\w_t)/\alpha) + \frac{\sigma\eta_t}{\alpha\sqrt{|B_t|}} \|\nabla L_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% \end{align*}
% Bt taking $\eta_t = \frac{1}{\sqrt{T}}$, $|B_t| = T$ \yzcomment{This requires $n > = T$, usually we use $|B_t| = \sqrt{T}$ } by telescope sum we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \left(\alpha f(\nabla L_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla L_S(\w_t)\|_1\right) \right] \leq \frac{1}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% \end{equation}
% % Note that $T\rightarrow \infty $, equation implies $$\frac{1}{T}\sum_{t=1}^T \left(\alpha f(\nabla L_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla L_S(\w_t)\|_1\right)  \rightarrow 0,$$ implies $$\alpha f(\nabla L_S(\w_T)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla L_S(\w_T)\|_1\rightarrow 0, $$ implies $$\alpha f(\nabla L_S(\w_T)/\alpha ) \rightarrow 0, $$ implies $$\nablaL_S(\w_T) \rightarrow 0.$$
% Since we have
% \begin{equation}
%     x\tanh x/2 > x^2 \frac{1}{2(1+2\log(\frac{\sinh x}{x})},
% \end{equation}
% and
% \begin{equation}
%     \sinh x 
% \end{equation}
% \begin{align*}
%     \alpha f(\nabla L_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla L_S(\w_t)\|_1 \geq 
% \end{align*}}
% \section{Noisy-SignSGD Optimization analysis}

\subsection{Optimization Guarantees for Noisy Sign-SGD}


The ``density'' for a mini-batch $B$ at scale $\alpha$ is:
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\alpha}) = \exp(\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha} \triangleq \frac{\btheta_B}{\alpha} = \frac{\nabla \ell(\w_{t}, S_{B})}{\alpha}~.
\end{equation}
Note that the corresponding expectation parameter
\begin{equation}
\m_{B,\alpha} = \nabla_{\btheta_{B,\alpha}} \psi( \theta_{B,\alpha} )~.
\end{equation}
The full-batch Noisy Sign-SGD update the parameters as 
\begin{equation}
\label{eq:app_signSGD_full_batch}
    \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim \text{Rad}\left(\frac{1}{1+\exp \left(-2\nabla L_S(\w_t)/\alpha_{t}\right)}\right)~, ~ \forall i\in [d]~,
\end{equation}
where $\text{Rad}(x)$ is the parametric Rademacher distribution with density $x$ at $1$ and density $1-x$ at $-1$.
For mini-batch $B_t$ and scaling $\alpha_t$, mini-batch Noisy Sign-SGD updates the parameters as  
\begin{equation}\label{eq:app_signSGD_mini_batch}
    \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim \text{Rad}\left(\frac{1}{1+\exp \left(-2\boldsymbol{\theta}_{B_{t}, \alpha_{t}}\right)}\right)~, ~ \forall i\in [d]~.
\end{equation}
% Here we consider the special case of Bernoulli distribution. Thus
% $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$
We make the following smoothness assumptions of the empirical loss function $L_S(\w)$:
\asmpsmooth*
% \begin{asmp}\label{asmp: smooth}
% The loss function $L_S$ satisfies: for all $\w$ and $\w^\prime$, for some non-negative constant $\vec{K}:=\left[L_{1}, \ldots, L_{d}\right]$, we have
% \begin{align}
% L_S(\w) \leq L_S(\w^\prime) + \nabla L_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} L_i (\w_i - \w^\prime_i)^2
% \end{align}
% \end{asmp}
The assumption on on the empirical loss $L_S(\w)$ is common in optimization analysis, besides that, we also assume some natural statistical properties of the batch gradient of the loss $\nabla \ell(\w_{t}, S_{B_t})$, where the randomness comes from batches conditioned on $\w_t$, satisfies the following assumptions:
\asmpbatch*
% \begin{asmp}\label{asmp:batch}
% [Batch Gradient] Given $\w_t$, the batched gradient $\nabla \ell(\w_t, S_{B_t})$ satisfies the following property:
% \begin{itemize}
%     \item (Unbiased) The batched gradient $\nabla \ell(\w_{t}, S_{{B_t}})$ is an unbiased estimator of true gradient $L_S(\w_{t})$: $$\E_{B_t|\w_t}\nabla \ell(\w_{t}, S_{B_t}) = \nabla L_S(\w_{t}).$$
%     \item (Symmetricity) The pdf $p_{BG}(x)$ of batched gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is symmetric around its expectation $L_S(\w_{t})$:$$p_{BG}(x) = p_{BG}(2\nablaL_S(\w_{t})-x).$$
%     \item (Sub-Gaussian) The batched gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is Sub-Gaussian with $\psi_2$ norm $\kappa_t$, where $\kappa_t \leq \kappa_t/\sqrt{|B_t|}$: for any $\lambda >0$, $v\in S^{d-1}$, we have $$\E_{B_t|\w_t}\exp \lambda\langle v,\nabla \ell(\w_{t}, S_{B_{t}})-\nabla L_S(\w_{t})\rangle \leq \exp(\lambda^2\kappa_t^2/2)\leq \exp\left(\frac{\lambda^2\kappa_t^2}{2|B_t|}\right).$$
% \end{itemize}
% \end{asmp}
With Assumption \ref{asmp: smooth} and Assumption \ref{asmp:batch}, we have the following guarantee for convergence of noisy signSGD under full batch and mini batch settings. The following is a restate theorem from the main paper for the mini-batch Noisy Sign-SGD
\begin{theo}
The following holds for any $S$, any initialization $\w_0$, and the expectation is taken over the randomness of algorithm: if the loss satisfies Assumption~\ref{asmp: smooth}, for full-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$ and $\alpha_t$ satisfying $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}$, we have
\vspace*{-3mm}
\begin{equation}
\label{eq:sign_SGD_full_batch_convergence_1}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{5c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
\vspace*{-3mm}
\end{equation}
Further, if Assumption~\ref{asmp:batch} holds, for mini-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$, and $\alpha_t$ satisfying $c \geq \alpha_t \geq \max[\sqrt{2}\kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, we have
\vspace*{-3mm}
\begin{equation}
\label{eq:sign_SGD_mini_batch_convergence_1}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
\vspace{-5mm}
\end{equation}
\end{theo}
% \begin{theo}\label{theo:signSGD_conv}
% Assume Assumption~\ref{asmp: smooth} holds for loss function $L_S$. For Full-batch Noisy Sign-SGD algorithm equation~\eqref{eq:signSGD_full_batch} with stepsize $\eta_t = 1/\sqrt{T}$ and choose $\alpha_t$ satisfies $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}/2$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{10c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
% \end{equation}
% Further assume Assumption~\ref{asmp:batch} holds for batch gradient $\nabla\ell(\w_t,S_{B_t})$, for mini-batch noisy Sign-SGD algorithm equation~\eqref{eq:signSGD_mini_batch} with stepsize $\eta_t = 1/\sqrt{T}$, $|B_t|=T$, and 
% % $\alpha_t = 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa_t^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% % \end{equation}
% % or choose $c\geq\alpha_t\geq 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{2c (1+\exp(\frac{\kappa_t^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% % \end{equation}
% % or without assuming $G$, 
% choose $\alpha_t$ by $c \geq \alpha_t \geq \max[\frac{\kappa_t}{\sqrt{2T}}, 2\|\nabla L_S(\w_t)\|_{\infty}]$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{8c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% \end{equation}
% \end{theo}
% Here we restate our results
% \begin{restatable}{theo}\label{theo:signSGD}
% If the loss satisfies Assumption~\ref{asmp: smooth}, for full-batch noisy Sign-SGD with step size $\rho_t = 1/\sqrt{T}$ and $\alpha_t$ satisfying $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}$, we have
% \begin{equation}\label{eq:sign_SGD_full_batch_convergence_1}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{5c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% \end{equation}
% Further, if Assumption~\ref{asmp:batch} holds, for mini-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$, and 
% % $\alpha_t = 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% % \end{equation}
% % or choose $c\geq\alpha_t\geq 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{2c (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% % \end{equation}
% % or without assuming $G$, 
% $\alpha_t$ satisfying $c \geq \alpha_t \geq \max[\sqrt{2}\kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, we have
% \begin{equation}\label{eq:sign_SGD_mini_batch_convergence_1}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
% \end{equation}
% where equation \eqref{eq:sign_SGD_full_batch_convergence_1}\eqref{eq:sign_SGD_mini_batch_convergence_1} holds for any $S$, any initialization $\w_0$, and the expectation is taken over the randomness of  algorithm.
% \end{restatable}





% The result shows the same $O(\frac{1}{\sqrt{T}})$ convergence speed with slightly different constants for both full-batched and mini-batched noisy Sign-SGD.


\proof First we prove Equation \eqref{eq:sign_SGD_full_batch_convergence_1} for full-batched settings.
Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have 
\begin{align*}
    L_S(\w_{t+1}) -L_S(\w_{t}) & \leq \nabla L_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d K_i (\w_{t+1,i} - \w_{t,i})^2\\
    & = - \eta_t  \nabla L_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{K_i}{2}.
\end{align*}
% \abbcomment{how are $K_i$ and $L_i$ related?}
% Define a function $f:\R^d \rightarrow \R$, where $d$ is the dimension of model parameters: 
% \begin{align*}
%     f(\theta) = \sum_i \theta_i \frac{\exp \theta_i -1}{\exp \theta_i +1} = \sum_i \theta_i \tanh \frac{\theta_i}{2},
% \end{align*}
% we have $f(\theta) \geq 0$, and equality holds if and only if $\theta_i = 0$. 
Then taking conditional expectation on both side for above equation we have
\begin{align*}
\mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla L_S(\w_t)^T \E_{\bxi_t|\w_t}\bxi_t  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \left(\frac{2}{1+\exp \left(-2\nabla L_S(\w_t)_i/\alpha_t\right)}-1\right)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \left(\frac{\exp \left(2\nabla L_S(\w_t)_i/\alpha_t\right) -1 }{\exp \left(2\nabla L_S(\w_t)_i/\alpha_t\right)+1}\right)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \tanh (\nabla L_S(\w_t)_i/\alpha_t)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i |\nabla L_S(\w_t)_i| |\tanh (\nabla L_S(\w_t)_i/\alpha_t)|  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{align*}
By taking $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}$, and $\eta_t=1/\sqrt{T}$, we have $\nabla L_S(\w_t)_i/\alpha_t\leq 1$ so we can apply Lemma \ref{lemm:tanh_bound} to have
\begin{align*}
\mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq  - \frac{e^2-1}{(e^2+1)\alpha_t\sqrt{T}}  \|\nabla L_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{K}\|_1\\
&\leq - \frac{3}{5c\sqrt{T}}  \|\nabla L_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{K}\|_1.
\end{align*}
% \abbcomment{what is the para, text, punctuation here?? lets please get our act together}
By telescope sum we have
\begin{equation*}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{5c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
\end{equation*}
which completes the proof of full-batch updates.   


Then we turn to prove Equation \eqref{eq:sign_SGD_mini_batch_convergence_1} for mini-batch settings.
From smoothness condition Assumption \ref{asmp: smooth}, we have
\begin{align*}
\mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq \E_{\w_{t+1}|\w_t}\nabla L_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \E_{\w_{t+1}|\w_t} \sum_{i=1}^d L_i (\w_{t+1,i} - \w_{t,i})^2\\
&= \E_{\bxi_t|\w_t} \nabla L_S(\w_t)^T(-\eta_t \bxi_t) + \frac{1}{2} \E_{\bxi_t|\w_t} \sum_{i=1}^d L_i (-\eta_t \bxi_t)^2\\
    &=- \eta_t  \nabla L_S(\w_t)^T \E_{\bxi_t|\w_t}\bxi_t  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \E_{B_t|\w_t}\left[\frac{2}{1+\exp \left(-2\nabla_i \ell(\w_t, S_{B_{t}}/\alpha_t)\right)}-1\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \E_{B_t|\w_t}\left[\frac{\exp \left(2\nabla_i \ell(\w_t, S_{B_{t}})/\alpha_t\right) -1 }{\exp \left(2\nabla_i \ell(\w_t, S_{B_{t}})/\alpha_t\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
& = - \eta_t  \sum_i \E_{B_t|\w_t} [\theta_{B_{t},i}] \E\left[\frac{\exp \left(2\theta_{B_{t},i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_{t},i}/\alpha_t\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{align*}

Focus on each individual term in the sum, we have
\begin{align*}
\E_{B_t|\w_t}&[\theta_{B,i}] \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_t,i}/\alpha_t\right)+1}\right]\\ 
& = \E_{B_t|\w_t}[\theta_{B_t,i}] \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t - 2\E_{B_t|\w_t}[\theta_{B_t,i}/\alpha_t] \right) -\exp - 2\E_{B_t|\w_t}\theta_{B_t,i}/\alpha_t }{\exp \left(2\theta_{B_t,i}/\alpha_t - 2\E_{B_t|\w_t}[\theta_{B_t,i}/\alpha_t]\right)+\exp - 2\E_{B_t|\w_t}\theta_{B_t,i}/\alpha_t}\right]
\end{align*}


For ease of notation, denote $2\theta_{B,i}/\alpha_t - \E_{B_t|\w_t}[2\theta_{B,i}/\alpha_t] = \theta,~\E_{B_t|\w_t}[2\theta_{B,i}/\alpha_t] =\mu$, %\abbcomment{this is bad notation as we keep $\mu$ for the expectation parameters} 
and the pdf of $\theta$ is $p_{\theta}$ for the moment, then from Assumption \ref{asmp:batch}, we have $\theta$ is mean zero, symmetric around zero, and subgaussian with $\psi_2$ norm $2\kappa_t/\alpha_t$ by taking $\lambda=1,~v = \1_i$ in the sub-Gaussian assumption: $\E_\theta[\exp\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$.

Therefore, by changing notation we have 
\begin{align*}
     \E_{B_t|\w_t}[\theta_{B,i}] \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_t,i}/\alpha_t\right)+1}\right] = \frac{\alpha_t \mu}{2} \E_\theta\left[\frac{\exp \theta -\exp(-\mu) }{\exp \theta +\exp(-\mu)}\right].
\end{align*}
By symmetry of the distribution of $\theta$, we have
\begin{align*}
\frac{\alpha_t \mu}{2} \mu\E&_\theta\left[\frac{\exp \theta -\exp(-\mu) }{\exp \theta +\exp(-\mu)}\right]\\
    &= \frac{\alpha_t \mu}{2}\int_{-\infty}^{\infty}p_\theta(x)\left[\frac{\exp x-\exp(-\mu) }{\exp x +\exp(-\mu)}\right]dx\\
    &=\frac{\alpha_t \mu}{2}\int_{0}^{\infty}p_\theta(x)\left[\frac{\exp x -\exp(-\mu) }{\exp x +\exp(-\mu)}+\frac{\exp (-x) -\exp(-\mu) }{\exp (-x) +\exp(-\mu)}\right]dx\\
    &=\frac{\alpha_t \mu}{2}\int_{0}^{\infty}p_\theta(x)\frac{(\exp x -\exp(-\mu))(\exp (-x) +\exp(-\mu)) + (\exp (-x) -\exp(-\mu))(\exp x +\exp(-\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\alpha_t/2 \int_{0}^{\infty}p_\theta(x)\frac{2\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx
\end{align*}
By symmetry, we have $p_\theta(x) = p_\theta(-x)$, and therefore
\begin{align*}
\alpha_t/2 & \int_{0}^{\infty}p_\theta(x)\frac{2\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\alpha_t/2\int_{-\infty}^{\infty}p_\theta(x)\frac{\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \E_\theta\frac{1}{(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}
\end{align*}
Since $\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu)))\geq 0$, and $\frac{1}{x}$ is convex on $\R_+$, we have
\begin{align*}
   & \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \E_\theta\frac{1}{(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}\\ \geq &\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{\E_\theta(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}.
\end{align*}


Using the sub-Gaussian property of $\theta$: $\E_\theta[\exp\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$, and symmetry so $\E_\theta[\exp -\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$, we have
\begin{align*}
    &\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{\E_\theta(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}\\
    &= \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+\exp(-\mu)(\E\exp \theta +\E\exp (-\theta))}\\
    &\geq  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+2\exp(-\mu)\exp(2\kappa_t^2/\alpha_t^2)}\\
    &\geq  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}.
\end{align*}
Switching back to our previous notation:
\begin{align*}
    \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}
  & = \E_{B_t|\w_t} \theta_{B,i} (1-\exp(-4\E_{B_t|\w_t}\theta_{B,i}/\alpha_t)) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}\\
  & = \nabla L_S(\w_t)_i (1-\exp(-4\nabla L_S(\w_t)_i/\alpha_t)) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)},
\end{align*}


which implies we have
\begin{align*}
    \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{2+2\exp(2\kappa_t^2/\alpha_t^2)}  \sum_i \nabla L_S(\w_t)_i (1-\exp(-4\nabla L_S(\w_t)_i/\alpha_t))  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{align*}
Using Lemma \ref{lemm:mix_norm}, we have
\begin{equation}
    \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{2(1+\exp(2\kappa_t^2/\alpha_t^2))}  \sum_i |\nabla L_S(\w_t)_i| \min \bigg[ |2\nabla L_S(\w_t)_i/\alpha_t| ,0.5\bigg]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
 \end{equation}

We choose $\alpha_t$ such that $\alpha_t \geq 4\|\nabla L_S(\w_t)\|_{\infty}$, then we have
\begin{equation}
\mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{\alpha_t (1+\exp(2\kappa_t^2/\alpha_t^2))}  \|\nabla L_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{equation}
We choose $\alpha_t$ such that $c\geq \alpha_t \geq \max[\sqrt{2} \kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, then we have 
\begin{equation}
    \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{c (1+e)}  \|\nabla L_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{equation}
Therefore, if we choose $\eta_t = 1/\sqrt{T}$, we have
\begin{equation}
    \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{1}{c (1+e)\sqrt{T}}  \|\nabla L_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{K}\|_1.
\end{equation}
By telescope sum, we have
\begin{equation}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{(1+e)c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
\end{equation}
With $\w_R$ to be uniformly randomly sampled from $\{\w_1, .., \w_T\}$, we have
\begin{equation}
    \E \|\nabla L_S(\w_R)\|_2^2\leq  \frac{(1+e)c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
\end{equation}
and note that $1+e<4 $ which completes the proof.   \qed

%--------------------------------------------

% \noindent \abcomment{alternative analysis starts here}

% Using the sub-Gaussian property of $\theta$: $\E_\theta[\exp\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$, and symmetry so $\E_\theta[\exp -\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$, we have
% \begin{align*}
%     &\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{\E_\theta(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}\\
%     &= \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+\exp(-\mu)(\E\exp \theta +\E\exp (-\theta))}\\
%     &\geq  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+2\exp(-\mu)\exp(2\kappa_t^2/\alpha_t^2)}\\
%     &\overset{(a)}{\geq}  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{(1+\exp(-\mu))^2}~,
% \end{align*}
% where (a) follows since $\alpha_t^2 \geq 2\kappa_t^2$. Switching back to our previous notation:
% \begin{align*}
%     \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{(1+\exp(-\mu))^2}
%   & =  \frac{\E_{B_t|\w_t} [\theta_{B,i}] (1-\exp(-4\E_{B_t|\w_t}\theta_{B,i}/\alpha_t))}{(1+ \exp(-\E_{B_t|\w_t} [2\theta_{B,i}/\alpha_t]))^2}\\
%   & =  \frac{\nabla \ell(\w_t)_i (1-\exp(-4\nabla \ell(\w_t)_i/\alpha_t))}{(1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t))^2}~,
% \end{align*}
% which implies we have
% \begin{align*}
%     \mathbb{E}[ \ell(\w_{t+1}) -\ell(\w_{t})|\w_{t}] \leq - \eta_t  \sum_i \frac{\nabla \ell(\w_t)_i (1-\exp(-4\nabla \ell(\w_t)_i/\alpha_t))}{(1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t))^2}  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% \end{align*}
% Since $\alpha_t \geq 4 \| \nabla \ell(\w_t) \|_\infty$, we have $(1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t))^2 \leq 8$. Further, using Lemma \ref{lemm:mix_norm}, we have
% \begin{align*}
% \mathbb{E}[ \ell(\w_{t+1}) -\ell(\w_{t})|\w_{t}] & \leq - \frac{\eta_t}{8}  \sum_i |\nabla \ell(\w_t)_i| \min \bigg[ |2\nabla \ell(\w_t)_i/\alpha_t| ,0.5\bigg]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1 \\
% & \leq - \frac{\eta_t}{8}  \|\nabla \ell(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1~,  
%  \end{align*}
% where (a) follows since $\alpha_t \geq \| \nabla \ell(\w_t) \|_\infty$. \tccomment{The last step becomes $\frac{\eta_t}{4\alpha_t}  \|\nabla \ell(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1$ so we still need upper bound on $\alpha_t$? Or shall we express the bound into L1 norm instead of L2 square so we can avoid c?}

% % \tccomment{How about this:
% % we have
% % \begin{align*}
% %     \mathbb{E}[ \ell(\w_{t+1}) -\ell(\w_{t})|\w_{t}] &\leq - \eta_t  \sum_i \frac{\nabla \ell(\w_t)_i (1-\exp(-4\nabla \ell(\w_t)_i/\alpha_t))}{(1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t))^2}  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% %     &= - \eta_t  \sum_i \frac{\nabla \ell(\w_t)_i (1-\exp(-2\nabla \ell(\w_t)_i/\alpha_t))}{1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t)}  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% % \end{align*}
% % we prove for $x\in[-1,1]$, $x\frac{1-\exp(-2x)}{1+\exp(-2x)}\geq $
% % }





% % We choose $\alpha_t$ such that $\alpha_t \geq 4\|\nabla L_S(\w_t)\|_{\infty}$, then we have
% % \begin{equation}
% % \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{\alpha_t (1+\exp(2\kappa_t^2/\alpha_t^2))}  \|\nabla L_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% % \end{equation}
% % We choose $\alpha_t$ such that $\alpha_t \geq \max[\sqrt{2} \kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, then we have \abbcomment{remind readers that $c \geq \alpha_t$}
% % \begin{equation}
% %     \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{c (1+e)}  \|\nabla L_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% % \end{equation}
% Therefore, if we choose $\eta_t = 1/\sqrt{T}$, we have
% \begin{equation}
%     \mathbb{E}[ \ell(\w_{t+1}) -\ell(\w_{t})|\w_{t}] \leq - \frac{1}{8\sqrt{T}}  \|\nabla \ell(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{K}\|_1.
% \end{equation}
% By a telescopic sum, we have 
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \ell(\w_t)\|_2^2  \right] \leq  \frac{8}{\sqrt{T}}\left(\ell(\w_{0}) - \ell(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right)~,
% \end{equation}
% That completes the proof.  \qed 

% \abcomment{with the new analysis, the result is not in terms of $c \geq \alpha_t$}




% Using Lemma \ref{lemm:mix_norm}, we have
% \begin{align*}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \sum_i^d \min (\nabla_i L_S(\w_t)^2/\alpha_t^2,|\nabla_i L_S(\w_t)|/2\alpha_t  )  \right] \leq \frac{2+2\exp(\kappa_t^2/2\alpha_t^2)}{\alpha_t} \frac{1}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right)
% \end{align*}
% Since $\exp(\theta) \geq 1+ \theta + \frac{1}{2} \theta^2$ for $\theta \geq 0$ and reverse for $\theta <0$, so $\theta\exp(\theta) \geq \theta+ \theta^2 + \frac{1}{2} \theta^3$ then
% \begin{align*}
%     \theta_i(1-\exp(-2\theta_i)) \geq \theta_i - \theta_i -2 \theta_i^2 - 2\theta_i^3
% \end{align*}


\begin{lemm}\label{lemm:tanh_bound}
For any $-1\leq x\leq 1$, the following holds:
\begin{equation}
    |\tanh x|\geq \frac{e^2-1}{e^2+1}|x|
\end{equation}
\end{lemm}
\proof Without loss of generality, we focus on $0<x\leq 1$. we prove $\tanh x/ x$ is decreasing function on $\R^+$, which is equivalent to
\begin{align*}
    (\frac{\tanh x}{x})' =  \frac{x(1-\tanh^2 x) - \tanh x }{x^2}\leq 0,
\end{align*}
and is equivalent to 
\begin{align*}
    x\leq \frac{\tanh x}{1 -\tanh^2 x},
\end{align*}
where the right hand side is $\sinh x$ and use the fact that $x\leq \sinh x$ for $x > 0$ implies $\tanh x/x$ is decreasing function, so 
\begin{align*}
    \tanh x/x\geq \tanh 1 = \frac{e^2-1}{e^2 +1},
\end{align*} which completes the proof. \qed

\begin{lemm}\label{lemm:mix_norm} For any $x$,
$$|1-\exp(-2x))|\geq \min (|x|,\frac{1}{2}).$$
\end{lemm}
\proof 
Since $\exp(-x)\geq 1-x$, so we have for $x<0$:
$$1-\exp (-2x)\leq 2x\leq x.$$

For $x>0$, since $\exp x \geq 1+x$, we have $\exp -x\leq \frac{1}{1+x}$, so
$$1-\exp (-2x)\geq \frac{2x}{1+2x}.$$
Then when $\frac{1}{2}>x>0$, $$\frac{2x}{1+2x} > x,$$
and when $x\geq \frac{1}{2}$, $$\frac{2x}{1+2x} \geq \frac{1}{2},$$
which completes the proof.\qed


\theoSGLDopt*

\proof Recall that the update of SGLD is
\begin{equation}
\mathbf{w}_{t+1}=\mathbf{w}_{t}-\eta_{t} \nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)+ \sigma_{t}  \mathcal{N}\left(0, \mathbb{I}_{d}\right)~.
\end{equation}
By smoothness of the loss, taking expectation w.r.t.~the randomness of the mini-batch $B_t$ and the Gaussian draw $\g_t \sim \cN(0,\I_d)$ conditioned on $\w_{1:t}$, we have
\begin{align*}
\mathbb{E} [L_S(\w_{t+1})] &\leq L_S(\w_t) + \mathbb{E} [\left\langle \nabla L_S(\w_t), \w_{t+1} - \w_t \right\rangle ]  + \frac{K}{2} \mathbb{E} [ \|  \w_{t+1} - \w_t\|^2] \\
& =  L_S(\w_t) + \mathbb{E} [\left\langle \nabla L_S(\w_t), -\eta_t \nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right) + \sigma_t \g_t \right\rangle] + \frac{K}{2} \E[\| -\eta_t \nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right) + \sigma_t \g_t \|^2] \\
& \overset{(a)}{\leq}  L_S(\w_t) -\eta_t \|\nabla L_S(\w_t)\|^2 + \frac{K \eta_t^2}{2} \left(c_3 \kappa_t^2 + p\sigma_t^2/\eta_t^2\right)~,
\end{align*}
where (a) follows since $\E[\nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)]=0, \E[\g]=0, \E[\|\g\|^2] = p$, and $\E[\|\nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)\|^2] \leq c_3 \kappa_t^2$ for some absolute constant $c_3$ since $\nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)$ is sub-Gaussian with $\psi_2$-norm $\kappa_t$.
%where $\kappa^2$ is the upper bound of the variance of $\nabla \ell(\w_{t}, S_{B_t})$.

Rearranging the above inequality and using $\alpha_t = \sigma_t/\eta_t$ we have
\begin{align} \label{eq:one_step_descend}
    \eta_t \| \nabla L_S(\w_t)\|^2 \leq  L_S(\w_t) - \mathbb{E} [L_S(\w_{t+1})]  + \frac{K \eta_k^2}{2}\left(c_3 \kappa_t^2 + p\alpha_t^2\right)~.
\end{align}
Summing over $t =1$ to $t =T$ and apply expectation over the trajectory at each step, we have
\begin{align*}
\sum_{t =1}^T \eta_t\mathbb{E}\| \nabla L_S(\w_t)\|^2 
\leq L_S(\w_1) - L_S(\w^\star) +  \sum_{t=1}^T \frac{K \eta_t^2}{2} (p \alpha_t^2 + \kappa_t^2)~,
%+\frac{(p \sigma^2 + G^2) \sum_{k=1}^T \eta_k^2}{\sum_{k=1}^T \eta_k}.  
\end{align*}
where $\w^*$ is a minima of $L_S(\w)$. With $\eta_t= \frac{1}{\sqrt{T}}$ for all $t \in [T]$, we have
\begin{align*}
\frac{1}{T} \sum_{t =1}^T \mathbb{E} \| \nabla L_S(\w_t)\|^2 
%\min_{k\in [T]} \mathbb{E} \| \nabla L_S(\w_t)\|^2
\leq\frac{L_S(\w_1) - L_S(\w^\star)}{\sqrt{T}} + \frac{  \frac{K}{2T} \sum_{t=1}^T (p \alpha_t^2 +  c_3 \kappa_t^2) }{\sqrt{T}}~.  
\end{align*}
With $\w_R$ to be uniformly randomly sampled from $\{\w_1, .., \w_T\}$, we have

\begin{align*}
\mathbb{E} \| \nabla L_S(\w_R)\|^2 
\leq\frac{L_S(\w_1) - L_S(\w^\star)}{\sqrt{T}} + \frac{  \frac{K}{2T} \sum_{t=1}^T (p \alpha_t^2 +  c_3 \kappa_t^2) }{\sqrt{T}}~.  
\end{align*}

That completes the proof.  \qed 

==> ICML2022/sec/abstract.tex <==
%We study generalization bounds for noisy stochastic algorithms based on the notion of stability. 
Recent years have seen advances in generalization bounds for noisy stochastic algorithms,
%such algorithms, 
especially stochastic gradient Langevin dynamics (SGLD) based on stability~\citep{mou2018generalization, Li2020On} and information theoretic approaches~\citep{xu2017information,negrea2019information,steinke2020reasoning}. 
%
In this paper, we unify and substantially generalize stability based generalization bounds and make three technical contributions. First, we bound the generalization error  in terms of expected (not uniform) stability which arguably leads to quantitatively sharper bounds.
%
Second, as our main contribution, we introduce Exponential Family Langevin Dynamics (EFLD), a substantial generalization of SGLD, which includes noisy versions of Sign-SGD and quantized SGD as special cases.
%First, we bound the generalization error of general noisy stochastic iterative algorithms in terms of expected (not uniform) stability which in turn be bounded by a Le Cam Style Divergence. 
% Second, as our main contribution, we introduce Exponential Family Langevin Dynamics (EFLD), 
% a substantial generalization of SGLD which allows exponential family noise to be used with SGD. In addition to SGLD, EFLD includes noisy versions of Sign-SGD and quantized SGD as special cases. 
We establish data-dependent expected stability based generalization bounds for any EFLD algorithm with a $O(1/n)$ sample dependence and  dependence on gradient discrepancy rather than the norm of gradients, yielding significantly sharper bounds.
%
Third, we establish optimization guarantees for special cases of EFLD.
%noisy Sign-SGD and also revisit such guarantees for SGLD.
%consider an important special case of EFLD: noisy sign-SGD, which extends sign-SGD using \tcedit{skewed Rademacher} noise over $\{-1,+1\}$. Generalization bounds for noisy sign-SGD is implied by that of EFLD and we also establish optimization guarantees for the algorithm. 
%
Further, empirical results on benchmarks
%benchmark datasets to 
illustrate that our bounds are non-vacuous, quantitatively sharper than existing bounds, and behave correctly under noisy labels.


% We study generalization bounds for noisy stochastic mini-batch iterative algorithms based on the notion of stability. Recent years have seen key advances in data-dependent generalization bounds for noisy iterative learning algorithms such as stochastic gradient Langevin dynamics (SGLD) based on stability~\citep{mou2018generalization, Li2020On} and information theoretic approaches~\citep{xu2017information,negrea2019information,steinke2020reasoning,haghifam2020sharpened}. In this paper, we unify and substantially generalize stability based generalization bounds and make three technical advances. First, we bound the generalization error of general noisy stochastic iterative algorithms (not necessarily gradient descent) in terms of expected (not uniform) stability. The expected stability can in turn be bounded by a Le Cam Style Divergence. Such bounds have a $O(1/n)$ sample dependence unlike many existing bounds with $O(1/\sqrt{n})$ dependence. Second, we introduce Exponential Family Langevin Dynamics (EFLD) 
% which is a substantial generalization of SGLD and which allows exponential family noise to be used with stochastic gradient descent (SGD). We establish data-dependent expected stability based generalization bounds for general EFLD algorithms. Third, we consider an important special case of EFLD: noisy sign-SGD, which extends sign-SGD using \tcedit{skewed Rademacher} noise over $\{-1,+1\}$. Generalization bounds for noisy sign-SGD is implied by that of EFLD and we also establish optimization guarantees for the algorithm. Further, we present empirical results on benchmark datasets to illustrate that our bounds are non-vacuous and quantitatively much sharper than existing bounds.

==> ICML2022/sec/conc.tex <==
\vspace*{-2mm}
Inspired by recent advances in stability based and information theoretic approaches to generalization bounds \citep{mou2018generalization,pensia2018generalization,negrea2019information,Li2020On,haghifam2020sharpened}, we have presented a framework for developing such bounds based on expected stability for noisy stochastic iterative algorithms. We have also introduced Exponential Family Langevin Dynamics (EFLD), a large family of noisy gradient descent algorithms based on exponential family noise, including SGLD and Noisy Sign-SGD as two special cases.  We have developed an expected stability based generalization bound applicable to any EFLD algorithm with a $O({1}/{n})$ sample dependence and a dependence on gradient discrepancy, rather than gradient norms. Further, we have provided optimization guarantees for special cases of EFLD, viz.~Noisy Sign-SGD and SGLD. Our experiments on various benchmarks illustrate that our bounds are non-vacuous and quantitatively much sharper than existing bounds~\citep{Li2020On,negrea2019information}. 


%Further, we have simplified the task to one of bounding expected for the NSI algorithm. We have developed a specific bound for SGD with Gaussian noise which inherits strengths of a variety of existing results and quantitatively outperforms them based on preliminary experiments. We have also developed similar bounds for SGD with exponential family noise, which seem to be the first result of this type. Our work also highlights few key directions for future work, including sharper notions of gradient discrepancy/incoherence and better understanding of the trade-offs between stability and optimization for NSI algorithms.

==> ICML2022/sec/efld.tex <==
%\vspace*{-2mm} 

Recent years have seen advances in establishing generalization bounds for SGLD \citep{Li2020On, pensia2018generalization, negrea2019information, haghifam2020sharpened} which adds isotropic Gaussian noise at every step of SGD:
%\vspace*{-2mm}
\begin{align}
\label{eq:sgld}
\w_{t+1} = \w_{t} - \eta_t \nabla \ell(\w_t, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}\right)~,
%\vspace*{-2mm}
\end{align}
where $ \nabla \ell(\w_t, S_{B_t})$ is the stochastic gradient on mini-batch $B_t$, $\eta_t$ is the step size, and $\sigma_t^2$ is noise vairance.  We introduce a substantial generalization of SGLD called Exponential Family Langevin Dynamics (EFLD) which uses general exponential family noise in noisy iterative updates of the form~\eqref{eq:nmia}. In addition to being a mathematical generalization of the popular SGLD, the proposed EFLD provides flexibility to use noisy gradient algorithms with different representation of the gradient, e.g., skewed Rademacher noise for Sign-SGD, discrete distribution for quantized or finite precision SGD, etc. \citep{canonne2020discrete, quantized-sgd, jiang2018, yang2019swalp}. All technical proofs for results in this section are in Appendix~\ref{sec:app_efld}.

\subsection{Exponential Family Langevin Dynamics (EFLD)}\label{subsec:efld}


Exponential families \citep{barndorff2014information,brown1986fundamentals,wainwright2008graphical} constitute a large family of parametric distributions which include Gaussian, Bernoulli, gamma, Poisson, Dirichlet, etc., as special cases. Exponential families are typically represented in terms of natural parameters $\btheta$, and we consider component-wise independent distributions with scaled natural parameter $\btheta_{\alpha} = \btheta/\alpha$ with scaling $\alpha > 0$, i.e.,
%\vspace{-2mm}
\begin{align*}
%\vspace{-3mm}
p_{\psi}(\bxi, \btheta_{\alpha})  &= \exp(\langle \bxi, \btheta_{\alpha} \rangle - \psi(\btheta_{\alpha})) \ppi_{0,\alpha}(\bxi)  \\
&= \prod_{j=1}^p \exp( \xi_j \theta_{j\alpha} - \psi_j(\theta_{j\alpha})) \pi_{0,\alpha}(\xi_j)~,
\vspace*{-2mm}
\end{align*}
where $\bxi \in \R^p$ is the sufficient statistic, $\psi(\btheta_{\alpha})= \sum_{j=1}^p \psi_j(\theta_{j\alpha})$ is the log-partition function, and $\ppi_{0,\alpha}(\xi) = \prod_{j=1}^p \pi_{0,\alpha}(\xi_j)$ is the base measure. %\abdelete{Note that $\alpha=1$ gives the canonical form of the exponential family distributions. For general scaling $\alpha > 0$, for certain distributions the base measure $\pi_0$  may depend on the scaling, i.e., $\pi_{0,\alpha}$. A scaling $\alpha >0$ is valid as long as $\exp(\langle \bxi,\btheta_{\alpha} \rangle)$ is integrable, i.e., $\int_{\bxi} \exp(\langle \bxi,\btheta_{\alpha} \rangle \pi_{0,\alpha}(\bxi) d\bxi < \infty$. Further,}
$\psi$ is a smooth convex function by construction \citep{barndorff2014information,banerjee2005clustering,wainwright2008graphical} which implies $\nabla_{\btheta_\alpha}^2 \psi(\btheta_{\alpha}) \leq c_2 \I$ for some constant $c_2 > 0$. 


Exponential family Langevin dynamics (EFLD) uses noisy stochastic gradient updates similar to SGLD, but using exponential family noise rather than Gaussian noise as in SGLD. In particular, for mini-batch $S_{B_t}$, EFLD updates are as follows: with step size $\rho_t > 0$
%\vspace{-2mm}
\begin{equation}
    \w_t = \w_{t-1} - \rho_t \bxi_t~, \qquad \bxi_t \sim p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})~,
\vspace{-3mm}    
\label{eq:efld1}
\end{equation}
where 
%\vspace{-2mm}
\begin{align}
&p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})  = \exp(\langle \bxi, \btheta_{B_t,\alpha_t} \rangle - \psi(\btheta_{B_t,\alpha_t})) \ppi_{0,\alpha}(\bxi)   ~,\\
&\btheta_{B_t,\alpha_t}  \triangleq \frac{\btheta_{B_t}}{\alpha_t} = \frac{\nabla \ell(\w_{t-1}, S_{B_t})}{\alpha_t}~. 
\label{eq:efld2}
\end{align}
For EFLD, the natural parameter $\btheta_{B_t,\alpha_t}$ at step $t$ is simply a scaled version of the mini-batch gradient $\nabla \ell(\w_{t-1}, S_{B_t})$. 
EFLD becomes SGLD when the exponential family is {\em Gaussian} with $\btheta_{B_t} = \bmu_{B_t} = \nabla \ell(\w_{t-1},S_{B_t})$, i.e., the (unscaled) mean $\bmu_{B_t}$ is the mini-batch gradient, since the natural and expectation parameters are equal for Gaussians~\cite{barndorff2014information,banerjee2005clustering}. EFLD becomes noisy sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise} when the exponential family is a {\em skewed Rademacher distribution} over $\{-1,+1\}$ with $P(\xi_j=+1) = \frac{\exp(\nabla \ell_j)}{\exp(-\nabla \ell_j) + \exp(\nabla \ell_j)}, P(\xi_j=-1)= 1 - P(\xi_j=+1)$ where $\nabla \ell_j = [\nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t]_j$ which becomes Sign-SGD as $\alpha_t \rightarrow 0$ (Appendix \ref{app:example}).
%


% \begin{remark}
% \abcomment{briefly explain why absolute continuity is not being violated for the Bernoulli, and more general discrete cases}
% \end{remark}



\subsection{Expected Stability of EFLD}
\input{ICML2022/sec/stability}



\subsection{Optimization Guarantees for EFLD}

We now establish optimization guarantees for two examples of EFLD, i.e., Noisy Sign-SGD with skewed Rademacher noise over $\{-1,+1\}$ and SGLD with Gaussian noise. The details and the proof for results in this subsection are relegated in Appendix \ref{app:opt}.

\noindent {\bf Noisy Sign-SGD.} For noisy Sign-SGD with mini-batch $B_t$ and scaling $\alpha_t$, mini-batch Noisy Sign-SGD updates as $\w_{t} = \w_{t-1} - \eta_t \bxi_t$, where each component $j\in [p]$
%\vspace{-2mm}
\begin{equation*}\label{eq:signSGD_mini_batch}
\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(\xi_j) =  \frac{\exp(\xi_j \theta_{B_t,\alpha_t,j})}{\exp(-\theta_{B_t,\alpha_t,j})+\exp(\theta_{B_t,\alpha_t,j})},
\end{equation*}
where $\xi_j\in\{-1,+1\}$ and $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
The full-batch version uses parameters $\btheta_{B_t,\alpha_t} = \nabla L_S(\w_{t-1})/\alpha_t$.
% Here we consider the special case of Bernoulli distribution. Thus
% $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$
For full batch gradient descent, we assume that the loss is smooth.
%of the empirical loss function $L_S(\w)$:
\begin{restatable}{asmp}{asmpsmooth}\label{asmp: smooth}
The loss function $L_S(\w) = \frac{1}{n} \sum_{i=1}^n \ell(\w,z_i)$ satisfies: $\forall \w, \w^\prime$, for some non-negative constants $\vec{K}:=\left[K_{1}, \ldots, K_{p}\right]$, we have
%\begin{align}
$L_S(\w) \leq L_S(\w^\prime) + \nabla L_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} K_i (w_i - w^\prime_i)^2$. 
%\vspace*{-1mm}
\end{restatable}

For mini-batch analysis, we assume the mini-batch gradients are unbiased, symmetric, and sub-Gaussian.
\begin{restatable}{asmp}{asmpbatch}\label{asmp:batch}
Given $\w_{t-1}$, the mini-batch gradient $\nabla \ell(\w_{t-1}, S_{B_t})$ is
(a)  unbiased,  i.e., $\E_{B_t|\w_{t-1}}\nabla \ell(\w_{t-1}, S_{B_t}) = \nabla L_S(\w_{t-1})$; (b) symmetric, i.e., the density $p_{B_t|\w_{t-1}}(\bxi)$ of $\bxi \equiv \nabla \ell(\w_{t-1}, S_{B_{t}})$ is symmetric and 
(c) sub-Gaussian, i.e., for any $\lambda >0$, {any $\v$ s.t. $\|\v\|_2 =1$}, $
\E_{B_t|\w_{t-1}}[\exp \lambda\langle \v,\nabla \ell(\w_{t-1}, S_{B_{t}})-\nabla  L_S(\w_{t-1})\rangle] \leq \exp(\lambda^2\kappa_t^2/2)~,
$
for some constant $\kappa_t > 0$.
%\vspace{-5mm}
\end{restatable}
%With Assumption \ref{asmp: smooth} and Assumption \ref{asmp:batch}, we have the following guarantee for convergence of noisy signSGD under full batch and mini batch settings:
The smoothness assumption in Assumption \ref{asmp: smooth} is standard in non-convex optimization especially for sign-SGD literature \citep{bernstein2018signsgd,bernstein2018signsgdnoise}. Assumption \ref{asmp:batch} for the mini-batch setting helps the theoretical analysis, where (a) is satisfied when the batches $S_{B_t}$ are taken uniformly from samples $S$ as the standard training does; (b) assumes symmetry of the mini-batch gradients; and (c) is similar and stronger assumption compared to Assumption 3 in \citet{bernstein2018signsgd}, where they assume bounded variance for stochastic gradient and our assumption implies suitably bounded higher moments of $\nabla \ell(\w_{t-1}, S_{B_{t}})-\nabla  L_S(\w_{t-1})$, which is referred as the minibatch noise in recent noisy SGD literature e.g. \citet{damian2021label}. 
Similar to such literature, if we consider mini-batch stochastic gradient be modeled as the average of $|B_t|$ calls to the full-batch gradient, from concentration property $\kappa_t$ is scaled by $1/\sqrt{|B_t|}$. %\abbcomment{this is a bit unclear}

Based on the assumptions, we have following optimization guarantee for mini-batch noisy Sign-SGD, the full-batch version can be found in Appendix \ref{app:opt}.






\begin{restatable}{theo}{theosignSGDconv}\label{theo:signSGD}
The following holds for any $S$, any initialization $\w_0$, and the expectation is taken over the randomness of algorithm: if Assumption~\ref{asmp: smooth} and \ref{asmp:batch} hold, for mini-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$, and $\alpha_t$ satisfying $c \geq \alpha_t \geq \max[\sqrt{2}\kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, we have
%\vspace*{-3mm}
\begin{equation*}\label{eq:sign_SGD_mini_batch_convergence_1}
    \E \|\nabla L_S(\w_R)\|_2^2 \leq O\left(\frac{1}{\sqrt{T}}\right) + O\left(\frac{\|\vec{K}\|_1}{\sqrt{T}}\right)~,
        % \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
%\vspace{-2mm}
\end{equation*}
where $\w_R$ is uniformly randomly sampled from $\{\w_t\}_{t=1}^T$.
\end{restatable}
%\vspace{-2mm}
% \yzcomment{$\w^*$ is not defined, it might be good to use big O, so we don’t have to define $\w^*$ to save space. Also $\E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right]$ can be replaced with $\E\|\nabla L_S(\w_R)\|$ with $\w_R$ uniformly sampled from $\{\w_t\}_t$}


%\vspace*{-2mm}
\begin{figure*}[t] 
\centering
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-c-new.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-c-new.png}
 }
\subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-c-new.png}
 } 
 \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-c-new.png}
 } 
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-b-new.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-b-new.png}
 }
\subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-b-new.png}
 } 
 \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-b-new.png}
}
% \vspace*{-1mm}
%   \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a-new.png}
%  } 
%   \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a-new.png}
%  }
%   \subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-a-new.png}
%  } 
%   \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-a-new.png}
%  }
%\vspace*{-4mm}
\caption[]{Results for training CNN using SGLD on MNIST, Fashion-MNIST and CIFAR-10. %X-axis shows the number of training epochs. 
(a)-(d) shows our bound is non-vacuous and can be used to bound the empirical test error. (e)-(h) compare our bound with the existing bounds and show the effect on $\alpha_t^2$. Our bounds are numerically sharper than existing bounds, and larger $\alpha_t^2$ leads to tighter generalization bounds which is consistent with Theorem~\ref{theo:efldstab}. 
}
%\vspace*{-5mm}
\label{fig:sgld_bound}
\end{figure*}









\noindent {\bf Stochastic Gradient Langevin Dynamics (SGLD).} We acknowledge that following optimization result for SGLD exists in various forms, as noisy gradient descent algorithms with Gaussian noise have been studied in literature such as differential privacy, where SGLD can be viewed as DP-SGD  \citep{bassily2014private, wang2019differentially} and the proof technique boils down to bounding the stochastic variance of the noisy gradient \citep{shamir2013stochastic}.
%\abcomment{ack that this result exists in various forms, is not new}
\begin{restatable}{theo}{theoSGLDopt}
The following holds for any $S$, any initialization $\w_0$, and the expectation is taken over the randomness of algorithm: under Assumptions \ref{asmp: smooth} and \ref{asmp:batch} with $K_i = K, \forall i \in [p]$,  SGLD, i.e., EFLD with Gaussian noise, $\rho_t = \eta_t$, $\alpha_t = \sigma_t/\eta_t$,
% batch size $|B_t| = b$, 
and step size $\eta_t = \frac{1}{\sqrt{T}}$ satisfies 
%\vspace{-3mm}
\begin{align*}
%\vspace{-2mm}
\mathbb{E} \| \nabla L_S(\w_R)\|^2
\leq & O\left(\frac{1 }{\sqrt{T}}\right) 
 + O\left(\frac{  \frac{K}{2T} \sum_{t=1}^T (p \alpha_t^2 +   \kappa_t^2) }{\sqrt{T}} \right) ~,
% \mathbb{E}\left[\frac{1}{T} \sum_{t =1}^T  \| \nabla L_S(\w_t)\|^2\right]
% \leq & \frac{L_S(\w_0) - L_S(\w^*)}{\sqrt{T}} \nonumber\\
% & + \frac{  \frac{K}{2T} \sum_{t=1}^T (p \alpha_t^2 +  c_3 \kappa_t^2) }{\sqrt{T}}.
%\vspace{-5mm}
\end{align*}
where $\w_R$ is uniformly randomly sampled from $\{\w_t\}_{t=1}^T$.
%\vspace*{-2mm}
\end{restatable}
%\vspace*{-2mm}
The error rate of SGLD depends on the noise level $\alpha_t$ and the sub-Gaussian parameter $\kappa_t$.  The bound has a $O(1/\sqrt{T})$ rate as long as the average noise level and sub-Gaussian parameter are bounded by a constant. %We note that 
Similar to differentially private SGD, the convergence rate depends on the dimension of the gradient $p$ due to the isotropic Gaussian noise. %\abbcomment{we have discussed this -- if we show stability results for the general anisotropic case, the result can be updated with $\tr$ of covariance. We can anyway do that} 
Special noise structures such as anisotropic noise that align with the gradient structure can improve the dependence on dimension \citep{kairouz2020dimension,zhang2021wide,asi2021private, zhou2020bypassing}.  






%\abccomment{for each result, we have to say exactly which appendix has the proof}



==> ICML2022/sec/exp.tex <==
% %\vspace*{-2mm}
% \begin{figure*}[t] 
% \centering
% \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-c-new.png}
%  } 
%  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-c-new.png}
%  }
% \subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-c-new.png}
%  } 
%  \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-c-new.png}
%  } \vspace*{-3mm}
%  \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-b-new.png}
%  } 
%  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-b-new.png}
%  }
% \subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-b-new.png}
%  } 
%  \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-b-new.png}
% }
% % \vspace*{-1mm}
% %   \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
% %  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a-new.png}
% %  } 
% %   \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
% %  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a-new.png}
% %  }
% %   \subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
% %  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-a-new.png}
% %  } 
% %   \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
% %  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-a-new.png}
% %  }
% \vspace*{-2mm}
% \caption[]{Results for training CNN using SGLD %($\sigma_t = \sqrt{2\eta_t/\beta_t}$) 
% on MNIST, Fashion-MNIST and CIFAR-10. X-axis shows the number of training epochs. (a)-(d) shows our bound is non-vacuous and can be used to bound the empirical test error. (e)-(h) compare our bound with the existing bounds and show the effect on $\alpha_t^2$. Our bounds are numerically sharper than existing bounds, and larger $\alpha_t^2$ leads to tighter generalization bounds which is consistent with the theoretical analysis. 
% }
% %\vspace*{-3mm}
% \label{fig:sgld_bound}
% \end{figure*}






% In this section, we conduct a series of experiments to evaluate our generalization error bounds. For SGLD, we aim to compare the proposed  bound in Theorem \ref{theo:efldstab} with existing bounds in \cite{Li2020On} and  \cite{negrea2019information} for various datasets.
% Note that we do not consider the bound in \cite{haghifam2020sharpened} as a baseline because the bound in \cite{haghifam2020sharpened} only applies to full-batch setting, but we focus on noisy mini-batch gradient descent. We note that the squared norm of ``two-sample incoherence'' appeared in \cite{haghifam2020sharpened} (Theorem 4.2) roughly has the same order of magnitude as the gradient incoherence appeared in \cite{negrea2019information}. We also evaluate the optimization performance of proposed Noisy Sign-SGD by comparing it with the original sign-SGD \citep{bernstein2018signsgd} and present the corresponding generalization bound in Theorem \ref{theo:efldstab}. 



In this section, we conduct experiments to evaluate our generalization error bounds. For SGLD, we compare our bound in Theorem \ref{theo:efldstab} with existing bounds in \citet{Li2020On, negrea2019information, rodriguez2021random} for various datasets. Note that the bound presented in \citet{rodriguez2021random} is an extension of that in \citet{haghifam2020sharpened} from full-batch setting to mini-batch setting. We also evaluate the optimization performance of proposed Noisy Sign-SGD, comparing it with the original Sign-SGD \citep{bernstein2018signsgd} and present the corresponding generalization bound in Theorem \ref{theo:efldstab}. 

The details of model architectures, learning rate schedules, hyper-parameter selections, and additional experimental results can be found in Appendix \ref{app:exp}. Evaluation of the expectation in Theorem~\ref{theo:efldstab} is done based on (re)sampling (Appendix~\ref{app:exp}). We emphasize that the goal for the experiments is to do a comparative study relative to existing bounds. We note that the empirical performance of the methods can potentially be improved with better architectures and training strategies, e.g., deeper/wider networks, data augmentation, batch/layer normalization, etc. 
%that we did not achieve the state-of-the art predictive performance, mainly due to the simplicity of our model architectures. With more complex model and further tuning, the prediction results could be improved.








% \begin{figure*}[th!] 
% \centering
%   \subfigure[CNN, MNIST]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/cnn1-mnist-n0-bs100-sign-sgd-train-dynamics-reduced.png}
%  } 
%   \subfigure[CNN, Fashion]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/cnn1-fashion-n0-bs100-sign-sgd-train-dynamics-reduced.png}
%  }
%  \subfigure[ResNet-18, CIFAR10]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/resnet18-cifar10-n0-bs100-sign-sgd-train-dynamics-reduced.png}
%  }
%  \subfigure[ResNet-18, CIFAR100]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/resnet18-cifar100-n0-bs100-sign-sgd-train-dynamics-reduced.png}
%  }\vspace*{-2mm}
% \subfigure[MNIST, $\alpha_t=1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
%  } 
%   \subfigure[MNIST, $\alpha_t=0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-e.png}
%  }
%   \subfigure[Fashion, $\alpha_t=1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
%  } 
%   \subfigure[Fashion, $\alpha_t=0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-e.png}
%  }
% \vspace*{-4mm}
% \caption[]{(a)-(d) show the training dynamics of CNN on MNIST and Fashion-MNIST, and ResNet-18 on CIFAR-10 and CIFAR-100 using noisy sign-SGD with different scaling $\alpha_t$. Legends indicate the choice of $\alpha_t$ and the numbers in brackets are test errors at convergence. As $\alpha_t\to 0$, Nosiy sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original sign-SGD \citep{bernstein2018signsgd}. (e)-(f) show that empirical test error can be bounded based on our generalization bound and the corresponding training error. The larger $\alpha_t$ (noise) is the sharper our bound is.}
% %\vspace*{-3mm}
% \label{fig:noisy_signsgd}
% \end{figure*}

\begin{figure}[t!]
    \centering
      \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
      \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a-new.png}} 
      \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a-new.png}}
    %\vspace*{-4mm}
    \caption[]{Comparison of the squared gradient norm \cite{Li2020On}, the gradient incoherence \cite{negrea2019information}, the two-sample incoherence \cite{rodriguez2021random}, and the gradient discrepancy in our bound. Incoherence or discrepancy based quantities are orders of magnitude smaller than the gradient norm. }
    \label{fig:sgld_key_quantities}
    %\vspace*{-5mm}
\end{figure}

\subsection{Stochastic Gradient Langevin Dynamics}
%\vspace*{-2mm}
\noindent \textbf{Comparison with existing work.} We have derived generalization error bounds that depend on the data-dependent \emph{gradient discrepancy}, i.e., $\left\|\nabla \ell\left(\w_{t}, z_n \right)  -  \nabla \ell\left(\w_{t}, z'_n\right)\right\|_{2}^{2}$. Existing bounds in \citet{Li2020On} and \citet{negrea2019information} have also improved the Lipschitz constant in \citet{mou2018generalization} to a data-dependent quantity. All these generalization error bounds can be added to the empirical training error to get bounds on the empirical test error. As shown in Figure~\ref{fig:sgld_bound} (a)-(d), our bound is able to generate a much tighter upper bound on the test error. The improvements is mainly due to the fact that we replace the squared \emph{gradient norm} in \citet{Li2020On}, the squared norm of \emph{gradient incoherence}
in  \citet{negrea2019information}, and that of \emph{two-sample incoherence} in \citet{rodriguez2021random} with the gradient discrepancy while maintaining a $1/n$ sample dependence. Figure~\ref{fig:sgld_bound} (e)-(h) shows that our bounds are much sharper than those of \citet{Li2020On} because our gradient discrepancy norms (Figure~\ref{fig:sgld_key_quantities}) are usually 2-4 order of magnitude smaller than the squared gradient norms in \citet{Li2020On}. Our bounds are also sharper than those of \citet{negrea2019information} and \citet{rodriguez2021random} due to our $O(1/n)$ sample dependence compared to their $O(1/\sqrt{n})$ dependence. Although the gradient incoherence in \citet{negrea2019information} is can be about 1 to 2 order of magnitude smaller than the gradient discrepancy for simple problems such as MNIST (Figure~\ref{fig:sgld_key_quantities}(a)), the difference between the gradient incoherence and our gradient discrepancy reduces as the problem becomes harder (see results for CIFAR-10 in Figure~\ref{fig:sgld_key_quantities}(b)).







\begin{figure}[t] 
\centering
%\subfigure[CNN, MNIST, SGLD, $\alpha_t=0.2$, $\sigma_t=\alpha_t\eta_t \approx 10^{-4}$]{\includegraphics[width=0.95\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2.png}}
\subfigure[Training Error]{
\includegraphics[width=0.21\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-c.png}
 }
\subfigure[Gradient Discrepancy]{
\includegraphics[width=0.21\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-a.png}
 }\vspace*{-2mm}
\subfigure[Generalization Bound]{
\includegraphics[width=0.21\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-b.png}
 }
\subfigure[Test Error Bound]{
\includegraphics[width=0.21\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-d.png}
 }  
%\vspace*{-4mm}
\caption[]{Results for training CNN using SGLD on a subset of MNIST ($n=10000$) with different label randomness.(a) Training error: While training takes more epochs with random labels, training error does go to zero. (b) Gradient discrepancy: As the randomness increases, so does the gradient discrepancy, %$\left\|\nabla \ell\left(\w_t, z_n \right)-\nabla \ell\left(\w_t, z'_n\right)\right\|_{2}^{2}$, 
leading to the increase in the generalization bound. (c) Generalization bound: As the randomness increases, so does the generalization bound in Theorem \ref{theo:efldstab}. (d) Test error and bound: As the randomness increases, the empirical test error (dashed lines) increases and so does the test error bound (solid lines); overall, the bounds stay valid.
}
%\vspace{-5mm}
\label{fig:bound_random}
\end{figure}







\noindent \textbf{Effect of Random Labels.} Motivated by \citet{zhang2017understanding}, we train CNN with SGLD on a smaller subset of MNIST dataset ($n=10,000$) with randomly corrupted labels. The corruption fraction varies from $0\%$ (no label corruption) to $60\%$. As shown in Figure~\ref{fig:bound_random} (a), for long enough training time, all experiments with different levels of label randomness can achieve almost zero training error. However, increase in random labels leads to increase in gradient discrepancy (Figure~\ref{fig:bound_random}(b)) which in turn leads to increase in the generalization bound (Figure~\ref{fig:bound_random}(c)). 
%
% Our generalization bound also becomes larger as the randomness increases since the corresponding gradient discrepancy increases.
%
As a result, as the empirical error rate increases with increase in label randomness (Figure \ref{fig:bound_random}(d) dashed lines), we get the correct increase in the test error bound  (solid lines).


\begin{figure}[t] 
\centering
\subfigure[CNN, MNIST]{
 \includegraphics[width=0.21\textwidth]{ICLR2022/images/cnn1-mnist-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 } 
  \subfigure[CNN, Fashion]{
 \includegraphics[width=0.21\textwidth]{ICLR2022/images/cnn1-fashion-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }\vspace{-2mm}
\subfigure[CNN, MNIST, $\alpha_t=1$]{
 \includegraphics[width=0.21\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
 } 
 \subfigure[CNN, Fashion, $\alpha_t=1$]{
 \includegraphics[width=0.21\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
 }
%\vspace*{-4mm}
\caption[]{(a)-(b) show the training dynamics of CNN on MNIST and Fashion-MNIST using noisy sign-SGD with different scaling $\alpha_t$. Legends indicate the choice of $\alpha_t$ and the numbers in brackets are test errors at convergence. As $\alpha_t\to 0$, Nosiy sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original sign-SGD \citep{bernstein2018signsgd}. (c)-(d) show that empirical test error can be bounded by our bound and the corresponding training error.}
%\vspace{-5mm}
\label{fig:noisy_signsgd}
\end{figure}


\subsection{Noisy Sign-SGD}
In this section, we present numerical results for Noisy Sign-SGD proposed in section~\ref{subsec:efld}. %Example \ref{exam:noisy_signsgd}.  
Since none of the existing bounds can give a valid generalization bound for Noisy Sign-SGD, we only present our bound here.

\noindent \textbf{Optimization.} Figure~\ref{fig:noisy_signsgd} (a)-(b) show the training dynamics of Noisy Sign-SGD under various choices of $\alpha_t$. For small $\alpha_t$, Noisy Sign-SGD matches both the optimization trajectory as well as the test accuracy of the original Sign-SGD \citep{bernstein2018signsgd}. However, as $\alpha_t$ increases, the distribution over $\{-1,+1\}$ is more spread out and the corresponding Noisy Sign-SGD seems to converge but to a sub-optimal value. 

\noindent \textbf{Generalization Bound.} Figure \ref{fig:noisy_signsgd}(c)-(d) show that our bound successfully bounds the empirical test error.
%and the corresponding training error. 
Larger $\alpha_t$ leads to sharper generalization bounds. However, larger $\alpha_t$ adversely affects the optimization, e.g., Figure~\ref{fig:noisy_signsgd} (a)-(b) blue and orange lines. The results illustrate the trade-off between the empirical optimization and the generalization bound. In practice, one needs to balance the optimization error and generalization by choosing a suitable scaling $\alpha_t$.

















%Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to those for CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases, leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence. 

%We note that  \cite{haghifam2020sharpened} show that Negrea et al. bound is smaller than Li et al. in their empirical evaluation, which is opposite to what we observed in Figure \ref{fig:mnist}.We think this is because \cite{haghifam2020sharpened} consider the full-batch setting which has a different form of gradient incoherence compared to the mini-batch setting in our paper. \yzcomment{added the discussion about the inconsistent of our result and \cite{haghifam2020sharpened}}


% The second key difference is the order of dependence on the sample size $n$, i.e., both of our bound and $\cite{Li2020On}$ has a bound of order $\frac{1}{n}$, however, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$. 
%Figure \ref{fig:mnist} (a) and 
% (b) suggests that the gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors, and the gradient incoherence in \cite{negrea2019information} is much smaller than the gradient discrepancy in our bound as well.
% However, the results in (b-d) for MNIST and (f-h) for Fashion MNIST show that our bounds are much sharper than those of \cite{negrea2019information} due to improving the dependence on $n$ from a order of $\frac{1}{\sqrt{n}}$ to $\frac{1}{n}$. Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence.


%More details of our model architectures and addtional experimental results can be found in Appendix. We acknowledge that we did not aim to achieve the state-of-the art predictive performance. With further tuning, the prediction results could be improved








% \begin{figure*}[t] 
% \centering
% \includegraphics[ width=0.5\textwidth]{ICLR2022/images/vgg5-mnist-n1000-bs100-BernoulliSGD-train-dynamics.png}
% \caption[]{Training dynamics of Noisy SignSGD with Bernoulli noise with various selection of $\alpha$ for VGG5 trained on MNIST.When $\alpha \to 0$, Bernoulli SignSGD reduces to SignSGD. As a results, Bernoulli SignSGD with small enough $\alpha$ matches the training trajectory of SignSGD.
% } 
% \label{fig:mnist}
% \end{figure*}

% \textbf{To Do List}

% The following experiments follow the setting described in  \cite{negrea2019information}. \textbf{[By the end of this week (September 19)]}
% \begin{enumerate}
%     \item CNN (two convolutional layers + two fully connected layers) on MNIST and Fashion MNIST
%     \item CNN (two convolutional layers + three fully connected layers) on CIFAR-10
% \end{enumerate}

% The following experiments follow the standard setting most DL papers likely to perform. \textbf{[Before next Wednesday (September 22)]}
% \begin{enumerate}
%     \item VGG5 on MNIST and Fashion MNIST
%     \item ResNet-18 on CIFAR-10 and CIFAR-100
% \end{enumerate}



% \textbf{To Plot}
% \begin{enumerate}
%     \item Gradient norms \citep{Li2020On}
%     \item Gradient incoherence \citep{negrea2019information}
%     \item Gradient discrepancy $\| \mathbf{\theta}_{B,\alpha} - \mathbf{\theta}_{B',\alpha} \|_2^2$ (our bound)
%     \item Our bound, Negrea's bound, and Li et al., bound.
% \end{enumerate}

% \newpage

% \begin{table}
%   \caption{Summary of Experiments for SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $\beta_t$ & Our bound & Li bound & Negrea Bound \\
%     \midrule
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.96 & 55000 & $\checkmark$ & $\checkmark$ & $\checkmark$   \\
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.96 & 5000 & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
%     CNN-1 & Fashion  & $4\times 10^{-3}$ & 0.93 & 55000 & $\checkmark$ & $\checkmark$ & $\checkmark$  \\
%     CNN-1 & Fashion & $4\times 10^{-3}$ & 0.93 & 5000 & $\checkmark$ & $\checkmark$ &$\checkmark$  \\
%     \midrule
%     CNN-2 & CIFAR-10  & $5\times 10^{-3}$ & 0.95 & 55000 &  &  &   \\
%     CNN-2 & CIFAR-10  & $5\times 10^{-3}$ & 0.95 & 5000 &  &  &  \\
%   \midrule
%   ResNet-18/50 & Mini ImageNet & ? & ?&? & & &\\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for Noisy SGD with Gaussian Noise ($\sigma_t=c\eta_t$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $c$ & Our bound & Li bound & Negrea Bound \\
%     \midrule
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.995 & 0.002 &$\checkmark$  & $\checkmark$ &   \\
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.95 & 0.2 &$\checkmark$  &$\checkmark$  &  \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$) with pretrain ($|J_0|=m$)}
%   \label{tab:sgld_pretrain}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & m &$\eta_0$& decay & $\beta_t$ & Our bound\\
%     \midrule
%     CNN-1 & MNIST  & 100 & $4\times 10^{-3}$ & 0.96 & 55000 &   \\
%     CNN-1 & MNIST  & 1000 & $4\times 10^{-3}$ & 0.96 & 55000 &   \\
%     CNN-1 & MNIST  & 10000 & $4\times 10^{-3}$ & 0.96 & 55000 &    \\
%     CNN-1 & MNIST  & 50000 & $4\times 10^{-3}$ & 0.96 & 55000 &    \\
%     \midrule
%     CNN-1 & Fashion & 100 & $4\times 10^{-3}$ & 0.93 & 55000 &   \\
%     CNN-1 & Fashion & 1000 & $4\times 10^{-3}$ & 0.93 & 55000 &    \\
%     CNN-1 & Fashion & 10000 & $4\times 10^{-3}$ & 0.93 & 55000 &    \\
%     CNN-1 & Fashion & 50000 & $4\times 10^{-3}$ & 0.93 & 55000 &   \\
%     \bottomrule
%   \end{tabular}
% \end{table}



% \begin{table}
%   \caption{Summary of Experiments for Random Labels with SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & Randomness & $\eta_0$& decay & $\beta_t$ & Our bound  \\
%     \midrule
%     CNN-1 & MNIST  &0 &$4\times 10^{-3}$ & 0.96 & 55000 & $\checkmark$  \\
%     CNN-1 & MNIST  &10\% &? & ? & ? & \\
%     CNN-1 & MNIST & 20\% &? & ? & ? & \\
%     CNN-1 & MNIST & 50\% &? & ? & ? & \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for Noisy SGD with Bernoulli Noise ($\mu_{\alpha} = \frac{1}{1+\exp(-\theta/\alpha})$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $\alpha_t$ & Our bound \\
%     \midrule
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-6}$ &   \\
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-2}$ &  \\
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-1}$ &  \\
%     CNN-1 & Fashion  & $10^{-4}$ & 0.1 & $10^{-6}$ &     \\
%     CNN-1 & Fashion & $10^{-4}$ & 0.1 & $10^{-2}$&   \\
%     CNN-1 & Fashion & $10^{-4}$ & 0.1 & $10^{-1}$&   \\
%     \midrule
%     CNN-2 & CIFAR-10  & $10^{-3}$ &0.1  & $10^{-6}$ &   \\
%     CNN-2 & CIFAR-10  & $10^{-3}$ & 0.1 & $10^{-2}$ &  \\
%     CNN-1 & CIFAR-10  & $10^{-3}$ &0.1  & $10^{-1}$ &  \\
%   \midrule
%   ResNet-18/50 & Mini ImageNet & ? & ?&? & \\
%     \bottomrule
%   \end{tabular}
% \end{table}



==> ICML2022/sec/exp_stability.tex <==
In the setting of statistical learning, there is an instance space $\cZ$, a hypothesis space $\cW$, and a loss function $\ell : \cW \times \cZ \mapsto \R_+$. Let $D$ be an unknown distribution of $\cZ$ and let $S_n \sim D^n$ be $n$ i.i.d.~draws from $D$. For any specific hypothesis $\w \in \cW$, the population and empirical loss are respectively given by
%\vspace*{-3mm}
%\begin{equation}
$L_D(\w) \triangleq \E_{z \sim D}[\ell(\w,z)]$, and $L_S(\w) \triangleq \frac{1}{n} \sum_{i=1}^n \ell(\w,z_i)$.  
%\vspace*{-3mm}
%\end{equation}
For any distribution $P$ over the hypothesis space, we respectively denote the expected population and empirical loss as
%\vspace*{-3mm}
%\begin{equation}
$L_D(P) \triangleq \E_{z \sim D}\E_{\w \sim P}[\ell(\w,z)]~, \quad \text{and} \quad  L_S(P) \triangleq \frac{1}{n} \sum_{i=1}^n \E_{\w \sim P}[\ell(\w,z_i)]$.
%\vspace*{-3mm}
%\end{equation}
We consider a randomized algorithm $A$ which works with $S_n =\{z_1,\ldots,z_n\} \sim D^n$ and creates a distribution over the hypothesis space $\cW$. For convenience, we will denote the distribution as $A(S_n)$. The focus of our analysis is to bound the generalization error of $A$ defined as: 
%$\gen(A(S)) \triangleq L_D(A(S)) - L_S(A(S))~.  $
% \vspace{-3mm}
% \begin{align}
$\gen(A(S_n)) \triangleq L_D(A(S_n)) - L_S(A(S_n))$. 
% \vspace*{-2mm}
% \end{align} 
We will assume $A$ is permutation invariant, i.e., the ordering of samples in $S_n$ do not modify $A(S_n)$, an assumption satisfied by most learning algorithms. %\abdelete{We will focus on developing bounds for the expectation $\E_{S_n}[L_D(A(S_n)) - L_S(A(S_n))]$, and discuss high-probability bounds in the Appendix.} 
All technical proofs for results in this section are in Appendix~\ref{sec:app_exp_stability}.



\subsection{Bounds based on Expected Stability}
We start our analysis by noting that the expected generalization error can be upper bounded by {\em expected stability} based on the Hellinger divergence $H(P \| P')$ between two distributions given by~\citep{save16,Li2020On}: $H^2(P\| P') = \frac{1}{2}\int_{\w} (\sqrt{p(\w)} - \sqrt{p'(\w)})^2 d\w$.
\begin{restatable}{prop}{prophell}
Let $S_n \sim D^n$ and let $S'_{n}$ be a dataset obtained by replacing $z_n \in S_n$ with $z'_n \sim D$. Let $A(S_n),A(S'_{n})$ respectively denote the distributions over the hypothesis space $\cW$ obtained by running randomized algorithm $A$ on $S_n,S'_{n}$.
Assume that for all $S_n \in \cZ^n, z \in \cZ$, $\E_{W \sim  A(S_n)}[\ell^2(W,z)] \leq c^2_0/4$ for some constant $c_0>0$.  With $H(\cdot,\cdot)$ denoting the Hellinger divergence, we have
\begin{equation}
\begin{aligned}
&| \E_{S_n \sim D^n}[L_D(A(S_n)) - L_S(A(S_n))] |\\
&\leq c_0 \E_{S_n \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S_n), A(S'_{n})\big)}~. 
\end{aligned}
\end{equation}
%\vspace*{-3mm}
\label{prop:hell}
\end{restatable}
\begin{remark}
Proposition~\ref{prop:hell} does not need bounded losses. The {\em second moment} of $\ell(W,z), W \sim A(S_n), \forall S_n, z$ need to be bounded. In comparison, recent information theoretic bounds~\citep{haghifam2020sharpened,xu2017information} assume $\ell(\w,Z), Z \sim D, \forall \w \in \cW$ to be {\em sub-Gaussian}. \qed 
\end{remark}
\begin{remark}
The bound in Proposition~\ref{prop:hell} is in terms of {\em expected stability} where we consider $\E_{S_n \sim D^n} \E_{z'_n \sim D}[\cdots]$, an important departure from bounds based on {\em uniform stability} \citep{elisseeff2005stability, bousquet2002stability, mou2018generalization,bousquet2020sharper}
%feldman2018generalization,feldman2019high} 
where one considers $\sup_{S_n,S_n' \in \cZ^n, |S_n \Delta S_n'| = 1}[\cdots]$. 
Replacing $\sup$ by $\E$ makes the bounds distribution dependent, avoids the worst case analysis associated with uniform stability, and arguably leads to quantitatively tighter bounds. \qed 
\end{remark}


\subsection{Expected Stability of Noisy Iterative Algorithms}
\label{sec: exp_stab_nsi}
We consider a general family of noisy stochastic iterative (NSI) algorithms. Given $S_n \sim D^n$, such iterative algorithms have two (additional) sources of randomness in each iteration $t$: (a) a stochastic mini-batch of samples $S_{B_t}$, with $|S_{B_t}| = b \leq n$, drawn uniformly at random with replacement from $S_n$; and (b) noise $\bxi_t$ suitably included in the iterative update. 
Given a trajectory (realization) of past iterates $W_{0:(t-1)} = \w_{0:(t-1)}$, the new iterate $W_t$ is drawn from a distribution $P_{B_t,\bxi_t|\w_{0:(t-1)}}$ over $\cW$:
%\vspace*{-2mm}
\begin{align}
\label{eq:nmia}
%\vspace{-2mm}
W_{t} \sim P_{B_t,\bxi_t|\w_{0:(t-1)}}(W) ~.
%\vspace{-2mm}
\end{align}
%for some suitable function $f_t$. 
We will often drop conditioning $\w_{0:(t-1)}$ to avoid clutter. % in the sequel.

Let $\bar{S}_{n+1} \sim D^{n+1}$ with $\bar{S}_{n+1} = \{z_1,\ldots,z_{n+1}\}$. Let $S_0 = \{z_1,\ldots,z_{n-1}\}$. $S_n,S'_{n}$ are size $n$ subsets of $\bar{S}_{n+1}$ with $S_n= S_0 \cup \{z_n\}$ and $S'_{n} = S_0 \cup \{z'_n\}$, where $z'_n = z_{n+1}$. 
The algorithms we consider use a mini-batch of size $b$ in each iteration uniformly sampled from $S_n$ or $S'_n$. Let $G, G_0, G_1$ respectively denote the set of all mini-batches of size $b$ drawn from $\bar{S}_{n+1}$, the set only drawn from $S_0$, and the set which includes the last sample, viz.~$z_n$ for $S_n$ and $z'_n$ for $S'_n$.
Note that $|G_0| = \binom{n-1}{b}$, $|G_1| = \binom{n-1}{b-1}$, and 
$|G_0| + |G_1| = \binom{n-1}{b} + \binom{n-1}{b-1} = \binom{n}{b} = |G|$.


Based on \eqref{eq:nmia}, let $P_{0:(t-1)}$ denote the joint distribution over $W_{0:(t-1)} = (W_0,\ldots,W_{t-1})$, and 
let $P_{t|} := P_{B_t,\bxi_t|\w_{0:(t-1)}}$ compactly denote the conditional distribution on $W_t$. 
Let $P_T, P'_T$ denote the marginal distributions over hypotheses $\w \in \cW$ after $T$ steps of the algorithm based on $S_n,S'_{n}$ respectively. For randomized algorithms of the form \eqref{eq:nmia}, from Proposition \ref{prop:hell} we first bound the Hellinger divergence with KL-divergence, i.e., $2H^2(P_T,P'_T) \leq KL(P_T,P'_T)$ (Proposition~\ref{prop:hellkl} in Appendix~\ref{sec:app_exp_stability}), and then 
use the following chain rule \citep{pensia2018generalization,negrea2019information,haghifam2020sharpened} to bound the KL-divergence between $P_T$ and $P'_T$:
$KL(P_T \| P'_T) \leq KL(P_{0:T} \| P'_{0:T} ) = \sum_{t=1}^T \E_{P_{0:(t-1)}}\left[ KL(P_{t|} \| P'_{t|}) \right]$.
%
%Following \cite{Li2020On}, 
We can bound the per-step conditional KL-divergences $KL(P_{t|} \| P'_{t|})$ 
%in the right-hand-side of \eqref{eq:klchain} 
in terms of a Le Cam Style Divergence (LSD). While the classical Le Cam divergence~\citep{save16} is $LSD(P\|P') \triangleq \frac{1}{2} \int \frac{(dP - dP')^2}{dP + dP'}$ (where $dP$ denotes the density), our bounds are in terms of
%\vspace*{-2mm}
\begin{equation}
\begin{split}
\label{eq:lsd}
&LSD(P_{t|}| \| P'_{t|})  := \underset{B_t \in G_1}{\E} \underset{A_t \in G_0}{\E}  \left[ \Lambda(B_t,A_t) \right]~, \\
&\Lambda(B_t,A_t)  := \int_{\bxi_t} \frac{(dP_{B_t,\bxi_t} - dP'_{B_t,\bxi_t})^2}{dP_{A_t,\bxi_t}} d \bxi_t ~.
\end{split}
%\vspace*{-2mm}
\end{equation}
%where $B_t \in G_1, A_t \in G_0$.
Note that $P_{B_t,\bxi_t}$ and $P'_{B_t,\bxi_t}$ represent the conditional distribution of $W_t$ for $S_n$ and $S_n^\prime$ respectively since the mini-batch $S_{B_t}$ of $S_n$ and $S_n^\prime$ differs in the $n$-th sample. 
%Putting Propositions~\ref{prop:hell} and \ref{prop:hellkl}, and \eqref{eq:klchain} together, with some additional analysis 
%Bounding the KL-divergences in \eqref{eq:klchain} with LSDs, 
Then, we have the following LSD based generalization bound.
\begin{restatable}{lemm}{theostab}
In the setting of Proposition~\ref{prop:hell} consider a noisy stochastic iterative algorithms of the form~\eqref{eq:nmia} with mini-batch size $b \leq n/2$. Then, with $c_1 = \sqrt{2} c_0$ (with $c_0$ as in Proposition~\ref{prop:hell}) and $\Lambda(B_t,A_t)$ as in \eqref{eq:lsd}, we have
%\vspace*{-1mm}
\begin{equation}
%\hspace*{-5mm}
\begin{aligned}
&| \E_{S_n}[L_D(A(S_n)) - L_{S}(A(S_n))] |\\
&\leq c_1 \frac{b}{n} \E_{S_n} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \underset{B_t \in G_1}{\E} \underset{A_t \in G_0}{\E} \left[ \Lambda(B_t,A_t) \right] }~.
\end{aligned}
\end{equation}
\label{theo:stab}
%\vspace*{-5mm}
\end{restatable}
\begin{remark}
Though not stated explicitly, \citet{Li2020On} essentially has this result for SGLD and inspired our work. Our proofs are significantly simpler, does not make any additional assumptions, and illustrates applicability to general noisy iterative algorithms of the form~\eqref{eq:nmia}. \qed
% not just SGLD with Gaussian noise as in \cite{Li2020On}. \qed 
\end{remark}
\begin{remark}
The bound depends on expectations over samples $S_n,z'_n$, trajectories $W_{0:(t-1)}$, and mini-batches $B_t,A_t$. Unlike uniform stability and other worst case analysis, there is no $\sup$ over samples, trajectories, or mini-batches. \qed 
%Further, 
%the bound depends on the distribution discrepancy as captured by the expected LSD. \qed 
\end{remark}
\begin{remark}
The bound seems to worsen with $b$, the size of the mini-batch. As we show in Section~\ref{sec:efld}, the LSD terms have a $\frac{1}{b^2}$ dependence for SGLD and its generalizations we introduce, so the leading $b$ is neutralized. \qed 
\end{remark}
\begin{remark}
A high probability version of the result based on an exponential version of the Efron-Stein inequality~\cite{boucheron2013concentration} is presented in Appendix~\ref{ssec:highp}.
\end{remark}

% \begin{remark}
% Check what happens when the r.v.~is discrete, e.g., Bernoulli. Does the transition to Hellinger, then to KL, and then to LSD go through without any issues? Current analysis assumes Lebesgue measure, need to check validity for counting measure.
% \end{remark}


==> ICML2022/sec/intro.tex <==


Recent years have seen renewed interest in characterizing generalization performance of learning algorithms in terms of stability which considers change in performance of a learning algorithm based on change of a single training point \citep{hardt2016train,bousquet2002stability,Li2020On,mou2018generalization}. 
For stochastic gradient descent (SGD), \citet{hardt2016train} established generalization bounds based on uniform stability \citep{bousquet2002stability}, although the analysis needed rather small step sizes $\eta_t = 1/t$ which is arguably not useful in practice. While improving the stability analysis for SGD has remained a challenge, advances have been made on noisy SGD algorithms, especially stochastic gradient Langevin dynamics (SGLD) \citep{WellingT11, mou2018generalization,Li2020On} which adds Gaussian noise to the stochastic gradients. In parallel, there has been key developments on related information-theoretic generalization bounds applicable to SGLD type algorithms \citep{negrea2019information,haghifam2020sharpened,xu2017information,russo2016controlling, pensia2018generalization, wang2021analyzing}.

While these developments have led to advances in analyzing generalization of noisy SGD algorithms, and we elaborate on these developments in Appendix \ref{sec:related_work}, they each have certain limitations, e.g., dependence on global Lipschitz constant $L$ \citep{mou2018generalization}, tiny $O(1/L)$ step sizes \citep{Li2020On}, $O(1/\sqrt{n})$ sample dependence \citep{mou2018generalization,negrea2019information}, dependence on gradient norms \citep{Li2020On}, restrictions on nature of mini-batching \citep{wang2021analyzing}, etc. Further, most prior work primarily focuses on SGLD and cannot be readily extended to popular variants such as noisy versions of Sign-SGD or quantized SGD \citep{bernstein2018signsgd,quantized-sgd,jiang2018}.
% \abbcomment{the following discussion is good, but really long -- can we move this to the Appendix, commenting out for now} 
%
% \abbdelete{\citet{mou2018generalization} considered SGLD with marginal Gaussian noise variance $\sigma_t$ and step size $\eta_t \leq {\sigma_t \ln 2}/{L}$, where $L$ is the global Lipschitz constant for the loss,  and established a generalization bound for SGLD of the form $\frac{L}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ using uniform stability.
% The bound has a desirable dependency of $O({1}/{n})$ on the samples, but has an undesirable dependence on $L$, and the step sizes, bounded by $O({\sigma_t}/{L})$, are arguably too small. \citet{mou2018generalization} also presented another bound which addresses some of these issues, but yields an undesirable $O({1}/{\sqrt{n}})$ sample dependence.  By building on the developments of \citet{russo2016controlling,xu2017information,pensia2018generalization}, \citet{negrea2019information} made advances from the information theoretic perspective and established bounds for SGLD which have a desirable dependence on the norm of gradient incoherence, i.e., a suitable difference in gradients over different mini-batches, avoids dependence on $L$, is applicable to unbounded sub-Gaussian losses, but have an undesirable $O({1}/{\sqrt{n}})$ sample dependence. \citet{haghifam2020sharpened} made further advances on the problem from an information theoretic perspective based on the conditional mutual information framework of~\citet{steinke2020reasoning} and obtained generalization bounds based on gradient incoherence with $O({1}/{n})$ sample dependence for full batch Langevin dynamics, which was later extended by \citet{rodriguez2021random} to SGLD with a time-decaying factor in their bounds. Recently, \citet{wang2021analyzing} provided a generalization bound for SGLD that incorporates the variance of gradients evaluated on the training data and has $O(1/n)$ sample dependence.
% \yzcomment{\citet{wang2021analyzing} bound is of the from $O(\frac{b}{n}\sum_{j=1}^m\sqrt{\sum_{t\in {\cT}_j}\eta_t^2\textit{Var}(\mathbf{g}_j(t))/\sigma_t^2})$, where $b$ is the mini-batch size, $m$ is the number of mini-batches,  ${\cT}_j$ contains the indices of iterations for mini-batch $S_j$ and $\textit{Var}(\mathbf{g}_j(t))$ is the gradient variance evaluated on the training set. Overall, their bound looks pretty good to me. The only weakness I can think is the sum of the square root is larger than the square root of the sum. Thus, it is obvious that their bound becomes $T/n$ for $b=1$, $m = T$}  However, \citet{wang2021analyzing} requires splitting the training samples into disjoint $m$ mini-batches before training and obtained a bound $O(m/n)$. \abcomment{how is it $O(m/n)$? is $m b = n$?} Their bound also scales inversely to the batch size since the number of mini-batches $m$ and gradient variance increase as the batch size decreases. 
% \citet{Li2020On} made advances on such bounds based on the notion of Bayes-stability, by combining ideas from PAC-Bayes bounds into stability, and established a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \mathbf{g}_e(t)/\sigma_t^2}$ for bounded losses, where $\mathbf{g}_e(t)$ is the expected gradient norm square at step $t$. While the bound has a desirable sample dependence of $O(1/n)$ and avoids dependence on the Lipschitz constant $K$, the dependence on the gradient norm makes such bounds much weaker than the information theoretic bounds of \citet{negrea2019information,haghifam2020sharpened, rodriguez2021random} which depend on the norm of gradient incoherence which are typically orders of magnitude smaller. Further, the analysis of \cite{Li2020On} still needs small step sizes, bounded by $O({\sigma_t}/{L})$. \citet{farghly2021timeindependent} provided a time-independent bound for SGLD of the form $O(1/n + \eta^{1/2}d^{1/2})$ which requires the step size scales as $O(1/(n^2d))$ to obtain an $O(1/n)$ bound.}
%
%
In this paper, we build on the core strengths of such existing approaches, most notably (a) the $O({1}/{n})$ sample dependence of stability based bounds~\citep{mou2018generalization,Li2020On}, (b) the dependence on
%the norm of 
some measures of gradient discrepancy rather than the norm of gradients~\citep{negrea2019information,haghifam2020sharpened}, and (c) no dependence on the global Lipschitz constant $L$, and develop a framework (Section~\ref{sec:exp_stability}) for establishing generalization bounds for a general family of noisy stochastic iterative algorithms which includes SGLD as a special case. Our framework considers generalization based on the concept of {\em expected stability}, rather than uniform stability \citep{hardt2016train,bousquet2002stability, bousquet2020sharper,mou2018generalization,farghly2021timeindependent}, and yields distribution dependent generalization bounds which avoid the worst-case setting of uniform stability. Recall that for any data domain $\cZ$ and a distribution $D$ over the domain, uniform stability considers the worst case difference in loss over two datasets $S_n,S'_n \in \cZ^n$ of size $n$ which differ by one point, i.e., over $\sup_{S_n, S'_n, |S_n \Delta S'_n|=1} \cdots$ \citep{bousquet2002stability,hardt2016train}. In Section~\ref{sec:exp_stability}, we show that one gets a valid generalization bound for stochastic algorithms  by replacing the supremum $\sup$ by an expectation $\E_{S_n,S'_n}$, where $S_n \sim D^n$ and, without loss of generality, $S'_n$ shares the first $(n-1)$ samples with $S_n$ with the $n$-th sample $z'_n \sim D$. Replacing $\sup$ by $\E$ makes the bound distribution dependent
%, avoids the worst case analysis associated with uniform stability, 
and arguably leads to quantitatively sharper and computable bounds with less assumptions. %Building on some analyses in \cite{Li2020On}, 
Further, we show that expected stability of general noisy stochastic iterative algorithms
%, not just noisy SGD, 
can be bounded by the expectation of a Le Cam Style Divergence (LSD) between  distributions over parameters obtained from $S_n$ and $S'_n$. Thus, getting an expected stability based generalization bound for a specific stochastic algorithm reduces to that of bounding the expected LSD.

In Section~\ref{sec:efld}, we introduce Exponential Family Langevin Dynamics (EFLD), a family of noisy stochastic gradient descent algorithms based on exponential family noise. Special cases of EFLD include SGLD and noisy versions of Sign-SGD or quantized SGD algorithms~\citep{bernstein2018signsgd, bernstein2018signsgdnoise, jin2020stochastic, quantized-sgd}. Our main result provides an expected stability based generalization bound for {\em any} EFLD algorithm with several aforementioned desirable properties: (a) a $O({1}/{n})$ sample dependence, (b) a dependence on the gradient discrepancy, a variant of gradient incoherence~\citep{negrea2019information}, rather than a dependence on the norm of gradients, (c) no dependence on the global Lipschitz constant $L$, and (d) step sizes $\eta_t$ need not be tiny, i.e., $\eta_t = O(1/L)$ is not needed. Existing generalization bounds for SGLD~\citep{Li2020On,negrea2019information} usually use properties of the Gaussian distribution, and do not generalize to EFLD. Our proof technique is new, and uses properties of exponential family distributions. 
%
%\abdelete{For the special case of SGLD, our bounds turn out to be tighter than existing bounds~\cite{negrea2019information,Li2020On}. }
We also provide optimization guarantees for EFLD, i.e., convergence results for noisy Sign-SGD and 
%revisit convergence of 
SGLD.
%\abdelete{based on skewed Rademacher noise over $\{-1,+1\}$ where the noise parameters depend on the stochastic gradients. The analysis for SGLD is a variant of existing analyses whereas the analysis for noisy sign-SGD based on gradient dependent Rademacher noise is new.} 
%and the first convergence result for the algorithm to the best of our knowledge. 

In Section~\ref{sec:exp}, we present experimental results on benchmark datasets. We illustrate that our bounds for SGLD are non-vacuous and quantitatively tighter than existing bounds~\citep{Li2020On,negrea2019information} due to the desirable dependence on sample size and gradient discrepancy norms, which are empirically shown to be orders of magnitude smaller than gradient norms. We also report results on random labels~\cite{zhang2017understanding} where as the training error goes to zero, our bound correctly captures the increase in generalization error due to increasing fraction of random labels. We also present results for Noisy Sign-SGD and illustrate that our bounds give a quantitatively tight upper bound on the empirical test error across epochs. %\abdelete{and the optimization performance is comparable to that of sign-SGD.}

%Our empirical results also illustrate a trade-off inherent in noisy gradient algorithms--a lower noise scale implies 

%Through experiments on benchmark datasets (), we illustrate that our bounds are non-vacuous and quantitatively much sharper than existing bounds.

%{\bf Related work.} Uniform stability has been a classical approach for bounding generalization error \citep{bousquet2002stability,bousquet2020sharper,feldman2018generalization,feldman2019high}, pioneered by \cite{rogers1978finite,devroye1979distribution}. Beyond the aforementioned work, there has been recent work on differential privacy that analyzes the uniform stability of differentially private SGD (DP-SGD) \citep{hardt2016train, bassily2020stability}. Beyond uniform stability, information-theoretic approaches \citep{russo2016controlling, xu2017information}  that bounds the generalization error by the mutual information between the algorithm input $S$ and the algorithm output $\w$, have been used for deriving generalization bounds for noisy iterative algorithms \citep{pensia2018generalization,bu2019tightening}. Along this line of literature, \cite{negrea2019information, haghifam2020sharpened, rodriguez2021random} prove  data-dependent generalization bounds dropping dependence on the Lipschitz constant. Further, tighter bounds \citep{haghifam2020sharpened, zhou2021individually, rodriguez2021random, neu2021informationtheoretic, hellstrom2021fast}  are proposed based on conditional mutual information \citep{steinke2020reasoning, grunwald2021pac, hellstrom2020generalization}. Due to space limitations, an extended discussion of the related work is deferred to Appendix~\ref{sec:related_work}. 



==> ICML2022/sec/related.tex <==

% \begin{itemize}
%     \item Generalization approaches (stability, information-theory bound, PAC Bayesian, Uniform Bound)
%     \item Noisy iterative algorithm (Sign SGD, SGLD, DP SGD etc)
%     \item More?
% \end{itemize}

% \textbf{(Old Materials)}]



\noindent \textbf{Uniform stability.} Uniform stability is a classical approach for bounding generalization error \citep{bousquet2002stability,hardt2016train,bousquet2020sharper, ShalevShwartz2009StochasticCO,feldman2018generalization,feldman2019high}, pioneered by \citet{rogers1978finite,devroye1979distribution}. Recently, uniform stability has been used in analyzing the  stability of stochastic gradient descent (SGD) \citep{hardt2016train}. 
\citet{mou2018generalization} prove the uniform stability of SGLD \citep{WellingT11, raginsky2017non} by showing that uniform stability can be bounded by the squared Hellinger distance, and further they establish discretized Fokker-Planck equations for analyzing the squared Hellinger distance. Then they provide uniform stability based generalization bounds for SGLD as $\frac{L}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ which depends on $L$, the global Lipschitz constant for gradients, and the step size $\eta_t \leq \frac{\sigma_t \ln 2}{L}$ \citep{mou2018generalization,Li2020On}. 
Recently, \citet{Li2020On} followed up on \citet{mou2018generalization} and derived a data-dependent bound based on Bayes-stability, and got a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \g_e(t)/\sigma_t^2}$, where $\g_e(t)$ is the expected gradient norm square at step $t$. Their bound improves the Lipschitz constant $L$ to the expected gradient norm square. Recently, \citet{farghly2021timeindependent} provided a time-independent bound for SGLD of the form $O(1/n + \eta^{1/2}d^{1/2})$ which requires the step size scales as $O(1/(n^2d))$ to obtain an $O(1/n)$ bound.  
\citet{bassily2019private} analyze the uniform stability of  differentially private SGD (DP-SGD) for convex optimization by showing the gradient update is a non-expansive operation, which is the key fact in proving the stability of SGD \citep{hardt2016train}. 
The approach in \citet{hardt2016train} can extend to non-convex setting as well, however it requires fast decaying in step size as $\eta_t = O(1/t)$.  \citet{bassily2020stability} provide stability analysis of SGD for convex and non-smooth functions. 

\noindent \textbf{Information-theoretic bounds.} Besides the works mentioned above, other theories of deriving generalization bounds for noisy iterative algorithms have been proposed via information-theoretic approaches \citep{russo2016controlling, xu2017information}. Such results show that the generalization error of any learning algorithm can be bounded as $O(\sqrt{I(S; W)/n})$, where $I(S; W)$ is the mutual information between the algorithm input $S$ and the algorithm output $W$. Recent work following this approach focus on bounding the mutual information for a broad class of iterative algorithms, including SGLD  to obtain a $O(\sqrt{\log T/n})$ generalization bound by choosing $\eta_t = O(1/t)$, where $T$ is the total number of iterations~\citep{pensia2018generalization,bu2019tightening}. Subsequent improvements to this technique were made by 
\citet{negrea2019information, haghifam2020sharpened, rodriguez2021random} 
to prove data-dependent generalization bounds that do not depend
on the Lipschitz constant of the loss function and obtain $\sqrt{\sum_t \eta_{t}/n} $ bounds. 
Especially, \citet{haghifam2020sharpened, zhou2021individually} introduce generalization bounds based on conditional mutual information inspired by \citet{steinke2020reasoning}, leading to tighter bounds than those based on mutual information, which was extended by \citet{rodriguez2021random} from full-batch gradient to stochastic setting. Recently, \citet{wang2021analyzing} provided a bound for SGLD of the from $O(\frac{b}{n}\sum_{j=1}^m\sqrt{\sum_{t\in {\cT}_j}\eta_t^2\textit{Var}(\mathbf{g}_j(t))/\sigma_t^2})$, where $b$ is the mini-batch size, $m$ is the number of mini-batches,  ${\cT}_j$ contains the indices of iterations for mini-batch $S_j$ and $\textit{Var}(\mathbf{g}_j(t))$ is the variance of mini-batch gradient on $S_j$ evaluated on the training set. However, \citet{wang2021analyzing} requires splitting training samples into disjoint $m$ mini-batches before training and obtained a bound dependending on the sum of gradient variance. Their bound also scales inversely to the batch size since the number of mini-batches $m$ and gradient variance increase as the batch size decreases. 
\citet{neu2021informationtheoretic} extend this information-theoretic approach  to derive generalization bound for vanilla SGD. \citet{hellstrom2021fast} provide a fast-rate bound for bounded loss functions based via Conditional Information Measures \citep{grunwald2021pac, hellstrom2020generalization}, which also provides a unified view of some of the above results.


%\textbf{PAC-Bayesian bound.} 

\noindent \textbf{Noisy iterative algorithms.} Introducing additional noise in the stochastic gradient has been popular in training deep nets. Noisy iterative methods have proven to be useful for machine learning applications, especially for deep neural networks in terms of escaping from saddle points \citep{jin2017escape,jin2019nonconvex}, preserving privacy  \citep{bassily2020stability,wang2019differentially}, boosting generalization and stability \citep{mou2018generalization,Li2020On}. SGLD \citep{WellingT11} has been one of the most popular noisy iterative algorithms for non-convex learning problems, where an isotropic Gaussian noise is added to the stochastic gradient. There has been some work \citep{wang2015privacy, li2019connecting} connecting SGLD with differentially private SGD  algorithm (DP-SGD) \citep{bassily2020stability,wang2019differentially} which usually adds noise with constant variance to the stochastic gradient. 
Uniform stability has also been popular in the differential privacy literature for analyzing the generalization error bound of DP-SGD algorithms. Recently, noise has been proven to be useful in Sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise, chen2019distributed} which has gained popularity as it reduces communication cost in distributed learning.  Existing versions of noisy sign-SGD first adds symmetric noise to the stochastic gradient, then take the sign of the noisy stochastic gradient to update the parameters \citep{chen2019distributed, jin2020stochastic}. \citet{bernstein2018signsgdnoise, chen2019distributed, jin2020stochastic} have shown that when noise is unimodal and symmetric, sign-SGD can guarantee convergence to stationary point.  Recently, \citet{wang2021optimizing} study the anisotropic noise for SGLD, where they optimize
the information-theoretical generalization bound by manipulating the noise structure in SGLD. They prove that with constraint to guarantee low empirical risk, the optimal noise covariance is the square root of the expected gradient covariance. In recent work, \citet{Lei2020} considered ``on average stability'' based generalization bounds, which is related to our work. Their bound has a dependence either on $L$ or on some form of convexity. 







==> ICML2022/sec/stability.tex <==
%\vspace*{-2mm} 

From Lemma~\ref{theo:stab}, conditioned on a trajectory $W_{0:(t-1)}=\w_{0:(t-1)}$, mini-batches $S_{B_t}, S_{A_t}$, %\yzcomment{sometimes, we use $S_{B_t}$ as mini-batch, sometimes we use $B_t$ as mini-batch. To be consistent, let’s use $S_{B_t}$ for mini-batch, and ${B_t}$ for indexes} 
we can get an expected stability based generalization bound by suitably bounding the expected LSD $\E[\Lambda(B_t,A_t)]$ as in \eqref{eq:lsd}.
% \begin{align}
% I_{A_t,B_t} = \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t~.
% \label{eq:plsd}
% \end{align}
For EFLD, %\abdelete{the density functions $dP_{B_t,\bxi_t},dP'_{B_t,\bxi_t}$ are exponential family densities $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t}), p_{\psi}(\bxi; \btheta'_{B_t,\alpha_t})$ as in \eqref{eq:efld1}-\eqref{eq:efld2}, and}
we have the following bound on the per step LSD $\Lambda(B_t,A_t)$.

\begin{restatable}{theo}{theoefld}
\label{theo:efld}
For a given set $\bar{S}_{n+1} \sim D^{n+1}$ and $\w_{t-1}$ at iteration $(t-1)$, let $\Delta_{t|\w_{t-1}}(\bar{S}_{n+1}) = \max_{z, z' \in  \bar{S}_{n+1}} \left\|\nabla \ell(\w_{t-1}, z\right) - \nabla \ell\left(\w_{t-1}, z')\right\|_{2}$. Further, for a $c_2$-smooth log-partition function $\psi$, let the scaling $\alpha_{t|\w_{t-1}}$ be data-dependent such that $\alpha_{t|\w_{t-1}}^2 \geq  8 c_2 \Delta_{t|\w_{t-1}}^{2}(\bar{S}_{n+1})$. Then, for $\Lambda(A_t, B_t)$ as in \eqref{eq:lsd} we have
%\abmargincomment{Two uses of $\Delta$ -- change one}
%\vspace*{-2mm} 
%{\small 
\begin{align*}
%\hspace*{-3mm} 
\Lambda & (A_t, B_t) \leq 5 c_2 \| \btheta_{B_t,\alpha_t} - \btheta_{B'_t,\alpha_t} \|_2^2 \\
& = \frac{5c_2}{2\alpha_{t|\w_{t-1}}^2} \left[\left\|\nabla \ell\left(\w_{t-1}, {S_{B_t}}\right)  -  \nabla \ell\left(\w_{t-1}, S'_{B_t}\right)\right\|_{2}^{2}\right]~.
\end{align*}
%}
%\vspace*{-3mm}
\end{restatable}
\begin{remark}
Theorem~\ref{theo:efld} shows that per step LSD $\Lambda(B_t,A_t)$ can be bounded by the (scaled) mini-batch gradient discrepancy. The result holds for {\em all} EFLD algorithms of the form \eqref{eq:efld1}-\eqref{eq:efld2}. \qed 
%not just Gaussian noise based SGLD. 
\end{remark}
\begin{remark}
Since $S_{B_t}$ and  $S'_{B_t}$ only differ at samples $z_n$ and $z'_n=z_{n+1}$, $\nabla \ell(\w_{t-1}, S_{B_t})  -  \nabla \ell(\w_{t-1}, S'_{B_t} ) = \frac{1}{b} (\nabla \ell (\w_{t-1}, z_n) - \nabla \ell(\w_{t-1},z'_n))$. The $1/b$ scale factor neutralizes the leading $b$ term in Lemma~\ref{theo:stab}. \qed 
 \end{remark}

Theorem~\ref{theo:efld} can now be directly applied to Lemma~\ref{theo:stab} to get expected stability based generalization bounds for EFLD.
\begin{restatable}{theo}{theoefldstab}
\label{theo:efldstab}
In the setting of Proposition~\ref{prop:hell} consider an exponential family Langevin dynamics (EFLD) algorithm of the form~\eqref{eq:efld1}-\eqref{eq:efld2} with a $c_2$-smooth log-partition function $\psi$.  Then, for mini-batch size $b \leq n/2$, with $c = c_0 \sqrt{5 c_2}$ (with $c_0$ as in Proposition~\ref{prop:hell}) and $\alpha_{t|}^2 \geq 8 c_2 \Delta_{t|}^2(\bar{S}_{n+1})$ (as in Theorem~\ref{theo:efld}, with the conditioning on $\w_{t-1}$ hidden to avoid clutter), we have
% \small
\begin{equation}
\begin{aligned}
&| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq  \\
&\frac{c}{n} ~\underset{\bar{S}_{n+1}}{\E} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E}  \frac{\left\|\nabla \ell\left(\w_{t-1}, {z_n} \right)  -  \nabla \ell\left(\w_{t-1}, {z'_n}\right)\right\|_{2}^{2}}{\alpha_{t|}^2}   }.
\end{aligned}
% \normalsize
\end{equation}
%\vspace*{-5mm}
\end{restatable}


\begin{remark}
The key term in the bound is the expected gradient discrepancy only on the sample $z_n, z'_n$ where $S_n,S'_n$ differ. Further, the only dependence on the specific exponential family is through the smoothness constant $c_2$. \qed 
\end{remark}


\begin{remark}
Since SGLD is a special case of EFLD, Theorem \ref{theo:efldstab} gives a generalization bound for SGLD.
The bound has effectively the same dependence on $n$ and $T$ as the bound in \citet{Li2020On}. 
However, the bound is quantitatively much sharper since the \emph{gradient norm} term $\frac{1}{n}\sum_{z \in S}\| \nabla \ell(\w_t,z)\|^2$ in \citet{Li2020On} gets replaced by the {\em gradient discrepancy} term $\|\nabla \ell(\w_t,z) - \nabla \ell(\w_t, z^\prime) \|^2$. As illustrated in our experiments (Section~\ref{sec:exp}), the gradient discrepancy is orders of magnitude smaller than the gradient norm.
The bound in \citet{negrea2019information} depends on a related \emph{gradient incoherence} which we found to be empirically smaller than gradient discrepancy in our experiments (Section~\ref{sec:exp}). However, their bound has a ${1}/{\sqrt{n}}$ sample dependence, which is worse than the ${1}/{n}$ dependence in our bound. \citet{wang2021analyzing} also obtained a $1/n$ rate in their bound depending on the sum of gradient variances. However, their bound scales inversely with $b$, since gradient variance increases as $b$ decreases. In contrast, our bound is suitable for small batch size as well. \citet{Lei2020} considered ``on average stability'' based generalization bounds, but has a dependence either on $L$ or on some form of convexity. Our bound does not depend on $L$, and works for any non-convex and non-smooth loss.  \qed
\end{remark}

\begin{remark}
Our bounds hold for non-convex and/or non-smooth loss functions. \citet{hardt2016train} developed uniform stability based generalization bounds for SGD for smooth losses. To compare with \citet{hardt2016train} for the non-convex case, note that by construction, 
$\gamma_t^2 := \frac{\|\nabla \ell (w,z_n) - \nabla \ell (w,z_n')\|_2^2}{\alpha^2} \leq \frac{\Delta^2(\bar{S}_{n+1})}{\alpha^2} \leq \frac{1}{8c_2}$,
so that our bound in Theorem~\ref{theo:efldstab} can be upper bounded by
$\frac{c}{n} \underset{\bar{S}_{n+1}}{\E} \sqrt{ \sum_{t=1}^T \underset{W_{0:(t-1)}}{\E}\left[\frac{1}{8c_2} \right]} \leq \frac{\sqrt{5}c_0}{2\sqrt{2}} \frac{\sqrt{T}}{n}$, 
since $c=c_0 \sqrt{5c_2}$. For a $\beta=1$ smooth loss, with step size $\eta_t = 1/t$, \citet{hardt2016train} gets a $O(\sqrt{T}/n)$ bound by their Theorem 3.12. However, {\em we do not need the loss to be smooth} and {\em we work with constant step sizes}. Their results do not extend to non-smooth losses or constant step sizes. \qed 
\end{remark}

\begin{remark}
EFLD can be extended to work with anisotropic noise by using $\btheta_{B_t,\aalpha_t} = \nabla \ell(\w_{t-1},S_{B_t}) \oslash \aalpha_t$ in \eqref{eq:efld2} where $\aalpha_t \in \R^p$ determines different scaling for each dimension and $\oslash$ denotes Hadamard division. Theorems~\ref{theo:efld} and \ref{theo:efldstab} can be extended to such anisotropic noise by using $\aalpha$-scaled norms for the gradient discrepancy, i.e., $\| \g - \g'\|_{2,\aalpha}^2 = \sum_j (g_j - g'_j)^2/\alpha_j^2$. \qed 
\end{remark}


\begin{remark}
The lower bound on $\alpha_t$ in Theorem~\ref{theo:efldstab} is a data-dependent quantity $\Delta_{t|}(\bar{S}_{n+1})$. %which can be computed during training. 
%\abdelete{From Example~\ref{exam:sgld}, since $\alpha_t = \sigma_t/\eta_t$, the lower bound $\alpha_t \geq c_3 \Delta_{t|}(\bar{S}_{n+1})$ for a constant $c_3$ implies an upper bound on the step size: $\eta_t \leq \sigma_t/c_3 \Delta_{t|}(\bar{S}_{n+1})$.} 
For SGLD in \eqref{eq:sgld}, the condition implies $\eta_t \leq \sigma_t/c_3 \Delta_{t|}(\bar{S}_{n+1})$, a much more benign (and computable) condition on the step size compared to those in the related work~\cite{mou2018generalization,Li2020On,hardt2016train} which require step size to be bounded by ${\sigma_{t}}/{L}$, where $L$ is the global Lipschitz constant for the loss $\ell$. Note that $\Delta_{t|}(\bar{S}_{n+1}) \ll L$ because $L$ is a uniform bound. 
%on the entire space, and $\Delta_{t|}(\bar{S}_{n+1})$ is computable data-dependent measure based on gradient discrepancy. 
Further, $\Delta_{t|}(\bar{S}_{n+1})$ is expected to decrease over iterations, i.e., as $t$ increases, and gradients get smaller. \qed
\vspace*{-2mm} 
 \end{remark}




\subsection{Proof Sketches of Main Results: Theorems~\ref{theo:efld} and \ref{theo:efldstab}}
\vspace*{-3mm} 
We focus on Theorem~\ref{theo:efld}. To avoid clutter, we drop the subscript $t$ for the analysis and note that the analysis holds for any step $t$.  When the densities $dP_{B,\bxi} = p_{\psi}(\bxi;\btheta_{B,\alpha})$ and $dP'_{B,\bxi} = p_{\psi}(\bxi;\btheta'_{B,\alpha})$, i.e., densities in the same exponential family but with different parameters 
$\btheta_{B,\alpha}$ and $\btheta'_{B,\alpha}$ because of the difference in the mini-batches,
by mean-value theorem, for each $\bxi$, we have 
\vspace{-2mm}
\begin{equation*}
p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta'_{B,\alpha}) 
= \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle~,
\vspace{-2mm}
\end{equation*}
for some $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$ where $\gamma_{\bxi} \in [0,1]$ with the subscript $\bxi$ illustrating dependence on $\bxi$. Then,
\vspace{-2mm}
{\small
\begin{align}
\hspace*{-3mm}
\Lambda_{A,B} &=  \bigintsss_\bxi \frac{\big( p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta'_{B,\alpha}) \big)^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber \\
 =& \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber \\
= &\bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla_{\tilde{\btheta}_{B,\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2~p_{\psi}^2(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi,
\label{eq:expcore1}
\vspace{-3mm}
\end{align}}
where since $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) = \exp(\langle \bxi, \tilde{\btheta}_{B,\alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha})) \pi_0(\bxi)$ we have 
%\begin{align*}
$\nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) = (\bxi - \nabla_{\tilde{\btheta}_{B,\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) ) p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})$.
%\end{align*}


\noindent {\bf Handling Distributional Dependence of $\tilde{\btheta}_{B,\alpha}$.}
Note that it is difficult to proceed with the analysis with the density term depending on parameter $\tilde{\btheta}_{B,\alpha}$ since $\tilde{\btheta}_{B,\alpha}$ depends on $\bxi$ and there is an outside integral over $\bxi$ in \eqref{eq:expcore1}. So, we first bound the density term depending on $\tilde{\btheta}_{B,\alpha}$ in terms of exponential family densities with parameters $\btheta_{B,\alpha}$ and $\btheta'_{B,\alpha}$ essentially using $c_2$-smoothness of $\psi$.
\begin{restatable}{lemm}{exptilde}
With $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$ for some $\gamma_{\bxi} \in [0,1]$, we have 
% \vspace{-3mm}
\small
\begin{align*}
&\frac{\exp\left[\langle \bxi, \tilde{\btheta}_{B, \alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha}) \right]}{ \max\left( \exp\big[\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha}) \big] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right]\right) }\\
&\leq \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta'_{B,\alpha} \|_2^2 \right] ~.
% \vspace{-2mm}
\end{align*}
\normalsize
\label{lemm:exp_step2}
\end{restatable}
In other words, for any $\bxi$ we have
\begin{align*}
& p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) \leq \\
& \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta'_{B,\alpha} \|_2^2 \right] \max \left( p_{\psi}(\bxi;\btheta_{B,\alpha}), p_{\psi}(\bxi;\btheta'_{B,\alpha}) \right)~.
% \vspace*{-2mm}
\end{align*}
Since the parameters $\btheta_{B,\alpha}, \btheta'_{B,\alpha}$ in the right-hand-side depend on $\bxi$, the outside integral over $\bxi$ in \eqref{eq:expcore1} will not pose any unusual challenges.

\noindent {\bf Bounding the Density Ratio.} Next we focus on the density ratio $p^2_{\psi}(\bxi,\tilde{\btheta}_{B,\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$ in \eqref{eq:expcore1}. By Lemma~\ref{lemm:exp_step2}, it suffices to focus on $p^2_{\psi}(\bxi,\btheta_{B,\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$ or the equivalent term for $\btheta'_{B,\alpha}$. We show that the density ratio can be bounded by another distribution in the same exponential family $p_{\psi}$ with parameters $(2\btheta_{B,\alpha} - \btheta_{A,\alpha})$.
\begin{restatable}{lemm}{expdr}
\vspace*{-1mm}
For any $\bxi$, we have 
\begin{align*}
&\frac{\exp\left[\langle \bxi, 2\btheta_{B, \alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A,\alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]} \leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] \\
& \qquad \qquad \times \exp \left[  \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha} \rangle - \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha} )\right].
\end{align*}
\label{lemm:exp_step3}
\end{restatable}
% \vspace*{-4mm}
In other words, for any $\bxi$ we have
{\small
\begin{align*}
\frac{p^2_{\psi}(\bxi,\btheta_{B,\alpha})}{p_{\psi}(\bxi;\btheta_{A,\alpha})} \leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2\btheta_{B,\alpha} - \btheta_{A,\alpha})~.
\end{align*}}
The analysis for the term $p^2_{\psi}(\bxi,\btheta'_{B,\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$ is exactly the same. 

\noindent {\bf Bounding the Integral.} Ignoring multiplicative terms which do not depend on $\bxi$ for the moment, the analysis needs to bound an integral term of the form
\vspace{-2mm}
\begin{equation*}
\bigintsss_\bxi \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2 ~p_{\psi}(\bxi;2 \btheta_{B,\alpha} - \btheta_{A,\alpha}) d\bxi~,
\vspace{-2mm}
\end{equation*}
and a similar term with $p_{\psi}(\bxi;2 \btheta'_{B,\alpha} - \btheta_{A,\alpha})$. First, note that  $\nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) = \tilde{\m}_{B,\alpha}$, the expectation parameter for $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})$~\citep{wainwright2008graphical,banerjee2005clustering}. The integral, however, is with respect to $p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})$, not $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})$. We handle this discrepancy by using
\vspace{-2mm}
{\small 
\begin{align*}
& \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle^2 \\
& = \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, (\bxi - \E[\bxi]) + (\E[\bxi] - \nabla \psi (\bxi; \tilde{\btheta}_{B,\alpha})) \rangle^2 \\
& \leq 2 \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \E[\bxi] \rangle^2  \\
&\qquad +2 \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \E[\bxi] - \nabla \psi (\bxi; \tilde{\btheta}_{B,\alpha}) \rangle^2~,
\vspace{-2mm}
\end{align*}
}
where the expectation $\E[\bxi]$ is with respect to $p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})$.
Quadratic form for the first term yields the covariance $\E[(\bxi- \E[\bxi])(\bxi - \E[\bxi])^T] = \nabla^2 \psi(\btheta_{2\btheta_{B,\alpha} - \btheta_{A,\alpha}}) \leq c_2 \I$, by smoothness and since the covariance matrix of an exponential family is the Hessian of the log-partition function~\citep{wainwright2008graphical}. Since $\E[\bxi] = \nabla \psi ( 2\btheta_{B,\alpha} - \btheta_{A,\alpha})$, the second term depends on the difference of gradients $\nabla \psi ( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\tilde{\btheta}_{B,\alpha})$ which, using smoothness and additional analysis, can be bounded by the norm of $(\btheta_{B,\alpha} - \btheta_{A,\alpha})$. All the pieces can be put together to get the bound in Theorem~\ref{theo:efld}, which when used in Lemma~\ref{theo:stab}
yields Theorem~\ref{theo:efldstab}.








==> Neurips2021/app/exp.tex <==
% \textsc{Proof for Proposition~[]} Since $p_{\btheta,\sigma}(\bxi)$ is a product of marginal exponential families, $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$, so that the $j$-th component of the gradient $\nabla \psi(\theta)$ is $\nabla_j \psi(\theta) = \psi'_j(\theta_j)$, where $\psi'_j(\theta_j)$ denotes the derivative of $\psi_j(\theta_j)$. Noting that $\psi'_j$ is a monotonic function since $\psi_j$ is convex, we have
% \begin{align*}
% \left\| \nabla \psi(\tilde{\theta}_B/2\sigma^2) \right\|_2^2 & = \sum_{j=1}^p \left| \psi'_j(\tilde{\theta}_{j,B}/2\sigma^2) \right|^2 \\
% & \stackrel{(a)}{\leq} \sum_{j=1}^p \max\left\{ \left| \psi'_j(\theta_{j,B}/2\sigma^2) \right|^2, \left| \psi'_j(\theta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
% & \leq \sum_{j=1}^p \left\{ \left| \psi'_j(\btheta_{j,B}/2\sigma^2) \right|^2 + \left| \psi'_j(\btheta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
% & = \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2 \\
% & \stackrel{(b)}{=} \left\| \m_{B,\sigma} \right\|_2^2 + \left\| \m'_{B,\sigma} \right\|_2^2
% \end{align*}
% where (a) follows since $\tilde{\theta}_{j,B} \in ~\text{interval}(\theta_{j,B},\theta'_{j,B})$\footnote{We use interval$(a,b)$ to denote $[a,b]$ or $[b,a]$, depending on their ordering.} and $\psi'_j$ is monotonic, $\psi'_j(\tilde{\theta}_{j,B}) \in~\text{interval}(\psi'_j(\theta_{j,B}),\psi'_j(\theta'_{j,B}))$, and (b) follows since for exponential families, the mean parameter $\m = \nabla \psi(\theta)$ by Legendre duality [][], and $\m_{B,\sigma}, \m_{B',\sigma}$ are respectively the mean parameters for $p_{\btheta_B,\sigma}, p_{\btheta_{B'},\sigma}$. As a result,
% \begin{align*}
% \bigg( \exp & (\langle \bxi, \btheta_B/2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2)) - \exp(\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2)) \bigg)^2 \\
% & \leq \frac{\| \btheta_B - \btheta'_B \|_2^2}{2\sigma^4} \bigg( \big\langle \u_{B,B'}, \bxi \big\rangle^2 + \| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|^2 \bigg) \exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]~.
% \end{align*}
% % \tcedit{Instead, we can do
% % \begin{align*}\leq \frac{\| \theta_A - \theta_B \|_2^2}{2\sigma^4} \bigg(  \langle u_{A,B},x\rangle^2 + \| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|^2 \bigg) \exp\left[\langle x, \tilde{\theta}_B / \sigma^2 \rangle - 2\psi(\tilde{\theta}_B/2\sigma^2)\right]\end{align*}}
% \abcomment{The $\btheta$ difference can be written as $\m$ difference, see Section 6.3}



% \begin{prop}
% For any $\bxi$, we have 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }
% \leq \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right] ~.
% \end{align*}
% \end{prop}
% \proof Given $\bxi$, for some $\alpha_{\bxi} \in [0,1]$, $\tilde{\btheta} = \alpha_{\bxi} \btheta_B + (1-\alpha_{\bxi}) \btheta'_B$. Denoting $\alpha_{\bxi}$ as $\alpha$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
% \begin{align*}
% \langle \bxi, & \tilde{\btheta}_B / 2\sigma^2 \rangle  - \psi(\tilde{\btheta}_B/2\sigma^2) 
%  = \langle \bxi, \alpha \btheta_B/ 2\sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \rangle - \psi\left( \alpha \btheta_B/ 2 \sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \right) \\
% & = \alpha \bigg[ \langle \bxi , \btheta_B / 2 \sigma^2 \rangle - \psi(\btheta_B/ 2 \sigma^2) \bigg]  + (1-\alpha) \bigg[ \langle \bxi , \btheta'_B /2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2) \bigg] \\
% & ~~~~~~~~~~~~~~~
%   + \bigg[ \alpha \psi(\btheta_B/ 2\sigma^2 ) + (1-\alpha) \psi(\btheta'_B/2 \sigma^2) - \psi( \alpha \btheta_B/2\sigma^2 + (1-\alpha) \btheta'_B/2\sigma^2 ) \bigg] \\
% & \stackrel{(a)}{\leq} \max\bigg[ \langle \bxi , \btheta_B/ 2\sigma^2 \rangle - \psi(\btheta_B/2 \sigma^2) , \langle \bxi , \btheta'_B / 2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2 )  \bigg] \\
% & ~~~~~~~~~~~~~~~ 
%   + \bigg[ \alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2 , \tilde{\btheta}_B/2\sigma^2) \bigg]~,
% \end{align*}
% where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation [Section 3.1.1](Banerjee'05).
% Now, note that
% \begin{align*}
% \alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  
% & \leq \alpha d_{\psi}(\btheta_B/2\sigma^2, \btheta'_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \btheta_B/2\sigma^2) \\
% & \stackrel{(a)}{=} \alpha d_{\phi}(\m'_{\sigma}, \m_{\sigma}) + (1-\alpha) d_{\phi}(\m_{\sigma},\m'_{\sigma})~\\
% & \stackrel{(b)}{\leq} \alpha c_2 \| \m'_{\sigma} - \m_{\sigma} \|_2^2 + (1-\alpha) c_2 \| \m_{\sigma} - \m'_{\sigma} \|_2^2 \\
% & \leq \frac{c_2}{4\sigma^2} \| \hat{\m}_{\sigma} - \hat{\m}'_{\sigma} \|_2^2~,
% \end{align*}
% where (a) follows by duality [][], and (b) follows due to smoothness.
% As a result,
% \begin{align*}
% & \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }\\
% & ~~~~~ \leq \exp\left[ \frac{c_2}{4\sigma^2} \| \hat{\m}_{\sigma} - \hat{\m}'_{\sigma} \|_2^2\right]
% \frac{ \exp \left[ \max\bigg[ \langle \bxi , \btheta_B \rangle - \psi(\btheta_B) , \langle \bxi , \btheta'_B \rangle - \psi(\btheta'_B)  \bigg] \right] }{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] } \\
% & ~~~~~ \leq \exp\left[ \frac{c_2}{4\sigma^2} \| \hat{\m}_{\sigma} - \hat{\m}'_{\sigma} \|_2^2\right] ~.
% \end{align*}
% That completes the proof.\qed 



% \textsc{Proof of Proposition }
% \subsection{Step 3}
% Finally, focusing on density ratio, we have
% \begin{align*}
% & \frac{\left(\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right] \right)^2 }{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi)
% = \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) \\
% & ~~~ \leq 2 \exp \left[ \frac{c_2}{2\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B,\sigma} \|_2^2 \right] \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / \sigma^2 \rangle - 2\psi(\btheta'_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% \end{align*}
% Now, note that
% % \begin{align*}
% % \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}  
% % & = \exp\left[ \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] \\
% % & = \beta_{B,A,\sigma} \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
% % \end{align*}
% % where
% % \begin{align*}
% % \beta_{B,A,\sigma} & = \exp \left[ \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] ~.
% % \end{align*}
% % Note that
% % \begin{align*}
% % \log \beta_{B,A,\sigma} & = \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big)\\
% % & = - \bigg( \psi(\btheta_B/2\sigma^2) - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \bigg) - \bigg( \psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \bigg) \\
% % & \stackrel{(a)}{\leq} \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) /2\sigma^2 \bigg\rangle + \bigg\langle (\btheta_A - \btheta_B)/2\sigma^2, \nabla \psi( \btheta_A/2\sigma^2) /2\sigma^2 \bigg\rangle   \\
% % & = \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \nabla \psi(\btheta_A/2\sigma^2)  \bigg\rangle /2\sigma^2 \\
% % & \stackrel{(b)}{=} \bigg( d_{\psi}(\btheta_B/2\sigma^2, \btheta_A/2\sigma^2) + d_{\psi}(\btheta_A/2\sigma^2 , (2 \btheta_B - \btheta_A)/2\sigma_A^2 ) - d_{\psi}(\btheta_B/2\sigma^2, (2 \btheta_B - \btheta_A)/2\sigma^2 \bigg) / 2 \sigma^2 \\
% % & \leq \big( c_2 \| \btheta_B - \btheta_A \|_2^2 + c_2 \| \btheta_A - (2\btheta_B - \btheta_A) \|_2^2 - c_1 \| \btheta_B - (2\btheta_B - \btheta_A) \|_2^2 \big) / 8 \sigma^6 \\
% % & = (5c_2 - c_1) \| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 / 2 \sigma^2~,
% % \end{align*}
% \begin{align*}
%     \log \beta_{B,A,\sigma} & = \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big)\\
%     & \stackrel{(a)}{=}  d_{\psi}((2\btheta_B - \btheta_A)/2\sigma^2, \btheta_B/2\sigma^2) + d_{\psi}(\btheta_A/2\sigma^2, \btheta_B/2\sigma^2)\\
%     &\stackrel{(b)}{=}  d_{\phi}(\m'_{\sigma}, \m_{\sigma}) +  d_{\phi}(\m_{\sigma},\m'_{\sigma})\\
%     &\leq 2c_2\|(\btheta_B - \btheta_A)/2\sigma^2\|_2^2
% \end{align*}
% where (a) follows from the Bregman information of $\psi$, and (b) follows from duality.
% Since $\phi$ is smooth, we also have
% \begin{align*}
% \| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 & = \| \nabla \phi( \m_{B,\sigma} ) - \nabla \phi (\m_{A,\sigma}) \|_2^2 \leq  c_2^2 \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 = \frac{c_2^2}{4\sigma^2} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 ~,
% \end{align*}
% we have 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}
% \leq \exp \left[ \frac{(5c_2 - c_1)c_2^2}{8\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
% \end{align*}
% The analysis for the term involving $\btheta'_B$ is similar. 

% \subsection{Wrap Up}

% \abcomment{These are notes to wrap up the analysis}

% Note that we have managed to bound the density ratio term involving $\tilde{\btheta}_B$ and $\btheta_A$ as a sum of two exponential family distributions with parameters $(2\btheta_B - \btheta_A)$ and $(2\btheta'_B - \btheta_A)$. Note that the joint distributions continue to be product of marginal distributions. Thus if the marginals are sub-Gaussian (sub-exponential) distributions, the joint distributions will be sub-Gaussian (sub-Exponential) since they are a product of independent univariate sub-Gaussian (sub-exponential) distributions.

% The only technical part left to show is to bound the expectation of $\langle \u_{B,B'}, \bxi \rangle^2$. If the marginals have a subG distribution with $\psi_2$ norm $\kappa$, we should be able to bound the expectation by $c_3 \kappa^2$. The argument for subE distribution would be similar, the bound may be $\c_4 \kappa^4$.

% \abcomment{Finally, similar to the Gaussian case, choose $\eta_t$ to control the multiplicative terms, and show the stability bound.}\abcomment{which is a sub-Gaussian (sub-exponential) distribution since it is a product of univariate sub-Gaussian (sub-exponential) distributions}

% \begin{lemm}
% For exponential family, 
% \begin{align*}
%     I_{A,B} &=  \bigintsss_\bxi \frac{(p_{\btheta_B,\sigma} - p_{\btheta'_B,\sigma})^2}{p_{\btheta_A,\sigma}} d\bxi\leq 
% \end{align*}

% \end{lemm}

% \proof
% From equation~\eqref{eq:exp_target}\eqref{eq:exp_step1}\eqref{eq:exp_step2}\eqref{eq:exp_step3}, we have
% \begin{align*}
%     &I_{A,B}\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi\\
%     &\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2 \bigg) \exp\left[ c_2 \| \nabla \psi(\btheta_B/2\sigma^2) - \nabla \psi(\btheta'_B/2\sigma^2) \|_2^2 \right]}{2\sigma^4 } \\
%     &2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B-\btheta_A,\sigma}+ 2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B-\btheta_A,\sigma}d\bxi\\
%     &\leq\bigintsss_\bxi \frac{\| \btheta_B - \btheta'_B \|_2^2}{2\sigma^4} \bigg( \big\langle \u_{B,B'}, \bxi \big\rangle^2 + \| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|_2^2 \bigg) 2\exp\left[ \frac{c_2}{4} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right]\\
%     \qquad &\left(2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B - \btheta_A,\sigma} +2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B - \btheta_A,\sigma}\right)\pi_0(\bxi) d\bxi\\
%     &\stackrel{(a)}{\leq} c_2^2\| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 (\psi_j^{''}(2\btheta_B-\btheta_A)+\psi_j^{''}(2\btheta'_B-\btheta_A)+ \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2+\| \m'_{B,\sigma} - \m_{A,\sigma} \|_2^2+\| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|_2^2)\\
%     &\exp\left[ \frac{c_2}{4} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right]\left(\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8} \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right]  +\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8} \| \m'_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right] \right),
% \end{align*}
% where $(a)$ is from $\|\E[\bxi\bxi^\top]\|_{\operatorname{op}} = \|\E[\bxi]\E[\bxi]^\top +\operatorname{Var}(\bxi)\|_{\operatorname{op}} \leq \|\E[\bxi]\E[\bxi]^\top\|_{\operatorname{op}}+ \|\operatorname{Var}(\bxi)\|_{\operatorname{op}}\leq \|\E[\bxi]\|_2^2 + \max_j \operatorname{Var}(\bxi_j)$, which completes the proof.
% \qed


% \textbf{Examples.}

% \begin{array}{|l||c|c|c|c|}
% \hline \text { Distribution } & \theta & \psi( \theta ) & \psi'(\theta)&\psi''(\theta)\\
% \hline \hline \text {  Gaussian } & \frac{a}{\sigma^{2}} & \frac{\sigma^{2}}{2} \theta^{2} & \sigma^2\theta & \sigma^2 \\
% \hline \text { Poisson } & \log \lambda & \exp (\theta)& \exp (\theta)& \exp (\theta) \\
% \hline \text { Bernoulli } & \log \left(\frac{q}{1-q}\right) & \log (1+\exp (\theta)) & \frac{\exp(\theta)}{1+\exp(\theta)} & \frac{\exp(\theta)}{(1+\exp(\theta))^2}\\
% \hline \text { Binomial } & \log \left(\frac{q}{1-q}\right) & N \log (1+\exp (\theta)) & N\frac{\exp(\theta)}{1+\exp(\theta)} & N\frac{\exp(\theta)}{(1+\exp(\theta))^2}\\
% \hline \text { Exponential } & -\lambda & -\log (-\theta) & -\frac{1}{\theta} & \frac{1}{\theta^2}\\
% % \hline \text { Laplace } & -\frac{1}{b} & \log(-\frac{2}{\theta}) & -\frac{1}{\theta} & \frac{1}{\theta^2}\\
% \hline
% \end{array}


% \begin{array}{|l||c|c|c|c|}
% \hline \text { Distribution } & p( x ; \theta ) & \m & \phi( \m ) & d_{\phi}( x , \m ) \\
% \hline \hline \text { Gaussian } & \frac{1}{\sqrt{\left(2 \pi \sigma^{2}\right)}} \exp \left(-\frac{(x-a)^{2}}{2 \sigma^{2}}\right) & a & \frac{1}{2 \sigma^{2}} \m^{2} & \frac{1}{2 \sigma^{2}}(x-\m)^{2} \\
% \hline \text { Poisson } & \frac{\lambda^{x} \exp (-\lambda)}{x !} & \lambda & \m \log \m-\m & x \log \left(\frac{x}{\m}\right)-(x-\m) \\
% \hline \text { Bernoulli } & q^{x}(1-q)^{1-x} & q & \m \log \m+(1-\m) \log (1-\m) & x \log \left(\frac{x}{\m}\right)+(1-x) \log \left(\frac{1-x}{1-\m}\right) \\
% \hline \text { Binomial } & \frac{N !}{(x) !(N-x) !} q^{x}(1-q)^{N-x} & N q & \m \log \left(\frac{\m}{N}\right)+(N-\m) \log \left(\frac{N-\m}{N}\right) & x \log \left(\frac{x}{\m}\right)+(N-x) \log \left(\frac{N-x}{N-\m}\right) \\
% \hline \text { Exponential } & \lambda \exp (-\lambda x) & 1 / \lambda & -\log \m-1 & \frac{x}{\m}-\log \left(\frac{x}{\m}\right)-1 \\
% % \hline \text { Laplace } & \frac{1}{2 b} \exp \left(-\frac{|x|}{b}\right) & b & -\log \m-1 & \frac{x}{\m}-\log \left(\frac{x}{\m}\right)-1 \\
% \hline
% \end{array}



% \section{Proof for Exponential family}

% We assume that the multi-variate noise is sub-Gaussian and from a suitable exponential family, so that for $\bxi \in W \subseteq \R^p$
% \begin{align*}
% p_{\btheta}(\bxi) = \exp(\langle \bxi, \btheta \rangle - \psi(\btheta)) \pi_0(\bxi)~,
% \end{align*}
% where $\psi(\btheta)$ is the log-partition function and $\pi_0(\w)$ is the base measure. In our context, we will work with a scaled form based on natural parameter $\btheta/2\sigma^2$, so that
% \begin{align*}
% p_{\btheta,\sigma}(\bxi) = \exp(\langle \bxi, \btheta/2\sigma^2 \rangle - \psi(\btheta/2\sigma^2)) \pi_0(\bxi)~.
% \end{align*}
% Note that the base measure $\pi_0(\bxi)$ does not change with such scaling. Recall that by construction, for $\btheta \in \Theta \subseteq \R^p$, $\psi(\theta)$ is smooth and strongly convex [][][]. Our analysis will cover several
% popular exponential families including Gaussians, Poisson, gamma, Laplace, exponential, among others (see Table ?) [][]. Further, we always consider symmetric versions of one sided distributions such as Poisson, gamma, Laplace, and exponential. 

% We consider adding independent exponential family noise to every component of the gradient update, i.e.,
% for a mini-batch $B$, 
% \begin{align*}
% \w_{t+1} = \w_t - \eta_t \nabla F(\w_{t-1},S_B) + \bxi_t~,
% \end{align*}
% where $\bxi_t \sim p_{\theta_t,\sigma_t}$ so that the components $\xi_t^j, j=1,\ldots,p$ are independent. As a result, the joint distribution $p_{\btheta,\sigma}(\bxi)$ can be written as a product over marginal distributions:
% \begin{align*}
% p_{\btheta,\sigma}(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_j/2\sigma^2 - \psi_j(\theta_j)) \pi_0(\xi_j/2\sigma^2)~,
% \end{align*}
% where we have overloaded notation and used $\pi_0$ to also denote the marginal base measure respectively. Note that in our notation, $\pi_0(\bxi) = \prod_{j=1}^p \pi_0(\xi_j)$ and also $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$. 
% \abcomment{The marginal distributions can be assumed to be sub-Gaussian (sub-Exponential), so the high-d distribution will also be sub-G (sub-E) since its a product of marginal sub-G. Need to add text on this, along with examples.}

\subsection{Preliminary}
We introduce preliminary of exponential family for the analysis. We will use both the natural and expectation parameterization form. Let $\hat{\btheta}_{\sigma} = \btheta/(2\sigma^2)$, and the mean parameter $\hat{\m}_{\sigma} = \nabla_{\hat{\btheta}_{\sigma}} \psi(\hat{\btheta}_{\sigma})$. In our settings, the mean parameter for distribution on batch $B$ is $\m_B = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t})$ so we use $\hat{\m}_{B,\sigma},\hat{\m}'_{B',\sigma}$ to denote $\m_B,\m'_B$ respectively. 
For ease of computation, we denote $\m_{\sigma}$ as the natural gradient: $\m_{\sigma} := \nabla_{\btheta} \psi(\btheta/(2\sigma^2)) = \hat{\m}_{\sigma}/(2\sigma^2)$. Further, $\btheta/(2\sigma^2) = \nabla \psi^{-1}(\m_{\sigma}) = \nabla \phi_{\sigma}(\m_{\sigma})$. 
% Then, 
% \begin{align*}
% \langle \bxi, \btheta/(2\sigma^2) \rangle - \psi(\btheta/(2\sigma^2)) 
% & = \langle \m_{\sigma}, \btheta/(2\sigma^2) \rangle - \psi(\btheta/(2\sigma^2)) + \langle \bxi - \m_{\sigma}, \btheta/(2\sigma^2) \rangle~\\
% & = \phi(\m_{\sigma}) + \langle \bxi - \m_{\sigma}, \nabla \phi(\m_{\sigma}) \rangle \\
% & = - d_{\phi}(\bxi, \m_{\sigma}) + \phi(\bxi)~.
% \end{align*}
Further, since $\psi$ is strongly convex and smooth, so is $\phi$ by Legendre duality, and there are strongly convex constant $c_1$ and Lipschitz smooth constant $c_2$, where $c_1 \leq c_2$ such that
\begin{equation*}
    c_1 \| \bxi - \m \|_2^2 \leq d_{\phi_\sigma}(\bxi,\m) \leq c_2 \| \bxi - \m \|_2^2~,
\end{equation*}
for any $\bxi,\m$ in the domain $\Theta$, any $\sigma\in \Omega$. From the definition of $d_{\phi_\sigma}$:
\begin{equation}
    d_{\phi_\sigma}(\bxi,\m) = \phi_\sigma(\bxi)-\phi_\sigma(\m)-\langle \bxi - \m, \nabla \phi_\sigma (\m)\rangle,
\end{equation}
the strongly convexity and Lipschitz smoothness on $d_{\phi_\sigma}$ implies $\phi_{\sigma}$ is strongly convex and Lipschitz smooth. By duality, we have $\psi$ is strongly convex and Lipschitz smooth  [see Theorem 6 in \cite{kakade2009duality}]:
\begin{equation}
    \frac{1}{4c_2} \| \bxi - \btheta \|_2^2 \leq d_{\psi}(\bxi,\btheta) \leq \frac{1}{4c_1} \| \bxi - \btheta \|_2^2.
\end{equation}


%We further assume that the base measure $\pi_0(\xi_j) \leq 1, j=1,\ldots,p$, \abcomment{may not be necessary} which is satisfied by many 


Following the earlier analysis, by mean-value theorem, for some $\tilde{\btheta}_B = \alpha_x \btheta_B + (1-\alpha_x) \btheta'_B$, $\alpha_x \in [0,1]$, our goal is to bound:
\begin{align}
\nonumber I_{A,B} &=  \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \nabla_{\btheta}p_{\tilde{\btheta}_B,\sigma}\rangle ^2}{p_{\btheta_A,\sigma}} d\bxi = \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/2\sigma^2)\rangle ^2p_{\tilde{\btheta}_B,\sigma}^2}{4\sigma^4 p_{\btheta_A,\sigma}} d\bxi \\
&\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi~.
\end{align}



\subsection{Step 1}
Our goal in this step is to prove the following lemma:
\begin{lemm}\label{lemm:exp_step1}
For some $\tilde{\btheta}_B = \alpha_x \btheta_B + (1-\alpha_x) \btheta'_B$, $\alpha_x \in [0,1]$, we have
\begin{equation}
    \left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2\leq \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2.
\end{equation}
\end{lemm}

\proof
Since $p_{\btheta,\sigma}(\bxi)$ is a product of marginal exponential families, $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$, so that the $j$-th component of the gradient $\nabla \psi(\theta)$ is $\nabla_j \psi(\theta) = \psi'_j(\theta_j)$, where $\psi'_j(\theta_j)$ denotes the derivative of $\psi_j(\theta_j)$. Noting that $\psi'_j$ is a monotonic function since $\psi_j$ is convex, we have
\begin{align*}
\left\| \nabla \psi(\tilde{\theta}_B/2\sigma^2) \right\|_2^2 & = \sum_{j=1}^p \left| \psi'_j(\tilde{\theta}_{j,B}/2\sigma^2) \right|^2 \\
& \stackrel{(a)}{\leq} \sum_{j=1}^p \max\left\{ \left| \psi'_j(\theta_{j,B}/2\sigma^2) \right|^2, \left| \psi'_j(\theta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
& \leq \sum_{j=1}^p \left\{ \left| \psi'_j(\btheta_{j,B}/2\sigma^2) \right|^2 + \left| \psi'_j(\btheta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
& = \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2
\end{align*}
where (a) follows since $\tilde{\theta}_{j,B} \in ~\text{int}(\theta_{j,B},\theta'_{j,B})$\footnote{We use int$(a,b)$ to denote $[a,b]$ or $[b,a]$, depending on their ordering.} and $\psi'_j$ is monotonic, $\psi'_j(\tilde{\theta}_{j,B}) \in~\text{int}(\psi'_j(\theta_{j,B}),\psi'_j(\theta'_{j,B}))$, which completes the proof. \qed

\subsection{Step 2}
Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. In this step we focus on bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$. 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% \end{align*}



\begin{lemm}\label{lemm:exp_step2}
For some $\alpha_{\bxi} \in [0,1]$, $\tilde{\btheta} = \alpha_{\bxi} \btheta_B + (1-\alpha_{\bxi}) \btheta'_B$, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }
\leq \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right] ~.
\end{align*}
\end{lemm}
\proof Denoting $\alpha_{\bxi}$ as $\alpha$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
\begin{align*}
\langle \bxi, & \tilde{\btheta}_B / 2\sigma^2 \rangle  - \psi(\tilde{\btheta}_B/2\sigma^2) 
 = \langle \bxi, \alpha \btheta_B/ 2\sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \rangle - \psi\left( \alpha \btheta_B/ 2 \sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \right) \\
& = \alpha \bigg[ \langle \bxi , \btheta_B / 2 \sigma^2 \rangle - \psi(\btheta_B/ 2 \sigma^2) \bigg]  + (1-\alpha) \bigg[ \langle \bxi , \btheta'_B /2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2) \bigg] \\
& ~~~~~~~~~~~~~~~
  + \bigg[ \alpha \psi(\btheta_B/ 2\sigma^2 ) + (1-\alpha) \psi(\btheta'_B/2 \sigma^2) - \psi( \alpha \btheta_B/2\sigma^2 + (1-\alpha) \btheta'_B/2\sigma^2 ) \bigg] \\
& \stackrel{(a)}{\leq} \max\bigg[ \langle \bxi , \btheta_B/ 2\sigma^2 \rangle - \psi(\btheta_B/2 \sigma^2) , \langle \bxi , \btheta'_B / 2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2 )  \bigg] \\
& ~~~~~~~~~~~~~~~ 
  + \bigg[ \alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2 , \tilde{\btheta}_B/2\sigma^2) \bigg]~,
\end{align*}
where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation (See section 3.1.1 in \cite{banerjee2005clustering}).
Now, note that
\begin{align*}
\alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  
& \leq \alpha d_{\psi}(\btheta_B/2\sigma^2, \btheta'_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \btheta_B/2\sigma^2) \\
& \stackrel{(a)}{=} \alpha d_{\phi}(\m'_{\sigma}, \m_{\sigma}) + (1-\alpha) d_{\phi}(\m_{\sigma},\m'_{\sigma})~\\
& \leq \alpha c_2 \| \m'_{\sigma} - \m_{\sigma} \|_2^2 + (1-\alpha) c_2 \| \m_{\sigma} - \m'_{\sigma} \|_2^2 \\
& \leq \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2~,
\end{align*}
where (a) follows by duality.
As a result,
\begin{align*}
& \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }\\
& ~~~~~ \leq\exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right]
\frac{ \exp \left[ \max\bigg[ \langle \bxi , \btheta_B \rangle - \psi(\btheta_B) , \langle \bxi , \btheta'_B \rangle - \psi(\btheta'_B)  \bigg] \right] }{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] } \\
& ~~~~~ \leq \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2 \right]~.
\end{align*}
That completes the proof.\qed 

% \abcomment{Old proof - not complete/correct} Using the expectation parameterization form, we have 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \tilde{\theta}_B / 2\sigma^2 \rangle - \psi(\tilde{\theta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \theta_B / 2\sigma^2 \rangle - \psi(\theta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \theta'_B / 2\sigma^2 \rangle - \psi(\theta'_B/2\sigma^2) \right] } 
% & = \frac{ \exp \left[ -d_{\phi}(\bxi,\tilde{\m}_{\sigma}) \right]}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} 
% \end{align*}
% For $\bxi$ outside interval$[\m_{B,\sigma}, \m'_{B,\sigma})$, the ratio is at most 1 \abcomment{show details, one component of the denominator will dominate, use 1-d argument if it helps}. For $\bxi$ inside interval$[\m_{B,\sigma}, \m'_{B,\sigma}]$, we have
% \begin{align*}
% \frac{ \exp \left[ -d_{\phi}(\bxi,\tilde{\m}_{\sigma}) \right]}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} 
% & \leq \frac{1}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} \\
% &  \leq \frac{1}{ \exp \left[ - c_2 \| \bxi - \m_{B,\sigma} \|_2^2 \right] +  \exp \left[ - c_2 \| \bxi - \m'_{B,\sigma} \|_2^2 \right]} \\
% & \stackrel{(a)}{\leq} \frac{1}{2} \exp \left[ \frac{c_2}{2} \left( \| \bxi - \m_{B,\sigma}\|_2^2 + \| \bxi - \m'_{B,\sigma} \|_2^2 \right) \right] \\
% & \leq \frac{1}{2} \exp \left[ \frac{c_2}{2} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right] \\
% & = \frac{1}{2} \exp \left[ \frac{c_2}{8\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B,\sigma} \|_2^2 \right]~,
% \end{align*}
% where (a) follows from AM-GM inequality. That completes the proof. \qed

\subsection{Step 3}
Finally, focusing on density ratio, we have
\begin{lemm}\label{lemm:exp_step3}
For any $\bxi$, we have
\begin{align*}
&\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}\\
&\leq \exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right].
\end{align*}

\end{lemm}

\proof
% \begin{align*}
% & \frac{\left(\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right] \right)^2 }{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi)
% = \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) \\
% & ~~~ \leq 2 \exp \left[ \frac{c_2}{2\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B,\sigma} \|_2^2 \right] \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / \sigma^2 \rangle - 2\psi(\btheta'_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% \end{align*}
Note that
\begin{align*}
\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}  
& = \exp\left[ \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] \\
& = \beta_{B,A,\sigma} \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
\end{align*}
where
\begin{align*}
\beta_{B,A,\sigma} & = \exp \left[ \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] ~.
\end{align*}
Note that
\begin{align*}
\log \beta_{B,A,\sigma} & = \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big)\\
& = - \bigg( \psi(\btheta_B/2\sigma^2) - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \bigg) - \bigg( \psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \bigg) \\
& \stackrel{(a)}{\leq} \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) /2\sigma^2 \bigg\rangle + \bigg\langle (\btheta_A - \btheta_B)/2\sigma^2, \nabla \psi( \btheta_A/2\sigma^2) /2\sigma^2 \bigg\rangle   \\
& = \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \nabla \psi(\btheta_A/2\sigma^2)  \bigg\rangle /2\sigma^2 \\
& \stackrel{(b)}{=} \bigg( d_{\psi}(\btheta_B/2\sigma^2, \btheta_A/2\sigma^2) + d_{\psi}(\btheta_A/2\sigma^2 , (2 \btheta_B - \btheta_A)/2\sigma_A^2 ) - d_{\psi}(\btheta_B/2\sigma^2, (2 \btheta_B - \btheta_A)/2\sigma^2 \bigg) / 2 \sigma^2 \\
& \leq \big( 1/c_1 \| \btheta_B - \btheta_A \|_2^2 + 1/c_1 \| \btheta_A - (2\btheta_B - \btheta_A) \|_2^2 - 1/c_2 \| \btheta_B - (2\btheta_B - \btheta_A) \|_2^2 \big) / 8 \sigma^6 \\
& = (3/c_1 - 1/c_2) \| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 / 2 \sigma^2~,
\end{align*}
where (a) follows from the convexity of $\psi$, and (b) follows from the three-point property of Bregman divergences [See Appendix A, property 8 in \cite{banerjee2005clustering}] given by
\begin{equation*}
\langle \x_1 - \x_2, \nabla \psi(\x_3) - \nabla \psi(\x_2) \rangle = d_{\psi}(\x_1,\x_2) + d_{\psi}(\x_2,\x_3) - d_{\psi}(\x_1,\x_3) ~,
\end{equation*}
with $\x_1 = \btheta_B/2\sigma^2, \x_2 = \btheta_A/2\sigma^2, \x_3 = (2\btheta_B - \btheta_A)/2\sigma^2$.
Since $\phi$ is smooth, we also have
\begin{align*}
\| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 & = \| \nabla \phi( \m_{B,\sigma} ) - \nabla \phi (\m_{A,\sigma}) \|_2^2 \leq  c_2^2 \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 = \frac{c_2^2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 ~,
\end{align*}
we have 
\begin{align*}
&\frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}\\
&\leq \exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
\end{align*}
which completes the proof.\qed

The analysis for the term involving $\btheta'_B$ is similar. 

\subsection{Final step}


% Note that we have managed to bound the density ratio term involving $\tilde{\btheta}_B$ and $\btheta_A$ as a sum of two exponential family distributions with parameters $(2\btheta_B - \btheta_A)$ and $(2\btheta'_B - \btheta_A)$. Note that the joint distributions continue to be product of marginal distributions. Thus if the marginals are sub-Gaussian (sub-exponential) distributions, the joint distributions will be sub-Gaussian (sub-Exponential) since they are a product of independent univariate sub-Gaussian (sub-exponential) distributions.

% The only technical part left to show is to bound the expectation of $\langle \u_{B,B'}, \bxi \rangle^2$. If the marginals have a subG distribution with $\psi_2$ norm $\kappa$, we should be able to bound the expectation by $c_3 \kappa^2$. The argument for subE distribution would be similar, the bound may be $\c_4 \kappa^4$.

% \abcomment{Finally, similar to the Gaussian case, choose $\eta_t$ to control the multiplicative terms, and show the stability bound.}\abcomment{which is a sub-Gaussian (sub-exponential) distribution since it is a product of univariate sub-Gaussian (sub-exponential) distributions}
We gather the above three steps to bound $I_{A,B}$:
\lemmexpinfo*

\proof 
From Lemma~\ref{lemm:exp_step1},\ref{lemm:exp_step2},\ref{lemm:exp_step3}, we have
\begin{align*}
    &I_{A,B}\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi\\
    &\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2 \bigg) \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]}{2\sigma^4 } \\
    &2\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B-\btheta_A,\sigma}+ 2\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B-\btheta_A,\sigma}d\bxi\\
    &\leq\bigintsss_\bxi \frac{1}{\sigma^4} \bigg(  \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg) \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]\\
   &\left(\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B - \btheta_A,\sigma} +\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B - \btheta_A,\sigma}\right)\pi_0(\bxi) d\bxi.
   \end{align*}
   For $p_{2\btheta_B - \btheta_A,\sigma}$, we have
   \begin{align*}
   &\bigintsss_\bxi \frac{1}{\sigma^4} \bigg(  \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg) \exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma}\|_2^2\right]\\
   &\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B - \btheta_A,\sigma}\pi_0(\bxi) d\bxi\\
   &=\frac{1}{\sigma^4} \bigg(  \big(\btheta_B -\btheta'_B)^\top \E_{\bxi\sim p_{2\btheta_B-\btheta_A,\sigma}}\bxi\bxi^\top(\btheta_B -\btheta'_B)  + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{\|\btheta_B -\btheta'_B\|_2^2}{4\sigma^4}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg)\\
   &\exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]\\
    % &\stackrel{(a)}{\leq} c_2^2\| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 (\psi_j^{''}(2\btheta_B-\btheta_A)+\psi_j^{''}(2\btheta'_B-\btheta_A)+ \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2+\| \m'_{B,\sigma} - \m_{A,\sigma} \|_2^2+\| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|_2^2)\\
    % &\exp\left[ \frac{c_2}{4} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right]\left(\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8} \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right]  +\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8} \| \m'_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right] \right),\\
    &\stackrel{(a)}{\leq}\frac{1}{\sigma^4}  c_2^2 \| \hat{\m}_{B,\sigma} - \hat{\m}_{B',\sigma} \|_2^2 \bigg(\frac{c_2^2}{16c_1^2\sigma^4}\|2\hat{\m}_{B,\sigma}-\hat{\m}_{A,\sigma}\|_2^2 + \frac{1}{8c_1 \sigma^4}  + \frac{1}{4\sigma^4}\left\| \hat{\m}_{B,\sigma} \right\|_2^2 + \frac{1}{4\sigma^4}\left\|\hat{\m}'_{B,\sigma}\right\|_2^2  \bigg)\\
    &\exp\left[ \frac{c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}'_{B',\sigma} \|_2^2\right]\exp \left[ \frac{(3c_2 - c_1)c_2}{8c_1\sigma^6} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]
\end{align*}
where $(a)$ is from $\|\E[\bxi\bxi^\top]\|_{\operatorname{op}} = \|\E[\bxi]\E[\bxi]^\top +\operatorname{Var}(\bxi)\|_{\operatorname{op}} \leq \|\E[\bxi]\E[\bxi]^\top\|_{\operatorname{op}}+ \|\operatorname{Var}(\bxi)\|_{\operatorname{op}}\leq \|\E[\bxi]\|_2^2 + \max_j \operatorname{Var}(\bxi_j) =\frac{1}{4\sigma^4} \|\nabla\psi(2\btheta_B-\btheta_A)\|_2^2 +\frac{1}{4\sigma^4} \max_j |\nabla^2_{jj}\psi(2\btheta_B-\btheta_A)|\leq \frac{1}{4c_1^2}\|2\btheta_B-\btheta_A\|_2^2 + \frac{1}{8c_1 \sigma^4}\leq \frac{c_2^2}{16c_1^2\sigma^4}\|2\hat{\m}_{B,\sigma}-\hat{\m}_{A,\sigma}\|_2^2 + \frac{1}{8c_1 \sigma^4}$. Similar analysis holds for $p_{2\btheta'_B - \btheta_A,\sigma}$, with adaptive choice of step size $\eta_t$ completes the proof.
\qed



% \subsection{OLD Text: keeping for ref, remove in the final version}
% \abcomment{Key observation, the ``projection view" (PV), different from previous (Gaussian) analysis } Since $u_{A,B} = \frac{\theta_A - \theta_B}{\|\theta_A - \theta_B \|_2}$ is a unit vector and the distribution is subG, the projection of $\frac{x-\tilde{\m}_B}{2\sigma^2}$ on the unit vector is a 1-d subG random variable. As a result, the second moment will be bounded as long as $p^2_{\tilde{\theta}_B,\sigma}/p_{\theta_A,\sigma}$ is subG. In fact, it suffices to show that the 1-d projection is subG. 

% Key questions: 
% \begin{enumerate}
% \item Should the analysis be done in expectation or natural parameterization?
% \item How should subG exp family be formalized, w.r.t.~the mean or natural parameters?
% \end{enumerate}

% Switching to mean parameterization: We have
% \begin{align*}
% p_{\theta,\sigma}(x) = p_{\m,\sigma}(x) = \exp(-d_{\phi}(x,\m)/2\sigma^2) q_\sigma(x) 
% \end{align*}
% where $q_\sigma(x)$ may have a dependency on $\sigma$.
% So, we have
% \begin{align*}
% I_{A,B} 
% &=  \bigintsss_x \frac{(p_{\theta_B,\sigma} - p_{\theta'_B,\sigma})^2}{p_{\theta_A,\sigma}} dx \\
% & = \bigints_x \frac{ \bigg[ \exp(-d_{\phi}(x,\m_B)/2\sigma^2) - \exp(-d_{\phi}(x,\m'_B)/2\sigma^2) \bigg]^2}{\exp(-d_{\phi}(x,\m_A)/2\sigma^2)} q_\sigma(x) dx     
% \end{align*}
% By mean-value theorem, for some $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B$, $\alpha_x \in [0,1]$, we have
% \begin{align*}
% \exp & (-d_{\phi}(x,\m_B)/2\sigma^2) - \exp(-d_{\phi}(x,\m'_B)/2\sigma^2) \\
% & = \left\langle \m_B - \m'_B, \nabla_{\tilde{\m}_B} \exp(- d_{\phi}(x,\tilde{\m}_B)/2\sigma^2) \right\rangle \\
% & = \| \m_B - \m'_B \|_2 \left\langle \frac{\m_B-\m'_B}{\|\m_B - \m'_B\|_2} , \frac{H_{\phi}(\tilde{\m}_B) (x - \tilde{\m}_B)}{\sigma^2}  \right\rangle \exp\left[ -d_{\phi}(x,\tilde{\m}_B)/\sigma^2 \right] ~,
% \end{align*}
% \abcomment{need to bound probability terms with $\tilde{\theta}$ or $\tilde{\m}$ with corresponding $\theta_B$ or $\m_B$ terms which do not depend on $x$. Fix the analysis for Gaussians first.}
% where $H_{\phi}(\tilde{\m}_B) = \nabla^2 \phi(\tilde{\m}_B)$ is the Hessian. Since $\phi$ is smooth, with $c_{2,\phi} = \| H_{\phi}\|_2$, and with unit vector $u_{B,B'} = \frac{\m_B - \m_B'}{\|\m_B - \m_B' \|_2}$, we have 
% \begin{align*}
% \langle u_{B,B'}^T H_{\phi}(\tilde{\m}_B) (x - \tilde{\m}_B)\rangle ^2 & \leq 2 \langle u_{B,B'}^T H_{\phi}(\tilde{\m}_B) x \rangle^2 + 2 \langle u_{B,B'}^T H_{\phi}(\tilde{\m}_B) \tilde{\m}_B \rangle^2     \\
% & \leq 2 \| H_{\phi}(\tilde{\m}_B) u_{B,B'} \|_2^2 \bigg\{ \big( v_{B.B'}^T x \big)^2 + \big(v_{B,B'}^T \m_B \big)^2 + \big(v_{B,B'}^T \m_B \big)^2 \bigg\}~,
% \end{align*}
% where $v_{B,B'} = \frac{H_{\phi}(\tilde{\m}_B) u_{B,B'}}{ \| H_{\phi}(\tilde{\m}_B) u_{B,B'} \|_2}$ is a unit vector. As a result, $z = v_{B.B'}^T x$ is a univariate subGaussian distribution, and $v_{B,B'}^T \m_B \leq \| \m_B\|_2$ and $v_{B,B'}^T \m'_B \leq \| \m'_B \|_2$. Hence
% \begin{align*}
% \big(u_{B.B'}^T H_{\phi}(\tilde{\m}_B) (x - \tilde{\m}_B)\big)^2 & \leq 2 c_{\phi} \bigg\{ z^2 + \| \m_B\|_2^2 + \| \m'_B \|_2^2 \bigg\}~.
% \end{align*}
% The distribution ratio term is given by
% \begin{align*}
% \frac{\big(\exp\left[ -d_{\phi}(x,\tilde{\m}_B)/2\sigma^2 \right]\big)^2}{\exp\left[ -d_{\phi}(x,\m_A)/2\sigma^2 \right]} q_\sigma(x)
% & = \exp\left[ -\frac{1}{2\sigma^2} \left[ 2 d_{\phi}(x,\tilde{\m}_B) - d_\phi(x,\m_A) \right] \right] \\
% & \leq \exp\left[ \langle x, 2\tilde{\theta}_B - \theta_A \rangle/2\sigma^2 - \left(2\psi(\tilde{\theta}_B/2\sigma^2) - \psi(\theta_A/2\sigma^2\right) \right] \pi_0(x)    \\
% & = \beta_{A,B} \exp \left[ \left \langle x, (2\tilde{\theta}_B - \theta_A)/2\sigma^2 \right\rangle - \psi((2\tilde{\theta}_B - \theta_A)/2\sigma^2) \right] \pi_0(x)~,
% \end{align*}
% where
% \begin{align*}
% \beta_{A,B} & = \exp \left[ \psi((2\tilde{\theta}_B - \theta_A)/2\sigma^2 ) - \left(2 \psi(\tilde{\theta}_B/2\sigma^2) - \psi(\theta_A/2\sigma^2) \right) \right]~.
% \end{align*}



==> Neurips2021/app/experiment.tex <==
{\bf Datasets and Network Structure.} The MNIST and Fashion MNIST datasets both consist of 60,000 training examples and 10,000 test examples. To construct the experiments, we randomly sample $10,000$  samples from the original training set of MNIST and Fashion MNIST. 
Details refer to  Table \ref{tab::network_setup_app}. 
For both MNIST and Fashion MNIST, we use a convolutional neural network with architecture  described in Table \ref{tab:network_app}. 
We also consider a MLP network with three hidden layers with 128, 128 and 64 nodes respectively in each layer. 
All experiments have been run on NVIDIA Tesla v100 GPUs.

\begin{table}[h]
\caption{CNN architecture for MNIST and Fashion MNIST.}
\centering
\begin{tabular}{cc} 
Layer & Parameters \\
\hline \hline Convolution & 16 filters of $8 \times 8,$ strides 2 \\
Max-Pooling & $2 \times 2$ \\
Convolution & 32 filters of $4 x 4,$ strides 2 \\
Max-Pooling & $2 \times 2$ \\
Fully connected & 32 units \\
Softmax & 10 units \\
\hline
\end{tabular}
    \label{tab:network_app}
\end{table}



\begin{table}[h]
  \caption{Neural network and datasets setup.}
	\centering
	\footnotesize{
	%\resizebox{\columnwidth}{!}{%
	\begin{tabular}{cccccc}	
	\toprule[1pt]
	Dataset & Model  & features & classes & Training size  & Test size\\ 	
	\toprule[1pt]
		MNIST            & CNN \& MLP & 28$\times$ 28 & 10 &  10,000  & 10,000\\
Fashion MNIST   & CNN \& MLP  &  28$\times$ 28 & 10 &  10,000  & 10,000\\
		\toprule[1pt]
	\end{tabular}}
%	}
	\label{tab::network_setup_app}
\end{table}


\textbf{Training and Hyper-parameters.} 
We use Noisy SGD with Gaussian noise to train the model, i.e., $\mathbf{w}_{t}=\mathbf{w}_{t-1}-\eta_{t} \nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)+\boldsymbol{\xi}_{t}$, where $\boldsymbol{\xi}_{t} \sim$
$\mathcal{N}\left(0, \sigma_{t}^{2} \mathbb{I}_{d}\right)$. In order to balance the optimization error and generalization error and consider improving the predictive performance, we consider learning rate decay and noise variance decay, such that we set $\sigma_t = c\cdot \eta_t$, wich $c \in [0.05, 0.1]$ and we decay $\eta_t$ every 30 epochs by 0.1. We consider  initial step size $\eta_0 \in \{0.01, 0.005 \}$. 
We set batch size $\left|B_{t}\right|=128$ for all datasets, and minimize cross-entropy loss for a fixed number of epochs. We repeat each experiment for 10 runs.

\textbf{Additional Experimental Results.} Figure \ref{fig: mnist_sigma} (a) and (b) compare our bound with the existing bounds for different noise variance, which shows that as the noise variance/step size ratio increase from 0.05 to 0.1, the bound increase as well. Figures \ref{fig: mnist_eta} and \ref{fig: fashion_eta} compare our bound with  the existing bounds for different initial step sizes for CNN, which shows that our bound is sharper than existing bounds under different step size settings. The training and test accuracy are presented in Table \ref{tab:acc}. 

\begin{figure*}[h] 
\centering
  \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr05alpha01_mnist_fnn.png}
 } 
  \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr05alpha05_mnist_fnn.png}
 }  
%   \subfigure[CNN, $\sigma_0 = 0.01$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr01alpha05_mnist_cnn.png}
%  }  
%   \subfigure[CNN,  $\sigma_0 = 0.005$ ]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_cnn.png}
%  }
\caption[]{Numerical results for MLP for MNIST with (a) $\sigma_t = 0.1\eta_t$ and (b)  $\sigma_t = 0.05\eta_t$. $\sigma_0 = 0.005$ for both (a) and (b). All x-axes show the number of Epochs of training.  Figure (a-b) compare our bound with the existing bounds for different noise variance, which shows that as the noise variance/step size ratio increase from 0.05 to 0.1, the bound increase as well. 
%But the optimization error is better compared to larger ratio. Figure (c-d) compare our bound with the existing bounds for different initial step sizes for CNN, which shows that as the bounds with $\eta_0 = 0.01$ are slightly smaller compared to $\eta_0 = 0.005$. 
} \label{fig: mnist_sigma}
\end{figure*}

\begin{figure*}[h] 
\centering
%   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
%  } 
%   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
%  }  
  \subfigure[CNN, $\sigma_0 = 0.01$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr01alpha05_mnist_cnn.png}
 }  
  \subfigure[CNN,  $\sigma_0 = 0.005$ ]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr05alpha05_mnist_cnn.png}
 }
\caption[]{Numerical results for CNN for MNIST with (a) $\eta_0 = 0.01$  and (b) $\eta_0 = 0.005$. $\sigma_t = 0.05\eta_t$ for both (a) and (b).  Figure (a-b) compare our bound with  the existing bounds for different initial step sizes for CNN, which shows that our bound is sharper than existing bounds under different step size settings.
}\label{fig: mnist_eta}
\end{figure*}

\begin{table}[t]
\caption{Train and test accuracy for different datasets and models.}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &  & CNN, $\eta_0 = 0.01$ & CNN, $\eta_0 = 0.005$ & MLP, $\sigma_t = 0.1\eta_t$  & MLP, $\sigma_t = 0.05\eta_t$ \\ \hline
\multirow{2}{*}{MNIST} & Train accuracy & 98.21 & 96.69 & 90.45 & 90.39 \\ \cline{2-6} 
 & Test accuracy & 97.28 & 96.37 & 89.99 & 89.92 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fashion\\ MNIST\end{tabular}} & Train accuracy & 83.81 & 79.37 & 81.60 & 81.32 \\ \cline{2-6} 
 & Test accuracy & 82.28 & 78.20 & 79.70 & 79.55 \\ \hline
\end{tabular}\label{tab:acc}
\end{table}

\begin{figure*}[h] 
\centering
%   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
%  } 
%   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
%  }  
  \subfigure[CNN, $\sigma_0 = 0.01$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr01alpha01_fashion_fnn.png}
 }  
  \subfigure[CNN,  $\sigma_0 = 0.005$ ]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{img/lr05alpha01_fashion_fnn.png}
 }
\caption[]{Numerical results for MLP for Fashion MNIST with (a) $\eta_0 = 0.01$  and (b) $\eta_0 = 0.005$ .  Figure (a-b) compare our bound with  the existing bounds for different initial step sizes for CNN, which shows that our bound is sharper than existing bounds under different step size settings.
}\label{fig: fashion_eta}
\end{figure*}






% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%  &  & CNN 0.01 & CNN 0.005 & MLP & MLP \\ \hline
% \multirow{2}{*}{MNIST} & Train accuracy & 98.21 & 96.69 & 90.45 & 90.39 \\ \cline{2-6} 
%  & Test accuracy & 97.28 & 96.37 & 89.99 & 89.92 \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fashion\\ MNIST\end{tabular}} & Train accuracy & 83.81 & 79.37 & 81.60 & 81.32 \\ \cline{2-6} 
%  & Test accuracy & 82.28 & 78.20 & 79.70 & 79.55 \\ \hline
% \end{tabular}
% \end{table}

==> Neurips2021/app/gen.tex <==

\prophell*
\proof Let $S=\left(z_{1}, \ldots, z_{n}\right)$ and $\tilde S^{\prime}=\left(z_{1}^{\prime}, \ldots, z_{n}^{\prime}\right)$ two independent random samples and let $S^{(i)}=\left(z_{1}, \ldots, z_{i-1}, z_{i}^{\prime}, z_{i+1}, \ldots, z_{n}\right)$ be the sample that is identical to $S$ except in the $i$-th example where we replace $z_{i}$ with $z_{i}^{\prime}$. 
\begin{align*}
& \E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))] \\
&= \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \mathbb{E}_{A} \left[\frac{1}{n} \sum_{i=1}^{n}\left(\ell(A(S^{(i)}), z_{i}^{\prime})-\ell(A(S), z_{i}^{\prime}) \right)\right] \\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime}  \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_{A} \left(\ell(A(S^{(i)}), z_{i}^{\prime})-\ell(A(S), z_{i}^{\prime}) \right)\\
& \overset{(a)}{=} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \left(\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p^{(i)}(\mathbf{w}) d \mathbf{w}-\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p(\mathbf{w}) d \mathbf{w} \right)\\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) \left( p^{(i)}(\mathbf{w}) d \mathbf{w}- p(\mathbf{w}) \right)d \mathbf{w} \\
& = \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime)\left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)  d \mathbf{w} \\
& \overset{(b)}{\leq} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \left\{\left(\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime)^{2}\left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\}
\end{align*}
where (a): $p^{(i)}(\w)$ is the distribution obtained by $A(S^{(i)})$, and (b) 
follows by Cauchy-Schwartz inequality. Focusing on the first integral, we have: 
\begin{align*}
\left(\int_{\mathbb{R}^{d}} \ell(\w ; z_i^\prime)^{2}\left(\sqrt{p^{(i)}(\w)}+\sqrt{p(\w)}\right)^{2} d \w \right)^{1/2} 
& \leq \left(2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}p^{(i)}(\w) d\w +  2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2} p(\w) d \w \right)^{1/2} \\
& \leq \left( c_0^2 + c_0^2 \right)^{1/2} =\sqrt{2} c_0~.
\end{align*}

Hence,
\begin{align*}
\E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))]
& \leq   \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n}c_0 \sqrt{2H^{2}\left(A(S), A(S'_n)\right)}\\
& = c_0 \E_{S \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S), A(S'_{n})\big)}~.
\end{align*}
% (b): need to double check if we can apply the previous argument that ``for any $z$, the loss $\ell(\w;z)$ has bounded expectation and variance'' because there are dependence between $\ell(\w; z_i^\prime)$ and $p^{(i)}(\w)$. The worst case, we bound it by uniform upper bound $C$ on the loss. (c) is true because $z_i^\prime$ for $i =1,...,n$ are i.i.d., so that we can write it as $z^{\prime}$.
% $p^{\prime}(\mathbf{w})$ is the distribution obtained by $A(S^\prime)$, where $S^\prime$ is the dataset differing on only single sample $z^{\prime}$ with $S$.  

% \abcomment{(a) For the analysis, lets use $| \cdots |$ throughout, (b) pls clean up the $\mu^2 + \sigma^2$ analysis, and use a constant. This part needs work}

% \abcomment{For the last part, change to:}
% \begin{align*}
% & \overset{(b)}{\leq} 2c_0  \mathbb{E}_S \mathbb{E}_{S^\prime} \left[ \frac{1}{n} \sum_{i=1}^{n}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)} \right] \\
% & = 2c_0 \mathbb{E}_S \mathbb{E}_{S'} \mathbb{E}_{z_i^\prime \sim S'}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)}\\
% & \overset{(c)}{=} 2c_0 \mathbb{E}_S \mathbb{E}_{z^{\prime}} \sqrt{D_{H}^{2}\left(p^{\prime}(\mathbf{w}), p(\w)\right)}~.
% \end{align*}
That completes the proof. \qed 


\prophellkl*
\proof For the first part, note that:
\begin{align*}
KL(P ,P') & = \int \log \frac{p(\w)}{p'(\w)} p(\w) ~d\w \\
& =  2 \int  \left\{ - \log \sqrt{\frac{p'(\w)}{p(\w)}} \right\} p(\w)~ d\w \\
& \overset{(a)}{\geq} 2 \int \left\{ 1 - \sqrt{\frac{p'(\w)}{p(\w)}} \right\} p(\w)~ d\w \\ 
& = 2 \int \left( p(\w) - \sqrt{p(\w) p'(\w)}) \right) ~d\w \\
& = \int \left(p(\w) + p'(\w) - 2 \sqrt{p(\w)p'(\w)} \right) ~d\w \\
& = \int \left(\sqrt{p(\w)} - \sqrt{p'(\w)}\right)^2~ d\w\\
& = 2 H^2(P,P')~,
\end{align*}
where (a) follows since for $x > 0$, $-\log x = - \log(1- (1-x)) \geq 1-x$.

For the second part, note that:
\begin{align*}
2H^2(P,P') & =  \int_\w ( \sqrt{p(\w)} - \sqrt{p'(\w)} )^2 d\w \\
& =  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| | \sqrt{p(\w)} - \sqrt{p'(\w)}| ~d\w \\
& \leq  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| | \sqrt{p(\w)} + \sqrt{p'(\w)}|~ d\w \\
& =  \int_\w | p(\w) - p'(\w)|~ d\w \\
& =  TV(P,P')~,
\end{align*}
where $TV(P,P')$ denotes the total variation distance \cite{pollard2002user}. Further, from Pinsker's inequality \cite{tsybakov2008introduction}, we have
\begin{align*}
TV(P,P') \leq \sqrt{\frac{1}{2} KL(P,P')}~.
\end{align*}
Combining the two results completes the proof. \qed 


\subsection{Proofs for Section 2.2}

\mixmodel*
\proof The proof follows the argument in the proof of Lemma 21 in \cite{Li2020On}.\qed

\subsection{Proofs for Section 2.3}

Similar results have appeared in \citep{Li2020On, bun2018composable}, we give a simple proof.
\begin{lemm}\label{lemm:mix_bound}
Let $Q,Q',R$ be any three distributions such that $Q,Q'$ are both absolutely continuous w.r.t.~$R$. Then, for $s \in (0,1)$
\begin{equation}
KL\left(sQ+(1-s)R ~\big\| ~sQ' + (1-s)R \right) \leq 
\frac{s^2}{1-s}~\int_{\w} \frac{(Q(\w) - Q'(\w))^2}{R(\w)} d\w~ .
%\frac{s^2}{1-s} \lsd( Q - Q', R)~.
\end{equation}
\end{lemm}

\proof Let $U=sQ' + (1-s)R$. Then, with $F(x) = Q(x)-Q'(x)$, we have
\begin{align*}
     KL(sQ+(1-s)R \| sQ' + (1-s)R) & =  KL(U + s(Q - Q')  \| U ) \\
     & = \int (U(x) + sF(x)) \log \left( \frac{U(x) + s F(x)}{U(x)} \right) dx \\
     & = \int (U(x) + sF(x)) \log \left( 1 + \frac{s F(x)}{U(x)} \right) dx \\
     & = \int sF(x) + \frac{s^2 F^2(x)}{2U(x)} -  \frac{s^3 F^3(x)}{6U^2(x)} + \frac{s^4 F^4(x)}{12U^3(x)}  -\cdots dx \\
     & = s^2 \int \frac{F^2(x)}{U(x)}\left(  \frac{1}{2} -  \frac{s F(x)}{6U(x)} + \frac{s^2 F^2(x)}{12U^2(x)} - \cdots \right) dx~,
%     & = \int U(x) \left( \left(1+ \frac{sF(x)}{U(x)} \right) \log \left(1 + \frac{sF(x)}{U(x)} \right) - \frac{sF(x)}{U(x)} \right) dx
\end{align*}
where the first term vanishes since $\int F(x) dx = \int (Q(x) - Q'(x)) dx = 0$. This is the reason the dependency is on $s^2$, not $s$. With $W(x) = s F(x)/U(x)$, noting that $W(x) > -1$, and 
\begin{equation}
    \left( \frac{1}{2} - \frac{W(x)}{6} + \frac{W^2(x)}{12} - \cdots \right) = \frac{(1+W(x))\log(1+W(x)) - W(x)}{W^2(x)} \leq 1~,
\end{equation}
we have
\begin{align*}
   KL(sP+(1-s)R \| sQ + (1-s)R) 
     & = s^2 \int \frac{F^2(x)}{U(x)} \left( \frac{ (1+W(x)) \log (1+W(x)) - W(x)}{W^2(x)} \right) dx \\
     & \leq s^2 \int \frac{F^2(x)}{U(x)} dx~ \\
     & \leq \frac{s^2}{(1-s)} \int \frac{(Q(x) - Q'(x))^2}{R(x)} dx~.
\end{align*}
That completes the proof. \qed


\begin{lemm}
Consider a general NSI algorithm with updates of the form~\eqref{eq:nmia} with mini-batch size $B_t = b$. Then, for any trajectory $\w_{0:t-1}$, we have
\begin{align}
KL\left(P_{t|} \| P_{t|} \right) \leq  \frac{b^2}{n^2} \frac{n}{n-b} \E_{B_t \in G_1} \E_{A_t \in G_0} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t}(\bxi_t)} d\bxi_t \right]~.
\end{align}
\label{lemm:lsd}
\vspace*{-6mm}
\end{lemm}

\proof By definition,
\begin{align*}
KL\left(P_{t|} \| P'_{t|}\right) & \stackrel{(a)}{\leq} \left(\frac{b}{n} \right)^2 \left(\frac{n}{n-b}\right) \int_{\w} \frac{(Q - Q')^2}{R} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \bigintsss_{\w} \frac{ \left(  \frac{1}{|G_1|} \left[ \sum_{B \in G_1} P_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right] \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} P_{A,\bxi}(\w)} d\w \\
 & \stackrel{(b)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}\sum_{B \in G_1}  \frac{ \left(  P_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} P_{A,\bxi}(\w)} d\w \\
 & \stackrel{(c)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}  \sum_{B \in G_1} \left\{ \left(  P_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right)^2  \frac{1}{|G_0|}\sum_{A \in G_0} \frac{ 1 }{ P_{A,\bxi}(\w)} \right\} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \frac{1}{|G_1| |G_0|}  \sum_{B \in G_1} \sum_{A \in G_0}  \bigintsss_{\w} \frac{ \left( P_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right)^2 }{ P_{A,\bxi}(\w)} d\w ~,
\end{align*}
where (a) is from Lemma \ref{lemm:mix_bound}, (b)(c) is from Jensen's inequality since function $f(x) = x^2$ is convex and $f(x)=\frac{1}{x}$ is convex on $(0,\infty)$. That completes the proof. \qed



\theostab*

\subsection{Proofs for Section 2.4}

If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered very stable; if $\kappa_A=O(\sqrt[4]{n})$, then $A$ can be considered somewhat stable; and if $\kappa^2_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as the generalization error $\frac{1}{n}Y(S)$ itself. 

\theohighp*

%
%
\proof Let $S=(Z_1,\ldots,Z_n)$ and let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% % Let
% % \begin{align}
% % Y & = f(Z_1,\ldots,Z_n) \\
% % Y'_i & = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)~,~i=1,2,\ldots,n~.
% % \end{align}
With $(x)_+ = max(x,0)$, let
\begin{align}
    V^+ = V^+(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_+^2 ]~,
\end{align}
% % Let
% With $(x)_- = min(x,0)$, let
% \begin{align}
%     V^- = V^-(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~,
% \end{align}

Our proof uses the following exponential version of the Efron-Stein inequality [Theorem 6.16 in \cite{boucheron2013concentration}], whose proof is based on a combination of the symmetric modified log-Sobolev inequality [Theorem 6.15 in \cite{boucheron2013concentration}] with the change of measure:
\begin{theo}\label{theo:exp_efst}
Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
\begin{equation}
\log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
\end{equation}
\end{theo}

% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$ such that $(Y-Y'_i)$ is bounded and $\| Y-Y'_i\|_{\psi_2} = \kappa_A$. Then, with $(x)_+ = \max(0,x)$,
% \begin{equation}
% V^+_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
% \end{equation}
% is sub-Gaussian and $\| V_i^+ \|_{\psi_2} \leq 4\kappa_A^2$. \abcomment{should follow by definition, by bounding $L_p$ norms, since $Y-Y'_i$ is bounded.}
% \end{lemm}


For the proof of Theorem~\ref{theo:hp}, note that $V^+$ is sub-Gaussian with $\| V^+ \|_{\psi_2} \leq n \kappa_A^2$.
Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_2}$. Then from Theorem \ref{theo:exp_efst}, we have
\begin{align*}
\psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right].
\end{align*}
Then, by Markov's inequality we have
\begin{align*}
\log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
 & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
\end{align*}
Choosing $\theta = 1/(2\lambda)$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) 
& \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
\end{align*}
Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
\Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
\end{align*}
With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa_A^2$, with $c_1 = c_0 \sqrt{2}$, we have
\begin{align*}
\P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right) ~.
\end{align*}
Now, we choose $\delta$ such that
\begin{align*}
 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right)   
 \leq 8 \exp \left( - n \epsilon \right)  + 8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta~.
\end{align*}
It suffices to choose $\epsilon$ such that
\begin{align*}
8 \exp \left( - n \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{1}{n} \log \left( \frac{16}{\delta} \right) \\
8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{c_1 \kappa_A}{\sqrt{n}} \log \left( \frac{16}{\delta} \right)~.
\end{align*}
As a result,
\begin{align*}
\P\left( \frac{1}{n}(Y - \E Y) >  \max \left( \frac{1}{n}, \frac{c_1 \kappa_A}{\sqrt{n}} \right) \log \left( \frac{16}{\delta} \right) \right) & \leq \delta~.
\end{align*}
That completes the proof. \qed







% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of random variables. Let $Y= f(Z_1,\ldots,Z_n)$ be sub-Gaussian. Then $\E_{Z_i}[Y]$ is sub-Gaussian. 
% \end{lemm}

% \tcedit{Proof. By Jensen's inequality, we have for any convex function $f$,
% \begin{align*}
%     \E_{Z_2,\cdots, Z_n} f(\E_{Z_1}[Y])\leq \E_{Z_2,\cdots, Z_n} \E_{Z_1}f(Y) = \E f(Y),
% \end{align*}
% by taking $f(x) = |x|^p$, we have $\E_{Z_i}[Y]$ is sub-Gaussian with $\psi_2$ norm bounded by the $\psi_2$ norm of $Y$.}

% \tccomment{Checked.}

% \begin{corr}
% In the setting of Lemma ?, let $Z'_i$ be an independent copy of $Z_i$, and $Y'_i = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, $\E_{Z'_i}[Y'_i]$ is sub-Gaussian.
% \end{corr}

% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, with $(x)_+ = \max(0,x)$,
% \begin{equation}
% V_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
% \end{equation}
% is sub-Exponential. 
% \end{lemm}

% \begin{lemm}
% Let $V_1,\ldots,V_n$ be a set of (identically distributed) sub-Exponential random variables as in Lemma 2 such that $\| V_i \|_{\psi_1} \leq \kappa$ for $i=1,\ldots,n$. Then, 
% \begin{align}
%   \| V^+ \|_{\psi_1} = \left\| \sum_{i=1}^n V_i \right\|_{\psi_1} \leq n \kappa~. 
% \end{align}
% \end{lemm}
% \tcedit{Proof. By triangle inequality:
% \begin{align*}
%     \| V^+ \|_{\psi_1} = \left\| \sum_{i=1}^n V_i^+ \right\|_{\psi_1}\leq \sum_{i=1}^n \left\| V_i^+ \right\|_{\psi_1} \leq n \kappa.
% \end{align*}}\tccomment{checked}



% \subsubsection{Upper Tail Bound}

% The following result is a consequence of combining the Symmetric Modified Logarithmic Sobolev Inequalities (SM-LSI) and the change of measure inequality, which also forms the basis of PAC-Bayes bounds:
% \begin{theo}
% Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
% \begin{equation}
% \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
% \end{equation}
% \end{theo}
% Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_1}$. Then, we have
% \begin{align*}
% \psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right] 
% \end{align*}
% Then, by Markov's inequality we have
% \begin{align*}
% \log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
%  & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
% \end{align*}
% Choosing $\theta = 1/(2\lambda)$, we have 
% \begin{align*}
% \log \P( Y - \E Y > t ) 
% & \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
% \end{align*}
% Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
% \begin{align*}
% \log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
% \Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
% \end{align*}
% With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa$ for a constant $\kappa$, with $c_1 = c_0 \sqrt{2\kappa}$, we have
% \begin{align*}
% \P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \sqrt{n}/c_1 \right\} \epsilon \right) ~.
% \end{align*}
% \abcomment{Instead of $\epsilon$, write the bound in terms of $\log(1/\delta)$}

% \subsubsection{Lower Tail Bound}
% For the lower tail bound, we will use the following result which comes from combining LSI with Chebyshev's association inequality.
% \begin{theo}
% Assume that for some non-decreasing function $g : \R \mapsto \R$, 
% \begin{align*}
%     V^{-} \leq g(Y)~.
% \end{align*}
% Then for all $t > 0$,
% \begin{align*}
%     \P [ Y < \E Y -t ] \leq e^{-t^2/(4 \E [g(Y)])}~.
% \end{align*}
% \end{theo}

% We have
% \begin{align*}
%      V^- & = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~ \\
%      & \leq \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)^2 ] \\
%      & \leq 2 \sum_{i=1}^n \E_{S'} \left[ Y^2 + (Y'_i)^2 \right] \\
%      & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{S'}[ (Y'_i)^2] \\
%      & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{Z'_i}[ (Y'_i)^2] \\
%      & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{Z_i}[ Y^2] \\
%      & \triangleq g(Y)~.
% \end{align*}
% Further, note that
% \begin{align*}
%     \E[g(Y)] = |\E[g(Y)]| \leq \E|g(Y)| \leq \| g(Y) \|_{\psi_1} \leq c n \kappa~.
% \end{align*}
% As a result,
% \begin{align*}
%     \P [ Y < \E Y -t ] \leq e^{-t^2/(4c n \kappa)}~.
% \end{align*}
% With $t = n \epsilon$, we have
% \begin{align*}
%     \P [ Y < \E Y - n \epsilon ] \leq e^{-n\epsilon^2/(4 c \kappa)}~.
% \end{align*}


==> Neurips2021/app/guss.tex <==
\lemmaiabguss*


\proof Recall that we want to bound

\begin{align}
 \nr I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t},~~\text{where} ~~ \bxi_t \sim \cN(0, \sigma_t^2\mathbb{I}_d) ~. 
\end{align}

For Noisy SGD with Gaussian noise, we have $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ to be two Gaussian distributions with variance $\sigma_t^2\mathbb{I}_d$, and with mean $\m_{B_t}$ and $\m^\prime_{B_t}$ respectively to be
\begin{align*}
    \m_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t}) \\
    \m'_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_{B_t}) ~.
\end{align*}

Similarly, $P_{A_t,\bxi_t}$ is also a Gaussian noise with mean 
$\m_{A_t}  = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{A_t})$. 
Thus, for any $B_t$ and $A_t$, since $P_{B_{t}, \boldsymbol{\xi}_{t}}$, $P^\prime_{B_{t}, \boldsymbol{\xi}_{t}}$ and $P_{A_{t}, \boldsymbol{\xi}_{t}}$ are Gaussian distributions, $d P_{B_{t}, \boldsymbol{\xi}_{t}}$, $d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}$ and $d P_{A_{t},\boldsymbol{\xi}_{t}}$ are distribution density functions of Gaussian distribution. Then, it is straightforward to have 
\begin{align}
\nr I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{d}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w-\m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
\end{align}
Note that the above calculation considers integral over $d$-dimensional space which introduced an undesired dimension dependence. However, isotropic Gaussian noise is spherical symmetric, we can translate and rotate the coordinate system so that 
$\m_{A_t}=0$  and $ \m_{B_t}, \m_{B_t}^{\prime}$ are mapped to a 2-dimensional space and the Euclidean distances $\|\w-\m_{B_t} + \m_{A_t}\|$, $\|\w-\m_{B_t}^\prime + \m_{A_t}\|$ do not change.  Now, we omit the subscript $t$ in $A_t$, $B_t$, $\bxi_t$ and $\sigma_t$, since the analysis below holds at any $t$-th iteration. We first translate them by $\m_A$ and write $\Delta \m = \m_B - \m_A$, $\Delta \m' = \m'_B - \m_A$. 
% \begin{align*}
%      p_{\m_B,\sigma} \rightarrow x - \m_B + \m_A = x - \Delta \m 
% \end{align*}
% \begin{align*}
%      p_{\m'_B,\sigma} \rightarrow x - \m'_B + \m_A = x - \Delta \m'
% \end{align*}
% \begin{align*}
%      p_{\m_A,\sigma} \rightarrow x - \m_A + \m_A = x~.
% \end{align*}

Let $\w$ be a $d$-dimensional Gaussian distribution with zero mean. Fix a basis $\mathbf{b}_1,...,\mathbf{b}_p$ and draw $\w$ by first drawing signed lengths $\lambda_{i} \sim \mathcal{N}\left(0, \sigma^{2}\right), \text { for } i \in[d]$, then $\w = \sum_{i=1}^d \lambda_i \mathbf{b}_i$. We can choose the basis such that $\Delta \m$ and $\Delta \m'$ are parallel to $\mathbf{b}_1$ and $\mathbf{b}_2$ such that $\Delta \m = a_1 \mathbf{b}_1 + a_2 \mathbf{b}_2$ and $\Delta \m' = a'_1 \mathbf{b}_1 + a'_2 \mathbf{b}_2$. Note that $a_1^2 + a_1^2 = \|\Delta \m\|_2^2 = \|\m_B - \m_A\|_2^2$ and $a'_1^2 + a'_1^2 = \|\Delta \m'\|_2^2 = \|\m'_B - \m'_A\|_2^2$
\begin{align*}
I_{A,B}  & = \bigintsss_\w \frac{ \left(  d P_{\m_B,\bxi} -    d P_{\m'_B,\bxi} \right)^2 }{  d P_{\m_A,\bxi}} d \w   \\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| \w -  \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| \w -  \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \w -  \m_A\|_2^2/2\sigma^2)} d \w  ~\\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| \w -  \Delta\m \|_2^2 / 2\sigma^2 ) - \exp(- \| \w -  \Delta \m'\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x\|_2^2/2\sigma^2)} d \w ~ \\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\sum_{i=1}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~ \\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(-  (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2+ \sum_{i=3}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~\\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\mathbb{R}^2} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2)} d_{\lambda_1, \lambda_2}~\\
 & \qquad \cdot \bigints_{\mathbb{R}^{d-2}}\frac{1}{(\sqrt{2 \pi} \sigma)^{d-2}} \exp(- \sum_{i=3}^d \lambda_i^2/2\sigma^2) ~ d_{\lambda_3,...,\lambda_d} \\
 & =  \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\x \in \mathbb{R}^2} \frac{ \bigg( \exp(- \|\x -  \Delta \m \|_2^2 / 2\sigma^2 ) - \exp(- \|\x -  \Delta \m'\|_2^2 / 2\sigma^2 )\bigg)^2 }{\exp( - \|\x\|_2^2 / 2\sigma^2)} d_{\x}
\end{align*}
We abuse the notation and write $ \m_B - \m_A = \Delta \m$ and $ \m'_B - \m_A = \Delta \m'$ as a two dimensional vector with the norm preserved. Then 
\begin{align*}
I_{A,B} 
 = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\x \in \mathbb{R}^p} \frac{ \bigg( \exp(- \| \x -  \m_B + \m_A \|_2^2 / 2\sigma^2 ) - \exp(- \| \x -  \m'_B + \m_A\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \x \|_2^2/2\sigma^2)} d \x ~.
\end{align*}



Then
we have $I_{A_t, B_t}$ as 
\begin{align}
I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{2}} \int_{\x} \frac{\left(\exp \left(-\left\|\x-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\x-\m_{B}^{\prime} + \m_{A_t} \right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \x~.
\end{align}
Then we treat $\exp \left(-\left\|\x-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ and $\exp \left(-\left\|\x-\m_{B_t}^\prime + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ as two functions of $\x$ where we can 
use Taylor expansion and apply mean-field theorem. Thus, 
%to bound $I_{A_t, B_t}$ as
for each $\x$, we have:
\begin{align*}
 \exp(- \| \x - \m_B +  {\m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| \x - \m'_B +  {\m_A}\|_2^2 / 2\sigma^2 ) 
 & = \bigg\langle \m_B - \m'_B , \nabla \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
\end{align*}
where $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B  {- \m_A}$, where $\alpha_x \in [0,1]$ depends on $\x$. 
Let $\| \tilde{\m}_B\|_2 \leq \max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2) \triangleq \bar{\m}_B$. 

We have
\begin{align*}
  \nabla \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2) & = -\frac{\x -\tilde{\m}_B}{\sigma^2} \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2)~, 
\end{align*}
so that
\begin{align*}
& \frac{ \bigg( \exp(- \| \x - \m_B  { + \m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| \x - \m'_B  { + \m_A} \|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
= \frac{\bigg\langle \m_B - \m'_B , -\frac{\x -\tilde{\m}_B}{\sigma^2} \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{\| \m_B - \m'_B \|_2^2 \| \frac{\x -\tilde{\m}_B}{\sigma^2} \|_2^2 \exp(- \| \x - \tilde{\m}_B\|_2^2 / \sigma^2) }{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|\x\|^2 + \| \tilde {\m}_B \|_2^2 \bigg)  \exp\left(-\frac{\| \x-\tilde{\m}_B\|_2^2}{\sigma^2} + \frac{\|\x\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
= \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|\x\|^2 + \|  \tilde{\m}_B \|_2^2 \bigg)  \exp\left( \frac{ {3}\|\tilde{\m}_B\|_2^2}{ {2}\sigma^2}\right)  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
\leq \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{ {3}\|\bar{\m}_B\|_2^2}{ {2}\sigma^2}\right) \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) ~.
\end{align*}

Since $\tilde{\m}_B$ interpolate between $\m_B  { - \m_A}$ and $\m'_B  { - \m_A} $ and $\exp$ is positive, based on Proposition \ref{prop:mid_step}, with $\m = 2(\m_B  { - \m_A})$, $\m' = 2(\m'_B  { - \m_A})$ and $\tilde \m = 2 \tilde \m_B$,
we have 
% \abcomment{This step is not correct, should be fixable with a scale factor}
% \begin{align*}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left(-\frac{\|x-2(\m_B   { - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2(\m'_B   { - \m_A})\|_2^2}{2\sigma^2}~, \right) 
% \end{align*}

\begin{align*}
\exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) 
\max\left(\exp\left(-\frac{\|\x -2\m_B + 2\m_A\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|\x -2\m_B' + 2\m_A\|_2^2}{\sigma^2}\right) \right)\\
& \leq \exp \left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \left(\exp\left(-\frac{\|\x -2\m_B + 2\m_A\|_2^2}{\sigma^2}\right) + \exp\left(-\frac{\|\x -2\m_B' + 2\m_A\|_2^2}{\sigma^2}\right) \right)
\end{align*}

% \begin{align*}
% \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) \leq \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right).
% \end{align*}



Continuing
\begin{align*}
& \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) d\x \\
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)  \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|\x-2(\m_B { - \m_A})\|_2^2}{2\sigma^2} \right) d\x \\ 
& \phantom{\leq ......} + \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|\x-2(\m'_B  { - \m_A})\|_2^2}{2\sigma^2} \right) d\x \\
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \bigg( 2\sigma^2 + 4\|\m_B  { - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 + 2\sigma^2 + 4\|\m'_B  { - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) \\
& \leq 4 \big(\sigma^2 + \|\m_B  { - \m_A}\|_2^2 + \|\m'_B   { - \m_A} \|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)
\end{align*}


Putting everything back together, we have 
%\yzcomment{Now it just depends on the gradient difference.}
\begin{align*}
I_{A,B} & \leq \frac{1}{2\pi \sigma^2} \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{ {3}\|\bar{\m}_B\|_2^2}{ {2}\sigma^2}\right) 4 \big(\sigma^2 + \|\m_B  { - \m_A}\|_2^2 + \|\m'_B  { - \m_A}\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)\\
& \leq \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{ \|\bar{\m}_B\|_2^2}{2\sigma^2} \bigg) \exp\left( \frac{3\|\bar{\m}_B\|_2^2}{2\sigma^2}\right)~\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \|\m_B-\m_B'\|_2^2 \\
& = \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2)^2}{2\sigma^2} \bigg) \\
& \qquad \exp\left( \frac{\max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2)\|_2^2}{\sigma^2}\right)~\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)\|\m_B-\m_B'\|_2^2
\end{align*}

Now we are interested in $\|\m_B -\m_A\|_2$,  $\|\m'_B -\m_A\|_2$ and $\|\m_B -\m_B'\|_2$. Recall that we have $B \in G_1$ which contains the $z_n'$ and $A \in G_0$: 
\begin{align*}
    \m_B & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_B) \\
    \m'_B & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_B) ~.
\end{align*}
\begin{align*}
    \m_A & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_A) ~.
\end{align*}

So that 

\begin{align*}
\m_B - \m_A & = \eta_t \nabla \ell(\w_{t-1},S_B)  - \eta_t \nabla \ell(\w_{t-1},S_A) \\
& = \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell(\w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(\w_{t-1},\tilde{z}) \right]~,
\end{align*}
and
\begin{align*}
\m'_B - \m_A & = \eta_t \nabla \ell(\w_{t-1},S'_B)  - \eta_t \nabla \ell(\w_{t-1},S_A) \\
& = \frac{\eta_t}{m} \left[ \sum_{z \in S'_B} \nabla \ell(\w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(\w_{t-1},\tilde{z}) \right]~.
\end{align*}
Also, 
\begin{align*}
\m'_B - \m_B = \frac{\eta_t}{m} \left( \nabla \ell (\w_{t-1}, z_n) - \nabla \ell (\w_{t-1}, z'_n) \right) ~.  
\end{align*}

Let $\Delta_t(\bar{S}) \triangleq \max_{z,\tilde{z} \in \bar{S}} \| \nabla \ell(w_{t-1},z) - \nabla \ell( \w_{t-1},\tilde{z}) \|_2$, where $\bar{S} \sim D^{n+1}$ as before. Now, note that 
%\abcomment{note that the pairing $(z_i,\tilde{z}_i)$ below is arbitrary, the analysis does not depend on the pairing}
\begin{align*}
\| \m_B - \m_A \|_2^2 & = \left\| \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell( \w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell( \w_{t-1},\tilde{z} \right] \right\|_2^2 \\
& \leq \eta_t^2 \left\| \frac{1}{m} \sum_{i=1}^m \big( \nabla \ell( \w_{t-1},z_i) - \nabla \ell( \w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
& \leq \eta_t^2 \frac{1}{m} \sum_{i=1}^m  \left\|  \big( \nabla \ell( \w_{t-1},z_i) - \nabla \ell( \w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
& \leq \eta_t^2 \Delta^2_t(\bar{S})~.
\end{align*}

Also, $\| \m_B' - \m_A \|_2^2 \leq \eta_t^2 \Delta^2_t(\bar{S})$ and  $\| \m_B' - \m_B \|_2^2 \leq \eta_t^2 \Delta^2_t(\bar{S})$. With the setting that $ \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \leq \ln 3/2$, we have

\begin{align}
I_{A_t, B_t} \leq  \frac{\|\m_{B_t} - \m_{B_t}^\prime \|_2^2}{\sigma_t^2}=  18(1+ \frac{5}{2}\ln\frac{3}{2})\ln \frac{3}{2} \frac{\eta_t^2\left\|\nabla \ell\left( \w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}}{\sigma_t^2}~, \label{eq:guss_with_c}
\end{align}
That completes the proof. \qed


\genboundguss*

\proof Based on Lemma \ref{lemm:iab_guss}, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate,  we have
\begin{align}
\nr K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right) & = \underset{B_{t} \in G_{1},A_{t} \in G_{0}}{\mathbb{E}}\left[\int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}\right]   \leq  \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c = 41 \ln \frac{3}{2}$ based on \eqref{eq:guss_with_c}.

Then, based on the chain rule of KL-divergence, we have
\begin{align}
\nr K L\left(P_{0: T} \| P_{0: T}^{\prime}\right) 
& = \sum_{t=1}^{T} \mathbb{E}_{\w_{t-1}} \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

Following Theorem \ref{theo:stab}, we have
\begin{align*}
\left|\mathbb{E}_{S}\left[L_{D}\left(\mathbf{w}_{T}\right)-L_{S}\left(\mathbf{w}_{T}\right)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar{S}} \sqrt{\sum_{t=1}^{T} \underset{\mathbf{w}_{t-1}}{\mathbb{E}}\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z_{n}\right)-\ell\left(\mathbf{w}_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]},  
\end{align*}
where $c = 41 \ln \frac{3}{2}$. 


\begin{prop}
Assume $\m,\m'$ fixed and $\tilde{\m}$ on the line segment of $\m$ and $\m'$, we have
    \begin{align*}
    \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) \leq \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right).
\end{align*} \label{prop:mid_step}
\end{prop}

\proof  From the law of cosine, we have 
\begin{align*}
    \|x -\m\|_2^2 = \|x-\tilde{\m}\|_2^2 + \|\m-\tilde{\m}\|_2^2 -2 \|x-\tilde{\m}\|_2  \|\m-\tilde{\m}\|_2 \cos \angle x\tilde{\m} \m,
\end{align*}
and
\begin{align*}
    \|x -\m'\|_2^2 = \|x-\tilde{\m}\|_2^2 + \|\m'-\tilde{\m}\|_2^2 -2 \|x-\tilde{\m}\|_2  \|\m'-\tilde{\m}\|_2 \cos \angle x\tilde{\m} \m',
\end{align*}
where $\angle x\tilde{\m} \m + \angle x\tilde{\m} \m' = \frac{\pi}{2}$ so we have $\cos\angle x\tilde{\m} \m + \cos\angle x\tilde{\m} \m' = 0$. By canceling out $\cos$ via weighted sum of the above two equations, we have
\begin{align*}
    &\|x -\m\|_2^2 \|\m'-\tilde{\m}\|_2 + \|x -\m'\|_2^2 \|\m-\tilde{\m}\|_2\\
    =& \|x-\tilde{\m}\|_2^2\|\m'-\tilde{\m}\|_2 + \|\m-\tilde{\m}\|_2^2\|\m'-\tilde{\m}\|_2 + \|x-\tilde{\m}\|_2^2\|\m-\tilde{\m}\|_2 + \|\m'-\tilde{\m}\|_2^2\|\m-\tilde{\m}\|_2.
\end{align*}
Equivalently we have 
\begin{align*}
    \|x-\tilde{\m}\|_2^2 = \frac{\|\m-\tilde{\m}\|_2}{\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2} \|x -\m'\|_2^2 + \frac{\|\m'-\tilde{\m}\|_2}{\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2} \|x -\m\|_2^2 - \|\m-\tilde{\m}\|_2\|\m'-\tilde{\m}\|_2.
\end{align*}
Since $\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2 = \|\m-\m'\|_2$, from AM-GM inequality we have
\begin{align*}
    \|x-\tilde{\m}\|_2^2\geq \min \left(\|x -\m\|_2^2,\|x -\m'\|_2^2\right) - \frac{1}{4} \|\m-\m'\|_2^2,
\end{align*}
therefore we have
\begin{align*}
    \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) &\leq \exp\left(-\min \left(\frac{\|x -\m\|_2^2}{\sigma^2},\frac{\|x -\m'\|_2^2}{\sigma^2}\right) + \frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\\
    &= \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right),
\end{align*}
which completes the proof.
\qed





% Consider two collection of points $\{\m_B : B \in G \}$ and $\{\m_B : B \in G\}$. In our context, at any stage $t$, conditioned on $w_{t-1}$, for mini-batch $B$, we have
% \begin{align*}
%     \m_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S_B) \\
%     \m'_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S'_B) ~.
% \end{align*}
% Let $p_{\m,\sigma}$ denote the Gaussian distribution $\cN(\m, \sigma^2 \I)$.


% If the noise added is Gaussian, without loss of generality, we can translate and rotate the coordinate system so that $\m_A=0$, and $\m_B,\m'_B$ have the last $(d-2)$ coordinates as 0. With abuse of notation, we denote the first two coordinates of $\m_A,\m_B,\m'_B$ as $\m_{A},\m_B,\m'_B$, noting that the remaining $(d-2)$ coordinates are 0.  Note that the translation and rotation does not change the Euclidean distances $\|\m_B - \m'_B\|_2$, $\|\m_B - \m_A\|_2 = \| \m_B \|_2$, and $\|\m'_B - \m_A\|_2 = \| \m'_B \|_2$. Then, since the integral over the last $(d-2)$ simply cancel out the partition function $1/(\sqrt{2\pi \sigma^2}^{d-2}$, we have
% \yzcomment{I think it should be  $\exp(- \| x - \m_B + \m_A\|_2^2/2\sigma^2  )$ and  $\exp(- \| x - \m'_B + \m_A\|_2^2/2\sigma^2  )$}
% \begin{align*}
% I_{A,B}  & = \bigintsss_x \frac{ \left(  p_{\m_B,\sigma} -   p_{\m'_B,\sigma} \right)^2 }{ p_{\m_A,\sigma}} d \w  \\

%  = \frac{1}{2\pi \sigma^2} \bigints_\w \frac{ \bigg( \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} d \w ~,
% \end{align*}
% where the latter is a 2-d integral. For each $\w$, we can apply mean-field theorem [][] to get:
% \begin{align*}
%  \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) 
%  & = \bigg\langle \m_B - \m'_B , \nabla \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
% \end{align*}
% where $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B$, where $\alpha_x \in [0,1]$ depends on $\w$. Note that $\| \tilde{\m}_B\|_2 \leq \max(\|\m_B\|_2,\|\m'_B\|_2) \triangleq \bar{\m}_B$. We have
% \begin{align*}
%   \nabla \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2) & = -\frac{x -\tilde{\m}_B}{\sigma^2} \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2)~, 
% \end{align*}
% so that
% \begin{align*}
% & \frac{ \bigg( \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% = \frac{\bigg\langle \m_B - \m'_B , -\frac{x -\tilde{\m}_B}{\sigma^2} \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% \leq \frac{\| \m_B - \m'_B \|_2^2 \| \frac{x -\tilde{\m}_B}{\sigma^2} \|_2^2 \exp(- \| x - \tilde{\m}_B\|_2^2 / \sigma^2) }{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% \leq \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \exp\left(-\frac{\|x-\tilde{\m}_B\|_2^2}{\sigma^2} + \frac{\|x\|_2^2}{2\sigma^2} \right) \\
% & \phantom{......................} 
% = \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \exp\left( \frac{\|\tilde{\m}_B\|_2^2}{\sigma^2}\right)  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) \\
% & \phantom{......................} 
% \leq \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{\|\bar{\m}_B\|_2^2}{\sigma^2}\right) \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) ~.
% \end{align*}
% % Now, consider the random variable $\tilde{X} \sim \cN(\tilde{\m}_B, \sigma^2 )$. 
% % Note that $\tilde{X}$ is sub-Gaussian with $\| \tilde{X} \|_{\psi_2} \leq c_0 (\sigma^2 + \| \tilde{\m}_B\|_2^2) \leq c_0 (\sigma^2 + \|\bar{\m}_B\|_2^2)$, where $c_0$ is an absolute constant. Then \abcomment{this needs to be shown, some variant of this should be true}, for an absolute constant $c_1$ \abcomment{apply Jensen's?}
% Since $\tilde{\m}_B$ interpolate between $\m_B$ and $\m'_B$ and $\exp$ is positive, we have
% \begin{align*}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left(-\frac{\|x-2\m_B\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2\m'_B\|_2^2}{2\sigma^2}~, \right) 
% \end{align*}
% so that
% \begin{align*}
% \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) & \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) d \w  \\
% & \leq \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|x-2\m_B\|_2^2}{2\sigma^2} \right) d \w  \\ 
% & \phantom{\leq ......} + \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|x-2\m'_B\|_2^2}{2\sigma^2} \right) d \w  \\
% & \leq \bigg( 2\sigma^2 + 4\|\m_B\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) + \bigg( 2\sigma^2 + 4\|\m'_B\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) \\
% & \leq 4 \big(\sigma^2 + \|\m_B\|_2^2 + \|\m'_B\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)
% \end{align*}

% \yzcomment{It is better to work with gradient difference, instead of $\m_B$ and $\bar \m_B$ which contains $w$.}

% Putting everything back together, we have 
% \begin{align*}
% I_{A,B} & \leq \frac{1}{2\pi \sigma^2} \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{\|\bar{\m}_B\|_2^2}{\sigma^2}\right) 4 \big(\sigma^2 + \|\m_B\|_2^2 + \|\m'_B\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\\
% & \leq \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B\|_2^2}{\sigma^2} + \frac{\|\m'_B\|_2^2}{\sigma^2} + \frac{ \|\bar{\m}_B\|_2^2}{2\sigma^2} \bigg) \exp\left( \frac{\|\bar{\m}_B\|_2^2}{\sigma^2}\right)~~\| \m_B - \m'_B \|_2^2
% \end{align*}


% \yzcomment{ --------- updated analysis below --------}

% Details on the rotation and translation:\\
% We are interested in three $d$-dimensional Gaussian distributions:
% \begin{align*}
%  p_{\m_B,\sigma} =   \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 )~,
% \end{align*}
% \begin{align*}
%  p_{\m'_B,\sigma} =   \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 )~,
% \end{align*}
% \begin{align*}
%  p_{\m_A,\sigma} =   \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \exp(- \| x - \m_A\|_2^2 / 2\sigma^2 )~.
% \end{align*}
% By definition, we want to calculate:
% \begin{align*}
% I_{A,B}  = \bigintsss_x \frac{ \left(  p_{\m_B,\sigma} -   p_{\m'_B,\sigma} \right)^2 }{ p_{\m_A,\sigma}} d \w  
%  = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x - \m_A\|_2^2/2\sigma^2)} d \w ~.
% \end{align*}
% Since Gaussian is a spherically symmetric normal which
% is independent of the orthogonal basis from which its constituent
% normals are drawn. We first translate three of them by $\m_A$ and write $\Delta \m = \m_B - \m_A$, $\Delta \m' = \m'_B - \m_A$:
% \begin{align*}
%      p_{\m_B,\sigma} \rightarrow x - \m_B + \m_A = x - \Delta \m 
% \end{align*}
% \begin{align*}
%      p_{\m'_B,\sigma} \rightarrow x - \m'_B + \m_A = x - \Delta \m'
% \end{align*}
% \begin{align*}
%      p_{\m_A,\sigma} \rightarrow x - \m_A + \m_A = x~.
% \end{align*}
% Note that $\w$ is a $d$-dimensional Gaussian distribution with zero mean. $\w$ is a  spherically symmetric distribution. Fix a basis $\mathbf{b}_1,...,\mathbf{b}_p$ and draw $\w$ by first drawing signed lengths $\lambda_{i} \sim \mathcal{N}\left(0, \sigma^{2}\right), \text { for } i \in[d]$, then $x = \sum_{i=1}^d \lambda_i \mathbf{b}_i$. We can choose the basis such that $\Delta \m$ and $\Delta \m'$ are parallel to $\mathbf{b}_1$ and $\mathbf{b}_2$ such that $\Delta \m = a_1 \mathbf{b}_1 + a_2 \mathbf{b}_2$ and $\Delta \m' = a'_1 \mathbf{b}_1 + a'_2 \mathbf{b}_2$. Note that $a_1^2 + a_1^2 = \|\Delta \m\|_2^2 = \|\m_B - \m_A\|_2^2$ and $a'_1^2 + a'_1^2 = \|\Delta \m'\|_2^2 = \|\m'_B - \m'_A\|_2^2$
% \begin{align*}
% I_{A,B}  & = \bigintsss_x \frac{ \left(  p_{\m_B,\sigma} -   p_{\m'_B,\sigma} \right)^2 }{ p_{\m_A,\sigma}} dx 
%  = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| x - \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x - \m_A\|_2^2/2\sigma^2)} dx ~\\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| x - \Delta\m \|_2^2 / 2\sigma^2 ) - \exp(- \| x - \Delta \m'\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x\|_2^2/2\sigma^2)} dx~ \\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_{\mathbb{R}^d} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\sum_{i=1}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~ \\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_{\mathbb{R}^d} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(-  (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2+ \sum_{i=3}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~\\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\mathbb{R}^2} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2)} d_{\lambda_1, \lambda_2}~\\
%  & \qquad \cdot \bigints_{\mathbb{R}^{d-2}}\frac{1}{(\sqrt{2 \pi} \sigma)^{d-2}} \exp(- \sum_{i=3}^d \lambda_i^2/2\sigma^2) ~ d_{\lambda_3,...,\lambda_d} \\
%  & =  \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{x \in \mathbb{R}^2} \frac{ \bigg( \exp(- \|x - \Delta \m \|_2^2 / 2\sigma^2 ) - \exp(- \|x - \Delta \m'\|_2^2 / 2\sigma^2 )\bigg)^2 }{\exp( - \|x\|_2^2 / 2\sigma^2)} d_{x}
% \end{align*}
% We abuse the notation and write $ \m_B - \m_A = \Delta \m$ and $ \m'_B - \m_A = \Delta \m'$ as a two dimensional vector with the norm preserved. Then 
% \begin{align*}
% I_{A,B}  = \bigintsss_x \frac{ \left(  p_{\m_B,\sigma} -   p_{\m'_B,\sigma} \right)^2 }{ p_{\m_A,\sigma}} dx 
%  = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{x \in \mathbb{R}^p} \frac{ \bigg( \exp(- \| x - \m_B + \m_A \|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B + \m_A\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} dx~.
% \end{align*}


% \yzcomment{----------- below mainly follows Prof. Banerjee's analysis ------}

% For each $\w$, we can apply mean-field theorem [][] to get:
% \begin{align*}
%  \exp(- \| x - \m_B + \yzedit{\m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B + \yzedit{\m_A}\|_2^2 / 2\sigma^2 ) 
%  & = \bigg\langle \m_B - \m'_B , \nabla \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
% \end{align*}
% where $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B \yzedit{- \m_A}$, where $\alpha_x \in [0,1]$ depends on $\w$. Note that $\| \tilde{\m}_B\|_2 \leq \max(\|\m_B \yzedit{-\m_A}\|_2,\|\m'_B \yzedit{-\m_A} \|_2) \triangleq \bar{\m}_B$. We have
% \begin{align*}
%   \nabla \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2) & = -\frac{x -\tilde{\m}_B}{\sigma^2} \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2)~, 
% \end{align*}
% so that
% \begin{align*}
% & \frac{ \bigg( \exp(- \| x - \m_B \yzedit{ + \m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \m'_B \yzedit{ + \m_A} \|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% = \frac{\bigg\langle \m_B - \m'_B , -\frac{x -\tilde{\m}_B}{\sigma^2} \exp(- \| x - \tilde{\m}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% \leq \frac{\| \m_B - \m'_B \|_2^2 \| \frac{x -\tilde{\m}_B}{\sigma^2} \|_2^2 \exp(- \| x - \tilde{\m}_B\|_2^2 / \sigma^2) }{\exp(-\| x \|_2^2/2\sigma^2)} \\
% & \phantom{......................} 
% \leq \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|x\|^2 + \| \tilde {\m}_B \|_2^2 \bigg)  \exp\left(-\frac{\|x-\tilde{\m}_B\|_2^2}{\sigma^2} + \frac{\|x\|_2^2}{2\sigma^2} \right) \\
% & \phantom{......................} 
% = \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|x\|^2 + \|  \tilde{\m}_B \|_2^2 \bigg)  \exp\left( \frac{\yzedit{3}\|\tilde{\m}_B\|_2^2}{\yzedit{2}\sigma^2}\right)  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) \\
% & \phantom{......................} 
% \leq \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{\yzedit{3}\|\bar{\m}_B\|_2^2}{\yzedit{2}\sigma^2}\right) \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) ~.
% \end{align*}
% % Now, consider the random variable $\tilde{X} \sim \cN(\tilde{\m}_B, \sigma^2 )$. 
% % Note that $\tilde{X}$ is sub-Gaussian with $\| \tilde{X} \|_{\psi_2} \leq c_0 (\sigma^2 + \| \tilde{\m}_B\|_2^2) \leq c_0 (\sigma^2 + \|\bar{\m}_B\|_2^2)$, where $c_0$ is an absolute constant. Then \abcomment{this needs to be shown, some variant of this should be true}, for an absolute constant $c_1$ \abcomment{apply Jensen's?}
% Since $\tilde{\m}_B$ interpolate between $\m_B \yzedit{ - \m_A}$ and $\m'_B \yzedit{ - \m_A} $ and $\exp$ is positive, we have \abcomment{This step is not correct, should be fixable with a scale factor}
% \begin{align*}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left(-\frac{\|x-2(\m_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2(\m'_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2}~, \right) 
% \end{align*}
% \begin{prop}
% We have 
% \begin{align}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left( \frac{\| \m_B - \m'_B \|_2^2}{2\sigma^2} \right) \exp\left(-\frac{\|x-2(\m_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2(\m'_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2}~ \right)~.     
% \end{align}
% \end{prop}
% \abcomment{needs a proof}
% \proof (outline, need to check) Consider the ratio and note that we can set $x=\tilde{\m}_B$. Then, the problem reduces to lower bounding
% \begin{align*}
% \exp\left(-\frac{\|\tilde{\m}_B-2(\m_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|\tilde{\m}_B -2(\m'_B  \yzedit{ - \m_A})\|_2^2}{2\sigma^2}~ \right)~,
% \end{align*}
% which gives the desired bound. \qed





% \abcomment{We should use the fact that integral (expectation) is really 1-d}

% Continuing
% \begin{align*}
% \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) & \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) dx \\
% & \leq \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|x-2(\m_B \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) dx \\ 
% & \phantom{\leq ......} + \bigintss_x \bigg(\|x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|x-2(\m'_B \yzedit{ - \m_A})\|_2^2}{2\sigma^2} \right) dx \\
% & \leq \bigg( 2\sigma^2 + 4\|\m_B \yzedit{ - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) + \bigg( 2\sigma^2 + 4\|\m'_B \yzedit{ - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) \\
% & \leq 4 \big(\sigma^2 + \|\m_B \yzedit{ - \m_A}\|_2^2 + \|\m'_B  \yzedit{ - \m_A} \|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)
% \end{align*}


% Putting everything back together, we have \yzcomment{Now it just depends on the gradient difference.}
% \begin{align*}
% I_{A,B} & \leq \frac{1}{2\pi \sigma^2} \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{\yzedit{3}\|\tilde{\m}_B\|_2^2}{\yzedit{2}\sigma^2}\right) 4 \big(\sigma^2 + \|\m_B \yzedit{ - \m_A}\|_2^2 + \|\m'_B \yzedit{ - \m_A}\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\\
% & \leq \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B \yzedit{ - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B \yzedit{ - \m_A}\|_2^2}{\sigma^2} + \frac{ \|\bar{\m}_B\|_2^2}{2\sigma^2} \bigg) \exp\left( \frac{\|\bar{\m}_B\|_2^2}{\sigma^2}\right)~~\| \m_B - \m'_B \|_2^2 \\
% & = \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B \yzedit{ - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B \yzedit{ - \m_A}\|_2^2}{\sigma^2} + \frac{\max(\|\m_B \yzedit{-\m_A}\|_2,\|\m'_B \yzedit{-\m_A} \|_2)^2}{2\sigma^2} \bigg) \\
% & \qquad \exp\left( \frac{\max(\|\m_B \yzedit{-\m_A}\|_2,\|\m'_B \yzedit{-\m_A} \|_2)\|_2^2}{\sigma^2}\right)~~\| \m_B - \m'_B \|_2^2
% \end{align*}

% \abcomment{I think the first part $(1+x^2+y^2+z^2)$ term can be avoided. See how it is being done for the subG case, based on the ``projection view" (PV), i.e., the analysis is essentially 1-dimensional. I will help transfer that argument to Gaussian. The main term $\exp(\Delta \m^2/\sigma^2)$ will stay, but we expect that.}

% \yzcomment{-------- Calculate KL-divergence ----------}

% Note that we are interested in $\|\m_B -\m_A\|_2$ and  $\|\m'_B -\m_A\|_2$. Recall that $B \in G_1$ which contains the $z_n'$ and $A \in G_0$ which contains the same mini-batch for $w$ and $w'$: 
% \begin{align*}
%     \m_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S_B) \\
%     \m'_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S'_B) ~.
% \end{align*}
% \begin{align*}
%     \m_A & = w_{t-1} - \eta_t \nabla F(w_{t-1},S_A) ~.
% \end{align*}

% So that \abcomment{minor typo: second line is based on gradient, not loss. Assume gradient is subG, for a fixed $w_{t-1}$, then we can get a $1/\sqrt{b}$ concentration. Also, the analysis may improve based on the "projection view".}
% \begin{align*}
% \m_B - \m_A & = \eta_t \nabla F(w_{t-1},S_B)  - \eta_t \nabla F(w_{t-1},S_A) \\
% %& = \eta _t \frac{1}{b} \left(\sum_{z \in \{S_B/z_{n}\} } \nabla \ell (w_{t-1}, z) + \ell (w_{t-1}, z_n) - \sum_{z \in \{S_A\} } \nabla \ell (w_{t-1}, z) \right)  \\
% & = \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell(w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(w_{t-1},\tilde{z}) \right]~,
% \end{align*}
% and
% \begin{align*}
% \m'_B - \m_A & = \eta_t \nabla F(w_{t-1},S'_B)  - \eta_t \nabla F(w_{t-1},S_A) \\
% %& = \eta _t \frac{1}{b} \left(\sum_{z \in \{S_B/z_{n}\} } \ell (w_{t-1}, z) + \ell (w_{t-1}, z'_n) - \sum_{z \in \{S_A\} } \ell (w_{t-1}, z) \right)  \\
% %& \triangleq \eta_t \Delta_t({S'_B,S_A})~
% & = \frac{\eta_t}{m} \left[ \sum_{z \in S'_B} \nabla \ell(w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(w_{t-1},\tilde{z}) \right]~.
% \end{align*}
% Also, 
% \begin{align*}
% \m'_B - \m_B = \frac{\eta_t}{m} \left( \nabla \ell (w_{t-1}, z_n) - \nabla \ell (w_{t-1}, z'_n) \right) ~.  
% \end{align*}

% Let $A_*$ and $B_*$ be the set that maximize $\|\m_B - \m_A\|^2$  and $\|\m'_B - \m_A\|^2$.  \abcomment{Lets see if we can avoid bounding things by $I_{A*,B*}$. We can assume that the stochastic gradients are sub-Gaussian, so an average over $b$ samples will have concentration with rate $1/\sqrt{b}$. Alternative is to assume expected gradient discrepancy is bounded. The goal is to avoid taking sup over samples/mini-batches. We already have the result as an expectation over mini-batches, lets keep that if possible.}
% Now we put $I_{A,B}$ back to the KL-divergence and set $b \leq \frac{n}{2}$: 
% \begin{align*}
%  & KL(w_t | w_{t-1} \| w_t' | w_{t-1})  \\
%  & \leq \frac{b^{2}}{n^{2}}\left(1+\frac{b}{n-b}\right) \frac{1}{\left|G_{0}\right|\left|G_{1}\right|} \sum_{A \in G_{0}} \sum_{B \in G_{1}} \int_{x} \frac{\left(p_{\m_{B}, \sigma}-p_{\m_{B}^{\prime}, \sigma}\right)^{2}}{p_{\m_{A}, \sigma}} d x = \frac{b^{2}}{n^{2}}\left(1+\frac{b}{n-b}\right) \frac{1}{\left|G_{0}\right|\left|G_{1}\right|} \sum_{A \in G_{0}} \sum_{B \in G_{1}} I_{A,B} \\
%  & \leq \frac{b^{2}}{n^{2}}\left(1+\frac{b}{n-b}\right) \frac{1}{\left|G_{0}\right|\left|G_{1}\right|} \sum_{A \in G_{0}} \sum_{B \in G_{1}}  I_{A_*,B_*} \\
%  & \leq \frac{b^{2}}{n^{2}}\left(1+\frac{b}{n-b}\right)   I_{A_*,B_*} \\
%  & \leq \frac{b^{2}}{n^{2}}  \frac{3}{2} I_{A_*,B_*} \\
%  & \leq \frac{b^{2}}{n^{2}}  \frac{12}{\sigma^2}  \bigg(1 + \frac{\|\m_{B_*} - \m_{A_*}\|_2^2}{\sigma^2} + \frac{\|\m'_{B_*} - \m_{A_*}\|_2^2}{\sigma^2} + \frac{\max(\|\m_{B_*} {-\m_{A_*}}\|_2,\|\m'_{B_*} {-\m_{A_*}} \|_2)^2}{2\sigma^2} \bigg) \\
% & \qquad \exp\left( \frac{\max(\|\m_{B_*} {-\m_{A_*}}\|_2,\|\m'_{B_*} {-\m_{A_*}} \|_2)\|_2^2}{\sigma^2}\right)~~\| \m_{B_*} - \m'_{B_*} \|_2^2\\
% & \leq \frac{b^{2}}{n^{2}}  \frac{12}{\sigma^2}  \bigg(1 + \frac{5}{2} \frac{\max(\|\m_{B_*} {-\m_{A_*}}\|_2^2,\|\m'_{B_*} {-\m_{A_*}} \|_2^2)}{2\sigma^2} \bigg)  \exp\left( \frac{\max(\|\m_{B_*} {-\m_{A_*}}\|_2^2,\|\m'_{B_*} {-\m_{A_*}} \|_2^2)}{\sigma^2}\right)\| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2\\
% & = \frac{b^{2}}{n^{2}}  \frac{12}{\sigma^2}  \bigg(1 + \frac{5 }{2} \frac{ \eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{2\sigma^2} \bigg)  \\
% & \qquad
% \exp\left( \frac{\eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{\sigma^2}\right)~\| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2
% \end{align*}


% \textbf{Condition: } Let $\exp\left( \frac{\eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{\sigma_t^2}\right) \leq c $ for all $t \in [T]$, which means
% \begin{align*}
% \frac{\eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{\sigma_t^2} \leq \ln c~.
% \end{align*}
% Then we have
% \begin{align*}
%  KL(w_t | w_{t-1} \| w_t' | w_{t-1}) \leq \frac{b^{2}}{n^{2}}  \frac{12 c }{\sigma^2} (1 + \frac{5\ln c}{2})  \| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2~.
% \end{align*}

% Note that for $b=1$, the \textbf{condition} translates to, for all $t \in [T]$
% \begin{align*}
% \frac{\eta_t^2\max_{z \in S_0, z_n, z'_n}(\|\nabla \ell (w_{t-1},z_n) - \nabla \ell (w_{t-1},z) \|_2^2,\|\nabla \ell (w_{t-1},z'_n) - \nabla \ell (w_{t-1},z) \|_2^2)}{\sigma_t^2} \leq \ln c~,  
% \end{align*}

% \tccomment{The quantity of interest:
% $\E_S\E_{w_{t-1}}\E_{z_n} \exp \frac{\eta_t^2\max(\|\nabla \ell (w_{t-1},z_n) - \nabla \ell (w_{t-1},z) \|_2^2,\|\nabla \ell (w_{t-1},z'_n) - \nabla \ell (w_{t-1},z) \|_2^2)}{\sigma_t^2}$, if we fix $S$ and $w_{t-1}$ then randomness come from minibatch, then $\max(\|\nabla \ell (w_{t-1},z_n) - \nabla \ell (w_{t-1},z) \|_2^2,\|\nabla \ell (w_{t-1},z'_n) - \nabla \ell (w_{t-1},z) \|_2^2)$ is a random pick from constant and its $\psi_2$ norm has dependence on $A*,B*$; if we fix $S$, randomness comes from $w_{t-1}$ and mini-batch, then $\nabla \ell (w_{t-1},z_n)$ has dependent coordinates on $w_{t-1}$ where norm cannot be easily controlled.}



% \begin{theo}
% With $T$ iterations, for a given training set $\bar S$, and for $\{\eta_t, \sigma_t\}_{t=1}^T$ satisfying 
% \begin{align*}
% \frac{\eta_t^2\max(\|\Delta_t(S_{B_*}, S_{A_*})\|_2^2,\|\Delta_t(S'_{B_*}, S_{A_*})\|_2^2)}{\sigma_t^2} \leq \ln c~,
% \end{align*}
% we have
% \begin{align*}
%  KL(w_1,..., w_T \| w'_1,..., w'_T) \leq  \frac{b^{2}}{n^{2}}  \frac{12 c }{\sigma^2} (1 + \frac{5\ln c}{2})  \sum_{t=1}^T \| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2~.
% \end{align*}
% \end{theo}

% The generalization bound follows by taking the expectation of the  KL divergence over the random draw of $\bar S$. If one uses uniform stability, then the generalization bound follows by taking the supreme of the  KL divergence over $\bar S$. 

% \subsection*{Bounding the exp term} 
% Let $\Delta_t(\bar{S}) \triangleq \max_{z,\tilde{z} \in \bar{S}} \| \nabla \ell(w_{t-1},z) - \nabla \ell(w_{t-1},\tilde{z}) \|_2$, where $\bar{S} \sim D^{n+1}$ as before. Now, note that \abcomment{note that the pairing $(z_i,\tilde{z}_i)$ below is arbitrary, the analysis does not depend on the pairing}
% \begin{align*}
% \| \m_B - \m_A \|_2^2 & = \left\| \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell(w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(w_{t-1},\tilde{z} \right] \right\|_2^2 \\
% & \leq \eta_t^2 \left\| \frac{1}{m} \sum_{i=1}^m \big( \nabla \ell(w_{t-1},z_i) - \nabla \ell(w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
% & \leq \eta_t^2 \frac{1}{m} \sum_{i=1}^m  \left\|  \big( \nabla \ell(w_{t-1},z_i) - \nabla \ell(w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
% & \leq \eta_t^2 \Delta^2_t(\bar{S})~.
% \end{align*}
% Note that $\eta_t = \eta_t(\bar{S})$ and $\sigma_t = \sigma_t(\bar{S})$, i.e., they would be data dependent.
% Then, the overall bound is \abcomment{need to add the $\sum_t$, this is just one term}
% \begin{align*}
% KL & \leq \frac{m^2}{n^2} \frac{12}{\sigma_t^2} \exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \E_{B,B'}\left[ \| \m_B - \m'_B\|_2^2 \right] ~\\
% & = \frac{m^2}{n^2} \frac{\eta_t^2}{m^2} \frac{12}{\sigma_t^2} \exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \E_{z_n,z'_n}\left[\| \nabla \ell(w_{t-1},z_n) - \ell(w_{t-1},z'_n) \|_2^2 \right] \\
% & = \frac{12}{m n^2} \frac{\eta_t^2}{\sigma_t^2} \exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \E_{z_n,z'_n}\left[\| \nabla \ell(w_{t-1},z_n) - \ell(w_{t-1},z'_n) \|_2^2 \right]~.
% \end{align*}
% For any $\sigma_t$, it suffices to choose $\eta_t$ such that $\eta_t \leq \sigma_t/(2\Delta_t(\bar{S}))$, so that $\exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \leq 3/2$. 

% Or,  for any $\eta_t$, it suffices to choose $\sigma_t$ such that $\sigma_t \geq \eta_t \Delta_t(\bar{S})/2$, so that $\exp \left( \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \right) \leq 3/2$.

% {\bf Adpative choice of $\eta_t,\sigma_t$.} Check if $\eta_t$ can deterministically depend on the history. Check if $\sigma_t$ can depend on history and depend on $\eta_t$ to satisfy the scaling condition.




% \abcomment{we can discuss the fresh sample case, and why the condition depending on $\Delta_t$ is unnecessary as long as gradients are subG. I wll add a proof.}



==> Neurips2021/app/high-prob.tex <==

% \subsection{Bounded Deviation}
% If the loss function $\ell(w,z)$ is bounded, then we can get a high probability bound by the bounded difference inequality. 

\subsection{Sub-Gaussian Deviation}

Let $S=(Z_1,\ldots,Z_n)$ and let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. Let
\begin{align}
Y & = f(Z_1,\ldots,Z_n) \\
Y'_i & = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)~,~i=1,2,\ldots,n~.
\end{align}
Let
\begin{align}
    V^+ = V^+(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_+^2 ]~,
\end{align}
and let
\begin{align}
    V^- = V^-(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~,
\end{align}

\begin{lemm}
Let $Z_1,\ldots,Z_n$ be a set of random variables. Let $Y= f(Z_1,\ldots,Z_n)$ be sub-Gaussian. Then $\E_{Z_i}[Y]$ is sub-Gaussian. 
\end{lemm}

\tcedit{Proof. By Jensen's inequality, we have for any convex function $f$,
\begin{align*}
    \E_{Z_2,\cdots, Z_n} f(\E_{Z_1}[Y])\leq \E_{Z_2,\cdots, Z_n} \E_{Z_1}f(Y) = \E f(Y),
\end{align*}
by taking $f(x) = |x|^p$, we have $\E_{Z_i}[Y]$ is sub-Gaussian with $\psi_2$ norm bounded by the $\psi_2$ norm of $Y$.}

\tccomment{Checked.}

\begin{corr}
In the setting of Lemma ?, let $Z'_i$ be an independent copy of $Z_i$, and $Y'_i = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, $\E_{Z'_i}[Y'_i]$ is sub-Gaussian.
\end{corr}

\begin{lemm}
Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, with $(x)_+ = \max(0,x)$,
\begin{equation}
V_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
\end{equation}
is sub-Exponential. 
\end{lemm}

\begin{lemm}
Let $V_1,\ldots,V_n$ be a set of (identically distributed) sub-Exponential random variables as in Lemma 2 such that $\| V_i \|_{\psi_1} \leq \kappa$ for $i=1,\ldots,n$. Then, 
\begin{align}
   \| V^+ \|_{\psi_1} = \left\| \sum_{i=1}^n V_i \right\|_{\psi_1} \leq n \kappa~. 
\end{align}
\end{lemm}
\tcedit{Proof. By triangle inequality:
\begin{align*}
    \| V^+ \|_{\psi_1} = \left\| \sum_{i=1}^n V_i^+ \right\|_{\psi_1}\leq \sum_{i=1}^n \left\| V_i^+ \right\|_{\psi_1} \leq n \kappa.
\end{align*}}\tccomment{checked}
\subsubsection{Upper Tail Bound}

The following result is a consequence of combining the Symmetric Modified Logarithmic Sobolev Inequalities (SM-LSI) and the change of measure inequality, which also forms the basis of PAC-Bayes bounds:
\begin{theo}
Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
\begin{equation}
\log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
\end{equation}
\end{theo}
Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_1}$. Then, we have
\begin{align*}
\psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right] 
\end{align*}
Then, by Markov's inequality we have
\begin{align*}
\log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
 & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
\end{align*}
Choosing $\theta = 1/(2\lambda)$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) 
& \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
\end{align*}
Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
\Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
\end{align*}
With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa$ for a constant $\kappa$, with $c_1 = c_0 \sqrt{2\kappa}$, we have
\begin{align*}
\P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \sqrt{n}/c_1 \right\} \epsilon \right) ~.
\end{align*}
\abcomment{Instead of $\epsilon$, write the bound in terms of $\log(1/\delta)$}

\subsubsection{Lower Tail Bound}
For the lower tail bound, we will use the following result which comes from combining LSI with Chebyshev's association inequality.
\begin{theo}
Assume that for some non-decreasing function $g : \R \mapsto \R$, 
\begin{align*}
    V^{-} \leq g(Y)~.
\end{align*}
Then for all $t > 0$,
\begin{align*}
    \P [ Y < \E Y -t ] \leq e^{-t^2/(4 \E [g(Y)])}~.
\end{align*}
\end{theo}

We have
\begin{align*}
     V^- & = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~ \\
     & \leq \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)^2 ] \\
     & \leq 2 \sum_{i=1}^n \E_{S'} \left[ Y^2 + (Y'_i)^2 \right] \\
     & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{S'}[ (Y'_i)^2] \\
     & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{Z'_i}[ (Y'_i)^2] \\
     & = 2 \sum_{i=1}^n Y^2 + 2 \sum_{i=1}^n \E_{Z_i}[ Y^2] \\
     & \triangleq g(Y)~.
\end{align*}
Further, note that
\begin{align*}
    \E[g(Y)] = |\E[g(Y)]| \leq \E|g(Y)| \leq \| g(Y) \|_{\psi_1} \leq c n \kappa~.
\end{align*}
As a result,
\begin{align*}
    \P [ Y < \E Y -t ] \leq e^{-t^2/(4c n \kappa)}~.
\end{align*}
With $t = n \epsilon$, we have
\begin{align*}
    \P [ Y < \E Y - n \epsilon ] \leq e^{-n\epsilon^2/(4 c \kappa)}~.
\end{align*}

==> Neurips2021/app/notes.tex <==

\abcomment{This is a place-holder section -- some/most of this will get dropped. Please do not add important proofs to this section. We should have a separate appendix section corresponding to each main section.}

\subsection{Bounding Uniform Stability.} %Bound uniform stability with Hellinger divergence, generalize to losses with first 2 moments bounded.
%
%
Take $p(\w)$ and $p^\prime(\w)$ as the probability density functions over $\w$ from running $\cA$ with $S$ and $S^\prime$. Thus, we have
\begin{align*}
\epsilon_{n} &=\sup _{x, S, S^{\prime}}\left|\int_{\mathbb{R}^{d}} \ell(\w ; z) p(\w) d \w-\int_{\mathbb{R}^{d}} \ell(\w ; z) p^\prime(\w) d \w\right| \\
&=\sup _{x, S, S^{\prime}}\left|\int_{\mathbb{R}^{d}} \ell(\w ; z)\left(\sqrt{p(\w)}+\sqrt{p(\w)^{\prime}}\right)\left(\sqrt{p(\w)}-\sqrt{p(\w)^{\prime}}\right) d \w\right| \\
& \leq \sup \left\{\left(\int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}\left(\sqrt{p(\w)}+\sqrt{p(\w)^{\prime}}\right)^{2} d \w\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p(\w)}-\sqrt{p(\w)^{\prime}}\right)^{2} d \w\right)^{\frac{1}{2}}\right\} ~.
%&<2 C \sqrt{D_{H}\left(p(\w) \| p(\w)^{\prime}\right)}~,
\end{align*}
where the inequality follows by Cauchy-Schwarz. Focusing on the first integral, we have:
\begin{align*}
 I & = \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}\left(\sqrt{p(\w)}+\sqrt{p(\w)^{\prime}}\right)^{2} d \w \\
 & \leq 2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2}p(\w) d\w + 
 2 \int_{\mathbb{R}^{d}} \ell(\w ; z)^{2} p^{\prime}(\w) d \w~.
\end{align*}
We assume that for any $z$, the loss $\ell(\w;z)$ has bounded expectation and variance, i.e., for $\w \sim p$ or $\w \sim p'$
\begin{align*}
    \E_{\w}[\ell(\w;z)] & \leq \mu \\
    \E_{\w}\left[\left(\ell(\w,z) - \E_{w}[\ell(\w;z)]  \right)^2 \right] & \leq \sigma^2~.
\end{align*}
Ideally, we want the analysis to be either over $\E_z$ or have the bounds hold with high probability over the distribution of $z$; otherwise, the assumption is uniform over $z$.

When the loss $\ell(w;z) = - \log p(z|\w)$, i.e., log-likelihood of $z$ on a model with parameter $\w$, the moment assumptions may be translated to assumptions on the tails of $p(z|\w)$, e.g., sub-Gaussian.

Based on the assumption, we have:
\begin{align*}
    I & \leq 2 \E_{\w \sim p} [ \ell^2(\w;z)] + 2 \E_{\w \sim p} [ \ell^2(\w;z)] \leq 4 (\mu^2 + \sigma^2)~.
\end{align*}
As a result,
\begin{align*}
\epsilon_{n} & \leq 2 \sqrt{\mu^2 + \sigma^2} \sqrt{D_H^2(P,P')}~,
\end{align*}
where $D_H^2$ denotes the squared Hellinger divergence. Now, recall that $D_H^2 \leq KL(P, P')$, the KL-divergence. As a result, we have
As a result,
\begin{align*}
\epsilon_{n} & \leq 2 \sqrt{\mu^2 + \sigma^2} \sqrt{KL(P,P')}
\end{align*}
Note that we can bound uniform stability with the square root of the KL-divergence, which gives a few advantages over the current literature:
\begin{itemize}
\item Avoids the "Bayes Stability" business of Li et al., which does not have a high-probability version and does not quite align with other results in stability.
\item Avoids the information theoretic approach of Pensia et al., etc., which also does not (yet) have a high probability bound.
\item Simplifies the approach of Mou et al., by working KL rather than Hellinger so more tools, such as chain rule become available. Note that the Hellinger bound is sharper, but the approach to bound the Hellinger in Mou et al., did not yield a data dependent bound (although this may be possible).
\end{itemize}

%\subsubsection{Expected Stability}


\subsection{Overall Argument [Old, Placeholder]}
\noindent {\bf Bounding squared Hellinger with TV and KL.} We have
\begin{equation}
H^2(P,P') \leq  TV(P.P') \leq \sqrt{KL(P,P')}~.
\end{equation}

\noindent {\bf Bounding KL with gradients.} For a noisy iterative algorithm, 
\begin{equation}
    w_{t+1} = w_t - \eta_t \nabla F(w_t,z_i) + \sigma_t \cN0(0,1)~,
\end{equation}
we have
\begin{equation}
    KL(P, P') \leq \frac{1}{n^2}  \E_{S \sim D^n} \left[ \sum_{t=1}^T \frac{\gamma_t^2}{\sigma_t^2} \E_{w \sim W_{t-1}}\left[ \frac{1}{n} \sum_{i=1}^n \| \nabla F(w,z)i) \|_2^2 \right] \right] ~.
\end{equation}
For basic SGD or Adam, the bound should be based on PAC-Bayes.

\noindent {\bf In expectation to High Probability.} Using the Feldman-Vondrak result.



\subsection{Bounding the KL divergence with $\chi^2$-divergence}

Recall that $f$-divergence is defined as: for any convex function $f : (0,\infty) \rightarrow \R$ and $P \ll Q$, the $f$ divergence from $P$ to $Q$ is defined by:
\[
D_f(P \| Q) = \int f\left( \frac{dP}{dQ} \right) dQ~. 
\]
For the special case of $f(t) = (t-1)^2$ or $f(t) = t^2 -1$, we get the $\chi^2$ divergence:
\begin{equation}
    \chi^2(P \| Q)  = \int \left( \frac{dP}{dQ} - 1\right)^2 dQ = \int \left( \frac{dP}{dQ} \right)^2 dQ - 1~. 
\end{equation}

Let $P,Q,R$ be any three distributions. Then, for $s \in (0,1)$
\begin{equation}
    KL\left(sP+(1-s)R ~\big\| ~sQ + (1-s)R \right) \leq s^2~\int \frac{(P(x) - Q(x))^2}{U(x)} dx~ = s^2 \E\left[ \frac{(P(x)-Q(x))^2}{U^2(x)}\right] ~.
\end{equation}
Using
\begin{equation}
    (P-Q)^2 = 2(P^2 + Q^2) - 4 \left( \frac{P}{2} + \frac{Q}{2} \right)^2~,
\end{equation}
we have
\begin{align*}
\frac{1}{s^2} KL\left(sP+(1-s)R ~\big\| ~sQ + (1-s)R \right) & \leq 2 \E_U \left[ \frac{P^2}{U^2} \right] 
+ 2 \E_U \left[ \frac{Q^2}{U^2} \right] - 4  \E_U \left[ \frac{(P/2+Q/2)^2}{U^2} \right] \\
& \leq 2 \E_U \left[ \frac{P^2}{U^2} \right] 
+ 2 \E_U \left[ \frac{Q^2}{U^2} \right] -   \E_U \left[ \frac{P^2+Q^2}{U^2} \right] \\
& = \E_U \left[ \frac{P^2}{U^2} \right] 
+ \E_U \left[ \frac{Q^2}{U^2} \right] \\
& =  \E_U \left[ \frac{P^2}{(sQ + (1-s)R)^2} \right] 
+ \E_U \left[ \frac{Q^2}{(sQ + (1-s)R)^2} \right] 
\end{align*}
We focus on each term.


\begin{comment}

We show that Assumption~\ref{asmp:subg} is related to the assumption of extended uniform stability:
\begin{asmp}
A randomized algorithm $A$ is $\gamma$-extended uniformly stable if
\begin{enumerate}[(a)]
\item $A$ is $\gamma$-uniformly stable, i.e., 
\begin{equation}
    \sup_{\substack{S,S' \in \cZ^n\\S \setminus S'=1}} \sup_{z \in \cZ} \E_A \big[ \ell(A(S),z) - \ell(A(S'),z) \big] \leq \gamma~.
    \label{eq:us}
\end{equation}
\item $A$ is $\gamma$-training set stable, i.e.,
\begin{equation}
    \sup_{S,S'_i \in \cZ^n} \E_A \big[ \ell(A(S),z_i) - \ell(A(S'_i),z'_i) \big] \leq \gamma~.
    \label{eq:tss}
\end{equation}
\end{enumerate}
\label{asmp:us}
\end{asmp}
Note that \eqref{eq:us} is standard uniform stability (US). We call \eqref{eq:tss} training set stability (TSS), as it measures the change in training set loss on $z_i$ when it is swapped with an independent copy $z'_i$ before training. TSS is arguably a more benign assumption as it involves only the training set. For example, recent work on over-parameterized models show that they interpolate the training set, which would imply TSS. For squared loss, interpolation achieves zero training set loss on each $z_i$; for logistic loss, interpolation can achieve desired low loss (say, $\gamma$) if one continues training [][][].  

\begin{lemm}
Under Assumption~\ref{asmp:us}, $\| Y - Y'_i \|_{\psi_2} \leq c \gamma \sqrt{n} $, for some absolute constant $c > 0$.
\end{lemm}
\proof \abcomment{Do not read} Note that
\begin{align*}
Y - Y'_i & = \sum_{i=1}^n \E_A \big[  \ell(A(S),z_i) - \E_z [\ell(A(S),z) ]\big] - \left( \sum_{i=1, i\neq i'}^n \E_A \big[  \ell(A(S'_i),z_i)] + \ell(A(S'_i),z'_i) - \E_z [\ell(A(S'_i),z) ]\big] \right) \\
& = \sum_{j=1,j\neq i}^n  \E_A \bigg[ \big(\ell(A(S),z_j) - \ell(A(S'_i),z_j)\big) \bigg] + \big( \ell(A(S),z_i) - \ell(A(S'_i),z'_i) \big) -  n (\E_z [\ell(A(S),z) - \ell(A(S'_i),z)]  \\
& = \sum_{i=1}^n U_i(S,S'_i)~,
\end{align*}
where 
\begin{align*}
U_i(S,S'_i) & = \E_A \bigg[ \big(\ell(A(S),z_i) - \ell(A(S'_i),z'_i)\big)  -  \E_z [\ell(A(S),z) - \ell(A(S'_i),z) ] \bigg] ~.
\end{align*}

\abcomment{Check this argument, need not be correct} Note that $U_i(S,S')$ is a symmetric random variable since (i) $\ell(A(S),z_i)$ and $\ell(A(S'_i,z'_i)$ are identically distributed, and (ii) $\E_z [\ell(A(S),z)]$ and $\E_z [\ell(A(S'_i),z)]$ are also identically distributed. So, $U_i(S,S'_i)$ is identically distributed as $U_i(S'_i,S)$. Further, for an independent Rademacher random variable $\varepsilon_i$, $U_i(S,S'_i)$ is identically distributed as $\varepsilon_i U_i(S,S'_i)$. Finally, note that swapping $Z_i$ and $Z'_i$ does not change the distribution of $U_{j}(S,S'_j)$ for $j \neq i$, and the distribution of $\sum_{j\neq i} U_{j}(S,S'_j)$. As a result, $(Y-Y'_i)$ is identically distributed as $\sum_{i=1}^n \varepsilon_i U_i(S,S'_i)$, i.e.,
\begin{align*}
  \sum_{i=1}^n U_i(S,S'_i) \sim  \sum_{i=1}^n \varepsilon_i U_i(S,S'_i)~.
\end{align*}


\abcomment{if the above is correct, we know how to do the rest [not written out fully]}
Let $\varepsilon = (\varepsilon_1,\ldots,\varepsilon_n)$ where $\varepsilon_i, i=1,\ldots,n$ are independent Rademacher random variables. Then, for any $p \geq 1$,
\begin{align*}
\| Y - Y'_i \|_p^p & =  \E_{S,S'}|Y - Y'_i|^p  
  =  \E_{S,S'}\left|\sum_{i=1}^nU(S,S'_i)\right|^p  \\
& =  \E_{S,S',\varepsilon}\left|\sum_{i=1}^n \varepsilon_i U(S,S'_i)\right|^p 
  =  \E_{S,S'}  \E_{\varepsilon} \left[\left|\sum_{i=1}^n \varepsilon_i U(S,S'_i)\right|^p \bigg| S,S' \right]  
\end{align*}
Focusing on the conditional expectation, for any fixed realization of $S,S'$, by Khintchine's inequality we have
\begin{align*}
\E_{\varepsilon} \left|\sum_{i=1}^n \varepsilon_i U(S,S'_i)\right|^p \leq c_0^p p^{p/2} \left[ \sum_{i=1}^n |U(S,S'_i)|^2 \right]^{p/2}~,
\end{align*}
where $c_0$ is an absolute constant.

\abcomment{ongoing ...} \qed 

The desired operating regime for the uniform stability assumption (Assumption~\ref{asmp:us}) is $\gamma \lesssim \frac{1}{\sqrt{n}}$ [][][], and in this operating regime, the uniorm stability assumption (Assumption~\ref{asmp:us}) implies the sub-Gaussian assumption (Assumption~\ref{asmp:subg}).


\begin{corr}
If a randomized algorithm $A$ is $\gamma$-uniformly stable with $\gamma \lesssim \frac{1}{\sqrt{n}}$, then $\| Y - Y'_i \|_{\psi_2} \leq \kappa$ for some absolute constant $\kappa > 0$.
\end{corr}
\end{comment}

==> Neurips2021/notation.tex <==
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\htn}{\hat{\theta}_{\lambda_n}}
\newcommand{\hdn}{\hat{\Delta}_n}


%% ========================================================
\newcommand\B{\mathbb{B}}
\newcommand\E{\mathbb{E}}
\renewcommand\P{\mathbb{P}}
\newcommand\I{\mathbb{I}}
\newcommand\N{\mathbb{N}}
\newcommand\s{\mathbb{S}}
\newcommand\R{\mathbb{R}}
\newcommand\W{\mathbb{W}}
\newcommand\X{\mathbb{X}}
\newcommand\Y{\mathbb{Y}}

\newcommand\1{\mathbbm{1}}
\newcommand\0{\mathbbm{0}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

%% ========================================================
%% Some useful commands. Note the dangerous \r command!
%% ========================================================



\newcommand{\bd}{\boldsymbol}
\newcommand{\mf}{\mathbf}


\newcommand{\g}{\mathbf{g}}

\renewcommand{\a}{\mathbf{a}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\f}{\mathbf{f}}
\renewcommand{\r}{\mathbf{r}} % since \r was already defined in altex
\renewcommand{\u}{\mathbf{u}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\es}{\mathbf{s}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}




%----------------------------------------
%      THE SETS
%----------------------------------------
\newcommand{\cC}{{\cal C}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cZ}{{\cal Z}}

\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cE}{{\cal E}}


%--------------------------------------------
%         THE VARIABLES & APPROXIMATES
%--------------------------------------------

% Bold variables for vectors, matrices
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\bgg}{\mathbf{g}}

\newcommand{\bz}{\mathbf{z}}
\newcommand{\hZ}{\hat{Z}}
\newcommand{\hbZ}{\hat{\bZ}}
\newcommand{\hz}{\hat{z}}

\newcommand{\hU}{\hat{U}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}


\newcommand{\hX}{\hat{X}}
\newcommand{\hY}{\hat{Y}}
\newcommand{\hatx}{{\hat{x}}}
\newcommand{\haty}{{\hat{y}}}

%---------MISC-----------------------------

\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\BNi}{\bB_N^{(i)}}
\newcommand{\xai}{\x_i^{(a)}}
\newcommand{\yai}{\bY_i^{(i)}}
\newcommand{\Xai}{\bX_i^{(a)}}
\newcommand{\Yai}{\bY_i^{(i)}}

%\newcommand{\pr}{\mathbf{P}}
%\newcommand{\E}{\mathbf{E}}

\newcommand{\m}{\boldsymbol{\mu}}
\newcommand{\llambda}{\boldsymbol{\lambda}}
\newcommand{\xx}{\boldsymbol{\chi}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\Eta}{\boldsymbol{\eta}}
\newcommand{\oomega}{\boldsymbol{\omega}}
\newcommand{\ppi}{\boldsymbol{\pi}}
\newcommand{\pphi}{\boldsymbol{\phi}}
\newcommand{\ggamma}{\boldsymbol{\gamma}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\aalpha}{\boldsymbol{\alpha}}

\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}

\newcommand{\norm}[2]{\ensuremath \|#1\|_{#2}}
\newcommand{\no}[1]{\norm{#1}{}}
\newcommand{\myref}[1]{(\ref{#1})}
\newcommand{\del}[2]{\frac{\partial #1}{\partial #2}}


%----------------------------------------------
%        NEW OPERATORS
%----------------------------------------------
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\avg}{avg}
\DeclareMathOperator{\Int}{int}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\bnd}{bd}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\ri}{ri}
\DeclareMathOperator{\co}{co}
\DeclareMathOperator{\sgn}{sign}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\discrete}{Discrete}
\DeclareMathOperator{\gam}{GAM}
\DeclareMathOperator{\uni}{Uniform}
\DeclareMathOperator{\dir}{Dir}
\DeclareMathOperator{\gaam}{GAM}
\DeclareMathOperator{\Beta}{Beta}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\gen}{gen}
\DeclareMathOperator{\lsd}{LSD}

%---------------------------------------------
% EQUATION, FIGURE, TABLE NUMBERS
%---------------------------------------------

%\renewcommand{\theequation}{\thesection.\arabic{equation}}
%\renewcommand{\thefigure}{\thesection.\arabic{figure}}
%\renewcommand{\thetable}{\thesection.\arabic{table}}
%\numberwithin{equation}{section}



%---------------------------------------------
% THEOREMS, EXAMPLES ETC.
%---------------------------------------------

\newcounter{exampleI}
\setcounter{exampleI}{1}
\renewcommand{\theexampleI}{\arabic{exampleI}}

{\theorembodyfont{\rmfamily} \theoremstyle{plain} \newtheorem{subexampleI}{Example}[exampleI]}
\renewcommand{\thesubexampleI}{\theexampleI.\Alph{subexampleI}}

\newcounter{exampleII}
\setcounter{exampleII}{2}
\renewcommand{\theexampleII}{\arabic{exampleII}}

{\theorembodyfont{\rmfamily} \theoremstyle{plain} \newtheorem{subexampleII}{Example}[exampleII]}
\renewcommand{\thesubexampleII}{\theexampleII.\Alph{subexampleII}}

\newcounter{exampleIII}
\setcounter{exampleIII}{3}
\renewcommand{\theexampleIII}{\arabic{exampleIII}}

{\theorembodyfont{\rmfamily} \theoremstyle{plain} \newtheorem{subexampleIII}{Example}[exampleIII]}
\renewcommand{\thesubexampleIII}{\theexampleIII.\Alph{subexampleIII}}


{\theorembodyfont{\rmfamily} \newtheorem{exm}{Example}}
{\theorembodyfont{\rmfamily} \newtheorem{defn}{Definition}}
%{\theorembodyfont{\rmfamily} \newtheorem{remark}{Remark}}
\newtheorem{theo}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemm}{Lemma}
\newtheorem{corr}{Corollary}
\newtheorem{clm}{Claim}
\newtheorem{asmp}{Assumption}
\newcommand{\proof}{\noindent{\itshape Proof:}\hspace*{1em}}
\newcommand{\proofsketch}{\noindent{\itshape Proof Sketch:}\hspace*{1em}}
\newcommand{\qed}{\nolinebreak[1]~~~\hspace*{\fill} \rule{5pt}{5pt}\vspace*{\parskip}\vspace*{1ex}}



\newcommand{\cx}{{\hat{x}}}
\newcommand{\cy}{{\hat{y}}}
\newcommand{\bp}{{\bar{p}}}
\newcommand{\eqn}[1]{(\ref{eq:#1})}
\newcommand {\commentout}[1] {}

%------------------------------------------

%%%%%%%%%%%Definitions and Macros

\def\ints{{{\rm Z} \kern -.35em {\rm Z} }}  % ints
\def\smallints{{{\rm Z} \kern -.3em {\rm Z} }}  % small ints
\def\pints{{{\rm I} \kern -.15em {\rm N} }}      % pints
\newcommand{\reals}{\mathbb R}
\newcommand{\integers}{\mathbb Z}

\newcommand{\lapn}{\lessapprox_{\,n}}
\newcommand{\gapn}{\gtrapprox_{\,n}}
\newcommand{\apn}{\approx_n}

%\def\reals{{{\rm I} \kern -.2em {\rm R} }} % reals
\newcommand{\RR}{\mathbb R}
\def\cplx{{{\rm I} \kern -.45em {\rm C} }}       % complex
\def\l2{\rm {\mathcal L}^{2}(\reals)}            % l2

\newcommand{\seqz}[2]{\mbox{$\{#1_{#2}\}$}_{#2 \in \smallints }}
\newcommand{\seqn}[2]{\mbox{$\{#1_{#2}\}$}_{#2 \in \pints }}
\renewcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\abs}[1]{\left|#1\right|}


\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}[section]
\newtheorem{nad}{Notation and Definitions}[section]
\newtheorem{notation}{Notation}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}{Claim}[theorem]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\newtheorem{conjecture}{Conjecture}
%\newtheorem{algorithm}{Algorithm}
\newtheorem{exercise}{Exercise}
\newtheorem{step}{Step}

\newcommand{\nr}{\nonumber}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}
\newcommand{\bnad}{\begin{nad}}
\newcommand{\enad}{\end{nad}}


\newcommand{\gb}{\beta_{\infty}}
\newcommand{\mgb}{\tilde{\beta}_{\infty}}
\newcommand{\gbb}{\beta_{2}}
\newcommand{\mgbb}{\tilde{\beta}_{2}}
\newcommand{\Jf}{J_{\infty}}
\newcommand{\mmJf}{\overline{J}_{\infty}}
\newcommand{\mJf}{\tilde{J}_{\infty}}
\newcommand{\Jff}{J_{2}}
\newcommand{\mJff}{\tilde{J}_{2}}
\newcommand{\Jc}{{\calJ_{\infty}}}
\newcommand{\mJc}{{\tilde{\calJ}_{\infty}}}
\newcommand{\Jcc}{{\calJ_{2}}}
\newcommand{\ptq}{P_{3 \overline{Q}}}
\newcommand{\pq}{P_{Q}}


\newcommand{\di}{{\,\mathrm{d}}}
\newcommand{\latop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}


%\newcommand{\Th}[1]{Theorem~\ref{#1}} % when starting a sentence
%\renewcommand{\th}[1]{Theorem~\ref{#1}}
%\newcommand{\ths}[2]{Theorems~\ref{#1} and~\ref{#2}}
%\newcommand{\thst}[2]{Theorems~\ref{#1}-\ref{#2}}
%\newcommand{\lem}[1]{Lemma~\ref{#1}}
%\newcommand{\prop}[1]{Proposition~\ref{#1}}
%\newcommand{\defin}[1]{Definition~\ref{#1}}
%\newcommand{\eq}[1]{equation~(\ref{#1})}
%\newcommand{\ineq}[1]{inequality~(\ref{#1})}
%\newcommand{\Ineq}[1]{Inequality~(\ref{#1})}
%\newcommand{\ineqs}[2]{inequalities~(\ref{#1}) and~(\ref{#2})}
%\newcommand{\Eq}[1]{Equation~(\ref{#1})}
%\newcommand{\eqs}[2]{equations~(\ref{#1}) and~(\ref{#2})}
%\newcommand{\eqss}[3]{equations~(\ref{#1}), (\ref{#2}) and~(\ref{#3})}
%\newcommand{\eqst}[2]{equations~(\ref{#1})-(\ref{#2})}
%\newcommand{\sect}[1]{Section~\ref{#1}}
%\newcommand{\subsect}[1]{Subsection~\ref{#1}}

\newcommand{\lip}{\langle}
\newcommand{\rip}{\rangle}
\newcommand{\uu}{\underline}
\newcommand{\oo}{\overline}
\newcommand{\La}{\Lambda}
\newcommand{\la}{\lambda}
%\newcommand{\eps}{\epsilon}
\newcommand{\eps}{\varepsilon}
\newcommand{\veps}{\varepsilon}
\newcommand{\rmT}{{\rm T}}
\newcommand{\rmW}{{\rm W}}
\newcommand{\Ga}{\Gamma}

\newcommand{\sign}{{\mbox{\rm sign}}}
\newcommand{\ang}{{\mbox{\rm ang}}}
%\newcommand{\supp}{{\mbox{\rm supp}}}
\newcommand{\dist}{{\mbox{\rm dist}}}

\newcommand{\nin}{\in\!\!\!\!\!/\,}

\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\tcD}{{\tilde{\cal D}}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}

\newcommand{\RE}{{\cal R}e}
%\newcommand{\IM}{{\cal I}m}


\newcommand{\Prob}{{\rm Prob\,}}
\newcommand{\diam}{{\rm diam\,}}
\renewcommand{\mod}{{\rm mod\,}}
\newcommand{\sinc}{{\rm sinc\,}}
\newcommand{\ctg}{{\rm ctg\,}}
\newcommand{\ifff}{\mbox{\ if and only if\ }}
%\newcommand{\proof}{\noindent {\bf Proof:\ }}

%\renewcommand{\bar}{\overline}
\renewcommand{\overline}{\bar}
%\renewcommand{\tilde}{\widetilde}
\renewcommand{\widetilde}{\tilde}
%\renewcommand{\ell}{l}
%\renewcommand{\hat}{\widehat}
\renewcommand{\widehat}{\hat}


\newcommand{\boldx}{{\bf x}}
\newcommand{\boldX}{{\bf X}}
\newcommand{\boldy}{{\bf y}}
\newcommand{\indic}{{\large \bf 1}}
\newcommand{\uux}{\uu{x}}
\newcommand{\uuY}{\uu{Y}}

\newcommand{\opt}{\rm{opt}}


%fraction with round brackets
\newcommand{\ffrac}[2]
  {\left( \frac{#1}{#2} \right)}

\newcommand{\one}{\frac{1}{n}\:}
\newcommand{\half}{\frac{1}{2}\:}


\newcommand{\BAMS}{{\em Bulletin of the Amer. Math. Soc.}}
\newcommand{\TAMS}{{\em Transactions of the Amer. Math. Soc.}}
\newcommand{\PAMS}{{\em Proceedings of the Amer. Math. Soc.}}
\newcommand{\JAMS}{{\em Journal of the Amer. Math. Soc.}}
\newcommand{\LNM}{{\em Lect. Notes in Math.}}
\newcommand{\LNCS}{{\em Lect. Notes in Comp. Sci.}}
\newcommand{\IV}{{\em Invent. Math.}}
\newcommand{\JAM}{{\em J. Anal. Math.}}
\newcommand{\Sc}{{\em Science}}


==> Neurips2021/sec/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  %For example:
% % \begin{itemize}
% %   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
% %   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% %   \item Did you include the license to the code and datasets? \answerNA{}
% % \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerTODO{}
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerTODO{}
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    % \answerTODO{}
    \answerYes{}
    %See %Appendix~\ref{sec:app_tsgd},~\ref{sec:app_opt}, and \ref{sec:app_gen}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See our supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes
    %{See Section~\ref{sec:experiments} and Appendix~\ref{sec:app_exp}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> Neurips2021/sec/conc.tex <==

Inspired by recent advances in stability based and information theoretic approaches to generalization bounds [Mou et al][Pensea et al.][Negrea et al][Li et al][Hegifam et al], we have presented a framework for developing such bounds based on expected stability for noisy stochastic iterative (NSI) learning algorithms. Further, we have simplified the task to one of bounding expected for the NSI algorithm. We have developed a specific bound for SGD with Gaussian noise which inherits strengths of a variety of existing results and quantitatively outperforms them based on preliminary experiments. We have also developed similar bounds for SGD with exponential family noise, which seem to be the first result of this type. Our work also highlights few key directions for future work, including sharper notions of gradient discrepancy/incoherence and better understanding of the trade-offs between stability and optimization for NSI algorithms.

==> Neurips2021/sec/exp.tex <==
\begin{figure*}[t] 
\centering
  \subfigure[CNN, $\sigma_t = 10^{-3}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/grad_mnist_cnn_lr2.png}
 } 
  \subfigure[CNN, $\sigma_t = 10^{-3}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha3mo0_mnist_cnn.png}
 }  
  \subfigure[CNN, $\sigma_t = 10^{-4}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_mnist_cnn.png}
 }  
  \subfigure[MLP, $\sigma_t = 10^{-4}$ ]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_mnist_fnn.png}
 }
  \subfigure[CNN, $\sigma_t = 10^{-3}$]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/grad_fashion_cnn_lr2.png}
 }
  \subfigure[CNN, $\sigma_t = 10^{-3}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha3mo0_fashion_cnn.png}
 }  
   \subfigure[CNN, $\sigma_t = 10^{-4}$]{
 \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_fashion_cnn.png}
 }  
  \subfigure[MLP, $\sigma_t = 10^{-4}$]{
  % [trim=left bottom right top, clip]
 \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_fashion_fnn.png}
 }
\caption[]{Numerical results for MNIST (a-d) and Fashion MNIST (e-h) with CNN and MLP. All x-axes show the number of Epochs of training. Figure (a) (MNIST)  and (e) (Fashion MNIST) show the key factors in the bounds, i.e., gradient norms in \cite{Li2020On}, gradient incoherence in \cite{negrea2019information}, gradient discrepancy in our bound. Figure (b-d) and (f-h) compare our bound with the existing bounds for small noise variance, i.e., $\sigma_t^2 = 10^{-4}$ and large  variance i.e., $\sigma_t^2 = 10^{-3}$ for CNN, and MLP, demonstrating that our bounds are numerically sharper than the existing bounds. Figure (b-c) and (f-g) suggest that increasing noise variance leading to smaller generalization bounds which is consistent with the theoretical analysis.
}
\label{fig:mnist}
\end{figure*}





In this section, we conduct a series of experiments to evaluate the generalization error bounds. We aim to compare the proposed  bound in Theorem \ref{theo:guss_gen} with the existing bounds in \cite{Li2020On} and  \cite{negrea2019information} for various datasets, model structures and noise scales. Note that we do not consider the bound in \cite{haghifam2020sharpened} as a baseline because the bound in \cite{haghifam2020sharpened} only applies to full-batch setting, but we focus on noisy mini-batch gradient descent.
%however the bound in \cite{haghifam2020sharpened} only applies to full-batch setting which is not in the scope of our empirical evaluation. 

\textbf{Experimental setup.} We consider MNIST \cite{mnist} and Fashion-MNIST \cite{fashion-mnist} with a 2- layer convolutional neural networks (CNN) and 3-layer multilayer perceptron (MLP). We use Noisy SGD with Gaussian noise to train the model, i.e., $\mathbf{w}_{t}=\mathbf{w}_{t-1}-\eta_{t} \nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)+\boldsymbol{\xi}_{t}, \text { where } \boldsymbol{\xi}_{t} \sim \mathcal{N}\left(0, \sigma_{t}^{2} \mathbb{I}_{d}\right)$.
We use constant learning rate $\eta_t = 0.001$ and batch size $|B_t| = 128$ for all datasets, and minimize cross-entropy loss for a fixed number of epochs. We consider small and large noise variance for $\sigma_t$, i.e., $\sigma_t \in \{10^{-4},, 10^{-3}\}$. We repeat each experiment for 20 runs. 

\textbf{Experimental results.} We derive theoretical generalization error bounds that depend on the data-dependent quantity \emph{gradient discrepancy}, i.e., $\|\ell(\w,z) - \ell(\w,z^\prime)\|$. We acknowledge that existing bounds in \cite{Li2020On} and \cite{negrea2019information} also
have improved the Lipschitz constants in \cite{mou2018generalization} to a data-dependent quantity. Since the first key difference between our bound and others is that we replace the \emph{gradient norms}, i.e., $\frac{1}{n}\sum_{z \in S}\|\ell(\w,z)\|$ in \cite{Li2020On} and \emph{gradient incoherence} in  \cite{negrea2019information} with
gradient discrepancy. We report those data-dependent quantities in Figure \ref{fig:mnist} (a) and 
(b) for MNIST and Fashion MNIST respectively. The results suggest that the gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors, and the gradient incoherence in \cite{negrea2019information} is much smaller than the gradient discrepancy in our bound as well. 
However, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$ which has a worse sample dependence compared to our bound. The results in (b-d) for MNIST and (f-h) for Fashion MNIST show that our bounds are much sharper than those of \cite{negrea2019information} due to improving the dependence on $n$ from a order of $\frac{1}{\sqrt{n}}$ to $\frac{1}{n}$. Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to those for CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases, leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence.

% The second key difference is the order of dependence on the sample size $n$, i.e., both of our bound and $\cite{Li2020On}$ has a bound of order $\frac{1}{n}$, however, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$. 
%Figure \ref{fig:mnist} (a) and 
% (b) suggests that the gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors, and the gradient incoherence in \cite{negrea2019information} is much smaller than the gradient discrepancy in our bound as well.
% However, the results in (b-d) for MNIST and (f-h) for Fashion MNIST show that our bounds are much sharper than those of \cite{negrea2019information} due to improving the dependence on $n$ from a order of $\frac{1}{\sqrt{n}}$ to $\frac{1}{n}$. Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence.


More details of our model architectures and addtional experimental results can be found in Appendix. 
We acknowledge that we did not aim to achieve the state-of-the art predictive performance. With further tuning, the prediction results could be improved.

% \begin{figure*}[t] 
% \centering
%  \subfigure[CNN for F-MNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/grad_fashion_cnn_lr2.png}
%  }
%   \subfigure[CNN for F-MNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha3mo0_fashion_cnn.png}
%  }  
%   \subfigure[CNN for F-MNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_fashion_cnn.png}
%  }  
%   \subfigure[MLP for F-MNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr3alpha4mo0_fashion_fnn.png}
%  }
% \caption[]{$\eta = 0.001$, $\sigma = 0.001$, repeat = 20
% }
% \label{fig:fashion}
% \end{figure*}


% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN for MNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/lr3alpha3mo0_mnist_cnn.png}
%  }  \vspace{-2mm}
%   \subfigure[MLP for MNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/lr3alpha3mo0_mnist_fnn.png}
%  }\vspace{-2mm}
% \caption[]{$\eta = 0.001$, $\sigma = 0.001$, repeat = 20
% }\vspace*{-2mm}
% \label{fig:mnist_large_sigma}
% \end{figure*}



% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN for FashionMNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/lr3alpha4mo0_fashion_cnn.png}
%  }  \vspace{-2mm}
%   \subfigure[MLP for FashionMNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/lr3alpha4mo0_fashion_fnn.png}
%  }\vspace{-2mm}
% \caption[]{$\eta = 0.001$, $\sigma = 0.0001$, repeat = 20
% }\vspace*{-2mm}
% \label{fig:mnist_small_sigma}
% \end{figure*}



% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN for MNIST]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/grad_mnist_cnn_lr2.png}
%  }  \vspace{-2mm}
%   \subfigure[CNN for FashionMNIST]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.40\textwidth]{img/grad_fashion_cnn_lr2.png}
%  }\vspace{-2mm}
% \caption[]{$\eta = 0.001$, $\sigma = 0.001$, repeat = 20
% }\vspace*{-2mm}
% \label{fig:mnist_large_sigma}
% \end{figure*}



==> Neurips2021/sec/gen_stability.tex <==

In the setting of statistical learning, there is an instance space $\cZ$, a hypothesis space $\cW$, and a loss function $\ell : \cW \times \cZ \mapsto \R_+$. Let $D$ be an unknown distribution of $\cZ$ and let $S \sim D^n$ be $n$ i.i.d.~draws from $D$. For any specific hypothesis $\w \in \cW$, the population and empirical loss are respectively given by
\vspace*{-3mm}
\begin{equation}
L_D(\w) \triangleq \E_{z \sim D}[\ell(\w,z)]~, \qquad \text{and} \qquad  L_S(\w) \triangleq \frac{1}{n} \sum_{i=1}^n \ell(\w,z_i)~.   
\vspace*{-3mm}
\end{equation}
\\For any distribution $P$ over the hypothesis space, we respectively denote the expected population and empirical loss as
\vspace*{-3mm}
\begin{equation}
L_D(P) \triangleq \E_{z \sim D}\E_{\w \sim P}[\ell(\w,z)]~, \qquad \text{and} \qquad  L_S(P) \triangleq \frac{1}{n} \sum_{i=1}^n \E_{\w \sim P}\ell(\w,z_i)~.
\vspace*{-3mm}
\end{equation}
\\Consider a randomized algorithm $A$ which works with $S =\{z_1,\ldots,z_n\} \sim D^n$ and creates a distribution over the hypothesis space $\cW$. For convenience, we will denote the distribution as $A(S)$. The focus of the analysis is to bound the generalization error of $A$ defined as:
\begin{align}
\gen(A(S)) \triangleq L_D(A(S)) - L_S(A(S))~.    
\end{align} 
We will assume $A$ is permutation invariant, i.e., the ordering of samples in $S$ do not modify $A(S)$, an assumption satisfied by most learning algorithms. We will primarily focus on developing bounds for the expectation $\E_S[L_D(A(S)) - L_S(A(S))]$, and subsequently discuss high-probability bounds.
%\abcomment{mention that $A$ is assumed to be permutation invariant}




\subsection{Bounds based on Expected Stability}
% For our analysis, we assume that the $L_2$ norm of the loss is bounded:
% \begin{asmp}
% Let $c_{\ell_2}(z) = \E_{w \sim  p_{A(S)}}[\ell^2(w,z)]$. Two options:
% \begin{enumerate}
% \item Uniform bound: $\forall z$, $c_{\ell_2}(z) \leq c_0$.
% \item Expectation bound: $\E_{z \sim D}[c_{\ell_2}(z)] \leq c_0$ \abedit{and $\E_{z \sim S}[c_{\ell_2}(z)] \leq c_0$}.
% \end{enumerate}
% The analysis would look different depending on which one we choose. \abcomment{Discuss}
% \end{asmp}
% \abcomment{need a discussion on assumptions for info-theoretic analysis}

We start our analysis by noting that the expected generalization error can be upper bounded by stability based on the Hellinger divergence~\cite{save16,Li2020On}: $H^2(P\| P') = \frac{1}{2}\int_{\w} (\sqrt{p(\w)} - \sqrt{p'(\w)})^2 d\w$.
\begin{restatable}{prop}{prophell}
Let $S \sim D^n$ and let $S'_{n}$ be a dataset obtained by replacing $z_n \in S$ with $z'_n \sim D$. Let $A(S),A(S'_{n})$ respectively denote the distributions over the hypothesis space $\cW$ obtained by running randomized algorithm $A$ on $S,S'_{n}$.
Assume that for any $S \sim D^n, z \in \cZ$, $\E_{\w \sim  A(S)}[\ell^2(\w,z)] \leq c_0/2, c_0>0$. Then, with $H(\cdot,\cdot)$ denoting the Hellinger divergence, we have
\begin{equation}
| \E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))] | \leq c_0 \E_{S \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S), A(S'_{n})\big)}~. 
\end{equation}
\vspace*{-6mm}
\label{prop:hell}
\end{restatable}
Note that the result does not need the loss function to be bounded, but just the second moment of $\ell(\w,z), \w \sim A(S)$ to be bounded for any $z \in \cZ$. The assumption is satisfied by bounded losses. It is also instructive to compare the assumption to that in recent information theoretic bounds~\cite{haghifam2020sharpened,xu2017information}, where one assumes $\ell(\w,z), z \sim D$ to be sub-Gaussian for any $\w \in \cW$.

Next, we note that the Hellinger divergence can be bounded by the KL-divergence, so we focus on bounding the KL divergence in the sequel. 
\begin{restatable}{prop}{prophellkl}
For any two distributions $P$ and $P'$, we have
\begin{equation}
    2 H^2(P,P') \leq \min \bigg\{ KL(P,P'),\sqrt{\frac{1}{2}KL(P,P')} \bigg\}~.
\end{equation}
\vspace*{-6mm}
\label{prop:hellkl}
\end{restatable}





\subsection{Noisy Stochastic Iterative Algorithms: The Mixture Model Perspective}

We consider a general family of noisy stochastic iterative (NSI) algorithms. Given $S \sim D^n$, such iterative algorithms have two additional sources of randomness in each iteration $t$: (a) a stochastic mini-batch of samples $S_{B_t}$, with $|S_{B_t}| = b$, drawn uniformly at random with replacement from $S$; and (b) noise $\bxi_t$ suitably included in the iterative update. Given a trajectory of past iterates $\w_{0:(t-1)}$, the new iterate $\w_t$ is drawn from a distribution $P_{B_t,\bxi_t,\w_{0:(t-1)}}$ over $\cW$:
\begin{align}
\w_{t} \sim P_{B_t,\bxi_t|\w_{0:(t-1)}} = f_t(B_t,\bxi_t,\w_{0:(t-1)})~,
\label{eq:nmia}
\end{align}
for some suitable function $f_t$. We will often drop the conditioning $\w_{0:(t-1)}$ to avoid clutter and represent the distribution as $P_{B_t,\bxi_t}$ in the sequel.
Since our analysis is based on KL-divergence, we assume that the distributions $P_{B_t,\bxi_t}$ are absolutely continuous with respect to each other. 

From Propositions~\ref{prop:hell} and \ref{prop:hellkl}, to get a bound on the expected generalization of such NSI algorithms, it suffices to focus on the KL-divergence between $A(S)$ and $A(S'_{n})$. Let $P_T, P'_T$ denote the distributions over hypotheses $\w \in \cW$ after $T$ steps of the algorithm based on $S,S'_{n}$ respectively. 
% \abdelete{i.e., $P_T = A(S)$ and $P'_T = A(S'_{(n)})$.} 
Further, let $P_{0:(t-1)}$ denote the joint distribution over $\w_{0:(t-1)} = (\w_0,\ldots,\w_{t-1})$, and let $P_{t|} \equiv P_{B_t,\bxi_t}$ denote the conditional distribution conditioned as $\w_{0:t-1}$. We will use the following chain rule for KL-divergence which has been effectively used in recent advances in information theoretic bounds for generalization~\cite{negrea2019information,haghifam2020sharpened,pensia2018generalization}:
\vspace*{-2mm}
\begin{equation}
KL(P_T \| P'_T) \leq KL(P_{0:T} \| P'_{0:T} ) = \sum_{t=1}^T P_{0:(t-1)}\left[ KL(P_{t|} \| P'_{t|}) \right]~.
\label{eq:klchain}
\end{equation}
Note that the analysis which follows also apply to such information theoretic bounds~\cite{negrea2019information,haghifam2020sharpened,pensia2018generalization}.

We present a mixture model perspective for $P_{t|},P'_{t|}$ following [Li et al.]. Consider sampling $\bar{S} \sim D^{n+1}$. Let $S,S'_{n}$ be size $n$ subsets of $\bar{S}$ such that $S=\{Z_1,\ldots,Z_{n-1},Z_n\}$ and $S'_{n} = \{Z_1,\ldots,Z_{n-1},Z'_n\}$, where $Z'_n = Z_{n+1}$. Let $S_0 = \{Z_1,\ldots,Z_{n-1}\}$. The algorithms we consider use a mini-batch of size $b$ in each iteration. Let the set of all mini-batches be denoted by $G$. Let the set of all mini-batches drawn from $S_0$ be denoted by $G_0$. Note that $|G_0| = \binom{n-1}{b}$. Let the set of all mini-batches which includes the last sample, viz.~$z_n$ for $S$ and $z'_n$ for $S'_n$, be denoted by $G_1$. Note that $|G_1| = \binom{n-1}{b-1}$. Also note that 
%\begin{align*}
$|G_0| + |G_1| = \binom{n-1}{b} + \binom{n-1}{b-1} = \binom{n}{b} = |G|$.
%\end{align*}
%the total number of $b$-sized mini-batch samples from a dataset of size $n$. \abcomment{The subsets of $S$ and $S'_{(n)}$ corresponding to mini-batch $B$ will be denoted as $S_B$ and $S'_B$.}

We focus on bounding $KL(P_{t|} \| P'_{t|})$. 
For for a given $\w_{0:(t-1)}$ and a fixed mini-batch $B_t$, following \eqref{eq:nmia}, let $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively be distributions over $\cW$ corresponding to $S, S'_{n}$. Then, $P_{t|}$ and $P'_{t|}$ can be viewed as mixture models with shared components~\cite{Li2020On}:
%due to the randomness in $\bxi_t$. 
\begin{restatable}{prop}{mixmodel}
Consider the mixture models 
%\begin{align*}
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  
%\end{align*}
Then, with 
%\begin{equation*}
$s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}$,
%\end{equation*}
we have 
\begin{align*}
    P_{t|} = s Q_{t|} + (1-s) R_{t|}~, \qquad \text{and} \qquad P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~.
\end{align*}
\label{prop:mixmodel}
\vspace*{-6mm}
\end{restatable}
%Thus, $P_{t|}$ and $P'_{t|}$ are each mixture models with (a set of) shared components $R_{t|}$

% Consider two collection of points $\{\mu_B : B \in G \}$ and $\{\mu_B : B \in G\}$. In our context, at any stage $t$, for mini-batch $B$ and step specific randomness $\bxi_t$, \yzcomment{$S_B$ is random due to the random draw of mini-batch. What is randomness $\bxi_t$? example of $\bxi_t$? } we have 
% \begin{align*}
%     \w_t \sim P_{\mu_B,t} where \qquad  \mu_B = \E[f_t(w_{1:t-1},S_B, \bxi_t)]
% \end{align*}
% \abcomment{highlight the fact that $f_t$ can be general, may depend on the entire trajectory, etc.} \abcomment{DISCUSS -- examples}
% Let $p_{\mu,\sigma}$ denote the Gaussian distribution $\cN(\mu, \sigma^2 \I)$. Let $P = \frac{1}{|G|} \sum_{B \in G} p_{\mu_B,\sigma}$ and  $P' = \frac{1}{|G|} \sum_{B \in G} p_{\mu'_B,\sigma}$. Our goal is to bound $KL(P \| P')$ {\em without making any additional assumptions}. Note that $\eta_t,\sigma_t$ can depend on $w_{1:t-1}$, but since the analysis is conditioned on $w_{1:t-1}$, these are effectively constants for the current analysis. 

% \abcomment{This analysis immediately shows why KL-divergence cannot be used for the non-noisy case -- these will be Dirac measures, and KL-div will be $\infty$. A bound based on TV or Hellinger would still be valid.}

% Let 
% \begin{align*}
% Q_1 = \frac{1}{|G_1|} \sum_{B \in G_1} p_{\mu_B,\sigma} \qquad Q_2 = \frac{1}{|G_1|} \sum_{B \in G_1} p_{\mu'_B,\sigma} \qquad R = \frac{1}{|G_0|} \sum_{B \in G_0} p_{\mu_B,\sigma}~.  
% \end{align*}
% Then, with 
% \begin{equation*}
% s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}~,
% \end{equation*}
% we have 
% \begin{align*}
%     P = s Q_1 + (1-s) R \qquad P' = s Q_2 + (1-s) R~.
% \end{align*}


\subsection{Bounds with Le Cam Style Divergence (LSD)}
The mixture model structure in $P_{t|}, P'_{t|}$ can be utilized to bound their KL-divergence in terms of Le Cam Style Divegence (LSD). While the classical Le Cam divergence~\cite{save16} is $LCD(P\|P') = \frac{1}{2} \int \frac{(dP - dP')^2}{dP + dP'}$ (where $dP$ denotes the density), given the mixture model structure in $P_{t|}, P'_{t|}$ in Proposition~\ref{prop:mixmodel}, we get our bounds in terms of  $\int \frac{(dP_{B,\bxi} - dP'_{B,\bxi})^2}{dP_{A}(\bxi)}, B \in G_1, A \in G_0$, %\yzcomment{$P_B(\bxi)$ should be  $dP_{B_t,\bxi_t}$? }\abcomment{fixed}
which we call LSD. 
[Li et al.] pursued a similar route for SGLD, but our proofs are significantly more simple and illustrates applicability of LSD to general NSI algorithms, not just SGLD. 
Putting Propositions~\ref{prop:hell} and \ref{prop:hellkl}, and \eqref{eq:klchain} together, with some additional analysis we have the following LSD based generalization bound: 
\begin{restatable}{theo}{theostab}
Consider a noisy stochastic iterative algorithms of the form~\eqref{eq:nmia} with mini-batch size $b \leq n/2$. Then, with $c = \sqrt{2} c_0$, we have
\vspace*{-2mm}
\begin{equation}
\hspace*{-5mm}
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq c\frac{b}{n} \E_{S} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \E_{\w_{0:(t-1)}}\E_{B_t \in G_1} \E_{A_t \in G_0} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t}(\bxi_t)} d\bxi_t \right] }~.
\end{equation}
\label{theo:stab}
\vspace*{-6mm}
\end{restatable}
%A few properties of the bound can be immediately notes: 
\\Note that the bound holds for any NSI algorithm of the form~\eqref{eq:nmia}, does not assume the loss to be bounded, depends on expectations over samples, trajectories, and mini-batches, and does not depend on any uniform assumptions. Further, as an expected stability based bound to generalization error, the bound depends on the distribution discrepancy as captured by the expected LSD. 

%Qualitatively, even if we assume that each term in $\sum_t$ is bounded by a constant

%In Sections~\ref{sec:stab_gauss}

%\abcomment{We are still missing an overall bound by combining (4)-(7)}

%The analysis upto this point does not need the distributions to be Gaussian.




\subsection{High Probability Bounds}
\label{sec:highp}
\input{sec/high_prob}

==> Neurips2021/sec/high_prob.tex <==

Let $S \sim D^n$ with $S=(Z_1\ldots,Z_n)$ corresponding to the training data. Consider the random variable $Y(S)$, the Scaled (by $n$) Generalization Error (SGE), defined as
\begin{align}
Y(S) \triangleq \sum_{i=1}^n \E_A \big[  \E_{Z \sim D} [\ell(A(S),Z) ] - \ell(A(S),Z_i) \big] = n\big(L_D(A(S)) - L_S(A(S))\big) ~.
\end{align}
%where $A(S)$ is the distribution over $\cW$ due to randomized algorithm $A$ run on $S$.
Theorem~\ref{theo:stab} establishes a bound on $|\frac{1}{n}\E_S[Y(S)]|$. We now focus on establishing a high probability bound on $\frac{1}{n}(Y(S)-\E_S[Y(S)])$. Let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. Further, let $S'_i = (Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, the change in SGE
\begin{equation}
Y(S) - Y(S'_i) = n \big[ \big( L_D(A(S)) - L_D(A(S'_i)) \big) - \big( L_S(A(S)) - L_{S'_i}(A(S'_i) \big) \big]    
\end{equation}
is a symmetric random variable, and is identically distributed for $i=1,\ldots,n$.
% \begin{align}
% Y(S) - Y(S'_i) = \sum_{j=1}^n \E_A \big[ \ell(A(S'_i),Z_j) - \ell(A(S),Z_j) \big] = n \big(L_{S'_i}(A(S'_i) - L_S(A(S)) \big)
% \end{align}
%Note that $(Y-Y'_i)$ \abedit{is symmetric} and are identically distributed for any $i$. 
Our analysis is based on the following assumption: %\abcomment{cite for $\psi_2$ norm} 
\begin{asmp}
The random variable $(Y(S)-Y(S'_i))^2$ is sub-Gaussian with $\psi_2$-norm $\kappa_A^2$, i.e., $\| (Y-Y'_i)^2 \|_{\psi_2} = \sup_{q \geq 1} (\E_{S.S'}|Y(S)-Y(S'_i)|^{2q})^{1/q}/\sqrt{q} = \kappa_A^2$. 
%has bounded second moment, i.e., $\E_{S,Z'_i}[(Y(S)-Y(S'_i))^2] \leq \nu_A$, for some constant $\nu_A$.\abcomment{should this be a definition? i.e., just call the second moment $\nu_A$?}
\label{asmp:2moment}
\end{asmp}
Assumption~\ref{asmp:2moment} implies that $\|Y-Y'_i\|_{\psi_2} \leq \kappa_A$.
Note that since $Y(S) - Y(S'_i)$ is identically distributed for all $i$, $\kappa_A$ is the same for all $i$. Further, $\kappa_A$ is a property of the algorithm $A$, and can be viewed as a measure of stability.
If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered stable; on the other hand, if $\kappa_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as typical generalization error $\frac{1}{n}Y(S)$ itself. The sharpness of the high-probability bound we present meaningfully depends on $\kappa_A$, with smaller values implying sharper bounds.



\begin{restatable}{theo}{theohighp}
Under Assumption~\ref{asmp:2moment}, with probability at least $(1-\delta)$ over the draw $S \sim D^n$, we have
\begin{equation}
L_D(A(S)) \leq L_S(A(S)) + \E_S\bigg[L_D(A(S) - L_S(A(S))\bigg] + \max\left( \frac{1}{n}, \frac{ c_1 \kappa_A}{\sqrt{n}} \right) \log \left(\frac{16}{\delta} \right)~.      
\end{equation}
\label{theo:hp}
\vspace*{-5mm}
\end{restatable}


==> Neurips2021/sec/intro.tex <==


Recent years have seen renewed interest and advances in characterizing generalization performance of learning algorithms in terms of stability, which considers change in performance of a learning algorithm based on change of a single training point \cite{hardt2016train,bousquet2002stability,Li2020On,mou2018generalization}. For stochastic gradient descent (SGD), \cite{hardt2016train} established generalization bounds based on uniform stability \cite{hardt2016train,bousquet2002stability}, although the analysis needed rather small step sizes $\eta_t = 1/t$ which is not useful in practice. While improving the analysis for SGD has remained a challenge, advances have been made on noisy SGD algorithms such as stochastic gradient Langevin dynamics (SGLD) \cite{mou2018generalization,Li2020On}. In parallel, there has been key developments on related information-theoretic generalization bounds applicable to SGLD type algorithms \cite{negrea2019information,haghifam2020sharpened,xu2017information,russo2016controlling, pensia2018generalization}.

While these developments have led to major advances in analyzing generalization of noisy SGD algorithms, they each have certain limitations which leave room for further improvements. Using uniform stability, \cite{mou2018generalization} established a bound for SGLD of the form $\frac{L}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ which depends on $L$, the Lipschitz constant for the gradient, and the step size $\eta_t \leq \frac{\sigma_t \ln 2}{L}$. The bound has a desirable dependency of $O(\frac{1}{n})$ on the samples, but has an undesirable dependence on $L$, and the step sizes, bounded by $\frac{\sigma_t}{L}$, are too small. \cite{mou2018generalization} also presented another bound which addresses some of these issues, but gets an undesirable $O(\frac{1}{\sqrt{n}})$ sample dependence. \cite{Li2020On} made advances on such results based on Bayes-stability, and got a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \g_e(t)/\sigma_t^2}$, where $\g_e(t)$ is the expected gradient norm square at step $t$. While the bound avoids dependency on $L$ with expected gradient norm, as shown in the information theoretic bounds of \citep{negrea2019information,haghifam2020sharpened}, the dependency can be potentially be improved to some measure of gradient incoherence. Further, the analysis of \cite{Li2020On} still needs small step sizes, bounded by $\frac{\sigma_t}{L}$. By building on the developments of \citep{russo2016controlling,xu2017information,pensia2018generalization}, \cite{negrea2019information} made advances from the information theoretic perspective and established bounds for SGLD which have the desirable dependence on gradient discrepancy, but has an undesirable $O(\frac{1}{\sqrt{n}})$ sample dependence. \cite{haghifam2020sharpened} also approached the problem from an information theoretic perspective and obtained bounds based on gradient incoherence with $O(\frac{1}{n})$ sample dependence, but their analysis holds for full batch Langevin dynamics, not mini-batch SGLD.

In this paper, we build on the strengths of these stability based and information theoretic approaches to develop a general framework (Section~\ref{sec:gen}) for analyzing stability of noisy stochastic iterative (NSI) algorithms, which include SGLD as an important special case. Our framework considers generalization based on the concept of {\em expected stability}, rather than uniform stability \cite{mou2018generalization,hardt2016train,bousquet2002stability, bousquet2020sharper}, and arguably puts less demands on the assumptions needed to analyze NSI algorithms. We show that expected stability can be bounded by KL-divergence between posterior distribution over hypothesis from training sets differing in one point, connecting our analysis to the information theoretic approach initiated by \cite{pensia2018generalization} and followed by \citep{negrea2019information,haghifam2020sharpened}. Building on the developments of \cite{Li2020On}, we show that posterior distribution for general NSI algorithms can be viewed as mixture models, and the KL divergence over posteriors can be bounded by the expectation of Le Cam Style Diveregnces (LSD). For any specific NSI algorithm, the task then reduces to suitable bounding the expected LSD. While our analysis mainly focuses on expected generalization \cite{Li2020On,mou2018generalization,negrea2019information,haghifam2020sharpened}, we show that one get high probability generalization bounds under suitable assumptions. 

In Section~\ref{sec:stab_gauss}, we apply the expected stability approach to SGLD by suitably bounding the expected LSD  for Gaussian noise. The resulting bound inherits the strengths of the existing bounds with dependence on norms of gradient discrepancy, no dependence on $L$, flexible data dependent choices for $\eta_t,\sigma_t$, and a $O(\frac{1}{n})$ sample dependence. The concept of gradient incoherence in \citep{negrea2019information,haghifam2020sharpened} and our gradient discrepancy are mildly different, but they all qualitatively capture a much more desirable and quantitatively smaller quantity compared to the gradient norm in \cite{Li2020On}. Conceptually, gradient discrepancy norm captures the notion of stability, which the gradient norm does not. The crux of the technical argument in our analysis relies on an approach to bounding the LSD based on an application of mean-value theorem and a careful approach to handle density ratios. We briefly discuss the relationship of our bound for mini-batch SGLD with \citep{mou2018generalization,Li2020On,negrea2019information}, and demonstrate how our bound picks up most of the strengths of each while avoiding the weakness. 
%Further, we show that the gradient incoherence of \cite{negrea2019information} are quantitatively smaller than our gradient discrepancy, but our bounds are tighter because of the $O(\frac{1}{n})$ sample dependence compared to the $O(\frac{1}{\sqrt{n}})$ sample dependence of \cite{negrea2019information}. 

In Section~\ref{sec:stab_exp_family}, we establish expected stability based generalization bounds for mini-batch stochastic gradient descent with exponential family noise. The result is an important technical extension to existing work on SGLD and, to the best of our knowledge, the first result of its type. The extension also illustrates the power of our framework as we only needed to bound the expected LSD for exponential family noise. The technical argument for bounding the expected LSD for general exponential families are a bit more involved compared to the Gaussian case. As in the case of SGLD with Gaussian noise, the bounds with exponential family noise also depends on the gradient discrepancy, have data dependent flexibly on the choices  of $\eta_t,\sigma_t$, and a $O(\frac{1}{n})$ sample dependence.  

In Section~\ref{sec:experiment}, we empirically verify the sharpness of our bounds for SGLD in comparison to \citep{Li2020On,negrea2019information} on standard benchmarks (MNIST, Fashion-MNIST) using both multi-layer perceptrons (MLPs) and convolution neural networks (CNNs). For both datasets, both models, and for the entire range of training epochs in each setting, our bounds are shown to be substantially smaller than that of \cite{Li2020On}\cite{negrea2019information}. Interestingly, gradient incoherence of \cite{negrea2019information} is quantitatively smaller than our gradient discrepancy, but our bounds are tighter because of the $O(\frac{1}{n})$ sample dependence compared to $O(\frac{1}{\sqrt{n}})$ of \cite{negrea2019information}. We present additional empirical results and all technical proofs in the Appendix.



% {\bf Post on April 9 [slack]:} A tentative task assignment for the near term — lets see if we can meet next Fri:
% \begin{itemize}
% \item  Related work on uniform stability of noisy iterative algorithms: @Yingxue
% \item Related work on information theoretic bounds for noisy iterative algorithms: @Tiancong
% \item Related work on generalization bounds for normalizing flows: @robert
% \item Detailed analysis of SGD with Gaussian noise (Section 4): @Yingxue and @Tiancong (pls work out the details based on the sketch)
% \item Validity of assumptions for NF analysis + alternatives (Section 3.3): @Yingxue and @robert
% \item Related work on noisy SGD with Levy processes, stable distributions: @Tiancong
% \item Prelim analysis of noisy SGD with Levy processes: @arindam
% \item Experiments with deep networks, include image-net variants: @Tiancong
% \item Experiments with NFs: @robert
% \end{itemize}

% For the related work, we want
% to have a fine grained exposition, using our notation + language
% differences in (a) assumptions and (b) results w.r.t. our new material



==> Neurips2021/sec/noisy_iterative.tex <==









==> Neurips2021/sec/notes.tex <==
\subsection{Gaussian Noise: Without Projection}
\abcomment{this is just for reference, will be removed}

If the noise added is Gaussian, then we have
\begin{align*}
I_{A,B}  = \bigintsss_x \frac{ \left(  p_{\mu_B,\sigma} -   p_{\mu'_B,\sigma} \right)^2 }{ p_{\mu_A,\sigma}} dx 
 = \frac{1}{(\sqrt{2\pi} \sigma)^d} \bigints_x \frac{ \bigg( \exp(- \| x - \mu_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \mu'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} dx~,
\end{align*}
where the latter is a full $p$-dimensional integral. For each $x$, we can apply mean-field theorem [][] to get:
\begin{align*}
 \exp(- \| x - \mu_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \mu'_B\|_2^2 / 2\sigma^2 ) 
 & = \bigg\langle \mu_B - \mu'_B , \nabla \exp(- \| x - \tilde{\mu}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
\end{align*}
where $\tilde{\mu}_B = \alpha_x \mu_B + (1-\alpha_x) \mu'_B$, where $\alpha_x \in [0,1]$ depends on $x$. Note that $\| \tilde{\mu}_B\|_2 \leq \max(\|\mu_B\|_2,\|\mu'_B\|_2) \triangleq \bar{\mu}_B$. We have
\begin{align*}
  \nabla \exp(- \| x - \tilde{\mu}_B\|_2^2 / 2\sigma^2) & = \frac{x -\tilde{\mu}_B}{\sigma^2} \exp(- \| x - \tilde{\mu}_B\|_2^2 / 2\sigma^2)~, 
\end{align*}
so that
\begin{align*}
& \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{ \bigg( \exp(- \| x - \mu_B\|_2^2 / 2\sigma^2 ) - \exp(- \| x - \mu'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
= \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{\bigg\langle \mu_B - \mu'_B , \frac{x -\tilde{\mu}_B}{\sigma^2} \exp(- \| x - \tilde{\mu}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{\| \mu_B - \mu'_B \|_2^2 \| \frac{x -\tilde{\mu}_B}{\sigma^2} \|_2^2 \exp(- \| x - \tilde{\mu}_B\|_2^2 / \sigma^2) }{\exp(-\| x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{2}{\sigma^4} \| \mu_B - \mu'_B \|_2^2 \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg)  \exp\left(-\frac{\|x-\tilde{\mu}\|_2^2}{\sigma^2} + \frac{\|x\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
= \frac{1}{(\sqrt{2\pi} \sigma)^d} \frac{2}{\sigma^4} \| \mu_B - \mu'_B \|_2^2 \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg)  \exp\left( \frac{\|\tilde{\mu}_B\|_2^2}{\sigma^2}\right)  \exp\left(-\frac{\|x-2\tilde{\mu}_B\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
\leq \frac{2}{\sigma^4} \| \mu_B - \mu'_B \|_2^2 \exp\left( \frac{\|\bar{\mu}_B\|_2^2}{\sigma^2}\right) \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg)  \frac{1}{(\sqrt{2\pi} \sigma)^d} \exp\left(-\frac{\|x-2\tilde{\mu}_B\|_2^2}{2\sigma^2} \right) ~.
\end{align*}
% Now, consider the random variable $\tilde{X} \sim \cN(\tilde{\mu}_B, \sigma^2 )$. 
% Note that $\tilde{X}$ is sub-Gaussian with $\| \tilde{X} \|_{\psi_2} \leq c_0 (\sigma^2 + \| \tilde{\mu}_B\|_2^2) \leq c_0 (\sigma^2 + \|\bar{\mu}_B\|_2^2)$, where $c_0$ is an absolute constant. Then \abcomment{this needs to be shown, some variant of this should be true}, for an absolute constant $c_1$ \abcomment{apply Jensen's?}
We have
\begin{align*}
\exp\left(-\frac{\|x-2\tilde{\mu}_B\|_2^2}{2\sigma^2} \right) 
\leq \exp\left(-\frac{\|x-2\mu_B\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2\mu'_B\|_2^2}{2\sigma^2}~, \right) 
\end{align*}
so that
\begin{align*}
\bigintss_x \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg) & \frac{1}{(\sqrt{2\pi} \sigma)^d} \exp\left(-\frac{\|x-2\tilde{\mu}_B\|_2^2}{2\sigma^2} \right) dx \\
& \leq \bigintss_x \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg) \frac{1}{(\sqrt{2\pi} \sigma)^d} \exp\left(-\frac{\|x-2\mu_B\|_2^2}{2\sigma^2} \right) dx \\ 
& \phantom{\leq ......} + \bigintss_x \bigg(\|x\|^2 + \| \bar{\mu}_B \|_2^2 \bigg) \frac{1}{(\sqrt{2\pi} \sigma)^d} \exp\left(-\frac{\|x-2\mu'_B\|_2^2}{2\sigma^2} \right) dx \\
& \leq \bigg( d\sigma^2 + 2d\|\mu_B\|_2^2 + \| \bar{\mu}_B\|_2^2 \bigg) + \bigg( d\sigma^2 + 2d\|\mu'_B\|_2^2 + \| \bar{\mu}_B\|_2^2 \bigg) \\
& \leq 2d \big(\sigma^2 + 2\|\mu_B\|_2^2 + 2\|\mu'_B\|_2^2 + \frac{1}{d} \|\bar{\mu}_B\|_2^2 \big)
\end{align*}
Putting everything back together, we have
\begin{align*}
I_{A,B} & \leq \frac{2}{\sigma^4} \| \mu_B - \mu'_B \|_2^2 \exp\left( \frac{\|\bar{\mu}_B\|_2^2}{\sigma^2}\right) 2 \big(d\sigma^2 + 2d\|\mu_B\|_2^2 + 2d\|\mu'_B\|_2^2 + \frac{1}{2} \|\bar{\mu}_B\|_2^2 \big)\\
& \leq 2  \bigg( \frac{d}{\sigma^2} + \frac{d\|\mu_B\|_2^2}{\sigma^4} + \frac{d\|\mu'_B\|_2^4}{\sigma^4} + \frac{ \|\bar{\mu}_B\|_2^2}{2\sigma^4} \bigg) \exp\left( \frac{\|\bar{\mu}_B\|_2^2}{\sigma^2}\right)~~\| \mu_B - \mu'_B \|_2^2~.
\end{align*}
The current analysis without projection ends up getting a dependence on $d$, so that we need $d \leq c_0 \sigma^2$.

==> Neurips2021/sec/related.tex <==


\textbf{Uniform stability.} Uniform stability has been a classical approach for bounding generalization error \citep{bousquet2002stability,bousquet2020sharper,feldman2018generalization,feldman2019high}, pioneered by \citet{rogers1978finite,devroye1979distribution}. 
Recently, uniform stability has been shown powerful in analyzing the  stability of SGLD \cite{WellingT11}. 
There has been work on analyzing its uniform stability with the state-of-the-art bound to be $\sqrt{\sum_{t} \beta\eta_{t}}/n $ ~\citep{mou2018generalization,Li2020On}. \citet{mou2018generalization} prove the uniform stability of SGLD
by showing that the uniform stability can be bounded by the squared Hellinger distance, and further they establish discretized Fokker-Planck equations for analyzing the squared Hellinger distance. 
Recently, \citet{Li2020On} follow up on \citet{mou2018generalization} and derive a data-dependent bound, dropping the dependence on the Lipschitz constant of the loss. As a special case, SGLD can be viewed as a differentially private SGD algorithm (DP-SGD) with constant noise variance. 
Uniform stability has also been popular in the differential privacy literature for analyzing the generalization error bound of DP-SGD algorithms. 
Recently, \citet{bassily2019private} analyze the uniform stability of DP-SGD for convex optimization by showing the gradient update is a non-expansive operation, which is the key fact in proving the stability of SGD \cite{hardt2016train}. 
The approach in \citet{hardt2016train} can extend to non-convex setting as well, however it requires fast decaying in step size as $\eta_t = O(1/t)$.  \citet{bassily2020stability} provide stability analysis of SGD for convex and non-smooth functions. 

\textbf{Information-theoretic bound.} Besides the works mentioned above, other theories of deriving generalization bounds for noisy iterative algorithms have been proposed via information-theoretic approaches \citep{russo2016controlling, xu2017information}. Such results show that the generalization error of any learning algorithm can be bounded as $O(\sqrt{I(S; \w)/n})$, where $I(S; \w)$ is the mutual information
between the algorithm input $S$ and the algorithm output $\w$. Thus, recent works following this approach focus on bounding the mutual information for a broad class of iterative algorithms, including SGLD  which obtains a $O(\sqrt{\log T/n})$ generalization bound by choosing $\eta_k = O(1/k)$\cite{pensia2018generalization,bu2019tightening}. Subsequent improvements to this technique were made by 
\citet{negrea2019information, haghifam2020sharpened, Li2020On} 
to prove data-dependent generalization bounds that do not depend
on the Lipschitz constant of the loss function and obtain $\sqrt{\sum_k \beta\eta_{k}}/n $ bounds, showing an improvement with respect to $n$ over results in \citet{bu2019tightening,pensia2018generalization}. 
Especially, \citet{haghifam2020sharpened} introduce generalization bounds based on conditional mutual information inspired by \cite{steinke2020reasoning}, leading to tighter bounds than those based on mutual information. Recently, \citet{neu2021informationtheoretic} extend this information-theoretic to derive generalization bound for vanilla SGD. Our result matches the state-of-the-art bound, i.e., $\sqrt{\sum_k \beta\eta_{k}}/n $ \cite{negrea2019information, haghifam2020sharpened, Li2020On,mou2018generalization}, ignoring the Lipschitz constant factor. 


==> Neurips2021/sec/stab_exp_familly.tex <==
% We assume that the multi-variate noise is sub-Gaussian and from a suitable exponential family, so that for $\bxi \in W \subseteq \R^p$
% \begin{align*}
% p_{\btheta}(\bxi) = \exp(\langle \bxi, \btheta \rangle - \psi(\btheta)) \pi_0(\bxi)~,
% \end{align*}
% where $\psi(\btheta)$ is the log-partition function and $\pi_0(\w)$ is the base measure. In our context, we will work with a scaled form based on natural parameter $\btheta/2\sigma^2$, so that
% \begin{align*}
% p_{\btheta,\sigma}(\bxi) = \exp(\langle \bxi, \btheta/2\sigma^2 \rangle - \psi(\btheta/2\sigma^2)) \pi_0(\bxi)~.
% \end{align*}
% Note that the base measure $\pi_0(\bxi)$ does not change with such scaling. Recall that by construction, for $\btheta \in \Theta \subseteq \R^p$, $\psi(\theta)$ is smooth and strongly convex [][][]. Our analysis will cover several
% popular exponential families including Gaussians, Poisson, gamma, Laplace, exponential, among others (see Table ?) [][]. Further, we always consider symmetric versions of one sided distributions such as Poisson, gamma, Laplace, and exponential. 

% We consider adding independent exponential family noise to every component of the gradient update, i.e.,
% for a mini-batch $B$, 
% \begin{align*}
% \w_{t+1} = \w_t - \eta_t \nabla F(\w_{t-1},S_B) + \bxi_t~,
% \end{align*}
% where $\bxi_t \sim p_{\theta_t,\sigma_t}$ so that the components $\xi_t^j, j=1,\ldots,p$ are independent. As a result, the joint distribution $p_{\btheta,\sigma}(\bxi)$ can be written as a product over marginal distributions:
% \begin{align*}
% p_{\btheta,\sigma}(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_j/2\sigma^2 - \psi_j(\theta_j)) \pi_0(\xi_j/2\sigma^2)~,
% \end{align*}
% where we have overloaded notation and used $\pi_0$ to also denote the marginal base measure respectively. Note that in our notation, $\pi_0(\bxi) = \prod_{j=1}^p \pi_0(\xi_j)$ and also $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$. 
% \abcomment{The marginal distributions can be assumed to be sub-Gaussian (sub-Exponential), so the high-d distribution will also be sub-G (sub-E) since its a product of marginal sub-G. Need to add text on this, along with examples.}

% For the analysis, we will use both the natural and expectation parameterization form.
% Recall that exponential families can be represented in terms of the expectation parameterization as follows [][]:
% \begin{align*}
% p_{\btheta}(\bxi) = p_{\m}(\bxi) = \exp(-d_{\phi}(\bxi,\m)) q_0(\bxi) ~,
% \end{align*}
% where $q_0(\bxi)$ is the (modified) base measure, $\m = \nabla \psi(\btheta)$, $\nabla \phi = \nabla \psi^{-1}$, i.e., Legendre duals [][], and $d_{\phi}(\bxi,\m)$ is the Bregman divergence based on $\phi$. Let $\btheta_{\sigma} = \btheta/(2\sigma^2)$, and let $\m_{\sigma} = \nabla \psi(\btheta_{\sigma})$. Then, $\m_{\sigma} = \nabla \psi(\btheta/(2\sigma^2)) = \m/(2\sigma^2)$\abcomment{the last step is incorrect, where did $\hat{\mu}_{\sigma}$ go?}. Further, $\btheta/(2\sigma^2) = \nabla \psi^{-1}(\m_{\sigma}) = \nabla \phi(\m_{\sigma})$. Then, \abcomment{can possibly be moved to appendix}
% \begin{align*}
% \langle \bxi, \btheta/(2\sigma^2) \rangle - \psi(\btheta/(2\sigma^2)) 
% & = \langle \m_{\sigma}, \btheta/(2\sigma^2) \rangle - \psi(\btheta/(2\sigma^2)) + \langle \bxi - \m_{\sigma}, \btheta/(2\sigma^2) \rangle~\\
% & = \phi(\m_{\sigma}) + \langle \bxi - \m_{\sigma}, \nabla \phi(\m_{\sigma}) \rangle \\
% & = - d_{\phi}(\bxi, \m_{\sigma}) + \phi(\bxi)~.
% \end{align*}
% Further, since $\psi$ is strongly convex and smooth, so is $\phi$ [][], and there are constants $c_1, c_2, c_1 \leq c_2$ such that
% \begin{equation*}
%     c_1 \| \bxi - \m \|_2^2 \leq d_{\phi}(\bxi,\m) \leq c_2 \| \bxi - \m \|_2^2~,
% \end{equation*}
% for any $\bxi,\m$ in the domain [][].


% %We further assume that the base measure $\pi_0(\xi_j) \leq 1, j=1,\ldots,p$, \abcomment{may not be necessary} which is satisfied by many 


% \abcomment{There are 3 key steps in the analysis, which will be converted into Lemma}

% \subsection{Step 1}
% Following the earlier analysis, our goal is to bound:\abcomment{use $\bxi$ instead of $x$}
% \begin{align*}
% I_{A,B} &=  \bigintsss_\bxi \frac{(p_{\btheta_B,\sigma} - p_{\btheta'_B,\sigma})^2}{p_{\btheta_A,\sigma}} d\bxi \\
% & = \bigints_\bxi \frac{ \bigg( \exp(\langle \bxi, \btheta_B/2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2)) - \exp(\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2))\bigg)^2}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) d\bxi
% \end{align*}
% Now, by mean-value theorem, for some $\tilde{\btheta}_B = \alpha_x \btheta_B + (1-\alpha_x) \btheta'_B$, $\alpha_x \in [0,1]$, we have
% \begin{align*}
% \bigg( \exp & (\langle \bxi, \btheta_B/2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2)) - \exp(\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2)) \bigg)^2 \\
% & \leq \big( \langle \btheta_B - \btheta'_B , \nabla_{\btheta} \exp(\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2)) \rangle  \big)^2 \\
% & = \| \btheta_B - \btheta'_B \|_2^2 \left\langle \frac{\btheta_B - \btheta'_B}{\|\btheta_B - \btheta'_B \|_2}, \frac{\bxi - \nabla \psi(\tilde{\btheta}_B/2\sigma^2)}{2\sigma^2} \exp\left[\langle \bxi, \tilde{\btheta}_B /2 \sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right] \right\rangle^2 \\
% & \stackrel{(a)}{=} \frac{\| \btheta_B - \btheta'_B \|_2^2}{4\sigma^4} \left\langle \u_{B,B'}, \left(\bxi - \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right) \right\rangle^2 \exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right] \\
% %& \stackrel{(b)}{\leq} \frac{\| \theta_A - \theta_B \|_2^2}{4\sigma^4} \left\| x - \nabla \psi(\tilde{\theta}_B/2\sigma^2) \right\|_2^2 \exp\left[\langle x, \tilde{\theta}_B / \sigma^2 \rangle - 2\psi(\tilde{\theta}_B/2\sigma^2) \right] \\
% & \leq \frac{\| \btheta_B - \btheta'_B \|_2^2}{2\sigma^4} \bigg( \big\langle \u_{B,B'}, \bxi \big\rangle^2 + \left\| \nabla \psi(\tilde{\theta}_B/2\sigma^2) \right\|_2^2 \bigg) \exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right] ~,
% \end{align*}
%  where in (a), $u_{B,B'} = \frac{\theta_B - \theta'_B}{\|\theta_B - \theta'_B \|_2}$ is a unit vector.

% Since $p_{\btheta,\sigma}(\bxi)$ is a product of marginal exponential families, $\psi(\btheta) = \sum_{j=1}^p \psi_j(\theta_j)$, so that the $j$-th component of the gradient $\nabla \psi(\theta)$ is $\nabla_j \psi(\theta) = \psi'_j(\theta_j)$, where $\psi'_j(\theta_j)$ denotes the derivative of $\psi_j(\theta_j)$. Noting that $\psi'_j$ is a monotonic function since $\psi_j$ is convex, we have
% \begin{align*}
% \left\| \nabla \psi(\tilde{\theta}_B/2\sigma^2) \right\|_2^2 & = \sum_{j=1}^p \left| \psi'_j(\tilde{\theta}_{j,B}/2\sigma^2) \right|^2 \\
% & \stackrel{(a)}{\leq} \sum_{j=1}^p \max\left\{ \left| \psi'_j(\theta_{j,B}/2\sigma^2) \right|^2, \left| \psi'_j(\theta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
% & \leq \sum_{j=1}^p \left\{ \left| \psi'_j(\btheta_{j,B}/2\sigma^2) \right|^2 + \left| \psi'_j(\btheta'_{j,B}/2\sigma^2) \right|^2 \right\} \\
% & = \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2 \\
% & \stackrel{(b)}{=} \left\| \m_{B,\sigma} \right\|_2^2 + \left\| \m'_{B,\sigma} \right\|_2^2
% \end{align*}
% where (a) follows since $\tilde{\theta}_{j,B} \in ~\text{interval}(\theta_{j,B},\theta'_{j,B})$\footnote{We use interval$(a,b)$ to denote $[a,b]$ or $[b,a]$, depending on their ordering.} and $\psi'_j$ is monotonic, $\psi'_j(\tilde{\theta}_{j,B}) \in~\text{interval}(\psi'_j(\theta_{j,B}),\psi'_j(\theta'_{j,B}))$, and (b) follows since for exponential families, the mean parameter $\mu = \nabla \psi(\theta)$ by Legendre duality [][], and $\m_{B,\sigma}, \m_{B',\sigma}$ are respectively the mean parameters for $p_{\btheta_B,\sigma}, p_{\btheta_{B'},\sigma}$. As a result,
% \begin{align*}
% \bigg( \exp & (\langle \bxi, \btheta_B/2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2)) - \exp(\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2)) \bigg)^2 \\
% & \leq \frac{\| \btheta_B - \btheta'_B \|_2^2}{2\sigma^4} \bigg( \big\langle \u_{B,B'}, \bxi \big\rangle^2 + \| \m_{B,\sigma} \|_2^2 + \| \m'_{B,\sigma} \|_2^2 \bigg) \exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]~.
% \end{align*}
% % \tcedit{Instead, we can do
% % \begin{align*}\leq \frac{\| \theta_A - \theta_B \|_2^2}{2\sigma^4} \bigg(  \langle u_{A,B},x\rangle^2 + \| \mu_{B,\sigma} \|_2^2 + \| \mu'_{B,\sigma} \|^2 \bigg) \exp\left[\langle x, \tilde{\theta}_B / \sigma^2 \rangle - 2\psi(\tilde{\theta}_B/2\sigma^2)\right]\end{align*}}
% \abcomment{The $\btheta$ difference can be written as $\m$ difference, see Section 6.3}

% \subsection{Step 2}
% Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. Next we focus on the bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$. 
% % \begin{align*}
% % \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% % \end{align*}



% \begin{lemm}
% For any $\bxi$, we have 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }
% \leq \exp\left[ \frac{c_2}{4\sigma^4} \| \m_\sigma - \m'_\sigma \|_2^2 \right] ~.
% \end{align*}
% \end{lemm}
% \proof Given $\bxi$, for some $\alpha_{\bxi} \in [0,1]$, $\tilde{\btheta} = \alpha_{\bxi} \btheta_B + (1-\alpha_{\bxi}) \btheta'_B$. Denoting $\alpha_{\bxi}$ as $\alpha$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
% \begin{align*}
% \langle \bxi, & \tilde{\btheta}_B / 2\sigma^2 \rangle  - \psi(\tilde{\btheta}_B/2\sigma^2) 
%  = \langle \bxi, \alpha \btheta_B/ 2\sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \rangle - \psi\left( \alpha \btheta_B/ 2 \sigma^2 + (1-\alpha) \btheta'_B/ 2 \sigma^2 \right) \\
% & = \alpha \bigg[ \langle \bxi , \btheta_B / 2 \sigma^2 \rangle - \psi(\btheta_B/ 2 \sigma^2) \bigg]  + (1-\alpha) \bigg[ \langle \bxi , \btheta'_B /2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2) \bigg] \\
% & ~~~~~~~~~~~~~~~
%   + \bigg[ \alpha \psi(\btheta_B/ 2\sigma^2 ) + (1-\alpha) \psi(\btheta'_B/2 \sigma^2) - \psi( \alpha \btheta_B/2\sigma^2 + (1-\alpha) \btheta'_B/2\sigma^2 ) \bigg] \\
% & \stackrel{(a)}{\leq} \max\bigg[ \langle \bxi , \btheta_B/ 2\sigma^2 \rangle - \psi(\btheta_B/2 \sigma^2) , \langle \bxi , \btheta'_B / 2 \sigma^2 \rangle - \psi(\btheta'_B/2 \sigma^2 )  \bigg] \\
% & ~~~~~~~~~~~~~~~ 
%   + \bigg[ \alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2 , \tilde{\btheta}_B/2\sigma^2) \bigg]~,
% \end{align*}
% where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation [Section 3.1.1](Banerjee'05).
% Now, note that
% \begin{align*}
% \alpha d_{\psi}(\btheta_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \tilde{\btheta}_B/2\sigma^2)  
% & \leq \alpha d_{\psi}(\btheta_B/2\sigma^2, \btheta'_B/2\sigma^2) + (1-\alpha) d_{\psi}(\btheta'_B/2\sigma^2, \btheta_B/2\sigma^2) \\
% & \stackrel{(a)}{=} \alpha d_{\phi}(\m'_{\sigma}, \m_{\sigma}) + (1-\alpha) d_{\phi}(\m_{\sigma},\m'_{\sigma})~\\
% & \stackrel{(b)}{\leq} \alpha c_2 \| \m'_{\sigma} - \m_{\sigma} \|_2^2 + (1-\alpha) c_2 \| \m_{\sigma} - \m'_{\sigma} \|_2^2 \\
% & \leq c_2 \| \m_{\sigma} - \m'_{\sigma} \|_2^2~,
% \end{align*}
% where (a) follows by duality [][], and (b) follows due to smoothness.
% As a result,
% \begin{align*}
% & \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] }\\
% & ~~~~~ \leq \exp\left[ \frac{c_2}{4\sigma^4} \| \m_{\sigma} - \m'_{\sigma} \|_2^2\right]
% \frac{ \exp \left[ \max\bigg[ \langle \bxi , \btheta_B \rangle - \psi(\btheta_B) , \langle \bxi , \btheta'_B \rangle - \psi(\btheta'_B)  \bigg] \right] }{ \exp\left[\langle \bxi, \btheta_B / 2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2) \right] } \\
% & ~~~~~ \leq \exp\left[ \frac{c_2}{4\sigma^4} \| \m_{\sigma} - \m'_{\sigma} \|_2^2\right] ~.
% \end{align*}
% That completes the proof.\qed 

% % \abcomment{Old proof - not complete/correct} Using the expectation parameterization form, we have 
% % \begin{align*}
% % \frac{\exp\left[\langle \bxi, \tilde{\theta}_B / 2\sigma^2 \rangle - \psi(\tilde{\theta}_B/2\sigma^2) \right]}{ \exp\left[\langle \bxi, \theta_B / 2\sigma^2 \rangle - \psi(\theta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \theta'_B / 2\sigma^2 \rangle - \psi(\theta'_B/2\sigma^2) \right] } 
% % & = \frac{ \exp \left[ -d_{\phi}(\bxi,\tilde{\m}_{\sigma}) \right]}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} 
% % \end{align*}
% % For $\bxi$ outside interval$[\m_{B,\sigma}, \m'_{B,\sigma})$, the ratio is at most 1 \abcomment{show details, one component of the denominator will dominate, use 1-d argument if it helps}. For $\bxi$ inside interval$[\m_{B,\sigma}, \m'_{B,\sigma}]$, we have
% % \begin{align*}
% % \frac{ \exp \left[ -d_{\phi}(\bxi,\tilde{\m}_{\sigma}) \right]}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} 
% % & \leq \frac{1}{ \exp \left[ -d_{\phi}(\bxi,\m_{B,\sigma}) \right] +  \exp \left[ -d_{\phi}(\bxi,\m'_{B,\sigma}) \right]} \\
% % &  \leq \frac{1}{ \exp \left[ - c_2 \| \bxi - \m_{B,\sigma} \|_2^2 \right] +  \exp \left[ - c_2 \| \bxi - \m'_{B,\sigma} \|_2^2 \right]} \\
% % & \stackrel{(a)}{\leq} \frac{1}{2} \exp \left[ \frac{c_2}{2} \left( \| \bxi - \m_{B,\sigma}\|_2^2 + \| \bxi - \m'_{B,\sigma} \|_2^2 \right) \right] \\
% % & \leq \frac{1}{2} \exp \left[ \frac{c_2}{2} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right] \\
% % & = \frac{1}{2} \exp \left[ \frac{c_2}{8\sigma^4} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right]~,
% % \end{align*}
% % where (a) follows from AM-GM inequality. That completes the proof. \qed

% \subsection{Step 3}
% Finally, focusing on density ratio, we have
% \begin{align*}
% & \frac{\left(\exp\left[\langle \bxi, \tilde{\btheta}_B / 2\sigma^2 \rangle - \psi(\tilde{\btheta}_B/2\sigma^2) \right] \right)^2 }{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi)
% = \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) \\
% & ~~~ \leq 2 \exp \left[ \frac{c_2}{2\sigma^4} \| \m_{B,\sigma} - \m'_{B,\sigma} \|_2^2 \right] \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] + \exp\left[\langle \bxi, \btheta'_B / \sigma^2 \rangle - 2\psi(\btheta'_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% \end{align*}
% Now, note that
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}  
% & = \exp\left[ \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] \\
% & = \beta_{B,A,\sigma} \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
% \end{align*}
% where
% \begin{align*}
% \beta_{B,A,\sigma} & = \exp \left[ \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big) \right] ~.
% \end{align*}
% Note that
% \begin{align*}
% \log \beta_{B,A,\sigma} & = \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \big( 2\psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \big)\\
% & = - \bigg( \psi(\btheta_B/2\sigma^2) - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \bigg) - \bigg( \psi(\btheta_B/2\sigma^2) - \psi(\btheta_A/2\sigma^2) \bigg) \\
% & \stackrel{(a)}{\leq} \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2)  \bigg\rangle + \bigg\langle (\btheta_A - \btheta_B)/2\sigma^2, \nabla \psi( \btheta_A/2\sigma^2)  \bigg\rangle   \\
% & = \bigg\langle (\btheta_B - \btheta_A)/2\sigma^2, \nabla \psi( (2\btheta_B - \btheta_A)/2\sigma^2) - \nabla \psi(\btheta_A/2\sigma^2)  \bigg\rangle  \\
% & \stackrel{(b)}{=} \bigg( d_{\psi}(\btheta_B/2\sigma^2, \btheta_A/2\sigma^2) + d_{\psi}(\btheta_A/2\sigma^2 , (2 \btheta_B - \btheta_A)/2\sigma^2 ) - d_{\psi}(\btheta_B/2\sigma^2, (2 \btheta_B - \btheta_A)/2\sigma^2) \bigg)  \\
% & \leq \big( c_2 \| \btheta_B - \btheta_A \|_2^2 + c_2 \| \btheta_A - (2\btheta_B - \btheta_A) \|_2^2 - c_1 \| \btheta_B - (2\btheta_B - \btheta_A) \|_2^2 \big) / 8 \sigma^4 \\
% & = (5c_2 - c_1) \| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 / 2 ~,
% \end{align*}
% where (a) follows from the convexity of $\psi$, and (b) follows from the three-point property of Bregman divergences [][] given by
% \begin{equation*}
% \langle \x_1 - \x_2, \nabla \psi(\x_3) - \nabla \psi(\x_2) \rangle = d_{\psi}(\x_1,\x_2) + d_{\psi}(\x_2,\x_3) - d_{\psi}(\x_1,\x_3) ~,
% \end{equation*}
% with $\x_1 = \btheta_B/2\sigma^2, \x_2 = \btheta_A/2\sigma^2, \x_3 = (2\btheta_B - \btheta_A)/2\sigma^2$.
% Since $\phi$ is smooth, we also have
% \begin{align*}
% \| \btheta_B/2\sigma^2 - \btheta_A/2\sigma^2 \|_2^2 & = \| \nabla \phi( \m_{B,\sigma} ) - \nabla \phi (\m_{A,\sigma}) \|_2^2 \leq  c_2^2 \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 = \frac{c_2^2}{4\sigma^2} \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 ~,
% \end{align*}
% we have 
% \begin{align*}
% \frac{\exp\left[\langle \bxi, \btheta_B / \sigma^2 \rangle - 2\psi(\btheta_B/2\sigma^2) \right] }{\exp\left[\langle \bxi, \btheta_A / 2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2) \right]}
% \leq \exp \left[ \frac{(5c_2 - c_1)c_2^2}{8\sigma^4} \| \m_{B,\sigma} - \m_{A,\sigma} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/2\sigma^2 \rangle - \psi( (2\btheta_B - \btheta_A)/2\sigma^2) \right]~,
% \end{align*}

% The analysis for the term involving $\btheta'_B$ is similar. 

% \subsection{Wrap Up}

% \abcomment{These are notes to wrap up the analysis}

% Note that we have managed to bound the density ratio term involving $\tilde{\btheta}_B$ and $\btheta_A$ as a sum of two exponential family distributions with parameters $(2\btheta_B - \btheta_A)$ and $(2\btheta'_B - \btheta_A)$. Note that the joint distributions continue to be product of marginal distributions. Thus if the marginals are sub-Gaussian (sub-exponential) distributions, the joint distributions will be sub-Gaussian (sub-Exponential) since they are a product of independent univariate sub-Gaussian (sub-exponential) distributions.

% The only technical part left to show is to bound the expectation of $\langle \u_{B,B'}, \bxi \rangle^2$. If the marginals have a subG distribution with $\psi_2$ norm $\kappa$, we should be able to bound the expectation by $c_3 \kappa^2$. The argument for subE distribution would be similar, the bound may be $\c_4 \kappa^4$.

% \abcomment{Finally, similar to the Gaussian case, choose $\eta_t$ to control the multiplicative terms, and show the stability bound.}




% --------------------------

% \tccomment{Recovery starts here}

In this section, we consider Noisy SGD with Exponential family noise \citep{barndorff2014information,brown1986fundamentals,wainwright2008graphical}. Exponential families are typically represented in terms of natural parameters, and we consider componentwise independent distributions with scaling $\sigma^2 > 0$, i.e., 
\begin{align*}
\vspace{-3mm}
p_{\btheta,\sigma}(\bxi) = \exp(\langle \bxi, \btheta/2\sigma^2 \rangle - \psi(\btheta/2\sigma^2)) \ppi_0(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_j/2\sigma^2 - \psi_j(\theta_j/2\sigma^2)) \pi_0(\xi_j)~,
\end{align*}
where the log-partition function $\psi(\btheta/2\sigma^2)= \sum_{j=1}^p \psi_j(\theta_j/2\sigma^2)$ is smooth and strongly convex \citep{barndorff2014information,banerjee2005clustering}, and $\ppi_0(\xi) = \prod_{j=1}^p \pi_0(\xi_j)$ is the base measure. By Lengendre duality, exponential families can also be written in terms of Bregman divergences as $\exp(-d_{\phi_\sigma}(\bxi,\mu))q_\sigma(\bxi)$ \citep{barndorff2014information,banerjee2005clustering,frigyik2008functional,forster2002relative}, where $\phi_\sigma$ is the dual convex function, $\mu$ is the mean parameter, and $q_0$ is the base measure. Noisy SGD with exponential families at step $t$ have mean parameter $\m_{B_t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t})$ so that the next iterate 
%Specifically, we consider noisy SGD update by sampling from an exponential exponential family, i.e., 
%with mean at gradient update
\begin{align}
\label{eq:exp_update}
  \w_{t} \sim P_{B_t,\bxi_t,\sigma|\w_{0:t-1}} & = \exp(-d_{\phi_\sigma}(\bxi,\m_{B_t})) q_\sigma(\bxi) \\
  &= \exp(-d_{\phi_\sigma}(\bxi, \w_{t-1} - \eta_t \nabla \ell (\w_{t-1},S_{B_t})) q_\sigma(\bxi)~.\nonumber
\end{align}
% where $d_{\phi_{\sigma}}(\bxi,\m)$ (e.g., $\m =\w_{t-1} - \eta_t \nabla \ell (\w_{t-1},S_{B_t})$ in \eqref{eq:exp_update}) is the Bregman divergence based on $\phi_{\sigma}$ and 
% $S_{B_t}$ is a mini-batch drawn randomly from training set $S$, $\nabla \ell (w_{t-1},S_{B_t})$ is the stochastic gradient evaluated on $S_{B_t}$, and 
By duality~\cite{kakade2009duality}, $\phi_{\sigma}:\R^d\rightarrow \R$ is a strongly convex and smooth function parameterized by $\sigma$.
%the way $\phi_\sigma$ depends on $\sigma $ in domain $\Omega$ will be specified by its dual function, 
%and $q_\si(\bxi)$ is the base measure. 
% Note that for Gaussian noise, we have $\phi_{\sigma}(\bxi) = \bxi^2/2\sigma^2$, $d_{\phi_{\sigma}}(\bxi, \m_B) = \|\bxi- \mu_B\|_2^2/2\sigma^2$, $q_0(\bxi)=1/\sqrt{\left(2 \pi \sigma^{2}\right)^{d}}$. 
Since $\phi_{\sigma}$ is strongly convex and smooth, there exists constants 
%so we assume there exists strongly convexity constant $c_1$ and Lipschitz smoothness constant 
$c_1, c_2$, $c_1 \leq c_2$ such that
\begin{equation*}
    c_1 \| \bxi - \m \|_2^2 \leq d_{\phi_{\sigma}}(\bxi,\m) \leq c_2 \| \bxi - \m \|_2^2~,
    % \quad\text{and}~ c_1 \| \bxi - \btheta \|_2^2 \leq d_{\psi}(\bxi,\btheta) \leq c_2 \| \bxi - \btheta \|_2^2
\end{equation*}
for any $\bxi,\m$ in the domain $\Theta$ and any $\sigma\in \Omega$.  
% \yzcomment{between line 239-245, the material reads disconnected from the noisy algorithm, either we drop them or add connections. }\abcomment{done}
% \abdelete{For the analysis, we consider the natural parameter form: \yzcomment{can we write something to connect $p_{\btheta,\sigma}(\bxi) $ with $\w_t$ or $d_{\phi_{\sigma}}(\bxi,\m)$? }
% \begin{align*}
% p_{\btheta,\sigma}(\bxi) = \exp(\langle \bxi, \btheta/2\sigma^2 \rangle - \psi(\btheta/2\sigma^2)) \Pi_0(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_j/2\sigma^2 - \psi_j(\theta_j/2\sigma^2)) \pi_0(\xi_j)~,
% \end{align*}
% where $\psi(\btheta/2\sigma^2)= \sum_{j=1}^p \psi_j(\theta_j/2\sigma^2)$ is the dual function of $\phi_{\sigma}$ which is also smooth and strongly convex and $\Pi_0(\xi) = \prod_{j=1}^p \pi_0(\xi_j)$ is the base measure.  Properties about $\psi,\phi$ and their Bregman divergence can be found in Appendix \ref{app:exp}.} 
% In our context, we will work with a scaled form based on natural parameter $\btheta/2\sigma^2$, so that
% \begin{align*}
% p_{\btheta,\sigma}(\bxi) = \exp(\langle \bxi, \btheta/2\sigma^2 \rangle - \psi(\btheta/2\sigma^2)) \Pi_0(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_j/2\sigma^2 - \psi_j(\theta_j/2\sigma^2)) \pi_0(\xi_j)~.
% \end{align*}
% Note that the base measure $\pi_0(\bxi)$ does not change with such scaling.
% For the analysis, we will use both the natural and expectation parameterization form.
% Recall that exponential families can be represented in terms of the expectation parameterization as follows [][]:
% \begin{align*}
% p_{\btheta}(\bxi) = p_{\m}(\bxi) = \exp(-d_{\phi}(\bxi,\m)) q_0(\bxi) ~,
% \end{align*}
% where $q_0(\bxi)$ is the (modified) base measure, $\m = \nabla \psi(\btheta)$, $\nabla \phi = \nabla \psi^{-1}$, i.e., Legendre duals [][], and $d_{\phi}(\bxi,\m)$ is the Bregman divergence based on $\phi$. Let $\hat{\btheta}_{\sigma} = \btheta/(2\sigma^2)$, and let $\hat{\m}_{\sigma} = \nabla_{\hat{\btheta}_{\sigma}} \psi(\hat{\btheta}_{\sigma})$. Then, $\m_{\sigma} = \nabla \psi(\btheta/(2\sigma^2)) = \hat{\m}_{\sigma}/(2\sigma^2)$. Further, $\btheta/(2\sigma^2) = \nabla \psi^{-1}(\m_{\sigma}) = \nabla \phi(\m_{\sigma})$. Then,
% \begin{align*}
% \langle \bxi, \btheta/(2\sigma^2) \rangle - \psi(\btheta/(2\sigma^2)) 
% & = \langle \m_{\sigma}, \btheta/(2\sigma^2) \rangle - \psi(\btheta/(2\sigma^2)) + \langle \bxi - \m_{\sigma}, \btheta/(2\sigma^2) \rangle~\\
% & = \phi(\m_{\sigma}) + \langle \bxi - \m_{\sigma}, \nabla \phi(\m_{\sigma}) \rangle \\
% & = - d_{\phi}(\bxi, \m_{\sigma}) + \phi(\bxi)~.
% \end{align*}
%Further, since $\psi$ is strongly convex and smooth, so is $\phi$ \citep{banerjee2005clustering, kakade2009duality}, 


Recall that running SGD with Exponential family noise with $S$ and $S_n^\prime$, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate, for a fixed mini-batch $B_t$, following \eqref{eq:nmia}, we have $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively to denote distributions over $\cW$ corresponding to $S, S'_{n}$, where $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively have mean parameters:
\begin{align*}
    \m_{B_t}  = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t}) \qquad \text{and} \qquad
    \m'_{B_t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_{B_t}) ~.
\end{align*}
Based on Proposition \ref{prop:mixmodel}, the conditional distributions $P_{t \mid} $ and $ P_{t}^{\prime}$  over $\cW$ respectively corresponding to $S, S'_{n}$ are mixture of Exponential family, i.e., $ P_{t|} = s Q_{t|} + (1-s) R_{t|}~$ and$ P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~$, where 
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  In order to bound
the KL divergence $K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right)$
based on Theorem \ref{theo:stab}, 
the goal is to bound 
$$I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}$$
for  $B_t \in G_1$ and  $A_t \in G_0$. 
%We further assume that the base measure $\pi_0(\xi_j) \leq 1, j=1,\ldots,p$, \abcomment{may not be necessary} which is satisfied by many 
%
% \abcomment{There are 3 key steps in the analysis, which will be converted into Lemma}
%
% \subsection{Analysis for Exponential Family}
% Following the earlier analysis, our goal is to bound:
% \begin{align*}
%     I_{A,B} &=  \bigintsss_\bxi \frac{(p_{\btheta_B,\sigma} - p_{\btheta'_B,\sigma})^2}{p_{\btheta_A,\sigma}} d\bxi 
% \end{align*}
% % \begin{align*}
% % I_{A,B} &=  \bigintsss_\bxi \frac{(p_{\btheta_B,\sigma} - p_{\btheta'_B,\sigma})^2}{p_{\btheta_A,\sigma}} d\bxi \\
% % & = \bigints_\bxi \frac{ \bigg( \exp(\langle \bxi, \btheta_B/2\sigma^2 \rangle - \psi(\btheta_B/2\sigma^2)) - \exp(\langle \bxi, \btheta'_B / 2\sigma^2 \rangle - \psi(\btheta'_B/2\sigma^2))\bigg)^2}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) d\bxi
% % \end{align*}
Similar as the analysis for Gaussian noise, we have the following result for Exponential family noise:
\begin{restatable}{lemm}{lemmexpinfo}\label{lemm:exp_info}
Consider Noisy SGD with exponetial family noise such that $d_{\phi}$ in \eqref{eq:exp_update} is  $c_1$-strongly convex and $c_2$-smooth, for a given set $\bar S$ and $\w_{t-1}$, let $\Delta_{t}(\bar{S}) = \max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ be data-dependent and adaptively chosen such that $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq c(c_1,c_2)$, then for any $B_t \in G_1$ and  $A_t \in G_0$,  we have
\begin{align}
I_{A_t, B_t} \leq c_0 c_2^2\frac{\eta_{t}^{2}}{\sigma_t^2} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c(c_1,c_2) = \frac{c_1^2}{(3c_2-c_1)c_2(1+c_1)}$.
\end{restatable} 


%\tccomment{Shall we use $c_0$ as a universal constant.}

Here we outline the main ideas of the proof. The details can be found in the Appendix~\ref{app:exp}. Compared to Gaussian case, exponential family does not maintain invariant under rotation, here we apply mean-value theorem to the natural parameter form
\begin{align}
\label{eq:exp_target}
\nonumber I_{A,B} &=  \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \nabla_{\btheta}p_{\tilde{\btheta}_B,\sigma}\rangle ^2}{p_{\btheta_A,\sigma}} d\bxi = \bigintsss_\bxi \frac{\langle \btheta_B -\btheta'_B, \bxi - \nabla \psi(\tilde{\btheta}_B/2\sigma^2)\rangle ^2p_{\tilde{\btheta}_B,\sigma}^2}{4\sigma^4 p_{\btheta_A,\sigma}} d\bxi \\
&\leq \bigintsss_\bxi \frac{\bigg( \big\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2 + \|\btheta_B -\btheta'_B\|_2^2\left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2 \bigg) p_{\tilde{\btheta}_B,\sigma}^2}{2\sigma^4 p_{\btheta_A,\sigma}} d\bxi~.
\end{align}
So far we have rewritten $I_{A,B}$ as a sum of a second moment of $\xi$: $\langle \btheta_B -\btheta'_B, \bxi \big\rangle^2$ and a seemingly constant based on $\tilde{\btheta}_B$: $\left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2$ evaluated on a seemingly scaled probabilistic function $\frac{p_{\tilde{\btheta}_B,\sigma}^2}{p_{\btheta_A,\sigma}}$.
However, since $\tilde{\btheta}_B$ depends on $\bxi$ by $\alpha_\xi$ which has an intractable dependence on $\bxi$, we derive technical arguments: 1) We bound $\left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2$ by a combination of $\left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2$ and $\left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2$: $
    \left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2\leq \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2$; 2) We bound $p_{\tilde{\btheta}_B,\sigma}$ by a combination of $p_{\btheta_B,\sigma}$ and $p_{\btheta'_B,\sigma}$: $
p_{\tilde{\btheta}_B,\sigma}
\leq \exp\left[ c_2 \| \m_B-\m'_B \|_2^2 \right] (p_{\btheta_B,\sigma}+p_{\btheta'_B,\sigma})
$; 3) We show the combination of $p_{\btheta_B,\sigma}$ and $p_{\btheta'_B,\sigma}$ derived by step 2 divided by $p_{\btheta_A,\sigma}$ can be bounded by a proper probabilistic function: $\frac{p_{\btheta_B,\sigma}^2}{p_{\btheta_A,\sigma}}
    \leq \exp \left[ \frac{(3c_2-c_1)c_2}{8c_1\sigma^4} \| \m_{B} - \m_{A} \|_2^2 \right] p_{2\btheta_B-\btheta_A,\sigma}$


% For step 1, recall that $\psi$ is a strongly convex function so the first order derivative of $\psi$ at each component is a monotonic function. With the monotonicity and the fact that $\tilde{\btheta}_B$ lies on the interval between $\btheta_B$ and $\btheta'_B$, we have the following 
% \begin{align}
% \label{eq:exp_step1}
%     \left\| \nabla \psi(\tilde{\btheta}_B/2\sigma^2) \right\|_2^2\leq \left\| \nabla \psi(\btheta_B/2\sigma^2) \right\|_2^2 + \left\| \nabla \psi(\btheta'_B/2\sigma^2) \right\|_2^2,
% \end{align}
% which accomplishes step 1. Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. For step 2, we focus on the bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$, we have the following  
% % \begin{align*}
% % \frac{\exp\left[\langle \bxi, \tilde{\btheta}_B / \sigma^2 \rangle - 2\psi(\tilde{\btheta}_B/2\sigma^2) \right]}{\exp(\langle \bxi, \btheta_A/2\sigma^2 \rangle - \psi(\btheta_A/2\sigma^2))} \pi_0(\bxi) ~.
% % \end{align*}

% Assume there exists constant $c_2>0$ such that $d_{\phi}(\bxi,\m) \leq c_2 \| \bxi - \m \|_2^2$ for any $\bxi,\m$ in the domain $W$, then for any $\btheta_B,\btheta'_B$, we have 
% \begin{align}
% \label{eq:exp_step2}
% p_{\tilde{\btheta}_B,\sigma}
% \leq \exp\left[ c_2 \| \nabla \psi(\btheta_B/2\sigma^2) - \nabla \psi(\btheta'_B/2\sigma^2) \|_2^2 \right] (p_{\btheta_B,\sigma}+p_{\btheta'_B,\sigma})~.
% \end{align}

% The proof is an application of the inversed Jensen's inequality given by the Bregman information [], the details of the proof is relegated in Appendix~\ref{app:exp}. Equation~\eqref{eq:exp_step1} together with equation~\eqref{eq:exp_step2} bridge the gap between $\tilde{\btheta}_B$ and $\btheta_B,\btheta'_B$ which eliminates the $\alpha_\bxi$ term in equation~\eqref{eq:exp_target}.
% The rest of the step is to relate the density ratio term to a probability density with coefficient based on $B,B',A$, we have the following proposition
% \begin{prop}
% \label{prop:exp_step3}
% \begin{equation}
% \begin{split}
% \label{eq:exp_step3}
%     &\frac{(p_{\btheta_B,\sigma}+p_{\btheta'_B,\sigma})^2}{p_{\btheta_A,\sigma}}\leq \frac{2p_{\btheta_B,\sigma}^2}{p_{\btheta_A,\sigma}} +\frac{2p_{\btheta'_B,\sigma}^2}{p_{\btheta_A,\sigma}}\\
%     & \leq 2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta_B-\btheta_A,\sigma}+ 2\exp \left[ \frac{2c_2}{4\sigma^4} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right] p_{2\btheta'_B-\btheta_A,\sigma}
%     \end{split}
% \end{equation}
% \end{prop}
The final step is to gather Equation~\eqref{eq:exp_target},  three steps above, and a proper choice of step size stated in Lemma~\ref{lemm:exp_info}, to complete the proof. 
%The details can be found in Appendix~\ref{app:exp}.
Combining Lemma~\ref{lemm:exp_info} with Theorem~\ref{theo:stab}, we have the following generalization bound for update based on Exponential family:
\begin{theo}
Consider the noisy SGD with Exponential family noise of the update rule \eqref{eq:exp_update},  with mini-batch size $b \leq n/2$, for any given sample $\bar S$, let step size $\eta_t$ and noise $\sigma_t$ be adaptively chosen as in Lemma \ref{lemm:exp_info},
%such that, for any observed $\w_{t-1}$,  $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq c(c_1,c_2)$, where $\Delta_{t}(\bar{S})=\max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z\right)-\nabla \ell\left(\mathbf{w}_{t-1}, \tilde{z}\right)\right\|_{2}$ 
%Then 
we have 
\begin{align}
\left|\mathbb{E}_{S}\left[L_{D}(\w_T)-L_{S}(\w_T)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar S} \sqrt{\sum_{t=1}^{T} \underset{\w_{t-1}}{\mathbb{E} }\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~}~.
\end{align}
where $c$ is a constant with detailed value presented in Appendix.
\label{theo:exp_bound}
\end{theo}


% \tccomment{
% \begin{theorem}
% For exponential family, we have
% \begin{align*}
%     I_{A,B} =  \bigintsss_\bxi \frac{(p_{\btheta_B,\sigma} - p_{\btheta'_B,\sigma})^2}{p_{\btheta_A,\sigma}} d\bxi &\leq \bigintsss_\bxi \frac{p_{\btheta_B,\sigma}^2}{p_{\btheta_A,\sigma}}+\frac{p_{\btheta'_B,\sigma}^2}{p_{\btheta_A,\sigma}} d\bxi \leq 2\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8\sigma^4} \| \hat{\m}_{B,\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]\\
%     &+ 2\exp \left[ \frac{(5c_2 - c_1)c_2^2}{8\sigma^4} \| \hat{\m}_{B',\sigma} - \hat{\m}_{A,\sigma} \|_2^2 \right]
% \end{align*}
% \end{theorem}
% }

Theorem~\ref{theo:exp_bound} extends the result on the expected generalization error of Gaussian noise in Theorem~\ref{theo:guss_gen} to general Exponential family distribution and shows the bound scales as $O(\sqrt{\sum_t^T \frac{\eta_t^2}{\sigma_t^2}}/n)$ which is the same as in the Gaussian noise case.



% \subsection{OLD Text: keeping for ref, remove in the final version}
% \abcomment{Key observation, the ``projection view" (PV), different from previous (Gaussian) analysis } Since $u_{A,B} = \frac{\theta_A - \theta_B}{\|\theta_A - \theta_B \|_2}$ is a unit vector and the distribution is subG, the projection of $\frac{x-\tilde{\mu}_B}{2\sigma^2}$ on the unit vector is a 1-d subG random variable. As a result, the second moment will be bounded as long as $p^2_{\tilde{\theta}_B,\sigma}/p_{\theta_A,\sigma}$ is subG. In fact, it suffices to show that the 1-d projection is subG. 

% Key questions: 
% \begin{enumerate}
% \item Should the analysis be done in expectation or natural parameterization?
% \item How should subG exp family be formalized, w.r.t.~the mean or natural parameters?
% \end{enumerate}

% Switching to mean parameterization: We have
% \begin{align*}
% p_{\theta,\sigma}(x) = p_{\mu,\sigma}(x) = \exp(-d_{\phi}(x,\mu)/2\sigma^2) q_\sigma(x) 
% \end{align*}
% where $q_\sigma(x)$ may have a dependency on $\sigma$.
% So, we have
% \begin{align*}
% I_{A,B} 
% &=  \bigintsss_x \frac{(p_{\theta_B,\sigma} - p_{\theta'_B,\sigma})^2}{p_{\theta_A,\sigma}} dx \\
% & = \bigints_x \frac{ \bigg[ \exp(-d_{\phi}(x,\mu_B)/2\sigma^2) - \exp(-d_{\phi}(x,\mu'_B)/2\sigma^2) \bigg]^2}{\exp(-d_{\phi}(x,\mu_A)/2\sigma^2)} q_\sigma(x) dx     
% \end{align*}
% By mean-value theorem, for some $\tilde{\mu}_B = \alpha_x \mu_B + (1-\alpha_x) \mu'_B$, $\alpha_x \in [0,1]$, we have
% \begin{align*}
% \exp & (-d_{\phi}(x,\mu_B)/2\sigma^2) - \exp(-d_{\phi}(x,\mu'_B)/2\sigma^2) \\
% & = \left\langle \mu_B - \mu'_B, \nabla_{\tilde{\mu}_B} \exp(- d_{\phi}(x,\tilde{\mu}_B)/2\sigma^2) \right\rangle \\
% & = \| \mu_B - \mu'_B \|_2 \left\langle \frac{\mu_B-\mu'_B}{\|\mu_B - \mu'_B\|_2} , \frac{H_{\phi}(\tilde{\mu}_B) (x - \tilde{\mu}_B)}{\sigma^2}  \right\rangle \exp\left[ -d_{\phi}(x,\tilde{\mu}_B)/\sigma^2 \right] ~,
% \end{align*}
% \abcomment{need to bound probability terms with $\tilde{\theta}$ or $\tilde{\mu}$ with corresponding $\theta_B$ or $\mu_B$ terms which do not depend on $x$. Fix the analysis for Gaussians first.}
% where $H_{\phi}(\tilde{\mu}_B) = \nabla^2 \phi(\tilde{\mu}_B)$ is the Hessian. Since $\phi$ is smooth, with $c_{2,\phi} = \| H_{\phi}\|_2$, and with unit vector $u_{B,B'} = \frac{\mu_B - \mu_B'}{\|\mu_B - \mu_B' \|_2}$, we have 
% \begin{align*}
% \langle u_{B,B'}^T H_{\phi}(\tilde{\mu}_B) (x - \tilde{\mu}_B)\rangle ^2 & \leq 2 \langle u_{B,B'}^T H_{\phi}(\tilde{\mu}_B) x \rangle^2 + 2 \langle u_{B,B'}^T H_{\phi}(\tilde{\mu}_B) \tilde{\mu}_B \rangle^2     \\
% & \leq 2 \| H_{\phi}(\tilde{\mu}_B) u_{B,B'} \|_2^2 \bigg\{ \big( v_{B.B'}^T x \big)^2 + \big(v_{B,B'}^T \mu_B \big)^2 + \big(v_{B,B'}^T \mu_B \big)^2 \bigg\}~,
% \end{align*}
% where $v_{B,B'} = \frac{H_{\phi}(\tilde{\mu}_B) u_{B,B'}}{ \| H_{\phi}(\tilde{\mu}_B) u_{B,B'} \|_2}$ is a unit vector. As a result, $z = v_{B.B'}^T x$ is a univariate subGaussian distribution, and $v_{B,B'}^T \mu_B \leq \| \mu_B\|_2$ and $v_{B,B'}^T \mu'_B \leq \| \mu'_B \|_2$. Hence
% \begin{align*}
% \big(u_{B.B'}^T H_{\phi}(\tilde{\mu}_B) (x - \tilde{\mu}_B)\big)^2 & \leq 2 c_{\phi} \bigg\{ z^2 + \| \mu_B\|_2^2 + \| \mu'_B \|_2^2 \bigg\}~.
% \end{align*}
% The distribution ratio term is given by
% \begin{align*}
% \frac{\big(\exp\left[ -d_{\phi}(x,\tilde{\mu}_B)/2\sigma^2 \right]\big)^2}{\exp\left[ -d_{\phi}(x,\mu_A)/2\sigma^2 \right]} q_\sigma(x)
% & = \exp\left[ -\frac{1}{2\sigma^2} \left[ 2 d_{\phi}(x,\tilde{\mu}_B) - d_\phi(x,\mu_A) \right] \right] \\
% & \leq \exp\left[ \langle x, 2\tilde{\theta}_B - \theta_A \rangle/2\sigma^2 - \left(2\psi(\tilde{\theta}_B/2\sigma^2) - \psi(\theta_A/2\sigma^2\right) \right] \pi_0(x)    \\
% & = \beta_{A,B} \exp \left[ \left \langle x, (2\tilde{\theta}_B - \theta_A)/2\sigma^2 \right\rangle - \psi((2\tilde{\theta}_B - \theta_A)/2\sigma^2) \right] \pi_0(x)~,
% \end{align*}
% where
% \begin{align*}
% \beta_{A,B} & = \exp \left[ \psi((2\tilde{\theta}_B - \theta_A)/2\sigma^2 ) - \left(2 \psi(\tilde{\theta}_B/2\sigma^2) - \psi(\theta_A/2\sigma^2) \right) \right]~.
% \end{align*}




==> Neurips2021/sec/stab_gauss.tex <==
% \abcomment{The initial part, before the analysis specific to Gaussian noise, should be moved to Section 3}

% Consider sampling $\bar{S} \sim D^{n+1}$. Let $S,S'$ be size $n$ subsets of $\bar{S}$ which differ by one point. Without loss of generality, we let $S=\{z_1,\ldots,z_{n-1},z_n\}$ and $S' = \{z_1,\ldots,z_{n-1},z'_n\}$, where $z'_n = z_{n+1}$. let $S_0 = \{z_1,\ldots,z_{n-1}\}$. The algorithm uses a mini-batch $B$ of size $b$ in each step. Let the set of all mini-batches be denoted by $G$. Let the set of all mini-batches drawn from $S_0$ be denoted by $G_0$. Note that $|G_0| = \binom{n-1}{b}$. Let the set of all mini-batches which includes the last sample, viz., $z_n$ for $S$ and $z'_n$ for $S'$, be denoted by $G_1$. Note that $|G_1| = \binom{n-1}{b-1}$. Also note that 
% \begin{align*}
%     |G_0| + |G_1| = \binom{n-1}{b} + \binom{n-1}{b-1} = \binom{n}{b} = |G|~,
% \end{align*}
% the total number of $b$-sized mini-batch samples from a dataset of size $n$. The subset of $S$ and $S'$ corresponding to mini-batch $B$ will be denoted as $S_B$ and $S'_B$.

% Consider two collection of points $\{\mu_B : B \in G \}$ and $\{\mu_B : B \in G\}$. In our context, at any stage $t$, conditioned on $w_{t-1}$, for mini-batch $B$, we have
% \begin{align*}
%     \mu_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S_B) \\
%     \mu'_B & = w_{t-1} - \eta_t \nabla F(w_{t-1},S'_B) ~.
% \end{align*}
% Let $p_{\mu,\sigma}$ denote the Gaussian distribution $\cN(\mu, \sigma^2 \I)$. Let $P = \frac{1}{|G|} \sum_{B \in G} p_{\mu_B,\sigma}$ and  $P' = \frac{1}{|G|} \sum_{B \in G} p_{\mu'_B,\sigma}$. Our goal is to bound $KL(P \| P')$ {\em without making any additional assumptions}. Note that $\eta_t,\sigma_t$ can depend on $w_{1:t-1}$, but since the analysis is conditioned on $w_{1:t-1}$, these are effectively constants for the current analysis. 

% Remark: This analysis immediately shows why KL-divergence cannot be used for the non-noisy case -- these will be Dirac measures, and KL-div will be $\infty$. A bound based on TV or Hellinger would still be valid.

% Let 
% \begin{align*}
% Q_1 = \frac{1}{|G_1|} \sum_{B \in G_1} p_{\mu_B,\sigma} \qquad Q_2 = \frac{1}{|G_1|} \sum_{B \in G_1} p_{\mu'_B,\sigma} \qquad R = \frac{1}{|G_0|} \sum_{B \in G_0} p_{\mu_B,\sigma}~.  
% \end{align*}
% Then, with 
% \begin{equation*}
% s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}~,
% \end{equation*}
% we have 
% \begin{align*}
%     P = s Q_1 + (1-s) R \qquad P' = s Q_2 + (1-s) R~.
% \end{align*}
% Then,
% \begin{align*}
% KL(P \| P') & \stackrel{(a)}{\leq} \left(\frac{b}{n} \right)^2 \left(\frac{n}{n-b}\right) \int_x \frac{(Q_1 - Q_2)^2}{R} dx \\
%  & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \bigintsss_x \frac{ \left(  \frac{1}{|G_1|} \left[ \sum_{B \in G_1} p_{\mu_B,\sigma} -  \sum_{B \in G_1} p_{\mu'_B,\sigma} \right] \right)^2 }{\frac{1}{|G_0|} \sum_{B \in G_0} p_{\mu_B,\sigma}} dx \\
%  & \stackrel{(b)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_x \frac{1}{|G_1|}\sum_{B \in G_1}  \frac{ \left(  p_{\mu_B,\sigma} -   p_{\mu'_B,\sigma} \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} p_{\mu_A,\sigma}} dx \\
%  & \stackrel{(c)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_x \frac{1}{|G_1|}  \sum_{B \in G_1} \left(  p_{\mu_B,\sigma} -   p_{\mu'_B,\sigma} \right)^2  \frac{1}{|G_0|}\sum_{A \in G_0} \frac{ 1 }{ p_{\mu_A,\sigma}} dx \\
%  & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \frac{1}{|G_0| |G_1|}  \sum_{A \in G_0} \sum_{B \in G_1} \bigintsss_x \frac{ \left(  p_{\mu_B,\sigma} -   p_{\mu'_B,\sigma} \right)^2 }{ p_{\mu_A,\sigma}} dx ~,
% \end{align*}
% where (a) is from Lemma [], (b)(c) is from Jensen's inequality since function $f(x) = x^2$ is convex and $f(x)=\frac{1}{x}$ is convex on $(0,\infty)$. 
% The analysis upto this point does not need the distributions to be Gaussian.

% \abcomment{Lets move the above part to Section 3. The following can become Section 4 -- the analysis specific to Gaussians, the above is general}

%\subsection{Gaussian Noise: With Projection}

% \abcomment{start by stating the noisy gradient descent algorithm. The earlier sections will be written for general iterative algorithms (not necessarily gradient descnet) with additive noise}

In this section, we consider Noisy SGD with Gaussian noise. Specifically, we consider the following update
\begin{align}
  \w_{t} =  \w_{t-1} - \eta_t \nabla \ell (\w_{t-1},S_{B_t}) + \bxi_t, ~~\text{where}~~
  \bxi_t \sim  \cN(0, \sigma_t^2\mathbb{I}_d)~, \label{eq: sgd_guss_update}
\end{align}

where $S_{B_t}$ is a mini-batch drawn randomly from training set $S$ and 
$\nabla \ell (\w_{t-1},S_{B_t})$ is the stochastic gradient evaluated on $S_{B_t}$, i.e., $\nabla \ell (\w_{t-1},S_{B_t}) = \frac{1}{|S_{B_t}|} \sum_{z \in {S_{B_t}}}\nabla \ell(\w_{t-1},z)$. $\bxi \sim \cN(0, \sigma_t^2\mathbb{I}_d)$ is a d-dimensional isotropic Gaussian noise with variance $\sigma_t^2\mathbb{I}_d$. 
Note that the update in \eqref{eq: sgd_guss_update} with the
special case of $\sigma_t = \sqrt{{2\eta_t}/{\beta}}$ for $\beta >0$  captures the SGLD algorithm. 

Consider running Noisy SGD with Gaussian noise on two datasets $S$ and $S_n^\prime$, 
% we get two joint distributions $P_{0: T}$ and $P_{0: T}^\prime$ over $\w_{0:T}$. Based on the chain rule of KL-divergence in \eqref{eq:klchain}, in order to bound $K L\left(P_{0: T} \| P_{0: T}^{\prime}\right)$, we are interested in analyzing the KL-divergence $K L(P_{t \mid} \| P_{t \mid}^{\prime})$ conditioned on past iterates $\w_{0:(t-1)}$. 
conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate, for a fixed mini-batch $B_t$, following \eqref{eq:nmia}, we have $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ respectively to denote distributions over $\cW$ corresponding to $S, S'_{n}$. Note that, since $\bxi_t$ is Gaussian noise, 
$P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ are two Gaussian distributions with the same variance $\sigma_t^2\mathbb{I}_d$, and with mean $\m_{B_t}$ and $\m^\prime_{B_t}$ respectively  to be
\begin{align*}
    \m_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t}) \\
    \m'_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_{B_t}) ~.
\end{align*}

Based on Proposition \ref{prop:mixmodel}, the conditional distributions $P_{t \mid} $ and $ P_{t}^{\prime}$  over $\cW$ respectively corresponding to $S, S'_{n}$ are mixture of Gassuains, i.e., $ P_{t|} = s Q_{t|} + (1-s) R_{t|}~$ and$ P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~$, where 
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  In order to bound
the KL divergence $K L(P_{t \mid} \| P_{t \mid}^{\prime})$
based on Theorem \ref{theo:stab}, for  $B_t \in G_1$ and  $A_t \in G_0$，we need to bound
\begin{align}
 I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t},~~\text{where} ~~ \bxi_t \sim \cN(0, \sigma_t^2\mathbb{I}_d) ~. 
\end{align}

% $$I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}$$
% with $\bxi_t \sim \cN(0, \sigma_t^2\mathbb{I}_d)$ 

In the following lemma, we show that we can bound $I_{A_t, B_t}$ by the gradient discrepancy between $S$ and $S_n^\prime$, i.e., $\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|$, if we slightly control the step size $\eta_t$, noise variance $\sigma_t^2$ based on a data-dependent quantity that can be evaluated given $S$ and $S_n^\prime$.

\begin{restatable}{lemm}{lemmaiabguss}
For a given set $\bar S$ and $\w_{t-1}$ observed at ${t-1}$ iteration, let $\Delta_{t}(\bar{S}) = \max _{z, \bar{z} \in \bar S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ and $\sigma_t$ to be data-dependent and adaptively chosen such that $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$, for any $B_t \in G_1$ and  $A_t \in G_0$,  we have
\begin{align}
I_{A_t, B_t} \leq c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c$ is a constant~\footnote{ Detail value of $c$ can be found in Appendix.}.\label{lemm:iab_guss}
\end{restatable}


% \begin{lemm}
% For a given set $\bar S$ and $\w_{t-1}$ observed at ${t-1}$ iteration, let $\Delta_{t}(\bar{S}) = \max _{z, \bar{z} \in \bar S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ and $\sigma_t$ to be data-dependent and adaptively chosen such that $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$, for any $B_t \in G_1$ and  $A_t \in G_0$,  we have
% \begin{align}
% I_{A_t, B_t} \leq c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
% \end{align}
% where $c$ is a constant~\footnote{ Detail value of $c$ can be found in Appendix.}.
% \label{lemm:iab_guss}
% \end{lemm}

% To analyze $I_{A_t, B_t}$, we note that $d P_{B_{t}, \boldsymbol{\xi}_{t}}$, $d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}$ and $d P_{A_{t},\boldsymbol{\xi}_{t}}$ are distribution functions of Gaussian distribution with different mean, i.e., $\m_{B_t}$, $\m_{B_t}^\prime$ and $\m_{A_t}^\prime$. Thus it is straightforward to write 
% \begin{align}
% I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{d}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w-\m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
% \end{align}


We highlight the essentials of the proofs here. For any $B_t$ and $A_t$, since $P_{B_{t}, \boldsymbol{\xi}_{t}}$, $P^\prime_{B_{t}, \boldsymbol{\xi}_{t}}$ and $P_{A_{t}, \boldsymbol{\xi}_{t}}$ are Gaussian distributions. Thus, $d P_{B_{t}, \boldsymbol{\xi}_{t}}$, $d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}$ and $d P_{A_{t},\boldsymbol{\xi}_{t}}$ are distribution density functions of Gaussian distribution. Then, it is straightforward to have 
\begin{align}
I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{d}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w-\m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
\end{align}
Note that the above calculation considers integral over $d$-dimensional space which introduced an undesired dimension dependence. However, we note that
isotropic Gaussian noise is spherical symmetric,  we can translate and rotate the coordinate system so that 
$\m_{A_t}=0$  and $ \m_{B_t}, \m_{B_t}^{\prime}$ are mapped to a 2-dimensional space and the Euclidean distances $\|\w-\m_{B_t} + \m_{A_t}\|$, $\|\w-\m_{B_t}^\prime + \m_{A_t}\|$ do not change (Details  can be found in  Appendix \ref{app:guss}). Then
we have $I_{A_t, B_t}$ as 
\begin{align}
I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{2}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime} + \m_{A_t} \right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
\end{align}
Then we treat $\exp \left(-\left\|\w-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ and $\exp \left(-\left\|\w-\m_{B_t}^\prime + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ as two functions of $\w$ where we can 
use Taylor expansion and apply mean-field theorem to bound $I_{A_t, B_t}$ as
\begin{align*}
I_{A_t, B_t} \leq c \frac{\|\m_{B_t} - \m_{B_t}^\prime \|_2^2}{\sigma_t^2}=  c \frac{\eta_t^2\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}}{\sigma_t^2}~,
\end{align*}
where $c$ is a constant with detailed value in  Appendix. Thus, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate,  we have
\begin{align}
\nr K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right) & = \underset{B_{t} \in G_{1},A_{t} \in G_{0}}{\mathbb{E}}\left[\int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}\right]   \leq  \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

Then, based on the chain rule of KL-divergence, we have
\begin{align}
\nr K L\left(P_{0: T} \| P_{0: T}^{\prime}\right) 
& = \sum_{t=1}^{T} \mathbb{E}_{\w_{t-1}} \left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

\begin{restatable}{theo}{genboundguss}
Consider Noisy SGD of update rule \eqref{eq: sgd_guss_update},  with mini-batch size $b \leq n/2$, for any given sample $\bar S$, at every $t$-th iteration, let step size $\eta_t$ and noise $\sigma_t$ be adaptively chosen as in Lemma \ref{lemm:iab_guss}, 
% such that, for any observed $\w_{t-1}$,  $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$, where $\Delta_{t}(\bar{S})=\max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z\right)-\nabla \ell\left(\mathbf{w}_{t-1}, \tilde{z}\right)\right\|_{2}$ 
%Then, with $c = \sqrt{2} c_0$, 
we have 
\begin{align}
\left|\mathbb{E}_{S}\left[L_{D}(\w_T)-L_{S}(\w_T)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar S} \sqrt{\sum_{t=1}^{T} \underset{\w_{t-1}}{\mathbb{E} }\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~},
\end{align}
where $c$ is a constant with detailed value presented in Appendix.
\label{theo:guss_gen}
\end{restatable}

% \begin{theo}
% Consider Noisy SGD of update rule \eqref{eq: sgd_guss_update},  with mini-batch size $b \leq n/2$, for any given sample $\bar S$, at every $t$-th iteration, let step size $\eta_t$ and noise $\sigma_t$ be adaptively chosen as in Lemma \ref{lemm:iab_guss}, 
% % such that, for any observed $\w_{t-1}$,  $\frac{\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})}{\sigma_{t}^{2}} \leq \ln \frac{3}{2}$, where $\Delta_{t}(\bar{S})=\max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z\right)-\nabla \ell\left(\mathbf{w}_{t-1}, \tilde{z}\right)\right\|_{2}$ 
% %Then, with $c = \sqrt{2} c_0$, 
% we have 
% \begin{align}
% \left|\mathbb{E}_{S}\left[L_{D}(\w_T)-L_{S}(\w_T)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar S} \sqrt{\sum_{t=1}^{T} \underset{\w_{t-1}}{\mathbb{E} }\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~},
% \end{align}
% where $c$ is a constant with detailed value presented in Appendix.
% \label{theo:guss_gen}
% \end{theo}

Theorem \ref{theo:guss_gen} shows that 
the expected generalization error of Noisy SGD with Gaussian noise scales as $O(\sqrt{\sum_t^T \frac{\eta_t^2}{\sigma_t^2}}/n)$, capturing the same dependence on $n$, $T$, step size $\eta_t$ as the bound in \cite{Li2020On}. However there are two key differences making our bound sharper than existing bounds in \cite{Li2020On} and \cite{negrea2019information}. The first key difference between our result and \cite{Li2020On} is that we replace the \emph{gradient norms}, i.e., $\frac{1}{n}\sum_{z \in S}\|\ell(\w_t,z)\|$ in \cite{Li2020On} and with gradient discrepancy $\|\nabla \ell(\w_t,z) - \nabla \ell(\w_t, z^\prime) \|$, which is quantitatively smaller than gradient norms as we show in the experiment section. 
The second key difference is the sample dependence compared to  \cite{negrea2019information}.
Although, \cite{negrea2019information} also derived a generalization error bound depending a factor that is similar to gradient discrepancy, named  \emph{gradient incoherence} in their paper, their bound depends on $\frac{1}{\sqrt{n}}$, which is worse than the $\frac{1}{n}$ dependence in our bound. 
% The difference between gradient discrepancy and gradient incoherence is that, gradient discrepancy is evaluated on $z$ from training set and $z^\prime$ from a validation set. The gradient incoherence is the difference between gradients on subset of training samples. Although gradient incoherence is empirically smaller as overved in the 
Thus, our bound in Theorem \ref{theo:guss_gen} inherits the strengths of the existing bounds with dependence on norms of gradient discrepancy, and an $O(1/n)$ sample dependence

% The key difference is the order of dependence on the sample size $n$, i.e., both of our bound and $\cite{Li2020On}$ has a bound of order $\frac{1}{n}$, however, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$.




%Based on the chain rule of  KL-divergence, we have
% \begin{align*}
%  KL(w_1,..., w_T \| w'_1,..., w'_T) \leq  \frac{b^{2}}{n^{2}}  \frac{12 c }{\sigma^2} (1 + \frac{5\ln c}{2})  \sum_{t=1}^T \| \nabla \ell(w_{t-1},z_n) - \nabla \ell(w_{t-1},z'_n) \|_2^2~.
% \end{align*}




%\newpage

==> Neurips2021/sec/stab_heavy_tailed.tex <==

Results for noise with $\exp(-t)$ tail

\subsection{Laplace Noise}


\subsection{Sub-Exponential Noise}


\subsection{Heavy Tails: Infinitely Divisible, Stable Noise}


\section{Experiment}

Model: MLP,~ CNN.

Datasets: MNIST, Fashion MNIST, CIFAR10.

Noise: Gaussian, discrete noise

Plot: Bounds, gradient norm, gradient difference norm. 


==> arXiv/app/app_exp.tex <==
{\bf Datasets.} We use MNIST \cite{mnist}, Fashion-MNIST \cite{fashion-mnist}, CIFAR-10 \cite{cifar10} and CIFAR-100 \cite{cifar10} in our experiments.


%The MNIST and Fashion MNIST datasets both consist of 60,000 training examples and 10,000 test examples. %To construct the experiments, we randomly sample $10,000$  samples from the original training set of MNIST and Fashion MNIST. 
%Details refer to  Table \ref{tab::network_setup_app}. 

\noindent {\bf MNIST dataset:} 60,000 black and white training images, including handwritten digits 0 to 9. We use a subset of MNIST with $n = 10,000$ data points where 1,000 samples from each class are randomly selected. Each image of size $28 \times 28$ is first re-scaled into [0,1] by dividing each pixel value by 255, then z-scored by subtracting the mean and dividing the standard deviation of the training set.


\noindent {\bf Fashion-MNIST dataset:} 60,000 gray-scale training images and 10,000 test images, including 10 clothing categories such as shirts, dresses, sandals, etc. Each image of size $28 \times 28$ is first re-scaled into [0,1] by dividing each pixel value by 255, then z-scored by subtracting the mean and dividing the standard deviation of the training set. 


\noindent {\bf CIFAR-10/-100 dataset:} 60,000 color images consisting of 10/100 categories, e.g., airplane, cat, dog etc. The training set includes 50,000 images while the test set contains the rest 10,000 images. Each image of size $32 \times 32$ has 3 color channels. We first re-scale each image into [0, 1] by dividing each pixel value by 255, then each image is normalized by subtracting the mean and dividing the standard deviation of the training set for each color channel. We also use \textit{RandomCrop} and \textit{RandomHorizontalFlip} for data augmentation.




{\bf Network Architectures.} For experiments on both MNIST and Fashion-MNIST, we use a convolutional neural network with two convolutional layers followed by two fully connected layers with ReLU activations. For experiments use the CIFAR-10 dataset, we consider CNN architecture with two convolutional layers
and three fully connected layers. The detail of each CNN architecture can be found in Table \ref{tab:cnn1} and Table~\ref{tab:cnn2}.

\begin{table}[h]
\caption{CNN architecture for MNIST and Fashion MNIST.}
\centering
\begin{tabular}{cc} 
Layer & Parameters \\
\hline \hline Convolution & 32 filters of $5 \times 5$ \\
Max-Pooling & $2 \times 2$ \\
Convolution & 64 filters of $5 \times 5$\\
Max-Pooling & $2 \times 2$ \\
Fully connected & 1024 units \\
Softmax & 10 units \\
\hline
\end{tabular}
    \label{tab:cnn1}
\end{table}


\begin{table}[h]
\caption{CNN architecture for CIFAR-10.}
\centering
\begin{tabular}{cc} 
Layer & Parameters \\
\hline \hline Convolution & 64 filters of $5 \times 5$ \\
Max-Pooling & $2 \times 2$ \\
Convolution & 192 filters of $5 \times 5$\\
Max-Pooling & $2 \times 2$ \\
Fully connected & 384 units \\
Fully connected & 192 units \\
Softmax & 10 units \\
\hline
\end{tabular}
    \label{tab:cnn2}
\end{table}



% \begin{table}[h]
%   \caption{Neural network and datasets setup.}
% 	\centering
% 	\footnotesize{
% 	%\resizebox{\columnwidth}{!}{%
% 	\begin{tabular}{cccccc}	
% 	\toprule[1pt]
% 	Dataset & Model  & features & classes & Training size  & Test size\\ 	
% 	\toprule[1pt]
% 		MNIST            & CNN \& MLP & 28$\times$ 28 & 10 &  10,000  & 10,000\\
% Fashion MNIST   & CNN \& MLP  &  28$\times$ 28 & 10 &  10,000  & 10,000\\
% 		\toprule[1pt]
% 	\end{tabular}}
% %	}
% 	\label{tab::network_setup_app}
% \end{table}


\textbf{Experimental setup.}  We are interested in stochastic gradient Langevin dynamics,
whose iterative updates are given by $\w_{t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1}, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right).$ %$\w_{t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1}, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right)$. 
We also denote $\beta_t =2\eta_t/\sigma_t^2$ as the inverse temperature at time t. 
For MNIST and Fashion-MNIST, the initial learning rate is $\eta_0=0.004$ and it decays by 0.96 after every 5 epochs. For CIFAR-10,the initial learning rate is $\eta_0=0.005$ and it decays by 0.995 after every 5 epochs. We use batch size $|B_t| = 100$ for MNIST and Fashion-MNIST, and $|B_t| = 200$ for CIFAR-10. %We also consider SGLD with $\sigma_t=\alpha_t\cdot\eta_t$ can be found in Figure~\ref{fig:mnist_noisysgd} in Appendix \ref{app:exp}. 


Motivated by \cite{zhang2017understanding}, we train CNN with SGLD on a smaller subset of MNIST dataset ($n=10000$) with randomly corrupted labels. The corruption fraction varies from $0\%$ (without label corruption) to $60\%$. For different level of randomness, we use the same training setting with batch size $|B_t|=100$, initial step size $\eta_0 = 0.005$, noise variance $\sigma_t = 0.2 \cdot \eta_t$, and we decay $\eta_t$ by 0.995 for every 30 epochs. 



We are also interested in Noisy Sign-SGD whose iterative updates are given by %$\mathbf{w}_{t}=\mathbf{w}_{t-1}-\eta_{t}\boldsymbol{\xi}_{t}$, where $\boldsymbol{\xi}_{t} \sim \text{Bernoulli} \left(\frac{1}{1+\exp{\left(-\frac{\nabla \ell(w_{t-1},S_{B_{t}})}{\alpha_t}\right)}}\right)$
$\w_{t+1} = \w_{t} - \eta_t \bxi_t$, where $\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(\xi_j)=\frac{\exp(\xi_j \btheta_{B_t,\alpha_t})}{\exp(-\btheta_{B_t,\alpha_t})+\exp(\btheta_{B_t,\alpha_t})}$. The initial learning rate is $\eta_0=10^{-4}$ and it decays by 0.1 after every 30 epochs. We use batch size $|B_t| = 100$ for all benchmarks.




%where $~ \bxi_{t,i} \sim p_{\alpha_t}(\xi) = \frac{1}{\exp((1-\xi)\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)/\alpha_t)+\exp((-1-\xi)\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)/\alpha_t)}~, ~ \xi\in\{-1,+1\}$. 




All experiments minimize cross-entropy loss for a fixed number of epochs and have been run on NVIDIA Tesla K40m GPUs. For CNN, we repeat each experiment 30 times, and for ResNet-18, we repeat 5 times.


\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:sgld_bound} and \ref{fig:sgld_mnist} for MNIST and Fashion-MNIST with CNN}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & MNIST/ Fashion-MNIST \\\hline
Architecture & CNN with 2 conv. layers and 2 linear layers \\\hline
Batch Size & $100$\\\hline
Learning Rate & $\eta_0=4\times10^{-3}$, decay epochs=5, decay rate=0.96 \\\hline
Inverse Temperature& $\beta \in [5000, 55000]$ \\\hline
Number of Epochs & 50\\\hline
No. of training examples & 55000 \\\hline
Number of Repeated Runs & 30 \\
\hline
\end{tabular}
\label{tab:mnist}
\end{table}


\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:sgld_bound} and \ref{fig:sgld_cifar10} for CIFAR-10 with CNN}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & CIFAR-10\\\hline
Architecture & CNN with 2 conv. layers and 3 linear layers \\\hline
Batch Size & $200$\\\hline
Learning Rate & $\eta_0=5\times10^{-3}$, decay epochs=5, decay rate=0.995 \\\hline
Inverse Temperature& $\beta \in [5000, 55000]$ \\\hline
Number of Epochs & 1000\\\hline
No. of training examples & 55000 \\\hline
Number of Repeated Runs & 20 \\
\hline
\end{tabular}
\label{tab:cifar10}
\end{table}



\begin{table}[h]
\caption{Details of Experiments reported in Figure~\ref{fig:bound_random} for MNIST with CNN ($\sigma_t = 0.2 \cdot \eta_t$)}
\centering
\begin{tabular}{c|c} 
\hline
Parameter & Values \\
\hline
Dataset & MNIST\\\hline
Architecture & CNN with 2 conv. layers and 2 linear layers \\\hline
Batch Size & $100$\\\hline
Learning Rate & $\eta_0=5\times10^{-3}$, decay epochs=30, decay rate=0.995 \\\hline
Number of Epochs & 1000\\\hline
No. of training examples & 10000 \\\hline
Number of Repeated Runs & 30 \\
\hline
\end{tabular}
\label{tab:random}
\end{table}





\begin{figure*}[t] 
\centering
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-c.png}
 }
  \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-c.png}
 }
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
\includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-b.png}
 }
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
\includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-b.png}
 }   
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-a.png}
 }
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a.png}
 } 
\caption[]{Numerical results for CNN trained on MNIST using SGLD %($\sigma_t=\sqrt{2\eta_t/\beta_t}$). $\beta=55000$ which is equivalent 
with a small noise variance $\sigma_t\approx 10^{-4}$.
}
\label{fig:sgld_mnist}
\end{figure*}




\begin{figure*}[t] 
\centering
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-c.png}
 }
\subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-c.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-b.png}
 } 
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-b.png}
 }
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$, $\beta_t=55000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-a.png}
 }
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$, $\beta_t=5000$]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a.png}
 } 

%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-5000.0-b.png}
%  } 
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-55000.0-b.png}
%  }
%   \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a.png}
%  } 
%   \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-55000.0-a.png}
%  }
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.1$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-5000.0-a.png}
%  } 
%   \subfigure[CIFAR-100, $\alpha_t^2 \approx 0.01$]{
%  \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar100-bounds-beta-55000.0-a.png}
%  }  
\caption[]{Numerical results for training CNN using SGLD %with $\sigma_t = \sqrt{2\eta_t/\beta_t}$ 
on CIFAR-10. 
}
\label{fig:sgld_cifar10}
\end{figure*}






% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN, MNIST]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/cnn1-mnist-n0-bs100-sign-sgd-train-dynamics.png}
%  } 
%   \subfigure[CNN, Fashion]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/cnn1-fashion-n0-bs100-sign-sgd-train-dynamics.png}
%  }
%  \subfigure[ResNet-18, CIFAR10]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/resnet18-cifar10-n0-bs100-sign-sgd-train-dynamics.png}
%  }
%  \subfigure[ResNet-18, CIFAR100]{
%  \includegraphics[width=0.4\textwidth]{ICLR2022/images/resnet18-cifar100-n0-bs100-sign-sgd-train-dynamics.png}
%  }
% \caption[]{Training dynamics of Noisy sign-SGD with different scaling $\alpha_t$. Legends indicate the choice of  $\alpha_t$ and the numbers in brackets are the test accuracy at convergence. As $\alpha_t\to 0$, Nosiy sign-SGD matches both the optimization trajectory as well as the final test accuracy of original sign-SGD \citep{bernstein2018signsgd}.
% }
% \label{fig:train_noisy_signsgd_full}
% \end{figure*}






% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN, MNIST, Noisy sign-SGD, $\alpha_t = 0.1$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-bernoulli-beta-0.1.png}
%  } 
%  \subfigure[CNN, Fashion, Noisy sign-SGD, $\alpha_t = 0.1$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-bernoulli-beta-0.1.png}
%  }
%  \subfigure[ResNet-18, CIFAR-10, Noisy sign-SGD, $\alpha_t = 0.1$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/resnet18-cifar10-bounds-bernoulli-beta-0.1.png}
%  }
%  \subfigure[ResNet-18, CIFAR-100, Noisy sign-SGD, $\alpha_t = 0.1$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/resnet18-cifar100-bounds-bernoulli-beta-0.1.png}
%  } 
 
% \caption[]{Numerical results for training CNN on MNIST and Fashion-MNIST, and ResNet-18 on Cifar-10 and Cifar-100 using Noisy Sign-SGD.
% }
% \label{fig:bound_noisy_signsgd_full}
% \end{figure*}









\begin{figure*}[th] 
\centering
  \subfigure[CNN, MNIST, Noisy-SGD, $\alpha_t = 0.2$, $\sigma_t\approx 10^{-4}$]{
 \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-beta-0.2.png}
 } 
  \subfigure[CNN, MNIST, Noisy-SGD, $\alpha_t = 0.002$, $\sigma_t\approx 10^{-6}$]{
 \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-beta-0.002.png}
 }
\caption[]{Numerical results for CNN trained on MNIST using Noisy SGD. %where $\sigma_t=\alpha_t\eta_t$. 
We follow the setting described in \cite{Li2020On}. The initial $\eta_t$ is $4\times 10^{-3}$, and decays by 0.95 ($\alpha_t=0.2$) or 0.995 ($\alpha_t=0.002$) for every 5 epochs. 
}
\label{fig:mnist_noisysgd}
\end{figure*}




\begin{figure*}[t] 
\centering
 \subfigure[MNIST, $\alpha_t = 1.0$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
 }
 \subfigure[MNIST, $\alpha_t = 0.1$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-d.png}
 }
 \subfigure[MNIST, $\alpha_t = 0.01$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-e.png}
 }
  \subfigure[MNIST, Our Bound]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-b.png}
 }  
 \subfigure[MNIST, Gradient Discrepancy]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-a.png}
 }
 
 \subfigure[Fashion, $\alpha_t = 1.0$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
 }
 \subfigure[Fashion, $\alpha_t = 0.1$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-d.png}
 }
 \subfigure[Fashion, $\alpha_t = 0.01$]{
 \includegraphics[width=0.3\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-e.png}
 }
  \subfigure[Fashion, Our Bound]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-b.png}
 }  
 \subfigure[Fashion, Gradient Discrepancy]{
 \includegraphics[width=0.4\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-a.png}
 }  
 
\caption[]{Numerical results for training CNN on MNIST and Fashion-MNIST using Noisy Sign-SGD. Increasing $\alpha_t$ leads to a tighter generalization bound even though it leads to a slightly larger gradient discrepancy. 
}
\label{fig:bound_noisy_signsgd}
\end{figure*}





% \clearpage
% \textbf{Experiments on Cifar10 dataset.} We run experiments and compare our bound with the bound in \cite{Li2020On} and \cite{negrea2019information} on Cifar10 dataset. We consider vgg 11 network model with 10,000 training samples randomly sampled from Cifar10 dataset. For training we use initial learning rate 0.001, and noise variance decay such that $\sigma_t = 0.3\eta_t$ and $\sigma_t = 0.5\eta_t$, and we decay $\eta_t$ every 10 epochs with decaying rate 0.93. Figure \ref{fig:cifar10} shows our bound is sharper than existing bound under different noise variance settings.
% \begin{figure*}[h] 
% \centering
% %   \subfigure[MLP, $\sigma_t = 0.1\eta_t$]{
% %  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha01_mnist_fnn.png}
% %  } 
% %   \subfigure[MLP,  $\sigma_t = 0.05\eta_t$]{
% %  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.23\textwidth]{img/lr05alpha05_mnist_fnn.png}
% %  }  
%   \subfigure[$\sigma_t = 0.3 \eta_t$]{
%  \includegraphics[trim =3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_lr0.001_alpha0.3_mo0.0_decay0.93.png}
%  }  
%   \subfigure[$\sigma_t = 0.5 \eta_t$]{
%   % [trim=left bottom right top, clip]
%  \includegraphics[trim = 3mm 1mm 4mm 4mm, clip, width=0.3\textwidth]{Arxiv/img/cifar_lr0.001_alpha0.5_mo0.0_decay0.93.png}
%  }

% \caption[]{Numerical results for cifar10 dataset. Figure (a-b) shows our bound is sharper than existing bound under different settings of noise variance.
% }\label{fig:cifar10}
% \end{figure*}






% \textbf{Random Label Experiments.} Inspired by \cite{zhang2017understanding}, we run SGLD to fit 10,000 samples from MNIST dataset Figure \ref{fig:random_label_mnist} and fashionMNSIT dataset Figure \ref{fig:random_label_fashion_mnist}, with increasing fractions of randomly labeled data, from fractions $0\%$ (normal data) to $60\%$. We consider a MLP network with two hidden layers with 128,128 nodes respectively in each layer. For different level of randomly labeled data, we use the same training setting with batch size $|B_t|=128$, initial step size $\eta_0 = 0.05$, noise variance $\sigma_t = 0.07 \cdot \eta_t$, and we decay $\eta_t$ every 10 epochs by 0.95. As shown in Figure~\ref{fig:random_label_mnist} (a) and \ref{fig:random_label_fashion_mnist} (a), with a fixed running time, the experiment with higher level of randomly labeled data has lower training accuracy. Figure \ref{fig:random_label_mnist} (b) and \ref{fig:random_label_fashion_mnist} (b) show higher level of randomly labeled data has higher generalization error and our bound also increase with higher level of randomness, which matches the behavior of generalization error.



==> arXiv/app/efld.tex <==

%\abcomment{some text}

In this section, we provide the proofs for Section \ref{sec:efld}. We first review and show details of a few examples of exponential family.



\subsection{Examples of Exponential Family}\label{app:example}
\begin{exam}[Gaussian]
For univariate Gaussians with fixed variance $\sigma^2$, the scaling $\alpha = \sigma$, the sufficient statistic $\xi = x/\sigma$, the log-partition function  $\psi(\theta) = \theta^2/2$, and the base measure $\pi_0(\xi) = \frac{1}{\sqrt{2\pi}} \exp(-\xi^2/2)$ or equivalently $\pi_0(x) = \frac{1}{\sqrt{2\pi}\sigma} \exp(-x^2/2\sigma^2)$ using $\xi = x/\sigma$ and $d\xi = dx/\sigma$. The scaled parameter $\theta_{\alpha} = \theta_{\sigma} = \theta/\sigma$. Then, the distribution from the natural parameter form is:
\begin{equation}
    p_{\theta/\sigma}(x) = \exp( x \theta / \sigma^2 - \theta^2/(2\sigma^2) ) \times \frac{1}{\sqrt{2\pi}\sigma} \exp(-x^2/2\sigma^2)
    = \frac{1}{\sqrt{2\pi}\sigma} \exp(-(x-\mu)^2/2\sigma^2)~.
\end{equation}
The expectation parameter $\mu = \nabla \psi(\theta) = \theta$. The scaled expectation parameter $\mu_{\alpha} = \nabla \psi(\theta_\alpha) = \theta_\alpha = \theta/\sigma = \mu/\sigma$. Since $\xi = x/\sigma$ and the Bregman divergence $d_{\phi}(\xi,\mu) = \frac{1}{2}(\xi-\mu)^2$, the expectation parameter form
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(-(x/\sigma - \mu/\sigma )^2/2) \frac{1}{\sqrt{2\pi} \sigma} = \frac{1}{\sqrt{2\pi}\sigma} \exp(-(x-\mu)^2/2\sigma^2)~.\qed
\end{equation}
\end{exam}

\begin{exam}[Bernoulli over $\{0,1\}$]
For Bernoulli over $\{0,1\}$, the sufficient statistic $\xi = x \in \{0,1\}$, base measure is 1 on $\{0,1\}$, and the log-partition function $\psi(\theta) = \log(1+\exp(\theta))$ for natural parameter $\theta \in \R$. The expectation parameter $\mu = \nabla \psi(\theta) = \frac{exp(\theta)}{1+\exp(\theta)} = \frac{1}{1+\exp(-\theta)}$, the sigmoid function of $\theta$. The Bregman divergence is the Bernoulli KL-divergence given by: $d_{\phi}(\xi,\mu) = x \log \frac{x}{\mu} + (1-x) \log \frac{1-x}{1-\mu}$. For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{1}{1+\exp(-\theta_{\alpha})}$. 
The mean parameter form distribution is given by
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha})) = \mu_{\alpha}^{\xi} (1-\mu_{\alpha})^{1-\xi}~.
\end{equation}
\qed
\end{exam}

\begin{exam}[Bernoulli over $\{-1,1\}$]
For Bernoulli over $\{-1,1\}$, the sufficient statistic $\xi = x \in \{-1,1\}$, base measure is 1 on $\{-1,1\}$, and the log-partition function $\psi(\theta) = \log(\exp(-\theta)+\exp(\theta))$ for natural parameter $\theta \in \R$. The expectation parameter $\mu = \nabla \psi(\theta) = \frac{\exp(\theta)- \exp(-\theta)}{\exp(-\theta)+\exp(\theta)} = \frac{\exp(2\theta)-1}{\exp(2\theta)+1}$, then its inverse function $\theta = \nabla \phi(\mu) = \frac{1}{2}\log \left(\frac{1+\mu}{1-\mu}\right)$, by integration we have $\phi(\mu) = \frac{1+\mu}{2}\log\frac{1+\mu}{2}+ \frac{1-\mu}{2}\log\frac{1-\mu}{2}$. The Bregman divergence is given by: $d_{\phi}(\xi,\mu) = \frac{1+\xi}{2} \log \frac{1+\xi}{1+\mu} + \frac{1-\xi}{2} \log \frac{1-\xi}{1-\mu}$. For scaled parameters $\theta_{\alpha} = \theta/\alpha$, the corresponding expectation parameter $\mu_{\alpha} = \frac{\exp(2\theta_\alpha)-1}{\exp(2\theta_\alpha)+1}$. Noting that $\frac{1+\xi}{2} \log \frac{1+\xi}{2} = \frac{1-\xi}{2} \log \frac{1-\xi}{2} = 0$ for the base measure, the distribution is given by
\begin{equation}
p_{\mu_{\alpha}}(\xi) = \exp(- d_{\phi}(\xi,\mu_{\alpha})) = \left(\frac{1+\mu_\alpha}{2}\right)^{\frac{1+\xi}{2}} \left(\frac{1-\mu_\alpha}{2}\right)^{\frac{1-\xi}{2}},
\end{equation}
which is $\xi = 1$ with probability $\frac{1+\mu_\alpha}{2}$ and $\xi = -1$ with probability $\frac{1-\mu_\alpha}{2}$.\qed
% Therefore, the EFLD update reduces to a noisy version of sign-SGD: \begin{equation}\label{eq:signSGD_mini_batch_1}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, ~\bxi_{t,i} \sim p_{\btheta_{B_t,\alpha_t,i}}(\xi) =  \frac{1}{\exp((1-\xi)\btheta_{B_t,\alpha_t,i})+\exp((-1-\xi)\btheta_{B_t,\alpha_t,i})}~, ~ \xi\in\{-1,+1\}
% \end{equation}
% for any $i\in [d]$, where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
\end{exam}

% \begin{exam}[Categorical]
% \abcomment{do we have the details for this? otherwise deop}
% The sufficient statistic $\xi = x = \{-1,0,1\}$, base measure is 1 on $\{-1,0,1\}$, natural parameters $\btheta = [\theta_1~~~\theta_2]^T \in \R^2$, and the log-partition function $\psi(\btheta) = \log(1+\exp(\theta_1) + \exp(-\theta_2))$. The expectation parameter $\mu  = \nabla \psi(\btheta) = [\frac{\exp(\theta_1)}{1+\exp(\theta_1) + \exp(-\theta_2)}, \frac{\exp(-\theta_2)}{1+\exp(\theta_1) + \exp(-\theta_2)}]$ \qed
% \end{exam}











\subsection{Proof of Theorem~\ref{theo:efld}}

\theoefld*

To avoid clutter, we drop the subscript $t$ for the analysis and note that the analysis holds for any step $t$.  When the density $dP_{B,\bxi} = \p_{\psi}(\bxi;\btheta_{B,\alpha})$, by mean-value theorem, for each $\bxi$, we have 
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) 
= \langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ~,
\end{equation}
for some $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$ where $\gamma_{\bxi} \in [0,1]$. Then,
\begin{align}
I_{A,B} &=  \bigintsss_\bxi \frac{\big( p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta_{B',\alpha}) \big)^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber 
= \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber \\
& = \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla_{\tilde{\btheta}_{B',\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2p_{\psi}^2(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi ~,
\label{eq:expcore}
\end{align}
since $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) = \exp(\langle \bxi, \tilde{\btheta}_{B,\alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha})) \pi_0(\bxi)$. 


\subsubsection{Handling Distributional Dependency of $\tilde{\btheta}_B$}
Note that we cannot proceed with the analysis with the density term depending on $\tilde{\btheta}_B$ since $\tilde{\btheta}_B$ depends on $\bxi$. In this step we focus on bounding the density term depending on $\tilde{\btheta}_B$ in terms of exponential family densities with parameters $\btheta_B$ and $\btheta'_B$. 


\exptilde*

\proof Denoting $\gamma_{\bxi}$ as $\gamma$ for convenience (the dependence on $\bxi$ does not play a role in the analysis), we have 
\begin{align*}
\langle \bxi, & \tilde{\btheta}_{B,  \alpha} \rangle  - \psi(\tilde{\btheta}_{B,\alpha}) 
 = \langle \bxi, \gamma \btheta_{B, \alpha} + (1-\gamma) \btheta'_{B,\alpha} \rangle - \psi\left( \gamma \btheta_{B, \alpha} + (1-\gamma) \btheta'_{B, \alpha} \right) \\
& = \gamma \bigg[ \langle \bxi , \btheta_{B,\alpha} \rangle - \psi(\btheta_{B, \alpha}) \bigg]  + (1-\gamma) \bigg[ \langle \bxi , \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \bigg] \\
& ~~~~~~~~~~~~~~~
  + \bigg[ \gamma \psi(\btheta_{B, \alpha} ) + (1-\gamma) \psi(\btheta'_{B,\alpha}) - \psi( \gamma \btheta_{B,\alpha} + (1-\gamma) \btheta'_{B,\alpha} ) \bigg] \\
& \stackrel{(a)}{\leq} \max\bigg( \langle \bxi , \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) , \langle \bxi , \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha} )  \bigg) \\
& ~~~~~~~~~~~~~~~ 
  + \bigg[ \gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha} , \tilde{\btheta}_{B,\alpha}) \bigg]~,
\end{align*}
where the second term in (a) follows since difference between two sides of Jensen's inequality is given by the Bregman information, i.e., expected Bregman divergence to the expectation (See section 3.1.1 in \cite{banerjee2005clustering}):
\begin{align*}
  \gamma \psi(\btheta_{B, \alpha} ) + (1-\gamma) \psi(\btheta'_{B,\alpha}) - \psi( \gamma \btheta_{B,\alpha} + (1-\gamma) \btheta'_{B,\alpha} )  =  \gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha} , \tilde{\btheta}_{B,\alpha})~.
\end{align*}
Now, note that
\begin{align*}
\gamma d_{\psi}(\btheta_{B,\alpha}, \tilde{\btheta}_{B,\alpha})  + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha}, \tilde{\btheta}_{B,\alpha})  
& \leq \gamma d_{\psi}(\btheta_{B,\alpha}, \btheta'_{B,\alpha}) + (1-\gamma) d_{\psi}(\btheta'_{B,\alpha}, \btheta_{B,\alpha}) \\
%& \stackrel{(a)}{=} \gamma d_{\phi}(\m'_{B,\alpha}, \m_{B,\alpha}) + (1-\gamma) d_{\phi}(\m_{B,\alpha},\m'_{B,\alpha})~\\
& \leq \gamma c_2 \| \btheta'_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 + (1-\gamma) c_2 \| \btheta_{B,\alpha} - \btheta'_{B,\alpha} \|_2^2 \\
& \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2~.
\end{align*}
As a result,
\begin{align*}
& \frac{\exp\left[\langle \bxi, \tilde{\btheta}_{B, \alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha}) \right]}{\max\left( \exp\left[\langle \bxi, \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) \right] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right] \right) }\\
& ~~~~~ \leq\exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right]
\frac{ \exp \left[ \max\bigg( \langle \bxi , \btheta_{B, \alpha} \rangle - \psi(\btheta_{B,\alpha}) , \langle \bxi , \btheta'_{B,\alpha} \rangle - \psi(\btheta'_{B,\alpha})  \bigg) \right] }{ \max\left( \exp\left[\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha}) \right] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right] \right) } \\
& ~~~~~ = \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right]~.
\end{align*}
That completes the proof.\qed 







\subsubsection{Bounding the Density Ratio}



Focusing on density ratio, we have

\expdr*

\proof  Note that
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B,\alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A , \alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}  
& = \exp\left[ \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \rangle - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big) \right] \\
& = \beta_{B,A,\alpha} \exp \left[  \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha} \rangle - \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \right]~,
\end{align*}
where
\begin{align*}
\beta_{B,A,\alpha} & = \exp \left[ \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big) \right] ~.
\end{align*}
Note that
\begin{align*}
\log \beta_{B,A,\alpha} & = \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \big( 2\psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \big)\\
& = - \bigg( \psi(\btheta_{B,\alpha}) - \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \bigg) - \bigg( \psi(\btheta_{B,\alpha}) - \psi(\btheta_{A,\alpha}) \bigg) \\
& \stackrel{(a)}{\leq} \bigg\langle \btheta_{B,\alpha} - \btheta_{A,\alpha}, \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \bigg\rangle + \bigg\langle \btheta_{A,\alpha} - \btheta_{B,\alpha}, \nabla \psi( \btheta_{A,\alpha} \bigg\rangle   \\
& = \bigg\langle \btheta_{B,\alpha} - \btheta_{A,\alpha}, \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\btheta_{A,\alpha})  \bigg\rangle  \\
& \stackrel{(b)}{\leq} \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2 \| \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\btheta_{A,\alpha}) \|_2  \\
& \stackrel{(c)}{\leq} c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2 \| (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \btheta_{A,\alpha} \|_2 \\
& = 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2~,
\end{align*}
where (a) follows from the convexity of $\psi$, (b) follows from Cauchy-Schwartz, and (c) follows by smoothness of $\psi$.


As a result, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B,\alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A, \alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}
&\leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_B - \btheta_A)/\alpha \rangle - \psi( (2\btheta_B - \btheta_A)/\alpha) \right]~.
\end{align*}
That completes the proof.\qed

The analysis for the term involving $\btheta'_B$ is exactly the same. 

% \abcomment{state a Lemma by combining Lemma 2 and Lemma 3?}

% \abbcomment{Lemma will help the reader understand that the base measure scales correctly, and essentially stays unchanged}

Combining Lemma~\ref{lemm:exp_step2} and \ref{lemm:exp_step3}, we have the following result:
\begin{restatable}{lemm}{expcompile}
We have
\begin{equation}
\begin{split}
\frac{p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi;\btheta_{A,\alpha})} 
 & \leq \exp\left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right] \\
 & \phantom{...........} 
\times \max\big( \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B,\alpha} - \btheta_{A,\alpha})~,  \big. \\
& \phantom{........................} \left. 
\exp \left[2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B',\alpha} - \btheta_{A,\alpha}) \right)~.
\end{split}
\end{equation}
\label{corr:expcompile}
\end{restatable}
\proof 


From Lemma \ref{lemm:exp_step2}, we have
\begin{align*}
p_{\psi}^2(\boldsymbol{\xi} ; \tilde{\boldsymbol{\theta}}_{B, \alpha}) & = \exp \left[2\left\langle\boldsymbol{\xi}, \tilde{\boldsymbol{\theta}}_{B, \alpha}\right\rangle-2\psi\left(\tilde{\boldsymbol{\theta}}_{B, \alpha}\right)\right] \\
& \leq \exp \left[c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{B^{\prime}, \alpha}\right\|_{2}^{2}\right] \cdot \max \left(\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right], \exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B^{\prime}, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{B^{\prime}, \alpha}\right)\right]\right)
\end{align*}

Thus,

\begin{align*}
\frac{p_{\psi}^{2}\left(\boldsymbol{\xi} ; \tilde{\boldsymbol{\theta}}_{B, \alpha}\right)}{p_{\psi}\left(\boldsymbol{\xi} ; \boldsymbol{\theta}_{A, \alpha}\right)} \leq \exp \left[2 c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{B^{\prime}, \alpha}\right\|_{2}^{2}\right] \cdot  \frac{\max \left(\exp \left[2\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B, \alpha}\right\rangle-2\psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right], \exp \left[2\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{B^{\prime}, \alpha}\right\rangle-2\psi\left(\boldsymbol{\theta}_{B^{\prime}, \alpha}\right)\right]\right)}{\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{A, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{A, \alpha}\right)\right]}
\end{align*}

Based on Lemma \ref{lemm:exp_step3}, we have
\begin{align*}
\frac{\exp \left[\left\langle\boldsymbol{\xi}, 2 \boldsymbol{\theta}_{B, \alpha}\right\rangle-2 \psi\left(\boldsymbol{\theta}_{B, \alpha}\right)\right]}{\exp \left[\left\langle\boldsymbol{\xi}, \boldsymbol{\theta}_{A, \alpha}\right\rangle-\psi\left(\boldsymbol{\theta}_{A, \alpha}\right)\right]} \leq \exp \left[2 c_{2}\left\|\boldsymbol{\theta}_{B, \alpha}-\boldsymbol{\theta}_{A, \alpha}\right\|_{2}^{2}\right] \exp \left[\left\langle\boldsymbol{\xi},\left(2 \boldsymbol{\theta}_{B}-\boldsymbol{\theta}_{A}\right) / \alpha\right\rangle-\psi\left(\left(2 \boldsymbol{\theta}_{B}-\boldsymbol{\theta}_{A}\right) / \alpha\right)\right]
\end{align*}

Combining above inequalities we have
\begin{equation}
\begin{split}
\frac{p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi;\btheta_{A,\alpha})} 
 & \leq \exp\left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \right] \\
 & \phantom{...........} 
\times \max\big( \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B,\alpha} - \btheta_{A,\alpha})~,  \big. \\
& \phantom{........................} \left. 
\exp \left[2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2 \btheta_{B',\alpha} - \btheta_{A,\alpha}) \right)~.
\end{split}
\end{equation}

That completes the proof. \qed


\subsubsection{Bounding the Integral}

Ignoring multiplicative terms which do not depend on $\bxi$ for the moment, the analysis needs to bound an integral term of the form
\begin{equation}
    \bigintsss_\bxi \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2 ~p_{\psi}(\bxi;2 \btheta_{B,\alpha} - \btheta_{A,\alpha}) d\bxi~,
\end{equation}
and a similar term with $p_{\psi}^2(\bxi;2 \btheta_{B',\alpha} - \btheta_{A,\alpha})$. The proof of Theorem~\ref{theo:efld} can be done by suitably bounding the integral.
% \begin{restatable}{lemm}{lemmexpinfo}
% \label{lemm:exp_info}
% Consider Noisy SGD with exponetial family noise such that the log-partition function is  $c_1$-strongly convex and $c_2$-smooth, for a given sample set $\bar S$ and parameters $\w_{t-1}$, let $\Delta_{t}(\bar{S}) \triangleq \max _{z, \bar{z} \in S}\left\|\nabla \ell\left(\w_{t-1}, z\right)-\nabla \ell\left(\w_{t-1}, \tilde{z}\right)\right\|_{2}$, with $\eta_t$ be data-dependent and adaptively chosen such that $\eta_{t}^{2} \Delta_{t}^{2}(\bar{S})/\sigma_t^4 \leq \abedit{c(c_1,c_2)}$, then for any $B_t \in G_1$ and  $A_t \in G_0$,  we have \abcomment{notation and constants need work, result needs to be updated}
% \begin{align}
% I_{A_t, B_t} \leq c_0 c_2^2\frac{\eta_{t}^{2}}{\alpha_t^2} \left[\left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
% \end{align}
% where $c(c_1,c_2) = \frac{c_1^2}{(3c_2-c_1)c_2(1+c_1)}$.
% \end{restatable} 

{\em Proof of Theorem~\ref{theo:efld}.} From Lemma~\ref{corr:expcompile}, we have
\begin{align*}
&I_{A,B}\leq \bigintsss_\bxi \frac{ \left\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi( \tilde{\btheta}_{B,\alpha}) \right\rangle^2 p^2_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})}{ p_{\psi}(\bxi;\btheta_{A,\alpha})} d\bxi\\
&\leq  \exp\left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2\right] \\
& ~~~~~~~~~~~~~~~~~~~~\times \max\left(  \exp \left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \right. ~, \\
& ~~~~~~~~~~~~~~~~~~~~~~~~~~~
\left.   \exp \left[ 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B',\alpha}-\btheta_{A,\alpha}) d\bxi \right)~.
\end{align*}
Focusing on the integral in the first term (the analysis for the second term is essentially the same), we have
\begin{align*}
& \bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 p_{\psi}(\bxi; 2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = \bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \big( \bxi - \E[\bxi] \big) - \left(\nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right) \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& \leq 2\underbrace{\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \E[\bxi] \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi}_{T_1} \\
& \phantom{\leq} + 2 \underbrace{\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha}, \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right\rangle^2 p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi}_{T_2}~.
\end{align*}
For $T_1$, note that 
\begin{align*}
T_1 & = \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \E[\bxi] \right\rangle^2   \right] \\
& = (\btheta_{B,\alpha} -\btheta_{B',\alpha})^T \E_{\bxi \sim p_{\psi}(2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (\bxi - \E[\bxi]) (\bxi - \E[\bxi])^T \right] (\btheta_{B,\alpha} -\btheta_{B',\alpha})~\\
& = (\btheta_{B,\alpha} -\btheta_{B,\alpha})^T \nabla^2 \psi( 2\btheta_{B,\alpha}-\btheta_{A,\alpha})  (\btheta_{B,\alpha} -\btheta_{B',\alpha}) \\
& \leq c_2 \| \btheta_{B,\alpha} -\btheta_{B,\alpha} \|_2^2~,
\end{align*}
since, by smoothness, the spectral norm of $\nabla^2 \psi$ is bounded by $c_2$. 

For $T_2$, first note that 
\begin{align*}
\E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}[\bxi] = \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) ) ~.
\end{align*}
Hence, with $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta_{B',\alpha}$ for some $\gamma_{\bxi} \in [0,1]$, we have
\begin{align*}
T_2 & = \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B,\alpha},  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \E[\bxi] \right\rangle^2   \right] \\    
& = \E_{\bxi \sim p_{\psi}(\bxi; 2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha},  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \nabla \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha})  \right\rangle^2   \right]\\
& \leq  \| \btheta_{B,\alpha} -\btheta_{B,\alpha} \|_2^2 ~~~\E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\|  \nabla \psi(\tilde{\btheta}_{B,\alpha}) - \nabla \psi( (2\btheta_{B,\alpha} - \btheta_{A,\alpha}) \right\|_2^2  \right]\\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ \left\|  \tilde{\btheta}_{B,\alpha} - (2\btheta_{B,\alpha} - \btheta_{A,\alpha} ) \right\|_2^2  \right] \\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})} \left[ \big\| \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta_{B',\alpha} - \btheta_{B,\alpha} - (\btheta_{B,\alpha} - \btheta_{A,\alpha}) \big\|_2^2 \right] \\
& = c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}
\left[ \big\|  (1-\gamma_{\bxi}) (\btheta_{B',\alpha} - \btheta_{B,\alpha}) - (\btheta_{B,\alpha} - \btheta_{A,\alpha}) \big\|_2^2 \right] \\
& \leq  2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ 
\left( \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (1-\gamma_{\bxi})^2  \big\|  \btheta_{B',\alpha} - \btheta_{B,\alpha} \big\|_2^2 \right]
+  \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})} \left[ \big\|  \btheta_{B,\alpha} - \btheta_{A,\alpha} \big\|_2^2 \right]  \right) \\
& = 2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~ 
\left( \big\|  \btheta_{B',\alpha} - \btheta_{B,\alpha} \big\|_2^2 \E_{\bxi \sim p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})}\left[ (1-\gamma_{\bxi})^2   \right]
+   \big\|  \btheta_{B,\alpha} - \btheta_{A,\alpha} \big\|_2^2  \right) \\
& \leq  2c_2^2 \| \btheta_{B,\alpha} -\btheta_{B',\alpha} \|_2^2~~~  \left( \| \btheta_{B,\alpha} -\btheta_{B',\alpha}\|_2^2  + \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right) ~.
\end{align*}
Putting everything back together
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 & p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 ~~\left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
Similarly
\begin{align*}
\bigintsss_\bxi  \left\langle \btheta_{B,\alpha} -\btheta_{B',\alpha}, \bxi - \nabla \psi(\tilde{\btheta}_{B,\alpha}) \right\rangle^2 & p_{\psi}(\bxi;2\btheta_{B',\alpha}-\btheta_{A,\alpha}) d\bxi \\
& = c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 ~~\left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
%Since the bound is the same for both the terms, the $\max$ can be bounded by the right-hand-side.
% \abcomment{please finish the rest, need to check the scaling w.r.t.~$1/\sigma$ once the earlier notation is cleaned up}


Then, plugging into bound on $I_{A,B}$, we have
\begin{align*}
I_{A,B} & \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times 
\exp\left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2\right] \\
& ~~~~~ \times \max\big(  \exp \left[ 2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right) \big. ~,\\
& ~~~~~~~~~~~~  \exp \left[ 2 c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2 \right] 
 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \right) \big)~.
%\exp\bigg[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \max\left(  \| \btheta_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 , \| \btheta_{B,\alpha} - \btheta_{B,\alpha} \|_2^2 \right)  \bigg] \\
%& ~~~~~~~~~~ \times c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times \left( 1 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 + 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \right)~.
\end{align*}
Since $\alpha^2 \geq 8 c_2 \Delta^2(S_{n+1})$ where $\Delta(S_{n+1}) = \max_{z,z' \in S_{n+1}} \| \nabla \ell (\w,z) - \nabla \ell (\w,z') \|_2$, recalling that $\btheta_{B,\alpha} = \nabla \ell(\w,B)/\alpha$, we have 
\begin{align*}
2 c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 & \leq \frac{1}{4}~, ~~~
2 c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2  \leq \frac{1}{4} ~, ~~~
2 c_2 \| \btheta_{B',\alpha} - \btheta_{A,\alpha} \|_2^2  \leq \frac{1}{4} ~.
\end{align*}
As a result, we have 
\begin{align*}
I_{A,B} & \leq c_2 \| \btheta_{B,\alpha} - \btheta_{B',\alpha} \|_2^2 \times \exp\left( \frac{1}{4}\right) \times \exp\left(\frac{1}{4}\right) \times \left( 1 +\frac{1}{4} + \frac{1}{4} \right) \\
& \leq \frac{5c_2}{2 \alpha^2} \| \nabla \ell(\w,S_B) - \nabla \ell(\w,S'_B) \|_2^2~.
\end{align*}
That completes the proof. \qed

% \subsection{Coordinate-wise Scaling $\aalpha$}
% We use bold letter $\aalpha$ to denote the vector $[\alpha_1,\cdots,\alpha_p]^T$ representing different scaling for different coordinates.
% \begin{theo}
%     xxx
% \end{theo}




\subsection{Expected Stability of EFLD}

\theoefldstab*

\proof 
% \abcomment{add a proof -- just use Theorem~\ref{theo:efld} in Lemma~\ref{theo:stab}} 
% \yzcomment{added a proof here}

Based on Lemma \ref{theo:stab}, we have
\begin{equation}
\hspace*{-5mm}
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq c_1 \frac{b}{n} \E_{S} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \underset{B_t \in G_1}{\E} \underset{A_t \in G_0}{\E} \left[ I_{A_t, B_t} \right] }~.
\end{equation}
with $I_{A_t, B_t} = \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t$. 

From Theorem \ref{theo:efld}, we have 
\begin{align*}
I_{A_{t}, B_{t}} & \leq \frac{5 c_{2}}{2 \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\|\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}\right)-\nabla \ell\left(\mathbf{w}_{t-1}, S_{B_{t}}^{\prime}\right)\right\|_{2}^{2}\right] \\
& =\frac{5 c_{2}}{2  \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\| \frac{1}{b}  \sum_{z\in S'_{B_t}}\nabla \ell\left(\mathbf{w}_{t-1}, z \right)- \frac{1}{b}  \sum_{z\in S_{B_t}} \nabla \ell\left(\mathbf{w}_{t-1}, z \right)\right\|_{2}^{2}\right]  \\
& =\frac{5 c_{2}}{2 b \alpha_{t \mid \mathbf{w}_{t-1}}^{2}}\left[\left\| \nabla \ell\left(\mathbf{w}_{t-1}, z_n \right)-\nabla \ell\left(\mathbf{w}_{t-1}, z_n^\prime \right)\right\|_{2}^{2}\right]~,
\end{align*}
where the last equation holds because $S_{B_t}$ and $S'_{B_t}$ only differ at $z_n$ and $z_n^\prime$. 

Combining the above two inequalities, we have
\begin{align*}
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq c_1 \frac{b}{n} \E_{S} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \left[\left\| \nabla \ell\left(\mathbf{w}_{t-1}, z_n \right)-\nabla \ell\left(\mathbf{w}_{t-1}, z_n^\prime \right)\right\|_{2}^{2}\right] }~.
\end{align*}
That completes the proof. 
\qed


==> arXiv/app/exp_stability.tex <==
\prophell*
\proof Let $S_n=\left(z_{1}, \ldots, z_{n}\right)$ and $\tilde S^{\prime}_n=\left(z_{1}^{\prime}, \ldots, z_{n}^{\prime}\right)$ two independent random samples and let $S^{(i)}_n=\left(z_{1}, \ldots, z_{i-1}, z_{i}^{\prime}, z_{i+1}, \ldots, z_{n}\right)$ be the sample that is identical to $S$ except in the $i$-th example where we replace $z_{i}$ with $z_{i}^{\prime}$. Note that $S^{(n)}=S'_n$ where $S'_n$ is the dataset obtained by replacing $z_n \in S_n$ with $z'_n$ as in the Proposition statement. Now, by definition we have
\begin{align*}
& \left| \E_{S_n \sim D^n}[L_D(A(S_n)) - L_S(A(S_n))]\right| \\
&= \left|\mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \mathbb{E}_{A} \left[\frac{1}{n} \sum_{i=1}^{n}\left(\ell(A(S_n^{(i)}), z_{i}^{\prime})-\ell(A(S_n), z_{i}^{\prime}) \right)\right] \right| \\
& = \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime}  \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_{A} \left[ \ell(A(S_n^{(i)}), z_{i}^{\prime})-\ell(A(S_n), z_{i}^{\prime}) \right]\right|\\
& \overset{(a)}{=} \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n} \left(\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p^{(i)}(\mathbf{w}) d \mathbf{w}-\int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) p(\mathbf{w}) d \mathbf{w} \right) \right|\\
& = \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime) \left( p^{(i)}(\mathbf{w}) - p(\mathbf{w}) \right)d \mathbf{w} \right| \\
& = \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n} \int_{\mathbb{R}^{d}} \ell(\mathbf{w} ; z_i^\prime)\left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)  d \mathbf{w} \right| \\
& \overset{(b)}{\leq} \left| \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n} \left\{\left(\int_{\mathbb{R}^{d}} \ell^2(\mathbf{w} ; z_i^\prime) \left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\} \right|
\end{align*}
where in (a) $p^{(i)}(\w), p(\w)$ are respectively the distributions obtained by $A(S_n^{(i)}),A(S_n)$, and (b) 
follows by Cauchy-Schwartz inequality. Focusing on the first integral, we have: 


\yzcomment{We do need $\mathbb{E}_{W \sim A\left(S_{n}\right)}\left[\ell^{2}(W, z)\right] \leq c_{0} / 2$, \textbf{for all} $\forall S_{n} \sim D^{n}, \forall z \in \mathcal{Z} $, it is hard to relax the condition to  $\mathbb{E}_{S_n}\mathbb{E}_{W \sim A\left(S_{n}\right)}\left[\ell^{2}(W, z)\right] \leq c_{0} / 2$. Because:
\begin{align*}
    & \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \frac{1}{n} \sum_{i=1}^{n} \left\{\left(\int_{\mathbb{R}^{d}} \ell^2(\mathbf{w} ; z_i^\prime) \left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\}
    \\
& = \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} \left\{\left(\int_{\mathbb{R}^{d}} \ell^2(\mathbf{w} ; z_i^\prime) \left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)^{\frac{1}{2}}\right\} \\
& = \frac{1}{n} \sum_{i=1}^{n} \mathbb{E}_S \mathbb{E}_{\tilde S^\prime} [ U_{+}(S, \tilde S^\prime)^{\frac{1}{2}} ~ U_{-}(S, \tilde S^\prime)^{\frac{1}{2}} ]~,
\end{align*} 
where 
\begin{align*}
    U_{+}(S, \tilde S^\prime) = \left(\int_{\mathbb{R}^{d}} \ell^2(\mathbf{w} ; z_i^\prime) \left(\sqrt{p^{(i)}(\mathbf{w})}+\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)
\end{align*}
and
\begin{align*}
     U_{-}(S, \tilde S^\prime) = \left(\int_{\mathbb{R}^{d}}\left(\sqrt{p^{(i)}(\mathbf{w})}-\sqrt{p(\mathbf{w})}\right)^{2} d \mathbf{w}\right)~.
\end{align*}
We need the expectation $\mathbb{E}_S \mathbb{E}_{\tilde S^\prime}$ to go with $ U_{-}(S, \tilde S^\prime)^{\frac{1}{2}}$ so that we have the expected Hellinger  divergence:  $\mathbb{E}_S \mathbb{E}_{\tilde S^\prime} U_{-}(S, \tilde S^\prime)^{\frac{1}{2}} = \E_{S \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S), A(S'_{n})\big)}$. Thus, we need to uniformly bound $U_{+}(S, \tilde S^\prime)^{\frac{1}{2}}$.
}






\begin{align*}
\left(\int_{\mathbb{R}^{d}} \ell^2(\w ; z_i^\prime) \left(\sqrt{p^{(i)}(\w)}+\sqrt{p(\w)}\right)^{2} d \w \right)^{1/2} 
& \leq \left(2 \int_{\mathbb{R}^{d}} \ell^2(\w ; z_i^\prime) p^{(i)}(\w) d\w +  2 \int_{\mathbb{R}^{d}} \ell^2(\w ; z_i^\prime) p(\w) d \w \right)^{1/2} \\
& \leq \left( c_0^2/2 + c_0^2/2 \right)^{1/2} =c_0 ~.
\end{align*}

Hence, by definition of the Hellinger divergence, we have 
\begin{align*}
\E_{S_n \sim D^n}[L_D(A(S_n)) - L_S(A(S_n))]
& \leq   \mathbb{E}_{S_n} \mathbb{E}_{\tilde {S_n}^\prime} \frac{1}{n} \sum_{i=1}^{n}c_0 \sqrt{2H^{2}\left(A(S_n), A(S_n^{(i)})\right)}\\
& \overset{(a)}{=}   \mathbb{E}_{S_n} \mathbb{E}_{\tilde S_n^\prime} \frac{1}{n} \sum_{i=1}^{n}c_0 \sqrt{2H^{2}\left(A(S_n), A(S'_n)\right)}\\
& = c_0 \E_{S_n \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S_n), A(S'_{n})\big)}~,
\end{align*}
\abedit{where (a) follows since the samples are drawn i.i.d.~and the randomized algorithm $A(\cdot)$ is permutation invariant.}
That completes the proof. \qed 

% (b): need to double check if we can apply the previous argument that ``for any $z$, the loss $\ell(\w;z)$ has bounded expectation and variance'' because there are dependence between $\ell(\w; z_i^\prime)$ and $p^{(i)}(\w)$. The worst case, we bound it by uniform upper bound $C$ on the loss. (c) is true because $z_i^\prime$ for $i =1,...,n$ are i.i.d., so that we can write it as $z^{\prime}$.
% $p^{\prime}(\mathbf{w})$ is the distribution obtained by $A(S^\prime)$, where $S^\prime$ is the dataset differing on only single sample $z^{\prime}$ with $S$.  

% \abcomment{(a) For the analysis, lets use $| \cdots |$ throughout, (b) pls clean up the $\mu^2 + \sigma^2$ analysis, and use a constant. This part needs work}

% \abcomment{For the last part, change to:}
% \begin{align*}
% & \overset{(b)}{\leq} 2c_0  \mathbb{E}_S \mathbb{E}_{S^\prime} \left[ \frac{1}{n} \sum_{i=1}^{n}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)} \right] \\
% & = 2c_0 \mathbb{E}_S \mathbb{E}_{S'} \mathbb{E}_{z_i^\prime \sim S'}  \sqrt{D_{H}^{2}\left(p^{(i)}(\mathbf{w}), p(\w)\right)}\\
% & \overset{(c)}{=} 2c_0 \mathbb{E}_S \mathbb{E}_{z^{\prime}} \sqrt{D_{H}^{2}\left(p^{\prime}(\mathbf{w}), p(\w)\right)}~.
% \end{align*}


\prophellkl*
\proof For the first part, note that:
\begin{align*}
KL(P ,P') & = \int \left(\log \frac{p(\w)}{p'(\w)} \right) p(\w) ~d\w \\
& =  2 \int  \left( - \log \sqrt{\frac{p'(\w)}{p(\w)}} \right) p(\w)~ d\w \\
& \overset{(a)}{\geq} 2 \int \left( 1 - \sqrt{\frac{p'(\w)}{p(\w)}} \right) p(\w)~ d\w \\ 
& = 2 \int \left( p(\w) - \sqrt{p(\w) p'(\w)}) \right) ~d\w \\
& = \int \left(p(\w) + p'(\w) - 2 \sqrt{p(\w)p'(\w)} \right) ~d\w \\
& = \int \left(\sqrt{p(\w)} - \sqrt{p'(\w)}\right)^2~ d\w\\
& = 2 H^2(P,P')~,
\end{align*}
where (a) follows since for $z > -1$, $\log (1+z) \leq z$, using $x = 1+z$ and changing signs gives $-\log x \geq 1-x$.

For the second part, note that:
\begin{align*}
2H^2(P,P') & =  \int_\w ( \sqrt{p(\w)} - \sqrt{p'(\w)} )^2 d\w \\
& =  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| \times | \sqrt{p(\w)} - \sqrt{p'(\w)}| ~d\w \\
& \leq  \int_\w | \sqrt{p(\w)} - \sqrt{p'(\w)}| \times | \sqrt{p(\w)} + \sqrt{p'(\w)}|~ d\w \\
& =  \int_\w | p(\w) - p'(\w)|~ d\w \\
& =  TV(P,P')~,
\end{align*}
where $TV(P,P')$ denotes the total variation distance \citep{pollard2002user}. Further, from Pinsker's inequality \citep{tsybakov2008introduction}, we have
\begin{align*}
TV(P,P') \leq \sqrt{\frac{1}{2} KL(P,P')}~.
\end{align*}
Combining the two results completes the proof. \qed 


% \subsection{Proofs for Section 2.2}

% \mixmodel*
% \proof The proof follows the argument in the proof of Lemma 21 in \cite{Li2020On}.\qed

\subsection{Proofs for Section \ref{sec: exp_stab_nsi}}

Our first result establishes a bound on the KL-divergence between two component mixture models in terms of the mixing weight of the unique components. Similar results have appeared in \citep{Li2020On, bun2018composable} in related contexts. Our proof is different, simple, and self-contained.
\begin{lemm}\label{lemm:mix_bound}
Let $Q,Q',R$ be any three distributions such that $Q,Q'$ are both absolutely continuous w.r.t.~$R$. Then, for any $s \in (0,1)$
\begin{equation}
KL\left(sQ+(1-s)R ~\big\| ~sQ' + (1-s)R \right) \leq 
\frac{s^2}{1-s}~\int_{\w} \frac{(Q(\w) - Q'(\w))^2}{R(\w)} d\w~ .
%\frac{s^2}{1-s} \lsd( Q - Q', R)~.
\end{equation}
\end{lemm}

\proof Let $U=sQ' + (1-s)R$. Then, with $F(x) = Q(x)-Q'(x)$, we have
\begin{align*}
     KL(sQ+(1-s)R \| sQ' + (1-s)R) & =  KL(U + s(Q - Q')  \| U ) \\
     & = \int (U(x) + sF(x)) \log \left( \frac{U(x) + s F(x)}{U(x)} \right) dx \\
     & = \int (U(x) + sF(x)) \log \left( 1 + \frac{s F(x)}{U(x)} \right) dx \\
     & = \int sF(x) + \frac{s^2 F^2(x)}{2U(x)} -  \frac{s^3 F^3(x)}{6U^2(x)} + \frac{s^4 F^4(x)}{12U^3(x)}  -\cdots dx \\
     & = s^2 \int \frac{F^2(x)}{U(x)}\left(  \frac{1}{2} -  \frac{s F(x)}{6U(x)} + \frac{s^2 F^2(x)}{12U^2(x)} - \cdots \right) dx~,
%     & = \int U(x) \left( \left(1+ \frac{sF(x)}{U(x)} \right) \log \left(1 + \frac{sF(x)}{U(x)} \right) - \frac{sF(x)}{U(x)} \right) dx
\end{align*}
where the first term vanishes since $\int F(x) dx = \int (Q(x) - Q'(x)) dx = 0$. This is the reason the dependency is on $s^2$, not $s$. With $W(x) = s F(x)/U(x)$, noting that $W(x) > -1$, and 
\begin{equation}
    \left( \frac{1}{2} - \frac{W(x)}{6} + \frac{W^2(x)}{12} - \cdots \right) = \frac{(1+W(x))\log(1+W(x)) - W(x)}{W^2(x)} \leq 1~,
\end{equation}
we have
\begin{align*}
   KL(sP+(1-s)R \| sQ + (1-s)R) 
     & = s^2 \int \frac{F^2(x)}{U(x)} \left( \frac{ (1+W(x)) \log (1+W(x)) - W(x)}{W^2(x)} \right) dx \\
     & \leq s^2 \int \frac{F^2(x)}{U(x)} dx~ \\
     & \leq \frac{s^2}{(1-s)} \int \frac{(Q(x) - Q'(x))^2}{R(x)} dx~.
\end{align*}
That completes the proof. \qed


\begin{restatable}{prop}{mixmodel}
Consider the mixture models 
%\begin{align*}
$Q_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P_{B_t,\bxi_t}$,  $Q'_{t|} = \frac{1}{|G_1|} \sum_{B_t \in G_1} P'_{B_t,\bxi_t}$, $R_t = \frac{1}{|G_0|} \sum_{A_t \in G_0} P_{A_t,\bxi_t}$.  
%\end{align*}
Then, with 
%\begin{equation*}
$s = \frac{|G_1|}{|G|} = \frac{\binom{n-1}{b-1}}{\binom{n}{b}} = \frac{b}{n}$,
%\end{equation*}
we have 
\begin{align*}
    P_{t|} = s Q_{t|} + (1-s) R_{t|}~, \qquad \text{and} \qquad P'_{t|} = s Q'_{t|} + (1-s) R_{t|}~.
\end{align*}
\label{prop:mixmodel}
\vspace*{-6mm}
\end{restatable}
\proof The proof follows the argument in the proof of Lemma 21 in \cite{Li2020On}.\qed



\begin{lemm}
Consider a general noisy stochastic iterative algorithm with updates of the form~\eqref{eq:nmia} with mini-batch size $B_t = b$. Then, conditioned on any trajectory $\w_{0:t-1}$, we have
\begin{align}
KL\left(P_{t|} \| P_{t|} \right) \leq  \frac{b^2}{n^2} \frac{n}{n-b} \E_{B_t \in G_1} \E_{A_t \in G_0} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t \right]~.
\end{align}
\label{lemm:lsd}
\vspace*{-6mm}
\end{lemm}

\proof By definition, Proposition \ref{prop:mixmodel}, and Lemma~\ref{lemm:mix_bound} with $s=b/n$, we have 
\begin{align*}
KL\left(P_{t|} \| P'_{t|}\right) & \stackrel{(a)}{\leq} \left(\frac{b}{n} \right)^2 \left(\frac{n}{n-b}\right) \int_{\w} \frac{(Q - Q')^2}{R} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \bigintsss_{\w} \frac{ \left(  \frac{1}{|G_1|} \left[ \sum_{B \in G_1} dP_{B,\bxi}(\w) -  \sum_{B \in G_1} P'_{B,\bxi}(\w) \right] \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} dP_{A,\bxi}(\w)} d\w \\
 & \stackrel{(b)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}\sum_{B \in G_1}  \frac{ \left(  dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2 }{\frac{1}{|G_0|} \sum_{A \in G_0} dP_{A,\bxi}(\w)} d\w \\
 & \stackrel{(c)}{\leq} \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right)  \bigintsss_{\w} \frac{1}{|G_1|}  \sum_{B \in G_1} \left\{ \left(  dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2  \frac{1}{|G_0|}\sum_{A \in G_0} \frac{ 1 }{ dP_{A,\bxi}(\w)} \right\} d\w \\
 & = \frac{b^2}{n^2} \left(1 + \frac{b}{n-b}\right) \frac{1}{|G_1| |G_0|}  \sum_{B \in G_1} \sum_{A \in G_0}  \bigintsss_{\w} \frac{ \left( dP_{B,\bxi}(\w) -   P'_{B,\bxi}(\w) \right)^2 }{ dP_{A,\bxi}(\w)} d\w ~,
\end{align*}
% \yzcomment{In order to make sure (b) holdes, we do need $B = B^\prime$, which should be  defined as mini-batches of indexes. }
where (a) is from Lemma \ref{lemm:mix_bound}, (b)(c) is from Jensen's inequality since function $f(x) = x^2$ is convex and $f(x)=\frac{1}{x}$ is convex on $(0,\infty)$. That completes the proof. \qed

Now we have all the pieces to prove the following result:

\theostab*

\proof  Based on Propositions \ref{prop:hell} and \ref{prop:hellkl}, and \eqref{eq:klchain}, we have
\begin{align*}
\E_{S \sim D^n}[L_D(A(S)) - L_S(A(S))]
& \leq  \sqrt{K L\left(P_{T} \| P_{T}^{\prime}\right)} \leq \sqrt{ \sum_{t=1}^{T} \E_{P_{0:(t-1)}}\left[KL\left(P_{t \mid} \| P_{t \mid}^{\prime}\right)\right]} 
\end{align*}
Applying Lemma \ref{lemm:lsd} to bound $KL\left(P_{t \mid} \| P_{t \mid}^{\prime}\right)$ and noting that $b/(n-b) \leq 1$ for $b \leq n/2$ completes the proof. \qed


\subsection{High Probability Generalization Bounds}


%\subsection{High Probability Bounds}

%\yzcomment{strongly suggest moving this section to the appendix}

%\abbcomment{This subsection can be moved to the appendix}

Let $S \sim D^n$ with $S=(Z_1\ldots,Z_n)$ corresponding to the training data. Consider the random variable $Y(S)$, the Scaled (by $n$) Generalization Error (SGE), defined as
\begin{align}
Y(S) \triangleq \sum_{i=1}^n \E_A \big[  \E_{Z \sim D} [\ell(A(S),Z) ] - \ell(A(S),Z_i) \big] = n\big(L_D(A(S)) - L_S(A(S))\big) ~.
\end{align}
%where $A(S)$ is the distribution over $\cW$ due to randomized algorithm $A$ run on $S$.
Theorem~\ref{theo:stab} establishes a bound on $|\frac{1}{n}\E_S[Y(S)]|$. We now focus on establishing a high probability bound on $\frac{1}{n}(Y(S)-\E_S[Y(S)])$. Let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. Further, let $S'_i = (Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)$. Then, the change in SGE
\begin{equation}
Y(S) - Y(S'_i) = n \big[ \big( L_D(A(S)) - L_D(A(S'_i)) \big) - \big( L_S(A(S)) - L_{S'_i}(A(S'_i) \big) \big]    
\end{equation}
is a symmetric random variable, and is identically distributed for $i=1,\ldots,n$.
% \begin{align}
% Y(S) - Y(S'_i) = \sum_{j=1}^n \E_A \big[ \ell(A(S'_i),Z_j) - \ell(A(S),Z_j) \big] = n \big(L_{S'_i}(A(S'_i) - L_S(A(S)) \big)
% \end{align}
%Note that $(Y-Y'_i)$ \abedit{is symmetric} and are identically distributed for any $i$. 
Our analysis is based on the following assumption: %\abcomment{cite for $\psi_2$ norm} 
\begin{asmp}
The random variable $(Y(S)-Y(S'_i))^2$ is sub-Gaussian with $\psi_2$-norm $\kappa_A^2$, i.e., $\| (Y-Y'_i)^2 \|_{\psi_2} = \sup_{q \geq 1} (\E_{S.S'}|Y(S)-Y(S'_i)|^{2q})^{1/q}/\sqrt{q} = \kappa_A^2$. 
%has bounded second moment, i.e., $\E_{S,Z'_i}[(Y(S)-Y(S'_i))^2] \leq \nu_A$, for some constant $\nu_A$.\abcomment{should this be a definition? i.e., just call the second moment $\nu_A$?}
\label{asmp:2moment}
\end{asmp}
Assumption~\ref{asmp:2moment} implies that $\|Y-Y'_i\|_{\psi_2} \leq \kappa_A$.
Note that since $Y(S) - Y(S'_i)$ is identically distributed for all $i$, $\kappa_A$ is the same for all $i$. Further, $\kappa_A$ is a property of the algorithm $A$, and can be viewed as a measure of stability.
If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered stable; on the other hand, if $\kappa_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as typical generalization error $\frac{1}{n}Y(S)$ itself. The sharpness of the high-probability bound we present meaningfully depends on $\kappa_A$, with smaller values implying sharper bounds.



\begin{restatable}{theo}{theohighp}
Under Assumption~\ref{asmp:2moment}, with probability at least $(1-\delta)$ over the draw $S \sim D^n$, we have
\begin{equation}
L_D(A(S)) \leq L_S(A(S)) + \E_S\bigg[L_D(A(S) - L_S(A(S))\bigg] + \max\left( \frac{1}{n}, \frac{ c_1 \kappa_A}{\sqrt{n}} \right) \log \left(\frac{16}{\delta} \right)~.      
\end{equation}
\label{theo:hp}
\vspace*{-5mm}
\end{restatable}







If $\kappa_A=O(1)$, i.e., swapping one point effectively leads to $O(\frac{1}{n})$ change in the generalization error, then $A$ can be considered very stable; if $\kappa_A=O(\sqrt[4]{n})$, then $A$ can be considered somewhat stable; and if $\kappa^2_A = O(\sqrt{n})$, then $A$ is not stable since the effective change in generalization error $\frac{1}{n}(Y(S)-Y(S'_i))$ is $O(1/\sqrt{n})$, the same order as the generalization error $\frac{1}{n}Y(S)$ itself. 

%\theohighp*

%
%
\proof Let $S=(Z_1,\ldots,Z_n)$ and let $S' = (Z'_1,\ldots,Z'_n)$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% % Let
% % \begin{align}
% % Y & = f(Z_1,\ldots,Z_n) \\
% % Y'_i & = f(Z_1,\ldots,Z_{i-1},Z'_i,Z_{i+1},\ldots,Z_n)~,~i=1,2,\ldots,n~.
% % \end{align}
With $(x)_+ = max(x,0)$, let
\begin{align}
    V^+ = V^+(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_+^2 ]~,
\end{align}
% % Let
% With $(x)_- = min(x,0)$, let
% \begin{align}
%     V^- = V^-(S) = \sum_{i=1}^n \E_{S'}[ (Y - Y'_i)_-^2 ]~,
% \end{align}

Our proof uses the following exponential version of the Efron-Stein inequality [Theorem 6.16 in \cite{boucheron2013concentration}], whose proof is based on a combination of the symmetric modified log-Sobolev inequality [Theorem 6.15 in \cite{boucheron2013concentration}] with the change of measure:
\begin{theo}\label{theo:exp_efst}
Let $Y = f(Z_1,\ldots,Z_n)$, where $Z_i,i=1,\ldots,n$ are independent. Let $\theta,\lambda > 0$ be such that $\theta \lambda < 1$ and $\E[\exp(\lambda V^+/\theta)] < \infty$. Then,
\begin{equation}
\log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \log \E\left[ e^{\lambda V^+/\theta} \right]~.
\end{equation}
\end{theo}

% \begin{lemm}
% Let $Z_1,\ldots,Z_n$ be a set of i.i.d.~random variables, and $Z'_1,\ldots,Z'_n$ be such that $Z'_i$ is an independent copy of $Z_i$. 
% Let $Y = f(Z_1,\ldots,Z_n)$ be sub-Gaussian, and let $Y'_i = f(Z_1,\ldots,Z_{i=1},Z'_i,Z_{i+1},\ldots,Z_n)$ such that $(Y-Y'_i)$ is bounded and $\| Y-Y'_i\|_{\psi_2} = \kappa_A$. Then, with $(x)_+ = \max(0,x)$,
% \begin{equation}
% V^+_i = \E_{Z'_i}\left[ (Y - Y'_i)_+^2 \right]~,
% \end{equation}
% is sub-Gaussian and $\| V_i^+ \|_{\psi_2} \leq 4\kappa_A^2$. \abcomment{should follow by definition, by bounding $L_p$ norms, since $Y-Y'_i$ is bounded.}
% \end{lemm}


For the proof of Theorem~\ref{theo:hp}, note that $V^+$ is sub-Gaussian with $\| V^+ \|_{\psi_2} \leq n \kappa_A^2$.
Let $\mu_+ = \E[V^+]$ and $\kappa_+ = \| V^+\|_{\psi_2}$. Then from Theorem \ref{theo:exp_efst}, we have
\begin{align*}
\psi(\lambda) \triangleq \log \E \left[ e^{\lambda(Y - \E Y)} \right] \leq \frac{\lambda \theta}{1 - \lambda \theta} \left[ \frac{\lambda \mu_+}{\theta} + c \frac{\lambda^2 \kappa_+^2}{\theta^2} \right].
\end{align*}
Then, by Markov's inequality we have
\begin{align*}
\log \P( Y - \E Y > t ) & \leq \psi(\lambda) -\lambda t \\
 & \leq \frac{1}{1-\lambda \theta} \left[ \lambda^2 \mu_+ + c\lambda^3 \kappa_+^2/\theta - (1-\lambda \theta) \lambda t \right]~.
\end{align*}
Choosing $\theta = 1/(2\lambda)$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) 
& \leq 2 \lambda^2 \mu_+ + 4c \lambda^4 \kappa_+^2 - \lambda t~.
\end{align*}
Consider choosing $\lambda = \min \left\{ 1, \frac{1}{c_0\sqrt{2\kappa_+}} \right\}$, where $c_0 = \max(1,\sqrt[4]{c})$. Since $\mu_+ \leq \kappa_+$, we have 
\begin{align*}
\log \P( Y - \E Y > t ) & \leq 2 - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \\
\Rightarrow \quad \P( Y - \E Y > t ) & \leq 8 \exp \left( - \min \left\{1, \frac{1}{c_0 \sqrt{2\kappa_+}} \right\} t \right)~.
\end{align*}
With $t = n\epsilon$, and noting that $\kappa_+ \leq n \kappa_A^2$, with $c_1 = c_0 \sqrt{2}$, we have
\begin{align*}
\P\left( Y - \E Y >  n \epsilon \right) & \leq 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right) ~.
\end{align*}
Now, we choose $\delta$ such that
\begin{align*}
 8 \exp \left( - \min \left\{ n, \frac{\sqrt{n}}{c_1\kappa_A} \right\} \epsilon \right)   
 \leq 8 \exp \left( - n \epsilon \right)  + 8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta~.
\end{align*}
It suffices to choose $\epsilon$ such that
\begin{align*}
8 \exp \left( - n \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{1}{n} \log \left( \frac{16}{\delta} \right) \\
8 \exp \left( - \frac{\sqrt{n}}{c_1\kappa_A} \epsilon \right) \leq \delta/2 & \qquad \Rightarrow \qquad \epsilon \geq \frac{c_1 \kappa_A}{\sqrt{n}} \log \left( \frac{16}{\delta} \right)~.
\end{align*}
As a result,
\begin{align*}
\P\left( \frac{1}{n}(Y - \E Y) >  \max \left( \frac{1}{n}, \frac{c_1 \kappa_A}{\sqrt{n}} \right) \log \left( \frac{16}{\delta} \right) \right) & \leq \delta~.
\end{align*}
That completes the proof. \qed





==> arXiv/app/guss.tex <==
\lemmaiabguss*


\proof Recall that we want to bound

\begin{align}
 \nr I_{A_t, B_t} \triangleq \int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t},~~\text{where} ~~ \bxi_t \sim \cN(0, \sigma_t^2\mathbb{I}_d) ~. 
\end{align}

For Noisy SGD with Gaussian noise, we have $P_{B_t,\bxi_t},P'_{B_t,\bxi_t}$ to be two Gaussian distributions with variance $\sigma_t^2\mathbb{I}_d$, and with mean $\m_{B_t}$ and $\m^\prime_{B_t}$ respectively to be
\begin{align*}
    \m_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{B_t}) \\
    \m'_{B_t} & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_{B_t}) ~.
\end{align*}

Similarly, $P_{A_t,\bxi_t}$ is also a Gaussian noise with mean 
$\m_{A_t}  = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_{A_t})$. 
Thus, for any $B_t$ and $A_t$, since $P_{B_{t}, \boldsymbol{\xi}_{t}}$, $P^\prime_{B_{t}, \boldsymbol{\xi}_{t}}$ and $P_{A_{t}, \boldsymbol{\xi}_{t}}$ are Gaussian distributions, $d P_{B_{t}, \boldsymbol{\xi}_{t}}$, $d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}$ and $d P_{A_{t},\boldsymbol{\xi}_{t}}$ are distribution density functions of Gaussian distribution. Then, it is straightforward to have 
\begin{align}
\nr I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{d}} \int_{\w} \frac{\left(\exp \left(-\left\|\w-\m_{B_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\w-\m_{B}^{\prime}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w-\m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \w~.
\end{align}
Note that the above calculation considers integral over $d$-dimensional space which introduced an undesired dimension dependence. However, isotropic Gaussian noise is spherical symmetric, we can translate and rotate the coordinate system so that 
$\m_{A_t}=0$  and $ \m_{B_t}, \m_{B_t}^{\prime}$ are mapped to a 2-dimensional space and the Euclidean distances $\|\w-\m_{B_t} + \m_{A_t}\|$, $\|\w-\m_{B_t}^\prime + \m_{A_t}\|$ do not change.  Now, we omit the subscript $t$ in $A_t$, $B_t$, $\bxi_t$ and $\sigma_t$, since the analysis below holds at any $t$-th iteration. We first translate them by $\m_A$ and write $\Delta \m = \m_B - \m_A$, $\Delta \m' = \m'_B - \m_A$. 
% \begin{align*}
%      p_{\m_B,\sigma} \rightarrow x - \m_B + \m_A = x - \Delta \m 
% \end{align*}
% \begin{align*}
%      p_{\m'_B,\sigma} \rightarrow x - \m'_B + \m_A = x - \Delta \m'
% \end{align*}
% \begin{align*}
%      p_{\m_A,\sigma} \rightarrow x - \m_A + \m_A = x~.
% \end{align*}

Let $\w$ be a $d$-dimensional Gaussian distribution with zero mean. Fix a basis $\mathbf{b}_1,...,\mathbf{b}_p$ and draw $\w$ by first drawing signed lengths $\lambda_{i} \sim \mathcal{N}\left(0, \sigma^{2}\right), \text { for } i \in[d]$, then $\w = \sum_{i=1}^d \lambda_i \mathbf{b}_i$. We can choose the basis such that $\Delta \m$ and $\Delta \m'$ are parallel to $\mathbf{b}_1$ and $\mathbf{b}_2$ such that $\Delta \m = a_1 \mathbf{b}_1 + a_2 \mathbf{b}_2$ and $\Delta \m' = a'_1 \mathbf{b}_1 + a'_2 \mathbf{b}_2$. Note that $a_1^2 + a_1^2 = \|\Delta \m\|_2^2 = \|\m_B - \m_A\|_2^2$ and $a'_1^2 + a'_1^2 = \|\Delta \m'\|_2^2 = \|\m'_B - \m'_A\|_2^2$
\begin{align*}
I_{A,B}  & = \bigintsss_\w \frac{ \left(  d P_{\m_B,\bxi} -    d P_{\m'_B,\bxi} \right)^2 }{  d P_{\m_A,\bxi}} d \w   \\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| \w -  \m_B\|_2^2 / 2\sigma^2 ) - \exp(- \| \w -  \m'_B\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \w -  \m_A\|_2^2/2\sigma^2)} d \w  ~\\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- \| \w -  \Delta\m \|_2^2 / 2\sigma^2 ) - \exp(- \| \w -  \Delta \m'\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| x\|_2^2/2\sigma^2)} d \w ~ \\
%  & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 -\sum_{i=3}^d \lambda_i^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\sum_{i=1}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~ \\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{d}} \bigints_\w \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(-  (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2+ \sum_{i=3}^d \lambda_i^2/2\sigma^2)} d_{\lambda_1,...,\lambda_d}~\\
 & = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\mathbb{R}^2} \frac{ \bigg( \exp(- (a_1 -  \lambda_1)^2 - (a_2 - \lambda_2)^2 / 2\sigma^2 ) - \exp(- (a'_1 -  \lambda_1)^2 - (a'_2 - \lambda_2)^2 / 2\sigma^2 ) \bigg)^2 }{\exp( - (\lambda_1^2  +\lambda_2^2) / 2\sigma^2)} d_{\lambda_1, \lambda_2}~\\
 & \qquad \cdot \bigints_{\mathbb{R}^{d-2}}\frac{1}{(\sqrt{2 \pi} \sigma)^{d-2}} \exp(- \sum_{i=3}^d \lambda_i^2/2\sigma^2) ~ d_{\lambda_3,...,\lambda_d} \\
 & =  \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\x \in \mathbb{R}^2} \frac{ \bigg( \exp(- \|\x -  \Delta \m \|_2^2 / 2\sigma^2 ) - \exp(- \|\x -  \Delta \m'\|_2^2 / 2\sigma^2 )\bigg)^2 }{\exp( - \|\x\|_2^2 / 2\sigma^2)} d_{\x}
\end{align*}
We abuse the notation and write $ \m_B - \m_A = \Delta \m$ and $ \m'_B - \m_A = \Delta \m'$ as a two dimensional vector with the norm preserved. Then 
\begin{align*}
I_{A,B} 
 = \frac{1}{(\sqrt{2 \pi} \sigma)^{2}} \bigints_{\x \in \mathbb{R}^p} \frac{ \bigg( \exp(- \| \x -  \m_B + \m_A \|_2^2 / 2\sigma^2 ) - \exp(- \| \x -  \m'_B + \m_A\|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \x \|_2^2/2\sigma^2)} d \x ~.
\end{align*}



Then
we have $I_{A_t, B_t}$ as 
\begin{align}
I_{A_t, B_t} =\frac{1}{(\sqrt{2 \pi} \sigma_t)^{2}} \int_{\x} \frac{\left(\exp \left(-\left\|\x-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)-\exp \left(-\left\|\x-\m_{B}^{\prime} + \m_{A_t} \right\|_{2}^{2} / 2 \sigma_t^{2}\right)\right)^{2}}{\exp \left(-\left\|\w\right\|_{2}^{2} / 2 \sigma_t^{2}\right)} d \x~.
\end{align}
Then we treat $\exp \left(-\left\|\x-\m_{B_t} + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ and $\exp \left(-\left\|\x-\m_{B_t}^\prime + \m_{A_t}\right\|_{2}^{2} / 2 \sigma_t^{2}\right)$ as two functions of $\x$ where we can 
use Taylor expansion and apply mean-field theorem. Thus, 
%to bound $I_{A_t, B_t}$ as
for each $\x$, we have:
\begin{align*}
 \exp(- \| \x - \m_B +  {\m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| \x - \m'_B +  {\m_A}\|_2^2 / 2\sigma^2 ) 
 & = \bigg\langle \m_B - \m'_B , \nabla \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2 ) \bigg\rangle~,
\end{align*}
where $\tilde{\m}_B = \alpha_x \m_B + (1-\alpha_x) \m'_B  {- \m_A}$, where $\alpha_x \in [0,1]$ depends on $\x$. 
Let $\| \tilde{\m}_B\|_2 \leq \max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2) \triangleq \bar{\m}_B$. 

We have
\begin{align*}
  \nabla \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2) & = -\frac{\x -\tilde{\m}_B}{\sigma^2} \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2)~, 
\end{align*}
so that
\begin{align*}
& \frac{ \bigg( \exp(- \| \x - \m_B  { + \m_A}\|_2^2 / 2\sigma^2 ) - \exp(- \| \x - \m'_B  { + \m_A} \|_2^2 / 2\sigma^2 ) \bigg)^2 }{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
= \frac{\bigg\langle \m_B - \m'_B , -\frac{\x -\tilde{\m}_B}{\sigma^2} \exp(- \| \x - \tilde{\m}_B\|_2^2 / 2\sigma^2) \bigg\rangle^2}{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{\| \m_B - \m'_B \|_2^2 \| \frac{\x -\tilde{\m}_B}{\sigma^2} \|_2^2 \exp(- \| \x - \tilde{\m}_B\|_2^2 / \sigma^2) }{\exp(-\| \x \|_2^2/2\sigma^2)} \\
& \phantom{......................} 
\leq \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|\x\|^2 + \| \tilde {\m}_B \|_2^2 \bigg)  \exp\left(-\frac{\| \x-\tilde{\m}_B\|_2^2}{\sigma^2} + \frac{\|\x\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
= \frac{2}{\sigma^4} \| \m_B - \m'_B \|_2^2 \bigg(\|\x\|^2 + \|  \tilde{\m}_B \|_2^2 \bigg)  \exp\left( \frac{ {3}\|\tilde{\m}_B\|_2^2}{ {2}\sigma^2}\right)  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) \\
& \phantom{......................} 
\leq \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{ {3}\|\bar{\m}_B\|_2^2}{ {2}\sigma^2}\right) \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) ~.
\end{align*}

Since $\tilde{\m}_B$ interpolate between $\m_B  { - \m_A}$ and $\m'_B  { - \m_A} $ and $\exp$ is positive, based on Proposition \ref{prop:mid_step}, with $\m = 2(\m_B  { - \m_A})$, $\m' = 2(\m'_B  { - \m_A})$ and $\tilde \m = 2 \tilde \m_B$,
we have 
% \abcomment{This step is not correct, should be fixable with a scale factor}
% \begin{align*}
% \exp\left(-\frac{\|x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
% \leq \exp\left(-\frac{\|x-2(\m_B   { - \m_A})\|_2^2}{2\sigma^2} \right) + \exp\left(-\frac{\|x-2(\m'_B   { - \m_A})\|_2^2}{2\sigma^2}~, \right) 
% \end{align*}

\begin{align*}
\exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) 
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) 
\max\left(\exp\left(-\frac{\|\x -2\m_B + 2\m_A\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|\x -2\m_B' + 2\m_A\|_2^2}{\sigma^2}\right) \right)\\
& \leq \exp \left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \left(\exp\left(-\frac{\|\x -2\m_B + 2\m_A\|_2^2}{\sigma^2}\right) + \exp\left(-\frac{\|\x -2\m_B' + 2\m_A\|_2^2}{\sigma^2}\right) \right)
\end{align*}

% \begin{align*}
% \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) \leq \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right).
% \end{align*}



Continuing
\begin{align*}
& \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg)  \frac{1}{2\pi \sigma^2}  \exp\left(-\frac{\|\x-2\tilde{\m}_B\|_2^2}{2\sigma^2} \right) d\x \\
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)  \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|\x-2(\m_B { - \m_A})\|_2^2}{2\sigma^2} \right) d\x \\ 
& \phantom{\leq ......} + \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \bigintss_\x \bigg(\|\x\|^2 + \| \bar{\m}_B \|_2^2 \bigg) \frac{1}{2\pi \sigma^2} \exp\left(-\frac{\|\x-2(\m'_B  { - \m_A})\|_2^2}{2\sigma^2} \right) d\x \\
& \leq \exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \bigg( 2\sigma^2 + 4\|\m_B  { - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 + 2\sigma^2 + 4\|\m'_B  { - \m_A}\|_2^2 + \| \bar{\m}_B\|_2^2 \bigg) \\
& \leq 4 \big(\sigma^2 + \|\m_B  { - \m_A}\|_2^2 + \|\m'_B   { - \m_A} \|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)
\end{align*}


Putting everything back together, we have 
%\yzcomment{Now it just depends on the gradient difference.}
\begin{align*}
I_{A,B} & \leq \frac{1}{2\pi \sigma^2} \frac{4 \pi}{\sigma^2} \| \m_B - \m'_B \|_2^2 \exp\left( \frac{ {3}\|\bar{\m}_B\|_2^2}{ {2}\sigma^2}\right) 4 \big(\sigma^2 + \|\m_B  { - \m_A}\|_2^2 + \|\m'_B  { - \m_A}\|_2^2 + \frac{1}{2} \|\bar{\m}_B\|_2^2 \big)\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)\\
& \leq \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{ \|\bar{\m}_B\|_2^2}{2\sigma^2} \bigg) \exp\left( \frac{3\|\bar{\m}_B\|_2^2}{2\sigma^2}\right)~\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right) \|\m_B-\m_B'\|_2^2 \\
& = \frac{8}{\sigma^2}  \bigg(1 + \frac{\|\m_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\|\m'_B  { - \m_A}\|_2^2}{\sigma^2} + \frac{\max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2)^2}{2\sigma^2} \bigg) \\
& \qquad \exp\left( \frac{\max(\|\m_B  {-\m_A}\|_2,\|\m'_B  {-\m_A} \|_2)\|_2^2}{\sigma^2}\right)~\exp\left(\frac{\|\m_B-\m_B'\|_2^2 }{\sigma^2}\right)\|\m_B-\m_B'\|_2^2
\end{align*}

Now we are interested in $\|\m_B -\m_A\|_2$,  $\|\m'_B -\m_A\|_2$ and $\|\m_B -\m_B'\|_2$. Recall that we have $B \in G_1$ which contains the $z_n'$ and $A \in G_0$: 
\begin{align*}
    \m_B & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_B) \\
    \m'_B & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S'_B) ~.
\end{align*}
\begin{align*}
    \m_A & = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1},S_A) ~.
\end{align*}

So that 

\begin{align*}
\m_B - \m_A & = \eta_t \nabla \ell(\w_{t-1},S_B)  - \eta_t \nabla \ell(\w_{t-1},S_A) \\
& = \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell(\w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(\w_{t-1},\tilde{z}) \right]~,
\end{align*}
and
\begin{align*}
\m'_B - \m_A & = \eta_t \nabla \ell(\w_{t-1},S'_B)  - \eta_t \nabla \ell(\w_{t-1},S_A) \\
& = \frac{\eta_t}{m} \left[ \sum_{z \in S'_B} \nabla \ell(\w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell(\w_{t-1},\tilde{z}) \right]~.
\end{align*}
Also, 
\begin{align*}
\m'_B - \m_B = \frac{\eta_t}{m} \left( \nabla \ell (\w_{t-1}, z_n) - \nabla \ell (\w_{t-1}, z'_n) \right) ~.  
\end{align*}

Let $\Delta_t(\bar{S}) \triangleq \max_{z,\tilde{z} \in \bar{S}} \| \nabla \ell(w_{t-1},z) - \nabla \ell( \w_{t-1},\tilde{z}) \|_2$, where $\bar{S} \sim D^{n+1}$ as before. Now, note that 
%\abcomment{note that the pairing $(z_i,\tilde{z}_i)$ below is arbitrary, the analysis does not depend on the pairing}
\begin{align*}
\| \m_B - \m_A \|_2^2 & = \left\| \frac{\eta_t}{m} \left[ \sum_{z \in S_B} \nabla \ell( \w_{t-1},z) - \sum_{\tilde{z} \in S_A} \nabla \ell( \w_{t-1},\tilde{z} \right] \right\|_2^2 \\
& \leq \eta_t^2 \left\| \frac{1}{m} \sum_{i=1}^m \big( \nabla \ell( \w_{t-1},z_i) - \nabla \ell( \w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
& \leq \eta_t^2 \frac{1}{m} \sum_{i=1}^m  \left\|  \big( \nabla \ell( \w_{t-1},z_i) - \nabla \ell( \w_{t-1},\tilde{z}_i) \big) \right\|_2^2 \\
& \leq \eta_t^2 \Delta^2_t(\bar{S})~.
\end{align*}

Also, $\| \m_B' - \m_A \|_2^2 \leq \eta_t^2 \Delta^2_t(\bar{S})$ and  $\| \m_B' - \m_B \|_2^2 \leq \eta_t^2 \Delta^2_t(\bar{S})$. With the setting that $ \frac{\eta_t^2 \Delta^2_t(\bar{S})}{\sigma^2_t} \leq \ln 3/2$, we have

\begin{align}
I_{A_t, B_t} \leq  \frac{\|\m_{B_t} - \m_{B_t}^\prime \|_2^2}{\sigma_t^2}=  18(1+ \frac{5}{2}\ln\frac{3}{2})\ln \frac{3}{2} \frac{\eta_t^2\left\|\nabla \ell\left( \w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}}{\sigma_t^2}~, \label{eq:guss_with_c}
\end{align}
That completes the proof. \qed


\genboundguss*

\proof Based on Lemma \ref{lemm:iab_guss}, conditioned on past iterates $\w_{0:(t-1)}$, at $t$-th iterate,  we have
\begin{align}
\nr K L\left(P_{t \mid} \| P_{t \mid}^{\prime}\right) & = \underset{B_{t} \in G_{1},A_{t} \in G_{0}}{\mathbb{E}}\left[\int_{\bxi_{t}} \frac{\left(d P_{B_{t}, \boldsymbol{\xi}_{t}}-d P_{B_{t}, \boldsymbol{\xi}_{t}}^{\prime}\right)^{2}}{d P_{A_{t},\boldsymbol{\xi}_{t}}} d \boldsymbol{\xi}_{t}\right]   \leq  \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~,
\end{align}
where $c = 41 \ln \frac{3}{2}$ based on \eqref{eq:guss_with_c}.

Then, based on the chain rule of KL-divergence, we have
\begin{align}
\nr K L\left(P_{0: T} \| P_{0: T}^{\prime}\right) 
& = \sum_{t=1}^{T} \mathbb{E}_{\w_{t-1}} \left[c \frac{\eta_{t}^{2}}{\sigma_{t}^{2}} \left\|\nabla \ell\left(\w_{t-1}, z_{n}\right)-\ell\left(\w_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]~.
\end{align}

Following Theorem \ref{theo:stab}, we have
\begin{align*}
\left|\mathbb{E}_{S}\left[L_{D}\left(\mathbf{w}_{T}\right)-L_{S}\left(\mathbf{w}_{T}\right)\right]\right| \leq c \frac{b}{n} \mathbb{E}_{\bar{S}} \sqrt{\sum_{t=1}^{T} \underset{\mathbf{w}_{t-1}}{\mathbb{E}}\left[\frac{\eta_{t}^{2}}{\sigma_{t}^{2}}\left\|\nabla \ell\left(\mathbf{w}_{t-1}, z_{n}\right)-\ell\left(\mathbf{w}_{t-1}, z_{n}^{\prime}\right)\right\|_{2}^{2}\right]},  
\end{align*}
where $c = 41 \ln \frac{3}{2}$. 


\begin{prop}
Assume $\m,\m'$ fixed and $\tilde{\m}$ on the line segment of $\m$ and $\m'$, we have
    \begin{align*}
    \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) \leq \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right).
\end{align*} \label{prop:mid_step}
\end{prop}

\proof  From the law of cosine, we have 
\begin{align*}
    \|x -\m\|_2^2 = \|x-\tilde{\m}\|_2^2 + \|\m-\tilde{\m}\|_2^2 -2 \|x-\tilde{\m}\|_2  \|\m-\tilde{\m}\|_2 \cos \angle x\tilde{\m} \m,
\end{align*}
and
\begin{align*}
    \|x -\m'\|_2^2 = \|x-\tilde{\m}\|_2^2 + \|\m'-\tilde{\m}\|_2^2 -2 \|x-\tilde{\m}\|_2  \|\m'-\tilde{\m}\|_2 \cos \angle x\tilde{\m} \m',
\end{align*}
where $\angle x\tilde{\m} \m + \angle x\tilde{\m} \m' = \frac{\pi}{2}$ so we have $\cos\angle x\tilde{\m} \m + \cos\angle x\tilde{\m} \m' = 0$. By canceling out $\cos$ via weighted sum of the above two equations, we have
\begin{align*}
    &\|x -\m\|_2^2 \|\m'-\tilde{\m}\|_2 + \|x -\m'\|_2^2 \|\m-\tilde{\m}\|_2\\
    =& \|x-\tilde{\m}\|_2^2\|\m'-\tilde{\m}\|_2 + \|\m-\tilde{\m}\|_2^2\|\m'-\tilde{\m}\|_2 + \|x-\tilde{\m}\|_2^2\|\m-\tilde{\m}\|_2 + \|\m'-\tilde{\m}\|_2^2\|\m-\tilde{\m}\|_2.
\end{align*}
Equivalently we have 
\begin{align*}
    \|x-\tilde{\m}\|_2^2 = \frac{\|\m-\tilde{\m}\|_2}{\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2} \|x -\m'\|_2^2 + \frac{\|\m'-\tilde{\m}\|_2}{\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2} \|x -\m\|_2^2 - \|\m-\tilde{\m}\|_2\|\m'-\tilde{\m}\|_2.
\end{align*}
Since $\|\m-\tilde{\m}\|_2+\|\m'-\tilde{\m}\|_2 = \|\m-\m'\|_2$, from AM-GM inequality we have
\begin{align*}
    \|x-\tilde{\m}\|_2^2\geq \min \left(\|x -\m\|_2^2,\|x -\m'\|_2^2\right) - \frac{1}{4} \|\m-\m'\|_2^2,
\end{align*}
therefore we have
\begin{align*}
    \exp\left(-\frac{\|x-\tilde{\m}\|_2^2}{\sigma^2} \right) &\leq \exp\left(-\min \left(\frac{\|x -\m\|_2^2}{\sigma^2},\frac{\|x -\m'\|_2^2}{\sigma^2}\right) + \frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\\
    &= \exp\left(\frac{1}{4} \frac{\|\m-\m'\|_2^2 }{\sigma^2}\right)\max\left(\exp\left(-\frac{\|x -\m\|_2^2}{\sigma^2}\right),\exp\left(-\frac{\|x -\m'\|_2^2}{\sigma^2}\right) \right),
\end{align*}
which completes the proof.
\qed



==> arXiv/app/signSGD_opt.tex <==
% The ``density'' for a mini-batch $B$ at scale $\alpha$ is:
% \begin{equation}
% p_{\psi}(\bxi; \btheta_{B,\alpha}) = \exp(\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha} \triangleq \frac{\btheta_B}{\alpha} = \frac{\nabla \ell(\w_{t-1}, S_{B})}{\alpha}~.
% \end{equation}
% Note that the corresponding expectation parameter
% \begin{equation}
% \m_{B,\alpha} = \nabla_{\btheta_{B,\alpha}} \psi( \theta_{B,\alpha} )~.
% \end{equation}

% For mini-batch $B_t$ and scaling $\alpha_t$, Noisy Sign-SGD updates the parameters as
% \begin{equation}
%     \w_t = \w_{t-1} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim B\left(\frac{1}{1+\exp \left(-\boldsymbol{\theta}_{B_{t}, \alpha_{t}}\right)}\right)~, ~ \forall i\in [d]~.
% \end{equation}
% % Here we consider the special case of Bernoulli distribution. Thus
% % $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$

% \begin{asmp}\label{asmp: smooth}
% [Smoothness] For all $\w$ and $\w^\prime$, for some non-negative constant $\vec{K}:=\left[L_{1}, \ldots, L_{d}\right]$, we have
% \begin{align}
% L_S(\w) \leq L_S(\w^\prime) + \nabla L_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} L_i (\w_i - \w^\prime_i)^2
% \end{align}
% \end{asmp}

% Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have
% \begin{align*}
%     L_S(\w_{t+1}) -L_S(\w_{t}) & \leq \nabla L_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d L_i (\w_{t,i} - \w^\prime_{t,i})^2\\
%     & = - \eta_t  \nabla L_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{L_i}{2}\\
%     & = - \eta_t  \|\nabla L_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{K}\|_1 + 2 \eta_t \sum_{i=1}^d |\nabla_i L_S(\w_t)| \mathbb{I}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\}
% \end{align*}

% Take the conditional expectation, we have
% \begin{align*}
% \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq   - \eta_t  \|\nabla L_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{K}\|_1 + 2 \eta_t \sum_{i=1}^d |\nabla_i L_S(\w_t)| \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} 
% \end{align*}

% For now, we have the following approaches:
% \begin{itemize}
%     \item Option I: Show $ \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} \leq 1/2$ for all $i \in [d]$, then we will have $-\eta_t \cdot c \|\nabla L_S(\w_t)\|_1$ for $0<c < 1/2$ on the right hand side. The rest will be standard optimization analysis. 
%     \item Option II: 
%     \begin{align*}
%         \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} & \leq \mathbb{P}\{ |\bxi_{t, i} - \nabla_i L_S(\w_t)| > |\nabla_i L_S(\w_t)|\}\\
%         & \leq \frac{\mathbb{E}[|\bxi_{t, i} - \nabla_i L_S(\w_t)| ]}{ |\nabla_i L_S(\w_t)|}
%     \end{align*}
% \end{itemize}


% \tccomment{
% Case 1: $\nabla_i L_S(\w_t)) > 0$, we have
% \begin{align*}
%     \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} = \mathbb{P}\{\bxi_{t, i} = -1\} = 1-\frac{1}{1+\exp \left(-\nabla_i L_S(\w_t)\right)} < 1-\frac{1}{1+\exp \left(0\right)} = \frac{1}{2}.
% \end{align*}
% Case 2: $\nabla_i L_S(\w_t)) < 0$, we have
% \begin{align*}
%     \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} = \mathbb{P}\{\bxi_{t, i} = 1\} = \frac{1}{1+\exp \left(-\nabla_i L_S(\w_t)\right)} < \frac{1}{1+\exp \left(0\right)} = \frac{1}{2}.
% \end{align*}
% Therefore, we conclude that $ \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} < 1/2$ holds. $c$ approaches zero when $\nabla_i L_S(\w_t)$ approaches zero.
% \yzcomment{To be more rigours, it should be 
% \begin{align*}
% \mathbb{P}\{\bxi_{t, i} \neq \sign(\nabla_i L_S(\w_t))\} \leq  \mathbb{P}\{\bxi_{t, i} = -1|\nabla_i L_S(\w_t)) > 0\} +    \mathbb{P}\{\bxi_{t, i} = 1|\nabla_i L_S(\w_t)) < 0\} 
% \end{align*}
% I am not sure whether there is dependence between $\bxi_t$ and $ \nabla L_S(\w_t))$, i.e.,
% $\mathbb{P}\{\bxi_{t, i} = -1|\nabla_i L_S(\w_t)) > 0\} = \mathbb{P}\{\bxi_{t, i} = -1\}$ ?
% }
% \subsection{Choice 2:} 
% Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have
% \begin{align*}
%     L_S(\w_{t+1}) -L_S(\w_{t}) & \leq \nabla L_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d L_i (\w_{t,i} - \w^\prime_{t,i})^2\\
%     & = - \eta_t  \nabla L_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{L_i}{2}
% \end{align*}
% Define a function $f:\R^p \rightarrow \R$, where $p$ is the dimension of model parameters: 
% \begin{align*}
%     f(\theta) = \sum_i \theta_i \frac{\exp \theta_i -1}{\exp \theta_i +1} = \sum_i \theta_i \tanh \frac{\theta_i}{2},
% \end{align*}
% we have $f(\theta) \geq 0$, and equality holds if and only if $\theta_i = 0$. Then taking conditional expectation on both side we have 
% \begin{align*}
% \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla L_S(\w_t)^T \E\bxi_t  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  \sum_i \nabla L_S(\w_t)_i \left(\frac{2}{1+\exp \left(-\nabla L_S(\w_t)_i\right)}-1\right)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  \sum_i \nabla L_S(\w_t)_i \left(\frac{\exp \left(-\nabla L_S(\w_t)_i\right) -1 }{\exp \left(-\nabla L_S(\w_t)_i\right)+1}\right)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  f(\nabla L_S(\w_t))  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% \end{align*}
% Taking $\eta_t = \frac{1}{\sqrt{T}}$, by telescope sum we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T f(\nabla L_S(\w_t))\right] \leq \frac{1}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% \end{equation}
% \yzcomment{The distribution of $\bxi_t$ depends on $\nabla \ell(\w_t, S_B)$ instead of full batch gradient $\nabla L_S(\w_t)$, i.e., $\mathbb{P}\{\bxi_{t, i} = -1\} = 1-\frac{1}{1+\exp \left(-\nabla_i \ell(\w_t, S_B)/\alpha\right)}$, where $\mathbb{E}[\nabla \ell(\w_t, S_B)] = \nabla L_S(\w_t)$ . Can we use Jensen's inequality here?}
% Mini-batch settings: 
% \begin{align*}
% \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla L_S(\w_t)^T \E\bxi_t  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  \sum_i \nabla L_S(\w_t)_i \E\left[\frac{2}{1+\exp \left(-\nabla_i \ell(\w_{t-1}, S_{B}/\alpha)\right)}-1\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% &= - \eta_t  \sum_i \nabla L_S(\w_t)_i \E\left[\frac{\exp \left(\nabla_i \ell(\w_{t-1}, S_{B})/\alpha\right) -1 }{\exp \left(\nabla_i \ell(\w_{t-1}, S_{B})/\alpha\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% & = - \eta_t  \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% \end{align*}
% The first quantity can be decomposed as
% \begin{align*}
% & = - \eta_t  \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] - \eta_t\left( \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right)
% \end{align*}
% The first part is $- \eta_t \alpha  f(\nabla L_S(\w_t)/\alpha)$, the second part can be upper bounded by
% \begin{align*}
%   & - \eta_t\left( \sum_i \E\theta_{B,i} \E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \sum_i \E\theta_{B,i} \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right) \\
%     & \leq  \eta_t\sum_i |\E\theta_{B,i}|\left|\E\left[\frac{\exp \left(\theta_{B,i}/\alpha\right) -1 }{\exp \left(\theta_{B,i}/\alpha\right)+1}\right] - \left[\frac{\exp \left(\E\theta_{B,i}/\alpha\right) -1 }{\exp \left(\E\theta_{B,i}/\alpha\right)+1}\right] \right|\\
%     & \leq \eta_t/\alpha \sum_i |\E\theta_{B,i}|\left|\E|\theta_{B,i} -\E[\theta_{B,i}]|\right|\\
%     & = \eta_t/\alpha \sum_i |\E\theta_{B,i}| \|\theta_{B,i} -\E[\theta_{B,i}]\|_{L^1}\\
%     & \leq \frac{\sigma_t\eta_t}{\alpha} \|\E\theta_{B}\|_1\\
%     & \leq \frac{\sigma\eta_t}{\alpha\sqrt{|B_t|}} \|\E\theta_{B}\|_1
% \end{align*}
% where $\tanh$ is 1-Lipschitz function, and we assume first order moment of stochastic gradient is upper bounded by $\sigma_t$ and we can naturally define $\sigma_t\leq \sigma/\sqrt{|B_t|}$. \yzcomment{We can also assume bounded variance/second moment which is common.}
% Gathering everything we have
% \begin{align*}
%   \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}]\leq - \eta_t \alpha  f(\nabla L_S(\w_t)/\alpha) + \frac{\sigma\eta_t}{\alpha\sqrt{|B_t|}} \|\nabla L_S(\w_t)\|_1 + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% \end{align*}
% Bt taking $\eta_t = \frac{1}{\sqrt{T}}$, $|B_t| = T$ \yzcomment{This requires $n > = T$, usually we use $|B_t| = \sqrt{T}$ } by telescope sum we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \left(\alpha f(\nabla L_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla L_S(\w_t)\|_1\right) \right] \leq \frac{1}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% \end{equation}
% % Note that $T\rightarrow \infty $, equation implies $$\frac{1}{T}\sum_{t=1}^T \left(\alpha f(\nabla L_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla L_S(\w_t)\|_1\right)  \rightarrow 0,$$ implies $$\alpha f(\nabla L_S(\w_T)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla L_S(\w_T)\|_1\rightarrow 0, $$ implies $$\alpha f(\nabla L_S(\w_T)/\alpha ) \rightarrow 0, $$ implies $$\nablaL_S(\w_T) \rightarrow 0.$$
% Since we have
% \begin{equation}
%     x\tanh x/2 > x^2 \frac{1}{2(1+2\log(\frac{\sinh x}{x})},
% \end{equation}
% and
% \begin{equation}
%     \sinh x 
% \end{equation}
% \begin{align*}
%     \alpha f(\nabla L_S(\w_t)/\alpha ) - \frac{\sigma}{\alpha\sqrt{T}} \|\nabla L_S(\w_t)\|_1 \geq 
% \end{align*}}
% \section{Noisy-SignSGD Optimization analysis}

\subsection{Optimization Guarantees for Noisy Sign-SGD}


The ``density'' for a mini-batch $B$ at scale $\alpha$ is:
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\alpha}) = \exp(\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha})) \ppi_0(\bxi)   ~, \qquad \btheta_{B,\alpha} \triangleq \frac{\btheta_B}{\alpha} = \frac{\nabla \ell(\w_{t}, S_{B})}{\alpha}~.
\end{equation}
Note that the corresponding expectation parameter
\begin{equation}
\m_{B,\alpha} = \nabla_{\btheta_{B,\alpha}} \psi( \theta_{B,\alpha} )~.
\end{equation}
The full-batch Noisy Sign-SGD update the parameters as 
\begin{equation}\label{eq:app_signSGD_full_batch}
    \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim \text{Rad}\left(\frac{1}{1+\exp \left(-2\nabla L_S(\w_t)/\alpha_{t}\right)}\right)~, ~ \forall i\in [d]~,
\end{equation}
where $\text{Rad}(x)$ is the parametric Rademacher distribution with density $x$ at $1$ and density $1-x$ at $-1$.
For mini-batch $B_t$ and scaling $\alpha_t$, mini-batch Noisy Sign-SGD updates the parameters as  
\begin{equation}\label{eq:app_signSGD_mini_batch}
    \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim \text{Rad}\left(\frac{1}{1+\exp \left(-2\boldsymbol{\theta}_{B_{t}, \alpha_{t}}\right)}\right)~, ~ \forall i\in [d]~.
\end{equation}
% Here we consider the special case of Bernoulli distribution. Thus
% $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$
We make the following smoothness assumptions of the empirical loss function $L_S(\w)$:
\asmpsmooth*
% \begin{asmp}\label{asmp: smooth}
% The loss function $L_S$ satisfies: for all $\w$ and $\w^\prime$, for some non-negative constant $\vec{K}:=\left[L_{1}, \ldots, L_{d}\right]$, we have
% \begin{align}
% L_S(\w) \leq L_S(\w^\prime) + \nabla L_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} L_i (\w_i - \w^\prime_i)^2
% \end{align}
% \end{asmp}
The assumption on on the empirical loss $L_S(\w)$ is common in optimization analysis, besides that, we also assume some natural statistical properties of the batch gradient of the loss $\nabla \ell(\w_{t}, S_{B_t})$, where the randomness comes from batches conditioned on $\w_t$, satisfies the following assumptions:
\asmpbatch*
% \begin{asmp}\label{asmp:batch}
% [Batch Gradient] Given $\w_t$, the batched gradient $\nabla \ell(\w_t, S_{B_t})$ satisfies the following property:
% \begin{itemize}
%     \item (Unbiased) The batched gradient $\nabla \ell(\w_{t}, S_{{B_t}})$ is an unbiased estimator of true gradient $L_S(\w_{t})$: $$\E_{B_t|\w_t}\nabla \ell(\w_{t}, S_{B_t}) = \nabla L_S(\w_{t}).$$
%     \item (Symmetricity) The pdf $p_{BG}(x)$ of batched gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is symmetric around its expectation $L_S(\w_{t})$:$$p_{BG}(x) = p_{BG}(2\nablaL_S(\w_{t})-x).$$
%     \item (Sub-Gaussian) The batched gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is Sub-Gaussian with $\psi_2$ norm $\kappa_t$, where $\kappa_t \leq \kappa_t/\sqrt{|B_t|}$: for any $\lambda >0$, $v\in S^{d-1}$, we have $$\E_{B_t|\w_t}\exp \lambda\langle v,\nabla \ell(\w_{t}, S_{B_{t}})-\nabla L_S(\w_{t})\rangle \leq \exp(\lambda^2\kappa_t^2/2)\leq \exp\left(\frac{\lambda^2\kappa_t^2}{2|B_t|}\right).$$
% \end{itemize}
% \end{asmp}
With Assumption \ref{asmp: smooth} and Assumption \ref{asmp:batch}, we have the following guarantee for convergence of noisy signSGD under full batch and mini batch settings. The following is a restate theorem from the main paper for the mini-batch Noisy Sign-SGD
\theosignSGDconv*
% \begin{theo}\label{theo:signSGD_conv}
% Assume Assumption~\ref{asmp: smooth} holds for loss function $L_S$. For Full-batch Noisy Sign-SGD algorithm equation~\eqref{eq:signSGD_full_batch} with stepsize $\eta_t = 1/\sqrt{T}$ and choose $\alpha_t$ satisfies $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}/2$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{10c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
% \end{equation}
% Further assume Assumption~\ref{asmp:batch} holds for batch gradient $\nabla\ell(\w_t,S_{B_t})$, for mini-batch noisy Sign-SGD algorithm equation~\eqref{eq:signSGD_mini_batch} with stepsize $\eta_t = 1/\sqrt{T}$, $|B_t|=T$, and 
% % $\alpha_t = 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa_t^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% % \end{equation}
% % or choose $c\geq\alpha_t\geq 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{2c (1+\exp(\frac{\kappa_t^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% % \end{equation}
% % or without assuming $G$, 
% choose $\alpha_t$ by $c \geq \alpha_t \geq \max[\frac{\kappa_t}{\sqrt{2T}}, 2\|\nabla L_S(\w_t)\|_{\infty}]$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{8c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% \end{equation}
% \end{theo}
% Here we restate our results
% \begin{restatable}{theo}\label{theo:signSGD}
% If the loss satisfies Assumption~\ref{asmp: smooth}, for full-batch noisy Sign-SGD with step size $\rho_t = 1/\sqrt{T}$ and $\alpha_t$ satisfying $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}$, we have
% \begin{equation}\label{eq:sign_SGD_full_batch_convergence_1}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{5c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% \end{equation}
% Further, if Assumption~\ref{asmp:batch} holds, for mini-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$, and 
% % $\alpha_t = 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% % \end{equation}
% % or choose $c\geq\alpha_t\geq 2G$, we have
% % \begin{equation}
% %     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{2c (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
% % \end{equation}
% % or without assuming $G$, 
% $\alpha_t$ satisfying $c \geq \alpha_t \geq \max[\sqrt{2}\kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, we have
% \begin{equation}\label{eq:sign_SGD_mini_batch_convergence_1}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
% \end{equation}
% where equation \eqref{eq:sign_SGD_full_batch_convergence_1}\eqref{eq:sign_SGD_mini_batch_convergence_1} holds for any $S$, any initialization $\w_0$, and the expectation is taken over the randomness of  algorithm.
% \end{restatable}





% The result shows the same $O(\frac{1}{\sqrt{T}})$ convergence speed with slightly different constants for both full-batched and mini-batched noisy Sign-SGD.


\proof First we prove Equation \eqref{eq:sign_SGD_full_batch_convergence_1} for full-batched settings.
Conditioned at $t$-th iteration, with Assumption \ref{asmp: smooth}, we have 
\begin{align*}
    L_S(\w_{t+1}) -L_S(\w_{t}) & \leq \nabla L_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \sum_{i=1}^d K_i (\w_{t+1,i} - \w_{t,i})^2\\
    & = - \eta_t  \nabla L_S(\w_t)^T \bxi_t  + \eta_t^2 \sum_{i=1}^d \frac{K_i}{2}.
\end{align*}
% \abbcomment{how are $K_i$ and $L_i$ related?}
% Define a function $f:\R^d \rightarrow \R$, where $d$ is the dimension of model parameters: 
% \begin{align*}
%     f(\theta) = \sum_i \theta_i \frac{\exp \theta_i -1}{\exp \theta_i +1} = \sum_i \theta_i \tanh \frac{\theta_i}{2},
% \end{align*}
% we have $f(\theta) \geq 0$, and equality holds if and only if $\theta_i = 0$. 
Then taking conditional expectation on both side for above equation we have
\begin{align*}
\mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq   - \eta_t  \nabla L_S(\w_t)^T \E_{\bxi_t|\w_t}\bxi_t  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \left(\frac{2}{1+\exp \left(-2\nabla L_S(\w_t)_i/\alpha_t\right)}-1\right)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \left(\frac{\exp \left(2\nabla L_S(\w_t)_i/\alpha_t\right) -1 }{\exp \left(2\nabla L_S(\w_t)_i/\alpha_t\right)+1}\right)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \tanh (\nabla L_S(\w_t)_i/\alpha_t)  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i |\nabla L_S(\w_t)_i| |\tanh (\nabla L_S(\w_t)_i/\alpha_t)|  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{align*}
By taking $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}$, and $\eta_t=1/\sqrt{T}$, we have $\nabla L_S(\w_t)_i/\alpha_t\leq 1$ so we can apply Lemma \ref{lemm:tanh_bound} to have
\begin{align*}
\mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq  - \frac{e^2-1}{(e^2+1)\alpha_t\sqrt{T}}  \|\nabla L_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{K}\|_1\\
&\leq - \frac{3}{5c\sqrt{T}}  \|\nabla L_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{K}\|_1.
\end{align*}
% \abbcomment{what is the para, text, punctuation here?? lets please get our act together}
By telescope sum we have
\begin{equation}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{5c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
\end{equation}
which completes the proof of full-batch updates.   


Then we turn to prove Equation \eqref{eq:sign_SGD_mini_batch_convergence_1} for mini-batch settings.
From smoothness condition Assumption \ref{asmp: smooth}, we have
\begin{align*}
\mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] &\leq \E_{\w_{t+1}|\w_t}\nabla L_S(\w_t)^T(\w_{t+1} - \w_{t}) + \frac{1}{2} \E_{\w_{t+1}|\w_t} \sum_{i=1}^d L_i (\w_{t+1,i} - \w_{t,i})^2\\
&= \E_{\bxi_t|\w_t} \nabla L_S(\w_t)^T(-\eta_t \bxi_t) + \frac{1}{2} \E_{\bxi_t|\w_t} \sum_{i=1}^d L_i (-\eta_t \bxi_t)^2\\
    &=- \eta_t  \nabla L_S(\w_t)^T \E_{\bxi_t|\w_t}\bxi_t  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \E_{B_t|\w_t}\left[\frac{2}{1+\exp \left(-2\nabla_i \ell(\w_t, S_{B_{t}}/\alpha_t)\right)}-1\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
&= - \eta_t  \sum_i \nabla L_S(\w_t)_i \E_{B_t|\w_t}\left[\frac{\exp \left(2\nabla_i \ell(\w_t, S_{B_{t}})/\alpha_t\right) -1 }{\exp \left(2\nabla_i \ell(\w_t, S_{B_{t}})/\alpha_t\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
& = - \eta_t  \sum_i \E_{B_t|\w_t} [\theta_{B_{t},i}] \E\left[\frac{\exp \left(2\theta_{B_{t},i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_{t},i}/\alpha_t\right)+1}\right]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{align*}

Focus on each individual term in the sum, we have
\begin{align*}
\E_{B_t|\w_t}&[\theta_{B,i}] \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_t,i}/\alpha_t\right)+1}\right]\\ 
& = \E_{B_t|\w_t}[\theta_{B_t,i}] \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t - 2\E_{B_t|\w_t}[\theta_{B_t,i}/\alpha_t] \right) -\exp - 2\E_{B_t|\w_t}\theta_{B_t,i}/\alpha_t }{\exp \left(2\theta_{B_t,i}/\alpha_t - 2\E_{B_t|\w_t}[\theta_{B_t,i}/\alpha_t]\right)+\exp - 2\E_{B_t|\w_t}\theta_{B_t,i}/\alpha_t}\right]
\end{align*}


For ease of notation, denote $2\theta_{B,i}/\alpha_t - \E_{B_t|\w_t}[2\theta_{B,i}/\alpha_t] = \theta,~\E_{B_t|\w_t}[2\theta_{B,i}/\alpha_t] =\mu$,\abbcomment{this is bad notation as we keep $\mu$ for the expectation parameters} and the pdf of $\theta$ is $p_{\theta}$ for the moment, then from Assumption \ref{asmp:batch}, we have $\theta$ is mean zero, symmetric around zero, and subgaussian with $\psi_2$ norm $2\kappa_t/\alpha_t$ by taking $\lambda=1,~v = \1_i$ in the sub-Gaussian assumption: $\E_\theta[\exp\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$.

Therefore, by changing notation we have 
\begin{align*}
     \E_{B_t|\w_t}[\theta_{B,i}] \E_{B_t|\w_t}\left[\frac{\exp \left(2\theta_{B_t,i}/\alpha_t\right) -1 }{\exp \left(2\theta_{B_t,i}/\alpha_t\right)+1}\right] = \frac{\alpha_t \mu}{2} \E_\theta\left[\frac{\exp \theta -\exp(-\mu) }{\exp \theta +\exp(-\mu)}\right].
\end{align*}
By symmetry of the distribution of $\theta$, we have
\begin{align*}
\frac{\alpha_t \mu}{2} \mu\E&_\theta\left[\frac{\exp \theta -\exp(-\mu) }{\exp \theta +\exp(-\mu)}\right]\\
    &= \frac{\alpha_t \mu}{2}\int_{-\infty}^{\infty}p_\theta(x)\left[\frac{\exp x-\exp(-\mu) }{\exp x +\exp(-\mu)}\right]dx\\
    &=\frac{\alpha_t \mu}{2}\int_{0}^{\infty}p_\theta(x)\left[\frac{\exp x -\exp(-\mu) }{\exp x +\exp(-\mu)}+\frac{\exp (-x) -\exp(-\mu) }{\exp (-x) +\exp(-\mu)}\right]dx\\
    &=\frac{\alpha_t \mu}{2}\int_{0}^{\infty}p_\theta(x)\frac{(\exp x -\exp(-\mu))(\exp (-x) +\exp(-\mu)) + (\exp (-x) -\exp(-\mu))(\exp x +\exp(-\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\alpha_t/2 \int_{0}^{\infty}p_\theta(x)\frac{2\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx
\end{align*}
By symmetry, we have $p_\theta(x) = p_\theta(-x)$, and therefore
\begin{align*}
\alpha_t/2 & \int_{0}^{\infty}p_\theta(x)\frac{2\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\alpha_t/2\int_{-\infty}^{\infty}p_\theta(x)\frac{\mu (1-\exp(-2\mu))}{(\exp x +\exp(-\mu))(\exp (-x) +\exp(-\mu))}dx\\
    &=\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \E_\theta\frac{1}{(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}
\end{align*}
Since $\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu)))\geq 0$, and $\frac{1}{x}$ is convex on $\R_+$, we have
\begin{align*}
   & \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \E_\theta\frac{1}{(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}\\ \geq &\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{\E_\theta(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}.
\end{align*}
% Since $\exp \theta +\exp(-\mu)$ and $\exp (-\theta) +\exp(-\mu)$ are inversely monotone function, by chebyshev sum's inequality, we have
% \begin{align*}
%     \E(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))\leq \E(\exp \theta +\exp(-\mu)) 
% \end{align*}
\abcomment{please see alternative analysis from this point onwards after this proof, trying to avoid getting a bound in terms of $c \geq \alpha_t, \forall t$}

Using the sub-Gaussian property of $\theta$: $\E_\theta[\exp\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$, and symmetry so $\E_\theta[\exp -\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$, we have
\begin{align*}
    &\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{\E_\theta(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}\\
    &= \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+\exp(-\mu)(\E\exp \theta +\E\exp (-\theta))}\\
    &\geq  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+2\exp(-\mu)\exp(2\kappa_t^2/\alpha_t^2)}\\
    &\geq  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}.
\end{align*}
Switching back to our previous notation:
\begin{align*}
    \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}
  & = \E_{B_t|\w_t} \theta_{B,i} (1-\exp(-4\E_{B_t|\w_t}\theta_{B,i}/\alpha_t)) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)}\\
  & = \nabla L_S(\w_t)_i (1-\exp(-4\nabla L_S(\w_t)_i/\alpha_t)) \frac{1}{2+2\exp(2\kappa_t^2/\alpha_t^2)},
\end{align*}


which implies we have
\begin{align*}
    \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{2+2\exp(2\kappa_t^2/\alpha_t^2)}  \sum_i \nabla L_S(\w_t)_i (1-\exp(-4\nabla L_S(\w_t)_i/\alpha_t))  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{align*}
Using Lemma \ref{lemm:mix_norm}, we have
\begin{equation}
    \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{2(1+\exp(2\kappa_t^2/\alpha_t^2))}  \sum_i |\nabla L_S(\w_t)_i| \min \bigg[ |2\nabla L_S(\w_t)_i/\alpha_t| ,0.5\bigg]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
 \end{equation}

We choose $\alpha_t$ such that $\alpha_t \geq 4\|\nabla L_S(\w_t)\|_{\infty}$, then we have
\begin{equation}
\mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{\alpha_t (1+\exp(2\kappa_t^2/\alpha_t^2))}  \|\nabla L_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{equation}
We choose $\alpha_t$ such that $c\geq \alpha_t \geq \max[\sqrt{2} \kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, then we have 
\begin{equation}
    \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{c (1+e)}  \|\nabla L_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
\end{equation}
Therefore, if we choose $\eta_t = 1/\sqrt{T}$, we have
\begin{equation}
    \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{1}{c (1+e)\sqrt{T}}  \|\nabla L_S(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{K}\|_1.
\end{equation}
By telescope sum, we have
\begin{equation}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{(1+e)c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
\end{equation}
and note that $1+e<4 $ which completes the proof.   \qed

%--------------------------------------------

% \noindent \abcomment{alternative analysis starts here}

% Using the sub-Gaussian property of $\theta$: $\E_\theta[\exp\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$, and symmetry so $\E_\theta[\exp -\theta] \leq \exp(2\kappa_t^2/\alpha_t^2)$, we have
% \begin{align*}
%     &\frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{\E_\theta(\exp \theta +\exp(-\mu))(\exp (-\theta) +\exp(-\mu))}\\
%     &= \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+\exp(-\mu)(\E\exp \theta +\E\exp (-\theta))}\\
%     &\geq  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{1 +\exp(-2\mu)+2\exp(-\mu)\exp(2\kappa_t^2/\alpha_t^2)}\\
%     &\overset{(a)}{\geq}  \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{(1+\exp(-\mu))^2}~,
% \end{align*}
% where (a) follows since $\alpha_t^2 \geq 2\kappa_t^2$. Switching back to our previous notation:
% \begin{align*}
%     \frac{\alpha_t }{2}(\mu (1-\exp(-2\mu))) \frac{1}{(1+\exp(-\mu))^2}
%   & =  \frac{\E_{B_t|\w_t} [\theta_{B,i}] (1-\exp(-4\E_{B_t|\w_t}\theta_{B,i}/\alpha_t))}{(1+ \exp(-\E_{B_t|\w_t} [2\theta_{B,i}/\alpha_t]))^2}\\
%   & =  \frac{\nabla \ell(\w_t)_i (1-\exp(-4\nabla \ell(\w_t)_i/\alpha_t))}{(1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t))^2}~,
% \end{align*}
% which implies we have
% \begin{align*}
%     \mathbb{E}[ \ell(\w_{t+1}) -\ell(\w_{t})|\w_{t}] \leq - \eta_t  \sum_i \frac{\nabla \ell(\w_t)_i (1-\exp(-4\nabla \ell(\w_t)_i/\alpha_t))}{(1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t))^2}  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% \end{align*}
% Since $\alpha_t \geq 4 \| \nabla \ell(\w_t) \|_\infty$, we have $(1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t))^2 \leq 8$. Further, using Lemma \ref{lemm:mix_norm}, we have
% \begin{align*}
% \mathbb{E}[ \ell(\w_{t+1}) -\ell(\w_{t})|\w_{t}] & \leq - \frac{\eta_t}{8}  \sum_i |\nabla \ell(\w_t)_i| \min \bigg[ |2\nabla \ell(\w_t)_i/\alpha_t| ,0.5\bigg]  + \frac{\eta_t^2}{2} \|\vec{K}\|_1 \\
% & \leq - \frac{\eta_t}{8}  \|\nabla \ell(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1~,  
%  \end{align*}
% where (a) follows since $\alpha_t \geq \| \nabla \ell(\w_t) \|_\infty$. \tccomment{The last step becomes $\frac{\eta_t}{4\alpha_t}  \|\nabla \ell(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1$ so we still need upper bound on $\alpha_t$? Or shall we express the bound into L1 norm instead of L2 square so we can avoid c?}

% % \tccomment{How about this:
% % we have
% % \begin{align*}
% %     \mathbb{E}[ \ell(\w_{t+1}) -\ell(\w_{t})|\w_{t}] &\leq - \eta_t  \sum_i \frac{\nabla \ell(\w_t)_i (1-\exp(-4\nabla \ell(\w_t)_i/\alpha_t))}{(1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t))^2}  + \frac{\eta_t^2}{2} \|\vec{K}\|_1\\
% %     &= - \eta_t  \sum_i \frac{\nabla \ell(\w_t)_i (1-\exp(-2\nabla \ell(\w_t)_i/\alpha_t))}{1+\exp(-2\nabla \ell(\w_t)_i/\alpha_t)}  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% % \end{align*}
% % we prove for $x\in[-1,1]$, $x\frac{1-\exp(-2x)}{1+\exp(-2x)}\geq $
% % }





% % We choose $\alpha_t$ such that $\alpha_t \geq 4\|\nabla L_S(\w_t)\|_{\infty}$, then we have
% % \begin{equation}
% % \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{\alpha_t (1+\exp(2\kappa_t^2/\alpha_t^2))}  \|\nabla L_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% % \end{equation}
% % We choose $\alpha_t$ such that $\alpha_t \geq \max[\sqrt{2} \kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, then we have \abbcomment{remind readers that $c \geq \alpha_t$}
% % \begin{equation}
% %     \mathbb{E}[ L_S(\w_{t+1}) -L_S(\w_{t})|\w_{t}] \leq - \frac{\eta_t}{c (1+e)}  \|\nabla L_S(\w_t)\|_2^2  + \frac{\eta_t^2}{2} \|\vec{K}\|_1.
% % \end{equation}
% Therefore, if we choose $\eta_t = 1/\sqrt{T}$, we have
% \begin{equation}
%     \mathbb{E}[ \ell(\w_{t+1}) -\ell(\w_{t})|\w_{t}] \leq - \frac{1}{8\sqrt{T}}  \|\nabla \ell(\w_t)\|_2^2  + \frac{1}{2T} \|\vec{K}\|_1.
% \end{equation}
% By a telescopic sum, we have 
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla \ell(\w_t)\|_2^2  \right] \leq  \frac{8}{\sqrt{T}}\left(\ell(\w_{0}) - \ell(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right)~,
% \end{equation}
% That completes the proof.  \qed 

% \abcomment{with the new analysis, the result is not in terms of $c \geq \alpha_t$}




% Using Lemma \ref{lemm:mix_norm}, we have
% \begin{align*}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \sum_i^d \min (\nabla_i L_S(\w_t)^2/\alpha_t^2,|\nabla_i L_S(\w_t)|/2\alpha_t  )  \right] \leq \frac{2+2\exp(\kappa_t^2/2\alpha_t^2)}{\alpha_t} \frac{1}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right)
% \end{align*}
% Since $\exp(\theta) \geq 1+ \theta + \frac{1}{2} \theta^2$ for $\theta \geq 0$ and reverse for $\theta <0$, so $\theta\exp(\theta) \geq \theta+ \theta^2 + \frac{1}{2} \theta^3$ then
% \begin{align*}
%     \theta_i(1-\exp(-2\theta_i)) \geq \theta_i - \theta_i -2 \theta_i^2 - 2\theta_i^3
% \end{align*}


\begin{lemm}\label{lemm:tanh_bound}
For any $-1\leq x\leq 1$, the following holds:
\begin{equation}
    |\tanh x|\geq \frac{e^2-1}{e^2+1}|x|
\end{equation}
\end{lemm}
\proof Without loss of generality, we focus on $0<x\leq 1$. we prove $\tanh x/ x$ is decreasing function on $\R^+$, which is equivalent to
\begin{align*}
    (\frac{\tanh x}{x})' =  \frac{x(1-\tanh^2 x) - \tanh x }{x^2}\leq 0,
\end{align*}
and is equivalent to 
\begin{align*}
    x\leq \frac{\tanh x}{1 -\tanh^2 x},
\end{align*}
where the right hand side is $\sinh x$ and use the fact that $x\leq \sinh x$ for $x > 0$ implies $\tanh x/x$ is decreasing function, so 
\begin{align*}
    \tanh x/x\geq \tanh 1 = \frac{e^2-1}{e^2 +1},
\end{align*} which completes the proof. \qed

\begin{lemm}\label{lemm:mix_norm} For any $x$,
$$|1-\exp(-2x))|\geq \min (|x|,\frac{1}{2}).$$
\end{lemm}
\proof 
Since $\exp(-x)\geq 1-x$, so we have for $x<0$:
$$1-\exp (-2x)\leq 2x\leq x.$$

For $x>0$, since $\exp x \geq 1+x$, we have $\exp -x\leq \frac{1}{1+x}$, so
$$1-\exp (-2x)\geq \frac{2x}{1+2x}.$$
Then when $\frac{1}{2}>x>0$, $$\frac{2x}{1+2x} > x,$$
and when $x\geq \frac{1}{2}$, $$\frac{2x}{1+2x} \geq \frac{1}{2},$$
which completes the proof.\qed


\theoSGLDopt*

\proof Recall that the update of SGLD is
\begin{equation}
\mathbf{w}_{t+1}=\mathbf{w}_{t}-\eta_{t} \nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)+ \sigma_{t}  \mathcal{N}\left(0, \mathbb{I}_{d}\right)~.
\end{equation}
By smoothness of the loss, taking expectation w.r.t.~the randomness of the mini-batch $B_t$ and the Gaussian draw $\g_t \sim \cN(0,\I_d)$ conditioned on $\w_{1:t}$, we have
\begin{align*}
\mathbb{E} [L_S(\w_{t+1})] &\leq L_S(\w_t) + \mathbb{E} [\left\langle \nabla L_S(\w_t), \w_{t+1} - \w_t \right\rangle ]  + \frac{K}{2} \mathbb{E} [ \|  \w_{t+1} - \w_t\|^2] \\
& =  L_S(\w_t) + \mathbb{E} [\left\langle \nabla L_S(\w_t), -\eta_t \nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right) + \sigma_t \g_t \right\rangle] + \frac{K}{2} \E[\| -\eta_t \nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right) + \sigma_t \g_t \|^2] \\
& \overset{(a)}{\leq}  L_S(\w_t) -\eta_t \|\nabla L_S(\w_t)\|^2 + \frac{K \eta_t^2}{2} \left(c_3 \kappa_t^2 + p\sigma_t^2/\eta_t^2\right)~,
\end{align*}
where (a) follows since $\E[\nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)]=0, \E[\g]=0, \E[\|\g\|^2] = p$, and $\E[\|\nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)\|^2] \leq c_3 \kappa_t^2$ for some absolute constant $c_3$ since $\nabla \ell\left(\mathbf{w}_{t}, S_{B_{t}}\right)$ is sub-Gaussian with $\psi_2$-norm $\kappa_t$.
%where $\kappa^2$ is the upper bound of the variance of $\nabla \ell(\w_{t}, S_{B_t})$.

Rearranging the above inequality and using $\alpha_t = \sigma_t/\eta_t$ we have
\begin{align} \label{eq:one_step_descend}
    \eta_t \| \nabla L_S(\w_t)\|^2 \leq  L_S(\w_t) - \mathbb{E} [L_S(\w_{t+1})]  + \frac{K \eta_k^2}{2}\left(c_3 \kappa_t^2 + p\alpha_t^2\right)~.
\end{align}
Summing over $t =1$ to $t =T$ and apply expectation over the trajectory at each step, we have
\begin{align*}
\sum_{t =1}^T \eta_t\mathbb{E}\| \nabla L_S(\w_t)\|^2 
\leq L_S(\w_1) - L_S(\w^\star) +  \sum_{t=1}^T \frac{K \eta_t^2}{2} (p \alpha_t^2 + \kappa_t^2)~,
%+\frac{(p \sigma^2 + G^2) \sum_{k=1}^T \eta_k^2}{\sum_{k=1}^T \eta_k}.  
\end{align*}
where $\w^*$ is a minima of $L_S(\w)$. With $\eta_t= \frac{1}{\sqrt{T}}$ for all $t \in [T]$, we have
\begin{align*}
\frac{1}{T} \sum_{t =1}^T \mathbb{E} \| \nabla L_S(\w_t)\|^2 
%\min_{k\in [T]} \mathbb{E} \| \nabla L_S(\w_t)\|^2
\leq\frac{L_S(\w_1) - L_S(\w^\star)}{\sqrt{T}} + \frac{  \frac{K}{2T} \sum_{t=1}^T (p \alpha_t^2 +  c_3 \kappa_t^2) }{\sqrt{T}}~.  
\end{align*}
That completes the proof.  \qed 

==> arXiv/notation.tex <==
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\htn}{\hat{\theta}_{\lambda_n}}
\newcommand{\hdn}{\hat{\Delta}_n}


%% ========================================================
\newcommand\B{\mathbb{B}}
\newcommand\E{\mathbb{E}}
\renewcommand\P{\mathbb{P}}
\newcommand\I{\mathbb{I}}
\newcommand\N{\mathbb{N}}
\newcommand\s{\mathbb{S}}
\newcommand\R{\mathbb{R}}
\newcommand\W{\mathbb{W}}
\newcommand\X{\mathbb{X}}
\newcommand\Y{\mathbb{Y}}

\newcommand\1{\mathbbm{1}}
\newcommand\0{\mathbbm{0}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

%% ========================================================
%% Some useful commands. Note the dangerous \r command!
%% ========================================================



\newcommand{\bd}{\boldsymbol}
\newcommand{\mf}{\mathbf}


\newcommand{\g}{\mathbf{g}}

\renewcommand{\a}{\mathbf{a}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\f}{\mathbf{f}}
\renewcommand{\r}{\mathbf{r}} % since \r was already defined in altex
\renewcommand{\u}{\mathbf{u}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\es}{\mathbf{s}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}




%----------------------------------------
%      THE SETS
%----------------------------------------
\newcommand{\cC}{{\cal C}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cZ}{{\cal Z}}

\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cE}{{\cal E}}


%--------------------------------------------
%         THE VARIABLES & APPROXIMATES
%--------------------------------------------

% Bold variables for vectors, matrices
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\bgg}{\mathbf{g}}

\newcommand{\bz}{\mathbf{z}}
\newcommand{\hZ}{\hat{Z}}
\newcommand{\hbZ}{\hat{\bZ}}
\newcommand{\hz}{\hat{z}}

\newcommand{\hU}{\hat{U}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}


\newcommand{\hX}{\hat{X}}
\newcommand{\hY}{\hat{Y}}
\newcommand{\hatx}{{\hat{x}}}
\newcommand{\haty}{{\hat{y}}}

%---------MISC-----------------------------

\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\BNi}{\bB_N^{(i)}}
\newcommand{\xai}{\x_i^{(a)}}
\newcommand{\yai}{\bY_i^{(i)}}
\newcommand{\Xai}{\bX_i^{(a)}}
\newcommand{\Yai}{\bY_i^{(i)}}

%\newcommand{\pr}{\mathbf{P}}
%\newcommand{\E}{\mathbf{E}}

\newcommand{\m}{\boldsymbol{\mu}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\llambda}{\boldsymbol{\lambda}}
\newcommand{\xx}{\boldsymbol{\chi}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\Eta}{\boldsymbol{\eta}}
\newcommand{\oomega}{\boldsymbol{\omega}}
\newcommand{\ppi}{\boldsymbol{\pi}}
\newcommand{\pphi}{\boldsymbol{\phi}}
\newcommand{\ggamma}{\boldsymbol{\gamma}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\aalpha}{\boldsymbol{\alpha}}
\newcommand{\eepsilon}{\boldsymbol{\epsilon}}

\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}

\newcommand{\norm}[2]{\ensuremath \|#1\|_{#2}}
\newcommand{\no}[1]{\norm{#1}{}}
\newcommand{\myref}[1]{(\ref{#1})}
\newcommand{\del}[2]{\frac{\partial #1}{\partial #2}}


%----------------------------------------------
%        NEW OPERATORS
%----------------------------------------------
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\avg}{avg}
\DeclareMathOperator{\Int}{int}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\bnd}{bd}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\ri}{ri}
\DeclareMathOperator{\co}{co}
\DeclareMathOperator{\sgn}{sign}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\discrete}{Discrete}
\DeclareMathOperator{\gam}{GAM}
\DeclareMathOperator{\uni}{Uniform}
\DeclareMathOperator{\dir}{Dir}
\DeclareMathOperator{\gaam}{GAM}
\DeclareMathOperator{\Beta}{Beta}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\gen}{gen}
\DeclareMathOperator{\lsd}{LSD}

%---------------------------------------------
% EQUATION, FIGURE, TABLE NUMBERS
%---------------------------------------------

%\renewcommand{\theequation}{\thesection.\arabic{equation}}
%\renewcommand{\thefigure}{\thesection.\arabic{figure}}
%\renewcommand{\thetable}{\thesection.\arabic{table}}
%\numberwithin{equation}{section}



%---------------------------------------------
% THEOREMS, EXAMPLES ETC.
%---------------------------------------------

% \newcounter{exampleI}
% \setcounter{exampleI}{1}
% \renewcommand{\theexampleI}{\arabic{exampleI}}

% {\theorembodyfont{\rmfamily} \theoremstyle{plain} \newtheorem{subexampleI}{Example}[exampleI]}
% \renewcommand{\thesubexampleI}{\theexampleI.\Alph{subexampleI}}

% \newcounter{exampleII}
% \setcounter{exampleII}{2}
% \renewcommand{\theexampleII}{\arabic{exampleII}}

% {\theorembodyfont{\rmfamily} \theoremstyle{plain} \newtheorem{subexampleII}{Example}[exampleII]}
% \renewcommand{\thesubexampleII}{\theexampleII.\Alph{subexampleII}}

% \newcounter{exampleIII}
% \setcounter{exampleIII}{3}
% \renewcommand{\theexampleIII}{\arabic{exampleIII}}

% {\theorembodyfont{\rmfamily} \theoremstyle{plain} \newtheorem{subexampleIII}{Example}[exampleIII]}
% \renewcommand{\thesubexampleIII}{\theexampleIII.\Alph{subexampleIII}}


%{\theorembodyfont{\rmfamily} \newtheorem{exam}{Example}}
% {\theorembodyfont{\rmfamily} \newtheorem{defn}{Definition}}
%{\theorembodyfont{\rmfamily} \newtheorem{remark}{Remark}}
\newtheorem{theo}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemm}{Lemma}
\newtheorem{corr}{Corollary}
\newtheorem{clm}{Claim}
\newtheorem{asmp}{Assumption}

\theoremstyle{definition} 
\newtheorem{exam}{Example}[section]
\newtheorem{remark}{Remark}[section]

% \newcommand{\proof}{\noindent{\itshape Proof:}\hspace*{1em}}
% \newcommand{\proofsketch}{\noindent{\itshape Proof Sketch:}\hspace*{1em}}
% \newcommand{\qed}{\nolinebreak[1]~~~\hspace*{\fill} \rule{5pt}{5pt}\vspace*{\parskip}\vspace*{1ex}}



\newcommand{\cx}{{\hat{x}}}
\newcommand{\cy}{{\hat{y}}}
\newcommand{\bp}{{\bar{p}}}
\newcommand{\eqn}[1]{(\ref{eq:#1})}
\newcommand {\commentout}[1] {}

%------------------------------------------

%%%%%%%%%%%Definitions and Macros

\def\ints{{{\rm Z} \kern -.35em {\rm Z} }}  % ints
\def\smallints{{{\rm Z} \kern -.3em {\rm Z} }}  % small ints
\def\pints{{{\rm I} \kern -.15em {\rm N} }}      % pints
\newcommand{\reals}{\mathbb R}
\newcommand{\integers}{\mathbb Z}

\newcommand{\lapn}{\lessapprox_{\,n}}
\newcommand{\gapn}{\gtrapprox_{\,n}}
\newcommand{\apn}{\approx_n}

%\def\reals{{{\rm I} \kern -.2em {\rm R} }} % reals
\newcommand{\RR}{\mathbb R}
\def\cplx{{{\rm I} \kern -.45em {\rm C} }}       % complex
\def\l2{\rm {\mathcal L}^{2}(\reals)}            % l2

\newcommand{\seqz}[2]{\mbox{$\{#1_{#2}\}$}_{#2 \in \smallints }}
\newcommand{\seqn}[2]{\mbox{$\{#1_{#2}\}$}_{#2 \in \pints }}
\renewcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\abs}[1]{\left|#1\right|}


\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}[section]
\newtheorem{nad}{Notation and Definitions}[section]
\newtheorem{notation}{Notation}[section]
%\newtheorem{remark}{Remark}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}{Claim}[theorem]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\newtheorem{conjecture}{Conjecture}
%\newtheorem{algorithm}{Algorithm}
\newtheorem{exercise}{Exercise}
\newtheorem{step}{Step}

\newcommand{\nr}{\nonumber}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}
\newcommand{\bnad}{\begin{nad}}
\newcommand{\enad}{\end{nad}}


\newcommand{\gb}{\beta_{\infty}}
\newcommand{\mgb}{\tilde{\beta}_{\infty}}
\newcommand{\gbb}{\beta_{2}}
\newcommand{\mgbb}{\tilde{\beta}_{2}}
\newcommand{\Jf}{J_{\infty}}
\newcommand{\mmJf}{\overline{J}_{\infty}}
\newcommand{\mJf}{\tilde{J}_{\infty}}
\newcommand{\Jff}{J_{2}}
\newcommand{\mJff}{\tilde{J}_{2}}
\newcommand{\Jc}{{\calJ_{\infty}}}
\newcommand{\mJc}{{\tilde{\calJ}_{\infty}}}
\newcommand{\Jcc}{{\calJ_{2}}}
\newcommand{\ptq}{P_{3 \overline{Q}}}
\newcommand{\pq}{P_{Q}}


\newcommand{\di}{{\,\mathrm{d}}}
\newcommand{\latop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}


%\newcommand{\Th}[1]{Theorem~\ref{#1}} % when starting a sentence
%\renewcommand{\th}[1]{Theorem~\ref{#1}}
%\newcommand{\ths}[2]{Theorems~\ref{#1} and~\ref{#2}}
%\newcommand{\thst}[2]{Theorems~\ref{#1}-\ref{#2}}
%\newcommand{\lem}[1]{Lemma~\ref{#1}}
%\newcommand{\prop}[1]{Proposition~\ref{#1}}
%\newcommand{\defin}[1]{Definition~\ref{#1}}
%\newcommand{\eq}[1]{equation~(\ref{#1})}
%\newcommand{\ineq}[1]{inequality~(\ref{#1})}
%\newcommand{\Ineq}[1]{Inequality~(\ref{#1})}
%\newcommand{\ineqs}[2]{inequalities~(\ref{#1}) and~(\ref{#2})}
%\newcommand{\Eq}[1]{Equation~(\ref{#1})}
%\newcommand{\eqs}[2]{equations~(\ref{#1}) and~(\ref{#2})}
%\newcommand{\eqss}[3]{equations~(\ref{#1}), (\ref{#2}) and~(\ref{#3})}
%\newcommand{\eqst}[2]{equations~(\ref{#1})-(\ref{#2})}
%\newcommand{\sect}[1]{Section~\ref{#1}}
%\newcommand{\subsect}[1]{Subsection~\ref{#1}}

\newcommand{\lip}{\langle}
\newcommand{\rip}{\rangle}
\newcommand{\uu}{\underline}
\newcommand{\oo}{\overline}
\newcommand{\La}{\Lambda}
\newcommand{\la}{\lambda}
%\newcommand{\eps}{\epsilon}
\newcommand{\eps}{\varepsilon}
\newcommand{\veps}{\varepsilon}
\newcommand{\rmT}{{\rm T}}
\newcommand{\rmW}{{\rm W}}
\newcommand{\Ga}{\Gamma}

\newcommand{\sign}{{\mbox{\rm sign}}}
\newcommand{\ang}{{\mbox{\rm ang}}}
%\newcommand{\supp}{{\mbox{\rm supp}}}
\newcommand{\dist}{{\mbox{\rm dist}}}

\newcommand{\nin}{\in\!\!\!\!\!/\,}

\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\tcD}{{\tilde{\cal D}}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}

\newcommand{\RE}{{\cal R}e}
%\newcommand{\IM}{{\cal I}m}


\newcommand{\Prob}{{\rm Prob\,}}
\newcommand{\diam}{{\rm diam\,}}
\renewcommand{\mod}{{\rm mod\,}}
\newcommand{\sinc}{{\rm sinc\,}}
\newcommand{\ctg}{{\rm ctg\,}}
\newcommand{\ifff}{\mbox{\ if and only if\ }}
%\newcommand{\proof}{\noindent {\bf Proof:\ }}

%\renewcommand{\bar}{\overline}
\renewcommand{\overline}{\bar}
%\renewcommand{\tilde}{\widetilde}
\renewcommand{\widetilde}{\tilde}
%\renewcommand{\ell}{l}
%\renewcommand{\hat}{\widehat}
\renewcommand{\widehat}{\hat}


\newcommand{\boldx}{{\bf x}}
\newcommand{\boldX}{{\bf X}}
\newcommand{\boldy}{{\bf y}}
\newcommand{\indic}{{\large \bf 1}}
\newcommand{\uux}{\uu{x}}
\newcommand{\uuY}{\uu{Y}}

\newcommand{\opt}{\rm{opt}}


%fraction with round brackets
\newcommand{\ffrac}[2]
  {\left( \frac{#1}{#2} \right)}

\newcommand{\one}{\frac{1}{n}\:}
\newcommand{\half}{\frac{1}{2}\:}


\newcommand{\BAMS}{{\em Bulletin of the Amer. Math. Soc.}}
\newcommand{\TAMS}{{\em Transactions of the Amer. Math. Soc.}}
\newcommand{\PAMS}{{\em Proceedings of the Amer. Math. Soc.}}
\newcommand{\JAMS}{{\em Journal of the Amer. Math. Soc.}}
\newcommand{\LNM}{{\em Lect. Notes in Math.}}
\newcommand{\LNCS}{{\em Lect. Notes in Comp. Sci.}}
\newcommand{\IV}{{\em Invent. Math.}}
\newcommand{\JAM}{{\em J. Anal. Math.}}
\newcommand{\Sc}{{\em Science}}


==> arXiv/sec/conc.tex <==
\vspace*{-2mm}
Inspired by recent advances in stability based and information theoretic approaches to generalization bounds \citep{mou2018generalization,pensia2018generalization,negrea2019information,Li2020On,haghifam2020sharpened}, we have presented a framework for developing such bounds based on expected stability for noisy stochastic iterative learning algorithms. We have also introduced Exponential Family Langevin Dynamics (EFLD), a large family of noisy gradient descent algorithms based on exponential family noise, which includes SGLD and Noisy Sign-SGD as two special cases.  We have developed an expected stability based generalization bound applicable to any EFLD algorithm with a $O({1}/{n})$ sample dependence and a dependence on gradient incoherence, rather than gradient norms. Further, we have provided optimization guarantees for special cases of EFLD, viz.~Noisy Sign-SGD and SGLD. Our experiments on various benchmarks illustrate that our bounds are non-vacuous and quantitatively much sharper than existing bounds~\citep{Li2020On,negrea2019information}. 


%Further, we have simplified the task to one of bounding expected for the NSI algorithm. We have developed a specific bound for SGD with Gaussian noise which inherits strengths of a variety of existing results and quantitatively outperforms them based on preliminary experiments. We have also developed similar bounds for SGD with exponential family noise, which seem to be the first result of this type. Our work also highlights few key directions for future work, including sharper notions of gradient discrepancy/incoherence and better understanding of the trade-offs between stability and optimization for NSI algorithms.

==> arXiv/sec/efld.tex <==
%\vspace*{-2mm} 

In recent years, considerable advances have been made in establishing generalization bounds for stochastic gradient Langevin dynamics (SGLD) \citep{Li2020On, pensia2018generalization, negrea2019information, haghifam2020sharpened}. As an example of a nosiy stochastic iterative algorithm of the form~\eqref{eq:nmia}, SGLD adds isotropic Gaussian noise at every step of SGD:
%\begin{align}\label{eq:sgld}
 $\w_{t+1} = \w_{t} - \eta_t \nabla \ell(\w_t, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right)$,
%\end{align}
where $ \nabla \ell(\w_t, S_{B_t})$ is the stochastic gradient on mini-batch $B_t$, $\eta_t$ is the step size, and $\sigma_t^2$ is noise vairance. 


In this paper, we introduce a substantial generalization of SGLD called Exponential Family Langevin Dynamics (EFLD) which uses general exponential family noise in noisy iterative updates of the form~\eqref{eq:nmia}. 
In addition to being a mathematical generalization of the popular SGLD, the proposed EFLD provides flexibility to use noisy gradient algorithms with different representation of the gradient, e.g., Bernoulli noise for Sign-SGD, discrete distribution for quantized or finite precision SGD, etc. \citep{canonne2020discrete, quantized-sgd, jiang2018, yang2019swalp}.
%\abbcomment{pls add more cites}\yzcomment{done}\abcomment{great, pls drop one to prevent spill over to new line}.

\subsection{Exponential Family Langevin Dynamics (EFLD)}\label{subsec:efld}


Exponential families \citep{barndorff2014information,brown1986fundamentals,wainwright2008graphical} constitute a large family of parametric distributions which include Gaussian, Bernoulli, gamma, Poisson, Dirichlet, etc., as special cases. Exponential families are typically represented in terms of natural parameters $\btheta$, and we consider component-wise independent distributions with scaled natural parameter $\btheta_{\alpha} = \btheta/\alpha$ with scaling $\alpha > 0$, i.e.,
\vspace{-2mm}
\begin{align*}
\vspace{-3mm}
p_{\psi}(\bxi, \btheta_{\alpha}) = \exp(\langle \bxi, \btheta_{\alpha} \rangle - \psi(\btheta_{\alpha})) \ppi_{0,\alpha}(\bxi) = \prod_{j=1}^p \exp( \xi_j \theta_{j\alpha} - \psi_j(\theta_{j\alpha})) \pi_{0,\alpha}(\xi_j)~,
\vspace*{-2mm}
\end{align*}
where $\bxi \in \R^p$ is the sufficient statistic, $\psi(\btheta_{\alpha})= \sum_{j=1}^p \psi_j(\theta_{j\alpha})$ is the log-partition function, and $\ppi_{0,\alpha}(\xi) = \prod_{j=1}^p \pi_{0,\alpha}(\xi_j)$ is the base measure. Note that $\alpha=1$ gives the canonical form of the exponential family distributions. For general scaling $\alpha > 0$, for certain distributions the base measure $\pi_0$  may depend on the scaling, i.e., $\pi_{0,\alpha}$. A scaling $\alpha >0$ is valid as long as $\exp(\langle \bxi,\btheta_{\alpha} \rangle)$ is integrable, i.e., $\int_{\bxi} \exp(\langle \bxi,\btheta_{\alpha} \rangle \pi_{0,\alpha}(\bxi) d\bxi < \infty$. Further, $\psi$ is a smooth function by construction \citep{barndorff2014information,banerjee2005clustering,wainwright2008graphical} and the smoothness of $\psi$ implies $\nabla_{\btheta_\alpha}^2 \psi(\btheta_{\alpha}) \leq c_2 \I$ for some constant $c_2 > 0$. 
%\abcomment{briefly explain why $\psi$ is smooth, in the appendix} 


Exponential family Langevin dynamics (EFLD) uses noisy stochastic gradient updates similar to SGLD, but using exponential family noise rather than Gaussian noise as in SGLD. In particular, for mini-batch $S_{B_t}$, EFLD updates are as follows: with step size $\rho_t > 0$
\begin{equation}
    \w_t = \w_{t-1} - \rho_t \bxi_t~, \qquad \bxi_t \sim p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})~,
\vspace{-2mm}    
\label{eq:efld1}
\end{equation}
where 
\vspace*{-2mm}
\begin{equation}
p_{\psi}(\bxi; \btheta_{B_t,\alpha_t}) = \exp(\langle \bxi, \btheta_{B_t,\alpha_t} \rangle - \psi(\btheta_{B_t,\alpha_t})) \ppi_{0,\alpha}(\bxi)   ~, \qquad \btheta_{B_t,\alpha_t} \triangleq \frac{\btheta_{B_t}}{\alpha_t} = \frac{\nabla \ell(\w_{t-1}, S_{B_t})}{\alpha_t}~.
\label{eq:efld2}
\vspace*{-1mm}
\end{equation}
For EFLD, the natural parameter $\btheta_{B_t,\alpha_t}$ at step $t$ is simply a scaled version of the mini-batch gradient $\nabla \ell(\w_{t-1}, S_{B_t})$. We first show that EFLD becomes SGLD when the exponential family is Gaussian, and becomes a noisy version of sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise} when the exponential family is Bernoulli over $\{-1,+1\}$. More details and examples are in Appendix \ref{app:example}.
% \abdelete{\yzedit{Similarly, for EFLD with neighboring dataset $S'_n$, we write  $\btheta_{B'_t,\alpha_t} \triangleq \frac{\btheta_{B_t}}{\alpha_t} = \frac{\nabla \ell(\w_{t-1}, S'_{B_t})}{\alpha_t}$ as the natural parameter for distribution $p_{\psi}(\bxi; \btheta_{B'_t,\alpha_t})$, where $S'_{B_t}$ is the mini-batch sampled from $S'_n$. }
% As examples we first show that EFLD becomes SGLD when the exponential family is Gaussian, and then show that we get a noisy version of sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise} when the exponential family is Bernoulli over $\{-1,+1\}$. For the details of properties of examples, we refer to Appendix \ref{app:example}.}
\begin{exam}[SGLD] 
% \abbcomment{Example is incorrect -- in terms of choice of $\rho_t, \alpha_t$}
% \abcomment{just keep the part showing this is a special case of EFLD}\tccomment{Updated.}\abcomment{updated}
% \abccomment{For multi-variate Gaussians with fixed covariance $\sigma^2\I$, the scaling $\alpha = \sigma$, the sufficient statistic $\bxi = \x/\sigma$, the log-partition function  $\psi(\btheta) = \|\btheta\|_2^2/2$, and the base measure $\pi_0(\bxi) = \frac{1}{(\sqrt{2\pi)^d}} \exp(-\|\bxi\|_2 ^2/2)$ or equivalently $\pi_0(\x) = \frac{1}{\sqrt{(2\pi)^d}\sigma^d} \exp(-\|\x\|_2^2/2\sigma^2)$ using $\bxi = \x/\sigma$ and $d\bxi = d\x/\sigma$. The scaled parameter $\btheta_{\alpha} = \btheta_{\sigma} = \btheta/\sigma$. Then, the distribution from the natural parameter form is:
% \begin{equation}
%     p_{\btheta/\sigma}(\x) = \exp( \langle \x, \btheta\rangle / \sigma^2 - \|\btheta\|_2^2/(2\sigma^2) ) \times \frac{1}{\sqrt{(2\pi)^d}\sigma^d} \exp(-\|\x\|_2^2/2\sigma^2)
%     = \frac{1}{\sqrt{(2\pi)^d}\sigma^d} \exp(-\|\x-\btheta\|_2^2/2\sigma^2).
% \end{equation}}

% \tcdelete{SGLD uses scaled Gaussian noise with $\psi(\btheta)= \|\btheta\|_2^2/2, \alpha_t = \sqrt{\sigma_t/\eta_t}$, so that $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t}) = \mathcal{N}(\btheta_{B_t}, \alpha_t^2 \I_d)$. By taking $\rho_t = \sqrt{\eta_t\sigma_t}$, the update \eqref{eq:efld1} based on $\rho_t \bxi_t$ is distributed as $\mathcal{N}(\rho_t\btheta_{B_t}, \rho_t^2\alpha_t^2 \I_d) = \mathcal{N}(\eta_t\nabla \ell(\w_{t-1}, S_{B_t}), \sigma_t^2 \I_d)$. Thus the EFLD update reduces to the SGLD update: $\w_{t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1}, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right).$
% \qed}

SGLD uses scaled Gaussian noise with $\psi(\btheta)= \|\btheta\|_2^2/2, \alpha_t = \sigma_t/\eta_t$, %\tcedit{$\bxi = \x/\alpha_t,~\pi_0(\bxi) = \frac{1}{\sqrt{(2\pi)^d}} 
$\ppi_{0,\alpha_t}(\bxi) = \frac{1}{\sqrt{(2\pi)^p \alpha_t^p}} \exp(-\|\bxi\|_2^2/2\alpha_t^2)$ so that $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t}) = \mathcal{N}(\btheta_{B_t}, \alpha_t^2 \I_d)$. By taking $\rho_t = \eta_t$, the update \eqref{eq:efld1} based on $\rho_t \bxi_t$ is distributed as $\mathcal{N}(\eta_t \btheta_{B_t}, \eta_t^2 \alpha_t^2 \I_d) = \mathcal{N}(\eta_t\nabla \ell(\w_{t-1}, S_{B_t}), \sigma_t^2 \I_d)$. Thus the EFLD update reduces to the SGLD update: $\w_{t} = \w_{t-1} - \eta_t \nabla \ell(\w_{t-1}, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right).$
\label{exam:sgld}
\qed 


% \abccomment{By taking $\rho_t = \sqrt{\eta_t\sigma_t},~\alpha_t = \sqrt{\sigma_t/\eta_t},~ \psi(\btheta)= \|\btheta\|_2^2/2,~ \bxi = \x/\alpha_t,~\pi_0(\bxi) = \frac{1}{\sqrt{(2\pi)^d}} \exp(-\|\bxi\|_2 ^2/2)$ in exponential family update equation \eqref{eq:efld1}, the exponential family distribution $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ becomes
% \begin{align*}
%     p_{\btheta_{B_t,\alpha_t}}(\x) = \exp( \langle \x, \btheta_{B_t}\rangle / \alpha_t ^2 - \|\btheta_{B_t}\|_2^2/(2\alpha_t^2) )  \frac{1}{\sqrt{(2\pi)^d}\alpha_t^d} \exp(-\|\x\|_2^2/2\alpha_t^2)
%     = \frac{1}{\sqrt{(2\pi)^d}\alpha_t^d} \exp(-\|\x-\btheta_{B_t}\|_2^2/2\alpha_t^2),
% \end{align*}
% which is a normal distribution $\mathcal{N}(\btheta_{B_t}, \alpha_t^2 \I_d)$, by scaling $\rho_t$ it becomes $\mathcal{N}(\rho_t\btheta_{B_t}, \rho_t^2\alpha_t^2 \I_d)$ which is $\mathcal{N}(\eta_t\nabla \ell(\w_{t-1}, S_{B_t}), \sigma_t^2 \I_d)$. Thus the EFLD update reduces to the SGLD update:
% $\w_{t+1} = \w_{t} - \eta_t \nabla \ell(\w_t, S_{B_t}) + \mathcal{N}\left(0, \sigma_t^2 \mathbb{I}_{d}\right).$
% \qed}
\end{exam}

\begin{exam}[Noisy Sign-SGD]
\label{exam:noisy_signsgd}
%\abcomment{just keep the part showing this is a special case of EFLD}\tccomment{Updated.}
By taking $\rho_t = \eta_t$ and componentwise $\xi_j \in\{-1,1\},~\pi_{0,\alpha_t}(\xi_j)=1,~\psi(\theta) = \log(\exp(-\theta)+\exp(\theta))$ in exponential family update equation \eqref{eq:efld1}, the $j$-th component of exponential family distribution $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ becomes
$p_{\psi}(\xi_j; \btheta_{B_t,\alpha_t})  = \frac{\exp(\xi_j \btheta_{B_t,\alpha_t})}{\exp(-\btheta_{B_t,\alpha_t})+\exp(\btheta_{B_t,\alpha_t})}$.
%\begin{align*}
    % p_{\btheta_{B_t,\alpha_t,j}}(\xi) = \exp(x\btheta_{B_t,\alpha_t,j} - \log(\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j}))) = \frac{\exp(x\btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})}.
%\end{align*}
Thus, the EFLD update reduces to a noisy version of Sign-SGD: 
$\w_{t} = \w_{t-1} - \eta_t \bxi_t$, $\bxi_{t,j} \sim p_{\psi}(\xi_j,\btheta_{B_t,\alpha_t})$, 
% \begin{equation}\label{eq:signSGD_mini_batch_1}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, ~\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(x) =  \frac{\exp(x \btheta_{B_t,\alpha_t,j})}{\exp(-\btheta_{B_t,\alpha_t,j})+\exp(\btheta_{B_t,\alpha_t,j})},~ x\in\{-1,+1\}
% \end{equation}
$j\in [p]$, where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
% for mini-batch $B_t$ and scaling $\alpha_t$, mini-batch noisy sign-SGD updates the parameters as
% \begin{equation}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, \qquad \bxi_{t,i} \sim p_{\alpha_t}(\xi) =  \left(\frac{1}{0.5+\exp(-\theta_{B_t,\alpha_t})}\right)^{\frac{1+\xi}{2}} \left(\frac{1-\mu_\alpha}{2}\right)^{\frac{1-\xi}{2}}   ~, ~ \forall i\in [d],
% \end{equation}
\qed
\end{exam}

% \begin{remark}
% \abcomment{briefly explain why absolute continuity is not being violated for the Bernoulli, and more general discrete cases}
% \end{remark}



\subsection{Expected Stability of Exponential Family Langevin Dynamics}
\input{arXiv/sec/stability}



\subsection{Optimization Guarantees for EFLD}

We now establish optimization guarantees for two examples of EFLD, i.e., Noisy Sign-SGD with Bernoulli noise over $\{-1,+1\}$ and SGLD with Gaussian noise.  

\noindent {\bf Noisy Sign-SGD.}
\tcedit{From Example~\ref{exam:noisy_signsgd} in Section \ref{subsec:efld} for noisy sign-SGD,}
% We first provide a optimization guarantees for Noisy sign-SGD under both full-batch and mini-batch settings. Focusing on the natural parameter form, the full-batch Noisy Sign-SGD update the parameters as
% \begin{equation}\label{eq:signSGD_full_batch}
%     \w_{t+1} = \w_{t} - \eta_t \bxi_t~, ~ \bxi_{t,i} \sim p_{\alpha_t}(\xi) =  \frac{1}{\exp((1-\xi)\nabla L_S(\w_t)/\alpha_t)+\exp((-1-\xi)\nabla L_S(\w_t)/\alpha_t)}~, ~ \xi\in\{-1,+1\}
% \end{equation}
% for any $i\in [d]$.
for mini-batch $B_t$ and scaling $\alpha_t$, mini-batch Noisy Sign-SGD updates the parameters as $\w_{t} = \w_{t-1} - \eta_t \bxi_t$, 
%\abbcomment{step size is $\rho_t$, please be consistent, see Section 4.1}\tccomment{Update pointer to example} 
where each component $j\in [p]$ 
\begin{equation}\label{eq:signSGD_mini_batch}
\bxi_{t,j} \sim p_{\btheta_{B_t,\alpha_t,j}}(\xi_j) =  \frac{\exp(\xi_j \btheta_{B_t,\alpha_t})}{\exp(-\btheta_{B_t,\alpha_t})+\exp(\btheta_{B_t,\alpha_t})},~ \xi_j\in\{-1,+1\}
\end{equation}
where $\btheta_{B_t,\alpha_t} = \nabla \ell(\w_{t-1}, S_{B_t})/\alpha_t$ is the scaled mini-batch gradient.
The full-batch version uses parameters $\E_{B_t}[\btheta_{B_t,\alpha_t}] = \nabla L_S(\w_{t-1})$.
% Here we consider the special case of Bernoulli distribution. Thus
% $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t})$ is the probability distribution $B(\frac{1}{1+\exp(-\btheta_{B_t,\alpha_t})})$
For the optimization analysis for full batch gradient descent, we assume that the loss is smooth.
%of the empirical loss function $L_S(\w)$:
\begin{restatable}{asmp}{asmpsmooth}\label{asmp: smooth}
The loss function $L_S(\w) = \frac{1}{n} \sum_{i=1}^n \ell(\w,z_i)$ 
%\abbcomment{how is $L_S$ related to $\ell$? Please see earlier sections}\tccomment{here the assumption is on the full batch loss $L_S(\w)$, Assumption 2 is about the statistical properties of mini-batch loss. Here notation is used from the notation section above equation (1): "the population and empirical loss are respectively given by $L_D(\w) \triangleq \E_{z \sim D}[\ell(\w,z)]$, and $L_S(\w) \triangleq \frac{1}{n} \sum_{i=1}^n \ell(\w,z_i)$.  "} 
satisfies: $\forall \w, \w^\prime$, for some non-negative constants $\vec{K}:=\left[K_{1}, \ldots, K_{p}\right]$, we have
%\begin{align}
$L_S(\w) \leq L_S(\w^\prime) + \nabla L_S(\w^\prime)^T(\w - \w^\prime) + \frac{1}{2} \sum_{i} K_i (w_i - w^\prime_i)^2$. 
\vspace*{-1mm}
\end{restatable}
% The assumption on the empirical loss $L_S(\w)$ is common in optimization analysis [Bernstein's][][], besides that, we also assume some natural statistical properties of the batch gradient of the loss $\nabla \ell(\w_{t}, S_{B_t})$, where the randomness comes from batches conditioned on $\w_t$, satisfies the following assumptions:
For the mini-batch analysis, we additionally assume that the mini-batch gradients are unbiased, symmetric, and sub-Gaussian.
\begin{restatable}{asmp}{asmpbatch}\label{asmp:batch}
Given $\w_{t-1}$, the mini-batch gradient $\nabla \ell(\w_{t-1}, S_{B_t})$ is
\begin{enumerate}[(a)]
\item  unbiased,  i.e., $\E_{B_t|\w_{t-1}}\nabla \ell(\w_{t-1}, S_{B_t}) = \nabla L_S(\w_{t-1})$; \abbcomment{what is the relation between $L_S$ in Assumption 1 and $\ell$ in earlier sections} \abbcomment{Does `unbiased' not follow from the definition -- as finite sum average? why not?}\tccomment{Unbiased is followed when batch is taken uniformly, we can remove the assumption if it's too standard} \abbcomment{this is standard, let's remove}
%\abbcomment{notation not consistent}\tccomment{Switch $\cL$ to $L$, use $K$ for Lipschitz constants}; 
\item symmetric, i.e., the density $p_{B_t|\w_{t-1}}(\bxi)$ of $\bxi \equiv \nabla \ell(\w_{t-1}, S_{B_{t}})$ is symmetric \abbcomment{does this not follows from the finite sum/average definition? why not?}\tccomment{it might not, imagine we uniformly sample from $-1,-1,2$ with batch size 1, it's mean zero and density of 2 is 1/3 while density of -2 is 0, the dataset is not symmetric.} around its expectation $L_S(\w_{t-1})$: $p_{B_t|\w_{t-1}}(\bxi) = p_{B_t|\w_{t-1}}(2\nabla L_S(\w_{t-1})-\bxi)$; \abbcomment{what is $x$? why are we not using $\xi$ as before?} \tccomment{$x$ is the density of $\nabla \ell(\w_{t-1}, S_{B_{t}})$ in (15) which is a bit different from the $\xi$ in (15). Notations changed}
and 
\item sub-Gaussian, i.e., for any $\lambda >0$, {any $\v$ s.t. $\|\v\|_2 =1$}, \begin{align*}
\E_{B_t|\w_{t-1}}[\exp \lambda\langle \v,\nabla \ell(\w_{t-1}, S_{B_{t}})-\nabla  L_S(\w_{t-1})\rangle] \leq \exp(\lambda^2\kappa_t^2/2)~,
\end{align*}
for some constant $\kappa_t > 0$.\abcomment{will be good if we can say more about $\kappa_t$, e.g., see recent work by Tengyu Ma et al., and others on SGD noise} \tccomment{See below discussions.}
\end{enumerate}
%\end{itemize}
%[Batch Gradient] 
% Given $\w_{t-1}$, the mini-batch gradient $\nabla \ell(\w_t, S_{B_t})$ is
% \begin{itemize}
% \item (Unbiased)  The mini-batch gradient $\nabla \ell(\w_{t}, S_{{B_t}})$ is an unbiased estimator of true gradient $L_S(\w_{t})$: $\E_{B_t|\w_t}\nabla \ell(\w_{t}, S_{B_t}) = \nabla L_S(\w_{t}).$
%     \item (Symmetricity) The pdf $p_{BG}(x)$ of mini-batch gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is symmetric around its expectation $L_S(\w_{t})$: $p_{BG}(x) = p_{BG}(2\nabla L_S(\w_{t})-x).$
%     \item (Sub-Gaussian) The mini-batch gradient $\nabla \ell(\w_{t}, S_{B_{t}})$ is Sub-Gaussian with $\psi_2$ norm $\kappa$: for any $\lambda >0$, $v\in S^{d-1}$, we have $\E_{B_t|\w_t}\exp \lambda\langle v,\nabla \ell(\w_{t}, S_{B_{t}})-\nabla L_S(\w_{t})\rangle \leq \exp(\lambda^2\kappa^2/2).$
% \end{itemize}
\vspace{-2mm}
\end{restatable}
%With Assumption \ref{asmp: smooth} and Assumption \ref{asmp:batch}, we have the following guarantee for convergence of noisy signSGD under full batch and mini batch settings:
\tcedit{The smoothness assumption in Assumption \ref{asmp: smooth} is standard in non-convex optimization especially for sign-SGD literature \citep{bernstein2018signsgd,bernstein2018signsgdnoise}. Assumption \ref{asmp:batch} for the mini-batch setting helps the theoretical analysis, where (a) is satisfied when the batches $S_{B_t}$ are taken uniformly from samples $S$ as the standard training does; (b) assumes symmetry of the mini-batch gradients; and (c) is similar and stronger assumption compared to Assumption 3 in \cite{bernstein2018signsgd}, where they assume bounded variance for stochastic gradient and our assumption implies suitably bounded higher moments of $\nabla \ell(\w_{t-1}, S_{B_{t}})-\nabla  L_S(\w_{t-1})$, which is referred as the minibatch noise in recent noisy SGD literature e.g. \cite{damian2021label}. 
Similar to such literature, if we consider mini-batch stochastic gradient be modeled
as the average of $|B_t|$ calls to the full-batch gradient, from the Hoeffding's inequality for bounded variables, $\kappa_t$ is scaled by $1/\sqrt{|B_t|}$.} \abbcomment{this is a bit unclear}

Based on the assumptions, we have the following optimization guarantee for full-batch and mini-batch noisy Sign-SGD. 
%We defer the optimization guarantee for full-batch Noisy Sign-SGD to Appendix \ref{app:opt}. %\tccomment{Full-batch drops to appendix}



% \begin{restatable}{theo}{theosignSGDconv}\label{theo:signSGD_conv}
% Under Assumptions~\ref{asmp: smooth} and \ref{asmp:batch}, for mini-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$, 
% $\alpha_t$ satisfying $c \geq \alpha_t \geq \max[\sqrt{2}\kappa_t, 4\|\nabla L_S(\w_{t-1})\|_{\infty}]$, we have for any $S$ and any initialization $\w_0$
% \vspace{-2mm}
% \begin{equation}\label{eq:sign_SGD_mini_batch_convergence}
% \vspace{-1mm}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
% \end{equation}
% \abbcomment{what is $L_S$, see earlier comments}
% where the expectation is taken over the randomness of  algorithm.
% \vspace{-2mm}
% \end{restatable}

\begin{restatable}{theo}{theosignSGDconv}\label{theo:signSGD}
If the loss satisfies Assumption~\ref{asmp: smooth}, for full-batch noisy Sign-SGD with step size $\rho_t = 1/\sqrt{T}$ and $\alpha_t$ satisfying $c\geq \alpha_t \geq \|\nabla L_S(\w_t)\|_{\infty}$, we have
\begin{equation}\label{eq:sign_SGD_full_batch_convergence_1}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2\right] \leq \frac{5c}{3\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right).
\end{equation}
Further, if Assumption~\ref{asmp:batch} holds, for mini-batch noisy Sign-SGD with step size $\eta_t = 1/\sqrt{T}$, and 
% $\alpha_t = 2G$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4G (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% or choose $c\geq\alpha_t\geq 2G$, we have
% \begin{equation}
%     \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{2c (1+\exp(\frac{\kappa^2}{8T G^2}))}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{L}\|_1\right).
% \end{equation}
% or without assuming $G$, 
$\alpha_t$ satisfying $c \geq \alpha_t \geq \max[\sqrt{2}\kappa_t, 4\|\nabla L_S(\w_t)\|_{\infty}]$, we have
\begin{equation}\label{eq:sign_SGD_mini_batch_convergence_1}
    \E\left[\frac{1}{T}\sum_{t=1}^T \|\nabla L_S(\w_t)\|_2^2  \right] \leq  \frac{4c}{\sqrt{T}}\left(L_S(\w_{0}) - L_S(\w^*) + \frac{1}{2}\|\vec{K}\|_1\right),
\end{equation}
where equation \eqref{eq:sign_SGD_full_batch_convergence_1}\eqref{eq:sign_SGD_mini_batch_convergence_1} holds for any $S$, any initialization $\w_0$, and the expectation is taken over the randomness of  algorithm.
\end{restatable}

% \abcomment{add as remark or drop (space limit)} Theorem \ref{theo:signSGD_conv} shows the convergence rate for noisy-signSGD update is $O\left(\frac{1}{\sqrt{T}}\right)$ which matches the same rate as the noiseless signSGD in \cite{bernstein2018signsgd}.


% \begin{asmp} \label{asmp: sample_lip}
% The loss function $\ell(\w,z)$ is:\vspace*{-2mm}
% \begin{enumerate}
%     \item Bounded, i.e., $\forall \w, z, \ell(\w,z) \leq c_0$; and
%     \item Sample-Lipschitz, i.e., 
%     \begin{equation}
%       \forall z, z', \w  \quad \| \nabla f(\w,z) - \nabla f(\w,z') \| \leq L~.
%       \vspace*{-2mm}
%     \end{equation}
% \end{enumerate}
% \end{asmp}
% Note the Sample-Lipschitz property follows if the gradients $\nabla \ell(\w,z)$ are bounded, i.e., $\ell$ is Lipshitz. Further, the norm $\| \cdot \|$ can be viewed as the $L_2$ norm for now.

\noindent {\bf Stochastic Gradient Langevin Dynamics (SGLD).} We acknowledge that the following optimization result for SGLD exists in various forms, as noisy gradient descent algorithms with Gaussian noise have been studied in literature such as differential privacy, where SGLD can be viewed as DP-SGD  \citep{bassily2014private, wang2019differentially} and the proof technique boils down to bounding the stochastic variance of the noisy gradient \citep{shamir2013stochastic}.
%\abcomment{ack that this result exists in various forms, is not new}
\begin{restatable}{theo}{theoSGLDopt}
Under Assumptions \ref{asmp: smooth} and \ref{asmp:batch} with $K_i = K, \forall i \in [p]$, for any training set $S$, SGLD, i.e., EFLD with Gaussian noise, $\rho_t = \eta_t$, $\alpha_t = \sigma_t/\eta_t$), batch size $|B_t| = b$, and step size $\eta_t = \frac{1}{\sqrt{T}}$ satisfies 
\begin{align}
\vspace{-2mm}
\frac{1}{T} \sum_{t =1}^T \mathbb{E} \| \nabla L_S(\w_t)\|^2 
%\min_{k\in [T]} \mathbb{E} \| \nabla L_S(\w_t)\|^2
\leq \frac{L_S(\w_1) - L_S(\w^*)}{\sqrt{T}} + \frac{  \frac{K}{2T} \sum_{t=1}^T (p \alpha_t^2 +  c_3 \kappa_t^2) }{\sqrt{T}}~,
\end{align}
where $\w_1$ are the initial parameters, $\w^*$ is a minima of $L_S(\w)$, $c_3$ is an absolute constant, and the expectation is over the randomness of the algorithm.
%\vspace*{-2mm}
\end{restatable}
%\yzcomment{will add a comment here} \yzcomment{done}
%SGLD also converges with the rate of $O(1/\sqrt{T})$ which is the same as SGD for non-convex and smooth problems. 
The error rate of SGLD depends on the noise level $\alpha_t$ and the sub-Gaussian parameter $\kappa_rt$.  The bound has a $O(1/\sqrt{T})$ rate as long as the average noise level and sub-Gaussian parameter are bounded by a constant. 
%One can choose a decaying noise variance such as  $\alpha_t = 1/\sqrt[2]{t}$ to guarantee the convergence. Then the rate will become $O(\log T/\sqrt{T})$ as long as the average sub-Gaussian norms, i.e., $\frac{1}{T}\sum_t \kappa_t^2$ bounded by a constant. 
We note that similar to the optimization guarantees of differentially private SGD, the convergence rate depends on the dimension of the gradient $p$ due to the isotropic Gaussian noise. \abbcomment{we have discussed this -- if we show stability results for the general anisotropic case, the result can be updated with $\tr$ of covariance. We can anyway do that} Special noise structures such as anisotropic noise that align with the gradient structure can improve the dependence on dimension \citep{kairouz2020dimension,zhang2021wide,asi2021private, zhou2020bypassing}.  




\abccomment{for each result, we have to say exactly which appendix has the proof}



==> arXiv/sec/exp.tex <==
%\vspace*{-2mm}
\begin{figure*}[t] 
\centering
\subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-c-new.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-c-new.png}
 }
\subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-c-new.png}
 } 
 \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-c-new.png}
 } \vspace*{-3mm}
 \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-b-new.png}
 } 
 \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-b-new.png}
 }
\subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-b-new.png}
 } 
 \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-b-new.png}
 }\vspace*{-1mm}
  \subfigure[MNIST, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-5000.0-a-new.png}
 } 
  \subfigure[CIFAR-10, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-cifar10-bounds-beta-5000.0-a-new.png}
 }
  \subfigure[Fashion, $\alpha_t^2 \approx 0.1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-5000.0-a-new.png}
 } 
  \subfigure[Fashion, $\alpha_t^2 \approx 0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-beta-55000.0-a-new.png}
 }
\vspace*{-2mm}
\caption[]{Results for training CNN using SGLD %($\sigma_t = \sqrt{2\eta_t/\beta_t}$) 
on MNIST, Fashion-MNIST and CIFAR-10. X-axis shows the number of training epochs. (a)-(d) shows our bound is non-vacuous and can be used to bound the empirical test error. (e)-(h) compare our bound with the existing bounds and show the effect on $\alpha_t^2$. Our bounds are numerically sharper than existing bounds, and larger $\alpha_t^2$ leads to tighter generalization bounds which is consistent with the theoretical analysis. (i)-(l) show the key factors in each bound, i.e., the squared gradient norm in \cite{Li2020On}, the gradient incoherence in \cite{negrea2019information}, the two-sample incoherence in \cite{rodriguez2021random}, and the gradient discrepancy in our bound. Incoherence or discrepancy based quantities are orders of magnitude smaller than the gradient norm. 
}
%\vspace*{-3mm}
\label{fig:sgld_bound}
\end{figure*}


% In this section, we conduct a series of experiments to evaluate our generalization error bounds. For SGLD, we aim to compare the proposed  bound in Theorem \ref{theo:efldstab} with existing bounds in \cite{Li2020On} and  \cite{negrea2019information} for various datasets.
% Note that we do not consider the bound in \cite{haghifam2020sharpened} as a baseline because the bound in \cite{haghifam2020sharpened} only applies to full-batch setting, but we focus on noisy mini-batch gradient descent. We note that the squared norm of ``two-sample incoherence'' appeared in \cite{haghifam2020sharpened} (Theorem 4.2) roughly has the same order of magnitude as the gradient incoherence appeared in \cite{negrea2019information}. We also evaluate the optimization performance of proposed Noisy Sign-SGD by comparing it with the original sign-SGD \citep{bernstein2018signsgd} and present the corresponding generalization bound in Theorem \ref{theo:efldstab}. 



In this section, we conduct a series of experiments to evaluate our generalization error bounds. For SGLD, we aim to compare the proposed  bound in Theorem \ref{theo:efldstab} with existing bounds in \cite{Li2020On}, \cite{negrea2019information}, and \cite{rodriguez2021random} for various datasets. Note that the bound presented in \cite{rodriguez2021random} is an extension of that in \cite{haghifam2020sharpened} from full-batch setting to mini-batch setting. We also evaluate the optimization performance of proposed Noisy Sign-SGD by comparing it with the original sign-SGD \citep{bernstein2018signsgd} and present the corresponding generalization bound in Theorem \ref{theo:efldstab}. 





The details of our model architectures, learning rate scheduling, hyper-parameter selections and additional experimental results can be found in Appendix \ref{app:exp}. We emphasize that the goal for the experiments was to do a comparative study relative to existing approaches and bounds. We note that the empirical performance of the methods can potentially be improved with better architectures and training strategies, e.g., deeper/wider networks, data augmentation, batch/layer normalization, etc. 
%that we did not achieve the state-of-the art predictive performance, mainly due to the simplicity of our model architectures. With more complex model and further tuning, the prediction results could be improved.


\begin{figure*}[t] 
\centering
%\subfigure[CNN, MNIST, SGLD, $\alpha_t=0.2$, $\sigma_t=\alpha_t\eta_t \approx 10^{-4}$]{\includegraphics[width=0.95\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2.png}}
\subfigure[Test Error Bound]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-d.png}
 }  
\subfigure[Our Bound]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-b.png}
 }  
\subfigure[Gradient Discrepancy]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-a.png}
 } 
\subfigure[Training Error]{
\includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisySGD-random-beta-0.2-c.png}
 }
\vspace*{-3mm}
\caption[]{Results for training CNN using SGLD %($\sigma_t = 0.2\eta_t$) 
on a subset of MNIST ($n=10000$) with different randomness on labels. (a) Test error and bound: As the label randomness increases, the empirical test error (dashed lines) increases and so does the test error bound (solid lines); overall, the bounds stays valid. (b) Generalization bound: As the label randomness increases, so does the generalization bound in Theorem \ref{theo:efldstab}. (c) Gradient discrepancy: As the label randomness increases, so does the gradient discrepancy $\left\|\nabla \ell\left(\w_t, z_n \right)  -  \nabla \ell\left(\w_t, z'_n\right)\right\|_{2}^{2}$, which in turn leads to the increase in the generalization bound. (d) Training error: While training takes more epochs with random labels, training error does go to zero.
}
%\vspace*{-3mm}
\label{fig:bound_random}
\end{figure*}




\begin{figure*}[th!] 
\centering
  \subfigure[CNN, MNIST]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/cnn1-mnist-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 } 
  \subfigure[CNN, Fashion]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/cnn1-fashion-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
 \subfigure[ResNet-18, CIFAR10]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/resnet18-cifar10-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }
 \subfigure[ResNet-18, CIFAR100]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/resnet18-cifar100-n0-bs100-sign-sgd-train-dynamics-reduced.png}
 }\vspace*{-2mm}
\subfigure[MNIST, $\alpha_t=1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-c.png}
 } 
  \subfigure[MNIST, $\alpha_t=0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-noisy-signSGD-e.png}
 }
  \subfigure[Fashion, $\alpha_t=1$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-c.png}
 } 
  \subfigure[Fashion, $\alpha_t=0.01$]{
 \includegraphics[width=0.23\textwidth]{ICLR2022/images/smallcnn-fashion-bounds-noisy-signSGD-e.png}
 }
\vspace*{-4mm}
\caption[]{(a)-(d) show the training dynamics of CNN on MNIST and Fashion-MNIST, and ResNet-18 on CIFAR-10 and CIFAR-100 using noisy sign-SGD with different scaling $\alpha_t$. Legends indicate the choice of $\alpha_t$ and the numbers in brackets are test errors at convergence. As $\alpha_t\to 0$, Nosiy sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original sign-SGD \citep{bernstein2018signsgd}. (e)-(f) show that empirical test error can be bounded based on our generalization bound and the corresponding training error. The larger $\alpha_t$ (noise) is the sharper our bound is.}
%\vspace*{-3mm}
\label{fig:noisy_signsgd}
\end{figure*}



\subsection{Stochastic Gradient Langevin Dynamics}
%\vspace*{-2mm}
\noindent \textbf{Comparison with existing work.} We have derived generalization error bounds that depend on the data-dependent quantity \emph{gradient discrepancy}, i.e., $\left\|\nabla \ell\left(\w_{t}, z_n \right)  -  \nabla \ell\left(\w_{t}, z'_n\right)\right\|_{2}^{2}$. Existing bounds in \cite{Li2020On} and \cite{negrea2019information} have also improved the Lipschitz constant in \cite{mou2018generalization} to a data-dependent quantity. As shown in Figure~\ref{fig:sgld_bound} (a)-(d), by combining with the empirical training error, all four generalization error bounds can be used to bound the empirical test error, but our bound is able to generate a much tighter upper bound. Such difference is mainly due to the fact that we replace the squared \emph{gradient norm} in \cite{Li2020On}, the squared norm of \emph{gradient incoherence}
in  \cite{negrea2019information}, and that of \emph{two-sample incoherence} in \cite{rodriguez2021random} with the gradient discrepancy while maintaining a $1/n$ sample dependence. Results in Figure~\ref{fig:sgld_bound} (e)-(h) show that our bounds are much sharper than those of \cite{Li2020On} because our gradient discrepancy (Figure~\ref{fig:sgld_bound} (i)-(l)) is usually 2-4 order of magnitude smaller than the squared gradient norms appeared in \cite{Li2020On}. Our bounds are also sharper than those of \cite{negrea2019information} and \cite{rodriguez2021random} due to an improved dependence on $n$ from an order of $1/\sqrt{n}$ to ${1}/{n}$. Note that, even though the gradient incoherence in \cite{negrea2019information} is about 1 to 2 order of magnitude smaller than the gradient discrepancy for simple problems such as MNIST and Fashion-MNIST, the difference between the gradient incoherence and our gradient discrepancy reduces as the problem becomes harder (see results for CIFAR-10 in Figure~\ref{fig:sgld_bound}(j)).


%We report those data-dependent quantities in Figure \ref{fig:sgld_bound} for MNIST (i), Cifar-10 (j), and Fashion-MNIST (k)-(l),respectively. The results suggest that the squared gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors. The gradient incoherence in \cite{negrea2019information} is about 1 to 2 order of magnitude smaller than the gradient discrepancy for simple problems such as MNIST and Fashion-MNIST. %However, as problem becomes more difficult, i.e., CIFAR-10, the difference between the gradient incoherence and our gradient discrepancy reduces. Moreover, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$ which has a worse sample dependence compared to our bound. 










\noindent \textbf{Effect of Random Labels.} Motivated by \cite{zhang2017understanding}, we train CNN with SGLD on a smaller subset of MNIST dataset ($n=10000$) with randomly corrupted labels. The corruption fraction varies from $0\%$ (without label corruption) to $60\%$. As shown in Figure~\ref{fig:bound_random} (d), for long enough training time, all experiments with different level of label randomness can achieve almost zero training error. However, the one with higher level of randomness has higher generalization/test error (Figure \ref{fig:bound_random} (a) dashed lines). Our generalization bound also becomes larger as the randomness increases since the corresponding gradient discrepancy increases.



\subsection{Noisy Sign-SGD}
In this section, we present numerical results for Noisy Sign-SGD proposed in Example \ref{exam:noisy_signsgd}.  Since none of the existing bounds can give a valid generalization bound for Noisy Sign-SGD, we only present our bound here.

\noindent \textbf{Optimization.} Figures~\ref{fig:noisy_signsgd} (a)-(d) show the training dynamics of Noisy Sign-SGD under various choices of $\alpha_t$. As $\alpha_t\to 0$, Noisy Sign-SGD matches both the optimization trajectory as well as the final test accuracy of the original Sign-SGD \citep{bernstein2018signsgd}. However, as $\alpha_t$ increases, the distribution over $\{-1,+1\}$ approaches the uniform distribution, and with such high noise, the corresponding Noisy Sign-SGD seems to converge but to a rather sub-optimal value. 

\noindent \textbf{Generalization Bound.} Figure \ref{fig:noisy_signsgd}(e)-(f) show that our bound successfully bounds the empirical test error.
%and the corresponding training error. 
Larger $\alpha_t$ leads to sharper generalization bounds. However, larger $\alpha_t$ adversely affects the optimization, e.g., Figure~\ref{fig:noisy_signsgd} (a)-(d) blue and orange lines. The results illustrate the trade-off between the empirical optimization and the generalization bound. In practice, one needs to balance the optimization error and generalization by choosing a suitable scaling $\alpha_t$.
















% \begin{figure*}[t] 
% \centering
%   \subfigure[CNN, MNIST, SGLD, $\beta_t = 55000$, $\sigma_t\approx 4\times 10^{-4}$]{
%  \includegraphics[width=0.85\textwidth]{ICLR2022/images/smallcnn-mnist-bounds-beta-55000.0-pretrain.png}
%  } 
% \caption[]{Numerical results for CNN trained on MNIST with pre-training on a prertained dataset $\mathbf{J}_0$ where $|\mathbf{J}_0|=m$. As we increase the pretrain dataset size m, the gradient discrepancy decreases so does our bound.
% }
% \label{fig:mnist_sgld_pretrain}
% \end{figure*}




















%Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to those for CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases, leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence. 

%We note that  \cite{haghifam2020sharpened} show that Negrea et al. bound is smaller than Li et al. in their empirical evaluation, which is opposite to what we observed in Figure \ref{fig:mnist}.We think this is because \cite{haghifam2020sharpened} consider the full-batch setting which has a different form of gradient incoherence compared to the mini-batch setting in our paper. \yzcomment{added the discussion about the inconsistent of our result and \cite{haghifam2020sharpened}}


% The second key difference is the order of dependence on the sample size $n$, i.e., both of our bound and $\cite{Li2020On}$ has a bound of order $\frac{1}{n}$, however, the bound in \cite{negrea2019information} depends on $\frac{1}{\sqrt{n}}$. 
%Figure \ref{fig:mnist} (a) and 
% (b) suggests that the gradient norms in \cite{Li2020On} is much larger than the other two data-dependent factors, and the gradient incoherence in \cite{negrea2019information} is much smaller than the gradient discrepancy in our bound as well.
% However, the results in (b-d) for MNIST and (f-h) for Fashion MNIST show that our bounds are much sharper than those of \cite{negrea2019information} due to improving the dependence on $n$ from a order of $\frac{1}{\sqrt{n}}$ to $\frac{1}{n}$. Figure \ref{fig:mnist} (c-d) and (f-g) show that the bound decreases as the noise variance increases which is consistent with the theoretical bound. Figure \ref{fig:mnist} (d) and (h) present the bound for MLP model, showing that the bounds are smaller for MLP compared to CNN in (c) and (g). We think this is because, as the model size increases ( e.g., from MLP to CNN) the gradient dimension increases leading to a larger value of those gradient-dependent factors, i.e., gradient norm, gradient discrepancy and gradient incoherence.


%More details of our model architectures and addtional experimental results can be found in Appendix. We acknowledge that we did not aim to achieve the state-of-the art predictive performance. With further tuning, the prediction results could be improved








% \begin{figure*}[t] 
% \centering
% \includegraphics[ width=0.5\textwidth]{ICLR2022/images/vgg5-mnist-n1000-bs100-BernoulliSGD-train-dynamics.png}
% \caption[]{Training dynamics of Noisy SignSGD with Bernoulli noise with various selection of $\alpha$ for VGG5 trained on MNIST.When $\alpha \to 0$, Bernoulli SignSGD reduces to SignSGD. As a results, Bernoulli SignSGD with small enough $\alpha$ matches the training trajectory of SignSGD.
% } 
% \label{fig:mnist}
% \end{figure*}

% \textbf{To Do List}

% The following experiments follow the setting described in  \cite{negrea2019information}. \textbf{[By the end of this week (September 19)]}
% \begin{enumerate}
%     \item CNN (two convolutional layers + two fully connected layers) on MNIST and Fashion MNIST
%     \item CNN (two convolutional layers + three fully connected layers) on CIFAR-10
% \end{enumerate}

% The following experiments follow the standard setting most DL papers likely to perform. \textbf{[Before next Wednesday (September 22)]}
% \begin{enumerate}
%     \item VGG5 on MNIST and Fashion MNIST
%     \item ResNet-18 on CIFAR-10 and CIFAR-100
% \end{enumerate}



% \textbf{To Plot}
% \begin{enumerate}
%     \item Gradient norms \citep{Li2020On}
%     \item Gradient incoherence \citep{negrea2019information}
%     \item Gradient discrepancy $\| \mathbf{\theta}_{B,\alpha} - \mathbf{\theta}_{B',\alpha} \|_2^2$ (our bound)
%     \item Our bound, Negrea's bound, and Li et al., bound.
% \end{enumerate}

% \newpage

% \begin{table}
%   \caption{Summary of Experiments for SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $\beta_t$ & Our bound & Li bound & Negrea Bound \\
%     \midrule
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.96 & 55000 & $\checkmark$ & $\checkmark$ & $\checkmark$   \\
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.96 & 5000 & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
%     CNN-1 & Fashion  & $4\times 10^{-3}$ & 0.93 & 55000 & $\checkmark$ & $\checkmark$ & $\checkmark$  \\
%     CNN-1 & Fashion & $4\times 10^{-3}$ & 0.93 & 5000 & $\checkmark$ & $\checkmark$ &$\checkmark$  \\
%     \midrule
%     CNN-2 & CIFAR-10  & $5\times 10^{-3}$ & 0.95 & 55000 &  &  &   \\
%     CNN-2 & CIFAR-10  & $5\times 10^{-3}$ & 0.95 & 5000 &  &  &  \\
%   \midrule
%   ResNet-18/50 & Mini ImageNet & ? & ?&? & & &\\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for Noisy SGD with Gaussian Noise ($\sigma_t=c\eta_t$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $c$ & Our bound & Li bound & Negrea Bound \\
%     \midrule
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.995 & 0.002 &$\checkmark$  & $\checkmark$ &   \\
%     CNN-1 & MNIST  & $4\times 10^{-3}$ & 0.95 & 0.2 &$\checkmark$  &$\checkmark$  &  \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$) with pretrain ($|J_0|=m$)}
%   \label{tab:sgld_pretrain}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & m &$\eta_0$& decay & $\beta_t$ & Our bound\\
%     \midrule
%     CNN-1 & MNIST  & 100 & $4\times 10^{-3}$ & 0.96 & 55000 &   \\
%     CNN-1 & MNIST  & 1000 & $4\times 10^{-3}$ & 0.96 & 55000 &   \\
%     CNN-1 & MNIST  & 10000 & $4\times 10^{-3}$ & 0.96 & 55000 &    \\
%     CNN-1 & MNIST  & 50000 & $4\times 10^{-3}$ & 0.96 & 55000 &    \\
%     \midrule
%     CNN-1 & Fashion & 100 & $4\times 10^{-3}$ & 0.93 & 55000 &   \\
%     CNN-1 & Fashion & 1000 & $4\times 10^{-3}$ & 0.93 & 55000 &    \\
%     CNN-1 & Fashion & 10000 & $4\times 10^{-3}$ & 0.93 & 55000 &    \\
%     CNN-1 & Fashion & 50000 & $4\times 10^{-3}$ & 0.93 & 55000 &   \\
%     \bottomrule
%   \end{tabular}
% \end{table}



% \begin{table}
%   \caption{Summary of Experiments for Random Labels with SGLD ($\sigma_t=\sqrt{2\eta_t/\beta_t}$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & Randomness & $\eta_0$& decay & $\beta_t$ & Our bound  \\
%     \midrule
%     CNN-1 & MNIST  &0 &$4\times 10^{-3}$ & 0.96 & 55000 & $\checkmark$  \\
%     CNN-1 & MNIST  &10\% &? & ? & ? & \\
%     CNN-1 & MNIST & 20\% &? & ? & ? & \\
%     CNN-1 & MNIST & 50\% &? & ? & ? & \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}
%   \caption{Summary of Experiments for Noisy SGD with Bernoulli Noise ($\mu_{\alpha} = \frac{1}{1+\exp(-\theta/\alpha})$)}
%   \label{tab:exp}
%   \centering
%   \begin{tabular}{cccccc}
%     \toprule
%     %\multicolumn{2}{c}{Part}                   \\
%     %\cmidrule(r){1-2}
%     Model   & Dataset & $\eta_0$& decay & $\alpha_t$ & Our bound \\
%     \midrule
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-6}$ &   \\
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-2}$ &  \\
%     CNN-1 & MNIST  & $10^{-4}$ & 0.1 & $10^{-1}$ &  \\
%     CNN-1 & Fashion  & $10^{-4}$ & 0.1 & $10^{-6}$ &     \\
%     CNN-1 & Fashion & $10^{-4}$ & 0.1 & $10^{-2}$&   \\
%     CNN-1 & Fashion & $10^{-4}$ & 0.1 & $10^{-1}$&   \\
%     \midrule
%     CNN-2 & CIFAR-10  & $10^{-3}$ &0.1  & $10^{-6}$ &   \\
%     CNN-2 & CIFAR-10  & $10^{-3}$ & 0.1 & $10^{-2}$ &  \\
%     CNN-1 & CIFAR-10  & $10^{-3}$ &0.1  & $10^{-1}$ &  \\
%   \midrule
%   ResNet-18/50 & Mini ImageNet & ? & ?&? & \\
%     \bottomrule
%   \end{tabular}
% \end{table}



==> arXiv/sec/exp_stability.tex <==

In the setting of statistical learning, there is an instance space $\cZ$, a hypothesis space $\cW$, and a loss function $\ell : \cW \times \cZ \mapsto \R_+$. Let $D$ be an unknown distribution of $\cZ$ and let $S_n \sim D^n$ be $n$ i.i.d.~draws from $D$. For any specific hypothesis $\w \in \cW$, the population and empirical loss are respectively given by
%\vspace*{-3mm}
%\begin{equation}
$L_D(\w) \triangleq \E_{z \sim D}[\ell(\w,z)]$, and $L_S(\w) \triangleq \frac{1}{n} \sum_{i=1}^n \ell(\w,z_i)$.  
%\vspace*{-3mm}
%\end{equation}
For any distribution $P$ over the hypothesis space, we respectively denote the expected population and empirical loss as
%\vspace*{-3mm}
\begin{equation}
L_D(P) \triangleq \E_{z \sim D}\E_{\w \sim P}[\ell(\w,z)]~, \qquad \text{and} \qquad  L_S(P) \triangleq \frac{1}{n} \sum_{i=1}^n \E_{\w \sim P}[\ell(\w,z_i)]~.
%\vspace*{-3mm}
\end{equation}
Consider a randomized algorithm $A$ which works with $S_n =\{z_1,\ldots,z_n\} \sim D^n$ and creates a distribution over the hypothesis space $\cW$. For convenience, we will denote the distribution as $A(S_n)$. The focus of our analysis is to bound the generalization error of $A$ defined as: 
%$\gen(A(S)) \triangleq L_D(A(S)) - L_S(A(S))~.  $
\begin{align}
\gen(A(S_n)) \triangleq L_D(A(S_n)) - L_S(A(S_n))~.    
\end{align} 
We will assume $A$ is permutation invariant, i.e., the ordering of samples in $S_n$ do not modify $A(S_n)$, an assumption satisfied by most learning algorithms. We will focus on developing bounds for the expectation $\E_{S_n}[L_D(A(S_n)) - L_S(A(S_n))]$, and discuss high-probability bounds in the Appendix. All technical proofs for results in this section are in Appendix~\ref{sec:app_exp_stability}.



\subsection{Bounds based on Expected Stability}
% For our analysis, we assume that the $L_2$ norm of the loss is bounded:
% \begin{asmp}
% Let $c_{\ell_2}(z) = \E_{w \sim  p_{A(S)}}[\ell^2(w,z)]$. Two options:
% \begin{enumerate}
% \item Uniform bound: $\forall z$, $c_{\ell_2}(z) \leq c_0$.
% \item Expectation bound: $\E_{z \sim D}[c_{\ell_2}(z)] \leq c_0$ \abedit{and $\E_{z \sim S}[c_{\ell_2}(z)] \leq c_0$}.
% \end{enumerate}
% The analysis would look different depending on which one we choose. \abcomment{Discuss}
% \end{asmp}
% \abcomment{need a discussion on assumptions for info-theoretic analysis}

We start our analysis by noting that the expected generalization error can be upper bounded by {\em expected stability} based on the Hellinger divergence $H(P \| P')$ between two distributions given by~\citep{save16,Li2020On}: $H^2(P\| P') = \frac{1}{2}\int_{\w} (\sqrt{p(\w)} - \sqrt{p'(\w)})^2 d\w$.
\begin{restatable}{prop}{prophell}
Let $S_n \sim D^n$ and let $S'_{n}$ be a dataset obtained by replacing $z_n \in S_n$ with $z'_n \sim D$. Let $A(S_n),A(S'_{n})$ respectively denote the distributions over the hypothesis space $\cW$ obtained by running randomized algorithm $A$ on $S_n,S'_{n}$.
Assume that for all $S_n \in \cZ^n, z \in \cZ$, $\E_{W \sim  A(S_n)}[\ell^2(W,z)] \leq c^2_0/4$ for some constant $c_0>0$.  With $H(\cdot,\cdot)$ denoting the Hellinger divergence, we have
\begin{equation}
| \E_{S_n \sim D^n}[L_D(A(S_n)) - L_S(A(S_n))] | \leq c_0 \E_{S_n \sim D^n} \E_{z'_n \sim D} \sqrt{2 H^2\big(A(S_n), A(S'_{n})\big)}~. 
\end{equation}
\vspace*{-3mm}
\label{prop:hell}
\end{restatable}
\begin{remark}
Proposition~\ref{prop:hell} does not need bounded losses. Just the {\em second moment} of $\ell(W,z), W \sim A(S_n)$ need to be bounded. The assumption is satisfied by bounded losses. It is instructive to compare the assumption to that in recent information theoretic bounds~\citep{haghifam2020sharpened,xu2017information}, where one assumes $\ell(\w,Z), Z \sim D, \forall \w \in \cW$ to be {\em sub-Gaussian}. \qed 
\end{remark}
\begin{remark}
The bound in Proposition~\ref{prop:hell} is in terms of {\em expected stability} where we consider $\E_{S_n \sim D^n} \E_{z'_n \sim D}[\cdots]$, an important departure from bounds based on {\em uniform stability} \citep{elisseeff2005stability, bousquet2002stability, mou2018generalization,bousquet2020sharper, feldman2018generalization,feldman2019high} where one considers $\sup_{S,S' \in \cZ^n, |S \Delta S'| = 1}[\cdots]$. Replacing $\sup$ by $\E$ makes the bounds distribution dependent, avoids the worst case analysis associated with uniform stability, and arguably leads to quantitatively tighter bounds. \qed 
\end{remark}
Note that the Hellinger divergence can be bounded by the KL divergence, and our analysis in the sequel will focus on bounding the KL divergence.
%so we focus on bounding the KL divergence in the sequel. 
\begin{restatable}{prop}{prophellkl}
For any distributions $P$ and $P'$,
% \vspace*{-2mm}
% \begin{equation}
$2 H^2(P,P') \leq \min \big\{ KL(P,P'),\sqrt{\frac{1}{2}KL(P,P')} \big\}$. 
% \end{equation}
%\vspace*{-5mm}
\label{prop:hellkl}
\end{restatable}
\begin{remark}
While our analysis in the sequel focuses on bounding the KL-divergence, in certain settings one may be able to directly bound the Hellinger divergence possibly leading to sharper bounds. Further, the Hellinger divergence can be upper bounded by the Total Variation (TV) divergence (e.g., used in proof of Proposition~\ref{prop:hellkl}) which may also lead to sharp bounds. An analysis based on KL-divergence needs $P$ to be absolutely continuous w.r.t.~$P'$ which is not necessary when working with Hellinger or TV divergences. \qed 
\end{remark}



\subsection{Expected Stability of Noisy Stochastic Iterative Algorithms}
\label{sec: exp_stab_nsi}

We consider a general family of noisy stochastic iterative (NSI) algorithms. Given $S_n \sim D^n$, such iterative algorithms have two additional sources of randomness in each iteration $t$: (a) a stochastic mini-batch of samples $S_{B_t}$, with $|S_{B_t}| = b$, drawn uniformly at random with replacement from $S_n$; and (b) noise $\bxi_t$ suitably included in the iterative update. 
Given a trajectory (realization) of past iterates $W_{0:(t-1)} = \w_{0:(t-1)}$, the new iterate $W_t$ is drawn from a distribution $P_{B_t,\bxi_t|\w_{0:(t-1)}}$ over $\cW$:
\begin{align}
W_{t} \sim P_{B_t,\bxi_t|\w_{0:(t-1)}}(W) ~.
%= f_t(B_t,\bxi_t,\w_{0:(t-1)})~,
\label{eq:nmia}
\end{align}
%for some suitable function $f_t$. 
We will often drop the conditioning $\w_{0:(t-1)}$ to avoid clutter  in the sequel.

Let $P_{0:(t-1)}$ denote the joint distribution over $W_{0:(t-1)} = (W_0,\ldots,W_{t-1})$, and 
let $P_{t|} := P_{B_t,\bxi_t|\w_{0:(t-1)}}$ compactly denote the conditional distribution on $W_t$ conditioned on the trajectory $W_{0:(t-1)} = \w_{0:t-1}$. Further, let $P_T, P'_T$ denote the marginal distributions over hypotheses $\w \in \cW$ after $T$ steps of the algorithm based on $S_n,S'_{n}$ respectively, where $S'_n$ is as discussed in Proposition~\ref{prop:hell}, i.e., obtained from $S_n$ by replacing $z_n \in S_n \sim D^n$ by $z'_n \sim D$. Following \citep{pensia2018generalization,negrea2019information,haghifam2020sharpened}, we use the following chain rule to bound the KL-divergence between $P_T$ and $P'_T$:
%which has been effectively used in recent advances in information theoretic bounds for generalization~:
% \vspace*{-4mm}
\begin{equation}
KL(P_T \| P'_T) \leq KL(P_{0:T} \| P'_{0:T} ) = \sum_{t=1}^T \E_{P_{0:(t-1)}}\left[ KL(P_{t|} \| P'_{t|}) \right]~.
\label{eq:klchain}
%\vspace*{-2mm}
\end{equation}
Let $\bar{S}_{n+1} \sim D^{n+1}$ with $\bar{S}_{n+1} = \{z_1,\ldots,z_{n+1}\}$ so that $S_n,S'_{n}$ are size $n$ subsets of $\bar{S}_{n+1}$ with $S_n=\{z_1,\ldots,z_{n-1},z_n\}$ and $S'_{n} = \{z_1,\ldots,z_{n-1},z'_n\}$, where $z'_n = z_{n+1}$. Let $S_0 = \{z_1,\ldots,z_{n-1}\}$. The algorithms we consider use a mini-batch of size $b$ in each iteration uniformly sampled from $n$ samples in $S_n$ or $S'_n$. Let the set of all mini-batch index sets be denoted by $G$. Let the set of all mini-batch index sets $A$ drawn from $S_0$ be denoted by $G_0$. Note that $|G_0| = \binom{n-1}{b}$. Let $G_1$ denote the set of all mini-batch index sets $B$ which includes the last sample, viz.~$z_n$ for $S_n$ and $z'_n$ for $S'_n$. 
Note that $|G_1| = \binom{n-1}{b-1}$. Also note that 
$|G_0| + |G_1| = \binom{n-1}{b} + \binom{n-1}{b-1} = \binom{n}{b} = |G|$.


Following \cite{Li2020On}, we can bound their conditional KL-divergences $KL(P_{t|} \| P'_{t|})$ 
in the right-hand-side of \eqref{eq:klchain} 
in terms of a Le Cam Style Divergence (LSD). While the classical Le Cam divergence~\citep{save16} is $LCD(P\|P') \triangleq \frac{1}{2} \int \frac{(dP - dP')^2}{dP + dP'}$ (where $dP$ denotes the density), our bounds are in terms of  
\begin{align}
LSD(P_{t|}| \| P'_{t|}) \triangleq \underset{B_t \in G_1}{\E} \underset{A_t \in G_0}{\E}  \left[\int_{\bxi_t} \frac{(dP_{B_t,\bxi_t} - dP'_{B_t,\bxi_t})^2}{dP_{A_t,\bxi_t}} d \bxi_t \right]~,  
\end{align}
where $B_t \in G_1, A_t \in G_0$.
Note that $P_{B_t,\bxi_t}$ and $P'_{B_t,\bxi_t}$ represent the conditional distribution of $W_t$ for $S_n$ and $S_n^\prime$ respectively since the mini-batch $S_{B_t}$ of $S_n$ and $S_n^\prime$ differs in the $n$-th sample. 
%Putting Propositions~\ref{prop:hell} and \ref{prop:hellkl}, and \eqref{eq:klchain} together, with some additional analysis 
Bounding the KL-divergences in \eqref{eq:klchain} with LSDs, we have the following expected LSD based generalization bound.
\begin{restatable}{lemm}{theostab}
Consider a noisy stochastic iterative algorithms of the form~\eqref{eq:nmia} with mini-batch size $b \leq n/2$. Then, with $c_1 = \sqrt{2} c_0$ (with $c_0$ as in Proposition~\ref{prop:hell}), we have
%\vspace*{-1mm}
\begin{equation}
\hspace*{-5mm}
| \E_{S_n}[L_D(A(S_n)) - L_{S}(A(S_n))] | \leq c_1 \frac{b}{n} \E_{S_n} \E_{z'_n} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \underset{B_t \in G_1}{\E} \underset{A_t \in G_0}{\E} \left[ \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t \right] }~.
\end{equation}
\label{theo:stab}
%\vspace*{-6mm}
\end{restatable}
\begin{remark}
Though not stated explicitly, \cite{Li2020On} essentially has this result for SGLD and inspired our work. Our proofs are significantly simpler, does not make any additional assumptions, and illustrates applicability to general noisy iterative algorithms of the form~\eqref{eq:nmia}, not just SGLD with Gaussian noise as in \cite{Li2020On}. \qed 
\end{remark}
\begin{remark}
Note that the bound depends on expectations over samples $S_n,z'_n$, trajectories $W_{0:(t-1)}$, and mini-batches $B_t,A_t$. Unlike uniform stability and other worst case analysis, there is no $\sup$ over samples, trajectories, or mini-batches.
%does not assume the loss to be bounded and 
%and does not depend on any uniform assumptions. 
Further, 
%as an expected stability based bound to generalization error, 
the bound depends on the distribution discrepancy as captured by the expected LSD. \qed 
\end{remark}
\begin{remark}
The bound seems to worsen with $b$, the size of the mini-batch. As we shown in Section~\ref{sec:efld}, the expected LSD terms have a $\frac{1}{b^2}$ dependence for the Exponential Family Langevin dynamics (EFLD) models  we introduce, so the leading $b$ is neutralized. \qed 
\end{remark}

% \begin{remark}
% Check what happens when the r.v.~is discrete, e.g., Bernoulli. Does the transition to Hellinger, then to KL, and then to LSD go through without any issues? Current analysis assumes Lebesgue measure, need to check validity for counting measure.
% \end{remark}


==> arXiv/sec/intro.tex <==


Recent years have seen renewed interest and advances in characterizing generalization performance of learning algorithms in terms of stability, which considers change in performance of a learning algorithm based on change of a single training point \citep{hardt2016train,bousquet2002stability,Li2020On,mou2018generalization}. For stochastic gradient descent (SGD), \cite{hardt2016train} established generalization bounds based on uniform stability \citep{hardt2016train,bousquet2002stability}, although the analysis needed rather small step sizes $\eta_t = 1/t$ which is arguably not useful in practice. While improving the stability analysis for SGD has remained a challenge, advances have been made on noisy SGD algorithms, especially stochastic gradient Langevin dynamics (SGLD) \citep{WellingT11, mou2018generalization,Li2020On} which adds Gaussian noise to to the stochastic gradients. In parallel, there has been key developments on related information-theoretic generalization bounds applicable to SGLD type algorithms \citep{negrea2019information,haghifam2020sharpened,xu2017information,russo2016controlling, pensia2018generalization}.

While these developments have led to major advances in analyzing generalization of noisy SGD algorithms, they each have certain limitations which leave room for further improvements. \cite{mou2018generalization} considered SGLD with marginal Gaussian noise variance $\sigma_t$ and step size $\eta_t \leq {\sigma_t \ln 2}/{L}$, where $L$ is the global Lipschitz constant for the loss,  and established a generalization bound for SGLD of the form $\frac{L}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ using uniform stability.
The bound has a desirable dependency of $O({1}/{n})$ on the samples, but has an undesirable dependence on $L$, and the step sizes, bounded by $O({\sigma_t}/{L})$, are arguably too small. \cite{mou2018generalization} also presented another bound which addresses some of these issues, but gets an undesirable $O({1}/{\sqrt{n}})$ sample dependence.  By building on the developments of \cite{russo2016controlling,xu2017information,pensia2018generalization}, \cite{negrea2019information} made advances from the information theoretic perspective and established bounds for SGLD which have a desirable dependence on the norm of gradient incoherence, i.e., a suitable difference in gradients over different mini-batches, avoids dependence on Lipschitz constant $L$, and is applicable to unbounded sub-Gaussian losses, but have an undesirable $O({1}/{\sqrt{n}})$ sample dependence. \cite{haghifam2020sharpened} made further advances on the problem from an information theoretic perspective based on the conditional mutual information framework of~\cite{steinke2020reasoning} and obtained generalization bounds based on gradient incoherence with $O({1}/{n})$ sample dependence, but their analysis holds for full batch Langevin dynamics, not mini-batch SGLD. \abcomment{add recent extension to SGLD} \cite{Li2020On} made advances on such bounds based on the notion of Bayes-stability, by combining ideas from PAC-Bayes bounds into stability, and established a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \mathbf{g}_e(t)/\sigma_t^2}$ for bounded losses, where $\mathbf{g}_e(t)$ is the expected gradient norm square at step $t$. While the bound has a desirable sample dependence of $O(1/n)$ and avoids dependence on the Lipschitz constant $K$, the dependence on the gradient norm makes such bounds much weaker than the information theoretic bounds of \cite{negrea2019information,haghifam2020sharpened} which depend on the norm of gradient incoherence which are typically orders of magnitude smaller. Further, the analysis of \cite{Li2020On} still needs small step sizes, bounded by $O({\sigma_t}/{L})$. 


In this paper, we build on the core strengths of such existing approaches, most notably (a) the $O({1}/{n})$ sample dependence of stability based bounds~\citep{mou2018generalization,Li2020On}, (b) the dependence on the norm of gradient incoherence rather than the norm of gradient for information theoretic bounds~\citep{negrea2019information,haghifam2020sharpened}, and (c) no dependence on the global Lipschitz constant $K$, and develop a framework (Section~\ref{sec:exp_stability}) for establishing generalization bounds for noisy stochastic iterative algorithms. Our framework considers generalization based on the concept of {\em expected stability}, rather than uniform stability \citep{hardt2016train,bousquet2002stability, bousquet2020sharper,mou2018generalization}, and yields distribution dependent generalization bounds which avoid the worst-case setting of uniform stability. Recall that for any data domain $\cZ$ and a distribution $D$ over the domain, uniform stability considers the worst case difference in loss over two datasets $S_n,S'_n \in \cZ^n$ of size $n$ which differ by one point, i.e., over $\sup_{S_n, S'_n, |S_n \Delta S'_n|=1} \cdots$ \citep{bousquet2002stability,hardt2016train}. In Section~\ref{sec:exp_stability}, we show that one gets a valid generalization bound by replacing the supremum $\sup$ by and expectation $\E_{S_n,S'_n}$, where $S_n \sim D^n$ and, without loss of generality, $S'_n$ shares the first $(n-1)$ samples with $S_n$ with the $n$-th sample $z'_n \sim D$. Replacing $\sup$ by $\E$ makes the bound distribution dependent, avoids the worst case analysis associated with uniform stability, and can arguably lead to quantitatively sharper bounds will less assumptions. Building on some analyses in \cite{Li2020On}, we show that expected stability of general noisy mini-batch stochastic iterative algorithms, not just noisy SGD, can be bounded by the expectation of a Le Cam Style Divergence (LSD) over distributions over parameters obtained from $S_n$ and $S'_n$. Thus, getting an expected stability based generalization bound for a specific algorithm reduces to that of bounding the expected LSD.

In Section~\ref{sec:efld}, we introduce Exponential Family Langevin Dynamics (EFLD), a family of noisy stochastic gradient descent algorithms based on exponential family noise. Special cases of EFLD include SGLD and noisy versions of Sign-SGD or quantized SGD algorithms widely used in practice \citep{bernstein2018signsgd, bernstein2018signsgdnoise, jin2020stochastic, quantized-sgd}. 
Our main result provides an expected stability based generalization bound applicable to any EFLD algorithm with several desirable properties: (a) a $O({1}/{n})$ sample dependence, (b) a dependence on the norm of gradient discrepancy, a variant of gradient incoherence~\citep{negrea2019information}, rather than a dependence on the norm of gradients, (c) no dependence on the global Lipschitz constant $K$, and (d) step sizes $\eta_t$ need not be tiny, i.e., $\eta_t = O(1/K)$ is not necessary. Existing generalization bounds for SGLD~\citep{Li2020On,negrea2019information} usually use properties of the Gaussian distribution, and do not generalize to EFLD. Our proof technique is new, and uses properties of exponential family distributions. 
We also consider optimization guarantees for EFLD, establish convergence results for SGLD based on Gaussian noise and for noisy Sign-SGD based on Bernoulli noise over $\{-1,+1\}$ where the Bernoulli noise parameters depend on the stochastic gradients. The analysis for SGLD is a variant of existing analyses whereas the analysis for noisy sign-SGD based on gradient dependent Bernoulli noise is new. 
%and the first convergence result for the algorithm to the best of our knowledge. 

In Section~\ref{sec:exp}, we present experiment results on benchmark datasets and illustrate that our bounds for SGLD are non-vacuous and quantitatively tighter than existing bounds~\citep{Li2020On,negrea2019information} due to the desirable dependence on sample size and gradient discrepancy norms, which are empirically shown to be orders of magnitude smaller than gradient norms. We also present results for noisy Sign-SGD on benchmark datasets and illustrate that our bounds give a quantitatively tight upper bound to the empirical test error across epochs and the optimization performance is comparable to that of sign-SGD. 

%Our empirical results also illustrate a trade-off inherent in noisy gradient algorithms--a lower noise scale implies 

%Through experiments on benchmark datasets (), we illustrate that our bounds are non-vacuous and quantitatively much sharper than existing bounds.

%{\bf Related work.} Uniform stability has been a classical approach for bounding generalization error \citep{bousquet2002stability,bousquet2020sharper,feldman2018generalization,feldman2019high}, pioneered by \cite{rogers1978finite,devroye1979distribution}. Beyond the aforementioned work, there has been recent work on differential privacy that analyzes the uniform stability of differentially private SGD (DP-SGD) \citep{hardt2016train, bassily2020stability}. Beyond uniform stability, information-theoretic approaches \citep{russo2016controlling, xu2017information}  that bounds the generalization error by the mutual information between the algorithm input $S$ and the algorithm output $\w$, have been used for deriving generalization bounds for noisy iterative algorithms \citep{pensia2018generalization,bu2019tightening}. Along this line of literature, \cite{negrea2019information, haghifam2020sharpened, rodriguez2021random} prove  data-dependent generalization bounds dropping dependence on the Lipschitz constant. Further, tighter bounds \citep{haghifam2020sharpened, zhou2021individually, rodriguez2021random, neu2021informationtheoretic, hellstrom2021fast}  are proposed based on conditional mutual information \citep{steinke2020reasoning, grunwald2021pac, hellstrom2020generalization}. Due to space limitations, an extended discussion of the related work is deferred to Appendix~\ref{sec:related_work}. 



==> arXiv/sec/related.tex <==

% \begin{itemize}
%     \item Generalization approaches (stability, information-theory bound, PAC Bayesian, Uniform Bound)
%     \item Noisy iterative algorithm (Sign SGD, SGLD, DP SGD etc)
%     \item More?
% \end{itemize}

% \textbf{(Old Materials)}]



\noindent \textbf{Uniform stability.} Uniform stability is a classical approach for bounding generalization error \citep{bousquet2002stability,hardt2016train,bousquet2020sharper, ShalevShwartz2009StochasticCO,feldman2018generalization,feldman2019high}, pioneered by \cite{rogers1978finite,devroye1979distribution}. Recently, uniform stability has been used in analyzing the  stability of stochastic gradient descent (SGD) \citep{hardt2016train}. 
\cite{mou2018generalization} prove the uniform stability of SGLD \citep{WellingT11, raginsky2017non} by showing that uniform stability can be bounded by the squared Hellinger distance, and further they establish discretized Fokker-Planck equations for analyzing the squared Hellinger distance. Then they provide uniform stability based generalization bounds for SGLD as $\frac{L}{n} \sqrt{\sum_t\eta^2_t/\sigma_t^2}$ which depends on $L$, the global Lipschitz constant for gradients, and the step size $\eta_t \leq \frac{\sigma_t \ln 2}{L}$ \citep{mou2018generalization,Li2020On}. 
Recently, \cite{Li2020On} followed up on \cite{mou2018generalization} and derived a data-dependent bound based on Bayes-stability, and got a bound of the form $\frac{c}{n} \sqrt{\sum_t \eta^2_t \g_e(t)/\sigma_t^2}$, where $\g_e(t)$ is the expected gradient norm square at step $t$. Their bound improves the Lipschitz constant $L$ to the expected gradient norm square.  
Recently, \cite{bassily2019private} analyze the uniform stability of  differentially private SGD (DP-SGD) for convex optimization by showing the gradient update is a non-expansive operation, which is the key fact in proving the stability of SGD \citep{hardt2016train}. 
The approach in \cite{hardt2016train} can extend to non-convex setting as well, however it requires fast decaying in step size as $\eta_t = O(1/t)$.  \cite{bassily2020stability} provide stability analysis of SGD for convex and non-smooth functions. 

\noindent \textbf{Information-theoretic bounds.} Besides the works mentioned above, other theories of deriving generalization bounds for noisy iterative algorithms have been proposed via information-theoretic approaches \citep{russo2016controlling, xu2017information}. Such results show that the generalization error of any learning algorithm can be bounded as $O(\sqrt{I(S; W)/n})$, where $I(S; W)$ is the mutual information between the algorithm input $S$ and the algorithm output $W$. Recent work following this approach focus on bounding the mutual information for a broad class of iterative algorithms, including SGLD  to obtain a $O(\sqrt{\log T/n})$ generalization bound by choosing $\eta_t = O(1/t)$, where $T$ is the total number of iterations~\citep{pensia2018generalization,bu2019tightening}. Subsequent improvements to this technique were made by 
\cite{negrea2019information, haghifam2020sharpened, rodriguez2021random} 
to prove data-dependent generalization bounds that do not depend
on the Lipschitz constant of the loss function and obtain $\sqrt{\sum_t \eta_{t}/n} $ bounds. 
Especially, \cite{haghifam2020sharpened, zhou2021individually} introduce generalization bounds based on conditional mutual information inspired by \cite{steinke2020reasoning}, leading to tighter bounds than those based on mutual information. Recently, \cite{rodriguez2021random} extend the result of \cite{haghifam2020sharpened} from full-batch gradient to stochastic setting. 
\cite{neu2021informationtheoretic} extend this information-theoretic approach  to derive generalization bound for vanilla SGD. \cite{hellstrom2021fast} provide a fast-rate bound for bounded loss functions based via Conditional Information Measures \citep{grunwald2021pac, hellstrom2020generalization}, which also provides a unified view of some of the above results.


%\textbf{PAC-Bayesian bound.} 

\noindent \textbf{Noisy iterative algorithms.} Introducing additional noise in the stochastic gradient has been popular in training deep nets. Noisy iterative methods have proven to be useful for machine learning applications, especially for deep neural networks in terms of escaping from saddle points \citep{jin2017escape,jin2019nonconvex}, preserving privacy  \citep{bassily2020stability,wang2019differentially}, boosting generalization and stability \citep{mou2018generalization,Li2020On}. SGLD \citep{WellingT11} has been one of the most popular noisy iterative algorithms for non-convex learning problems, where an isotropic Gaussian noise is added to the stochastic gradient. There has been some work \citep{wang2015privacy, li2019connecting} connecting SGLD with differentially private SGD  algorithm (DP-SGD) \citep{bassily2020stability,wang2019differentially} which usually adds noise with constant variance to the stochastic gradient. 
Uniform stability has also been popular in the differential privacy literature for analyzing the generalization error bound of DP-SGD algorithms. Recently, noise has been proven to be useful in Sign-SGD \citep{bernstein2018signsgd, bernstein2018signsgdnoise, chen2019distributed} which has gained popularity as it reduces communication cost in distributed learning.  Existing versions of noisy sign-SGD first adds symmetric noise to the stochastic gradient, then take the sign of the noisy stochastic gradient to update the parameters \citep{chen2019distributed, jin2020stochastic}. \cite{bernstein2018signsgdnoise, chen2019distributed, jin2020stochastic} have shown that when noise is unimodal and symmetric, sign-SGD can guarantee convergence to stationary point.







==> arXiv/sec/stability.tex <==
%\vspace*{-2mm} 

From Lemma~\ref{theo:stab}, conditioned on a trajectory $W_{0:(t-1)}=\w_{0:(t-1)}$, mini-batches $S_{B_t}, S_{A_t}$, %\yzcomment{sometimes, we use $S_{B_t}$ as mini-batch, sometimes we use $B_t$ as mini-batch. To be consistent, let’s use $S_{B_t}$ for mini-batch, and ${B_t}$ for indexes} 
we can get an expected stability based generalization bound by suitably bounding the Le Cam Style Divergence (LSD) given by:
\begin{align}
I_{A_t,B_t} = \bigintsss_{\bxi_t} \frac{ \left(  dP_{B_t,\bxi_t} -   dP'_{B_t,\bxi_t} \right)^2 }{ dP_{A_t,\bxi_t}} d\bxi_t~.
\label{eq:plsd}
\end{align}
For EFLD, the density functions $dP_{B_t,\bxi_t},dP'_{B_t,\bxi_t}$ are exponential family densities $p_{\psi}(\bxi; \btheta_{B_t,\alpha_t}), p_{\psi}(\bxi; \btheta'_{B_t,\alpha_t})$ as in \eqref{eq:efld1}-\eqref{eq:efld2}, and we have the following bound on the per step LSD in \eqref{eq:plsd}.

\begin{restatable}{theo}{theoefld}
For a given set $\bar{S}_{n+1} \sim D^{n+1}$ and $\w_{t-1}$ at iteration $(t-1)$, let $\Delta_{t|\w_{t-1}}(\bar{S}_{n+1}) = \max_{z, z' \in  \bar{S}_{n+1}} \left\|\nabla \ell(\w_{t-1}, z\right) - \nabla \ell\left(\w_{t-1}, z')\right\|_{2}$. Further, for a $c_2$-smooth log-partition function $\psi$, let the scaling $\alpha_{t|\w_{t-1}}$ be data-dependent such that $\alpha_{t|\w_{t-1}}^2 \geq  8 c_2 \Delta_{t|\w_{t-1}}^{2}(\bar{S}_{n+1})$. Then, we have
\vspace*{-2mm} 
\begin{align}
I_{A_t, B_t} \leq 5 c_2 \| \btheta_{B_t,\alpha_t} - \btheta_{B'_t,\alpha_t} \|_2^2 = \frac{5c_2}{2\alpha_{t|\w_{t-1}}^2} \left[\left\|\nabla \ell\left(\w_{t-1}, {S_{B_t}}\right)  -  \nabla \ell\left(\w_{t-1}, S'_{B_t}\right)\right\|_{2}^{2}\right]~.
\end{align}
\label{theo:efld}
\vspace*{-5mm}
\end{restatable}
\begin{remark}
Theorem~\ref{theo:efld} shows that per step LSD can be bounded by a scaled version of the mini-batch gradient discrepancy. The result holds for {\em all} exponential family Langevin dynamics algorithms of the form \eqref{eq:efld1}-\eqref{eq:efld2}, not just Gaussian noise based SGLD. 
\end{remark}
\begin{remark}
Recall that for $\bar{S}_{n+1} \sim D^{n+1}$ with $\bar{S}_{n+1} = \{z_1,\ldots,z_{n+1}\}$, $S_{B_t}, S'_{B_t}$ are respectively drawn from $S_n,S'_{n}$ which are size $n$ subsets of $\bar{S}_{n+1}$ with $S_n=\{z_1,\ldots,z_{n-1},z_n\}$ and $S'_{n} = \{z_1,\ldots,z_{n-1},z'_n\}$, where $z'_n = z_{n+1}$ so that $S_{B_t}$ and  $S'_{B_t}$ only differ at samples $z_n$ and $z'_n$. As a result $\nabla \ell(\w_{t-1}, S_{B_t})  -  \nabla \ell(\w_{t-1}, S'_{B_t} ) =
\frac{1}{b} \sum_{z\in S_{B_t}} \nabla \ell (\w_{t-1}, z) - \frac{1}{b} \sum_{z' \in S'_{B_t}} \nabla \ell (\w_{t-1}, z') = \frac{1}{b} (\nabla \ell (\w_{t-1}, z_n) - \nabla \ell(\w_{t-1},z'_n))$. The $1/b$ scale factor neutralizes the leading $b$ term in Lemma~\ref{theo:stab}. 
\end{remark}

The bound in Theorem~\ref{theo:efld} can now be directly applied to Lemma~\ref{theo:stab} to get expected stability based generalization bounds for any EFLD algorithm.
\begin{restatable}{theo}{theoefldstab}
Consider an exponential family Langevin dynamics (EFLD) algorithm of the form~\eqref{eq:efld1}-\eqref{eq:efld2} with a $c_2$-smooth log-partition function $\psi$.  Then, for mini-batch size $b \leq n/2$, with $c = c_0 \sqrt{5 c_2}$ (with $c_0$ as in Proposition~\ref{prop:hell}) and $\alpha_{t|}^2 \geq 8 c_2 \Delta_{t|}^2(\bar{S}_{n+1})$ (as in Theorem~\ref{theo:efld}, with the conditioning on $\w_{t-1}$ hidden to avoid clutter), we have
\vspace*{-2mm}
\begin{equation}
\hspace*{-5mm}
% | \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq  c \frac{b}{n} ~\underset{S_{n+1}}{\E} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \frac{1}{\alpha_{t|}^2} \underset{S_{B_t}, S'_{B_t} \in G_1}{\E} \left[\left\|\nabla \ell\left(\w_{t-1}, B_t\right)  -  \nabla \ell\left(\w_{t-1}, B'_t\right)\right\|_{2}^{2}\right] }~.
| \E_{S}[L_D(A(S)) - L_S(A(S))] | \leq  \frac{c}{n} ~\underset{\bar{S}_{n+1}}{\E} \sqrt{ \sum_{t=1}^T  \underset{W_{0:(t-1)}}{\E} \left[ \frac{1}{\alpha_{t|}^2}  \left[\left\|\nabla \ell\left(\w_{t-1}, {z_n} \right)  -  \nabla \ell\left(\w_{t-1}, {z'_n}\right)\right\|_{2}^{2}\right] \right] }~.
\end{equation}
\label{theo:efldstab}
\vspace*{-5mm}
\end{restatable}
%\yzcomment{Deleted $\underset{{B_t} \in G_1}{\E}$ in the bound.  We don’t need this.}

\begin{remark}
Theorem~\ref{theo:efldstab} establishes generalization bounds for {\em all} exponential family Langevin dynamics algorithms. The key term in the bound is the expected gradient discrepancy only on the sample $z_n, z'_n$ where $S_n,S'_n$ differ. Further, the only dependence on the specific exponential family is through the constant $c_2$, the smoothness of the corresponding log-partition function.  \qed 
\end{remark}


\begin{remark}
Since SGLD is a special case of EFLD, Theorem \ref{theo:efldstab} gives a generalization bound for SGLD.
% Theorem \ref{theo:efldstab} shows that 
% the expected generalization error of EFLD  scales as $O(\sqrt{\sum_{t=1}^T \frac{1}{\alpha_t^2}}/n)$. With the special case $\alpha_t = \sigma_t/\eta_t$, EFLD reduces to SGLD and  Theorem \ref{theo:efldstab} captures the generalization error of SGLD, i.e., $O(\sqrt{\sum_{t=1}^T \frac{\eta_t^2}{\sigma_t^2}}/n)$ 
The bound has effectively the same dependence on $n$ and $T$ as the bound in \cite{Li2020On}. 
However, the bound is quantitatively much sharper since the \emph{gradient norm} term $\frac{1}{n}\sum_{z \in S}\| \nabla \ell(\w_t,z)\|^2$ in \cite{Li2020On} gets replaced by the {\em gradient discrepancy} term $\|\nabla \ell(\w_t,z) - \nabla \ell(\w_t, z^\prime) \|^2$. As illustrated in our experiments (Section~\ref{sec:exp}), the gradient discrepancy is orders of magnitude smaller than the gradient norm.
%which is quantitatively smaller than gradient norms as we show in the experiment section. 
The bound in \cite{negrea2019information} depends on a related \emph{gradient incoherence} which we found to be empirically smaller than gradient discrepancy in our experiments (Section~\ref{sec:exp}). However, their bound has a ${1}/{\sqrt{n}}$ sample dependence, which is worse than the ${1}/{n}$ dependence in our bound. \qed
\end{remark}




\begin{remark}
EFLD can be extended to work with anisotropic noise by using $\btheta_{B_t,\aalpha_t} = \nabla \ell(\w_{t-1},S_{B_t}) \oslash \aalpha_t$ in \eqref{eq:efld2} where $\aalpha_t \in \R^p$ determines different scaling for each dimension and $\oslash$ denotes Hadamard division. Theorems~\ref{theo:efld} and \ref{theo:efldstab} can be extended to such anisotropic noise by using $\aalpha$-scaled norms for the gradient discrepancy, i.e., $\| \g - \g'\|_{2,\aalpha}^2 = \sum_j (g_j - g'_j)^2/\alpha_j^2$. \qed 
\end{remark}


\begin{remark}
The lower bound on $\alpha_t$ in Theorem~\ref{theo:efldstab} is a data-dependent quantity $\Delta_{t|}(\bar{S}_{n+1})$ which can be computed during training. From Example~\ref{exam:sgld}, since $\alpha_t = \sigma_t/\eta_t$, the lower bound $\alpha_t \geq c_3 \Delta_{t|}(\bar{S}_{n+1})$ for a constant $c_3$ implies an upper bound on the step size: $\eta_t \leq \sigma_t/c_3 \Delta_{t|}(\bar{S}_{n+1})$. The upper bound is a much more benign (and computable) condition on the step size compared to those in the related work~\cite{mou2018generalization,Li2020On,hardt2016train} (Mou et al., 2018; Li et al., 2020, Hardt et al. 2016) which require step size being bounded by ${\sigma_{t}}/{K}$, where $K$ is the global Lipschitz constant for the loss $\ell$. Note that $\Delta_{t|}(\bar{S}_{n+1}) \ll K$ because global Lipschitz constant $K$ is a uniform bound on the entire space, and $\Delta_{t|}(\bar{S}_{n+1})$ is computable data-dependent measure based on gradient discrepancy. Further, $\Delta_{t|}(\bar{S}_{n+1})$ is expected to decrease over iterations, i.e., as $t$ increases, and gradients get smaller. \qed
% However, the step sizes in Theorem \ref{theo:efldstab} need to be bounded by ${\sigma_{t}}/{\Delta_{t}(\bar{S})}$, which is considerably more relaxed since $\Delta_{t}(\bar{S})$ is much smaller than Lipschitz constant $L$, which is a uniform bound over the whole parameter space. 
% %Also Hardt et al. (2016) requires $1/t$ step sizes.
% Also, usually one would expect $\Delta_{t}(\bar{S})$ to decrease as training proceeds since the gradients shrink as the loss function being minimized. Thus, the constraint on step size does not require the step sizes to be as small as $\sigma_t/L$.  \qed 
 \end{remark}




\subsection{Proof Sketches of Main Results: Theorems~\ref{theo:efld} and \ref{theo:efldstab}}
\vspace*{-2mm} 
We focus on Theorem~\ref{theo:efld}. To avoid clutter, we drop the subscript $t$ for the analysis and note that the analysis holds for any step $t$.  When the densities $dP_{B,\bxi} = p_{\psi}(\bxi;\btheta_{B,\alpha})$ and $dP'_{B,\bxi} = p_{\psi}(\bxi;\btheta'_{B,\alpha})$, i.e., densities in the same exponential family but with different parameters 
$\btheta_{B,\alpha}$ and $\btheta'_{B,\alpha}$ because of the difference in the mini-batches,
by mean-value theorem, for each $\bxi$, we have 
\begin{equation}
p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta'_{B,\alpha}) 
= \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle~,
\end{equation}
for some $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$ where $\gamma_{\bxi} \in [0,1]$ with the subscript $\bxi$ illustrating dependence on $\bxi$. Then,
{\small
\begin{align}
I_{A,B} &=  \bigintsss_\bxi \frac{\big( p_{\psi}(\bxi; \btheta_{B,\alpha}) - p_{\psi}(\bxi; \btheta'_{B,\alpha}) \big)^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber 
 = \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})\rangle ^2}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi \nonumber \\
& = \bigintsss_\bxi \frac{\langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla_{\tilde{\btheta}_{B,\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2~p_{\psi}^2(\bxi;\tilde{\btheta}_{B,\alpha})}{p_{\psi}(\bxi; \btheta_{A,\alpha})} d\bxi ~,
\label{eq:expcore1}
\end{align}}
where since $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) = \exp(\langle \bxi, \tilde{\btheta}_{B,\alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha})) \pi_0(\bxi)$ we have 
\begin{align*}
\nabla_{\tilde{\btheta}_{B,\alpha}} p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) = (\bxi - \nabla_{\tilde{\btheta}_{B,\alpha}} \psi(\bxi;\tilde{\btheta}_{B,\alpha}) ) p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})~.
\end{align*}


\noindent {\bf Handling Distributional Dependence of $\tilde{\btheta}_{B,\alpha}$.}
Note that it is difficult to proceed with the analysis with the density term depending on parameter $\tilde{\btheta}_{B,\alpha}$ since $\tilde{\btheta}_{B,\alpha}$ depends on $\bxi$ and there is an outside integral over $\bxi$ in \eqref{eq:expcore1}. So, we first bound the density term depending on $\tilde{\btheta}_{B,\alpha}$ in terms of exponential family densities with parameters $\btheta_{B,\alpha}$ and $\btheta'_{B,\alpha}$ essentially using $c_2$-smoothness of $\psi$.
\begin{restatable}{lemm}{exptilde}
With $\tilde{\btheta}_{B,\alpha} = \gamma_{\bxi} \btheta_{B,\alpha} + (1-\gamma_{\bxi}) \btheta'_{B,\alpha}$ for some $\gamma_{\bxi} \in [0,1]$, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, \tilde{\btheta}_{B, \alpha} \rangle - \psi(\tilde{\btheta}_{B,\alpha}) \right]}{ \max\left( \exp\big[\langle \bxi, \btheta_{B,\alpha} \rangle - \psi(\btheta_{B,\alpha}) \big] , \exp\left[\langle \bxi, \btheta'_{B, \alpha} \rangle - \psi(\btheta'_{B,\alpha}) \right]\right) }
\leq \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta'_{B,\alpha} \|_2^2 \right] ~.
\end{align*}
\vspace*{-3mm}
\label{lemm:exp_step2}
\end{restatable}

In other words, for any $\bxi$ we have
\begin{align*}
p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha}) \leq \exp\left[ c_2 \| \btheta_{B,\alpha} - \btheta'_{B,\alpha} \|_2^2 \right] \max \left( p_{\psi}(\bxi;\btheta_{B,\alpha}), p_{\psi}(\bxi;\btheta'_{B,\alpha}) \right)~.
\end{align*}
Since the parameters $\btheta_{B,\alpha}, \btheta'_{B,\alpha}$ in the right-hand-side depend on $\bxi$, the outside integral over $\bxi$ in \eqref{eq:expcore1} will not pose any unusual challenges.

\noindent {\bf Bounding the Density Ratio.} Next we focus on the density ratio $p^2_{\psi}(\bxi,\tilde{\btheta}_{B,\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$ in \eqref{eq:expcore1}. By Lemma~\ref{lemm:exp_step2}, it suffices to focus on $p^2_{\psi}(\bxi,\btheta_{B,\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$ or the equivalent term for $\btheta'_{B,\alpha}$. We show that the density ratio can be bounded by another distribution in the same exponential family $p_{\psi}$ with parameters $(2\btheta_{B,\alpha} - \btheta_{A,\alpha})$.
\begin{restatable}{lemm}{expdr}
\vspace*{-3mm}
For any $\bxi$, we have 
\begin{align*}
\frac{\exp\left[\langle \bxi, 2\btheta_{B, \alpha} \rangle - 2\psi(\btheta_{B,\alpha}) \right] }{\exp\left[\langle \bxi, \btheta_{A,\alpha} \rangle - \psi(\btheta_{A,\alpha}) \right]}
\leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] \exp \left[  \langle \bxi, (2\btheta_{B,\alpha} - \btheta_{A,\alpha} \rangle - \psi( 2\btheta_{B,\alpha} - \btheta_{A,\alpha} )\right].
\end{align*}
\label{lemm:exp_step3}
\vspace*{-4mm}
\end{restatable}
In other words, for any $\bxi$ we have
\begin{align*}
 \frac{p^2_{\psi}(\bxi,\btheta_{B,\alpha})}{p_{\psi}(\bxi;\btheta_{A,\alpha})} \leq \exp \left[ 2c_2 \| \btheta_{B,\alpha} - \btheta_{A,\alpha} \|_2^2 \right] p_{\psi}(\bxi; 2\btheta_{B,\alpha} - \btheta_{A,\alpha})~.
\end{align*}
The analysis for the term $p^2_{\psi}(\bxi,\btheta'_{B,\alpha})/p_{\psi}(\bxi;\btheta_{A,\alpha})$ is exactly the same. 

\noindent {\bf Bounding the Integral.} Ignoring multiplicative terms which do not depend on $\bxi$ for the moment, the analysis needs to bound an integral term of the form
\begin{equation*}
\bigintsss_\bxi \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle ^2 ~p_{\psi}(\bxi;2 \btheta_{B,\alpha} - \btheta_{A,\alpha}) d\bxi~,
\end{equation*}
and a similar term with $p_{\psi}(\bxi;2 \btheta'_{B,\alpha} - \btheta_{A,\alpha})$. First, note that  $\nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) = \tilde{\m}_{B,\alpha}$, the expectation parameter for $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})$~\citep{wainwright2008graphical,banerjee2005clustering}. The integral, however, is with respect to $p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})$, not $p_{\psi}(\bxi;\tilde{\btheta}_{B,\alpha})$. We handle this discrepancy by using
\begin{align*}
& \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \nabla \psi(\bxi;\tilde{\btheta}_{B,\alpha}) \rangle^2 
= \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, (\bxi - \E[\bxi]) + (\E[\bxi] - \nabla \psi (\bxi; \tilde{\btheta}_{B,\alpha})) \rangle^2 \\
& \leq 2 \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \bxi - \E[\bxi] \rangle^2 + 2 \langle \btheta_{B,\alpha} -\btheta'_{B,\alpha}, \E[\bxi] - \nabla \psi (\bxi; \tilde{\btheta}_{B,\alpha}) \rangle^2~,
\end{align*}
where the expectation $\E[\bxi]$ is with respect to $p_{\psi}(\bxi;2\btheta_{B,\alpha}-\btheta_{A,\alpha})$.
Quadratic form for the first term yields the covariance $\E[(\bxi- \E[\bxi])(\bxi - \E[\bxi])^T] = \nabla^2 \psi(\btheta_{2\btheta_{B,\alpha} - \btheta_{A,\alpha}}) \leq c_2 \I$, by smoothness and since the covariance matrix of an exponential family is the Hessian of the log-partition function~\citep{wainwright2008graphical}. Since $\E[\bxi] = \nabla \psi ( 2\btheta_{B,\alpha} - \btheta_{A,\alpha})$, the second term depends on the difference of gradients $\nabla \psi ( 2\btheta_{B,\alpha} - \btheta_{A,\alpha}) - \nabla \psi(\tilde{\btheta}_{B,\alpha})$ which, using smoothness and additional analysis, can be bounded by the norm of $(\btheta_{B,\alpha} - \btheta_{A,\alpha})$. All the pieces can be put together to get the bound in Theorem~\ref{theo:efld}, which when used in Lemma~\ref{theo:stab}
yields Theorem~\ref{theo:efldstab}.







